Convex Sparse Blind Deconvolution

In the blind deconvolution problem, we observe the convolution of an unknown filter and unknown signal and attempt to reconstruct the filter and signal. The problem seems impossible in general, since there are seemingly many more unknowns than knowns . Nevertheless, this problem arises in many application fields; and empirically, some of these fields have had success using heuristic methods -- even economically very important ones, in wireless communications and oil exploration. Today's fashionable heuristic formulations pose non-convex optimization problems which are then attacked heuristically as well. The fact that blind deconvolution can be solved under some repeatable and naturally-occurring circumstances poses a theoretical puzzle. To bridge the gulf between reported successes and theory's limited understanding, we exhibit a convex optimization problem that -- assuming signal sparsity -- can convert a crude approximation to the true filter into a high-accuracy recovery of the true filter. Our proposed formulation is based on L1 minimization of inverse filter outputs. We give sharp guarantees on performance of the minimizer assuming sparsity of signal, showing that our proposal precisely recovers the true inverse filter, up to shift and rescaling. There is a sparsity/initial accuracy tradeoff: the less accurate the initial approximation, the greater we rely on sparsity to enable exact recovery. To our knowledge this is the first reported tradeoff of this kind. We consider it surprising that this tradeoff is independent of dimension. We also develop finite-$N$ guarantees, for highly accurate reconstruction under $N\geq O(k \log(k) )$ with high probability. We further show stable approximation when the true inverse filter is infinitely long and extend our guarantees to the case where the observations are contaminated by stochastic or adversarial noise.

==> Backup_After_Dave_Editting/Inroduction_backup20210522.tex <==
\section{Introduction}
\subsection{Blind Deconvolution}
Suppose we are interested in an underlying time series $\bx = (x(t))$ which we cannot observe directly. What we can observe is  $\by = \ba * \bx$ where $\ba$ is an unknown `blurring' filter. Blind deconvolution is the problem of recovering $\bx$ merely from the observed $\by$ without knowing either $\ba$ or $\bx$. 

This problem occurs naturally in seismology and
digital communications
as well as astronomy, satellite imaging, and computer vision.

In its most ambitious form, the problem is literally impossible; there are simply too few data and too many unknowns. Indeed, imagine that $\bx$, $\by$ and $\ba$ all have $N$ entries; we observe only $N$ pieces of information ($\by$) but there are $2N$ unknowns ($\bx$ and $\ba$). 
Nevertheless, in \sout{various} \redit{some (not all)} fields, heuristic \redit{approaches}
\sout{methods showed occasional} \redit{have occasionally 
led to consistent } success \redit{in isolated applications};
\redit{presumably such success stories exploit} \sout{under various} specialized assumptions \redit{-- although not always in
an explicit or recognized way, and not with rigorous understanding}.

\redit{This paper, in contrast,  will exhibit a set of 
assumptions enabling practical algorithms for blind deconvolution,
backed by rigorous theoretical analysis}.

\subsection{The Promise of Sparsity}

\redit{Central to our approach
is an assumption about the}
{\it sparsity of the signal $\bx$ to be recovered}, 
in which case the problem \sout{becomes}
\redit{can be called} \emph{sparse blind deconvolution}. Sparse signals\sout{,} \redit{-- i.e. signals} having relatively few nonzero entries, arise frequently in many fields, including seismology, microscopy, astronomy, neuroscience spike identification. Even in more abstract settings such as representation learning for computer vision, 
it surfaces in recently popular research trends, 
such as single-channel convolutional dictionary learning   \cite{bristow2013fast, heide2015fast,zhang2017global,zhang2018structured}. 

The sparsity of $\bx$ \-- if it holds \-- would constrain the recovery problem significantly; and so possibly, sparsity can play a role
in enabling useful solutions to an otherwise hopeless problem.

An inspiring precedent can be found in modern commercial medical imaging, 
where sparsity of an image's wavelet coefficients enables 
MRIs from fewer observations than unknowns.
Taking fewer observations speeds up data collection,
a principle known as compressed sensing, which
already benefits tens of millions of patients yearly.

\subsection{Translating Heuristics into Effective Algorithms}

For sparsity to reliably enable blind deconvolution, there are two
apparent hurdles. First, develop an objective function which promotes
sparsity of the solution. Second, develop an algorithm 
which can reliably optimize the objective.

Many sparsity-promoting objectives have 
been proposed over the years; typically they 
imply non-convex optimization problems. Indeed
sparsity is quantified by the $\ell_0$
pseudo norm $\|\bx\|_0 = \#\{t: x(t) \neq 0\}$, which is the limit of
$\| \bx \|_p^p$ as $p \goto 0$
of concave $\ell_p$ pseudo-norms where $p <1$.

Traditionally, non-convex problems have been viewed
by mathematical scientists with skepticism;
for such problems, gradient descent and its various refinements
lack any guarantee of effectiveness. 
Still, the lack of guarantees has not stopped engineers from trying!

A noticeable success in blind signal processing
was scored in digital communications,
where blind equalization today 
benefits billions of smartphone users.
Blind equalization is a form of blind deconvolution 
where one exploits the known discrete-valued 
nature of the signal $\bx$ (for example the signal 
entries might take only two values $\{-1,1\}$).
Practitioners found that if an initial guess of 
the equalizer (i.e. our inverse filter $\ba^{-1}$) is `fairly good' 
(in engineer-speak `opening the eye' so that a `hint' 
of the `digital constellation` becomes
`visible'), then certain `discreteness-promoting' on-line gradient methods
can reliably `focus' the result better and better 
and allow reliable recovery.

Our work identifies an 
analogous phenomenon in the sparsity-promoting blind deconvolution
setting, however it exposes and crystallizes the phenomenon in a rigorous 
and dependably exploitable form.

Namely, we show that if sparsity of $\bx$ holds,
and if an initial guess of the filter $\ba$
is `fairly good' in a precise sense, 
then a specific convex optimization
algorithm will accurately recover 
both the filter and the original signal\footnote{As we explain below, recover means: recover up to rescaling and time shift.}.

In retrospect, our insights on sparsity-promoting blind deconvolution
can be cross-applied to explain the major successes of discreteness-promoting
blind equalization in modern digital communications.
Namely, a direct variation of our arguments 
provide a related convex optimization problem 
for discrete-valued signals which rigorously converts a 
a rough initial approximation into precise recovery.

In our view these new arguments clear away some persistent
fog, mystery and misunderstandings in blind signal processing; and pave
the way for future success stories.

%This work demonstrates that a convex formulation hiding behind the scene can explain the success of this poetic heuristic. Our mathematical formulation gives a crisp, clean view that clears all the fog in the claims of past practitioners. 

\subsection{Prior Work}
\begin{comment}
\paragraph{Non-convexity for blind deconvolution problems}
As both the sparse signal and the forward filter $\ba$ are unknown, the problem is bilinear in $\ba$ and $X$. And the expression $\ba*\bx$ has scaling and shift symmetry for $(\ba,\bx)$.
Therefore, blind deconvolution is often formulated as a non-convex problem. Lots of previous works \cite{kuo2019geometry, kuo2020geometry, lau2019short} studied the that problem of recovering short $a$ and sparse $x$ as an non-convex optimization problem.

\Dave{The previous paragraph is jumbled and also out of order. If it has any value or content it should come later.}
\end{comment}

\paragraph{Searching for an inverse filter that promotes desired output properties}
Instead of trying to recover $\ba$ and $\bx$ together from $\ba*\bx$, 
we could formulate this problem as looking for an approximate inverse  filter $\bw$ so that the output $\bw*\by$ exhibits \sout{desired} \redit{extremal} properties. 
\sout{Namely} \redit{Under this formulation, 
our goal is to find} $\bw\neq 0$, so that  
\begin{equation}
 \begin{array}{ll}
 \underset{\bw\neq 0}{\mbox{optimize}}   & J(\bw \star \by) \label{JoptBD}
\end{array}
\end{equation}
where the functional $J$ quantifies the properties we seek to promote.
(Depending on $J$, we might \redit{either prefer its maximum or minimum} \sout{it}).
 
 \newcommand{\bz}{{\bf z}}
\sout{Motivated by blind deconvolution} \redit{Working} in
exploration seismology, 
Wiggins \cite{wiggins1978minimum} adopted this approach
with the normalized $4$-norm, $J(\bz) = J_{4,2} = {\|\bz\|_4}/{\|\bz\|_2}$
and gave a few successful data-processing case studies. 
His \redit{successful} examples all
clearly exhibit sparsity, although this was not discussed at the time.
Other objectives 
considered at that time included $J_{2,1}(\bz) = \|\bz\|_2/\|\bz\|_1$
and $J_{\infty,2}(\bz) = \|\bz\|_\infty/\|\bz\|_2$ \cite{cabrelli1985minimum}.

It was fully understood at that time
that output property optimization could succeed in principle,
if one did not have to worry about an effective algorithm.
\cite{donoho1981minimum} showed that 
if the signal $\bx$ is a realization of
independent and identically distributed
entries from any nonGaussian distribution,  optimizing
$J$ of the output $\bw \star \by$ is successful in the large-$N$ setting \-- as long as the \redit{functional} \sout{property} $J$ belongs to a \redit{certain} large family of non-Gaussianity measures,
for example including $J_{4,2}$ and $J_{2,1}$ as well as many others. 
\footnote{Sparsity is of course a form of non-Gaussianity,
this very explicitly in the Bernoulli-Gaussian mixture model considered below.}

The issue left unresolved in those days was how to solve such
optimization problems. Indeed optimizations like $J_{4,2}$ are badly nonconvex,
as we see clearly by rewriting the $J_{4,2}$ problem as
\[
 \begin{array}{ll}
 \underset{\bw}{\mbox{maximize}}   &  
 \|\bw * \by\|_4 
 \\
\mbox{subject to} 
& \|\bw* \by\|_2 = 1.
\end{array}
  \]
The theory cited above derived favorable properties of a would-be procedure which truly finds the optimum of a badly nonconvex objective. It clarifies that  blind deconvolution is possible in principle but does not by itself help us algorithmically, i.e. in practice. In the intellectual climate of the time, solving badly nonconvex optimization problems was considered a pipe dream, a time-wasting charade for non-serious people.

Even \sout{up to} today, blind deconvolution 
continues to be studied as an non-convex optimization problem;
see recent work
\cite{kuo2019geometry, kuo2020geometry, lau2019short}, who study the \sout{that} problem of recovering short $a$ and sparse $x$ 
  
  \paragraph{Blind equalization}
  In digital communications, 
  the transmitted signal $\bx$ can be viewed as 
  \redit{discrete-alphabet valued;}
  for example, in PAM signaling, where $x(t) \in \{\pm 1\}$, and QAM signaling, where the signal \redit{alphabet} has equally spaced points on unit sphere in complex space \cite{kennedy1992blind,ding2000fast}.  
  
  \cite{vembu1994convex} considered the non-convex problem
   \[
 \begin{array}{ll}
 \underset{\bw}{\mbox{maximize}}   &  
 \|\bw * \by\|_8 
 \\
\mbox{subject to} 
& \|\bw* \by\|_2 = 1
\end{array}
  \]
If the data $\by$ were preprocessed to be serially uncorrelated,
this optimization is effectively of the earlier form $J_{8,2}$.

The authors attack this nonconvex problem
using projected gradient descent and give suggestive 
experimental results. They apparently view the $\ell_8$ norm objective as an approximation of the  $\ell_\infty$ norm objective $\|\bw * \by\|_\infty $.
Later, \cite{ding2000fast} used linear programming to solve the $\infty$ norm problem directly.

% \Dave{Are you really sure they wanted to maximize the 8 norm? I would have said that in digital com where the signal is not sparse but binary they should want to minimize.}
% \Sun{They want to maximize the $\infty$ norm, and as it is not simple to compute $\infty$ norm, they use $8$ norm as a replacement.}

\begin{comment}

\paragraph{Sparse projection pursuit and dictionary learning}
Sparse projection pursuit is the problem of finding  a sparse projection $d^T Y$ time from a high dimensional data matrix $Y\in \reals^{n\times M}$. Here $Y= D X$ is a matrix product of dictionary $D\in \reals^{n\times d}$ and sparse coefficient $X\in \reals^{d\times M}$. 

\Dave{I can't follow either what you are trying to do in the paragraph below
or what you are trying to say. You mention many different things, with no references definitions or discussion and all very telegraphically.  Why is it even here? What does it add? I don't see it.}

\Dave{In general it's really a huge mistake to put 
inconclusive aimless material at the beginning of a document.
Readers very quickly abandon reading and decide that you're at least confusing
and possibly confused.

In your writing you don't want to put in a lot of extraneous references that 
only distract from your central thread.
}
The projection pursuit problem was first studied by Friedman and collaborators in a series of important works \cite{friedman1974projection}, \cite{friedman1981projection} and \cite{friedman1987exploratory} as a tool for exploratory high dimensional data analysis. Then several statisticians like Huber \cite{huber1985projection}  and Jones \cite{jones1987projection}  also studied this problem. 

The projection pursuit problem is also related to blind source separation, independent component analysis (ICA) and the cocktail-party problem.
In the case of an orthogonal dictionary $D$, we could simply transform the problem into finding its inverse $D^{-1} = D^T$, such that $D^T Y = X$ sparse. A work by Daniel Spielman and John Wright\cite{spielman2012exact} used sparse projection pursuit formulation to find the orthogonal basis of $D$ one-by-one, by proposing a set of rule to select the initial guess $v$ and give theoretical guarantee of the convex method. In this work, due to this common population problem, the phase transition phenomenon would also be applicable to dictionary learning, as the first phase transition result for dictionary learning.

The sparse projection pursuit formulation is to solve the following linear-constrained convex optimization problem for some vector $u$:
\[
 \begin{array}{ll}
 \underset{q }{\mbox{minimize}}   & \frac{1}{M}\|q^T Y\|_{1}\\
\mbox{subject to}  & u^T q =1.
\end{array}
  \]
  This convex problem is also used in \cite{spielman2012exact} to solve sparse dictionary learning problem.
  
%   \Dave{Why don't you call $q$ simply $w$, to make it easier on readers.
% }
\end{comment}

%   \Dave{Here is my attempt to reformulate your text above.}
 
 \paragraph{Searching for a projection with desired output properties} 
Here is another setting for property-promoting
output optimization.
We have a data matrix $Y \in \bR^{n,p}$ \-- which we think of as
$n$ points in $\bR^p$,
and we have a unit vector $w \in \bR^p$
called the projection direction.  Our
output vector $Y\cdot w$ contains the 
projection of the $n$-points on the projection
direction q; it has $n$ entries.
We seek `interesting' projections; i.e. directions where the 
projection displays some structure. We
adopt a functional $J$ which measures properties we seek to promote
in the output, and we seek to solve:
\begin{equation}
 \begin{array}{ll}
 \underset{\|w\|=1}{\mbox{optimize}}   & J(Y \cdot w). \label{JoptPP}
\end{array}
\end{equation}

This was implemented by  [Friedman and Tukey, 1974], who proposed a
functional that promotes `clumping' or 'clustering' of the output.
They called it {\it projection pursuit} and
were motivated by exploratory  high  dimensional  data  analysis;
for $p$-dimensional data involve $p>2$ and we can't 
easily get a visual sense of what's in the data. 
It was hoped at the time that looking at selected
low-dimensional projections might lead to better insights.
For the most part, such hopes for exploration of high-dimensional data
never materialized.

However, output optimization of this type has proven to be
useful in important problems in blind signal processing,
where $Y$ has known structure that can be exploited systematically.

In {\it blind source separation}
we observe $Y = XA$, $Y \in \bR^{n,p}$, $X \in \bR^{n,p}$ and
$A \in \bR^{p,p}$ is an invertible matrix. 
(We don't observe $X$ or $A$ separately).

Think of the $X$ matrix as containing columns giving
successive time samples of $p$ clean source signals, for example $p$
individual acoustic signals. These signals arrive
at array of $p$ spatially distributed acoustic sensors, each
of which records the acoustic information it receives.
The matrix $Y$ contains in its
columns what was obtained by each of the $p$ different sensors.
In general, each sensor receives information from each of the sources.
This is colorfully called the {\it cocktail party problem}, referring to
the setting where $X$ records the sources are human speakers at a cocktail party,
and $Y$ records what is heard at various locations in a room.
Each column of $Y$ then contains a
superposition of different speakers; while
we would prefer to separate these and pay attention to 
just the ones of most immediate interest to us.

In this separation problem, sparsity of the signal might be valuable.
Suppose that each individual speaker is listening quite a bit
and so not speaking much of the time. Then the columns of $X$
are each sparse. On the other hand, if there are many people
in the room, the room
as a whole may still always be noisy, and so each
column of $Y$ may be fully dense.
Assuming $A$ is invertible, and the vector $w$
obeys $Aw= e_j$, then $Y \cdot w$ extracts column $j$ of $X$,
which will be sparse. Hence, we may hope that the projection
pursuit principle, with an appropriate measure $J$, might
identify the `sparse' projections we seek.  

Ju Sun, Qu Qing, Yu Bai, John Wright, Zibulevsky and Pearlmutter \cite{sun2015complete,sun2016complete,bai2018subgradient,zibulevsky2000blind} proposed the optimization
problem
 \[
 \begin{array}{ll}
 \underset{w }{\mbox{minimize}}   & \cancel{\frac{1}{n}}\| Y w\|_{1}\\
\mbox{subject to}  & \|w\|_2 =1.
\end{array}
  \]
Assuming the $Y$ data pre-processed so that $\frac{1}{n} Y'Y=I_p$ 
this is equivalent to projection pursuit (\ref{JoptPP}) 
applied to the objective $J_{2,1}$. Notably, this is 
again a highly non-convex optimization problem..
The authors proposed projected gradient descent
and recited some favorable empirical results.
 
There is a close relation between the
 blind deconvolution optimization (\ref{JoptBD}) 
 and the projection pursuit optimization (\ref{JoptPP}). Indeed, if the $Y$ matrix 
 is filled in from an observed time series appropriately, then 
 output optimization in \sout{the} 
 blind deconvolution and in projection pursuit are
 essentially identical. Namely, let $\by^{ser} = (y^{ser}(t))_{t=1}^N$ denote a time series of interest to us,
 and  $Y^{mat} = (Y^{mat}_{i,j})$ 
 denote an $n \times p$ matrix where $n = N-p$ constructed 
 using $\by^{ser}$ like so:
 \[
  Y^{mat}_{i,j} = y^{ser}(p+i-(j-1)) , \qquad 1 \leq i \leq n = N-p; \; 1 \leq j \leq p.
  \]
  Now suppose the filter vector 
  $\bw$ in the blind deconvolution optimization 
  and the projection direction $w$ in the projection pursuit optimization
  are chosen identically. Then the blind deconvolution output objective 
  $J(\bw \star \by^{ser})$ is identical to the projection pursuit objective
  $J(Y^{mat} w)$, except for
  possibly different treatment of the first $p$ entries of $\by^{ser}$.
 
 \paragraph{Convex Projection Pursuit}
 
 In view of the connection between blind deconvolution and
 projection pursuit, and in view of our results in this paper,
 it is quite interesting to consider the
 work of \cite{spielman2012exact} and \cite{gottlieb2010matrix}.
\begin{comment}
They call their problem sparsity-promoting projection pursuit,
 but they depart from the PP optimization framework (\ref{JoptPP}).
 \Sun{Their paper did not mention the name "projection pursuit", so I comment out this sentence.}
\end{comment}
They propose to solve the following 
linear-constrained convex optimization problem.
Given an $n \times p$ 
data matrix $Y$ and a constraint vector $u$,
they propose to solve:
\[
 \begin{array}{ll}
 \underset{w }{\mbox{minimize}}   & \cancel{\frac{1}{n}}\|Y w\|_{1}\\
\mbox{subject to}  & u^T w =1.
\end{array}
  \]
As it turns out, \redit{when the matrix $Y$ in this problem and
$\by$ in the time series deconvolution problem
are related by the} \sout{under the same} $Y^{mat}$-$\by^{ser}$
construction just mentioned, the objective we propose in this paper
is essentially identical, when $\tilde{\ba} = u$. \sout{However} \redit{As we will show},
our setting permits much more thorough studies and more penetrating analyses, \redit{and we find that success in 
sparse blind deconvolution is more
broadly prevalent than one might have expected, based on
earlier analyses such as \cite{spielman2012exact}
or \cite{sun2015complete,sun2016complete,bai2018subgradient,zibulevsky2000blind} }.


% \Sun{Thanks so much for the section, I learned a lot from your writting! About this part: "They call their problem sparsity-promoting projection pursuit,
%  but they depart from the PP optimization framework". From what I learned by talking to one of the author, Ju Sun, they first studied the convex projection pursuit problem and call it sparse dictionary learning. But they found the sparsity level need to be of order $O(\frac{1}{\sqrt{n}})$, which from our phase transition result, is now much better understood. Later in John Wright's research group, their motivation to study the $2$-norm constrained non-convex problem is to get a constant order sparsity level. So  in the time order, they study the convex problem first, and study the non-convex problem after they hit a bottleneck on sparsity level. And they call this problem "dictionary learning" more often than "projection pursuit".
 
%  They proved that this non-convex function have good landscape on sphere (for us, this function is $V_1$). However, for the non-convex method, their sample complexity from proof is much higher than the convex formulation, as the concentration of Hessian is required.  }


\subsection{Mathematical setup}
\paragraph{Sequence Space, and Filtering }
To make our results concrete, let's discuss things formally.
Let $\bX$ denote the collection of {\it bilaterally infinite sequences}
$\bx = (x(t): t = 0, \pm 1, \pm 2, \dots)$; for short
we call such objects {\it bisequences}. Then $\ell_1(\integers) \subset \bX$
denotes the collection of bisequences 
obeying $\| \bx \|_1 = \sum_t |x(t)| < \infty.$
For a bisequence $\bx$ we denote time reversal operator
$t \leftrightarrow -t$ by $\bx^{\dagger}$.
For whole number $k > 0$ let $\bX_k$ denote the subspace
of bisequences supported in $-k \leq t \leq k$. We sometimes
abuse notation: for a bisequence $\bx$ we might write
$\bx = (1, .3)$ when we really mean $\bx = (\ldots,0,0,1,.3,0,0,\ldots)$.

Let $\star$ denote the convolution 
product on pairs of bisequences in $\ell_1(\integers)$
\-- $( \bx \star \by ) = \sum_u x(t-u)y(u)$. 
Let $\be_0$ denote the  `delta'
or `Kronecker' bisequence: $\be_0(t) = 1_{\{t=0\}}$;
$\be_0$ is the unit of convolution. The convolution inverse
of $\bx$ $\--$ $\bx^{-1}$ $\--$ is a bisequence
obeying $ \bx \star \bx^{-1}  = \be_0$. For example,
the filter $\bx = (\dots,0,1,1/2,1/4,1/8,\ldots)$ 
anchored at the time origin so $\bx(0)=1$, has inverse
$\bx^{-1} = (\dots,0,1,-1/2,0,\dots)$, again anchored at the time origin.
Abusing notation we may simply write $\bx^{-1} = (1,-1/2)$.


Our approach to blind deconvolution searches 
among candidates for a filter ($\equiv$ bisequence) that extremizes a certain objective function. We then
show that the extremal is in fact the desired inverse filter
to our (unknown) true underlying filter. Hence, it helps know
conditions under which an inverse filter actually exists! 

For a bisequence $\bx \in \ell_1(\integers)$,
we define the Fourier transform 
$\hat{\bx}(w) = \mathcal{F} \bx (w) \equiv \sum_t x(t) \exp\{ i 2\pi w t \}$.
For the inverse transform, we use
$ x(t) = (\mathcal{F}^{-1} \hat{\bx} ) (t) =  \frac{1}{2\pi} \int_0^{2\pi} \hat{\bx}(w) \exp\{ -i 2\pi w t \} dw$.


\begin{lemma}[Wiener's lemma]
If $\ba\in \ell_1(\integers)$, and also  
$(\mathcal{F} \ba)(\widetilde{w}) \neq 0$, $\forall \widetilde{w}\in T$,
then an inverse filter exists in $\ell_1(\integers)$. 
The bilaterally infinite sequence defined formally by
$$\ba^{-1} := \mathcal{F}^{-1}(\frac{1}{\mathcal{F} \ba})$$
exists as an element of $\ell_1(\integers)$
and obeys $\ba^{-1}*\ba = \be_0.$
\end{lemma}
In the engineering literature, we
say that the bisequence $\ba$ has so-called $Z$-transform 
$A(z)$, defined by:
\[
 \begin{array}{ll}
A(z) =  \sum_{t=-\infty}^{\infty} a_{t} z^{-t}.
\end{array}
  \]

Evaluating $A$ on the unit circle in the complex plane, at $z$ of the form $z=\exp\{ -i 2\pi w \}$, we see that  the 
$Z$-transform is effectively the Fourier transform $A = \cF \ba$. 
Applying Wiener's lemma, we see that, if 
$\ba \in \ell_1$ and $ \min_w |A(\exp\{ - 2\pi i w \}) | > 0$,
i.e. $A$ is never zero on the unit circle, then $\ba^{-1} \in \ell_1$ and $1/A$ is the $Z$-transform of $\ba^{-1}$.


% \Dave{Ideally should define the Z transform right here and make clear the realtion to the Fourier transform. ADDED.}
% \newcommand{\goto}{\rightarrow}
% \newcommand{\bw}{{\bf w}}
\paragraph{Finite-sample observation model and finite-length inverse filter }
In searching for an inverse filter, our \sout{early} initial  results assume
existence of a {\it finite-length} inverse. Namely, we assume that $\ba\in \ell_1(\integers)$ is a forward filter with an inverse filter $\ba^{-1} \in \ell_1(\integers)$ supported in a centered window of radius $k$.

In practice we only have a finite dataset! Suppose that 
there is an underlying bisequence $\by \in \bX$
of the form $\by = \ba* \bx$, and let $\by^{[N]}$ denote the
restriction to an $N$-long centered window 
$\cT = \{ -T,\dots, T\}$ of radius $T$ and size $N=2T+1$.

Our goal is seemingly to 
recover $\bx$ or $\ba$ from the observed data $\by^{[N]}$.
However, in statistical theory we generally 
don't expect to exactly recover the true underlying 
representation (i.e. the generating $\ba$ and $\bx$) exactly.
Our goal is instead to find an inverse filter 
$\bw \in \ell_1^k$ such that the convolution $\bw*\by$ 
would be close\footnote{modulo time shift and rescaling}  to $\bx$, and where the closeness improves with
increasing data size $N \goto \infty$.

\paragraph{Finite-length filtering and practical algorithms}

While our analysis framework concerns bisequences (bilaterally infinite sequences), our data have finite length (as just mentioned). The algorithms we discuss are often {\it motivated by} convolutions on bisequences; however, they reduce {\it in practice} to truncated convolutions involving finite data windows. A certain ambiguity is helpful for efficient communication. Suppose we have $\by^{[N]}$, an N-long observed window of $\by$, and we also have $\bw$, a k-long filter, by which we mean a bisequence nonzero only within a 
fixed $k$-long window. We might encounter discussion both of 
$\bw \star \by^{[N]} $ as well as
$\bw \star \by$, both using the same filter $\bw$. In the first case, we would actually be thinking of $\by^{[N]}$ as zero-padded out to a bisequence, so that both situations involve bisequence convolutions. 

Finite $N$ effects are important in practice but tedious to discuss. It can be important to account for {\it end effects} in truncated convolution. In a setting where we initially
think to consider a norm $\| \bw \star \by^{[N]} \|_{\ell_p(\integers)}$, we might instead next think to rather consider the windowed norm
$\| \bw \star \by^{[N]} \|_{\ell_p(\{-T,\dots,T\})}$,
while finally we realize $\| \bw \star \by^{[N]} \|_{\ell_p(\{-T+k,\dots,T-k\})}$ is more correct for our purposes, as it includes only the terms which do not suffer from truncation of the convolution.
%\textbf{Remark} Circular Embedding trick: for linear convolution $\ba}x$ on finite observation where $a,x \in \cT$ of length $N$, we could embed the linear convolution into a circular convolution on the extended space by zero padding both of them to a large enough space of length $2N$. 

%\Dave{This last comment is bizarre. Why would that ever be in an introduction.}

% \textbf{Remark}: we will study the case when inverse filter is an infinite length filter, and provide tight approximation theory for the guarantee of our algorithm.

\paragraph{Algorithmic formulation}
%Now we propose a scalable convex optimization framework for blind deconvolution.

Under assumptions we will be making, the sequence $\bx$ underlying our observed data will be either exactly sparse -- having few nonzeros -- or approximately so. Moreover, there will be either an exact length $k$ inverse filter $\bw$, or approximately such. It follows that the filter output $\bw \star \by$ is sparse.
This suggests the would-be optimization principle 
\[
 \begin{array}{ll}
 \underset{\bw\neq 0}{\mbox{minimize}}   & \|\bw \star \by^{[N]}\|_{\ell_0(\{-T+k,\dots,T-k\}})
\end{array}
  \]
where the $\ell_0$ quasi-norm simply 
counts the number of nonzero entries. Unfortunately, this objective, though well-motivated, is not suitable for numerical optimization.

Inspired by this, we perform convex relaxation of the $\ell_0$ norm, replacing it with the $\ell_1$ norm, 
which is convex.

We also need to fix the scale to get a unique output. One might think to constrain $\|\bw\|_2 =1$, however, this would give a non-convex constraint and again is not suitable for effective algorithms.


%Here we propose a convex way to fix the scale symmetry by choosing a linear constraint that only allows non-zero $w$. 

%\paragraph{Transformed $\ell_\infty$ sphere constraint}
We instead suppose given a rough initial approximation  
$\widetilde{\ba}$ of the forward filter $\ba$, and impose 
an $\ell_\infty$ constraint on the 
`pseudo-delta' $\bw\star\widetilde{\ba}$,
forcing it to `peak' at target entry $t$.
\begin{comment}
\BEQ
 \begin{array}{ll}
& \|\widetilde{\ba}*\bw\|_\infty = 1.
\end{array}
% \tag{$P_{v}^T$ }
\EEQ 

This intuition for the choice is based on the fact that $a^{-1}*a = \be_0$, we know $(a^{-1}*a)_0 = 1$ is a constraint on the largest entry. Therefore, $\|\widetilde{\ba}*a^{-1}\|_\infty = 1$ would be true if  $\widetilde{\ba} = a$. 

Based on shift and scaling symmetry, without loss of generality, we could assume that   $\widetilde{\ba}* a^{-1}$ 
has $0$-th entry being the largest absolute value entry by shifting $\widetilde{\ba}$, and set its value to $1$ by scaling $\widetilde{\ba}$, then up to shift and scaling of $\widetilde{\ba}$, 
\[
(\widetilde{\ba}*a^{-1})_0 = \|\widetilde{\ba}*a^{-1}\|_\infty =1
\]


Although this transformed $\ell_\infty$ sphere constraint is still a non-convex constraint, we can focus on one surface by fixing the $t$-th coordinate of entry with largest magnitude:
\end{comment}
\BEQ
 \begin{array}{ll}
&  (\widetilde{\ba}*\bw)_t =1, \quad \|\widetilde{\ba}*\bw\|_\infty \leq 1.
\end{array}
% \tag{$P_{v}^T$ }
\EEQ
Combining these steps, we obtain a convex optimization problem 
associated to each possible target coordinate $t$:
\BEQ
 \begin{array}{ll}
 \underset{\bw \in \ell_1^k}{ \mbox{minimize} }   & \frac{1}{N-2k} \| \bw \star \by^{[N]}\|_{\ell_1(\{-T+k,T-k\})}\\
\mbox{subject to}  
&  (\widetilde{\ba}*\bw)_t =1, \quad \|\widetilde{\ba}*\bw\|_\infty \leq 1.
\end{array}
% \tag{$P_{v}^T$ }
\EEQ

\begin{comment}

\end{comment}In the case of perfect shift symmetry of convolution ( linear convolution on bisequence, or circular convolution for finite observation ), we could design the problem to fully utilize the shift symmetry of objective  $\frac{1}{N} \| w*Y\|_{\ell_1(\cT)}$, so that the convex problem is equivalent to a convex optimization problem with a simple linear constraint as the $\ell_\infty$ box constraint 
with a fixed location of largest entry at $0$ coordinate under shift:
\BEQ
 \begin{array}{ll}
\widetilde{\ba}^{T} w^{\dagger} = \langle \widetilde{\ba}, w^{\dagger}\rangle = (\widetilde{\ba}*w)_0  =1, 
\end{array}
\EEQ
where $w^{\dagger}$ is the time reversal of $w$.
\end{comment}

It will be convenient to reformulate slightly,  
hide consideration of end effects,
and force the peak to occur at target coordinate $t=0$.
Abusing notation somewhat, we then write:
\BEQ
 \begin{array}{ll}
 \underset{\bw \in \ell_1^k}{ \mbox{minimize} }   & \frac{1}{N} \| \bw* \by \|_{\ell_1^N}\\
\mbox{subject to}  
& \langle \widetilde{\ba},  \bw^{\dagger} \rangle =1, 
\end{array}
\tag{${C}_{\widetilde{\ba}}$ }
\EEQ

(Again $\bw^\dagger$ denotes time-reversal of $\bw$). In practice we
might truncate the convolution due to end effects, or truncate the window over which we take the norm, but we will hide such practical details in the coming material, for ease of exposition; they would not change our results. 

 
\paragraph{Stochastic models for sparse signals}
Although our algorithms make sense in the absence of any theory,
our theoretical results concern properties of our algorithm for data generated under a probabilistic generative model i.e. a {\it stochastic signal} model. 

Let $X = (X_t)$ be a bisequence
of independent identically distributed random variables indexed by $t \in \integers$, having a common marginal CDF $F = F_X$, such that $F(x) = 1 - F(-x)$. One realization is then a sequence $\bx$ of the type discussed in earlier paragraphs.

We assume that $F$ has an atom at $0$ \-- $F = (1-p) H +p G$, where $H$ is the standard Heaviside distribution and $G$ is the standard Gaussian distribution.  We say that $F$ follows the \emph{Bernoulli$(p)$-Gaussian} model. 
Equivalently, $X_t$ is sampled IID from the \emph{Bernoulli$(p)$-Gaussian} distribution
$p N(0,1) +(1-p) \delta_0$. 

The iid process $X$ is of course ergodic. 
If $\bx$ denotes one realization of $X$, then in a window $(x_t)_{-T}^T$ of length $N$,  $\approx p N$ nonzero values  will occur,
for large $N$. Consequently, if $p \ll 1$,
realizations from $X$
will empirically be sparse.

\newcommand{\bb}{{\bf b}}
Let $Y = \ba \star X$ denote the random bisequence produced as the output of convolution of the random signal $X$
with deterministic filter $\ba \in \ell_1(\integers)$. More explicitly,
\[
    Y_t = \sum_u a(u) X_{t-u}.
\]
This defines formally a so-called {\it stationary linear process},  a classical object for which careful foundational results are well established.\footnote{In our case, we assume that $X$ is iid Bernoulli-Gaussian, so
$E |X_0| = p \cdot E |N(0,1)|$ is finite. Using this,
we can see that the sum in the display above, 
even though possibly containing an 
infinite number of terms, converges in various natural senses.}
Consider now filtering $Y$, by a length-$k$ filter 
$\bw$, producing the random bisequence $V = \bw \star Y$.
The {\it end-to-end} filter $\bb = \bw \star \ba$ 
is a well-defined element of $\ell_1(\integers)$; 
using it, we can represent 
the filtered output in terms of the underlying iid process $X$:
$V  = \bb \star X$. 
This representation shows that the filtered output series $V$ is itself a well-defined stationary linear process, and moreover, since $E |X_0| < 1$ and $\| \bb \|_{\ell_1} \leq \|\bw \|_{\ell_1} \cdot  \| \ba \|_{\ell_1} < \infty$, we have $E | V_0| < \| \bb \|_{\ell_1} < \infty$.

Any such stationary linear process is ergodic.
By the ergodic theorem, the
large-$N$ limit of the objective 
will \redit{almost surely}  be an expectation over $X$:
\BEQ
 \begin{array}{ll}
\lim_{N\rightarrow \infty}\frac{1}{N} \| \bw*Y\|_{\ell_1^N}  = \lim_{N\rightarrow \infty}\frac{1}{N} \sum_{t\in \cT^N}|(\bb \star X)_t|  =  \Expect_X|(\bb \star X)_0|=\Expect|(\bw*Y)_0|.
\end{array}
\EEQ
\sout{Evidently} \redit{Consequently}, 
the large-$N$ properties of our proposed algorithm
are driven by properties of the following optimization problem
{\it in the population}:
 \[
 \begin{array}{ll}
 \underset{\bw }{\mbox{minimize}}   & \Expect|(\bw*Y)_0|\\
\mbox{subject to}  &  \langle \widetilde{\ba},  \bw^{\dagger} \rangle =1. 
\end{array}
  \]

  
  




\section{Main Results Overview}



% The $\ell_1$ norm or $\ell_2$ norm ball would still led to 



% If $G$ is some sub-Gaussian distribution instead, then we called it \emph{Bernoulli$(p)$-sub-Gaussian} model.





\subsection{Main Result $1$: Phase Transition Phenomenon for Sparse Blind Deconvolution}

We have at last defined a convex optimization problem 
at the population level, which we will now want to study in detail.
In our studies, we can make various choices of the sparsity parameter $p$, of the underlying forward filter $\ba$, and of the guess $\tilde{\ba}$. The tuple $(p,\ba,\tilde{\ba})$ defines in this way a kind of phase space. We can then study performance of the algorithm at different points in phase space. 

\newcommand{\ERP}{{\sc Exact}{\sc Recovery}}
Consider this performance property: 
\begin{quotation}
\ERP \, $\equiv$ \,  {\sl ``There is an unique solution of the population-based optimization problem --- modulo time shift and output rescaling --- and
this solution {\bf exactly} solves the blind deconvolution problem correctly. ''}
\end{quotation}
It probably seems too much to ask that such a property could {\sl ever} be true, i.e. could ever be true for even one 
choice of phase space tuple. After all the optimization problem doesn't have any apparent connection to blind deconvolution -- instead only to some sort of relaxation of the search for sparse output filters.


We will see that this phase space can be partitioned into two regions: one where the exact recovery property holds and its complement where the exact recovery property fails. Surprisingly the region where \ERP \  holds is nonempty and can be appreciable. And it can be described in a clear and insightful way.

\paragraph{Surprising phase transition for a special case of sparse blind deconvolution}



 \sout{To demonstrate the flavor of the} \redit{We first illustrate the phase transition phenomenon in possibly the most elementary situation}. \sout{we present the population phase transition theorem for} \redit{Consider the special case when} the forward filter $\ba$ is the exponential decay filter:  $\ba = (1, s, s^2, s^3, \ldots )$ with $|s|\leq 1$; then the inverse filter is a basic short filter  $\ba^{-1} = ( 1, -s )$. 
\begin{theorem}[Population phase transition for exponential decay filter]
\label{thm: single root PT}
Consider a linear process $Y = \ba * X$ with
\BIT
\item
$\ba = (1, s, s^2, s^3, \ldots )$ where $|s|\leq 1$, so $\ba^{-1} = ( 1, -s )$;
\item 
$X_t$ is IID \emph{Bernoulli$(p)$-Gaussian}
$p N(0,1) +(1-p) \delta_0$.
\EIT
Consider as initial approximation 
$\widetilde{\ba} = \be_0 = ( 1, 0, 0,0, \ldots)$,
and the resulting 
fully specified population
optimization problem, 
with parameter tuple $(p,\ba,\tilde{\ba})$:
 \[
 \begin{array}{ll}
 \underset{\bw }{\mbox{minimize}}   & \Expect|(\bw*Y)_0|\\
\mbox{subject to}  & \bw_0 =1.
\end{array}
\tag{${P}_1(e_0)$ }
\label{bd:population}
  \]
Let $\bw^\star$ denote the (or simply some) solution.
Define the threshold
\[
p^\star  = 1-|s| .
\]
The property \ERP experiences a phase transition at $p = p^\star$:
\BIT
    \item provided $p<p^\star$, then $\bw^\star$ is uniquely defined and equal to $\ba^{-1}$ up to shift and scaling ; and
    \item provided $p> p^\star$, then $\bw^\star$ is not $\ba^{-1}$ up to shift and scaling .
\EIT
  \end{theorem}
  
  
  \begin{figure}[!tb]
\centering
\includegraphics[width=.8\textwidth]{./figures_BD/PT_BD_1root_none.png}
\caption{Finite-sample phase transition diagram; ground truth filter is $\bw^\star =  ( 0, 1, -s )$ with $T=200$. Horizontal axis:  sparsity level $p$, ranging from $0.01$ to $0.99$; Vertical axis:  filter parameter $|s|$, ranging from $0$ to $0.99$.  The \redit{shaded attribute indicates the observed fraction of  
successful experiments at the given parameter combination from deep blue for 1.0 down to deep red for 0.0. Thus,} the red region indicates failure of recovery and the blue region indicates success. \redit{The transition from success to failure is quite abrupt.}}
\label{fig-PT-finite}
\end{figure}

We can empirically \sout{verify} observe that the population phase transition described in Theorem 1 
describes accurately the situation with finite-length signals.  \sout{by discretizing the} \redit{The setting of Theorem 1,
defines a phase space by the numbers $(p,s)$. We can
sample the phase space according to} a grid and then at each grid point, conducting a sequence of experiments like so:
\BIT
\item sample a realization of synthetic data $Y = \ba \star X$ according to the stochastic signal;
\item extract a window  $\by^{[N]}$ of size $N$ from within 
each generated $Y$; and
\item solve the resulting finite-$N$ optimization problem:
\[
 \begin{array}{ll}
 \underset{\bw }{\mbox{minimize}}   & \frac{1}{N}\|\bw*Y\|_1\\
\mbox{subject to}  & \bw_0 =1.
\end{array}
\tag{${P}^N_1(e_0)$ }
\label{bd:finite}
  \]
\EIT
% \Dave{There really should be labels on optimization problems,
% and there should be a finite-n problem with a label and
% a population problem with a label. 
% Otherwise the above is too mumbled. eg What exactly
% is the resulting finite-$N$ problem?}
Tabulating the fraction of instances with numerically precise recovery of the correct underlying inverse filter $\ba^{-1}$ 
and sparse signal $X$ across
grid points, we can make a heatmap of empirical success probability.

Specifically, we numerically run $20$ independent experiments, and choose an accuracy $\epsilon = 10^{-3}$ and count the number of successfully accurate recovery where the convex optimization solution $w$ satisfy $\|w^\star -w\|_1/\|w^\star\|_\infty<\epsilon$.

We do this in Figure~\ref{fig-PT-finite}; the reader will see there an empirical phase transition curve, produced by a logistic-regression calculation of the location in $p$ where $50\%$ success probability is achieved. 
We observe empirical behavior entirely consistent 
with $p^\star  = 1-|s|$.





% \newcommand{\bz}{{\bf z}}

\paragraph{Phase transition for sparse blind deconvolution with general filter}
Now we present the main phase transition theorem for blind deconvolution of general inverse filter.

To state the theorem,
define the operator $'$ that 
sets the largest entry in a bisequence to zero,
while preserving the other entries. Operating on bisequence $\bv$
it yields
 \[
 \bv' \equiv \bv - v_{t_m}\be_{i_m}
 \]
 where $t_m = \arg\max_t |v(t)|$;  if there are multiple largest entries, $t_m$ is the smallest such index.
Also, for, $k \in \{ 1, 2, 3 , \dots \}$, 
let $|\bv|_{(k)}$ denote
the $k$-th largest amplitude entry in bisequence 
$\bv$.

In addition, let $I$ denote an iid Bernoulli(p) bisequence.
For a bisequence $\bw$ let $ \bw \cdot I$ denote the 
elementwise multiplication
of $\bw$ by $I$.
Define the optimization problem
\[
 \begin{array}{ll}
 \underset{\bw}{\mbox{minimize}}   & \E_I \|\bw \cdot I\|_2\\
\mbox{subject to}  
& \langle   \bv, \bw\rangle =1
\end{array}
\tag{$Q_1(\bv)$ }
  \]


	\begin{theorem}[Population (large-$N$) phase transition]
	\label{thm:Population phase transition}
Consider  a linear process $Y = \ba \star X$ where
\BIT
\item
 $X = (X_t)_{t \in \integers}$ is IID with marginal distribution  $pN(0,1) + (1-p) \delta_0$; and
 \item
$\ba\in l_1(\integers)$ is invertible:  $(\mathcal{F} \ba)(\widetilde{w}) \neq 0$, $\forall \widetilde{w}\in T$; thus $\ba^{-1}$ exists in $\ell_1(\integers)$.
\EIT

Consider the convex optimization problem 
 \[
 \begin{array}{ll}
 \underset{\bw \in l_1(\integers)}{\mbox{minimize}}   & \Expect|(\bw*Y)_0|\\
\mbox{subject to}  
& \langle \widetilde{\ba},  \bw^{\dagger} \rangle =1,
\end{array}
\tag{${P}_1(\widetilde{\ba})$ }
\label{eqn:P1}
  \]
and let $\bw^\star$ denote any solution of the optimization problem. 

There is a threshold $p^\star > 0$,
\BIT
\item  $\bw^\star$ is $\ba^{-1}$ up to time shift and rescaling provided $p<p^\star$; and
\item   $\bw^\star$ is not $\ba^{-1}$ up to time shift and rescaling, provided $p> p^\star$.
\EIT
% \newcommand{\tbe}{\widetilde{\be}}
Define $\widetilde{\be}:= \widetilde{\ba}*\ba^{-1}$.
The threshold $p^\star$ obeys
 \[
\frac{p}{1-p}= val(Q_1(\tbe')).
\] 
We have an upper bound and lower bound
\[
 \frac{p}{\|\tbe'\|_\infty}  \geq val(Q_1(\tbe')) \geq  p \cot\angle(\tbe, \be_0) 
\]
explicitly, the upper bound can be expressed as
\[
1- \cot\angle(\tbe, \be_0)   \leq p^\star \leq 1- \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}
\]
Additionally, the upper bound 
takes equality if
\[
	\frac{|\tbe|_{(3)}}{|\tbe|_{(2)}} \leq \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}
	\]
% 	\[
% 	p\leq 1- \frac{|\tbe|_{(3)}}{|\tbe|_{(2)}}
% 	\]
Here \redit{the multiplicative gap} $\frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}$ denotes 
the ratio of the  first and second largest entries 
of $|\tbe|$,and is a natural measure of closeness 
between our approximate Kronecker delta $\tbe=\widetilde{\ba} * \ba^{-1}$ 
and true Kronecker delta  $\be_0$. In words {\it the less accurate the initial approximation $\widetilde{\ba} \approx \ba$, the greater we rely on sparsity of $X$ \redit{to allow exact recovery}.}

%Furthermore, after change of variable $\psi := (\ba}w)^{\dagger}$ and $\tbe:= \widetilde{\ba}*a^{-1}$, the optimization problem  ${P}_1(\widetilde{\ba})$ can be reduced to a convex projection pursuit problem $Q_1(\tbe)$ up to a constant factor $\sqrt{\frac{2}{\pi}} $ on objective:
%\[
% \begin{array}{ll}
% \underset{\psi}{\mbox{minimize}}   & \E_I \|\psi\cdot I\|_2\\
%\mbox{subject to}  
%& \langle   \tbe, \psi\rangle =1
%\end{array}
%\tag{$Q_1(\tbe)$ }
%  \]
	\end{theorem}

\Dave{This result fails to deliver on the reader's investment of time to this point. We are on page 14. The reader gets something quite non-tangible (value of an optimization problem which itself requires deciphering) and then all sorts of ancillary details that only add to the deciphering. It would be better to state the most insightful and easily appreciated result first, otherwise essentially no-one will continue reading beyond this moment.}


\Dave{Also spotlighting this way of looking at the problem pigeon holes the paper as providing detailed insights of very limited generality and unlikely connection to problems most readers could care about.}










\paragraph{Alternate: Phase transition for sparse blind deconvolution with general filter}
\redit{Consider now a more general situation where $\ba$ is a quite general filter, and $X$ is Bernoulli Gaussian. 
Our formal assumptions are:}

\redit{\begin{enumerate}
 \item  [{\bf A1}]
$\ba\in l_1(\integers)$ is invertible:  $(\mathcal{F} \ba)(\widetilde{w}) \neq 0$, $\forall \widetilde{w}\in T$; thus $\ba^{-1}$ exists in $\ell_1(\integers)$.
\item [{\bf A2}] $X = (X_t)_{t \in \integers}$ is IID with marginal distribution  $pN(0,1) + (1-p) \delta_0$; and
\item [{\bf A3}] $Y = (Y_t)_{t \in \integers}$ is a linear process
obeying $Y = \ba \star X$.
\end{enumerate}}

\redit{Consider the convex optimization problem 
 \[
 \begin{array}{ll}
 \underset{\bw \in l_1(\integers)}{\mbox{minimize}}   & \Expect|(\bw*Y)_0|\\
\mbox{subject to}  
& \langle \widetilde{\ba},  \bw^{\dagger} \rangle =1,
\end{array}
\tag{${P}_1(\widetilde{\ba})$ }
\label{eqn:P1}
  \]
and let $\bw^\star$ denote any solution of the optimization problem. }

\newcommand{\tba}{\widetilde{\ba}}
%\newcommand{\tbe}{\widetilde{\be}}
\newcommand{\mgap}{\mbox{Gap}}
\newcommand{\lOneZ}{l_1(\integers)}
\newcommand{\lInfZ}{l_\infty(\integers)}
\redit{Our results establish the existence of a general
phase transition phenomenon and a precise quantification of it,
in terms of a {\it phase transition functional} .}

\redit{Define the following {\bf deltaness discrepancy} $\Delta(\bv)$:
\[
 \Delta(\bv) =  \inf_{\alpha,k} \frac{\| \bv - \alpha \delta_k \|_\infty}{\|\bv\|_\infty}.
\]
}

\redit{This discrepancy  indeed obeys
$\Delta(\be_0) = 0$. However, it is not restricted only to
deltaness concentrating at the origin; in fact,
$\Delta( \alpha \cdot \be_k) = 0$ for
each $\alpha > 0$, $k \in \integers$.
Also, $0 \leq  \Delta(\bv) \leq 1$.
At the other extreme,
$\Delta([...,0,0,1/2,1/2,0,0,...]) = 1$. 
Finally,
$\Delta$ is a continuous function on $\lOneZ$:
so that, 
setting $\eps(\bv,\bw) \equiv \frac{\|v-w\|_\infty}{\|w\|_\infty}$,
\[
   | \Delta(\bv) - \Delta(\bw) | \leq \frac{2 \cdot \eps}{1-\eps}.
\]
}
	\begin{coro}
	[\redit{Alternative Population (large-$N$) phase transition}]
	\label{coro:AltPopulationPhaseTransition}

\redit{Under assumptions (A1)-(A3),}
\BIT
\item \redit{There is a functional
$\Pi^*$ defined on tuples $(\ba,\tba)$ in 
$\ell_1(\integers) \times \ell_1(\integers)$
with the property that, for $p > \Pi^*(\ba,\tba)$,
every solution of the optimization problem ${P}_1(\widetilde{\ba})$
is exactly the correct answer $\ba$, up to lateral shift and scaling.}

\item \redit{We have the upper bound:
\begin{equation}
    \label{eq:coro-upperbnd}
\Pi^*(\ba,\tba) \leq 1-\Delta(\tba*\ba^{-1}), \qquad (\ba,\tba) \in \ell_1(\integers) \times \ell_1(\integers).
\end{equation}
}

% \item \redit{Equality is generic:
% \[
% \Pi^*(\ba,\tba) =  \Delta(\tba*\ba^{-1}),
% \]
% for each $\ba \in \lOneZ$,
% on an open dense subset of $\tba \in \lOneZ$.}

% \item \redit{ In fact, 
% $\overline{\Pi}^* \equiv \Delta(\tba*\ba^{-1})$ 
% is the {\bf unique
% upper semicontinuous extension} of the Phase transition functional $\Pi^*$}.
\EIT
\end{coro}


\redit{The reader might compare this with our earlier example
in Theorem \ref{thm: single root PT}, the special case of
geometrically decaying filters. 
In that example $\ba = (\dots,0,0,1,s,s^2,\dots)$ while
$\tba = (\dots,0,0,1,0,0,\dots)$. $\Delta(\tba*\ba^{-1})= \Delta((\dots,0,0,1,s,s^2,\dots)) = |s|$. In short, the upper bound $\Pi^* = 1- |s|$ deriving from this general viewpoint agrees precisely with the the exact answer $p^* = 1- |s|$ given in that earlier Theorem. }

\redit{According to this corollary that there is a substantial
region in the space of $(\ba,\tba)$ pairs where a meaningful 
sparsity-accuracy of initialization tradeoff exists, such that
 any sufficiently accurate initial guess results in
exact recovery \-- provided that the sparsity of the underlying object $X$ exceeds a threshold.}

\begin{coro}
\redit{Let $r \in (0,1/2)$ and suppose 
that assumptions (A1)-(A3)
hold with $p > \frac{r}{1-r}$. 
Normalize the problem so that 
$\| \ba^{-1} \|_\infty =1$.}

\redit{Consider $\tba$ in the $\ell_1$ metric ball
(\ref{eq:lonemetricball}) of radius $r$
about $\ba$:
\BEQ \label{eq:lonemetricball}
    \| \tba - \ba \|_1 \leq r .
\EEQ
}
\redit{Every solution of the optimization problem $P_1(\tba)$ 
achieves exact recovery of $\ba$ up to shift and rescaling.}
\end{coro}

\redit{{\bf Proof:} Indeed, we can give a more explicit form
for $\Delta$; 
\[
 \Delta(\tbe) = \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}},
\]
where $|\tbe|_{(1)}$ denotes the largest entry
in $\tbe$ and $|\tbe|_{(2)}$ the second largest.
$\frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}$ 
is a kind of multiplicative gap functional,
measuring the extent to which the second-largest entry in $\tbe$
is small compared to the largest entry.}

\redit{Since 
\[
  \| \tbe - \be_0\|_\infty \leq \| \ba^{-1} \|_\infty \cdot \| \tba-\ba\|_1 = r,
\]
we have $|\tbe|_{(1)} \geq 1-r$ and $|\tbe|_{(2)} \leq r.$ This 
implies that $\Pi^* \leq \frac{r}{1-r}$. Now apply Corollary
\ref{coro:AltPopulationPhaseTransition}.
\qed
}


When does equality hold in (\ref{eq:coro-upperbnd})?
For a vector $\bv$, let $\bv'$ denote the same vector,
except the largest-amplitude  entry is replaced by $0$. We will see
that a sufficient condition for equality is:
\[
   \Delta(\tbe') \geq \Delta(\tbe).
\]
Put another way, equality holds if 
\BEQ \label{eq:suffcondsharp}
|\tbe|_{(3)} \leq  (1-\Delta(\tbe)) \cdot |\tbe|_{(2)}.
\EEQ
The set of situations where this occurs is ample but not overwhelming.
It has relative
Lebesgue measure at least  $1-\Delta$. In the situation covered by  Theorem \ref{thm: single root PT},
$|\tbe|_{(3)}  = s^2$, $ |\tbe|_{(2)} = s$,
$1- \Delta = s$, and so equality holds in (\ref{eq:suffcondsharp}).
Hence, the general-filter result of Corollary 
\ref{coro:AltPopulationPhaseTransition} along with the sufficient condition (\ref{eq:suffcondsharp})
imply as a special case
Theorem \ref{thm: single root PT}.

% \redit{}





\subsection{Main Result $2$: Finite Observation Window, Finite-length Inverse}

With a finite observation window of length $N$ we (surprisingly) still can have exact recovery, starting as soon as $N \geq \Omega(k\log(k))$.

\paragraph{Finite-observation phase transition}

%\newcommand{\bV}{{\bf V}}

Let 
% $\bV=\bV_k$ 
$\ell_1^k$
denote the collection of bisequences vanishing outside a centered window of radius $k$.

	\begin{theorem}[Finite observation window, finite-length inverse filter]
	\label{thm:fin_guarantee}
	Suppose $Y = \ba \star X$, where:
	\begin{enumerate}
 \item  [{\bf A1}]
$\ba\in l_1(\integers)$ is invertible and the inverse has finite-length:  $(\mathcal{F} \ba)(\widetilde{w}) \neq 0$, $\forall \widetilde{w}\in T$; thus $\ba^{-1}$ exists in $\ell_1(\integers)$; furthermore, $\ba^{-1} \in \ell_1^k$ vanishes off a centered window of length $k$.
\item [{\bf A2}] $X = (X_t)_{t \in \integers}$ is IID with marginal distribution  $pN(0,1) + (1-p) \delta_0$; 
\item [{\bf A3}] $Y = (Y_t)_{t \in \integers}$ is a linear process
obeying $Y = \ba \star X$. Suppose we observe a window $(Y_t)_{t\in \cT}$ of length $N = |\cT|$. 
\end{enumerate}


Consider the convex optimization problem
\BEQ
 \begin{array}{ll}
 \underset{\bw\in \ell_1^k}{  \mbox{minimize} }   & \frac{1}{N}\|\bw*Y\|_{\ell_1^N}\\
 \mbox{subject to}  
& (\widetilde{\ba}* \bw)_0 =1.
\end{array}
\tag{${P}_{1}^{N,k}(\widetilde{\ba})$}
\label{P1_finite}
\EEQ
and let $\bw^\star$  denote any solution of the optimization problem.

	Our result establishes that there exist $\epsilon>0, \delta>0$, so that when the number of observations $N$ satisfies
		\[
N \geq  k\log(\frac{k}{\delta}) ( \frac{C\kappa_\ba}{\epsilon}  )^2,
\]
and the sparsity level $p$ obeys $\frac{1}{N}\leq p < p^\star - \delta_p(N,\epsilon)$,
		then 	with probability exceeding $1-\delta$, $\bw^\star$   is $\ba^{-1}$ up to rescaling and time shift. In the statement, $\kappa_\ba$ is the condition number of the circular matrix with its first column being $\ba$; $C$ is a positive constant independent of $N$ and $k$.
	\end{theorem}
	
 


\subsection{Main Result $3$: Stability Guarantee with Finite Length Inverse Filter}
The results so far concern the ideal setting when true inverse filter has a known length $k$ and we use $k$ to set up a correctly matched optimization problem. In practice we do not know $k$ and $k$ might even be infinite.

We can provide practical guarantees even when the inverse filter is an infinite length inverse. To develop these, we must be more technical about the situation. We assume that $\ba$ has a Z-transform having $N_{-}$ roots and $N_{+}$ poles $(s_{i})$ inside the unit circle and we construct a finite length approximation $\bw$ to  $\ba^{-1}$, in fact of length
$r(N_{-}+N_{+})$.
This approximation has error 
$\|\bw*\ba-\be_0\|_2= O(\max_i |s|_{i}^{r}  )$. 

Since the objective value $\E_I\|\bw\cdot I\|_2$ of this approximation $\bw$ is an upper bound of the optimal value of the optimization solution $\bw^\star$, we could use the objective value upper bound  to derive a upper bound for $\|\bw^\star*\ba-\be_0\|_2= O(
\max_i |s|_{i}^{r}  )$ when $p<p^\star$, where the constant of this upper bound is determined by the Bi-Lipschitz constant of the finite difference of objective $\E_I\|\bw\cdot I\|_2-\E_I\|(\be_0)\cdot I\|_2$.

\paragraph{Approximation theory for infinite length inverse filter}
\begin{theorem}[Approximation theory for infinite length inverse filter based on roots of Z-transform]
\label{thm:RootNorm}
Let the finite-length forward filter $\ba$ have a Z-transform with roots inside the unit circle, namely $s_{k}:= e^{-\rho_k + i \varphi_k }$ with $|s_k|<1$ and $\rho_k>0$
for $k \in \{-N_{-}, \ldots -1, 1, \ldots N_{+}\}$.  Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible indexes.
\[
 \begin{array}{ll}
A(z) &=  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i}
\\
&= c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1});
\end{array}
  \]
here $c_0$ is a constant ensuring $a_0=1$.

Then for a scalar $r$
% vector index $r=(r_{-N_-}, \ldots, r_{-1}, r_{1},\ldots, r_{N_+} )$
, we construct an approximate inverse filter $\bw^r$ with Z-transform
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r-1} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r-1} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r}) (1- s_{i} z^{-1})^{-1}.
\end{array}
\]
We have
\[
 \begin{array}{ll}
 \|\bw^r*\ba-\be_0\|_2^2  
 &= \sum_{n\in \{1,2,3,\ldots,|\cI| \} }\sum_{ k_1, \ldots, k_n  \in \cI } \prod_{i\in [n]}|s_{k_i}|^{2r }
\end{array}
  \]
%   Let $\gamma^m := \min_{i}\big(r_{i} |\rho_{i}| \big) =  \min\{r_{-N_-}|\rho_{-N_-}|, \ldots, r_{-1}|\rho_{-1}|, r_{1}|\rho_{1}|, \ldots, r_{N_+}|\rho_{N_+}|\}.$
as $r \rightarrow \infty$, this converges to zero at an exponential rate, determined by the slowest decaying term,
\[
 \begin{array}{ll}
\|\bw^r*\ba-\be_0\|_2
&=  O( |s|_{(1)}^{r}  ) , \quad r \rightarrow \infty.
\end{array}
  \]
  where $|s|_{(1)}$ is the largest absolute value root.
 \end{theorem}
 
% \Dave{What is $\cI$?}
 
 \paragraph{Stability for infinite length inverse filter}
 \begin{theorem}[Stability for infinite length inverse filter]
 \label{thm:bd_stab}
 Let $\ba\in V_{N_-, N_+} $ be a forward filter with all the roots of Z-transform strictly in the unit circle. Let $\bw^\star \in V_{(r-1)N_-, (r-1)N_+} $ be the solution of the convex optimization problem. Let $\bw^r$ be the constructed filter in previous theorem with a uniform vector index $(r, \ldots, r, r,\ldots, r)$.
  Then provided $p<p^\star$, as 
  $r \rightarrow \infty$, 
  \[
 \begin{array}{ll}
  \| \bw^\star*\ba -\be_0\|_2 
   \leq
    O(
 |s|_{(1)}^{r}  ), \quad r \rightarrow \infty.
\end{array}
  \]
  where $|s|_{(1)}$ is the largest absolute value root.
In words, \textbf{the Euclidean distance between $\bw^\star*\ba$ and $\be_0$ converges to zero at an exponential rate as the approximation length is allowed to increase.} 
 \end{theorem} 
 
%  \Dave{I don't understand the roots of Z transform comment. Did you think clearly about this? I think what you mean is no roots are on the unit circle, some number are inside and some number are outside. Right now it looks very doubtful.}
 
 
\subsection{Main Result $4$: Robustness Against Stochastic Noise and Adversarial Noise}
We now extend the previous analysis of an exactly sparse model of $X$, exactly observed, to the more practical setting of approximate sparsity and observation noise. We consider two cases: first we add stochastic noise as an independent Gaussian linear process, and second adversarial noise with bounded $\ell_\infty$ norm.  

In each scenario, since the noisy objective value at $\be_0$ is an upper bound on the optimal value of the optimization solution $\bw^\star$, we use this upper bound on the objective value  to derive an upper bound of $\|\bw^\star*\ba-\be_0\|_2$ when $p<p^\star$.
%, where the constant of this upper bound is determined by the Bi-Lipschitzness constant of finite difference of objective $\E_I\|\bw\cdot I\|_2-\E_I\|(\be_0)\cdot I\|_2$. 
The upper bound shows that the distance $\|\bw^\star*\ba-\be_0\|_2$ is bounded by the (appropriately measured)
magnitude of input noise in both cases.


\paragraph{Robustness under stochastic noise }
 \begin{theorem}[Robustness against Gaussian Linear Process noise]
 \label{thm:rand_exact_rob}
 We consider a Gaussian linear process $Z = \sigma \cdot \bb \star G$ where: $\sigma > 0$ denotes the noise level;   $\bb$ is
 a bisequence having  unit $\ell_2$ norm $\|\bb\|_2=1$; and $G$ is a standard Normal iid bisequence:
 \[
\begin{array}{ll}
Y&= \ba* (X+ Z).
\end{array}
\]
 
 \newcommand{\wpsi}{{\bf w}}
 Let $\wpsi^\star$ be the solution of the convex optimization problem in Eq.(4.1);
 %for the moving average random noisy model
%  \[
%\begin{array}{ll}
%Y&= \ba* (X+ \sigma \bb*G),
%\end{array}
%\]

\label{thm:Bound_Normal_Noise}
\[
 \E_I  \| (\wpsi^\star)\cdot I \|_2 -\E_I  \| (\be_0)\cdot I \|_2 \leq  (1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1).
\]
%When $\sigma\leq 1,$
%\[
%(1-p) \sigma +
% p(\sqrt{1+ \sigma^2 }-1)  \leq \sigma;
%\]
%therefore, 
When $p<p^\star$, $\sigma\leq 1$, there exists a constant $C$,
\[
  \| \bw^\star*\ba -\be_0\|_2 = \|\wpsi^\star -\be_0\|_2 \leq C \sigma.
\]
In words, \textbf{the Euclidean distance between $\bw^\star \star \ba$ and $\be_0$ is bounded linearly by the magnitude of stochastic noise}.
\end{theorem}  

\newcommand{\bc}{{\bf c}}
\paragraph{Robustness under adversarial noise }
 \begin{theorem}[Robustness under adversarial noise with $\ell_p$ norm bound]
\label{thm:adv_exact_rob}
Suppose that an adversary chooses a disturbance bisequence
$\bc$ subject to the constraint:	
\[
	\| \bc\|_\infty \leq \eta;
\]
and perturbs the observation process $Y$ via:
	\[
	\begin{array}{ll}
	Y&= \ba* (X+  \bc) .
	\end{array}
	\]
\newcommand{\apsi}{{\bf v}}
Let $\bw^\star$ denote the solution of the convex optimization problem~\ref{eqn:P1}.
Define $\apsi^\star = (\ba*\bw^\star)^{\dagger}$, then $\apsi^\star$ satisfies the following bound on objective difference:
 \[
 \begin{array}{ll}
 \E_I  \| (\apsi^\star)\cdot I \|_2 -\E_I  \| (\be_0)\cdot I \|_2 \leq 
 p\sqrt{\frac{2}{\pi}}(\mathcal{R}(\eta) - 1)+(1-p)\eta.
\end{array}
  \]  
 
Therefore, when $p<p^\star$, there exists a constant $C'$, so that
 \[
 \| \bw^\star*\ba -\be_0\|_2 = \|\apsi^\star -\be_0\|_2  \leq C'  \eta, \forall \eta > 0.
 \]
 In words, \textbf{the Euclidean distance between $\bw^\star \star \ba$ and $\be_0$ is at most proportional to the magnitude of the adversarial noise}.
 
 
\end{theorem}  

\textbf{Remark}: Here $\mathcal{R}(\eta)$
is the folded Gaussian mean, for standard Gaussian $G$:
\[
\mathcal{R}(\eta) :=  \sqrt{\frac{\pi}{2}} E_G |\eta+  G| = \exp\{-\eta^2/2\} + \sqrt{\frac{\pi}{2}}\eta \left(1 - 2\Phi\left(-\eta\right) \right).
\]  
$\mathcal{R}(\eta)-1$ is an even function that is monotonically non-decreasing for $\eta \geq 0$ with quadratic upper and lower bound: there exists constants $C_1\leq C_2$,
  \[
C_1 \eta^2 \leq \mathcal{R}(\eta)-1 \leq C_2 \eta^2, \forall \eta.
\]

\newcommand{\bu}{{\bf u}}
	





\section{Rest of Old Introduction}

	


% %%%%%%%%%%%%%%%%%%%%















\paragraph{Sketch of proof ideas for Theorem~\ref{thm:Population phase transition}}
The full proof is in section $6$. Here we highlight some of the key ideas in the proof:
\BIT
\item
\textbf{Change of variable.}
Rewrite the population version of our convex sparse blind deconvolution problem, with the population objective 
$\Expect\frac{1}{N} \| \bw*Y\|_{\ell_1(\cT)} =\Expect|(\bw*Y)_0|=\Expect|(\bw*\ba*X)_0|=\Expect_X|\langle X, (\bw*\ba)^{\dagger} \rangle|$ due to  the ergodic property of stationary process and shift invariance, and $(\widetilde{\ba}*\bw)_0=((\widetilde{\ba}*\ba^{-1})*(\ba*\bw))_0  = \langle (\widetilde{\ba}*\ba^{-1})^{\dagger}, \bw*\ba\rangle$, the convex problem becomes 
\[
 \begin{array}{ll}
 \underset{\bw}{\mbox{minimize}}   & \Expect_X|\langle X ,  (\ba*\bw)^{\dagger} \rangle|\\
\mbox{subject to}  
& \langle \widetilde{\ba}*\ba^{-1} , (\ba*\bw)^{\dagger}\rangle =1,
\end{array}
 \]
 \newcommand{\apsi}{{\bf v}}
Let $\apsi$ denote  the time reversed version of $\ba*\bw$: $\apsi := (\ba*\bw)^{\dagger}$, and
  let $\tbe:= \widetilde{\ba}*\ba^{-1}$, then by previous assumptions, 
  $\tbe(0)=1$, $\tbe' = \tbe-\be_0$.
  
 Now we arrive at a simple and fundamental population convex problem: 
 \[
 \begin{array}{ll}
 \underset{\apsi}{\mbox{minimize}}   &\Expect_X|\langle X ,  \apsi  \rangle|\\
\mbox{subject to}  
& \langle \tbe ,  \apsi  \rangle  =1.
\end{array}
  \]
  \item
\textbf{Expectation using Gaussian.  }
Since $X$ follows Bernoulli-Gaussian IID probability model $X_t = I_t G_t$, we nest the expectation over $I_t$ outside the expectation over Gaussian $G_t$, for which we use $E |N(0,1)| = \sqrt{\frac{2}{\pi}}$:
\[
\Expect_X|\langle X ,  \apsi  \rangle|
= \E_I \E_G {|\sum_{t\in \integers}  I_t G_t \apsi(t)| }
= \sqrt{\frac{2}{\pi}} \cdot\E_I \|\apsi\cdot I\|_2
\]
\item
\textbf{KKT condition for $\be_0$.}
%Now we state the general phase transition with light assumption. Here we don't need to even assume that $X$ are independent, we just need to know the existence of one sparse element $X_0$.
Let $\apsi^\star$ denote the solution of the optimization problem:
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \sqrt{\frac{2}{\pi}} \cdot\E_I \|\apsi\cdot I\|_2\\
\mbox{subject to}  
& \langle   \tbe, \apsi\rangle =1
\end{array}
\tag{$Q_1(\tbe)$ }
  \]
  
To prove that $\apsi^\star=\be_0$, i.e. $\be_0$ solves ($Q_1(\tbe)$), we calculate the directional finite difference at $\be_0$. Then $\be_0$ solves this convex problem if the directional finite difference at $\apsi = \be_0$ is non-negative at every direction $\beta$ on unit sphere where $\tbe^T \beta =0$:
	 \[
	 \Expect\|(\be_0+\beta)\cdot I\|_2 - \Expect\|(\be_0)\cdot I\|_2 \geq 0.
	 \]


\item
\textbf{Conditional expectation at one sparse element $X_0$.} 
We decompose the objective into a sum of terms, 
conditioning on whether $I_0 = 1_{\{X_0\neq 0\}}$ is zero or not:
	 \[
	 \begin{array}{ll}
	    \Expect\|(\be_0+\beta)\cdot I\|_2 - \Expect\|(\be(0))\cdot I\|_2
	    &= p (1+\beta_0)  + (1-p) \nabla_{\beta}{\Expect_I[\|(\be_0+\beta)'\|_{\ell_2(I-\{0\})} \mid I_0 =0]} -p\\
	    &= p \beta_0  + (1-p) \Expect_{I'}[\|\beta'\|_{\ell_2(I')} ].
	 \end{array}
	\]
This will be non-negative in case either $\beta(0) > 0$, or else $\beta(0) < 0$ but
	\[
	\frac{p}{1-p} \leq  \frac{\Expect_{I'}\|\beta'\|_{\ell_2(I')}}{ |\beta_0|}
	\]
	for all $\beta $ that satisfy $ \tbe^T \beta =0$.
\item
\textbf{Reduction to $val(Q_1 (\tbe')).$}	
	We normalize the direction sequence $\beta$ so that $\beta(0)= -1$; 
	using $\tilde{e}(0)=1$, we obtain a lowerbound:
\[
 \inf_{\beta(0)=-1, \langle  \tbe, \beta\rangle  =0} \Expect_{I'}\|\beta'\|_{\ell_2(I')}
 =\inf_{ \beta(0)=-1, \beta(0) \tilde{e}(0)-\langle  \tbe', \beta'\rangle  =0} \Expect_{I'}\|\beta'\|_{\ell_2(I')}
= \inf_{\langle   \tbe', \beta'\rangle  =1} \E_{I'} \|\beta'\|_{\ell_2(I')} = val(Q_1 (\tbe'))
\]	
Here $Q_1(\tbe')$ is the optimization problem:
\[
 \begin{array}{ll}
 \underset{\beta \in l_1(\integers)}{\mbox{minimize}}   &\E_{I'} \|\beta'\|_{\ell_2(I')}\\
\mbox{subject to}  
& \langle  \tbe', \beta'\rangle  =1
\end{array}
  \]

\item 
\textbf{The explicit phase transition condition with upper and lower bound.}
We have shown the existence of  $p^\star$ so that for all $p<p^\star$, the KKT condition is satisfied. And we have represented $p^\star$ as the optimal value of a derived optimization problem $val(Q_1 (\tbe'))$. The following lemma finds simple upper and lower bounds for $p^\star=val(Q_1 (\tbe'))$. 
	\begin{lemma}[Explicit phase transition condition with upper and lower bound]
	\label{lemma:Condition phase transition}
The threshold $p^\star$ determined by
 \[
\frac{p}{1-p}= val(Q_1(\tbe')).
\]
obeys an upper bound and lower
\[
 \frac{p}{\|\tbe'\|_\infty}  \geq val(Q_1(\tbe')) \geq  \E_I\|\tbe'\cdot I\|_{2}^{-1}
\]
where $\|\tbe'\|_\infty  = \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}  $.
	Additionally, the upper bound 
is sharp if and only if
	\[
	\frac{p}{1-p} \leq val(Q_1(\frac{\tbe'}{\|\tbe'\|_\infty}))=val(Q_1(\tbe''))/\|\tbe'\|_\infty
	\]
	therefore, the upper bound 
holds with equality 
	\[
	p^\star= 1- \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}
	\]
if 
		\[
	p\leq 1- \frac{|\tbe|_{(3)}}{|\tbe|_{(2)}}
	\]
	Therefore, if 
		\[
	\frac{|\tbe|_{(3)}}{|\tbe|_{(2)}} \leq \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}
	\]
	then
	\[
	p^\star= 1- \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}.
	\]
	
	\end{lemma}

The above narrative gives a sketch of our result and its proof. The upper bound $ 1- \frac{|\tbe|_{(2)}}{|\tbe|_{(1)}}$ of $p^\star$ generalized the previous special case of exponential decay filter in theorem~\ref{thm: single root PT} with $p^\star = 1-|s|$.
\item
\begin{lemma}[Geometric lower bound $val(Q_1(\tbe'))$ for the phase transition condition]
\label{lemma: geo lower}
    \[
val(Q_1(\tbe'))
\geq p \cot\angle(\tbe, \be_0)
\]
where
\[
\cot\angle(\tbe, \be_0) = \frac{1}{\|\tbe'\|_2} 
\]
\end{lemma}
\item
Using the technical background provided in theorem~\ref{thm:BGPropLemmaNorm}, we can further provide a tighter upper bound to compute phase transition $p^\star$.  
\begin{lemma}[Tighter upper bound $val(Q_1(\tbe'))$ for the phase transition condition]
\label{lemma: tigher upper}
Let $|\tbe|$ be the entry-wise absolute value of $\tbe$. We can rank the entries of $|\tbe|$ to be $|\tbe|_{(1)}, |\tbe|_{(2)}, |\tbe|_{(3)},\ldots$, then the entries of $\tbe'$ will be ranked as $|\tbe|_{(2)}, |\tbe|_{(3)},\ldots$, we define $|\tbe|^{(m)}$ as the vector that only keep the entries $|\tbe|_{(2)}, |\tbe|_{(3)},\ldots, |\tbe|_{(m+1)}$ of $|\tbe|$, and send the rest of entries to zero. 
Then
    \[
val(Q_1(\tbe'))
\leq \inf \{ \frac{p}{|\tbe|_{(2)}}, \frac{V_1(|\tbe|^{(2)})}{\||\tbe|^{(2)}\|_2}, \frac{V_1(|\tbe|^{(3)})}{\||\tbe|^{(3)}\|_2}, \ldots, \frac{V_1(\tbe')}{\|\tbe'\|_2}   \}
\]
where $V_1$ function takes value in $[p, \sqrt{p})$.
Therefore, intuitively,
  \[
val(Q_1(\tbe'))
\leq 
\inf \{ \frac{p}{|\tbe|_{(2)}},  \sqrt{p} \cot\angle(\tbe, \be_0) \}
\]
\end{lemma}

\EIT

		
		
	
	



\subsection{Main Result $2$: Finite Observation Window, Finite-length Inverse}

With a finite observation window of length $N$ we (surprisingly) still can have exact recovery, starting as soon as $N \geq \Omega(k\log(k))$.

\paragraph{Finite-observation phase transition}

%\newcommand{\bV}{{\bf V}}

Let 
% $\bV=\bV_k$ 
$\ell_1^k$
denote the collection of bisequences vanishing outside a centered window of radius $k$.

	\begin{theorem}[Finite observation window, finite-length inverse filter]
	\label{thm:fin_guarantee}
	Suppose $Y = \ba \star X$, where:
	\BIT
\item
$(X_t)_{t \in \integers}$ is IID  $pN(0,1) + (1-p) \delta_0$. 
 \item
$\ba\in l_1(\integers)$ has a finite-length inverse: $\ba^{-1} \in \ell_1^k$ vanishes off a centered window of length $k$.
\EIT
\item
Suppose we are given a window $(Y_t)_{t\in \cT}$ of length $N = |\cT|$. 
Solve the optimization problem:
\BEQ
 \begin{array}{ll}
 \underset{\bw\in \ell_1^k}{  \mbox{minimize} }   & \frac{1}{N}\|\bw*Y\|_{\ell_1^N}\\
 \mbox{subject to}  
& (\widetilde{\ba}* \bw)_0 =1.
\end{array}
\tag{${P}_{1}^{N,k}(\widetilde{\ba})$}
\label{P1_finite}
\EEQ

	There exist $\epsilon>0, \delta>0$, so that when the number of observations $N$ satisfies
		\[
N \geq  k\log(\frac{k}{\delta}) ( \frac{C\kappa_\ba}{\epsilon}  )^2,
\]
and the sparsity level $p$ obeys $\frac{1}{N}\leq p \leq p^\star - \delta_p(N,\epsilon)$,
		then 		with probability exceeding $1-\delta$ the solution $\bw^\star$  of  $({P}_{1}^{N,k}(\widetilde{\ba}))$ is $\ba^{-1}$ up to rescaling and time shift.
	\end{theorem}
	
 


	







	

\subsection{Main Result $3$: Stability Guarantee with Finite Length Inverse Filter}
The results so far concern the ideal setting when true inverse filter has a known length $k$ and we use $k$ to set up a correctly matched optimization problem. In practice we do not know $k$ and $k$ might even be infinite.

We can provide practical guarantees even when the inverse filter is an infinite length inverse. To develop these, we must be more technical about the situation. We assume that $\ba$ has a Z-transform having $N_{-}$ roots and $N_{+}$ poles $(s_{i})$ inside the unit circle and we construct a finite length approximation $\bw$ to  $\ba^{-1}$, in fact of length
$r(N_{-}+N_{+})$.
This approximation has error 
$\|\bw*\ba-\be_0\|_2= O(\max_i |s|_{i}^{r}  )$. 

Since the objective value $\E_I\|\bw\cdot I\|_2$ of this approximation $\bw$ is an upper bound of the optimal value of the optimization solution $\bw^\star$, we could use the objective value upper bound  to derive a upper bound for $\|\bw^\star*\ba-\be_0\|_2= O(
\max_i |s|_{i}^{r}  )$ when $p<p^\star$, where the constant of this upper bound is determined by the Bi-Lipschitz constant of the finite difference of objective $\E_I\|\bw\cdot I\|_2-\E_I\|(\be_0)\cdot I\|_2$.

\paragraph{Approximation theory for infinite length inverse filter}
\begin{theorem}[Approximation theory for infinite length inverse filter based on roots of Z-transform]
\label{thm:RootNorm}
Let the finite-length forward filter $\ba$ have a Z-transform with roots inside the unit circle, namely $s_{k}:= e^{-\rho_k + i \varphi_k }$ with $|s_k|<1$ and $\rho_k>0$
for $k \in \{-N_{-}, \ldots -1, 1, \ldots N_{+}\}$.  Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible indexes.
\[
 \begin{array}{ll}
A(z) &=  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i}
\\
&= c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1});
\end{array}
  \]
here $c_0$ is a constant ensuring $a_0=1$.

Then for a scalar $r$
% vector index $r=(r_{-N_-}, \ldots, r_{-1}, r_{1},\ldots, r_{N_+} )$
, we construct an approximate inverse filter $\bw^r$ with Z-transform
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r-1} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r-1} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r}) (1- s_{i} z^{-1})^{-1}.
\end{array}
\]
We have
\[
 \begin{array}{ll}
 \|\bw^r*\ba-\be_0\|_2^2  
 &= \sum_{n\in \{1,2,3,\ldots,|\cI| \} }\sum_{ k_1, \ldots, k_n  \in \cI } \prod_{i\in [n]}|s_{k_i}|^{2r }
\end{array}
  \]
%   Let $\gamma^m := \min_{i}\big(r_{i} |\rho_{i}| \big) =  \min\{r_{-N_-}|\rho_{-N_-}|, \ldots, r_{-1}|\rho_{-1}|, r_{1}|\rho_{1}|, \ldots, r_{N_+}|\rho_{N_+}|\}.$
as $r \rightarrow \infty$, this converges to zero at an exponential rate, determined by the slowest decaying term,
\[
 \begin{array}{ll}
\|\bw^r*\ba-\be_0\|_2
&=  O( |s|_{(1)}^{r}  ) , \quad r \rightarrow \infty.
\end{array}
  \]
  where $|s|_{(1)}$ is the largest absolute value root.
 \end{theorem}
 
% \Dave{What is $\cI$?}
 
 \paragraph{Stability for infinite length inverse filter}
 \begin{theorem}[Stability for infinite length inverse filter]
 \label{thm:bd_stab}
 Let $\ba\in V_{N_-, N_+} $ be a forward filter with all the roots of Z-transform strictly in the unit circle. Let $\bw^\star \in V_{(r-1)N_-, (r-1)N_+} $ be the solution of the convex optimization problem. Let $\bw^r$ be the constructed filter in previous theorem with a uniform vector index $(r, \ldots, r, r,\ldots, r)$.
  Then provided $p<p^\star$, as 
  $r \rightarrow \infty$, 
  \[
 \begin{array}{ll}
  \| \bw^\star*\ba -\be_0\|_2 
   \leq
    O(
 |s|_{(1)}^{r}  ), \quad r \rightarrow \infty.
\end{array}
  \]
  where $|s|_{(1)}$ is the largest absolute value root.
In words, \textbf{the Euclidean distance between $\bw^\star*\ba$ and $\be_0$ converges to zero at an exponential rate as the approximation length is allowed to increase.} 
 \end{theorem} 
 
%  \Dave{I don't understand the roots of Z transform comment. Did you think clearly about this? I think what you mean is no roots are on the unit circle, some number are inside and some number are outside. Right now it looks very doubtful.}
 
 
\subsection{Main Result $4$: Robustness Against Stochastic Noise and Adversarial Noise}
We now extend the previous analysis of an exactly sparse model of $X$, exactly observed, to the more practical setting of approximate sparsity and observation noise. We consider two cases: first we add stochastic noise as an independent Gaussian linear process, and second adversarial noise with bounded $\ell_\infty$ norm.  

In each scenario, since the noisy objective value at $\be_0$ is an upper bound on the optimal value of the optimization solution $\bw^\star$, we use this upper bound on the objective value  to derive an upper bound of $\|\bw^\star*\ba-\be_0\|_2$ when $p<p^\star$.
%, where the constant of this upper bound is determined by the Bi-Lipschitzness constant of finite difference of objective $\E_I\|\bw\cdot I\|_2-\E_I\|(\be_0)\cdot I\|_2$. 
The upper bound shows that the distance $\|\bw^\star*\ba-\be_0\|_2$ is bounded by the (appropriately measured)
magnitude of input noise in both cases.


\paragraph{Robustness under stochastic noise }
 \begin{theorem}[Robustness against Gaussian Linear Process noise]
 \label{thm:rand_exact_rob}
 We consider a Gaussian linear process $Z = \sigma \cdot \bb \star G$ where: $\sigma > 0$ denotes the noise level;   $\bb$ is
 a bisequence having  unit $\ell_2$ norm $\|\bb\|_2=1$; and $G$ is a standard Normal iid bisequence:
 \[
\begin{array}{ll}
Y&= \ba* (X+ Z).
\end{array}
\]
 
 \newcommand{\wpsi}{{\bf w}}
 Let $\wpsi^\star$ be the solution of the convex optimization problem in Eq.(4.1);
 %for the moving average random noisy model
%  \[
%\begin{array}{ll}
%Y&= \ba* (X+ \sigma \bb*G),
%\end{array}
%\]

\label{thm:Bound_Normal_Noise}
\[
 \E_I  \| (\wpsi^\star)\cdot I \|_2 -\E_I  \| (\be_0)\cdot I \|_2 \leq  (1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1).
\]
%When $\sigma\leq 1,$
%\[
%(1-p) \sigma +
% p(\sqrt{1+ \sigma^2 }-1)  \leq \sigma;
%\]
%therefore, 
When $p<p^\star$, $\sigma\leq 1$, there exists a constant $C$,
\[
  \| \bw^\star*\ba -\be_0\|_2 = \|\wpsi^\star -\be_0\|_2 \leq C \sigma.
\]
In words, \textbf{the Euclidean distance between $\bw^\star \star \ba$ and $\be_0$ is bounded linearly by the magnitude of stochastic noise}.
\end{theorem}  

\newcommand{\bc}{{\bf c}}
\paragraph{Robustness under adversarial noise }
 \begin{theorem}[Robustness under adversarial noise with $\ell_p$ norm bound]
\label{thm:adv_exact_rob}
Suppose that an adversary chooses a disturbance bisequence
$\bc$ subject to the constraint:	
\[
	\| \bc\|_\infty \leq \eta;
\]
and perturbs the observation process $Y$ via:
	\[
	\begin{array}{ll}
	Y&= \ba* (X+  \bc) .
	\end{array}
	\]
\newcommand{\apsi}{{\bf v}}
Let $\bw^\star$ denote the solution of the convex optimization problem~\ref{eqn:P1}.
Define $\apsi^\star = (\ba*\bw^\star)^{\dagger}$, then $\apsi^\star$ satisfies the following bound on objective difference:
 \[
 \begin{array}{ll}
 \E_I  \| (\apsi^\star)\cdot I \|_2 -\E_I  \| (\be_0)\cdot I \|_2 \leq 
 p\sqrt{\frac{2}{\pi}}(\mathcal{R}(\eta) - 1)+(1-p)\eta.
\end{array}
  \]  
 
Therefore, when $p<p^\star$, there exists a constant $C'$, so that
 \[
 \| \bw^\star*\ba -\be_0\|_2 = \|\apsi^\star -\be_0\|_2  \leq C'  \eta, \forall \eta > 0.
 \]
 In words, \textbf{the Euclidean distance between $\bw^\star \star \ba$ and $\be_0$ is at most proportional to the magnitude of the adversarial noise}.
 
 
\end{theorem}  

\textbf{Remark}: Here $\mathcal{R}(\eta)$
is the folded Gaussian mean, for standard Gaussian $G$:
\[
\mathcal{R}(\eta) :=  \sqrt{\frac{\pi}{2}} E_G |\eta+  G| = \exp\{-\eta^2/2\} + \sqrt{\frac{\pi}{2}}\eta \left(1 - 2\Phi\left(-\eta\right) \right).
\]  
$\mathcal{R}(\eta)-1$ is an even function that is monotonically non-decreasing for $\eta \geq 0$ with quadratic upper and lower bound: there exists constants $C_1\leq C_2$,
  \[
C_1 \eta^2 \leq \mathcal{R}(\eta)-1 \leq C_2 \eta^2, \forall \eta.
\]

\newcommand{\bu}{{\bf u}}

\subsection{Technical Preparation:  Landscape of  Expected Homogeneous Function over Bernoulli Support on Sphere}

Let 
\[
V_k(\bu) := \frac{\E_J\|\bu\cdot J\|_2^k}{\|\bu\|^k_{2}} 
\]
where $\bu\in \reals^N$, $J$ is a Bernoulli sequence indexed from $1$ to $N$.


\paragraph{Expectation $V_1(\bu):= \E_J \|\bu\cdot J\|_2^{1}$ on sphere.}



% \Dave{I would not call this functional $V$. You are already using $V$ for a subspace of bisequences. It would be better to use a greek letter like $\Psi$ or $\Lambda$.}
% \Sun{Could I keep V here and replace the previous $V_k$ in sequence vector space to $\ell_1^k$ }

% \Dave{I would not call the bernoulli object $I$ here. Elsewhere $I$ is a bisequence. Here $I$ is a vector of $N$ elements. Better to introduce $J$ for this purpose.}

\begin{theorem} \label{thm:BGPropLemmaNorm}
Let $\bu \in \reals^N$, then
\[
p \leq V_{1}(\bu) \leq V_{1}(\frac{\sum_{j\in [N]}\pm \be_j}{\sqrt{N}} ) \leq \sqrt{p} .
\]
the lower bound is approached by on-sparse vectors $\bu \in \{ \pm \be_i, i\in [N]\}$, and the upper bound is approached by 
$\bu  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm \be_j\}$.

Furthermore, all the stationary points of $V_{1}(\bu)$ are $\{\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm \be_i, i\in [N]\}$ are the global minimizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm \be_j\}$ are the global maximizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}\}$ are saddle points with value
\[
V_1(\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}) = \E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}\sqrt{\frac{j}{N_J}}.
\]
\end{theorem}
To support geometric intuition, Figure~\ref{fig-landscape-V1}
visualizes $V_1$ on the $2-$dimensional sphere.

\begin{figure} 
\includegraphics[width=.7\textwidth]{./figures_BD/Ju_landscape.png}
% \includegraphics[width=.45\textwidth]{./figures_BD/Ju_landscape_m100.png}
\caption{The value of $V_1$ on a two-dimensional sphere in $\reals^3$, normalized by the affine transform to send the value in $[0,1].$  
}
\label{fig-landscape-V1}
\end{figure}


\paragraph{Expectation $V_{2k}(\bu):= \E_J \|\bu\cdot J\|_2^{2k}$ on sphere.}
\begin{theorem} \label{thm:BGPropLemmaSub_k}
For $k\geq 2$, let $\bu$ denote a vector in $\reals^N$, then
\[
p^k \leq V_{2k}(\frac{\sum_{j\in [N]}\pm \be_j}{\sqrt{N}} ) \leq V_{2k}(\bu) \leq p.
\]
the upper bound is approached by one-sparse vectors $\bu \in \{ \pm \be_i, i\in [N]\}$, and the lower bound is approached by 
$\bu  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm \be_j\}$.

Furthermore, all the stationary points of $V_{2k}(\psi)$ are $\{\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm \be_i, i\in [N]\}$ are the set of global maximizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm \be_j\}$ are the set of all the global minimizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}\}$ are saddle points with value
\[
V_{2k}(\frac{\sum_{i\in J} \pm \be_i}{\sqrt{N_J}}) = \E_J (\frac{\sum_{i\in J} 1_{I_i}}{N_J})^k = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}(\frac{j}{N_J})^k.
\]
\end{theorem}

\paragraph{Expectation $V_{-1}(\bu):= \E_J \|\bu\cdot J\|_2^{-1}$ on sphere.}
\begin{theorem}
\label{thm:TaylorSqrtInvExpect}
\beq 
  V_{-1}(\bu) 
%   = \frac{\E_J  \| \bu \cdot J \|^{-1}_{2} }{\| \bu \|^{-1}_{2}  
%   = \E_J (1- \frac{  \| \bu \cdot ([N]-J) \|_{2}}{\| \bu \|_{2})^{-1/2}
  \geq p^{-1/2} .
\eeq
\end{theorem}



\subsection{Technical Tool: Relation between Finite Difference of Objective and Euclidean Distance }
 \paragraph{Bi-Lipschitzness of finite difference of objective}
As an important proof tool, we study functional $B$ that allows us to bound the Euclidean distance $d_2(\psi, \be_0) := \| \psi - \be_0\|_2$ by the objective difference $\E_I  \| \psi\cdot I \|_2- \E_I  \| (\be_0)\cdot I \|_2$  : 
\[
B(\be_0,\phi) := \frac{\E_I  \| (\be_0+\phi)\cdot I \|_2 - \E_I  \| (\be_0)\cdot I \|_2}{\|\phi\|_2} 
\]
When we rescale $\phi$ to $\beta:= \frac{\phi}{\|\phi \|_2}$, we have
\[
B(\be_0,t \beta) = \frac{\E_I  \| (\be_0+t \beta)\cdot I \|_2 - \E_I  \| (\be_0)\cdot I \|_2}{t} 
\]
From the definition of directional derivative,
\[
\nabla_{\phi}{\E_I  \| (\be_0+\phi)\cdot I \|_2}\mid_{\phi=0}=\lim_{t\rightarrow 0^+}\frac{\E_I  \| (\be_0+t \beta)\cdot I \|_2 - \E_I  \| (\be_0)\cdot I \|_2}{t}=\lim_{t\rightarrow 0^+}B(\be_0,t \beta).
\]

We have upper and lower bound on their difference.
This upper and lower bound allows us to connect objective $\E_I  \| \psi\cdot I \|_2$ and the $2-$norm of $ \psi - \be_0$:
\begin{theorem}[Bi-Lipschitzness of finite difference of objective near $\be_0$ for linear constraint]
\label{thm:bound_diff}
We have upper and lower bound of $B(\be_0, \phi)$ :
\BEAS
0\leq B(\be_0,t \beta) -\lim_{t\rightarrow 0^+}B(\be_0,t \beta) 
\leq 
  \frac{t}{2}p\Big( 
  \beta_0^2 
 +
 p  (1-\beta_0^2) \Big) \leq \frac{pt}{2}.
\EEAS
This leads to
\[
0 \leq B(\be_0, \phi) -	 \nabla_{\phi}{\E_I  \| (\be_0+\phi)\cdot I \|_2}\mid_{\phi=0}\leq \frac{p}{2}\|\phi \|_2.
\]
Therefore, when $p<p^\star$, $\nabla_{\phi}{\E_I  \| (\be_0+\phi)\cdot I \|_2}\geq \epsilon(p,p^\star)>0$, 
we have $B(\be_0, \phi) \geq \epsilon(p,p^\star)>0$, which allows us to bound difference of objective by Euclidean distance .
Reversely, 
$1/B(\be_0, \phi) \leq  1/\epsilon(p,p^\star)$, which allows us to bound Euclidean distance by difference of objective.

\end{theorem}



\subsection{Initialization of forward filter}
Now we study how to get the initial guess $\widetilde{\ba}$.


First, let $C_Y$ denote the circular embedding of $Y$;  we can define $\Bar{Y} = (C_Y C_Y^T)^{-1/2}Y$, then from $Y=\ba*X$, we get $C_Y = C_a C_X$, then
\[
C_{\Bar{Y}} =  (C_Y C_Y^T)^{-1/2}C_Y = (C_a C_X C_X^T  C_a^T)^{-1/2}C_a C_X
\]
as $X$ are IID Bernoulli-Gaussian, 
we know approximately 
\[
C_{\Bar{Y}} =  (C_Y C_Y^T)^{-1/2}C_Y = (C_a C_X C_X^T  C_a^T)^{-1/2}C_a C_X \approx (C_a C_a^T)^{-1/2}C_a C_X
\]
We can also define $C_{\Bar{a}}=(C_a C_a^T)^{-1/2}C_a$.

One approach is to find initialization filter one root by another. The first step is to look for a single root inverse filter $\widetilde{\bw}^{[1]} = (1, -\widetilde{s_1}) $
\[
 \begin{array}{ll}
 \underset{\widetilde{s_1} \in \reals }{\mbox{minimize}}   & -\frac{1}{N} \| (1, -\widetilde{s_1})*\Bar{Y}\|_{\ell_4(\cT_N)}^4
\end{array}
  \]
then iterate by assuming $\Bar{Y}^{[1]} = (1, -\widetilde{s_1})*\Bar{Y}$, then try to look for $\widetilde{\bw}^{[2]} = (1, -\widetilde{s_2})$ by solving
\[
 \begin{array}{ll}
 \underset{\widetilde{s_2} \in \reals }{\mbox{minimize}}   & -\frac{1}{N} \| (1, -\widetilde{s_2})*\Bar{Y}\|_{\ell_4(\cT_N)}^4
\end{array}
  \]
  
We could find the initialization by running the projected gradient method on sphere with random initialization:
\[
 \begin{array}{ll}
 \underset{\widetilde{\bw} \in l_1^k}{\mbox{minimize}}   & -\frac{1}{N} \| \widetilde{\bw}*\Bar{Y}\|_{\ell_4(\cT_N)}^4\\
\mbox{subject to}  
& \|\widetilde{\bw}\|_2 =1,
\end{array}
  \]
  We could also approximate this objective via re-weighted PCA.

With the solution of one of the non-convex optimization as $\widetilde{\bw}^\star$, we have a initial guess of sparse signal:
\[
C_{\widetilde{\bw}^\star}\Bar{Y}
\]
and we can set the initial guess of forward filter $\widetilde{\ba}$ via least square solution
\[
\widetilde{\ba} = C_{\Bar{Y}}^{+} C_{\widetilde{\bw}^\star}^{+} Y 
\]

Another popular non-convex method is alternating minimization, which finds a good approximation of the forward filter $\ba$:
\[
 \begin{array}{ll}
 \underset{\widetilde{\ba}, \bx \in l_1^N}{\mbox{minimize}}   & \frac{1}{N} (\lambda \| \bx\|_{\ell_1(\cT_N)} + \| \Bar{Y}-\widetilde{\ba}*  \bx\|_{\ell_2(\cT_N)}^2)\\
\mbox{subject to}  
& \|\widetilde{\ba}\|_2 =1,
\end{array}
  \]

\subsection{Non-convex method initialization of forward filter}

Our method is an iterative alternating minimization algorithm on convolutional dictionary learning objective.
\[
 \begin{array}{ll}
 \underset{A \in \reals^{N_1\times N times K}, X \in \reals^{N}}{\mbox{minimize}}   & \frac{1}{N} (\lambda \| \bx\|_{\ell_1(\cT_N)} + \| \Bar{Y}-A  \bx\|_{\ell_2(\cT_N)}^2)\\
\mbox{subject to}  
& A \in \mbox{Riemann manifold},
\end{array}
  \]

\subsection{Dave: using full $4$ order moments tensor to solve a system of linear equation to initialization}

Iteration of full $4$-th order momentum matching equation.


\subsection{Paper Organization}
Now we have stated the main results of our paper.
The paper is organized as follows. 
\BIT
\item
In section $1$, we introduce the blind deconvolution problems and its related works.
\item
In Section $2$, we have presented the main results of this paper.
% \item
% In Section $3$, we discuss the existence of inverse filter.
% \item
% In Section $4$, we introduce a change of variable that connects convex blind deconvolution with projection pursuit. 
\item
In Section $3$, we provide a systematic study of the landscape of the expected projection pursuit loss on sphere for linear combination of IID Bernoulli Gaussian $X$.
\item
In Section $4$, we introduce the technical backgrounds for convex blind deconvolution problem, including the existence of inverse filter, the change of variable, the definition of directional derivative and projected sub-gradient. 
\item
In Section $5$, we prove the main theorem of phase transition for convex blind deconvolution problem. 
\item
In Section $6$, we provide tight upper and lower bound of $val(Q_1)$ to compute the phase transition threshold $p^\star$. 
\item
In Section $7$. we provide upper and lower bound on the directional finite difference near $\be_0$ as a tool for the study of stability and robustness in the section $9$ and $10$.
\item
In Section $8$, we prove the finite sample observation version of the phase transition theorem and give an observation sample complexity bound $N \geq O(k\log(k))$ for a length $k$ inverse filter $a^{-1}$.
\item
In Section $9$, we prove the stability of the convex algorithm with infinite length inverse filter approximation.
\item
In Section $10$, we prove the robustness of the convex algorithm under random and adversarial  noise.
\item
In Section $11$, we give a general phase transition condition for other probabilistic models on $X$ beyond IID Bernoulli-Gaussian.
\item
In Section $12$, we conclude the paper.
\EIT



==> old_sec/sec_old/Discrete_structure.tex <==

\section{Discrete signal structure}
\paragraph{Random model for discrete digital signals.}
We define a random model for discrete digital signals. 

Let $(X_t)$ be an independent
sequence of random variable indexed by  $t \in Z$, with a symmetric distribution with CDF $F$. 
\begin{itemize}
\item The two point symmetric distribution on real number, $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$ 
\item The four point symmetric distribution on complex number, 
$F = 1/4 \delta_{1+i} + 1/4 \delta_{-1+i}+1/4 \delta_{1-i}
+1/4 \delta_{-1-i}.$ 
\item A symmetric distribution on $\reals^s$,
$F = 1/2^s( \sum_{c\in \{\pm 1\}^s} \delta_{\sum_{i\in[s]} c_i e_i } ).$ 

\item Constallantion in unit sphere.
The $2k$ point symmetric distribution on complex number, 
$F_p = \sum_{j=0}^{2k-1} p_j \delta_{\exp{(i\pi\frac{j}{k})}},$
where $\sum_{j=0}^{2k-1} p_j =1, p_j>0.$
\end{itemize}



\paragraph{Convex loss for discrete digital structure.}
The convex loss  we choose could be a relaxation of the convex indictor function of the points.

\begin{itemize}
\item For the two point symmetric distribution on real number, 
\[
g(x) = (|x|-1)_+
\]
\item The four point symmetric distribution on complex number, 
\[
g(z) = (|z|-1)_+,
\]
or more accurately,
\[
g(z) = (\|z\|_{\infty}-1)_+.
\]
\item For $s$-dimensional symmetric distribution on $\{\pm 1\}^s$,
\[
g(x) = (\|x\|_{\infty}-1)_+.
\] 
\end{itemize}


\paragraph{Blind recovery problem.}
For observation $Y$, assume that there exist inverse filter $\mu^* (e_0 + f^*)$, where $f^*_0 = 0$. We try to find it by solving a convex problem,
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E \sum g(\mu (Y+ f*Y)).
\end{eqnarray*}
First, when we know the correct scale $\mu^*$.

Let 
\[
e_0+h = ( e_0 + f)(e_0 + f^*)^{-1},
\]
we have
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E g( x_0+ h*x)).
\end{eqnarray*}
For $g(x) =(|x|-1)_+$, then the sub-gradient is
\[
g'(x) =  \left.
  \begin{cases}
    1, & \text{for } x > 1 \\
    0, & \text{for } -1 < x < 1 \\
    -1, & \text{for }-1 > x \\
    [0,1], & \text{for }x = 1  \\
    [-1,0], & \text{for }x = -1
  \end{cases}
  \right\}
\]

And the proximal operator $\mbox{prox}_{\rho g}$ is
\[
\mbox{prox}_{\rho g}(x) =  \left.
  \begin{cases}
    x-\rho, & \text{for } x > 1+\rho \\
    x, & \text{for } -1 < x < 1 \\
    x+\rho, & \text{for }-1-\rho > x \\
    1, & \text{for }1 \leq x \leq 1 +\rho \\
    -1, & \text{for } -1 -\rho\leq x \leq -1
  \end{cases}
  \right\}
\]


Assume $(X_t)$ are independent
sequence of random variable with CDF $F_{p}^t = \sum_{j=0}^{1} p^t_j \delta_{(-1)^j},$
where $\sum_{j=0}^{1} p^t_j =1, p^t_j>0.$ We choose the objective
\[
g(z) = (|z|-1)_+.
\] 
To show that $h=0$ is the global minimizer of the convex problem, we only need to show that for any $h\neq 0$, there exists small $\epsilon>0$, 
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)>0.
\end{eqnarray*}
We use sub-gradient information,
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)
    &\approx& 
    E g'( x_0)(\epsilon h*x)\\
    &=&
    \epsilon( p^0 _1 g'( +1)(h_0)+p^0_{-1}g'( -1)(-h_0)  )
    \geq 0.
\end{eqnarray*}

\paragraph{Polar form and extension to complex plane}
We can rewrite a point on the complex plane as its polar form
\[
z = r \exp{i\theta},
\]
where $r\geq 0$.

Under the polar form, the loss function is 
\[
g(z) = (|z|-1)_+ = (r-1)_+,
\]

We can reparametrize

Using this polar form, we are able to generalize our result to the complex setting.

\paragraph{Non-convex loss for discrete digital structure.}
If we are allowed to use non-convex loss, then we can fix the scale by the loss function.

Instead of convex loss
\[
g(x) = (|x|-1)_+,
\]
or
\[
g(x) = (|x|^2-1)_+,
\]
we can choose
\begin{itemize}
\item The smooth loss 
\[
g(x) = (|x|^2-1)^2,
\]
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (|x|-1)^2,
\]
\item The composition of  smooth function with convex non-smooth function,
\[
g(x) = ||x|^2-1|,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = ||x|-1|.
\]
\end{itemize}


And instead of
\[
g(x) = (\|x\|_{\infty}-1)_+,
\]
we can choose
\begin{itemize}
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (\|x\|_{\infty}-1)^2,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = |\|x\|_{\infty}-1|.
\]
\end{itemize}

\subsection{Noisy observation}
We consider the noisy recovery problem, there are two noise model, one is
\[
y = w_0 * (x+  n),
\]
the other is 
\[
y = w_0 * x+  u = w_0 * (x+ w_0^{-1} *u).
\]
When $u$ is Gaussian $N(0,\Sigma) $ , $w_0^{-1} *u$ is Gaussian $N(0,C_{w_0}^{-1}\Sigma C_{w_0}^{-1,T}) $. Therefore, we could reduce this problem as a colored noise $n$. 

\paragraph{Post-process}
For noisy observation $y$, we apply the algorithm on $y$ to get a solution $\hat x$, then we apply our prior knowledge to project the solution to the constellation points by taking $\title{x} = \mbox{sign}(\hat x).$

Then we measure the ratio of correct recovery by mean of
$1_{\title{x} = x}$ over multiple MC samples.
\paragraph{Population analysis}
Assume that the observation model are $y = w_0 * (x+  \sigma n),$ where $n$ is IID $N(0,1)$. Then we analyze the population risk,
 \begin{eqnarray*}
    \min_{h_0 = 0} &    
     E_x E_n g( x_0+ \sigma n_0+ h^T (x+\sigma n) ).
\end{eqnarray*}
Here $g(x) =(|x|-1)_+$.

Assume that the optimal solution is $h^*_\sigma$, when $\sigma = 0$ we proved before that $h^*=0.$ Here we get
$\hat x_0 = x_0+ \sigma n_0+ h^{*,T} (x+\sigma n) $
want to prove
\[
\tilde x_0 = \mbox{sign}(x_0+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n) ) = x_0,
\]
when $\sigma<\sigma_{m}$.
Without loss of generality, we assume $x_0=1$, we want to ask that when would $1+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n)\leq 0$, in general, the condition we need to charaterize is when 
$ |\sigma n_0+ h_\sigma^{*,T} (x+\sigma n)|\leq 1$.

\paragraph{Huber version of loss}
Instead of using $g(x) =(|x|-1)_+$, when there are Gaussian noise on $x$, we can use the Huber version 
\[
g_{\mu}(x) =\min_z  \frac{\mu}{2}\|x-z\|^2_2+ (|z|-1)_+  .
\]
% \section{Numerical results}
% \subsection{Convex loss}
% For observation $Y\in \reals^{2N+1}$,  assume that there exist inverse filter $w^* = \mu^* (e_0 + f^*)$, where $f^*_0 = 0$, such that $w^* *Y=X$ is IID distributed by $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$  Let
% \[
% g(x) = (\|x\|_{\infty}-1)_+,
% \]
% we try to find it by solving a convex problem,
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2k+1}} &    
%      \sum g(\mu (Y+ f*Y)).
% \end{eqnarray*}
% And we also solve 
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2N+1}} &    
%      \sum g(\mu (Y+ f*Y))+\lambda \|f\|_1.
% \end{eqnarray*}

% In the following, we assume $\mu^* =1$ WOLG.

% We select $\mu$ in algorithmically by a line search over different choices.

% And the criteria to select is to look at the non-convex loss, say 
% \[
% h(x) = ||x|^2-1|^2,
% \]
% or its gradient. When $g$ or $g'$ is zero, then we know we selected the right scale.

% % \begin{algorithm}
% %   \caption{\textbf{Deconvolution t}}
% %   \label{alg:AA}
% % \begin{algorithmic}[1]
% %   \State {\bfseries Input:} initial point $x_0$, operator $F(\cdot)$, memory $m$
% %   \For{$k=1, 2, \dots$}
% %   \State $m_k=\min\{m, k\}$
% %   \State $\alpha^k$ determined by either the type $1$ or the type $2$ formula above.
% %   \State $x_{k+1} =   \alpha^{k,T}(X^k - \beta_k G_{k})$.
% %   \EndFor
% % \end{algorithmic}
% % \end{algorithm}

% Here is the matlab code,
% \begin{verbatim}
% % % Param
% T = 100;
% n_left = T;
% n_right = T;
% lam = 1e1;
% mu = 1e2;
% k_0 = 10;
% k_1 = 10; 
% k_2 = 100; 
% k_4 = 10;

% scale = 1.;
% % MAX_ITER = 1e1;
% % STEP_SIZE = 1e-4;
% % STEP_MIN = 1e-5;
% % GRAD_TOL = 1e-8;
% % mem_size= 10;
% % beta = 0.5;
% % EPS = 1e-2?;

% % % Set up
% n = n_left+n_right+1;
% delta = [zeros(n_left,1);1; zeros(n_right,1)];

% % % % Model
% % Create x

% % x0 = x0.*randn(n, 1);
% x0 = sign(randn(n, 1));
% % x0_mat = circulant(x0,1);
% J_1 = (x0 > 0);
% J_2 = (x0 < 0);



% % Create forward and inverse filter
% % inverse
% t = 0.1;
% w0_left =[t];
% for j=2:1:k_0
%     w0_left(j,1) =t^j;
% end
% % p1= 0.4;
% % w0_left = t*(rand(k_0, 1) < p1);

% w0 = [zeros(k_0,1);1; -w0_left ];
% w_pad =  [zeros(n_left-k_0,1); w0 ; zeros(n_right-k_0,1)];
% J_w = (max(1,n_left-2*k_0-2):min(2*T,n_left+2*k_0+2));
% % forward
% a0 = ifft(1./fft(w_pad,n),n);
% a_shift = circshift(a0,T);

% % % Property
% % Cos
% cos = norm(w_pad ,inf)/norm(w_pad ,2);
% % Correlation
% w0_mat =  circulant(w0,1);
% w_flip = w0_mat(1,:)';
% R_w = conv(w0, w_flip);

% % Y observation
% y = cconv(a0, x0, n); 
% y_mat =  circulant(y,1);



% cost = @(z) sum(((z).^2-1).^2); 
% grad = @(z) 2*sum(((z).^2-1).*(2*z)); 


% % % % Algorithm compare

% % % Algorithm1
% % %	Exact problem
% % 

% y_mtruc = y_mat(1:n,1:2*k_1+1);
% cvx_begin quiet
% cvx_solver mosek
%   variable w_1(2*k_1+1),
%   minimize( sum(pos(abs(scale*y_mtruc*w_1)-1)))
%   subject to
%       w_1(1+k_1) ==1
% cvx_end

% w_1pad = [zeros(n_left-k_1,1);w_1; zeros( n_right-k_1,1)];
% x_1 = cconv(w_1pad, y, n); 
% delta_1 = cconv(w_1pad,a_shift,n);
% c1 = cost(x_1);
% g1 = grad(x_1);
% % % Algorithm2
% % %	Regularized problem

% y_mtruc2 = y_mat(1:n,1:2*k_2+1);

% cvx_begin quiet
% cvx_solver mosek
%   variable w_2(2*k_2+1),
%   minimize(  sum(pos(abs(scale*y_mtruc2*w_2)-1))+lam* norm(w_2,1))
%   subject to
%       w_2(1+k_2) ==1
% cvx_end

% w_2pad = [zeros(n_left-k_2,1);w_2; zeros( n_right-k_2,1)];
% x_2 = cconv(w_2pad, y, n); 
% delta_2 = cconv(w_2pad,a_shift,n);
% c2 = cost(x_2);
% g2 = grad(x_2);
% \end{verbatim}


==> old_sec/sec_old/Expectation.tex <==
\section{Expectation calculation}
\subsection{Expectation over Bernoulli support}

We previously considered the identity
\beq \label{eq:startingPoint}
    \E | \sum_{i \in \cT}  \psi_i X_i | = \sqrt{\frac{2}{\pi}} \cdot \E_I \| \psi \|_{\ell_2(I)},
\eeq
where $X$ is a Bernoulli-Gaussian RV $BG(p;0,1)$,
and where $I$ is a random subset of the domain $\cT$
determined by Bernoulli-$p$ coin tossing.

% (Qingyun:)
% First of all, we know that 
% \[
% \E_I \| \psi \|^{s}_{\ell_2(I)} \leq \| \psi \|^s_{\ell_2(T)}
% \]
% for any $s \in \integers$.

% Because $$


This leads us to consider
\[
  \E_I \| \psi \|_{\ell_2(I)}^{2k}
 \]
 where $I$ is again a random subset, and $k \geq 1$ is an integer.
 The following lemma shows that $\E_I \| \psi \|_{\ell_2(I)}^{2k} \approx \| \psi \|_{\ell_2(\cT)}^{2k}$.

\begin{lemma} \label{lem:BGPropLemmaSub}
Let $\psi$ denote a vector in $\reals^N$.
\[
 \| \psi\|_2^{2k} \cdot \bar{B}(k-1;n,p)    \leq \E_I  \| \psi \|_{\ell_2(I)}^{2k}  \leq     \| \psi\|_2^{2k} ,
\]
where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
is the survivor function (Complementary CDF) of the Binomial.
\end{lemma}

In particular, if $k \leq n \cdot p - 3 \cdot \sqrt{np (1-p)}$ for large $n$, then $\bar{B}(k-1;n,p) > 0.99$.
 The following lemma infers from this that $\E_I \| \psi \|_{\ell_2(I)} \approx \| \psi \|_{\ell_2(\cT)}$.
 
\begin{lemma} \label{lem:BGPropLemmaNorm}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$ as $\eps_N$ could be quite large!}


There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
and so that for each $N$ and for each 
vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
\beq \label{eq:LemmConclu}
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\eeq
\end{lemma}
Applying (\ref{eq:startingPoint}), we get:
\begin{coro} \label{lem:BGPropLemma}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$!}
There exists a sequence $(\eps_N)$ depending only on $N$, so that  $\eps_N \goto 0$ and
and so that for each $N$ and for each 
vector $\psi$in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$.
\[
(1 - \eps_N) \cdot (1-N^{-1}) \leq  \frac{E | \sum_{i \in \cT}  \psi_i X_i |}{\sqrt{\frac{2}{\pi}}  \| \psi \|_{\ell_2(\cT)}}  \leq   ( 1 + \eps_N).
\]
% and
% \[
% E | \sum_{i \in \cT}  \psi_i X_i |  \geq  (1 - \eps_N) \cdot (1-N^{-1}) \cdot \sqrt{\frac{2}{\pi}} \cdot E \| \psi \|_{\ell_2(\cT)} .
% \]
\end{coro}


\subsection{Proof of Lemma \ref{lem:BGPropLemmaSub}}

\begin{proof}[Proof of Lemma \ref{lem:BGPropLemmaSub}]
Let's first suppose that $|\psi_t| \geq \eps > 0$ for $-T \leq t \leq T$. Let $N = 2T+1$, and
let $I$ denote a subset of indices in $ \cT = \{-T,\dots,T\}$ and
let $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|}$. 
\begin{eqnarray*}
\E_I  \| \psi \|_{\ell_2(I)}^{2k}  &=&  \sum_{n=1}^{N}  \sum_{ |I |=n} \pi(I)   \| \psi \|_{\ell_2(I)}^{2k} \\
% &=& 
%   \sum_{I \subset \cT} \pi(I)    \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&   \sum_{n=1}^{N}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k}  \\
   \end{eqnarray*}
where we used $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|} $.
We partition the sum  $\sum_{n=1}^{N} = \sum_{n=1}^{k-1} + \sum_{k}^N =  \sum_{n<k} + \sum_{n\geq k}$, say.
Now from $\#\{ |I|\leq n\} = {N \choose n}$ and $ \| \psi \|_{\ell_2(I)} \leq \| \psi \|_{\ell_2(\cT)}$,
\begin{eqnarray*}
 \sum_{n<k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
     &\leq&   \left( \sum_{n=1}^{k-1} (1-p)^n p^{N-n} {N \choose n} \right) \cdot  \left( \| \psi \|_{\ell_2}^{2k} \right) \\
     &=& B(k-1;n,p) \cdot   \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
where $B(x;n,p)$ denotes the cumulative distribution function of the binomial distribution.
For the sum $\sum_{n\geq k}$, we may write $\sum_{|I|=n} = {N \choose n}  \cdot Ave_{|I| = n}$
and $\sum_{t_1,\dots, t_k \in I} =  {n^k} \cdot  Ave_{t_1,\dots, t_k \in I}$, so
\begin{eqnarray*}
 \sum_{|I| = n}  \| \psi \|_{\ell_2(I)}^{2k} &=& \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2 \\
& =& {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2 \\
&=& {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot \sum_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot  \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
because the inner two averages  cover the $ {N \choose n} n^k$ terms in a uniform way.
We arrive at 
% \clearpage
 \begin{eqnarray*}
 \sum_{n\geq k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
  &=&     \| \psi \|_{\ell_2}^{2k} \cdot  \left( \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} \right) \\
  &=&    \| \psi \|_{\ell_2}^{2k} \cdot \bar{B}(k-1;n,p) .
 \end{eqnarray*} 
Here $\bar{B}(x;n,p) = 1- B(x;n,p)$ denotes the 
survivor function (complementary distribution function) of the binomial distribution.
We obtain:
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  
  & = &  \left( \sum_{n \geq k} + \sum_{n<k}   \right) \sum_{|I|=n}  \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k} \\
 &\leq &    \|\psi\|_2^{2k} \cdot  \left( \bar{B}(k-1;p,n)  + B(k-1;p,n) \right) \\
 & = &  \|\psi\|_2^{2k} .
 \end{eqnarray*}
 while
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}   & \geq & \sum_{n \geq k} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  \\
 &= &    \|\psi\|_2^{2k} \cdot \bar{B}(k-1;p,n) .
  \end{eqnarray*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:BGPropLemmaNorm}}

\begin{proof}
Fix $A > 0$ and $p \in (0,1)$
By the Weierstrass approximation theorem, we may find a sequence of polynomials $S_K(t) = \sum_{k=0}^{K} c_k t^k$
so that
\[
    | \sqrt{x} - S_K(x) |_{L^\infty([0,A])} \leq \eps_K, \quad \mbox { and } \eps_K \goto 0 \mbox{ as } K \goto \infty.
\]
Pick a sequence $(K_N)$ so that $K_N \goto \infty$ while
$K_N < N \cdot p -  \sqrt{2 \log(N) \sqrt{N} p (1-p)} $ and
\[
\bar{B}(K_N-1; n,p) > 1 - N^{-1}.
\]
Relabel $S_N  \equiv S_{K_N}$ and $\eps_N \equiv \eps_{K_N} $.
Then $\eps_N \goto 0$ as $N \goto \infty$.

Fix $N$. For each $I \subset \cT$,
let  $x_I \equiv \E_I \| \psi \|_{\ell_2(I)}^{2}$.  Then
\[
     E _I \| \psi \|_{\ell_2(I)} = \E_I \sqrt{\| \psi \|_{\ell_2(I)}^2} = \E_I \sqrt{ x_I }.
\]
while
\[
     E _I \| \psi \|_{\ell_2(I)}^{2k} = \E_I  x_I^k.
\]
Invoking our earlier lemma,
\[
 \bar{B}(k-1;n,p) \leq  \frac{\E_I  x_I^k}{\| \psi \|_{\ell_2(\cT)}^{2k}} \leq 1.
\]

Armed with  polynomial $S_N$ of degree $K_N$, consider
\begin{eqnarray*}
     \E_I S_{N}( x_I ) &=& \E_I \sum_{k=1}^{K_N} c_k x_I^{k}\\
     &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\leq& \sum_{k=1}^{K_N} c_k   \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& S_{N}( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\leq& ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} + \eps_{N} . 
\end{eqnarray*}
where we used $\E_I x_I^{k} \leq  \| \psi \|_{\ell_2(\cT)}^{2k}$ from the previous Lemma.
Similarly,
\begin{eqnarray*}
     \E_I S_N( x_I )   &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\geq& \sum_{k=1}^{K_N} c_k   \cdot \bar{B}(k-1; n,p) \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &\geq& \bar{B}(K_N-1; n,p) \cdot \sum_{k=1}^{K} c_k   \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& \bar{B}(K_N-1; n,p)  \cdot S_K( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\geq&  \bar{B}(K_N-1; n,p)  \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  \\
   &\geq&  (1- N^{-1}) \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  . 
\end{eqnarray*}
Here  we used $\E_I x_I^{k} \geq  \| \psi \|_{\ell_2(\cT)}^{2k} \cdot \bar{B}(k-1;n,p)$ from the previous Lemma.
We also used the monotonicity 
of the survivor function $\bar{B}(x) \geq \bar{B}(x+1)$.
We obtain (\ref{eq:LemmConclu}):
\[
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\]
\end{proof}


We define the functional  $\Gamma: \psi  \mapsto \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$,
from the previous calculation we know $\Gamma(\psi) $ is only a function of $\| \psi\|_0$. 
So we can identify  $\Gamma(\psi) $ as  $\Gamma(\| \psi\|_0)$. 





\subsection{Sharper bounds on $\frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$}




\begin{lemma}
\label{TaylorSqrt}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{1/2}
=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{1/2}
=\sum_{\ell=0}^\infty\binom{1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{1/2}{\ell}
&=\frac{\frac12(\frac12-1)(\frac12-2)\cdots(\frac12-\ell+1)}{\ell!}\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-3)\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}\frac{(2\ell-2)!}{2^{\ell-1}(\ell-1)!}\\
&=\frac{(-1)^{\ell-1}}{\ell2^{2\ell-1}}\binom{2\ell-2}{\ell-1}
\end{align}
then
\begin{align}
(1-x)^{1/2}
&=1-\sum_{\ell=1}^\infty\frac2\ell\binom{2\ell-2}{\ell-1}\left(\frac x4\right)^\ell\\
&=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}





% leveraging the 
%  Taylor series of $\sqrt{x}$ around any $a>0$:
%  \[
%  \sqrt{x} = \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {{a}^{\frac{1}{2}-n} \left( x-a\right)^{n}}{\Gamma\left( \frac{3}{2}-n \right)n! }}.
%  \]
%  We could apply the  Taylor series expansion around $1$ to  $\frac{ \| \psi \|_{\ell_2(I)}}{\| \psi \|_{\ell_2(T)}}$,
%  \begin{eqnarray*}
%   \sqrt{\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}} 
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}-1\right)^{n}\\
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \sum_{i=0}^n 
%  {n \choose i} (\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}})^i (-1)^{n-i}\right)
%  \end{eqnarray*}

\end{proof}

\begin{lemma}
\beq 
0 \leq 1- Q(N, p)\leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 .
\eeq
where 
\[
Q(N, p) := \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p),
\]
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|_{\ell_2(J)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(J)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq 1 .
\eeq
Therefore, 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ \frac{ \| \psi \|^2_{\ell_2(I)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq \E_I 1 = 1 .
\eeq

On the other hand, let 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}}}  .
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.

Applying Lemma \ref{TaylorSqrt},
\begin{align}
(1-\rho_J)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\rho_J^{\ell+1}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_I)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell;n,1-p)    \leq \E_I \rho_I^{\ell+1} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}\\
&\geq  1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1- \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
&= 1- Q(N, p)
\end{align}
% {\bf NOTE: I am not getting the inequality $Q(N,P) \leq N^{-1}$.
% See Below.}
{\bf Qingyun NOTE: I observe numerically that $Q(N,p)$ could be between $0$ and $1$ in a wide range, and $Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$, with $Q(N,1) = 0$, $\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$
.}
\end{proof}

\paragraph{Beta function and $Q(N,p)$}
If we define the complete beta function as 
\[
\Beta(a,b) := \int_0^1 t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then
% \[
% \Beta(x,y)=\frac{\Gamma(x)\,\Gamma(y)}{\Gamma(x+y)}
% \]
% therefore,
\[
\binom{n}{k} = \frac{1}{(n+1) \Beta(n-k+1, k+1)}
\]
the incomplete beta function as
\[
\Beta(x;\,a,b) = \int_0^x t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then the regularized incomplete beta function is defined in terms of the incomplete beta function and the complete beta function:
\[
I_x(a,b) = \frac{\Beta(x;\,a,b)}{\Beta(a,b)}.
\]
then
\[
I_p(k,N-k-1)= \bar{B}(k-1;N,p) = \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}
\]
and
\[
I_{1-p}(k+1, N-k) = 1 - I_p(N-k, k+1) = \bar{B}(k;N,1-p).
\]
Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$, from the classical De Moivre–Laplace theorem on normal approximation to the binomial, 
\[
{N \choose k}\, p^k q^{N-k} \approx \frac{1}{\sqrt{2 \pi Np(1-p)}}\,e^{-\frac{(k-Np)^2}{2Np(1-p)}}
\]
therefore, 
\[
I_{1-p}(\ell+1, N-\ell) = \bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;

\BEAS
Q(N,p) 
&\equiv& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&=& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1} \frac{1}{(2\ell+1) \Beta(\ell+1, \ell+1)}  I_{1-p}(\ell+1, N-\ell)\\
&\approx& \sum_{\ell=0}^N\frac{1}{2(\ell+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{-\frac{(\ell-\frac{N}{2})^2}{\frac{N}{2}}}  \bar{\Phi}( (\ell - N \cdot (1-p))/\sqrt{N \cdot p \cdot (1-p)} )\\
&\approx& \int_0^1 \frac{1}{2(Nt+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{- 2N(t-\frac{1}{2})^2}  \bar{\Phi}( \frac{\sqrt{N}(t - (1-p))}{\sqrt{ p \cdot (1-p)}} ) \,dt
\EEAS

Numerically, we can see that the first term in the sum is always $0.5.$
Also we know that by definition $Q(N, 1) = 1$ for any $N$.
From numerically calculation we guess that
$Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$.
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
$\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$


\begin{lemma}
Define:
\[
Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
\]
Then, 
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
\[
\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.
\]
\end{lemma}


% \begin{lemma}
% Define:
% \[
% Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
% \]
% Then, as $N \rightarrow \infty$ with $p$ fixed:
% \[
% Q(N,p)  \approx O(N^{-1/2}).
% \]
% \end{lemma}
\begin{proof}
The first term in the sum is $0.5$.

(Sketch). 
{\bf The sum has the lower bound $Q \geq 1/10$ just by inspecting
the first 10 terms (say), which are all positive and all greater
than $0.01$ (say). The following argument shows that later terms
add up to at least $\Omega(N^{-1/2})$.}
First, we know that
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]

Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$ 
\[
\bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;
this is the classical De Moivre theorem on normal approximation to the binomial. It can be made precise in many ways
that have been well documented over the centuries.
Roughly speaking, in terms of variable $z = (\ell - \mu)/\sigma$,
we have
\[
\bar{B}(\ell;N,1-p)  \approx \left \{ \begin{array}{ll}
1 & z < 3 \\
0 & z > 3 .
\end{array}
\right .
\]

Hence, defining for $m = \mu - 3 \sigma$
\[
\bar{B}(\ell;N,1-p) \approx 1, \mbox{ for } \ell \leq m.
\]
Now of course
\begin{eqnarray*}
Q(N,p) &\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} .
\end{eqnarray*}
Now from DeMoivre's theorem (case $p=1/2$, $N=2\ell$) we also know that
\[
    2^{-2\ell} { 2 \ell \choose \ell} = bin(\ell; 2 \ell, 1/2) \sim \sqrt{\frac{1}{\ell \cdot \pi}},
\]
where $bin(k;N,p)$ is the usual binomial probability mass function.
We obtain
\[
  \sum_{\ell=0}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2} \geq 
  \sum_{\ell=m/2}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2}  \geq 
  Const  \cdot m^{-1/2}
\]

\end{proof}





\subsection{Bounds on $\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}$}
\begin{lemma}
\label{TaylorSqrtInv}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(x\right)^{\ell}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\binom{-1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{-1/2}{\ell}(-1)^\ell
&=\frac{-\frac12(-\frac12-1)(-\frac12-2)\cdots(-\frac12-\ell+1)}{\ell!}\\
&=\frac{1}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-1)\\
&=\frac{1}{2^\ell\ell!}\frac{(2\ell)!}{2^{\ell}(\ell)!}\\
&=\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}
\end{align}
\end{proof}

\begin{lemma}
\label{TaylorSqrtInvExpect}
\beq 
1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p) \geq  \frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} \geq 1 .
\eeq
where 
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|^{-1}_{\ell_2(J)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(\cT)} }{\| \psi \|^2_{\ell_2(J)}}} \geq 1 .
\eeq
Therefore, 
\beq 
\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}  
 \geq   1 .
\eeq

On the other hand, let 
\beq 
\E_I (\frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} )^{-1}
 = \E_I ( 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}})^{-1/2}.
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.


\begin{align}
(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(\rho_J\right)^{\ell}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell-1;n,1-p)    \leq \E_I \rho_I^{\ell} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\\
&\geq  \sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)
\end{align}

\end{proof}





\subsection{Numerically calculate $\E_I  \| \psi_I \|_2/\| \psi \|_2$}

We numerically compute $Q(N,p)$, the result is in the following table. Compare the table with the tables of MC approximation, we see that our previous bound is still too loose.
\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{$Q(N,p)$} \\
\hline
  $p=$ &0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0.9439 & 0.9406 & 0.9370 & 0.920  & 0.8172 & 0.3358 & 0.0482 & 0 \\
\hline
$N=500$ & 0.9748  & 0.9734 & 0.9718 & 0.9643 & 0.9199 & 0.7302 & 0.209 & 0 \\
\hline      
\end{tabular}
\label{Q_table}
\end{table}

Then we use MC approximation to calculate $\E_I  \| \psi_I \|_2/\|  \psi \|_2$ for a few different $\psi.$
We will know that
\BIT
\item 
When $\psi = e_0$,  $\E_I  \| (e_0)_I \|_2=p$ 

\item
When $\psi = e_0+e_1$,  
\[
\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2 = \sqrt{\frac12} \E_I  \| (e_0+e_1)_I \|_2 = 
\E_I \sqrt{\frac{\sum_{i=\{0,1\}} I_i}{2}}=p^2+ 2p(1-p)\sqrt{\frac12}
\]
\item
We know that when $\psi = a =(1,\ldots,1)$, then
\[
\E_I  \| a_I \|_2/\| a \|_2=\E_I \sqrt{\frac{\sum_{i=[N]} I_i}{N}} 
\]
Using law of large numbers, 
\[
\lim_{N\rightarrow \infty }\sqrt{\frac{\sum_{i=[N]} I_i}{N}}  = \sqrt{p}.
\]
\item
For fixed support $J$, we can choose $\psi = \sum_{i\in J} e_i,$ then $\| \psi_J \|_2/\|  \psi \|_2 =1.$
However, the expectation is not going to be one. Let $M := |J|,$
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} = \sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}\leq \sqrt{p}
\]
The inequality can be seeing using central limit theorem, we have normal approximation  $\frac{\sum_{i\in J} I_i}{|J|} \sim N(p,  \frac{p(1-p)}{\sqrt{|J|}})$, then using Jensen's inequality, since square root fucntion is concave,
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} \approx \E_G\sqrt{p+ \frac{p(1-p)}{\sqrt{|J|}}G}  \leq \sqrt{\E_G[p+ \frac{p(1-p)}{\sqrt{|J|}}G]} =\sqrt{p} 
\]
\EIT
Using symmetry, we guess that the maximum value of $\E_I  \| \psi_I \|_2/\|  \psi \|_2$  is $\sqrt{p}$ instead of $1$, and the maximum value is achieved when $\psi$ is dense.

\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \| a_I \|_2/\| a \|_2$ where $a=(1,\ldots,1)$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0 & 0.3123 & 0.4460 & 0.7063  & 0.94865 & 0.9950 & 0.9995 & 1 \\
\hline
$N=500$ &0 &0.3153  & 0.4464 & 0.7068 & 0.94874 & 0.9950 & 0.9995 & 1\\
\hline      
\end{tabular}
\label{allone_table}
\end{table}


\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=500$ & 0 &0.1375 &	0.2667 &	0.6034 &	0.9365 &	0.9946 &	0.9994 & 1 \\
\hline      
\end{tabular}
\label{coordinatevector_table}
\end{table}



\subsection{Tight bound and stationary points of $\E_I  \| \psi_I \|_2/\| \psi \|_2$}
\begin{lemma}
\beq 
p \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq \sqrt{p}  .
\eeq
where the lower bound is achieved by $1-$sparse vectors $\pm e_i$, the upper bound is achieve by $\{\frac{\sum_{i\in \cT} \pm e_i}{\sqrt{N}}\}$.
Furthermore, all the stationary points of this objective are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ for different support $J\subset \cT$. 
\end{lemma}
\begin{proof}
This problem can be reformulate as the projection pursuit with sphere constraint,
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
Then from \cite{bai2018subgradient} Proposition $3.3$, we get the result. 

The main idea of the proof is to calculate the projected gradient
for $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$, when $|J| = M,$
\[
e_j^T  \E_I  \partial\| q_I \|_2 = q_j [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] 
\]
so
\[
(I-q q^T)  \E_I  \partial\| q_I \|_2 = [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q-[\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q = 0.
\]
then $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ is stationary points.
 
The other direction (all other points are not stationary) is implied by (the proof of) theorem $3.4$ in  \cite{bai2018subgradient}.
\end{proof}

==> old_sec/sec_old/Expectation_Updated.tex <==
\section{Expectation calculation}
\subsection{Expectation over Bernoulli support}

We previously considered the identity
\beq \label{eq:startingPoint}
    \E | \sum_{i \in \cT}  \psi_i X_i | = \sqrt{\frac{2}{\pi}} \cdot \E_I \| \psi \|_{\ell_2(I)},
\eeq
where $X$ is a Bernoulli-Gaussian RV $BG(p;0,1)$,
and where $I$ is a random subset of the domain $\cT$
determined by Bernoulli-$p$ coin tossing.

% Comment:
Let $J \subset \cT$ be the support of $X$, where $  N:=|\cT|$, $N_J:=|J|$. Let $\psi_J : = \psi\cdot 1_J$ denote the entrywise product of vector $\psi$ with the indicator vector of subset $J$. Then  we can consider our problem on the space $\cT$ by default, and rewrite for simplicity
\[
\| \psi_J \|_{2} : = \| \psi_J \|_{\ell_2(\cT)} = \| \psi \|_{\ell_2(J)}
\]

This leads us to consider the following ratio:
\[
  V^J_k(\psi) := \frac{\| \psi \|_{\ell_2(J)}^{k}}{\| \psi \|_{\ell_2(\cT)}^{k}}
 \]
 and its expectation over all Bernoulli random subset,
\[
  V_k(\psi) := \frac{\E_I \| \psi \|_{\ell_2(I)}^{k}}{\| \psi \|_{\ell_2(\cT)}^{k}}
 \]
 where $I$ is again a random subset.
%  The following lemma shows that $\E_I \| \psi \|_{\ell_2(I)}^{2k} \approx \| \psi \|_{\ell_2(\cT)}^{2k}$.
We remark that lower bound of $V_k(\psi)$ is the optimal value of the optimization problem:
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|^k_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
and the upper bound of $V_k(\psi)$ is the optimal value of the optimization problem
 \begin{eqnarray*}
    \max&   \E_I  \| \psi_I \|^k_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}




\begin{lemma} \label{lem:BGPropLemmaSub_fix}
Let $\psi$ denote a vector in $\reals^N$. For fixed support $J\subset [N]$ then for any $k\neq 0$, the deterministic quantity $V^J_{k}(\psi)$ satistfies
\[
0 \leq V^J_{k}(\psi) \leq 1.
\]
The upper bound is approached by the vectors $\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in J}\pm e_j\}$, where  $\| \psi_J \|_2^k/\|  \psi \|_2^k =1$,
 and the lower bound is approached by 
any $\psi$ that has all of its entries on $J$ to be zero.
\end{lemma}

\begin{lemma} \label{lem:BGPropLemmaSub_2}
Let $\psi$ denote a vector in $\reals^N$.
\[
V_2(\psi) =   p.
\]
\end{lemma}



\begin{theorem} \label{thm:BGPropLemmaNorm}
Let $\psi$ denote a vector in $\reals^N$, then
\[
p \leq V_{1}(\psi) \leq V_{1}(\frac{\sum_{j\in [N]}\pm e_j}{\sqrt{N}} ) \leq \sqrt{p} .
\]
the lower bound is approached by on-sparse vectors $\psi \in \{ \pm e_i, i\in [N]\}$, and the upper bound is approached by 
$\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$.

Furthermore, all the stationary points of $V_{1}(\psi)$ are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm e_i, i\in [N]\}$ are the set of global minimizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$ are the set of all the global maximizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ are saddles points with value
\[
V_1(\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}) = \E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}\sqrt{\frac{j}{N_J}}.
\]
\end{theorem}
Remark:
Specifically,
\[
V_1( e_i) = p.
\]
\[
V_1(\frac{ e_i+e_j}{\sqrt{2}}) = p(\sqrt{2}+(1-\sqrt{2}p)).
\]



\begin{theorem} \label{thm:BGPropLemmaSub_k}
For $k\geq 2$, let $\psi$ denote a vector in $\reals^N$, then
\[
p^k \leq V_{2k}(\frac{\sum_{j\in [N]}\pm e_j}{\sqrt{N}} ) \leq V_{2k}(\psi) \leq p.
\]
the upper bound is approached by on-sparse vectors $\psi \in \{ \pm e_i, i\in [N]\}$, and the lower bound is approached by 
$\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$.

Furthermore, all the stationary points of $V_{2k}(\psi)$ are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm e_i, i\in [N]\}$ are the set of global maximizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$ are the set of all the global minimizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ are saddles points with value
\[
V_{2k}(\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}) = \E_I (\frac{\sum_{i\in J} 1_{I_i}}{N_J})^k = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}(\frac{j}{N_J})^k.
\]
\end{theorem}







\paragraph{Tight bound on $V_1$ and $V_{2k}$ using mean and variance of $\frac{\sum_{i\in J} 1_{I_i}}{N_J}$}

Now notice that 
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} 
\]
has mean $p$ variance $\frac{p(1-p)}{N_J}$.
We could define a mean zero unit variance random variable $g^J$ as a function of $\{1_{I_i}\mid i\in J\}$ 
\[
g^J := \left(\frac{\sum_{i\in J} 1_{I_i}}{N_J}-p\right)/ \left( \sqrt{\frac{p(1-p)}{N_J}} \right)
\]
namely, $\E_I \left( g^I\right)=0, \E_I \left( g^I\right)^{2}=1$.
then
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} := p + \sqrt{\frac{p(1-p)}{N_J}} g^J = p(1 + \sqrt{\frac{1-p}{p N_J}} g^J)
\]
then
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \E_I\sqrt{p- \sqrt{\frac{p(1-p)}{N_J}}g^I} 
= \sqrt{p} \E_I\sqrt{1+ \sqrt{\frac{1-p}{pN_J}}g^I}  
\]
\[
\E_I \left(\frac{\sum_{i\in J} 1_{I_i}}{N_J}\right)^k 
= p^k \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^k 
\]
\begin{lemma}
\label{TaylorSqrt}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{1/2}
=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{lemma}

\begin{lemma}[Taylor expansion for $V_1$]
\label{TaylorSqrt_Expect}
and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
\BEAS
\frac{1}{\sqrt{p}}\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} 
&=& \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^{1/2} \\
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_I \left( g^I\right)^{\ell+1}\\
&=& 1- 2^{-3}({\frac{1-p}{pN_J}}) +O\left( ({\frac{1-p}{pN_J}})^2 \right)
\EEAS
\end{lemma}

\begin{lemma}[Taylor expansion for $V_{2k}$]
\label{TaylorSqrt_Expect_k}
and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
\BEAS
\frac{1}{p^k}\E_I ({\frac{\sum_{i\in J} 1_{I_i}}{N_J}})^k  
&=& \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^{k} \\
&=& 1 +\sum_{\ell=1}^{k} \binom{k}{\ell} ({\frac{1-p}{pN_J}})^{\ell/2} \E_I (g^I)^{\ell}\\
&=& 1 + \frac{k(k-1)}{2} ({\frac{1-p}{pN_J}}) +O\left( ({\frac{1-p}{pN_J}})^2 \right)
\EEAS
\end{lemma}
Therefore, we know what when $N_J>>1$, 
$V_1(\frac{\sum_{i\in J} 1_{I_i}}{N_J})$ is close to its upper bound $\sqrt{p}$, 
and for $k\geq 2$, 
$V_k(\frac{\sum_{i\in J} 1_{I_i}}{N_J})$ is close to its lower bound $p^k$ namely 
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} \approx \sqrt{p}
\]
\[
\E_I (\frac{\sum_{i\in J} 1_{I_i}}{N_J})^k \approx p^k
\]

% Using central limit theorem, when $N_J\rightarrow \infty$,
% \[
% \frac{\sum_{i\in J} 1_{I_i}}{N_J} \sim N(p,  \frac{p(1-p)}{N_J})
% \]
% we can further calculate the asymptotic using moments of Gaussian.
% \begin{lemma}[Taylor expansion and Gaussian approximation for $V_1$]
% \label{TaylorSqrt_Expect}
% and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
% \BEAS
% \frac{1}{\sqrt{p}}\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} 
% &\approx&  \E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G} \\
% &=& 1-\sum_{s=1}^\infty\frac1{s}\frac{(4s-2)!}{(2s-1)!(2s-1)!}2^{-4s} \frac{(2s-1)!}{2^{s-1}(s-1)!} (p^{-1}-1)^{s}  N_J^{-s}
% \EEAS
% \end{lemma}

% \begin{lemma}[Taylor expansion and Gaussian approximation for $V_{2k}$]
% \label{TaylorSqrt_Expect_k}
% and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
% \BEAS
% \frac{1}{p^k}\E_I ({\frac{\sum_{i\in J} 1_{I_i}}{N_J}})^k  
% &\approx&  \E_G({1+ \sqrt{\frac{1-p}{pN_J}}G})^k \\
% &=& 1 +\sum_{\ell=1}^{k} \binom{k}{\ell} ({\frac{1-p}{pN_J}})^{\ell/2} \E_G G^{\ell}\\
% &=& 1 +\sum_{s=1}^{\left\lfloor{k/2}\right\rfloor} \binom{k}{2s} ({\frac{1-p}{pN_J}})^{s} (2s-1)!!
% \EEAS
% \end{lemma}



\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/Full_compare_with_baseline.png}
\caption{The value of $V_1(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is the $V_1(\psi)$. }
\label{fig-V1}
\end{figure}



\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/landscape/L1_conv_Landscape_Sparsity0p1_.png}
\caption{The value of $V_1(\psi)$ for $\psi$ on two dimensional sphere in $\reals^3$, normalized by the affine transform to send the value in $[0,1].$ . }
\label{fig-landscape}
\end{figure}



\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/L4_plot.png}
\caption{The value of $V_4(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is the $V_4(\psi)$. }
\label{fig-V4}
\end{figure}



\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/L8_plot.png}
\caption{The value of $V_8(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is the $V_8(\psi)$. }
\label{fig-V4}
\end{figure}



\subsection{Proofs}


\begin{proof}[Proof of theorem~\ref{thm:BGPropLemmaNorm}]
First, we show that the upper and lower bound value we give is achievable.
\BIT
\item 
When $\psi = e_0$,  
\[
\E_I  \| (e_0)_I \|_2=p\| (e_0)\|_2+(1-p)\| 0\|_2 = p
\]
\item
When $\psi = \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j,$ then  
\[
V_1(\psi) = \E_I \sqrt{\frac{\sum_{i\in [N]} 1_{I_i}}{N}} \leq   \sqrt{\E_I \frac{\sum_{i\in [N]} 1_{I_i}}{N}} = \sqrt{p}
\]
The inequality comes from Jensen's inequality, since square root function is concave.
\item
For fixed support $J$, when $\psi = \frac{1}{\sqrt{N_J}}\sum_{i\in J} e_i,$  then $\| \psi_J \|_2/\|  \psi \|_2 =1.$
However, the expectation is going to be smaller for $p<1$. 
\[
V_1(\psi) = \E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \sum_{k=0}^{N_J} (1-p)^{N_J-k} p^{k} {N_J \choose k}\sqrt{\frac{k}{N_J}}.
\]
\EIT

This problem can be reformulate as the projection pursuit with sphere constraint,
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
Then from \cite{bai2018subgradient} Proposition $3.3$, we get the result. 

The main idea of the proof is to calculate the projected gradient
for $q  \in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$, when $N_J = M,$
\[
e_j^T  \E_I  \partial\| (q)_I \|_2 = q_j [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] 
\]
therefore,
\[
  \E_I  \partial\| (q)_I \|_2 =  [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] q
\]
so
\[
(I-q q^T)  \E_I  \partial\| q_I \|_2 = [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q -[\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q  = 0.
\]
then $q \in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ is stationary points.
 
The other direction (all other points are not stationary) is implied by (the proof of) theorem $3.4$ in  \cite{bai2018subgradient}.
\end{proof}





\begin{proof}[Proof of lemma~\ref{TaylorSqrt}]
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{1/2}
=\sum_{\ell=0}^\infty\binom{1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{1/2}{\ell}
&=\frac{\frac12(\frac12-1)(\frac12-2)\cdots(\frac12-\ell+1)}{\ell!}\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-3)\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}\frac{(2\ell-2)!}{2^{\ell-1}(\ell-1)!}\\
&=\frac{(-1)^{\ell-1}}{\ell2^{2\ell-1}}\binom{2\ell-2}{\ell-1}
\end{align}
then
\begin{align}
(1-x)^{1/2}
&=1-\sum_{\ell=1}^\infty\frac2\ell\binom{2\ell-2}{\ell-1}\left(\frac x4\right)^\ell\\
&=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{proof}







\begin{proof}[Proof of lemma~\ref{TaylorSqrt_Expect}]
\BEAS
\E_I\sqrt{1- \sqrt{\frac{1-p}{pN_J}}g^I}  
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_I \left( g^I\right)^{\ell+1}\\
&=& 1- 2^{-3}({\frac{1-p}{pN_J}}) - O(({\frac{1-p}{pN_J}})^2)
\EEAS
Using central limit theorem, when $N_J\rightarrow \infty$, we have normal approximation for $g^J$ so that
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} \sim N(p,  \sqrt{\frac{p(1-p)}{N_J}})
\]
then for $G\sim N(0,1),$ asymptotically when $N_J\rightarrow \infty$,
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} \approx  \sqrt{p} \E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G} =
\sqrt{p} \left( 1- 2^{-3}(1-p)^{2}  N_J^{-1} + O((1-p)^{4}  N_J^{-2})\right)
\]
where
\BEAS
\E_I\sqrt{1- \sqrt{\frac{1-p}{pN_J}}g^I}  
&\approx &\E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G}\\
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_G \left( G\right)^{\ell+1}\\
&=& 1-\sum_{\ell \mbox{ is odd}}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1} (\ell)!!\\
&=& 1-\sum_{s=1}^\infty\frac1{s}\binom{4s-2}{2s-1}2^{-4s} (2s-1)!! (p^{-1}-1)^{s}  N_J^{-s}\\
&=& 1-\sum_{s=1}^\infty\frac1{s}\frac{(4s-2)!}{(2s-1)!(2s-1)!}2^{-4s} \frac{(2s-1)!}{2^{s-1}(s-1)!} (p^{-1}-1)^{s}  N_J^{-s}\\
&=& 1-\sum_{s=1}^\infty\frac{(4s-2)!}{(2s-1)!(s)!}2^{-5s+1}  (p^{-1}-1)^{s}  N_J^{-s}
\EEAS
\end{proof}






==> old_sec/sec_old/Inequality.tex <==
\subsection{General sparse signal }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ have variance $\sigma^2$,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \sigma^2 \|\psi\|_2^2.
\]
The ratio indicate the sparsity level of random variable $ \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\sigma^2 \|\psi\|_2} 
\]
Now, we consider $E{|\sum_{i} \psi_i X_i| }$ for general symmetric setting when lower bound can be derived.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i Z_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $Z_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
\E_X{|\sum_{i} \psi_i X_i| }  
= \E_B \E_G {|\sum_{i} \psi_i B_i G_i| }
= \E_I \E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
\E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]


\paragraph{Symmetric distribution}

Dave Comment:
Put the generalization in the end.
Focus on Bernoulli Gaussian for the main part, and then talk about extension.


% \paragraph{General symmetric distribution case}
\begin{lemma} \label{lem:sym_Khintchine_inequality}
For we only know $\Xi_i$ are IID sampled from a symmetric distribution $F$ with unit variance, then we already have a lower bound,  
\[
     1/\sqrt{2}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
\] 
\end{lemma}
 \begin{proof}[Proof of Lemma \ref{lem:sym_Khintchine_inequality}]
 The upper bound come from Cauchy inequality.
 
Now we derive the lower bound. We write $\Xi_i = \sigma_i |\Xi_i|$, where $s_i =\pm 1$ with equal probability since $\Xi_i$ are symmetric RV, and $\{s_i,|\Xi_i|\}$  are all independent random variables.  
we could use Khintchine inequality,
here is the Wiki link for more detail:
\begin{quote}
\href{https://en.wikipedia.org/wiki/Khintchine_inequality}{Khintchine inequality}.
\end{quote}




\begin{eqnarray*}
\E_\Xi |\sum_i a_i \Xi_i| &=& E_{|\Xi_i|}E_{s_i} |\sum_i a_i s_i |\Xi_i||\\
&\geq&  
  1/\sqrt{2}  \sum_i a_i^2  E_{|\Xi_i|} |\Xi_i|^2 \\
  &=&   1/\sqrt{2}  \|a\|_2^2.
\end{eqnarray*}
\end{proof}

Let $\psi_I = a$, we have a corollary for Bernoulli Symmetric case,
   \[
 \E_I \|\psi_I\|_2  \geq \E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]


\begin{theorem}
Let $X_i = B_i \Xi_i$ be IID, where $B_i$ is sampled from Bernoulli with parameter $p$, let $I$ be the support where $B_i =1$. And $\Xi_i$ is variance $1$, sampled from: 
\begin{itemize}
    \item $N(0,1)$
    % \item sub-Gaussian with sub-Gaussian norm $K = \|Z\|_{\Psi_2}$
\item general symmetric distribution with variance $1$.
\end{itemize}
% Here sub-Gaussian norm is defined as
% $
% \|X\|_{\Psi_2} := \sup_{r\geq 1} r^{-1/2}  (E|X|^r)^{1/r}.
% $

Then 
\begin{itemize}
    \item(for Bernoulli Gaussian:)
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot \E_I \|\psi_I\|_2
\]
%     \item (for Bernoulli sub-Gaussian:) 
%      \[
% \E_X{|\sum_{i} \psi_i X_i| }  
% \geq  3^{-3/2}C^{-3} K^{-3}  \cdot (1-(1-p)^{\|\psi\|_0})^{1/2}   \cdot  \|\psi\|_2.
% \]
\item (for Bernoulli symmetric R.V. :) 
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]
\end{itemize}

\end{theorem}




% \paragraph{Sub-Gaussian case}
% For a sub-Gaussian random variable $\Xi$ with unit variance and symmetric c.d.f $F$, we define 
% \[
% K = \|\Xi\|_{\Psi_2} = \sup_{r\geq 1} r^{-1/2}  (E|\Xi|^r)^{1/r}
% \]
% as the sub-gaussian norm of $X$
% \begin{lemma} \label{lem:Khintchine}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then for all $r \geq 2$,
% \[
% \|\psi\|_2 \leq (E(Z)^p)^{1/p} \leq C K p^{1/2} \|\psi\|_2
% \]
% where $C$ is absolute constant.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% The lower bound follows by independence and Holder’s inequality.
% For the upper bound, since we have 
% \[
% \|\sum_i a_i X_i\|_{\Psi_2}^2\leq C\sum_i a_i^2 \| X_i\|_{\Psi_2}^2\leq C\|\psi\|_2^2 K^2,
% \]
% And $Z = \sum_i a_i X_i$ is sub-Gaussian, so for all $p\geq 2$,
% \[
%  (E(Z)^p)^{1/p} \leq \|Z\|_{\Psi_2} p^{1/2} \leq C^{1/2} p^{1/2}\|\psi\|_2 K 
% \]
% \end{proof}
% \begin{lemma} \label{lem:Khintchine for $p=1$}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then
% \[
%      3^{-3/2}C^{-3} K^{-3}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
% \] 
% \[
%      3^{-3/2}C^{-3} K^{-3}  \|\psi\|_2 \leq E |\sum_i a_i X_i| \leq \|\psi\|_2
% \]
% where $C$ is absolute constant, $K = \|X\|_{\Psi_2}$.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% We use the extrapolation trick. 
% Let $Z=\sum_i a_i X_i$, since we have 
% \[ (E(Z)^2){1/2} \leq (E|Z|)^{1/4}((E(Z)^3)^{1/3})^{3/4},\]
% we get 
% \[E|Z|\geq (E(Z)^2)^{2}/ (E(Z)^3).\]

% We get a bound on 
% \[
% \|\psi\|_2 \leq (E(Z)^r)^{1/r} \leq C K p^{1/2} \|\psi\|_2
% \]
% from Khinthine’s inequality for $r = 3$.
% \end{proof}




==> old_sec/sec_old/Intro.tex <==
\section{Introduction}
% \emph{Sparse blind deconvolution} is a method that solves problem including sparse blind deconvolution, sparse convolutional ICA and convolutional dictionary learning.

Blind deconvolution is the problem of recovering a kernel and a signal from 
their (noisy or corrupted) convolution.
This is a ubiquitous problem in fields including signal processing, 
machine learning, computer vision, seismology, time series and neuro-science.
Blind deconvolution is also a crucial problem at the core of digital communication that powers our modern society by enabling cell phone communication.

One important example of blind deconvolution is when the signal is sparse, as the sparse blind deconvolution setting. We call this problem \emph{sparse blind deconvolution}. The sparse signal setting of blind deconvolution appears in seismology, microscopy, astronomy, neuro-science spike identification. In representation learning for computer vision, computational imaging and speech analysis, sparse blind deconvolution is also interpreted as single-channel convolutional dictionary learning.



% \paragraph{Contribution}
\paragraph{First suprise: convex formulation for blind deconvolution}
Despite the importance of blind deconvolution, until recently there has been little understanding of when, how and why these non-convex algorithms succeed.
Practitioners have accumulated poetic yet vague observations like "when the initialization is close, gradient-based methods find the true signal", but there is no clear understanding of this statement.

In this paper, we proposed a scalable convex optimization framework for blind deconvolution.
Suppose there is a sparse signal $x$ and a forward filter $a$, the observation is their convolution $y$ defined as $y = a * x$. The blind deconvolution is a problem of finding the sparse signal $x$ from the observation $y$ without knowing the forward filter $a$. 
As both the sparse signal and the forward filter $a$ are unknown, the problem is often formulated as a non-convex problem. For example, in large collection of papers \cite{kuo2019geometry, bristow2013fast, heide2015fast,zhang2017global,zhang2018structured}, people designed alternating minimization type algorithms that jointly find a short $a$ on sphere and sparse $x$ from $y$ by solving the following non-convex problem: 
  \[
 \begin{array}{ll}
 \underset{a, x}{\mbox{minimize}}   & \|y-a*x\|_2^2+\lambda \|x\|_1 \\
\mbox{subject to}  & \|a\|_2 = 1.
\end{array}
  \]  

In this work, we formulate this problem as looking for a sparsifying filter $w$ so that $\Tilde{x} = w*y$ is sparse. This formulation is adapted in the earlier work of Wiggins \cite{wiggins1978minimum} and Donoho \cite{donoho1981minimum} for minimum entropy deconvolution, or maximum cumulant deconvolution. The core idea is that  Find $w\approx a^{-1}$, so that $w*y$ is the most non-Gaussian.
\item Find $w\neq 0$  
\[
 \begin{array}{ll}
 \underset{w\neq 0}{\mbox{maximize}}   & J(w*y)
\end{array}
  \]
\item Non-Gaussianity: 
\BIT
\item
$J(z) = -\mbox{Entropy}(p_z)$ 
\item
$J(z) = \frac{\|z\|_4^4}{\|z\|_2^4}$, normalized $4$-th order cumulant 

by solving the convex optimization problem for a chosen initial guess  $\Tilde{a}$ of the forward filter:
\BEQ
 \begin{array}{ll}
 \underset{w}{ \mbox{minimize} }   & \|w*y\|_{1}\\
\mbox{subject to}  
& (\Tilde{a}*w)_0 =1, 
\end{array}
% \tag{$P_{v}^T$ }
\EEQ


My work demonstrates that the hidden convex formulation behind the scene leads to the success of these heuristic algorithms. This mathematical formulation gives a crisp, clean view that clears all the fog in the claims of past practitioners. 

\paragraph{Random model for sparse signals}
We define a random model for sparse signals. Let $(X_t)$ be an independent
sequence of random variable indexed by  $t \in Z$, with a symmetric distribution with CDF $F_t$, such that $F_t(x) = 1 - F_t(-x)$. 
And we assume $F_0$ has an atom at $0$, $F_0 = (1-p) H +p G$, where $H$ is Heaviside distribution and $G$ is standard Gaussian distribution, we called it \emph{Bernoulli$(p)$-Gaussian} model. 
% If $G$ is some sub-Gaussian distribution instead, then we called it \emph{Bernoulli$(p)$-sub-Gaussian} model.


For a process $Y = a * X$, where $a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T,$ additionally, $a^{-1}$ is zero outside of a centered window of radius $2k+1$. 

Now given a series of observation $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$, we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse, where $V$ is a $2k+1$ dimensional subspace $V$ of the double infinite sequence. Let $\|\cdot\|_{1,\cT} =\|\cdot\|_{\ell_1(\cT)}= \|\cdot\|_{1,[-T,T]}  $ be the $1$ norm over the centered window of radius $T$. Let $N:= 2T+1$ be the total length of $X$.



\paragraph{Convex sparse blind deconvolution}
 In this work, we consider a convex formulation of the problem as
\BEQ
 \begin{array}{ll}
 \underset{w\in V}{ \mbox{minimize} }   & \frac{1}{N}\|w*Y\|_{\ell_1(\cT)}\\
\mbox{subject to}  
& v^T w =1, 
\end{array}
\tag{$P_{v}^T$ }
\EEQ

In the following, we first study the population problem of convex blind deconvolution, which coincident with the population problem of convex sparse dictionary learning, which is also called projection pursuit or convex sparse ICA.

We first prove the existence of population phase transition by analyzing projected sub-gradient and give a characterization of the population phase transition. Then we study finite sample guarantee, noisy perturbation stability, finite length inverter stability.

\paragraph{Application}
Image deblur, neural spike measurement, time series sparse feature transform learning, Seismic application with oil discovery, signal demixing. Audio deconvolution (dereverberation) is a reverberation reduction in audio mixtures. It is part of audio processing of recordings in ill-posed cases such as the cocktail party effect.






\paragraph{Ratio of norm formulation for blind deconvolution}
First, from the paper \cite{donoho1981minimum}, we know that we could minimize the ratio of norm of $X$ to recover $X$.

For example, \cite{donoho1981minimum,wiggins1978minimum} propose to study $(\ell_{2k}/\ell_2)$ problem for $k=2, 3, 4,\ldots$.
\begin{eqnarray*}
    (\ell_{2k}/\ell_2) \qquad  \max&    \frac{1}{N} \| w*Y\|^{2k}_{\ell_{2k}(\cT)}\\
    \mbox{ subject to }&   \frac{1}{N} \| w*Y\|^2_{\ell_2(\cT)} \geq 1.
\end{eqnarray*}


For $\ell_1/\ell_2$ ratio, we propose to use a non-convex (convex objective concave constraint) problem for blind deconvultion:
\begin{eqnarray*}
    (\ell_1/\ell_2) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
    \mbox{ subject to }&   \frac{1}{N} \| w*Y\|_{\ell_2(\cT)} \geq 1.
\end{eqnarray*}
This can be further reduced to sphere-constrained optimization
\begin{eqnarray*}
      \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
    \mbox{ subject to }&   \| w\|_{2}^2 = 1.
\end{eqnarray*}
If we use iterative linearization of the nonconvex sphere-constrained, on every iteration we could use convex form:
Let $w^0 = e_0$, iteratively find $w^{k}$ by
\begin{eqnarray*}
     \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
    \mbox{ subject to }&   w^{k-1,T} w = 1.
\end{eqnarray*}
This is analogous to use power method to solve PCA problem.


\paragraph{Infinity norm ball constraint}


Before stating the main theorem and its proof, we make some comments about the formulation.

If we study the population level, 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \expect |\tilde{w}^T Y|\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}$ }
\EEQ
then we only need solve one convex problems
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \expect |\tilde{w}^T Y|\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}$ }
\EEQ
Since the entry with largest magnitude will automatically be shifted to coordinate $0$ due to shift invariance.


If we want to solve the following non-convex problem with infinity norm ball constraint for finite sample,
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}^T$}
\EEQ
We can solve the following convex problems, and select the one with minimal objective value. This is equivalent to solve the problem with fixed infinity norm. 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_j =1.
\end{array}
\tag{$P_{e_j}^T$ }
\EEQ

==> old_sec/sec_old/Inverse.tex <==

\section{Analysis of the inverse kernel method}
\subsection{Inverse kernel approximation}
Now we consider a setting where there is a kernel whose corresponding the inverse kernel is infinite, and we give a finite length approximation. 
We assume that $a =  (a_{-t},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t) = \delta_0 + a_L + a_R$ 
is a length $ l= 2t+1$ filter, 
  and $\sum_{i\neq 0} |a_i|\leq M < 1$.    
 \begin{theorem} 
For a kernel $a = (a_{-s},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t)$ of length $l=1+s+t$, if 
\[
\sum_{i\neq 0} |a_i|\leq M < 1,
\]
 then there exists an approximate inverse kernel $w^r$ of length $rl$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M),\\
\end{array}
  \]
\end{theorem}
\begin{proof}
Consider the $z$ transform of $a$ to be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
let $\bar A(z) = 1-A(z)$, then 
from the condition 
$\sum_{i\neq 0} |a_i|\leq M < 1$,
we define $M' $ to be the maximum absolute value of $\bar A(z)$ on unit circle, as
\[
 \begin{array}{ll}
\mbox{maximize}   & |\bar A(z)| \\
\mbox{subject to}  & z\in \complex,|z|=1.
\end{array}
  \]
Then 
\[
 \begin{array}{ll}
M' \leq \sum_{i\neq 0} |a_i|\leq M<1.
\end{array}
  \]
The Z-transform of the inverse kernel of $a$ is defined by
\[
 \begin{array}{ll}
1/A(z) &=  (1-\bar A(z))^{-1},\\
&= 1+ \sum_{i=1}^{\infty} (\bar A(z))^i
\end{array}
  \]
 The infinite series absolutely converge on $|z| = 1$ because $|\bar A(z)|\leq M<1$.
Let the finite approximation of level $r$ of $w = a^{-1}$ be $w^r$, 
 its Z-transform is  $\sum_{i=0}^{r} (\bar A(z))^i$,
its length is at most $r(s+t+1)$, 
the $j$-th term of $w^r$ is $\sum_{b}bj_i=j \prod_{i} a_i^{j_i}$.
We have that for all  $|z| = 1$,
 \[
 \begin{array}{ll}
|1/A(z) - \sum_{i=0}^{r} (\bar A(z))^i | 
&= |\sum_{i=r+1}^{\infty} (\bar A(z))^i|\\
&\leq M^{r+1}/(1-M).
\end{array}
  \]
Therefore, 
   \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]
%   \[
%  \begin{array}{ll}
% \|a*w^r - e_0 \|_{1} &= \|a*(w^r - w) \|_{1}\\
% &\leq \|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} \\
% &\leq M^{r+1}/(1-M) \\
% &= M^{r+1}(1+M)/(1-M)
% \end{array}
%   \]
 
\end{proof}

Using this inverse approximation, we know for any kernel $a$ of length $l$ with possibly infinite inverse kernel $w$, there exists a length-$rl$ approximate inverse kernel $w^r$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]

Therefore, we can prove the following theorem on sparse blind deconvolution algorithm. 


\paragraph{Simple example.}
We consider a simple example, when $a = (0,\ldots, 0, 1, r, 0, \ldots, 0) = \delta_0 - r\delta_1$, $|r|<1$. Then $a^{-1} = \delta_0 + \sum_{j=1}^\infty  r^j \delta_j.$ Now our data generation model is $y = a*x.$ 

We analysis the optimization problem 
 \begin{eqnarray*}
    \min_{f_0 = 0} &    
    E_x\| (\delta_0+f)*a*x\|_1.
\end{eqnarray*}
Here $f = (0, 0, f_R)$ is in a $K$ dimensional subspace of the double infinite sequence.

% We also analysis the constrained optimization problem 
%  \begin{eqnarray*}
%     \min_{f_0 = 0} &    
%     E_x\| (\delta_0+f)*a*x\|_1,
%     \\
%     \mbox{ subject to }&  \|f\|_1\leq C.
% \end{eqnarray*}

For the objective, using IID property of $x$, we only need to analyze
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| .
\end{eqnarray*}
Let $f^*_K$ be the best length $K$ approximation, as the solution of 
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    \| (\delta_0+f)*a\|_2,
\end{eqnarray*}

In this specific example, $f^*_K = \sum_{j=1}^K  r^j \delta_j.$ And $(\delta_0+f^*_K)*a = (\delta_0 - r^{K+1}\delta_{K+1})*(\delta_0 - r^{1}\delta_{1})^{-1}$.
Let $\tilde{x} = (\delta_0 - r^{K+1}\delta_{K+1})*x$, as one approximation of $x$.
Since $x$ is IID symmetric, $ \tilde{x}$ is identically-distributed, symmetric and weakly correlated for $|r^{K+1}|$ small enough, and $\tilde{x}_0, \ldots, \tilde{x}_K$ are independent.

Let 
\begin{eqnarray*} 
\delta_0+h &=& (\delta_0+f)*(\delta_0+f^*_K)^{-1}\\
&=& (\delta_0+f)*(\delta_0 - r^{K+1}\delta_{K+1})
\end{eqnarray*}
then 
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| 
    &=& E_x | ((\delta_0+h)*\tilde{x})_0|\\
&=& E_x | \tilde{x}_0|+\mbox{sign}(\tilde{x}_0)(h*\tilde{x})_0\\
&\approx& 
 |1+  h_{0}| \cdot E |\tilde{x}_0| \cdot (1-\eta)+   \cdot  E{| (h*\tilde{x})_0| } \cdot \eta.
\end{eqnarray*}

Following the same analysis as the phase transition analysis, we have
\begin{eqnarray*}
     \min_\delta &E | ((\delta_0+f)*a*\tilde{x})_0 | \\
    \mbox{ subject to }  &f_{0} = 0.
\end{eqnarray*}


==> old_sec/sec_old/Metric.tex <==
 \subsection{Distance metrics}
% \paragraph{Distances to measure stability}
We care about three types of metrics, first, distance  in $w$ space, between the computed composed filter $w$ and ground truth $a^{-1}$; second, distance in $w$ space, between the computed inverse filter $w$ and ground truth inverse filter $a^{-1}$, second, distance  in $\psi = w*a$ space, between the computed composed filter $w*a$ and ground truth $e_0$; third,  distance  in $x$ space, between recovered signal sequence and true sparse signal sequence. 

First, the MSE in space of $\psi = w*a$,
  \[
 \begin{array}{ll}
d_{\psi,2}^2 := \|\phi\|_2^2 =  \|\psi-e_0\|_2^2= \|a*(w-a^{-1})\|_2^2
\end{array}
  \] 
 The MSE in space of $w$. 
   \[
 \begin{array}{ll}
d_{w,2}^2  = \|w-a^{-1}\|_2^2 = \|a^{-1}*(\psi-e_0))\|_2^2 = \|a^{-1}*\phi\|_2^2
\end{array}
  \]
Last, $\ell_1$ and $\ell_2$ distance in $x$ space:
\[
 \begin{array}{ll}
d_{x,1} &:= \frac{1}{2T+1}\|w*Y-X\|_{1,[-T,T]} =  \frac{1}{2T+1}\|\tilde \phi* X\|_{1,[-T,T]} \\
d_{x,2}^2 &:= \frac{1}{2T+1}\|w*Y-X\|_{2,[-T,T]}^2 = \frac{1}{2T+1}\|\tilde \phi* X\|_{2,[-T,T]}^2
\end{array}
  \]
We compute their expectation: 
\[
 \begin{array}{ll}
\Expect d_{x,1}  &=  \Expect|\phi^T X| = \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2\\
\Expect d_{x,2}^2 &=  \Expect|\phi^T X|^2 = p \|\phi\|^2  = p \|\psi-e_0\|^2 
\end{array}
  \]  
We remark that in the following we focus on distance in $x$ space to recover the signal. 

% And using the fact that $\Expect d_{x,1}= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2$ and $\Expect d_{x,2}^2 = p \|\phi\|^2$, we focus on calculate 
% \BIT
% \item $\Expect d_{x,1} \propto  \Expect_I \|\phi \cdot I\|_2$
% \item $\Expect d_{x,2}^2 = \Expect_I \|\phi \cdot I\|_2^2 = p\|\phi\|^2  = p d_{\psi,2}^2$ 
% \EIT



==> old_sec/sec_old/Noise.tex <==
\section{Stability for noisy observation}


\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]
\subsection{Stability for adversarial perturbation of sparse signal }
\paragraph{Mathematical formulation: sparse signal plus adversarial perturbation}

\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
$Z$ is a unit vector in $2$ sphere. 
\item
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
\Expect|(w*Y)_0|
&= \Expect|\psi^T (X+\eta Z )| \\
% &= \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
\end{array}
  \]

  
  
  
 \paragraph{Study the noisy problem}
Under the data generative model, 
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
    the constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta}   & \Expect|\psi^T (X+\eta Z ) - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
  
\paragraph{Worst case objective over $Z$}  
For the constrained problem, we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
  \]
Which is equivalent to 
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
In the following we study the min-max objective
  \[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi) : = \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| 
\end{array}
  \]
  
\paragraph{Robust optimization}
Let the deterministic residual function of $\psi, Z, \zeta$ be
\[
\mu_{\eta, \epsilon}(\psi, Z, \zeta): = \eta  \psi^T Z  - \epsilon \zeta
\]
We reparametrize $\epsilon$ as by defining 
\[
\tau :=  \frac{\epsilon}{\eta}
\]
then 
\[
\mu_{\eta, \epsilon} = \eta ( \psi^T Z  - \tau \zeta)
\]






\begin{lemma}
For any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, $Z$ is along the direction of $s\psi$ so that $s\psi^T Z = \|\psi\|_2$.

\end{lemma}  


\begin{lemma}[Hölder's inequality]
For any given sign $s =\pm 1$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $s|\psi|^q$ so that $s\psi^T Z = \|\psi\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
The min-max quantity  
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2 = (\eta \|\psi\|_2  - \epsilon )_+^2 = \eta^2 ( \|\psi\|_2  - \tau )_+^2
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}^2 
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2\\
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} [(\eta  \psi^T Z)^2+  (\epsilon \zeta)^2 - 2(\eta  \psi^T Z)(\epsilon \zeta)]\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \sup_{Z: \|Z\|_2\leq 1} [ (\psi^T Z)^2] + 2\eta \epsilon |\zeta|   \sup_{Z: \|Z\|_2\leq 1}[ (-\sign(\zeta) \psi^T Z)]\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \|\psi\|_2^2 + 2\eta \epsilon |\zeta|   \|\psi\|_2\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{  (\eta \|\psi\|_2  - \epsilon |\zeta| )^2\}\\
&= (\eta \|\psi\|_2  - \epsilon )_+^2
\end{array}
\]
The fourth equation is because for any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_2\leq 1}(s \psi^T Z) = \|\psi\|_2.
\]
\[
\sup_{Z: \|Z\|_2\leq 1}( \psi^T Z)^2 = \|\psi\|_2^2.
\]



\end{proof}

We have the following result, generalizing $\|Z\|_2\leq 1$ to $\|Z\|_p\leq 1, \quad, p\geq 1$, and then to $Z\in K$ for a closed compact convex set $K\in \reals^N$.



\begin{lemma}
\label{min-maxErrorL_p}
The min-max quantity 
for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates,
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_p\leq 1} F( \eta (\psi^T Z  - \tau \zeta)) = 
F(\eta( \|\psi\|_q  - \tau )_+)
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}

\begin{coro}
 \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_2  - \tau )_+|
\end{array}
  \]
  in general, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_p\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}


\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then for any constant $\mu$, using the rotation invariance of Gaussian, $\psi^T X +\mu$ is  Gaussian with mean $\mu$ and standard deviation $\|\psi_I\|_2$, therefore,
\[
|\psi^T X +\mu |
\]
following the folded Gaussian distribution.
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}

From general theory of folded Gaussian $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
hence
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
\end{array}
\]

\end{lemma}
\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}







==> old_sec/sec_old/Noise2.tex <==

% \paragraph{Bound on min-max objective}

% First of all, we find a lower and upper bound that is true independent of the distribution of $X$.
% \begin{lemma}
% Let $\psi^T X $ be fixed, we have upper and lower bound on the constrained problem objective:
%  \[
%  \begin{array}{ll}
% \sup_{s=\pm 1}|(\psi^T X +s\eta \|\psi\|_2  - \epsilon)_+| \leq
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} |\psi^T X +\eta  \psi^T Z  - \epsilon \zeta| 
% \leq |\psi^T X | +|(\eta \|\psi\|_2  - \epsilon)_+ |
% \end{array}
%   \] 
% \end{lemma}  
% \begin{proof}
% Let $A:=\psi^T X $ be fixed
% First, if we let $Z$ be along the direction of $s\psi$, we have a lower bound on the objective for both $s =\pm 1$,
%   \[
%  \begin{array}{ll}
%   \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| 
% \geq
%  |A +\eta s\|\psi\|_2  - \epsilon \zeta|
% \end{array}
%   \] 
%   Therefore, we can 
%   \[
%  \begin{array}{ll}
%  &\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \geq&
% \inf_{\zeta: \zeta^2 \leq 1} |A +\eta s\|\psi\|_2  - \epsilon \zeta|\\
% =&
%  |(A +s\eta \|\psi\|_2  - \epsilon)_+|
% \end{array}
%   \] 
% Second, if we let $ \sign(\eta  \psi^T Z  - \epsilon \zeta) = s'$ then
%   \[
%  \begin{array}{ll}
%  & \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \leq&
% \inf_{\zeta: \zeta^2 \leq 1}  \sup_{Z: \|Z\|_2\leq 1}   (|A |+ |\eta  \psi^T Z  - \epsilon \zeta|) \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} |\eta  \psi^T Z  - \epsilon \zeta| \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\sup_{Z: \|Z\|_2\leq 1} [\eta  s'\psi^T Z]  -s' \epsilon \zeta\} \\
%     =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\eta \|\psi\|_2  -s' \epsilon \zeta\} \\
%   =&
%   |A | +|(\eta \|\psi\|_2  - \epsilon)_+ |\\
% \end{array}
%   \] 
  
% \end{proof}
\paragraph{Folded Gaussian mean and asymptotically tight lower bound}
Now we exploit the property of folded Gaussian mean, and we find an exact asymptotic formula.
For simplicity of expression, we also define the deterministic residual function of $\psi, I$ to be
\[
\gamma_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}(\psi, Z, \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\psi\|_2 - \tau)_+}{\|\psi_I\|_2}
\]

\begin{coro}
\label{Cor:PerturbedObjectiveLowerBound}
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)
&= \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| \\
&= \sqrt{\frac{2}{\pi}}  \Expect_I \left[ \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I \left[\|\psi_I\|_2(1 + \frac{3}{2}\gamma_{\eta, \epsilon}^2 + \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma_{\eta, \epsilon}^6)\right]
\end{array}
\]
As $\gamma_{\eta, \epsilon}^2<1,$ 
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)-L_{0, 0}(\psi)
&\geq 3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}(\psi)^2\Expect_I \|\psi_I\|_2^{-1}
\end{array}
\]
\end{coro}
% \begin{proof}
% In the following proof, for clarity, we write $\gamma_{\eta, \epsilon}$ simply as $\gamma$.

% Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
% we have
% \beq
% \label{FoldedGaussianMean_Obj}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| = \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]
% \eeq
% Then we can plug in the lemma \ref{ExpansionMeanFoldedGaussian}.
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \{ 1- \frac{\gamma_{\eta, \epsilon}^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \sqrt{\frac{2}{\pi}}\Expect_I  \left[ \|\psi_I\|_2 
% \{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2_{\eta, \epsilon}))\gamma_{\eta, \epsilon}^2 +   \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} \}\right]\\
% \end{array}
% \] 
% Here the residual of this expansion after first order is
% \[
%  \begin{array}{ll}
% \mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2_{\eta, \epsilon})-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!} \\
% &=    \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma^6)
% \end{array}
% \] 
% From the lower bound in lemma \ref{ExpansionMeanFoldedGaussian}, we have that when $\gamma_{\eta, \epsilon}^2<1, \mbox{Res}(\gamma^2)\geq 0$
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}\mu_{\eta, \epsilon}^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \] 
% Now we could plug in lemma~\ref{min-maxError} to prove the last equation.
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \]
% \end{proof}









% We branch out to show a low-hanging result for the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem}.
% \begin{coro}
% For
% the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem} with min-max lower bound as objective
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]
%  If $\epsilon \geq \eta,$ then the minimizer is $1$-sparse vector $e_i$, the same as the minimizer of 
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]

% \end{coro}


  \paragraph{Calculate the robust objective at $e_0$}
First, at $\psi = e_0$, $X_0 =e_0^T X = I_0 G_0$, where $G_0$ is standard normal, $I_0$ is Bernoulli, we take expectation over $I_0$ first, 
Let 
 \[
 \mu_0 :=  \mu_{\eta, \epsilon}(e_0) = \eta ( 1-\tau)_+ 
 \]
 When $\epsilon\geq \eta,$ $\mu_0=0$; when $\epsilon< \eta,$ $\mu_0>0$.
 \begin{lemma}
  \label{Lemma:ObjectiveDiffAtEzero}
     \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
 \end{lemma}
%   \begin{lemma}
%   \label{Lemma:ObjectiveRatioAtEzero}
%      \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &=  [(1-p)\mu_0\sqrt{\frac{\pi}{2}}  + p  (e^{-\frac{\mu_0 ^2}{2}} )+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)]/p
% \end{array}
%   \] 
%  \end{lemma}
 
 \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveDiffAtEzero}]
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&= \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}\Expect |X_0+\eta   Z_0  - \epsilon \zeta|-\Expect | X_0| \\
&= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|-\Expect | X_0| \\
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
 \end{proof}
%   \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveRatioAtEzero}]
%   Using lemma~\ref{ExpansionMeanFoldedGaussian}, let $\gamma = \eta ( \|e_0\|_2-\tau)_+/B_0,a$
%     \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|/\Expect | X_0|\\

% % \Expect_I |(e_0)_I+\eta ( \|e_0\|_2-\tau)_+|/\Expect_I | (e_0)_I| 
% % &=  \sqrt{{\pi}\frac{2}} (1-p)\mu_0  + p (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
% % &= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
% \end{array}
%   \] 
% The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
%  \end{proof}
 
 
We observe that 
\BIT
\item
if $\tau\geq 1$,   $( 1-\tau)_+ = 0$, then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) = 0;$
\item
if $\tau < 1$ , then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) \approx (1-p)\mu_0  + p O(\mu_0^2).$
\EIT

  
  \paragraph{Bound $\|\phi^\star\|_2$ using the difference of objective }
   Now use the change of variable that $\psi =e_0+\phi$,
   the constrained problem becomes
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & L_{\eta, \epsilon}(e_0+\phi) \\
\mbox{subject to}  
&u^T \phi =0
\end{array}
  \] 
First, we assume the minimizer is $\phi^\star$. Since $e_0$ is  minimizer of $L_{0, 0}$ and $e_0+ \phi^\star$ is  minimizer of $L_{\eta, \epsilon}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star) 
 \geq L_{0, 0}(e_0+\phi^\star)
 \geq L_{0, 0}(e_0) 
\end{array}
  \] 

Remark: This chain is true for all  $\phi^\star$ that $L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star),$ we can pick a dense sequence converging to $\phi^\star$ in $\ell_2$ norm)  
  
 Then using the fact that $L_{\eta, \epsilon}(e_0) -L_{\eta, \epsilon}(e_0+\phi^\star) \geq 0,$ we have
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
 \geq   [L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)]+ 
 [L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) ]
\end{array}
  \]   
  
 Notice that 
      \[
 \begin{array}{ll}
 L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)  = \Expect |(e_0+\phi^\star)^T X| - \Expect |(e_0)^T X| 
 = \sqrt{\frac{2}{\pi}} B(p,N)  \|\phi^\star\|_2
\end{array}
  \] 
  where $N = \|\phi^\star\|_0$, since $\phi^\star$ is dense due to our assumption, we have .
    \[
  \lim_{N \rightarrow \infty } B(p,N) = B(p,\infty) =  [ p (-\cot{\theta}) + (1-p)].
  \]
  if $p<p^\star$, $\lim_{N \rightarrow \infty } B(p,N) > 0.$
 
\begin{theorem}


\label{Thm:StabilityMSE}
When $\epsilon\geq \eta,$ and $p<p^\star$, then
$\|\phi^\star\|_2 =0$, the minimizer of the min-max problem is exactly $\psi^\star = e_0.$
 
 When $\epsilon< \eta,$  and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B(p,\infty)\right) \|\phi^\star\|_2 
 &\leq& 
 \left(L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)\right)-\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)\\
  &\leq&  \left(  (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4) \right) - 
  \left(  3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}((e_0+\phi^\star))^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} \right)\\
    &\leq& 
    (1-p)\mu_0  +  
    3\sqrt{\frac{1}{2\pi}}\left(  p \mu_0 ^2- \mu_{\eta, \epsilon}((e_0+\phi^\star))^2 \|e_0+\phi^\star\|_2^{-1} \right) + O(\mu_0 ^4)
 \EEAS
\end{theorem}
\begin{proof}
The first inequality comes from the chain of inequality between objectives. 

The second inequality combines the previous calculation of $L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)$ with lemma~\ref{ExpansionMeanFoldedGaussian} and lemma~\ref{Lemma:ObjectiveDiffAtEzero}.

For the last inequality comes from lemma~\ref{TaylorSqrtInvExpect}, 
\[
\frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}} \geq 1 .
\]
\end{proof}

\paragraph{Interpretation}
For simplicity, we focus on the case when the optimization problem is the original one where $\epsilon = 0$,
then 
\[
 \mu_{\eta, 0}(e_0) = \eta.
\]
\BIT
\item
We comment that when our optimization constraint is sphere constraint $\|\psi\|_2 =1$, 
then
\[
 \mu_{\eta, 0}(\psi)  = \eta
\]
then
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B_s(p,\infty)\right) \|\phi^\star\|_2 
    &\leq& 
    (1-p)
    [\eta  - 
    3\sqrt{\frac{1}{2\pi}} \eta^2] + O(\eta^4)
 \EEAS

\item
For the case when our optimization constraint is $u^T \phi =0$, 
\[
 \|e_0+\phi^\star\|_2^2= 1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 
 \]
 Since it is dependent on $\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2$, and using the condition $u^T \phi^\star =0$, we could use the same argument as figure~\ref{fig-Angle} and lemma~\ref{Angle_Inequality}, we know that 
 \[
 |\cos{\angle(\phi^\star,e_0)}| \leq \sin\theta
 \]
 therefore,
 \[
 |\frac{\|e_0+\phi^\star\|_2^2 - (1+\|\phi^\star \|_2^2)}{\|\phi^\star \|_2 }| \leq 2\sin\theta
 \]
 \EIT
 
We first have a weak corollary by only using $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)$ and just use loose bound $L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\geq 0.$


\begin{coro}
\label{Cor:StabilityMSE_}
 When $\epsilon< \eta,$ and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \|\phi^\star\|_2 &\leq& (L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0))/(\sqrt{\frac{2}{\pi}} B(p,\infty))\\
 &\approx& 
 \eta \{\sqrt{\frac{\pi}{2}}(1-p) +  \frac{3p}{2}\eta \}/  
 \{ p (-\cot{\theta}) + (1-p)\}+ O(\eta^4)
 \EEAS
\end{coro}  

  To strengthen this bound, we further compute 
$L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) $.

  
\begin{coro}
 When $\epsilon =0,$ and $p<p^\star$, as $\eta\rightarrow 0$, $\|\phi^\star\|_2$  is bounded by a function of $\eta$:
  \BEAS
\|\phi^\star\|_2 
 &\leq& 
 \frac{    (1-p)\{\sqrt{\frac{\pi}{2}}\eta -  \frac{3}{2}\eta^2 )}{   p (-\cot{\theta}) + (1-p) + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} } + O(\eta^4)
 \EEAS 
\end{coro}    
\begin{proof}
Let 
\[
\Gamma_{-1}(e_0+\phi^\star) := \frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}}
\]
From lemma~\ref{TaylorSqrtInvExpect}, we have 
\[
\Gamma_{-1} \geq 1 .
\]
we have
  \[
 \begin{array}{ll}
\sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} 
&= \sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2
\Gamma_{-1}(e_0+\phi^\star)
\end{array}
  \] 
Now we use Taylor expansion,  we could expand $\|\phi^\star \|_2$ around $0$ to first order 
\[
 \begin{array}{ll}
 \|(e_0+\phi^\star)\|_2
&=  (1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{\frac{1}{2}}\\
&= 1+\sum_{\ell=1}^\infty \binom{\frac{1}{2}}{\ell}
[\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)
\end{array}
  \] 
  
 
  
  \BEAS
- \sqrt{\frac{\pi}{2}}\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)
 &\leq& 
 - \frac{3}{2} \eta^2 \Gamma_{-1}(e_0+\phi^\star) (1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\eta^2))
 \EEAS 
 Therefore
  \BEAS
 \left(  [p (-\cot{\theta}) + (1-p)] + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} \right)\|\phi^\star\|_2 
 &\leq& 
 \eta (1-p) \{\sqrt{\frac{\pi}{2}} -  \frac{3}{2}\eta )+ O(\eta^4)
 \EEAS 
% \[
%  \begin{array}{ll}
%  \|(e_0+\phi^\star)\|_2^{-1}
% &=  (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}\\
% &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \]   


  
% \[
%  \begin{array}{ll}
%  \Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}
% &=  \Expect_I(1+\|\phi^\star_I \|_2^2 + \cos{\angle(\phi^\star_I,e_0)}\|\phi^\star_I \|_2)^{-\frac{1}{2}}
% % &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% % [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \] 
 
  

% Therefore,
%  \[
%  \begin{array}{ll}
 
% &  p\sqrt{\frac{2}{\pi}}\left[ \frac{3}{2}\mu_0^2\right]+(1-p)\mu_0
%  \\
% \geq& \frac{3}{2}(\eta \|(e_0+\phi^\star)\|_2  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) \|e_0+\phi^\star\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % =& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}+ B(p) \|\phi^\star\|_2\\
% \end{array}
%   \] 



\end{proof}
 













\subsection{Other setting on $Z$}
\paragraph{ Adversarial outer noise} 
If our generative model is
\[
\begin{array}{ll}
Y&= a* X + \eta_2 Z_2\\
&= a* (X +\eta_2 a^{-1}* Z_2)
\end{array}
\] 
And we consider the worst case objective over $\|Z_2\|_p\leq 1, \quad p\geq 1.$

Let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, then following previous calculation,
\begin{coro}
For $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z_2\|_p \leq 1}  &  \Expect|\psi^T X+\eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|C_{a^{-1}}^T \psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}

Let $C_{a^{-1}}^T \psi =\bar{a}^{-1}*\psi$, where $\tilde{a}^{-1}$ is defined by flipping the coordinate of $a^{-1}$ (reflecting the coordinates around zero by map $i$ to $-i$ for $i\in \integers$.)
 
 We can replace the definition of $\gamma$ and $\mu_0$  by:
 \[
 \gamma^{a}_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\bar{a}^{-1}*\psi\|_q  - \tau)_+}{\|\psi_I\|_2}
\]
\[
\mu_0^{a} := \eta( \|\tilde{a}^{-1}\|_q-\tau)_+
\]
We can get the same result as theorem~\ref{Thm:StabilityMSE}.

% \paragraph{Distributional robust setting}
% When $Z$ following a distribution $P_Z \in \Pi$, where $\Pi$ is a closed convex set in probability simplex for probability defined on $\reals^N$, then our distributional robust objective is
%   \[
%  \begin{array}{ll}
%  \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{P_Z \in \Pi}  & \Expect_Z \Expect_X|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| 
% \end{array}
%   \]
% then 
% for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates, the quantity 
% \[
%  \begin{array}{ll}
%  \sup_{P_Z \in \Pi}  & \Expect_Z F( \psi^T  Z ) 
% \end{array}
% \]
% could be computed following the same approach as the distributional robust Kelly problem if $\Pi$ can be represented by finite combination of atoms.
  

  

\subsection{ Gaussian additional noise}
\paragraph{ Gaussian additional observation inner and outer noise} 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+  \sigma_1 G_1) +  \sigma_2 G_2\\
&= a* (X+\sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\] 
let $C_{a^{-1}}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, then $C_{a^{-1}} = C_a^{-1}$ and 
\[
\begin{array}{ll}
Z: = \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\sim N(0, \sigma_1^2 I_N + \sigma_2^2 C_{a^{-1}} C_{a^{-1}}^T)
\end{array}
\] 
then
\[
\begin{array}{ll}
\psi^T Z
\sim N(0, \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2 )
\end{array}
\] 
 Let $G$ be another standard normal $N(0,I_N)$, for any fixed vector $\mu \in \reals^N, $
 \[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2)  | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  |
\end{array}
  \]
In this case, it seems the previous constrained problem no longer can help us find exact solution $\psi^\star =e_0.$ 



We first study $\sigma_2 = 0$ case.
\[
\Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}G_3 | = 
\sqrt{\frac{2}{\pi}} \cdot \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) =  \sqrt{\frac{2}{\pi}} \cdot \|\psi\|_2 \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma_1^2})
\]
Define worst case objective
\[
F_{\sigma}(\psi):= \sup_{\sigma_1 \leq \sigma} \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) = \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma^2\|\psi\|_2^2})
\]
The second equality comes from monotonicity.

Again, we assume the minimizer is $\psi^\star $. Since $e_0$ is  minimizer of $L_{0}$ and $\psi^\star $ is  minimizer of $L_{\sigma}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\sigma}(e_0)
 \geq F_{\sigma}(\psi^\star ) 
 \geq F_{0}(\psi^\star )
 \geq F_{0}(e_0) 
\end{array}
  \] 
Then
    \[
 \begin{array}{ll}
F_{\eta}(e_0)/F_{0}(e_0)
 \geq (F_{\eta}(\psi^\star )/F_{0}(\psi^\star ))(F_{0}(\psi^\star )/F_{0}(e_0) )
\end{array}
  \] 

   \[
 \begin{array}{ll}
 F_{\eta}(\psi)/F_{0}(\psi) = \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )
\end{array}
  \] 
  
     \[
 \begin{array}{ll}
 F_{\eta}(e_0)/F_{0}(e_0) = \Expect_I(\sqrt{ \frac{\|(e_0)_I\|_2^2}{\|e_0\|_2^2} + \sigma^2})/\Expect_I(\frac{\|(e_0)_I\|_2}{\|e_0\|_2} )= (p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p
\end{array}
  \] 
  
    \[
 \begin{array}{ll}
 F_{0}(\psi)/F_{0}(e_0) 
 &= \Expect_I\|\psi_I\|_2/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+(\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2)/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+ (B(p,N)/\Expect_I\|(e_0)_I\|_2) \|\psi -e_0\|_2\\
 &= 1+ (B(p,N)/p) \|\phi\|_2
\end{array}
  \] 

   \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi\|_2 &\leq (F_{\eta}(e_0)/F_{0}(e_0))/ (F_{\eta}(\psi)/F_{0}(\psi)) \\
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}/\{\Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )\}
\end{array}
  \] 
  First, a loose bound on $\|\phi^\star\|_2$:
  \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi^\star\|_2 
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}
\end{array}
  \] 
We found that
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq (\{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}-1)/(B(p,N)/p) \\
&\leq ((p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})-p)/B(p,N)
\end{array}
  \] 

In general, when $\sigma_1, \sigma_2$ both non-zero, using the same argument,
\[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq \frac{(p[\sqrt{ 1 + \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2}-1]+ (1-p) \sqrt{ \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2})}{B(p,N)}
\end{array}
  \] 

\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Inner and outer Gaussian and adversarial noise together}
When 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
$Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$.

Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
We define our robust objective as   
\[
 \begin{array}{ll}
& F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)\\
:=& 
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2-\epsilon \zeta |
\end{array}
  \]  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  
 
  
  
  
  
  
  
  
  
  
  
  
  
  
% % \paragraph{Mathematical formulation: sparse plus gaussian signal with additional noise}

% % \BIT
% % \item
% % Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
% %  \item
% % The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
% % \item
% % $Z_1$ is IID sampled from  $N(0,I)$, $Z_2$ is IID sampled from  $N(0,I)$, they are independent.
% % \item
% % \[
% % \begin{array}{ll}
% % Y&= a* (X+\sigma_1 Z_1) + \sigma_2 Z_2\\
% % &= a* (X+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)\\
% % &= a* (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \end{array}
% % \]
% % let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, if we condition on $I$ fixed, then 
% % \[
% % \begin{array}{ll}
% % (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \sim N(0, (I+\sigma_1+\sigma_2 C_a^{-1} )(I+\sigma_1+\sigma_2 C_a^{-1} )^T)
% % \end{array}
% % \]
% % then let $\tilde{\psi} := w*a$,  
% % \[
% %  \begin{array}{ll}
% % \Expect|(w*Y)_0|
% % &= \Expect|\psi^T (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)| \\
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% % \end{array}
% %   \]

% % \EIT



% % \paragraph{The original convex problem analysis}
% % We still analyze 
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   & \Expect|(w*Y)_0|\\
% % \mbox{subject to}  
% % & v^T w =1,
% % \end{array}
% %   \]
% %   Which is 
% %   \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   &\sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2\\
% % \mbox{subject to}  
% % & u^T \psi =1,
% % \end{array}
% %   \]
% %   for $u = \tilde{a}^{-1}*v$.
% %  The subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % \partial [\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 ]
% % &= 
% % \Expect_I [N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
% %   the projected subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [
% % N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
  
% %   First the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| (I_0+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| (1+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_1 e_0+\sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
  
%  \paragraph{Study inner Gaussian noise only }
% %  First, we study the case when $\sigma_2 = 0$, $0<\sigma_1<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} | I_0+\sigma_1|
% %  &=p| 1+\sigma_1|+(1-p)| \sigma_1|\\
% %  &=p +\sigma_1
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( e_0\cdot (I+\sigma_1) )]
% % &= P_{u}^{\perp} e_0
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u=e_0$.
  

  
  
  
  
%   \paragraph{Study outer Gaussian noise only }
% %  First, we study the case when $\sigma_1 = 0$, $0<\sigma_2<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| I_0\cdot e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( I_0\cdot e_0+\sigma_2
% %  a^{-1} )]
% % &= P_{u}^{\perp} [p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )]
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u$ is along the direction of $p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )$.
  
  
%   \paragraph{Possible  goal}
%   \BIT
%   \item
%   Show that for minimizer $\psi^*$ of the noisy objective
%   \[
%  \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2 
%   \]
%   is small and bounded by $\sigma_1$ and $\sigma_2$.
  
  
  
%   \begin{lemma}
%   We get the upper bound and lower bound of optimal objective value between the noisy and the noiseless setting
%   \[
%   \Expect_I \|I\cdot e_0\|_2  \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2\leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  
%   \]
%   \end{lemma}
  
%     Now we get the bound of objective value between the noisy and the noiseless setting
%   \begin{lemma}
%   \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  p(\| (1+\sigma_1)e_0+\sigma_2
%  a^{-1}\|_2-1)+(1-p)\| \sigma_1 e_0+\sigma_2
%  a^{-1}\|_2 
%   \]
%     \[
%   \Expect_I \|(I\cdot+\sigma_1)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  \sigma_1
%   \]
%   \end{lemma}
%   \item
%   Describe the minimizer $\psi^*$ of the noisy objective by 
%      \[
%  \begin{array}{ll}
% 0= P_{u}^{\perp} \Expect_I [
% N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^* )]
% \end{array}
%   \]
%   Then find a norm $d$ so that
%   $
%   d(\psi^*, e_0) 
%   $
%   or
%   $
%   d(w^*, a^{-1}) 
%   $
%   is bounded by $\sigma_1$ and $\sigma_2$
%   \EIT
   
   
%  \paragraph{Lemma for expectation}  
%   Mimic the lemma from previous section, we know that 

% \begin{lemma} \label{lem:BGPropLemmaSub}
% \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq  \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
%   \[
%   \bar{B}(k-1;n,p) \cdot \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} + (1- \bar{B}(k-1;n,p)) \cdot \|(\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
% where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
% is the survivor function (Complementary CDF) of the Binomial.
% \end{lemma}



% \begin{lemma} 
% There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
% and so that for each $N$ and for each 
% vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
% \beq \label{eq:LemmObjNoise}
%  (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq 1 + \eps_N .
% \eeq
% \end{lemma}

 
 
 
%  \paragraph{Bound on objective and subgradient}
%   Using the lemma, we could link the objective to $2-$norm of $\phi^* = e_0 + \psi^*$, 
%   \[
%     \begin{array}{ll}
%   \|\psi^*-e_0\|_2 = \|\phi^*\|_2 
%   \end{array}
%   \]
  
  
  

% Define the following notation for function, where $I$ is a fixed support, 
% \[
%  \begin{array}{ll}
% F_1(\phi) &:=   \|(1 +\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F_I(\phi) &:=   \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F^E(\phi)&:= \Expect_I F_I(\phi)   
% \end{array}
% \]
% then
% \[
%  \begin{array}{ll}
% \partial  F_I(\phi) &:= N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi) )\\
% \partial F^E(\phi)&:= \partial \Expect_I F_I(\phi)  =   \Expect_I \partial  F_I(\phi)
% \end{array}
% \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% Using Lebourg’s mean value theorem, Theorem 2.3.7 of Clarke (1990) \cite{clarke1990optimization}, there exists $ t \in (0,1),$ so that
% \[
%  \begin{array}{ll}
% \Expect_I F_I(0) -   \Expect_I F_I( \phi^*)\in \langle  
% \partial \Expect_I F_I( t\phi^*), \phi^* \rangle
% \end{array}
% \]



%   We want to bound the finite difference:
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 } \in \langle  
% \partial \Expect_I F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
    
% % \frac{|\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi^*)\|_2| }{\|\phi^*\|_2 } 
% \end{array}
%   \]
%  And since $t\neq 1$, $\Expect_I N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) )$ is not a set but just a unit vector,
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
  
%   Since $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*)>0$ when the minimizer $\phi^*$ is not $0$, in this case,  a natural bound is
%   \[
%     \begin{array}{ll}
%  0 <  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   More specifically, there exists $\rho>0,$ 
%     \[
%     \begin{array}{ll}
%  \rho \leq  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   Therefore, using the fact that 
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 }  \in [\rho,1]
% \end{array}
%   \]
%  We could bound $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) $ by bound $\|\phi^*\|_2$.
   
   
% For $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
 
 
% We need a new lemma for subgradient, 
% % \begin{lemma} 
% % \beq \label{eq:LemmSubGradNoise}
% % C_{-}'  \leq  \frac{\partial\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\partial\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq C_+' .
% % \eeq
% % \end{lemma} 
 
%  \begin{lemma} 
%  For the minimizer $\phi^*$ so that $u^T \phi^* =0$,
% \beq \label{eq:LemmDirGradNoise}
% C_{-}  \leq  \frac{ \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   }{ \langle   \partial F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%  }  = \frac{\Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]}{\cos[\angle( (1+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]} \leq C_+ .
% \eeq
% \end{lemma} 
% \begin{proof}


% \begin{eqnarray*}
% & & E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   \end{eqnarray*}
 
 
% Using the fact that $\phi^*$ is minimizer,  we know that for any $\beta$ so that $u^T \beta = 0, \|\beta\|_2=1$,
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &\geq& 0
%   \end{eqnarray*}
% where
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &=& E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) ), \beta \rangle
%   \end{eqnarray*}
% It requires
% \begin{eqnarray*}
% 0 \in \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n}  P_{u}^{\perp} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) )
%   \end{eqnarray*}




%   \end{proof}   






















==> old_sec/sec_old/Noise_updated.tex <==
\section{Stability for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $\zeta_1$ and $\zeta_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 \zeta_1+  \sigma_1 G_1) + \eta_2 \zeta_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 

  
In the following,
let 
\[
D_R( \psi) :=  F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)-F_{0,0,0,0}(\psi).
\]
We use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$

Let $\phi^\star := \psi^\star-e_0$,
we have
   \[
 \begin{array}{ll}
D_R( e_0) &= F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)\\
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,\phi^\star) \|\psi^\star-e_0\|_2\\
 &\geq p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G| = \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
  \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_Monot}
$\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
\end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
\end{lemma}


\paragraph{Robust optimization}
% We want to find the min-max value 
% \[
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta)
% \]
% for a function $H$,
% \[
% H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
% \]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


% \begin{lemma}
% \label{min-maxError}
% For $A>0$, 
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
% \end{array}
% \]
% where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
% \end{lemma}
% \begin{lemma}
% \label{min-maxErrorL_p}
% Let
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
%  \end{array}
%   \]
%   where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
%   then
% \[
%  \begin{array}{ll}
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta) = 
% H( \mu(\psi))
% \end{array}
% \]

% \end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
%  \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
%  \end{array}
%   \]
 \[
 \begin{array}{ll}
 \mu(\psi) &=\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}\\
 \sigma_n^2(\psi) &=  \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}\Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2 |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}[\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
 
 The second inequality comes from the fact that $\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
  
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
For $p<p^\star_1 = 1-\tan(\theta),$
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2\leq 
  \frac{(1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

 
\end{theorem}  
\begin{proof}
 Since
 \[
 \begin{array}{ll}
  B(p,\phi^\star) \|\phi^\star\|_2\leq 
 D_R(e_0) = F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0) 
\end{array}
  \] 
  and
   \[
 \begin{array}{ll}
 p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2\leq  B(p,\phi^\star) \|\phi^\star\|_2 
\end{array}
  \]  
  where
\[
 \begin{array}{ll}
 D_R(e_0) = (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{proof}
\begin{coro}
When $\sigma_1 = \sigma_2 = 0,$
 \[
 \begin{array}{ll}
\|\psi^\star -e_0\|_2\leq 
 \frac{p\mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}

\begin{coro}
When $\eta_1 = \eta_2 = 0,$
 \[
 \begin{array}{ll}
 \|\psi^\star -e_0\|_2\leq 
 \frac{ (1-p) \sigma_n(e_0)^2 +  
 p\sqrt{1+ \sigma^2_n(e_0)}  - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}








\subsection{All the proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



% \subsection{Constrained Convex algorithms }
%  \paragraph{Constrained noisy convex problems}
% Then we define the constrained convex program that allows noise,
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,z}   & |\alpha| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
% \label{eq:ConstrainProb}
%   \]
%   If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \zeta^2 \leq 1
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
%   \]
% If we set $\epsilon = 0,$ then we recover 
% the original convex problems for noiseless setting
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
% \mbox{subject to}  
% & v^T w =1,
% \end{array}
% \tag{$P_1$}
%   \]

==> old_sec/sec_old/Noise_updated_constraint.tex <==
\section{Stability for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )-\epsilon \zeta|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2]-\epsilon \zeta |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )-\epsilon \zeta|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 
In the following, we use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$
   \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,N) \|\psi^\star-e_0\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
% hence
% \[
%  \begin{array}{ll}
% E_G |\mu+ \sigma G|
% &\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
% \end{array}
% \]
\end{lemma}


\paragraph{Robust optimization}
We want to find the min-max value 
\[
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta)
\]
for a function $H$,
\[
H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
\]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
For $A>0$, 
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{lemma}
\label{min-maxErrorL_p}
Let
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
 \end{array}
  \]
  where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
  then
\[
 \begin{array}{ll}
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta) = 
H( \mu(\psi))
\end{array}
\]

\end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

\subsection{Proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]

==> old_sec/sec_old/Numerical.tex <==

\section{Numerical experiments}
We set up a ground truth inverse filter as $a^{-1} = (0.5, 1, 0.5)$, and numerically run $10$ independent experiments of finding the inverse filter by the convex problem 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}^T$ }
\EEQ
We choose an accuracy $\epsilon = 10^{-3}$ and count the number of successfully accurate recovery of $a^{-1}$ where $\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<\epsilon$. We see a consistent sharp transition of success rate from $0$ to $1$ in a narrow parameter region.
\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/phase_transition_detail.png}
\caption{The finite sample phase transition phenomenon, where $a^{-1} = (0.5, 1, 0.5)$,  $x-$axis is the sparsity level $p$, $y-$axis is the empirical probability $P(\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<10^{-3})$. Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}

==> old_sec/sec_old/Phase_Transition.tex <==

\subsection{Population Phase transition theorem}
Qingyun: Old proof without subgradient language:

\paragraph{Population phase transition theorem}
\begin{theorem}
Under the previous assumption,
$
         p^\star   =\frac{\sin{\theta}}{\sin{\theta}+ \cos{\theta}} .
$
 The solution of  $P_{1,v}$ is $w^\star$, then 
 $w^\star$ is $a^{-1}$ up to shift and scaling provided $p<p^\star$,
and  $w^\star$ is not $a^{-1}$ up to shift and scaling provided $p> p^\star$.
  \end{theorem}
The population phase transition diagram is in figure~\ref{fig-PT}.

\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/Phase_T_sine.png}
\caption{The population phase transition diagram derived from theory for planted sparsity projection pursuit, $x-$axis is $\sin{\theta}$, $y-$axis is the sparsity level $p$ . Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}

\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/PT_BD_1root_pure.png}
\caption{The finite sample phase transition diagram when ground truth filter is $w^\star = (0,1,s)$ with $T=200$.$x-$axis is sparsity level $p$ ranging from $0.01$ to $0.99$ with step size $0.01$, $y-$axis is $\tan(\theta)=\| w_{(0)}^\star \|_2$, ranging from $0$ to $0.99$ with step size $0.02$.  Red part is failure, Blue part is success. The success probability is calculated over $10$ independent repeated experiments solved by cvx in matlab. }
\label{fig-PT-finite}
\end{figure}



% \begin{theorem} \label{lem:ica}
% We observe a sequence $Y\in \reals^n$, and we know that there exists a ground-truth filter $w^0$, such that $w^0*Y = X$, $X$ satisfy Bernoulli$(p)$-Gaussian model.  
% And we assume that we have a solution $w^\star$ to the Sparse convolutional ICA problem.
% Then if the angle $\theta$ between the vector $v$ and $w^0$ and the sparsity level $p$ satisfy that 
% \[
% \frac{p}{1-p}<\gamma \cot(\theta),
% \]
% then  $w^\star$ equals $w^0$ up to scaling, namely $w^\star = cw^0$ for $c\in \reals$ with probability $1-\exp\left( -C_0 \kappa_{w^0}^{-2} k\log(kp)\right)$, where $C_0$ is a constant, $\kappa_{w^0}$ is the condition number of the circulant matrix generated by $w^0$.

% \end{theorem}


\paragraph{Proof of the population phase transition theorem}
\BIT
 \item
  Let $\phi  := \psi -e_0 = \tilde w*\tilde a -e_0,$  then $|[w*Y]_0| = |[(e_0 +\tilde \phi)*X]_0| =  |[(e_0 + \phi)^T X| $, we define
  \[
  L(\phi) = |[(e_0 + \phi)^T X|.
  \] 
  WLOG, we can assume the ground truth $a^{-1}$ is scaled so that $v^T \tilde{a}^{-1} =1$
%   , then after the change of variable $w =  a^{-1}*(e_0 +\phi)$,  the condition $v^T w = 1$ can be transformed to $u^T \phi = 0$ where 
% $u: =\tilde{a}^{-1}*v$.

  We want to find a threshold $p^\star$ so that for all $p<p^\star$, the directional derivative  $ \Expect \nabla_{\phi}{L}|_{\phi = 0}>0$ for all directions $\phi$ that satisfy $u^T \phi = 0$.

 We define the finite difference
  \[
  D = L(\phi)-L(0) =  |[(e_0 + \phi)^T X| -|X_0| 
  \]
  Let $\epsilon : = \|\phi\|_2 $ and taking limit of $D$ as $\epsilon  \rightarrow 0,$ we have
    \BEQ
  \begin{array}{ll}
   \expect D &=  p\expect[D\mid X_0 \neq 0 ] + 
   (1-p)\expect[D \mid X_0 = 0 ] \\
   &=  p\expect[\mbox{sign}(X_0) ( \phi_0 X_0 + \sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid   \\
   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  
   \end{array}
 \EEQ
The last equality is because 
 $
 \expect[\mbox{sign}(X_0) (\sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] = 0 
$
 as $X_j$ are sampled independently. Notice that for Bernoulli Gaussian $X$,
$
\Expect [|X_0|\mid X_0 \neq 0 ]=\sqrt{\frac{2}{\pi}}.
$
 
 Then  $ \Expect \nabla_{\phi}{L}|_{\phi = 0} = \Expect \lim_{\epsilon \rightarrow 0}\frac{D}{\epsilon}>0$ 
 in case either $\phi_{0} > 0$, or in case $\phi_0 < 0$ and
\[
          \frac{p}{1-p} < \frac{ \Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  }{|\phi_0| 
          \Expect [|X_0|\mid X_0 \neq 0 ]} = \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} \frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\|\phi_{(0)}\|_2 \sqrt{\frac{2}{\pi}}}  .
\]
Here  $X_{(0)} = (X_i)_{i\neq 0}$
\item (Geometric lower bound:)
Using the fact that $u^T \phi = 0$. We define $v = \cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$, then $u =\tilde{a}^{-1}*v = \tilde{a}^{-1}*(\cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2})^{\bot}) =\cos{(\theta)} \frac{e_0}{\|\tilde{a}\|_2}+\sin{(\theta)} \tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot} $, 
where $\tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$ is perpendicular to $e_0$, 
therefore, 
$0= u^T \phi = \frac{1}{\|\tilde{a}\|_2}[\cos{(\theta)} \phi_0+\sin{(\theta)} \phi_{(0)}]$, therefore,  
$\frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} = \frac{\cos(\theta)}{\sin(\theta)} =\cot(\theta).$
\[
 \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|}\geq  \cot(\theta)
 \]

 
% \item 
% Let $h=\phi$, i.e. $h_i=\phi_{-i}$; and let $h_{(0)} = (h_i)_{i\neq 0}$, then
%   \[
%           \frac{p}{1-p} < \frac{ \Expect | h_{(0)}^T X_{(0)} |}{| h_{0}| \Expect |X_0|} = \frac{ \Expect | h_{(0)}^T X_{(0)} |}{\|h_{(0)}\|_2 \Expect |X_0|}  \frac{\|h_{(0)}\|_2}{| h_{0}|} .
% \]
\item
We showed that for IID Bernoulli Gaussian $X$,
\[
\frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\sqrt{\frac{2}{\pi}} \|\phi_{(0)}\|_2} = \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \in [p,1)
\]
Using semicontinuous extension, we can choose sequence of $\phi$ that is dense on doubly infinite sequence space $V_{-\infty, \infty}$, then we know that $\frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2}$ should be replaced by its semicontinuous extension on $V_{-\infty, \infty}$, which is $1$.

The phase transition $p^\star$ is the smallest $p$ so that 
\[
          \frac{p}{1-p} \leq  \cot(\theta) \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \leq  \cot(\theta).
\]
%  \BEQ
%   \begin{array}{ll}
%   \Expect D 
%   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  \\
%   &=  
%   \sqrt{\frac{2}{\pi}}\|{\phi}_{(0)}\|_2[ p (\mbox{sign}(\phi_{0})\tan(\theta)) + (1-p) (1-(1-p)^{\|{\phi}_{(0)}\|_0})]
%   \end{array}
%  \EEQ
Therefore,  generically, $ \frac{p^\star}{1-p^\star}  = \cot(\theta) $.
\EIT

==> old_sec/sec_old/Planted_Proj.tex <==
% \section{Projection pursuit for planted sparsity}
% \subsection{Setup} 
% \subsection{Perturbation analysis}
% First, without loss of generality, we suppose  there is a vector $\beta$, $\beta^T \Phi Y = X_0$.

% Consider a vector  $b $ which is a small perturbation of $\beta$, where
% $\beta^T \Phi =e_0$, we assume $ \cM_1$ is the constraint set for $b$. Let $b = \beta + \eps \delta$ where $\delta \in T_\beta \cM_1$, the tangent space at $\beta$. We assume the condition $\delta \in T_\beta \cM_1$ is given by $v^T \delta = 0$.


% Let $h = \Phi^T \delta$, then from $   v^T \delta = 0$, we have $   u^T h = 0$, where $ v = \Phi u$. We have
% \[
%     b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
% \]
%  where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 
%  Let 
% \[
% D_0 =  |(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -|X_0|, 
% \]
 
 
 
%  Then for sufficiently small $\eps$
% \begin{eqnarray*}
%  E D_0 = E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
%  (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot p+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot (1-p),
% \end{eqnarray*}
%  where $p = P(X_0\neq 0)$.
 
%  The perturbation increases the objective value 
% just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

% Now we consider the optimization problem
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
%     \mbox{ subject to }&  h_{0} = -1, \\
%     & h\in \Phi^T T_\beta \cM_1.
% \end{eqnarray*}


% We know $h = \Phi^T \delta$, then 
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
%     \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
%      & \delta \in T_\beta \cM_1.
% \end{eqnarray*}

% \subsection{Geometric lower bound}
% We know that from perturbation analysis, the condition for phase transition are
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

%  We know $X_0$ is random variable sampled from a symmetric distribution with atom at $0$, $F_p = p H +(1-p) F$, and $X_i, \quad i\neq 0$ are sampled from distribution $G$.
% Using the sparsity of $X_0$,
% \[
% E \{ D_0 | X_0\neq 0 \}  = (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0|.
% \]
% And
% \[
% E \{ D_0 | X_0 =  0 \}  = E{|h_{(0)}^T X_{(0)}| }.
% \]

% First, when $F_t$ are all Gaussian distributions for $t\neq 0$, we leverage the invariance property for linear transform of Gaussian, and get 
% \[
% E{|h_{(0)}^T X_{(0)}| } = \|h_{(0)}\|_2 E|G| = \sqrt{\frac{2}{\pi}} \cdot \|h_{(0)}\|_2.
% \]

% % And we have calculated $E{|h_{(0)}^T X_{(0)}| }$ for different cases of $F_t$. 
% % For example, it is  lower bounded by  a constant multiple $\|h_{(0)}\|_2$ .

% And since we know $v^T h=0$, when $X_i$ are IID Gaussian, then linear combination of Gaussian are still Gaussian, so without loss of generality, we can change coordinate and assume $h = h_0 e_0 + h_1 t_1 + h' $, where $e_0$ is the unit vector in the direction of ground truth, $t_1$ is the unit vector in the direction of the component of $v$ normal to $e_0$, and $h'$ is in the rest of directions .

% Then we have $\|h_{(0)}\|_2\geq |h_1|$,
% and 
 
% \[
%           \frac{1-p}{p} <  \frac{  |h_1|} {| h_{0}|} = \cot(\theta).
% \]


\section{Phase transition for sub-Gaussian}
From the Khinthine’s inequality for sub-Gaussian and $p = 1$, we have 
\[
E{|h_{(0)}^T X_{(0)}| }\geq  3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2,
\]
for Bernoulli-SubGaussian, we have,
\[
E{|h_{(0)}^T X_{(0)}| }\geq  (1-(1-p)^M)^{1/2} 3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2.
\]
In general, we define
\[
\gamma(F,p) = E{|h_{(0)}^T X_{(0)}| }/\|h_{(0)}\|_2 E |X_0|,
\]
as the ratio between the linear combination $E{|h_{(0)}^T X_{(0)}| }$ for $\|h_{(0)}\|_2=1$ and $ E |X_0|$.

Then we need
\[
          \frac{1-p}{p} < \frac{ \gamma(F,p)  \|h_{(0)}\|_2}{| h_{0}|}
\]
for all $h$ such that $   u^T h = 0$ .

Also, using the fact that
 
\[
         \frac{  \|h_{(0)}\|_2} {| h_{0}|} \geq \cot(\theta).
\]
we have 
\[
          \frac{1-p}{p} <\gamma(F,p) \cot(\theta).
\]

\section{Noisy  signal}
 \subsection{Folder Gaussian}
 For a Gaussian RV $Z \sim N(\mu, \sigma)$, then for RV $|Z|$,  
 \[
 \mu_{|Z|} = E|Z|=\sqrt{\frac{2}{\pi}}\sigma e^{-\frac{\mu^2}{2\sigma^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma}\right) \right] 
%  = f(\mu,\sigma),
 \]
  \[
 \sigma_{|Z|}^2 = \mu^2 + \sigma^2 - \mu_{|Z|}^2.,
 \]
%  Then for fixed $\sigma$, let
%  \[
%  h_\sigma(\mu) = f(\mu,\sigma) 
%  \]
%  then 
%   \[
%  h'_\sigma(\mu) = 
%  \]
 
 \subsection{Noisy perturbation analysis}
Consider a noisy perturbation $\bar X_i  =  X_i + \sigma  E_i $, where $E_i$ is standard Gaussian $N(0,1)$, $ X_i = B_i Z_i$ are iid product of Bernolli RV with parameter $p$ and subGaussian unit variance RV with c.d.f $F$. 

Then we let $b^{\sigma}$ be the solution of the optimization problem 
\[
E D_\sigma = E_X E_E( |(1+ \eps h_0)(X_0+\sigma  E_0) +  \eps h_{(0)}^T (X_{(0)}+\sigma  E_{(0)})| -|X_0+\sigma  E_0|)
% = E_X (h'_\sigma(\mu)), 
\]
for sufficiently small $\eps$, and fixed $\sigma<1$, we consider the asymptotic analysis when $\eps  << 1 $， $ \sigma<< 1 $. We know $\sigma ((1+ \eps h_0)(  E_0)+\eps h_{(0)}^T  E_{(0)}))$ is a centered Gaussian with standard deviation 
\[\sigma\sqrt{(1+ \eps h_0)^2+(\eps h_{(0)})^2}\approx \sigma(1+ \eps h_0)
\]
therefore,
\begin{eqnarray*}
 E D_\sigma &\approx&   E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}+\sigma (1+ \eps h_0) E_0| -E|X_0+\sigma  E_0| \\
 &\approx& 
  p \cdot(|1+\eps \cdot  h_{0}|-1) \cdot E |Z_0+\sigma  E_0| + (1-p) \cdot ( E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|} ),
\end{eqnarray*}
 where $p = P(X_0\neq 0)$.
 
 First we derive lower bounds,
 \[
 E |Z_0+\sigma  E_0|
 \geq E |Z_0| - E|\sigma  E_0| =   E |Z_0| - \sqrt{\frac{2}{\pi}}\sigma,
\]
 \begin{eqnarray*}
 E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|}&\geq& E{|\eps  \cdot h_{(0)}^T X_{(0)} | -2 E|\sigma  E_0|} \\
 &=&  E|\eps  \cdot h_{(0)}^T X_{(0)} | -2 \sqrt{\frac{2}{\pi}}\sigma
\end{eqnarray*}
Then we have 
\begin{eqnarray*}
 E D_\sigma 
\geq  E D_0 - (p+2(1-p)) \cdot \sqrt{\frac{2}{\pi}}\sigma.
\end{eqnarray*}

Therefore, in the existence of noise, we don't have exact recovery result, but we would have a lower bound. 
 
 Second, we use the mean of folded Gaussian to compute the condition expectation.
 
 Here, for a fixed $\mu$, we rescale the variance $\sigma' = \sigma/\eps$. Under the assumption $\eps/\sigma<< 1 $, using asymptotic expansion, we can compute the condition expectation 
 \begin{eqnarray*}
   E({|\mu+\sigma'  E_0| -|\sigma'  E_0|}\mid \mu)
 &=& \sqrt{\frac{2}{\pi}}\sigma' e^{-\frac{\mu^2}{2\sigma'^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma'}\right) \right] - \sqrt{\frac{2}{\pi}}\sigma'
 \\
 &\approx& -\sqrt{\frac{2}{\pi}}\sigma' {\frac{\mu^2}{2\sigma'^2}}+\mu\sqrt{\frac{2}{\pi}}(-\frac{\mu}{\sigma'}  )
 \\
  &=&- \sqrt{\frac{2}{\pi}}  {\frac{3\mu^2}{2\sigma'}}  
\end{eqnarray*}
The first equality is the formula for the mean of folded Gaussian.
The second equality uses the Taylor expansion of Gaussian c.d.f
\[
\Phi (z)  = \frac{1}{2}+  \frac{1}{\sqrt{\pi}} \left(z-\frac{z^3}{3}+\frac{z^5}{10}-\frac{z^7}{42}+\frac{z^9}{216}-\cdots\right)
\]

 Therefore, for $Z_0$ standard Gaussian,
  \begin{eqnarray*}
 E_X E_{E_0}(|Z_0+\sigma  E_0|) 
  &=&  \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}  
\end{eqnarray*}
 \begin{eqnarray*}
 E_X E_{E_0}({|\eps  \cdot h_{(0)}^T X_{(0)} +\sigma  E_0| -|\sigma  E_0|}) 
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{E_X( h_{(0)}^T X_{(0)})^2 }{2\sigma'}}  
   \\
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2\sigma'}}  
\end{eqnarray*}

Then 
\begin{eqnarray*}
 E D_\sigma 
 &\approx& 
 \eps \left[ p \cdot h_{0} \cdot \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}    - (1-p) \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2(\sigma/\eps)}} \right] .
\end{eqnarray*}



 

==> old_sec/sec_old/Population.tex <==
\section{Population problem}
\subsection{Population problem setting}
\paragraph{Doubly infinite sequence setting}
First, we study the population objective under doubly infinite sequence setting:
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let  $(Y_t)$ defined by $Y_t \equiv \sum_{h\in \integers} a_h X_{t-h}$ be a linear process, i.e.
\[
Y= a* X,
\]
\EIT

\paragraph{Population problem objective}
Due to shift invariance, the population loss is
 \[
 \Expect |[w*Y]_0| = \Expect |\tilde{w}^T Y| 
 \]
 where $\tilde{w}_i = w_{-i}.$

From the ergodic property of stationary process,
 \[
\Expect\frac{1}{N} \| w*Y\|_{\ell_1(\cT)} = \Expect |[w*Y]_0|
  \]
 Due to shift invariance, we only need to study 
 \[
 \Expect |[w*Y]_0| = \Expect |\tilde{w}^T Y| 
 \]
 where $\tilde{w}_i = w_{-i}.$
\paragraph{Population problem formulation}
Now we state the theorem for a general doubly infinite sequence $v$ with unit $2$ norm, we assume that $v$ and $a$ are not orthogonal so that the angle $\theta$ between $v$ and $a$ satisfies $\cos{\theta} = a^T v /\|a\|_2>0$, $\sin{\theta}\geq 0$. Then we define the optimization problem $P_{1,v}$ over  $w \in l_1(\integers)$  as
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \expect |\tilde{w}^T Y|\\
 \mbox{subject to}  
&  v^T w =1.
\end{array}
\tag{$P_{1,v}$}
\EEQ
% Without loss of generality, we could rescale $a$ so that
% \[
% v^T a^{-1} =1.
% \]
\paragraph{Change of variable}
We define global change of variable over the paper:
\[
\psi := \tilde{w}*\tilde{a}
\]
then
\[
 \tilde{\psi} :=w*a
\]
\[
 \tilde{\psi}*Y :=w*a*X
\]
also let $u$ be a unit vector along the direction of $C_{\tilde{a}}^{-1} \tilde{v}$
\[
u:= C_{\tilde{a}}^{-1} \tilde{v}/\|C_{\tilde{a}}^{-1} \tilde{v}\|_2 = \tilde{a}^{-1}* \tilde{v} /\|\tilde{a}^{-1}* \tilde{v}\|_2.
\]
then $ \theta =\angle({v, a}) = \angle({u, e_0})$.

Without loss of generality, we could rescale $v$ so that
\[
\|\tilde{a}^{-1}* \tilde{v}\|_2 = \| a* v\|_2 =1.
\]

% Leverage translation invariance, WLOG, we assume that the $0$-index achieves the maximum in absolute value, then  $  \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} =  \frac{1}{N}(w*Y)_0 =  \frac{1}{N}\Tilde Y^T w.$

% Then we have
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N}\Tilde Y^T w = 1.
% \end{eqnarray*}

\paragraph{Projection pursuit with linear constraint}
The population problem becomes the \textbf{convex projection pursuit problem with linear constraint}
\BEQ
 \begin{array}{ll}
  \underset{\psi \in V}{ \mbox{minimize} }  &  \expect |\psi^T X|\\
 \mbox{subject to}  
&  u^T \psi =1.
\end{array}
\tag{$P_{1,v}$}
\EEQ
\paragraph{Other objectives}

After the change of variable, $\tilde{\psi} :=w*a$, we have
% For $\ell_1/\ell_2$ ratio, we propose to use a non-convex (convex objective concave constraint) problem for blind deconvultion:
\begin{eqnarray*}
    (\ell_1/\ell_2) \qquad  \min&    \frac{1}{N} \| \tilde{\psi}*X\|_{\ell_1(\cT)}\\
    \mbox{ subject to }&   \frac{1}{N} \| \tilde{\psi}*X\|_{\ell_2(\cT)} =1 .
\end{eqnarray*}

In population, since $\E | \psi^T X|^2 = p\|\psi\|_{\ell_2(\cT)}$, we have
\begin{eqnarray*}
    (\ell_1/\ell_2) \qquad  \min&    \E | \psi^T X|\\
    \mbox{ subject to }&   \E | \psi^T X|^2 =p\|\psi\|_{\ell_2(\cT)} =1 .
\end{eqnarray*}
% Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| \tilde{\psi}*X\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N} \| \tilde{\psi}*X\|_{\ell_\infty(\cT)} = 1.
% \end{eqnarray*}

% Dave: This is bad since the max stats could be very large for Bernoulli Gaussian or Cauchy.
% This might work for digital PAM +-1 signal.


% In population, since $\E | \psi^T X|^2 = p\|\psi\|_{\ell_2(\cT)}$, we have
% \begin{eqnarray*}
%     (\ell_1/\ell_\infty) \qquad  \min&    \E | \psi^T X|\\
%     \mbox{ subject to }&  \frac{1}{N}  \E  \| \tilde{\psi}*X\|_{\ell_\infty(\cT)} = 1 .
% \end{eqnarray*}


\paragraph{Projection pursuit with sphere constraint}
We comment that the results we derive in the following sections are also applicable to the projection pursuit (orthogonal dictionary learning) problem.
\begin{lemma}
The problem
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect |\psi^T X|  \\
\mbox{subject to}  
&\Expect |\psi^T X|^2 \geq \Expect (X_0)^2
\end{array}
  \]
is equivalent to the following convex-concave problem
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
\mbox{subject to}  
&\|\psi\|_2^2 \geq 1
\end{array}
  \]
We claim that  it has the same minimizer as the \textbf{ projection pursuit (orthogonal dictionary learning) problem with sphere constraint}.
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect_I \|\psi_I\|_2  \\
\mbox{subject to}  
&\|\psi\|_2 = 1
\end{array}
  \]
  which is also equivalent to
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect_I \|\psi_I\|_2/\|\psi\|_2 
\end{array}
  \]
  And  also equivalent to
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect |\psi^T X|/\sqrt{\Expect |\psi^T X|^2} 
\end{array}
  \]
\end{lemma}


\subsection{Inverse filter}
\paragraph{Fourier transform and inverse filter}
The discrete-time Fourier transform $\mathcal{F}$ is defined by $\mathcal{F} a = \hat{a}$ where
\[
\hat{a}(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [-\frac{1}{2}, \frac{1}{2}];
\]
the inverse Fourier transform $\mathcal{F}^{-1}$ is defined by
\[
(\mathcal{F}^{-1} f)(n) =  \int_{-\frac{1}{2}}^\frac{1}{2} f(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
\]
Now, our condition on the filter $a$ is:
\[a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.
\]
In the following theorem, we show that this condition would provide the existence of an inverse filter in  $l_1(\integers)$.
\begin{theorem}
If $a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T,$ we could define the inverse filter of $a$ as
$$a^{-1} := \mathcal{F}^{-1}(\frac{1}{\mathcal{F} a})$$
so that $a^{-1}*a = e_0.$ Here $e_0$ is the sequence with $1$ at $0$ coordinate and $0$ elsewhere.
From Wiener's lemma on $\mathcal{F} a$,   $a^{-1} \in l_1(\integers)$ .
\end{theorem}

\begin{lemma}{\textbf{Wiener's lemma:}}
Assume that a function $f$ on unit circle has an absolutely converging Fourier series, and $f(t)\neq 0$ for all $t \in T$, then $1/f$ also has an absolutely convergent Fourier series.
\end{lemma}





==> old_sec/sec_old/Projection_set_up.tex <==



\section{Population loss and phase transition}
We first study population loss of the sparse deconvolution problem
 \begin{eqnarray*}
    (\mbox{Population sparse deconvolution}) \qquad  \min_{w\in \reals^k} &    
    E\| w * Y\|_1\\
    \mbox{ subject to }&  v^T w = 1,\\
    &  w\in \cM.
\end{eqnarray*}
\subsection{Population loss of projection pursuit}
Let's first consider the population objective $E|w^T \Phi X|$.

Consider a vector  $w \in \cM$ which is a small perturbation of $w^\star  \in \cM$, where
$w^T \Phi =e_0$. Let $w = w^\star + \eps \delta$ where $\delta \in T_{w^\star} \cM$, the tangent space at $w^\star$. And since $\delta \in T_{w^\star} \cM_1$ is a subspace, we assume the constraint is given by $M \delta = 0$.
Let $h = \Phi^T \delta$, then $   u^T \delta = 0$, where $ v = \Phi u$. We have
\[
    b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
\]
 where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 \subsection{Population phase transition}
 We want to study $E D =  E|(1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)}| -E|X_0|$.
 
 Then for sufficiently small $\eps$
\begin{eqnarray*}
 E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
 (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot (1-\eta)+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot \eta,
\end{eqnarray*}
 where $p = P(X_0=0)$.
 
 The perturbation increases the objective value 
just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
\[
          \frac{\eta}{1-\eta} > \frac{| h_{0}| E |X_0|}{ E | h_{(0)}^T X_{(0)} |. }
\]

Now we consider the optimization problem
\begin{eqnarray*}
    (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
    \mbox{ subject to }&  h_{0} = -1, \\
    & h\in \Phi^T T_\beta \cM_1.
\end{eqnarray*}


We know $h = \Phi^T \delta$, then 
\begin{eqnarray*}
    (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
    \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
     & \delta \in T_\beta \cM_1.
\end{eqnarray*}



Following the quadratic problem reduction, we can related $Q_1$ to the deterministic quadratic problem.

After the study of the general population model, we remark that for convolutional model, $A$ ad $B$ are both generated by the circular or Topelitz matrices from a single vector.





==> old_sec/sec_old/Regularized_Noise.tex <==
\subsection{Regularized convex problems}
\paragraph{Regularized convex problems}
For any $\epsilon>0$, we can find the Lagrangian form  of the constrained problem to define the regularized convex program, where we can find a corresponding $\lambda = \Lambda(\epsilon)$ so that $\frac{1}{2\lambda}$ is the dual variable.
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & |\tilde{w}^T Y -\zeta |+ \frac{1}{2\lambda}((\zeta)^2-\epsilon^2) \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
The convention to use for optimization is to ignorne the constant $-\epsilon^2$, and write the problem as
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2] \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
  Define soft-threshold operator as 
  \[
  S_{\mu}(x): = \sign (x) (|x| -\mu)_+
  \]
  and define its complement
   \[
  \bar{S}_{\mu}(x): = x-S_{\mu}(x) =  \sign (x)(x- (|x| -\mu)_+) =  \sign (x)\max(|x| ,\mu).
  \]
 \begin{lemma}
 If we partially minimize over $\alpha,$ the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
    \[
 \begin{array}{ll}
\mbox{inf}_{\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]   = [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 

\end{array}
  \]
  \end{lemma} 
  
  
 
\begin{proof}
Due to the proximal operator of $\ell_1$ norm,  the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
The objective can be further simplified to
  \[
 \begin{array}{ll}
&\Expect[|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]\\
=&\Expect[|S_{\lambda}(\tilde{w}^T Y)|+ \frac{1}{2\lambda}(\bar{S}_{\lambda}(\tilde{w}^T Y) )^2]\\
=& [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 
\end{array}
  \]
 \end{proof} 

Using the data generative model and do change of variable, 
the partially minimized regularized problem is
 \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi}   & \Expect[|(|\psi^T (X+\eta Z )|-\lambda)_+|+ \frac{1}{2\lambda}(\max(|\psi^T (X+\eta Z )| ,\lambda) )^2] \\
\mbox{subject to}  
& u^T \psi =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
%   For the regularized problem we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,  
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]
%   However, it seems hard to study it directly since its order is similar to $\inf_{\lambda} \sup_{Z: \|Z\|_2\leq 1}  \Expect \inf_{\zeta(\lambda)}$ .)
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]

==> old_sec/sec_old/Related_Work.tex <==
\section{Related work}
% Qingyun: Will turn these slides into proper writting latter, just trying to collect all the related reference for now.

Blind source seperation, cocktail party problem

ICA, sparse ICA

Projection pursuit (exploratory)

AR, non-causal AR (non-Gaussian)

dictionary learning


\paragraph{Prior work: analysis approach, non-Gaussianity, Ratio formulation}
  \begin{itemize}
  \item
  Key idea $1$: Find inverse filter $a^{-1}$ so that
$ a^{-1}*y = x $.
\item Key idea $2$: 
If $x$ is non-Gaussian, then $a*x$ is closer to Gaussian. 
\item Find $w\neq 0$  
\[
 \begin{array}{ll}
 \underset{w}{\mbox{maximize}}   & J(w*y)
\end{array}
  \]
\item Non-Gaussianity: $J$ is negative entropy function or normalized $4$-th order cumulant $J(z) = \frac{\|z\|_4^4}{\|z\|_2^4}$ \cite{wiggins1978minimum, donoho1981minimum}
  \item Sparsity: 
  $J(z) = - \| z\|_1/\|z\|_2$,  \cite{gray1979variable,donoho1981minimum,kijko1994seismological}.
  \item varimax norm: $\max_i \frac{|z_i|}{\|z\|_2}$ \cite{cabrelli1985minimum}
\end{itemize}




% Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} \geq 1.
% \end{eqnarray*}

% Leverage translation invariance, WLOG, we assume that the $0$-index achieves the maximum in absolute value, then  $  \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} =  \frac{1}{N}(w*Y)_0 =  \frac{1}{N}\Tilde Y^T w.$

% Then we have
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N}\Tilde Y^T w = 1.
% \end{eqnarray*}



\paragraph{Prior work: blind equalization for digital signal}
%   \begin{itemize}
% \item
% Digital signal: PAM signaling $\pm 1$ binary signal or QAM signaling with $|x|=1, x\in \complex$ \cite{kennedy1992blind,ding2000fast}. 
% \item More general,  $x$ are IID and bounded by $M = \mbox{max}(x_i)$ \cite{vembu1994convex,li2001blind}.
% \item 
%   Convex Cost Functions in Blind Equalization \cite{vembu1994convex}:
%   find $w$ so that $w*a = e_0 = (\ldots,0,1,0, \ldots)$ as minimizer of the ideal convex problem (
%  Not computable without knowing $a$!)
%   \[
%  \begin{array}{ll}
%  \underset{w}{\mbox{minimize}}   & \| w*a\|_1 
%  \\
% \mbox{subject to} 
% & (w*a)_0 = 1.
% \end{array}
%   \]  
  
%     \item
%   When $x$ are IID and bounded by $M = \mbox{max}(x_i)$, using duality, use surrogate objective for $\| w*a\|_1$ as
%   \[
%  \begin{array}{ll}
%  \underset{w}{\mbox{minimize}}   &  \frac{1}{M} E \|w * y\|_\infty 
%  \\
% \mbox{subject to} 
% & \|w*y\|_2 = 1.
% \end{array}
%   \]
%   In \cite{vembu1994convex}, they use projected SGD on $E \|w * y\|_8 $ to approximate $E \|w * y\|_\infty$ .
  
%   \item Later, use linear programming to solve $\infty$ norm problem directly \cite{ding2000fast}: 
%     \[
%  \begin{array}{ll}
%  \underset{w}{\mbox{minimize}}   &  E \|w * y\|_\infty
%  \\
% \mbox{subject to} 
% & w_0 = 1.
% \end{array}
%   \]
% \end{itemize}
There are a series of impactful digital communication work on blind deconvolution when the digital signal is discrete, which is called Blind Equalization. Examples of digital signal are PAM signaling, which is $\pm 1$ binary signal, and QAM signaling, where signal are equaly spaced points on unit sphere in complex space, as $|x|=1, x\in \complex$ \cite{kennedy1992blind,ding2000fast}.  In the work \cite{vembu1994convex}, they propose an ideal convex cost function for blind equalization:
  find $w$ so that $w*a = e_0 = (\ldots,0,1,0, \ldots)$ as minimizer of the ideal convex problem (
 Not computable without knowing $a$!)
  \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   & \| w*a\|_1 
 \\
\mbox{subject to} 
& (w*a)_0 = 1.
\end{array}
  \]  
   Using the condition that $x$ are IID and bounded by $M = \mbox{max}(x_i)$, using duality, they use surrogate objective for $\| w*a\|_1$ as
   \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  \frac{1}{M} E \|w * y\|_\infty 
 \\
\mbox{subject to} 
& \|w*y\|_2 = 1.
\end{array}
  \]
   In \cite{vembu1994convex}, they use projected SGD on $E \|w * y\|_8 $ to approximate $E \|w * y\|_\infty$.
   Later, use linear programming to solve $\infty$ norm problem directly \cite{ding2000fast}: 
    \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  E \|w * y\|_\infty
 \\
\mbox{subject to} 
& w_0 = 1.
\end{array}
  \]
  


\paragraph{Prior work: synthesis approach, sparsity}
\BIT
% \item
% Sparse signal has a long history in seismology and communication,
% see \cite{kijko1994seismological}, \cite{vembu1994convex}, \cite{osman1996seismic}, \cite{wang2010seismic}, \cite{romberg2009compressive},\cite{mendelson2016improved} etc.
\item
  Convolutional dictionary learning formulation \cite{bristow2013fast, heide2015fast}, etc.
  \item
  Synthesis blind deconvolution with $2$ norm ball constraint  \cite{zhang2017global,zhang2018structured, kuo2019geometry}, etc.
  \item
  Short $a$ and sparse $x$: 
  \[
 \begin{array}{ll}
 \mbox{minimize}   & \|y-a*x\|_2^2+\lambda \|x\|_1 \\
\mbox{subject to}  & \|a\|_2 = 1.
\end{array}
  \]  
%   \item Only empirical result so far.
%   \item Landscape could be complex.
\EIT

\paragraph{Prior work: synthesis approach, subspace assumption}
\[
 \begin{array}{ll}
 y &= a^0 * x^0\\
 \hat y  &= \hat a^0 \circ \hat x^0
\end{array}
  \]
   \begin{itemize}
  \item  $\hat a^0= D_a c_a$.
  \item $\hat x^0 = D_X c_x$.
  \item $D_X$ is often a complex Gaussian matrix.  
\end{itemize}
% \begin{figure}
%  \includegraphics[width=5cm,keepaspectratio]{figures/subspace.png}
%  \includegraphics[width=5cm,keepaspectratio]{figures/shift2.png}
% \end{figure}
No translation symmetry in this assumption!


Lifting:
 \[
 \begin{array}{ll}
 \hat y &= (D_a c_a) \circ (D_X c_x)\\
 &= \mathcal{D}(c_a c_x^T)
\end{array}
  \]
 $\mathcal{D}$ is a linear operator defined as 
 \[
 \begin{array}{ll}
\mathcal{D}(c_a c_x^T)_i = \mbox{trace}((D_{a,i}D_{X,i}^T)(c_a c_x^T))
\end{array}
  \]
  Rank one matrix $Z=c_a c_x^T$.
   \[
      \hat y =  \mathcal{D}(Z)
  \]
  \begin{itemize}  
  \item Convex optimization  \cite{ahmed2014blind},\cite{ling2015self}, \cite{chi2016guaranteed},\cite{romberg2013multichannel},\cite{lee2017blind} etc.
  \item Non-convex optimization  \cite{li2016rapid}.
\end{itemize}

\paragraph{Projection pursuit  with linear constraint}
We point out that the population problem formulation for sparse blind deconvolution is also the population problem formulation for sparse projection pursuit, which might also be called convex sparse ICA, or convex sparse dictionary learning.
\BEQ
 \begin{array}{ll}
  \underset{\psi \in V}{ \mbox{minimize} }  &  \expect |\psi^T X|\\
 \mbox{subject to}  
&  u^T \psi =1.
\end{array}
\tag{$P_{1,v}$}
\EEQ


In sparse projection pursuit with linear constraint, we observe a matrix $Y_M\in \reals^{n\times M }$, and we know that there exists a ground-truth filter $w^0$, such that $w^{0,T} Y_M = X_M$, $X_M$ satisfy Bernoulli$(p)$-Gaussian model.  

We consider the "projection pursuit" problem.
 \begin{eqnarray*}
    (\mbox{Projection pursuit}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&  v^T w = 1.
\end{eqnarray*}
Here $w$ is in a $k$ dimensional subspace of the double infinite sequence. 


\paragraph{Projection pursuit with sphere constraint}
We comment that the results we derive in the following sections are also applicable to the projection pursuit (orthogonal dictionary learning) problem \cite{bai2018subgradient, sun2016complete, sun2015complete}.
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 = 1.
\end{eqnarray*}
or
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 \geq 1.
\end{eqnarray*}
\begin{lemma}
The population problem is:
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect |\psi^T X|  \\
\mbox{subject to}  
&\Expect |\psi^T X|^2 \geq \Expect (X_0)^2
\end{array}
  \]
is equivalent to the following convex-concave problem
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
\mbox{subject to}  
&\|\psi\|_2^2 \geq 1
\end{array}
  \]
We claim that  it has the same minimizer as the \textbf{ projection pursuit (orthogonal dictionary learning) problem with sphere constraint}.
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect_I \|\psi_I\|_2  \\
\mbox{subject to}  
&\|\psi\|_2 = 1
\end{array}
  \]
  which is also equivalent to
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect_I \|\psi_I\|_2/\|\psi\|_2 
\end{array}
  \]
  And  also equivalent to
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect |\psi^T X|/\sqrt{\Expect |\psi^T X|^2} 
\end{array}
  \]
\end{lemma}


Inspired by this formulation, we propose a non-convex (convex objective concave constraint) problem for blind deconvultion:
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_2 \geq 1.
\end{eqnarray*}

Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_\infty \geq 1.
\end{eqnarray*}



\paragraph{Dirac re-parametrization and connection to residual CNN}
When $v = e_0$, we are imposing a constraint that the largest entry of $w$ is $w_0 =1$.  
We can re-parametrize our filter, as $w = \delta_0 + f$, $f_0 = 0$. Then our problem became 
 \begin{eqnarray*}
    \min_{f, f_0 = 0} &    
    \frac{1}{2T+1}\|(e_0 +f)*Y\|_{1,[-T,T]}.
\end{eqnarray*}
Here $f = (f_L, 0, f_R)$, $f_R$ and $f_L$ are in $k$ dimensional subspace of the double infinite sequence with positive and negative support.

Allowing Noise:
\[
 \begin{array}{ll}
 \mbox{minimize}   & \|x\|_ 1+\lambda/2\|Y+f*Y-x\|_2^2\\
\mbox{subject to}  
& f_0 =0,
\end{array}
  \]
  with variables $f\in \reals^k$, $x\in \reals^n$. 
  
 \texbf{General multi-channel approximate version}
\[
 \begin{array}{ll}
 \mbox{minimize}   & \sum_i(\|x^i\|_ 1+\lambda^i/2\|Y+f^i*Y-x^i\|_2^2)\\
\mbox{subject to}  
& f^i_0 =0,
\end{array}
  \]
  with variables $f^i\in \reals^k$, $x^i\in \reals^n$. 
  
\paragraph{Link to CNN}
Partial minimization:(similar to one-layer Residual CNN)
\[
 \begin{array}{ll}
 x^i = S_{1/\lambda^i}(Y+f^i*Y)
\end{array}
  \]
  with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $. 


\texbf{Method $1$: plug-in}
\[
 \begin{array}{ll}
 \mbox{minimize}   & \sum_i(\|S_{1/\lambda^i}(Y+f^i*Y)\|_ 1+\\
 &\lambda^i/2\|Y+f^i*Y-S_{1/\lambda^i}(Y+f^i*Y)\|_2^2)\\
\mbox{subject to}  
& f^i_0 =0,
\end{array}
  \]
  with variables $f^i\in \reals^k$, $x^i\in \reals^n$.   
  
%   Let $C_Y$ be the circulant matrix with first column $Y$, let $\hat Y = F_nY$, where $F_n$ is discrete Fourier transform, $U = \frac{1}{\sqrt{n}}F_n$ as a unitary matrix,
% \[
% C_Y = U^*\mbox{diag}(\hat Y)U.
% \]
% Block coordinate update (alternating): initialize: $ f^i(0) = 0;$.
% \[
%  \begin{array}{ll}
%  x^i(t) &= S_{1/\lambda^i}(Y+f^i(t-1)*Y);\\
%  f^i(t) &= (C_Y^T C_Y)^{-1}[C^T_Y(x^i(t)-Y)+\mu(t) \delta_0^T]\\
%  &= U^*\mbox{diag}(1/(\hat Y))U x^i(t)-\delta_0 
%  + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T\\
%  &= Y^{(-1)}*x^i(t) -\delta_0 + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T
% \end{array}
%   \]
%   with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $, $\mu(t)$ is the dual variable.

==> old_sec/sec_old/Stability.tex <==
\section{Stability for approximation of infinite length inverse filter}

 
 
 

\paragraph{Reduction}
 \begin{lemma} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then the previous convex optimization problem can be reduced to 
  \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  & B(p, \phi) \|\phi \|_2\\
 \mbox{subject to}  
&  \phi = a*w -e_0, \quad w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
  where
  \[
B(p, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
\]
 \end{lemma} 
  
  
\begin{proof}
Following the previous phase transition analysis, 
let the directional finite difference of the objective at $e_0$ be $D(w) = |(w*Y)_0| - |X_0|$, $I$ be the support of $\tilde{X}$, let $\phi = w*a-e_0$,  then we have 
\[
 \begin{array}{ll}
\Expect D(w) &= \sqrt{\frac{2}{\pi}}\Expect_I [\|(w*a)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\|{\phi}\|_2 B(p, \phi)  \\
\end{array}
  \]
The last inequality comes from the bi-Lipschitz property of $\Expect_I \|(e_0+\phi)_I\|_2$ around $e_0$. 

% Now, we use the \textbf{lower semicontinuous extension}!

% First, $\phi \mapsto \Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]$
% is Lipschitz for $\ell_2$ strong convergence.

% Second $\phi \mapsto \| \phi \|_2$ is Lipschitz for $\ell_2$ convergence.

% Hence we need to use a version of $B(p,\| \phi\|_0)$ that is continuous!
% (Qingyun: add a theorem to quote here!)

% Consider the USC (upper semicontinuous) envelope of $B(p,\| \phi\|_0)$:
% \[
% B^+ := \limsup_{\phi_k -> \phi}   B(p,\| \phi\|_0)
% \]
% where the $\limsup$ is over all sequences that converge to $\phi$.

% If we are dealing with $\phi\in \reals^n$,
% then
% \[
% B^+ =  B(p,n)
% \]

% For any contemplated optimizer $\phi^*$ of $\Expect D$ we can find a
% minor perturbation $\phi^{\epsilon}$ with full support, and with at worst a small
% increase in objective over the limit value!

Now using the optimality of $w^\star$ in $V_{rs, rt}$, for all $w in V_{s,t}, w\neq w^\star$,
we have
 \[
 \begin{array}{ll}
\Expect D(w^\star) \leq \Expect D(w)
\end{array}
  \]
We could directly reduce the problem to 
  \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2 
\end{array}
  \]
\end{proof}   
 
% \textbf{Qingyun: this argumemnt has a gap to the deterministic quantity because $B(p, \phi)$ is dependent on configuration of $\phi$. }

% \textbf{TODO}:

\begin{coro}
If there exists a $\phi$ with $\|{\phi}\|_2<1$ such that \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
 for  $\epsilon> 0$ when $p\leq p^\star(\epsilon)$, then 
  \[
  B(p, \phi) \geq \epsilon.
  \]
  for all $\phi$, 
  then
    \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 \leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  is also bounded.
\end{coro}
\begin{proof}
From
 \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
  We have
  \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 
&\leq \frac{B(p, \phi)}{B(p, \phi^\star)}
\|{\phi}\|_2 \\
&\leq \frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
p\Big(\phi_0  +
  \frac{\|{\phi}\|_2}{2} \phi_0^2 
 +
 p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}\|{\phi}\|_2 \\
&\leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  \end{proof}
% Now we want to show that there exists some constant $C$, depending on the worst case directional configuration of $\phi$ and $\phi^\star$,
% \[
% C \geq  \sup_{\phi, \phi^\star}\frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
% p\Big(\phi_0  +
%   \frac{\|{\phi}\|_2}{2} \phi_0^2 
%  +
%  p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
% p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}
% \]
% so that
%   \[
%  \begin{array}{ll}
% \|{\phi^\star}\|_2 \leq C \|{\phi}\|_2
% \end{array}
%   \]
  In the following we constructed a filter to give an upper bound on $\|{\phi}\|_2$. 


\paragraph{Setting for finite length approximation}
Now we consider a setting where there is a kernel whose corresponding inverse kernel has infinite support, and we give a finite-length approximation. 

Within the space $V_{-\infty,\infty}$ of bilaterally infinite real-valued sequences $(h(i))_{i \in \integers}$, consider the affine subspace $V_{N_{-}, N_{+}} = \{ (...,0,0,h_{-N_{-}},\ldots, h_{-1}, 1, h_1, h_2, \ldots, h_{N_{+}},0,0,...)\}$, an $N_{-}+N_{+}$-dimensional subspace of bilateral sequences with support at most $N_{-}+N_{+}+1$.
The coordinate that is fixed to one is 
located at index $i=0$.
Each coordinate is zero outside of a window
of size $N_{-}$ on the left of zero 
and  size $N_{+}$ on the right of zero.
The special sequence $e_0 = (\dots,0,0,1,0,0,\dots)$,
vanishing everywhere except the origin,
belongs to $V_{-\infty,\infty}$ and to every
$V_{N_-,N_+}$.

Let $a \in V_{N_-,N_+}$.
Then $a =  (...,0,0,a_{-N_{-}},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_{N_{+}},0,0,...)$.
We also write $a = e_0 + a_{(0)}$,
where $a_{(0)} \equiv (1-e_0) \cdot a$ 
denotes the `part of $a$ supported away from location
$i=0$'. We also write $a = e_0 + a_L + a_R$,
where $a_L = (a_L(i))_{i \in \integers} 
= (a(i) 1_{\{i < 0\}})_{i \in \integers}$ 
denotes the `part of $a$ supported to
the left of $i=0$' and 
where $a_R = (a_R(i))_{i \in \integers} 
= (a(i) 1_{\{i > 0\}})_{i \in \integers}$
denotes the `part of $a$
supported to the right of $i=0$'.
Finally, we say that $a \in V_{N_{-}, N_{+}}$ 
is a length $ L= N_{-}+N_{+}+1$ filter.

An interesting, if not implementable, objective
function for the blind deconvolution problem
is to minimize
$\Expect [|(w*a*X)_0| - |X_0|] $,
particularly when combined with constraints 
somehow ensuring ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
Defining $\phi \equiv w*a-e_0$, 
\[
 \begin{array}{lll}
\Expect [|(w*a*X)_0| - |X_0|] &=&\Expect [|((e_0 +\phi)*X)_0| - |X_0|].
\end{array}
  \]
  Below we establish the relation
  \[
   \begin{array}{lll}
\Expect [|((e_0 +\phi)*X)_0| - |X_0|] 
&\approx&  C \|{\phi}\|_2 ; \\
\end{array}
\]
This suggests that we should  seek to
minimize $\Expect |(w*Y)_0| $,
while constraining $w$ in some way that
ensures ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
This  the deterministic objective as 
$$
d_a(w, a^{-1}) :=\|{\phi}\|_2 = \|a*w -e_0 \|_2 =  \|a*(w -a^{-1}) \|_2.
$$

Therefore, we want to construct a finite length approximation of $a^{-1}$ to bound $d_a(w^\star, a^{-1}) = \|a*w -e_0 \|_2$ for the optimal point $w^\star$.








We construct the finite length approximation filter explicitly by truncation of Z-transform.

Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.






 
\subsection{A different approach to prove stability for factorized filter}
\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

If we choose this approximation $w^{r,1},$ then
\[
\|a*w^{r,1}-e_0\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 = s^{2(r+1)} 
\]

In the following, we show that this is indeed the best 

For $\gamma\in (0,1]$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem 
% \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

% If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
% \[
% \|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
% =  (1-\gamma_2)^2 + (\gamma_2 s)^2 
% = \frac{s^2}{1+s^2}
% \]
% And in this case,
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty
% &= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
% &=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
%  \end{array} \]
 
%  Therefore, 
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
%  \end{array} \]


\paragraph{Finite length approximation constructing using Z-transform truncation on factorization form }
Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i},
\end{array}
  \]
We can factorize the Z-transform as product of factors with roots $s_{-j}$ for $j = 1, \ldots N_{-}$ and  $i = 1, \ldots N_{+}.$
\[
 \begin{array}{ll}
A(z) =  c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1}),
\end{array}
  \]
  Where $c_0$ is a constant to make sure that the coefficient $a_0=1$.
  
 We assume that $|s_k|<1,$ for any $k = -N_{-}, \ldots , N_+.$  
  
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.
\[
 \begin{array}{ll}
1/A(z) &=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1})^{-1}\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{\infty} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{\infty} s^{\ell_i}_{i} z^{\ell_i} )
\end{array}
  \]

From previous single root study, we get a hint to study a single truncation of length $ 1 + \sum_{j=1}^{N_{-}} r_{-j}  +  \sum_{j=1}^{N_{+}}  r_i$,  we construct
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r_{-j}} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r_{-j}} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r_i+1}) (1- s_{i} z^{-1})^{-1}
\end{array}
  \]
Let the corresponding filter being $w$.
  
  
Now let $\psi =  a*w$ with Z-transform $\Psi(z)$, $\phi = a*w-e_0$ with Z-transform $\Phi(z)$,we have
\[
 \begin{array}{ll}
\Psi(z): = A(z)W(z) 
&=   \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) 
\end{array}
  \]
  therefore,
\[
 \begin{array}{ll}
\Phi(z): = A(z)W(z) -1 
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) -1
\end{array}
  \]
\paragraph{Upper Bound on  $\|\phi\|_2^2$ for constructed finite length approximation}
In the following,  we want to give upper bound for
  \[
\|a*w -e_0\|_2^2 =\|\phi\|_2^2 
 \]  
  
Redefine the index $\tau_{-j} := r_{-j}+1; \tau_{i} = r_i+1.$
Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible index.
And we define polar represenation of complex roots:
for any $k \in \cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$
\[
s_{k} := |s_{k}| e^{i \varphi_k } = e^{\rho_k + i \varphi_k }
\]
where 
\[
 \begin{array}{ll}
\varphi_k := \operatorname{Im}(\log( s_{k} )) = -i \log(\frac{s_{k}}{|s_{k}|}) 
\end{array}
\]
and since $|s_{k}|<1$ we have 
\[
\rho_k = \operatorname{Re}(\log( s_{k} ))<0
\]

Now we consider all $z = e^{2 \pi i t}$ on the unit circle for $t\in [\frac{-1}{2},\frac{1}{2}]$,
then for any $k \in \cI$
\[
 \begin{array}{ll}
- (s_{k} z^{-\mbox{sign}(k)})^{\tau_{k}} 
&= - |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\\
&=   \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) 
\end{array}
  \]
 Now we simplify the notation by defining 
 \[
 \upsilon_k(t) :=\tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi
 \]
then
 \[
 \begin{array}{ll}
\Phi(z)
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{\tau_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{\tau_{i}}) -1\\
&=  \prod_{k \in \cI} \Big(1- |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\Big)  -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) \bigg)     -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1
\end{array}
  \]
  
\begin{lemma}
 For any $z = \exp{(2 \pi i t )}$ on the unit circle,
 \[
 \begin{array}{ll}
\Phi\big(\exp{(2 \pi i t )}\big)
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1\\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big)
+ i \cdot \big( \upsilon_{k_1}(t) + \ldots+  \upsilon_{k_n}(t)  \big) \Big)  
\end{array}
  \]
 \end{lemma}
 
 \begin{lemma}
Additionally, for any $t \in [\frac{-1}{2},\frac{1}{2}]$,
\[
 \begin{array}{ll}
 |\Phi\big(\exp{(2 \pi i t )}\big)|^2  
= 
\sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
is independent of $t$, since the oscillation integral over the imaginary part is 
  \[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2}
\exp  \bigg( i \cdot \Big(  \big(\upsilon_{k_1}(t) - \upsilon_{k_1}(t) \big) + \ldots+  \big(\upsilon_{k_n}(t) -\upsilon_{k_n}(-t)\big)  \Big) \bigg)  dt
= 1
\end{array}
  \]
Therefore, using Fourier isometry,
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 &= \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi\big(\exp{(2 \pi i t )}\big)|^2 dt \\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
  
 \end{lemma}

\begin{theorem}
\label{thm: Root_2_norm}
Since $|s_{k}|<1$, i.e. $\rho_{k}<0$ for all $k\in \cI$.
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big) 
\end{array}
  \]
  Let $\gamma^m := \min_{i}\big(\tau_{i} |\rho_{i}| \big) =  \min\{\tau_{-N_-}|\rho_{-N_-}|, \ldots, \tau_{-1}|\rho_{-1}|, \tau_{1}|\rho_{1}|, \ldots, \tau_{N_+}|\rho_{N_+}|\}.$
When $\gamma^m \rightarrow \infty$, we have a finite sum of exponential rate  converging terms: the convergence rate is determined by the exponential term as a function of $\gamma^m$.
   \[
 \begin{array}{ll}
 \|\phi\|_2^2 
=    O(\exp \Big( -2 \min_{i}\big(\tau_{i} |\rho_{i}| \big) \Big))
= O(\exp \Big( -2 \gamma^m  \big) \Big))
\rightarrow 0
\end{array}
  \]

 \end{theorem}

 
% \begin{proof}
% Using the expansion, for $Z = \exp{(2 \pi i t )},$ then 
% \[
%  \left|(-1)^n( \prod_{j=1}^n \frac{s_{\ell_j}}{|s_{\ell_j}|}  (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })\right| = 1
% \]
% therefore, for any $t\in [\frac{-1}{2},\frac{1}{2} ]$ 
%  \[
%  \begin{array}{ll}
% \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|
% % &= |\sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % [(-1)^n( \sign[ \prod_{j=1}^n s_{\ell_j}] (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })]|\\
% &\leq \sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % \\
% % &= \prod_{\ell \in \cI} (1+ |s_{\ell}|^{r_\ell+1})-1 
% \end{array}
%   \]
% Therefore, from 
% \[
%  \begin{array}{ll}
% & \|\phi\|_2^2\\
%  =& \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt \\
%   \leq & \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|^2
% \end{array} \]
% we conclude the proof.




%  \[
%  \begin{array}{ll}
% S_{-j}(t) &:= \log(s_{-j} \exp{(2 \pi i t )}) \\
% &= \log(|s_{-j}|)+ i (\pi 1_{s_{-j}<0}+ 2 \pi  t)\\
% S_{i}(t) &:= \log(s_{i} \exp{(-2 \pi i t )})] \\
% &= \log(|s_{i}|)+ i ( \pi 1_{s_{i}<0}+ 2 \pi  t)
% \end{array} \]
% % \[
% %  \begin{array}{ll}
% % R_{+}^{j, r_{-j}}(t) &:= (s_{-j} \exp{(2 \pi i t )})^{r_{-j}+1} \\
% % &= \exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\}\\
% % R_{-}^{i, r_i}(t) &:= (s_{i} \exp{(-2 \pi i t )})^{r_i+1} \\
% % &= \exp\left\{(r_{-j}+1)S_{i}(t) \right\}
% % \end{array} \]
% % and let
% % \[
% %  \begin{array}{ll}
% % Q_{+}^{j, r_{-j}}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\} )\\
% % Q_{-}^{i, r_i}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{i}(t)  \right\} )
% % \end{array} \]

% \[
%  \begin{array}{ll}
%   \Psi(\exp{(2 \pi i t )})
% % &= \gamma \prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t))\\
% % &= \gamma \exp\{ \sum_{j=1}^{N_{-}} Q_{+}^{j, r_{-j}}(t) + \sum_{i=1}^{N_{+}} Q_{-}^{i, r_i}(t)  \}  \\
% &=  \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &=  \int_{\frac{-1}{2}}^\frac{1}{2}  |\Psi(\exp{(2 \pi i t )}) -1|^{2} dt\\
% &= \int_{\frac{-1}{2}}^\frac{1}{2}  | \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
% \end{array} \]
% Consider the case when all the $r_\ell$ are the same as $r,$ and $r\rightarrow \infty$.
% % From the fact that for $x\leq 0,$
% % \[\log( 1-\exp(-x)) = -x + \log(\exp(x) -1)\]
% % and the Laplace's method, 
% we know that to compute
% $\int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt,$
% We only need to compute the maximum value of $\sum_{ \ell \in \cI } S_{\ell}(t)$.
% The maximum value is gonna be $\sum_{ \ell \in \cI } \log(|s_{\ell}|)$, and it is achieved at either $t_0 = 0$, or $t_0 = 1,$ depending on the sum of all the $\sum_{ \ell \in \cI } 1_{s_{\ell}<0}$ is odd or even.

% Therefore, 
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2}  |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
%   \leq&    |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)\log(|s_{\ell}|  \right\} )  \right\} -1|^{2} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\ 
% \end{array} \]
% \end{proof}

==> old_sec/sec_old/Stability_old.tex <==

\paragraph{Finite length approximation by Z-transform truncation }

Let $\gamma>0$, then we define 
\[
\bar a^{\gamma} :=e_0-\gamma a
\]
with Z-transform 
\[
\bar A^{\gamma}(z) :=1-\gamma A(z)
\]
then
\[
 \begin{array}{ll}
1/A(z) &=  \gamma(1-\bar A^{\gamma}(z))^{-1}\\
&= \gamma[ 
\sum_{i=0}^{\infty} (\bar A^{\gamma})^i]
\end{array}
  \]
We can construct an approximation 
$w^{r,\gamma} \in V_{rs, rt} $ of length $r(1+s+t)$ 
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
with Z-transform
\[
 \begin{array}{ll}
W^{r,\gamma}(z) 
&= \gamma[\sum_{i=0}^{r} (\bar A^{\gamma}(z))^i] \\
&= \frac{1-(\bar A^{\gamma}(z))^{r+1}}{A(z)} 
\end{array}
\]
then
\[
a*(a^{-1}-w^{r,\gamma}) 
= *_{r+1} (\bar a^{\gamma})
\]
\begin{lemma}
\[
\|a*(a^{-1}-w^{r,\gamma})\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 
= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
 \]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt\\
&= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
\end{array} \]
\end{proof}


First, since:
%   \[
%  \begin{array}{ll}
%  \|\hat{\bar a}^{\gamma}\|_{\infty} \geq \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% Notice that 

\[
 \begin{array}{ll}
 \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2} = (|\hat{\bar a}^{\gamma}|^2(t_0))^{r+1} \geq  \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt
\end{array}
\]
We have a natural upper bound as
\[
 \begin{array}{ll}
\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}\leq \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2}
\end{array} \]
In the following we give a more accurate calculation of $\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}$ using Laplace method.
% Then using Parseval’s identity, 
%   \[
%  \begin{array}{ll}
% \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% (Here we remark that the Fourier transform and inverse Fourier transform are define as follows so that the there is no constant for Parseval’s identity)
% \[
% \mathcal{F}a(\omega) = \hat{a}(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]
% \[
% (\mathcal{F}^{-1} \hat{a})(n) =  \int_{\frac{-1}{2}}^\frac{1}{2} \hat{a}(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
% \]

%  Since $\|\hat{\bar a}^{\gamma}\|^2_{\infty} \geq
%  \|\hat{\bar a}^{\gamma}\|^2_{\infty} \leq \|\hat{\bar a}^{\gamma_2}\|^2_{2}  = \|\bar a^{\gamma} \|_{2} =  \sin{\theta}$.



\paragraph{Laplace's method}
 \begin{theorem}[Laplace's method]
 \label{Laplace}
  For $\bar a^{\gamma} :=e_0-\gamma a$, $a$ has a length $L$ window of non-zero entries.
 \BIT
 \item
 let $F(t) = |\bar a^{\gamma}(t)|^2$, and let $f(t) := \log F(t) = \log| \hat{\bar a}^{\gamma}|^2$ and $t_0 = \arg\max_{t\in [\frac{-1}{2},\frac{1}{2}]} F(t)$ achieves the global maximum, and let the maximum value be $F_{\max} :=F(t_0) = |\hat{\bar a}^{\gamma}(t_0)|^2$. 
\item
We define the second moment 
%   $M_2\leq \sum_{|k|\leq 2L} k^2$,
  \[M_2: = \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k)\]
  then $M_2$ is finite, upper bounded by $\frac{16}{3}(L+1)^3 \| \bar a^{\gamma}\|_2^2$ and $f$ is twice  differentiable near $t_0$.
%   with $|f''(t_0)|\leq M_2/F_{\max} $.
% \item
%  Assume
%  $F_{\max}<1$.
 \EIT
We have
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}  
  &= \int_{\frac{-1}{2}}^\frac{1}{2}  \exp((r+1)f(t)) dt  \\
  &=  [(\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0))](1+O(r^{-1})) 
  \\
  &=   [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.
\end{theorem}
\begin{proof}
From optimality $F'(t_0) =0,$ and 
\[
 \begin{array}{ll}
|f''(t_0)| &= |\partial^2 \log F(t_0)| \\
&= \frac{ |F''(t_0)|}{|F(t_0)|} 
\end{array}
\]

For $f$ to be twice  differentiable near $t_0$ with $|f''(t_0)|$, we only need to upper bound 
\[
|F''(t_0)|=|[\hat{\bar a}^{\gamma}]''(t_0)|^2 \leq \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k).
\]
As
\[
\frac{ M_2}{\|\bar a^{\gamma}\|_2^2}\leq \sum_{|k|\leq 2L} k^2.
\]
and  $a$ is of length $L = 1+s+t$, we know that $\bar a^{\gamma}  *  \tilde{\bar a}^{\gamma} $ is of length at most $2L$, then 
\[
\sum_{|k|\leq 2L} k^2 = 1+\frac{2L(2L+1)(4L+1)}{3}\leq \frac{16}{3}(L+1)^3.
\]

Then $f$ to be twice  differentiable near $t_0$ and
\[
 \begin{array}{ll}
|f''(t_0)| 
&= \frac{ |F''(t_0)|}{|F(t_0)|} \\
&\leq  \frac{ M_2}{F_{\max}}
\end{array}
\]

Now we go back to the main quantity,
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} &= \int_{\frac{-1}{2}}^\frac{1}{2} |\hat{\bar a}^{\gamma}(t)|^{2r+2} dt  \\
  &= \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  
\end{array}
\]
By Laplace's asymptotic method,
 \[
  \begin{array}{ll}
  & \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  \\
  =&\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.

Combining all the previous bounds, we have
\[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} 
  &= \sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))  \\
 &= [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
\end{proof}

\paragraph{Stability theorem}
Combing the calculation of expectation, the construction of finite length inverse, the Laplace method calculation, we arrive at our final result.
\begin{theorem} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then provided $p<p^\star - \delta$, we have
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq  [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
 \]
\end{theorem}
\begin{proof}
From previous result, 
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq \|a*(w^{r,c} -a^{-1}) \|_2^2
 \]
 and previous the previous construction of $w^{r,c}$, we know that 
 \[
 \|a*(w^{r,c} -a^{-1}) \|_2^2 \leq [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1})).
 \]
Hence we prove the geometric convergence for any $F_{\max} <1$.
\end{proof}


\paragraph{Sufficient condition for $F_{\max} <1$}
\begin{lemma}
Let
 \[
 \gamma_2 = \arg\min_{\gamma>0} \|\bar a^{\gamma} \|_{2}^2
 \]
 Then $\gamma_2 = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
And
  \[
 \|\bar a^{\gamma_2} \|_{2}^2 = 1- \gamma_2^2 = \sin^2{\theta}
 \]
 
\end{lemma}
\begin{proof}
Using the fact that $a_0 =1$, $\|a\|_2 = \frac{1}{\cos{\theta}}$,
\[
 \begin{array}{ll}
\|\bar a^{\gamma} \|_{2}^2 
&= 1+ \gamma^2 \|a\|_2^2 -2\gamma a_0\\
&= 1+ \gamma^2 \frac{1}{\cos^2{\theta}} -2\gamma \\
&= \frac{1}{\cos^2{\theta}} (\gamma - \cos^2{\theta})^2 + (1-\cos^2{\theta})
\end{array} \]
Hence $\|\bar a^{\gamma} \|_{2}^2 $ is mimimized at $\gamma_2 = \cos^2{\theta}$ with value $1-\cos^2{\theta}=\sin^2{\theta}$.
\end{proof}

Remark:
Is there any way to directly optimize $\|\hat{\bar a}^{\gamma}\|_{\infty}$? Would there be an improvement over optimize 2 norm?

\begin{lemma}
Let $S_a := \sum_{j\neq 0} |a_j|$, 
\[
 \gamma_\infty = \arg\min_{\gamma} \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 \]
 if $S_a<1,$ then  
 \[
 \gamma_\infty = 1
 \]
 and 
  \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]

%  Then $c = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
% And
%   \[
%  \|\bar a^{c} \|_{2}^2 = 1- c^2 = \sin^2{\theta}
%  \]
 
\end{lemma}
\begin{proof}
 Since
 \[
 \begin{array}{ll}
|\hat{\bar a}^{\gamma}(t)|^2
 &=  |\bar A^{\gamma}(e^{2\pi i  t})|^2  \\
 &= |1-\gamma A(e^{2\pi i  t})|^2 \\
 &= (1-\gamma A(e^{2\pi i  t}))(1-\gamma A(e^{-2\pi i  t})) \\
 &= 1 + \gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))
 \end{array} \]

 \[
 \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 = 1 + \max_{t\in [\frac{-1}{2},\frac{1}{2}]} [\gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))]
 \]
Since the coefficient $a_i$ are all really, we check different $t.$
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(0)|^2
  &= |1-\gamma (\sum_j a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} a_j)|^2
  \end{array}
 \]
 
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(\frac{1}{2})|^2
  &= |1-\gamma (\sum_i (-1)^{|j|} a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (-1)^{|j|}  a_j)|^2
  \end{array}
 \]
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2
  \end{array}
 \]
then
\[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2\\
  &\leq |(1-\gamma) + \gamma S_a|^2
  \end{array}
 \]
 if $S_a<1,$ then
 \[
  \begin{array}{ll}
  \min_\gamma |(1-\gamma) + \gamma S_a|^2 =  |S_a|^2<1.
  \end{array}
 \]
 Therefore if $S_a<1$,  $\gamma_\infty =1,$ and 
 \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]
\end{proof}

Remark: from this paragraph, we see upper and lower bound for $F_{\max}$, by choosing $\gamma =1,$ we have
\[
F_{\max}   \leq |S_a|^2
\]
also, we see that
\[
F_{\max}   \geq  \|\bar a^{1} \|_{2}^2 
=  \frac{1}{\cos^2{\theta}} -1 = \tan^2{\theta}
\]
So a natural consequence is that 
\[
\tan^2{\theta}   \leq |S_a|^2
\]
If $S_a<1$, we need $\tan^2{\theta}<1$, therefore $\theta<\frac{\pi}{4}$.

\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

For $\gamma\in (0,1)$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
\[
\|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
=  (1-\gamma_2)^2 + (\gamma_2 s)^2 
= \frac{s^2}{1+s^2}
\]
And in this case,
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty
&= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
&=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
 \end{array} \]
 
 Therefore, 
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
 \end{array} \]

==> old_sec/sec_old/Subgradient.tex <==
\section{Subgradient KKT condition and phase transition}
\paragraph{Exact calculation of subgradient for phase transition condition}

Here I try to give a clean proof of phase transition directly using sub-gradient and directional derivative.

\begin{lemma}
Let $J \subset [n]$ be the support of $X$, let $\psi_J : = \psi\cdot 1_J$ denote the entrywise product of vector $\psi$ with the indicator vector of subset $J$.  Let $B_J$ denote
the central section of the euclidean  ball $B(\reals^n)$,
where the slice is produced the linear space $\mbox{span} \{e_i : i\in J \}$.
Alternatively, we may write
$B_J: = \{ v_J: \| v_J\|_2 \leq 1\}$.  The set-valued subgradient
operator applied to $\|\psi_J\|$
evaluates as follows:
 \[
 \begin{array}{ll}
\partial_{\psi}    \| \psi_J \|
&=  N(\psi_J).
\end{array}
  \]
Here $N$ maps $\reals^n$ into  subsets of $\reals^n$,
and is given by:
\[
N(\psi_J):= 
\begin{cases}
    \psi_J/\|\psi_J\|_2, &  \psi_J\neq 0 \\
    B_J, &  \psi_J = 0
  \end{cases},
\]  
\end{lemma}

\begin{definition}
Consider a probability space containing just the possible  
outcomes  $J \subset [n]$.
Let $S_J$, $J \subset [n]$,  denote a closed compact subset of $\reals^n$.
Let $I$ be a random subset of
$[n]$ drawn at random from this probability space with probability $\pi_J = P\{ I = J \}$
of elementary event $J$.
Consider the set-valued random variable $S \equiv S_J$. We define its expectation as
\[
 {\Expect} S  := \sum_J \pi_J \cdot S_J.
\]
On the right side, we mean the closure of the 
compact set produced by all sums of the form
\[
 \sum_J \pi_J \cdot s_J
\]
where $s_J \in S_J$.
\end{definition}

\begin{lemma}
For any $\psi \in \reals^n$, and $X = (X_i)_{i=1}^n$ with $X_i \sim_{iid} BG(p,0,1)$.
Let now $I \subset [n]$ be the random support of $X$.
Let $\partial_\psi $ denote the set-valued subgradient
operator.
  \[
 \begin{array}{ll}
\partial_\psi [E{|\sum_{i} \psi_i X_i| }  ]
%&=  {\Expect}\,{\mbox{\rm sign}(\psi^T X) X }  \\
&= \sqrt{\frac{2}{\pi}} \cdot {\Expect}_I [N(\psi_I)].
\end{array}
  \]
\end{lemma}

\paragraph{Subgradient and directional derivative at $e_0$}
Now we focus on $e_0$. Note that for any subset $J \subset [n]$, $(e_0)_J$ is either the zero
vector or else $e_0$. Hence $N((e_0)_J)$
is either $B_{J}$ or $\{e_0\}$. What drives
this dichotomy is whether $0 \in J$ or not.

\begin{lemma}  
\[
 \begin{array}{ll}
\Expect_I [N((e_0)_I) ]
&= p e_0 + \sum_{J,0\not\in J } \pi_{J} B_{J} \\
& = p e_0 + (1-p) {\cal B}_0
\end{array}
  \]
where
\[
 \begin{array}{ll}
{\cal B}_0 = \Expect_{I}[ B_{I} | 0 \not \in I ] = 
(1-p)^{-1} \cdot \sum_{J,0\not\in J } {\pi_{J}} B_{J}.
\end{array}
\]
 
\end{lemma}


\begin{proof}
\begin{eqnarray*}
\Expect_I [N((e_0)_I) ] &=& \sum_{J } \pi_{J} B_{J} \\
&=&  \sum_{J, 0 \in J}   \pi_{J} e_0 +  \sum_{J,0\not\in J }  \pi_{J} B_{J}\\
&=& p \cdot e_0 + (1-p) \cdot {\cB}_0 .
\end{eqnarray*}
 \end{proof}
To compute with $\Expect_I [N((e_0)_I) ]$,
we need:
\begin{lemma} \label{eq:ComputeExpect}
For each fixed $\beta \in \reals^n$:
\[
  \sup_{b \in {\cal B}_0} \langle \beta, b \rangle
   = \Expect_{I}[ \|\beta_I\|_2 | 0 \not \in I  ].
  \]
\end{lemma}

\begin{proof}
Note that in the definition of the set 
\[
{\cal B}_0 = \Expect_{I}[ B_{I} | 0 \not \in I ],
\]
 each term $B_J$ obeys the bound
$\sup_{g_J \in B_J} \|g_J\|_2 = 1 $.
Now, given the fixed vector $\beta \in \reals^n$, define:
\begin{eqnarray*}
    b^* &=& \Expect_{I}[ \frac{\beta_I}{\| \beta_I \|_2} | 0 \not \in I  ]\\
     &=&  \sum_{0 \not \in J} \pi_J \frac{\beta_J }{\|\beta_J\|_2}.
 \end{eqnarray*}
 Since each term in this sum has euclidean norm at most $1$, $b^* \in {\cB}_0$.
Now
\begin{eqnarray*}
\langle  \beta, b^* \rangle &=&
\langle \beta , \sum_{0 \not \in J} \pi_J \frac{\beta_J }{\|\beta_J\|_2} \rangle \\
&=& \sum_{0 \not \in J} \pi_J \langle \beta , \frac{\beta_J }{\|\beta_J\|_2} \rangle \\
&=& \sum_{0 \not \in J} \pi_J \|\beta_J\|_2 .
 \end{eqnarray*}
On the other hand, for any fixed 
vector $g = \sum \pi_J g_J $,
with each $g_J \in B_J$,
we have
\begin{eqnarray*}
\langle  \beta, g \rangle &=&  \sum_{0 \not \in J} \pi_J \langle \beta , g_J  \rangle \\
&\leq& \sum_{0 \not \in J} \pi_J  \|\beta_J \|_2 \|g_J\|_2 \\
& \leq & \sum_{0 \not \in J} \pi_J  \|\beta_J \|_2 
= \langle  \beta, b^* \rangle.
 \end{eqnarray*}
\end{proof}

Lemma (\ref{eq:ComputeExpect}) 
can be viewed as a special instance of
Theorem \textbf{A.15} from \cite{bai2018subgradient}:
\begin{lemma}[Interchangeability of set expectation and support function] 
Suppose a random compact set $S \subset \reals^n$ is integrably bounded and the underlying probability space is non-atomic, then $\E[S]$ is a convex set and for any fixed vector $\beta \in \reals^n,$
 \begin{equation} \label{eq:SetExpectEquality}
 \sup_{g\in \Expect S} \langle\beta, g\rangle =  \sup_{g\in  S} \Expect\langle\beta, g\rangle .
 \end{equation}
\end{lemma}

Define $\beta_{(0)} = \beta \cdot 1_{\{0\}^c}$ as the part of $\beta$ supported away from $0$.
Further define 
\[
V_1(\beta_{(0)}):= \frac{\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]}{\|\beta_{(0)}\|_2}.
\]
Let $N = \|\beta_{(0)}\|_0$; then 
 $V_1(\beta_{(0)})$ satisfies
\beq 
 p  \leq  V_1(\beta_{(0)}) \leq \sqrt{p} .
\eeq

\begin{lemma}


 The directional derivative at $e_0$ along $\beta$ 
 evaluates to the following:
 \BEAS
 \lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2]) 
 &=&  p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
 &=& [p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} V_1(\beta_{(0)})] \|\beta\|_2
 \EEAS
\end{lemma}
 \begin{proof}

Let $\langle b, v \rangle  \equiv b^T v$.

Applying Lemma \ref{eq:ComputeExpect}, we proceed as follows:
\[
 \begin{array}{ll}
\lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
&= \sup_{g\in \Expect_I [N((e_0)_I)]} \langle\beta, g\rangle\\
% &= \sup_{g\in  [N((e_0)_I)]} \Expect_I\langle\beta, g\rangle\\
&= p \cdot \langle\beta, e_0\rangle + (1-p) \cdot  \sup_{g\in {\cal B}_0 } \langle\beta, g\rangle\\

&= p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] \\
&= [p \cdot \cos{\angle(\beta, e_0)} + (1-p) \cdot  \sin{\angle(\beta, e_0)} V_1(\beta_{(0)})] \|\beta\|_2
\end{array}
  \]
  \end{proof}


\paragraph{Projected subgradient}
\begin{lemma} 
If $\beta$ need to satisfy a constraint $u^T \beta =0$, then we only consider directional derivative at $e_0$ along $\beta$ for those $\beta$ that $u^T \beta =0$.
Therefore, let $P_{u}^{\perp}$ be the projection onto the hyperplane as the orthogonal complement of $u$, then the following three equivalent conditions all make sure $e_0$ is the stationary point.
\BIT
\item
  \[
 \begin{array}{ll}
0\in P_{u}^{\perp} \Expect_I [N((e_0)_I) ]
\end{array}
  \]
  \item
Equivalently, there exists a subgradient $g\in  P_{u}^{\perp} \Expect_I [N((e_0)_I) ]$ such that for all $\beta$ satisfy $u^T \beta = 0$,
\[
\beta^T g \geq 0
\]
\item
Also equivalently, for all $\beta$,
\[
 \begin{array}{ll}
\sup_{g\in  [N((e_0)_I)]}\Expect_I[ \langle   P_{u}^{\perp}  \beta, g\rangle] \quad \geq 0
\end{array}
  \]
  \EIT
\end{lemma}
 
 Let $\theta = \angle({u, e_0})$, for $\beta$ need to satisfy a constraint $u^T \beta =0$,
we get
\[
 \begin{array}{ll}
\lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
% &= \sup_{g\in \Expect_I [N((e_0)_I)]} <\beta, g\rangle\\
&= [p \cos{\angle(\beta, e_0)} + (1-p)  V_1(\beta_{(0)}) \sin{\angle(\beta, e_0)}] \|\beta\|_2
\end{array}
  \]
  Here $\angle(\beta, e_0)\in [0, \pi], \sin{\angle(\beta, e_0)}\in [0,1]$. 
  
\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/Angle_Diagram_label.png}
\caption{Demonstration of relation between
  $\angle( \beta, -e_0)$ and ${\angle(u, e_0)}$}
\label{fig-Angle}
\end{figure}
  
  \begin{lemma}
  \label{Angle_Inequality}
   \[
  \angle(  \beta, - e_0) \geq  \frac{\pi}{2} - \theta
  \]
  
    \[
  \tan(\angle(  \beta, - e_0)) \geq \cot{\theta}
  \]
  \end{lemma}
  
  \begin{proof}
   
%   Let  $e_{0,u} = N(P_{u}^{\perp} e_0)$ be the unit vector along $P_{u}^{\perp} e_0$, then 
we know that geometrically, using the property that projection of $e_0$ on the hyperplane with normal vector $u$ has the smallest angle among all the $\beta$ in that hyperplane, we have
   \[
  \angle(  \beta, - e_0) \geq \frac{\pi}{2} - \angle(u, e_0) = \frac{\pi}{2} - \theta
  \]
then
  \[
  \tan(\angle(  \beta, - e_0)) \geq \cot{\theta}
  \]
 
  \end{proof}
  
  
 \begin{lemma}
 Let $H_u=\{\beta : \quad u^T \beta =0 \}$. For all $p$ that 
   \[
      \frac{1-p}{ p}  \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]>1
  \]
 the convex program finds the correct inverse filter $a^{-1}$ and hence the sparse signal $X$.
  \end{lemma}
  


  \begin{proof}
 
We know that the KKT condition of the convex program is
  \[
  p \cos{\angle(\beta, e_0)} + (1-p)  V_1(\beta_{(0)}) \sin{\angle(\beta, e_0)}>0
  \]
  if and only if 
  $\cos{\angle(\beta, e_0)}\geq 0,$ or $\cos{\angle(\beta, e_0)}<0$ and 
  \[
      \frac{1-p}{ p}  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}>1
  \]
  If $\cos{\angle(\beta, e_0)}<0, \cos{\angle(\beta, -e_0)}>0, \angle(\beta, -e_0) \in [0, \frac{\pi}{2}).$ 
  
  Therefore,
  \[
      \frac{1-p}{ p}  \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]>1
  \]
  
   \end{proof}
 
  
   \begin{theorem}
 \label{thm:PT_lower}
 Let $p^\star_1 = 1- \tan{\theta},$ then if $p< p^\star_1 $, then the convex program finds the correct inverse filter $a^{-1}$ and hence the sparse signal $X$.
 \end{theorem}
 
%   \begin{theorem}
%  \label{thm:PT_upper}
%  Let $p^\star_2$ be the solution of 
%   \[
% \tan{\theta}  = 
%  (1-p^\star)(\sqrt{2}+(1-\sqrt{2})p^\star)
%  \]

%  \end{theorem}
 \begin{proof}
  Now we study the relation between
  `
  As demonstrated in figure~\ref{fig-Angle}. Since $u^T \beta =0, P_{u}^{\perp}  \beta = \beta.$ Without loss of generality we could assume $\angle(u, e_0) \in [0, \frac{\pi}{2}]$ (otherwise we could flip the sign of the final solution.)


  
  Therefore, we could find a lower bound
    \BEAS
      \frac{1-p}{ p}  \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]
      &\geq& \frac{1-p}{ p}  \inf_{\beta\in H_u} V_1(\beta_{(0)}) \inf_{\beta\in H_u}\tan{(\angle(\beta, -e_0))}]\\
      &=& \frac{1-p}{ p} \inf_{\beta\in H_u} V_1(\beta_{(0)}) \cot{\theta}
  \EEAS
 
Moreover,
\[
\inf_{\beta\in H_u} V_1(\beta_{(0)}) \geq p
\]
where the lower bound is achieved when $\beta_{(0)}$ is one-sparse.
So we have a lower bound $p^\star_1 $ (on the actual phase transition sparsity $p^\star$) defined as,
  \[
 \frac{1-p_1^\star}{ p_1^\star} p_1^\star \cot{\theta} =1
  \]
  Then $p^\star_1 = 1- \tan{\theta},$ then if $p< p^*$, then the convex program finds the correct inverse filter $a^{-1}$ and hence the sparse signal $X$.
  \end{proof}
  
  
  
  
   
%   We need the inequality to be true for all possible $\beta$ so that $u^T \beta =0$, to make the previous inequality tight we consider a small cone in that hyperplane define as $P_{u}^{\perp}\mathbb{K}(-e_0,\theta ,\epsilon) : =\{\beta : \quad u^T \beta =0, \tan{(\angle(\beta, -e_0))}-\cot{\theta}<\epsilon \}$, then 
%       \[
%       \inf_{ P_{u}^{\perp}\mathbb{K}(-e_0,\theta ,\epsilon)} [V_1(\beta_{(0)})]  \cot{\theta}> \frac{ p}{1-p}
%   \]
%   so the phase transition sparsity $p^\star$ 
%   \[
%  \frac{ p^\star}{1-p^\star}  = 
%  \inf_{ P_{u}^{\perp}\mathbb{K}(-e_0,\theta ,\epsilon)} V_1(\beta_{(0)})\cot{\theta} 
%   \]
  
%   (Qingyun: we could select dense sequence in $\beta_i \in P_{u}^{\perp}\mathbb{K}(-e_0,\theta ,\epsilon)$, so that the $\inf_{ P_{u}^{\perp}\mathbb{K}(-e_0,\theta ,\epsilon)} V_1(\beta_{(0)})$ could be calculated using this dense sequence, and therefore, we can replace $\beta_{(0)}$ with a dense sequence $\beta_i$ so that $\lim_{\|\beta_i-\beta_{(0)}\|_2\rightarrow 0}V_1(\beta_i) = V_1(\beta_{(0)})$. Therefore, $V_1(\beta_{(0)})$ can be computed using a vector $\|\beta_{(0)}\|_0$. )
 
  
% \textbf{TODO}:
% Give a more clear condition for the phase transition.  


\paragraph{Detailed characterization of phase transition threshold}
  We define 
  \[
  b:= \beta_{(0)}/\|\beta\|_2
  \]
   \[
  \nu:= u_{(0)}/\|u_{(0)}\|_2=u_{(0)}/\sin{\theta}
  \]
  so that $\|\nu\|_2=1$.
  Then using the fact that $u_0= \cos{\theta}$, $\|u\|_2=1$ and $\beta_0 = -\sqrt{1-\| \beta_{(0)}\|_2^2}$,
  the condition $u^T \beta =0$ can be translated into
  \[
  -\cos{\theta}\sqrt{1-\| b\|_2^2} + \sin{\theta} \nu^T b =0
  \]
  Then
   \[
  \nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}
  \]
  Therefore, using Cauchy inequality, we recover the geometric conclusion
    \[
  \|b\|_2/\sqrt{1-\| b\|_2^2}  \geq \nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}
  \]
   \begin{lemma}
  We define the phase transition threshold as
  \[
 p^\star(u):= 
 \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))> 0\}
 \]
then
 \[
 p^\star(u):= 
 \sup_{p\in [0,1]}\{\inf_{\| P_{u}^{\perp}\beta\|_2=1 }(-p \cdot \sqrt{1-\| P_{e_0}^{\perp}  P_{u}^{\perp}\beta\|_2^2} + (1-p) \cdot  \E_I\| ( P_{e_0}^{\perp} P_{u}^{\perp} \beta)_I\|_2 ) > 0\}
 \]

 Additionally, for a given $\epsilon>0$, we can define $p^\star(\epsilon),$ as 
 \[
 p^\star(u,\epsilon):= 
 \sup_{p}\{\inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))> \epsilon\}
 \]
 Then $p^\star(u,\epsilon)<p^\star(u).$
 \end{lemma}
 
 
    \begin{theorem}
 \label{thm:PT_upper}
 Let the $\mu$ dependent upper bound $p^\star_2(u)$ be the solution of the equation
      \[
  \tan{\theta}  = 
 \frac{1-p^\star}{p^\star}V_1(\nu)
 \] 
then for a given initial choice $v$ and true inverse filter $a^{-1}$, we define $u$ by $\title{u}= a^{-1} * v$, and reparemetrize $u = \cos{\theta} e_0 +\sin{\theta}\nu$, then the phase transition point has an upper bound given by $p^\star_2(u)$.
If $p> p^\star_2$, then the solution of the convex program is not the correct inverse filter $a^{-1}$.

And there is a $\mu$ independent upper bound $p^\star_3$, as the solution of the equation
    \[
  \tan{\theta}  = 
 \frac{1-p^\star}{p^\star}\sqrt{p^\star}
 \] 
 then $p^\star_1 \leq p^\star(u)\leq p^\star_2(u)\leq p^\star_3$.
 \end{theorem}
 \begin{coro}
If $u$ is two sparse, there exists $i$ such that $u_i = \pm \sin{\theta},$ then $u$ is also two sparse and we could get a two sparse $\beta = (0, \ldots,0, \beta_0, 0, \ldots,0, \beta_i, 0, \ldots,0). $ Then $ p_2^\star(u) = p^\star_1$, therefore, $p^\star(u) = p^\star_1 = 1-\tan{\theta} $. 
 \end{coro}
  
   \begin{proof}
  We want to calculate 
   \[
 B(p)= \inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))
  \]
 After the change of variable,
   \[
  B(p)= \inf_{\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta} }(-p \cdot \sqrt{1-\|b\|_2^2} + (1-p) \cdot  \| b\|_2 V_1(b))
  \]
  $\frac{b}{\|b\|_2}=\nu$, $\|b\|_2 =\cos{\theta}$ is one feasible point to the equation $\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}$, it correspond to $\beta = P_u (-e_0)$. 
  Therefore, plug in this specific $\beta$,
  \[
 \cot{\theta} }(-p \cdot \sin{\theta} + (1-p) \cdot  \cos{\theta} V_1(\nu)) \geq \inf_{\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta} }(-p \cdot \sqrt{1-\|b\|_2^2} + (1-p) \cdot  \| b\|_2 V_1(b))
  \]
  we find an upper bound on phase transition point  $p^\star_2(u) \geq p^\star(u)$. 
  Here $p^\star_2(u)$ is defined by
   \[
 p_2^\star(u):= 
 \sup_{p\in [0,1]}\{\cot{\theta} }(-p \cdot \sin{\theta} + (1-p) \cdot  \cos{\theta} V_1(\nu)) > 0\}
 \]
 then $p^\star_2(u)$ is the solution of the equation
   \[
  \tan{\theta}  = 
 \frac{1-p^\star}{p^\star}V_1(\nu)
 \] 
 Since $V_1(\nu)\leq \sqrt{p}$,
 the $\mu$ independent upper bound $p^\star_3$ is the solution of the equation
    \[
  \tan{\theta}  = 
 \frac{1-p^\star}{p^\star}\sqrt{p^\star}
 \] 
  \end{proof}
  
  

  \begin{lemma}
%   To find the phase transition parameter $p^\star$, we need to solve the constrained optimization problem 
%   \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}\\
%  \mbox{subject to}  
% &  u^T \beta = 0,\\
% &   \|\beta\|_2^2 =1.
% \end{array}
% \EEQ
% Assuming $\| u\|_2=1$.
% Using the fact that 
% \[
% \angle(\beta, -e_0))\geq \frac{\pi}{2}-\angle(u, e_0))=\frac{\pi}{2}-\theta
% \]
% We have an additional condition
% \[
% u^Te_0 = u_0 = \cos{\theta}
% \]
%   \[
%       \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]
%   \]
% Therefore, we could add a third condition into the optimization  
%  \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}\\
%  \mbox{subject to}  
% &  u^T \beta = 0,\\
% &   \|\beta\|_2^2 =1,\\
% & e_0^T \beta = \beta_0 \geq \sin{\theta}.
% \end{array}
% \EEQ
% There are two candidate solution, one is when $\beta_0 = \sin{\theta},$ then $\|\beta_{(0)}\|_2 =  \cos{\theta}$, and 
% the problem becomes
% \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \cot{\theta}\\
%  \mbox{subject to}  
% &  u^T \beta = u_0 \beta+ u_{(0)}^T\beta_{(0)} = \cos{\theta}\sin{\theta}+u_{(0)}^T\beta_{(0)}= 0,\\
% &   \|\beta_{(0)}\|_2^2 =\cos{\theta}^2.
% \end{array}
% \EEQ
 

% If $u$ is denser than two sparse, then we can choose a $3-$sparse $\beta$, so that $\beta_0 = \sin{\theta}.$Then let 
% $r =\cos{\theta} \beta_{(0)},$  reducing the constant $\cot{\theta}$, our problem becomes 
% \BEQ
%  \begin{array}{ll}
%  \underset{r}{ \mbox{minimize} }  & V_1(r)  \\
%  \mbox{subject to}  
% &  \sin{\theta}+u_{(0)}^T r= 0,\\
% &   \|r\|_2 =1.
% \end{array}
% \EEQ
% then if there does not exist $i$ such that $u_i = \pm \sin{\theta},$ we need to have a $r$ that is at least $2-$ sparse.
%   Noticing that   
%   \[
% V_1(\frac{ e_i+e_j}{\sqrt{2}}) = p(\sqrt{2}+(1-\sqrt{2}p)).
% \]
% is the maximum value of $V_1(r)$ among all  $2-$ sparse $r$ on sphere.

% Then 
% \[
% p\leq V_1(r)\leq p(\sqrt{2}+(1-\sqrt{2}p))
% \]
% We want to choose a $2-$sparse $r$ on the sphere $\|r\|_2 =1$ that is as unbalanced as possible so that $V_1(r)$ and still satisfy $\sin{\theta}+u_{(0)}^T r= 0.$

  \end{lemma}
  
  
%   Comment:
%  \[
%  V_1(\beta_{(0)})
%  \]
%   should be between $[p,\sqrt{p}]$, from empirical observation, it is closer to $\sqrt{p}$.
  
 
 


% % So that   
% %   \[
% % p^\star \cot{\theta} \leq \frac{ p^\star}{1-p^\star}  \leq
% %  \sqrt{p^\star}\cot{\theta} 
% %   \]
  
% %   So 
% %     \[
% % 1- \tan{\theta}  \leq p^\star  \leq \sqrt{(1+\tan{\theta}^2/2)^2 -1}+(1+\tan{\theta}^2/2)
% %   \]
  
%  If we know that for $\beta \in H_u$ near the direction $P_u^\perp (-e_0)$ must not be $1-$sparse but could be $2-$sparse, then  
%   \[
%       \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]\leq  p(\sqrt{2}+(1-\sqrt{2}p)) \cot{\theta} 
%   \]
  
%   If this is indeed the correct condition, then
%     \[
%   1  = 
%  \frac{1-p^\star}{ p^\star}
%  p^\star(\sqrt{2}+(1-\sqrt{2}p^\star))\cot{\theta} 
%  \]

%     \[
%   \tan{\theta}  = 
%  (1-p^\star)
% (\sqrt{2}+(1-\sqrt{2}p^\star)) 
%  \]


 
  
% \subsection{Locally robust objective and semi-continuous extension}  
% Now, we study the \textbf{lower semicontinuous extension}.


% \paragraph{Locally robust objective}
%  Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
%  \[
%  \begin{array}{ll}
%   \underset{w}{ \mbox{minimize} }  & \sup_{\|\omega-w\|_2\leq \epsilon} \Expect|(\omega*Y)_0|\\
%  \mbox{subject to}  
% &  \omega_0 =1, \quad w_0 =1, \quad w, \omega \in V_{rs, rt}.
% \end{array}
%   \]
% after change of variables, and modulo constant $\sqrt{\frac{2}{\pi}}$, we have
%   \[
%  \begin{array}{ll}
%   \underset{\psi    }{ \mbox{minimize} }  & \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2\\
%  \mbox{subject to}  
% &  u^T \psi =1, \quad a^{-1}*\psi \in V_{rs, rt}.
% \end{array}
% \tag{$P_\epsilon$}
%   \]
%   Our first question is to understand the relation between this objective and the following deterministic objective as $\epsilon \rightarrow 0$.
%   \[
%  \begin{array}{ll}
%   \underset{\psi    }{ \mbox{minimize} }  & \|\psi\|_2\\
%  \mbox{subject to}  
% &  u^T \psi =1, \quad a^{-1}*\psi \in V_{rs, rt}.
% \end{array}
% \tag{$P'_0$}
%   \]

% \begin{lemma} 
% Let
% \[
% V_1(\psi):=\frac{\Expect_I\|\psi_I\|_2}{\|\psi\|_2} 
% \]
% then
%  \[
%  \begin{array}{ll}
%  &\lim_{\epsilon\rightarrow 0^+}   \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2 \\
%  = & [\lim_{\epsilon\rightarrow 0^+}\sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h)] \|\psi\|_2
% \end{array}
%   \]
%   However, 
%   \[
%  \begin{array}{ll}
% p \leq  [\lim_{\epsilon\rightarrow 0^+}\sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h)] \leq \sqrt{p}
% \end{array}
%   \]
%   it does dependent on $\psi.$
%  \end{lemma} 
% \begin{proof}
%  \[
%  \begin{array}{ll}
%  &  \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2 \\
%  =&   \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \frac{\Expect_I\|\psi_I+\epsilon \cdot h_I\|_2}{\|\psi+\epsilon \cdot h\|_2} \|\psi+\epsilon \cdot h\|_2\\
%  = & \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h) \|\psi+\epsilon \cdot h\|_2
% \end{array}
%   \]
%   where 
%     \[
%  \begin{array}{ll}
%  &  \lim_{\epsilon\rightarrow 0^+}  \|\psi+\epsilon \cdot h\|_2 = \|\psi\|_2
% \end{array}
%   \]
%   But $p \leq  V_1(\psi+\epsilon \cdot h) \leq \sqrt{p} $ and it does dependent on $\psi$ globally.
% \end{proof}





























% Question:
% how to calculate the expectation
% \[
%  \begin{array}{ll}
% P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}
% \end{array}
% \]
% To show that 
% \[
%  \begin{array}{ll}
% 0\in P_{u}^{\perp} \Expect_I [N((e_0)_I) ]
% \end{array}
% \]
% we need to prove
% \[
%  \begin{array}{ll}
% \frac{p \sin{\theta} }{(1-p) \cos{\theta}}e_{0,u} \in \frac{1}{\cos{\theta}} P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}
% \end{array}
% \]
% This quantity should be something like
% \[
%  \begin{array}{ll}
%  \frac{1}{\cos{\theta}} P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}} = (1-(1-p)^n)\cdot D_1
% \end{array}
% \]
% where $D_1$ should be a unit disk that contains $-e_{0,u}$, but I am not sure how to prove it since I don't know how to calculate $\Expect_{I_{(0)}}D_{I_{(0)}}$ and $P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}$.

% \paragraph{Directional derivative}

% We can go back to the previous \textbf{directional finite difference} analysis by
% \begin{lemma}
%  The directional derivative
% \[
%  \begin{array}{ll}
% \lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
% &= \sup_{u\in \Expect_I [N((e_0)_I)]} <\beta, u\rangle\\
% \end{array}
%   \]
%  First, 
% \[
%  \begin{array}{ll}
% \sup_{u\in \Expect_I [N((e_0)_I)]} <\beta, u\rangle
% &= p <\beta,e_0\rangle + (1-p) \sup_{u\in \Expect_{I_{(0)}}D_{I_{(0)}} } <\beta, u\rangle
% \end{array}
%   \]
%  Second, 
% \[
%  \begin{array}{ll}
% \sup_{u\in P_{u}^{\perp} \Expect_I [N((e_0)_I)]} <\beta, u\rangle
% &= p   \sin{\theta} <\beta,e_{0,u}\rangle + (1-p)\cos{\theta} \sup_{u\in \Expect_{I_{(0)}}D_{I_{(0)}} } <\beta, u\rangle
% \end{array}
%   \]
% \end{lemma}





\subsection{Bi-Lipschitz property of finite difference of objective near $e_0$}
We study the upper and lower bound of: 
\[
B(p, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
\]


\paragraph{Bi-Lipschitzness of finite difference of objective for sphere constraint}
\begin{lemma}
For the sphere constraint $\|e_0 + \phi\|_2 =1$ for any $\phi$, 
  \[
 \begin{array}{ll}
\frac{1}{16}p(1-p) \|\phi\|_2 \leq  
% \Expect_I\|(e_0+\phi)_I\|_2 -  \Expect_I\|(e_0)_I\|_2 = 
V_1(e_0+\phi) - V_1(e_0) \leq 2\sqrt{N} \|\phi\|_2
\end{array}
  \]
\end{lemma}
This lemma is based on Proposition $C.7$(upper bound) and $C.8$(lower bound) of section $C.6$ of the paper \cite{bai2018subgradient}, proof can be found in there.

% \paragraph{A new metric to solve gradient non-Lipschitzness}

% First, $\psi \mapsto \| \psi \|_2$ is Lipschitz for $\ell_2$ convergence. And 
% $\psi \mapsto \E_I\| \psi_I \|_2$ is Lipschitz for $\ell_2$ convergence.
% Then $\beta \mapsto \Expect_I [\|(\psi+ \beta)_I\|_2 - \|(\psi)_I\|_2]$
% is Lipschitz for $\ell_2$ strong convergence.

% However, notice that 
%  $\beta \mapsto \lim_{t\rightarrow 0^+} 
% \frac{1}{t}\Expect_I [\|(\psi+ \beta)_I\|_2 - \|(\psi)_I\|_2]$
% and 
%  $
%  \E{\partial_\psi\| (\psi)_I\|_2 }  =  \E_I [N(\psi_I)]
% $
% are not Lipschitz in $\psi$ with respect to the Euclidean metric $d_2(a,b) :=\|a-b\|_2$ nor the angle metric $d_A(a,b) := \frac{1}{\pi}\angle(a, b)$. 

% They are Lipschitz with respect to a stronger metric on the sphere which is sign-pattern aware and averages all “subset angles” (see \cite{bai2018subgradient} section $4.2$ for detailed discussion and lemma $F.4$ for the proof of  Lipschitz property):
% \[
% d_E(a, b) := \frac{1}{\pi} \E_I\angle(a_I, b_I)
% \]


 
%   The directional gradient of the locally robust objective for a give direction $\beta$ so that $\|\beta\|_2 =1, u^T \beta =0, a^{-1}*\beta \in V_{rs, rt}.$ we study
%   \[
%  \begin{array}{ll}
% \lim_{\epsilon\rightarrow 0^+} \sup_{\|h\|_2\leq 1} \Expect_I\|\psi_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 
% \end{array}
%   \]
  
% \begin{lemma}
%  The locally robust directional derivative at $e_0$ along $\beta$ 
%  evaluates to the following:
%   \[
%  \begin{array}{ll}

%  & \lim_{\epsilon\rightarrow 0^+} \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2) \\
% =&\|\beta\|_2 \{p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} \lim_{\epsilon\rightarrow 0^+} [\sup_{\|h\|_2\leq 1} V_1((\beta+\epsilon \cdot h)_{(0)})] \} .
% \end{array}
%   \]
% \end{lemma}
%  \begin{proof}
% Applying Lemma \ref{eq:ComputeExpect}, we proceed as follows:
% \[
%  \begin{array}{ll}
%  & \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2)\\
% =& \sup_{\|h\|_2\leq 1} \sup_{g\in \Expect_I [N((e_0)_I)]} \langle\beta +\epsilon \cdot h, g\rangle\\
% % &= \sup_{g\in  [N((e_0)_I)]} \Expect_I\langle\beta, g\rangle\\
% =& \sup_{\|h\|_2\leq 1}[p \cdot \langle\beta +\epsilon \cdot h, e_0\rangle + (1-p) \cdot  \sup_{g\in {\cal B}_0 } \langle\beta +\epsilon \cdot h, g\rangle]\\
% =& \sup_{\|h\|_2\leq 1}[p \cdot \langle\beta +\epsilon \cdot h, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|(\beta +\epsilon \cdot h)_{I}\|_2 | 0 \not \in I ] ]\\
% =& \sup_{\|h\|_2\leq 1}[[p \cdot \cos{\angle(\beta +\epsilon \cdot h, e_0)} + (1-p) \cdot  \sin{\angle(\beta +\epsilon \cdot h, e_0)} V_1((\beta +\epsilon \cdot h)_{(0)})] \|\beta +\epsilon \cdot h\|_2]
% \end{array}
%   \]
%   Taking limit for $\epsilon\rightarrow 0^+$,using the fact that $\| \cdot \|_2, \sin(\cdot), \cos(\cdot) $ are all Lipschitz function, 
%  \[
%  \begin{array}{ll}
%  &\lim_{\epsilon\rightarrow 0^+} \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2)\\
% =& \lim_{\epsilon\rightarrow 0^+} \{\|\beta +\epsilon \cdot h\|_2 [p \cdot  \cos{\angle(\beta +\epsilon \cdot h, e_0)} + (1-p) \cdot  \sin{\angle(\beta +\epsilon \cdot h, e_0)} V_1((\beta +\epsilon \cdot h)_{(0)})]\} \\
% =&\|\beta\|_2 \{p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} \lim_{\epsilon\rightarrow 0^+} [\sup_{\|h\|_2\leq 1} V_1((\beta+\epsilon \cdot h)_{(0)})] \}
% \end{array}
%   \] 
%   \end{proof}

\paragraph{Bi-Lipschitzness of finite difference of objective for linear constraint}
We normalize the problem by defining $t:=\|\phi\|_2, \beta:=\frac{\phi}{\|\phi\|_2}$.
After normalization, and taking into account of the linear constraint $u^T \phi = 0$, we will study that  for $\beta\in \mathcal{B}_t :=\{\|\beta\|_2=1, u^T \beta = 0,  \|e_0+t\beta\|_\infty\leq 1 \}$ for finite $t$, what is the upper and lower bound of 
\[
\frac{\E_I  \| (e_0+t\beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\]
First, if $t\rightarrow 0^+$, then we get the directional derivative along direction of $\beta$. 
\BEAS
\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
&=&(1-p) \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]  + 
p\beta_0  
\\
&=&
(1-p) V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2} + 
p\beta_0  
\EEAS
where  $\|\beta_{(0)}\|_2 = \sqrt{1-\beta_0^2} $ since  $\|\beta\|_2 = 1$, and
\[
V_1(\beta_{{(0)}})= \frac{\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]}{\|\beta_{(0)}\|_2}.
\]
We know that for 
\BEAS
p \leq V_1(\beta_{{(0)}})
\leq \sqrt{p}
\EEAS
Where  
\[
\beta^a = ( \beta_0,\sqrt{1-\beta_0^2}, 0,\ldots,0 )
\]
achieves lower bound,
and 
\[
\beta^b = (\beta_0,\frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2},\ldots, \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} ) = \beta_0 e_0 + \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} (\sum_{i\neq 0} e_i)
\]
achieves upper bound.


For finite $t$, we calculate the finite difference condition on $I_0$:
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
&=&
(1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big)
\EEAS

We look into the following quantity for finite $t$,
\BEAS
\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t}
&=&
\Expect_{I}[ \left( (\frac{1}{t}+ \beta_0)^2+\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
&=& \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ]
\EEAS

\begin{lemma}
We have upper bound 
\BEAS
 \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ] 
\leq  \beta_0+ \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2
\EEAS
and a lower bound
\BEAS
\frac{1}{t} (\left| 1 + t \beta_0 \right|-1 ) \leq \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ] 
\EEAS
we comment that if $\beta_0 \geq -\frac{1}{t}$, the lower bound reduce to
\BEAS
\beta_0 \leq \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ] 
\EEAS
% \BEAS
%  \Expect_{I}[ \left( \| \beta_{I_{(0)}} \|_2^2+(\frac{1}{t}+ \beta_0)^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]
% \geq \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2
% \EEAS
\end{lemma}

\begin{proof}

Now we use the expansion
\[
\sqrt{1+x}-1= \frac{x}{2}-\frac{1}{8}x^2+1/16x^3-5/128x^4+O(x^5)
\]
first we have upper bound 
for any $x\geq -1$:
\[
\sqrt{1+x}-1 - \frac{x}{2}\leq 0
\]
% and a higher order upper bound that is tighter for $x\leq 2,$
% \[
% \sqrt{1+x}-1 - \frac{x}{2}\leq -\frac{1}{8}x^2+1/16x^3
% \]
% for any $x\geq 0$, we also have lower bound:
% \[
%   -\frac{1}{8}x^2 \leq \sqrt{1+x}-1-\frac{x}{2}
% \]
Additionally, using concavity of function $\sqrt{1+x}$, we have
\BEAS
 && \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ]\\
&\leq&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\Expect_{I}\| \beta_{I_{(0)}} \|_2^2| 0 \in I ] \right)^{1/2} -1]\\
&=&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p \| \beta_{{(0)}} \|_2^2 \right)^{1/2} -1]\\
&=&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p (1-\beta_0^2) \right)^{1/2} -1]
\EEAS
Now, apply the inequality above, we have
\BEAS
 \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p \| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1]
&\leq&  \beta_0 + \frac{t}{2} (p \| \beta_{{(0)}} \|_2^2  +  \beta_0^2)
\EEAS
On the other hand,
\BEAS
\frac{1}{t} \Expect_{I}[ \left( (1+ t\beta_0)^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]
&\geq&  \frac{1}{t} (\left| 1 + t \beta_0 \right|-1 )
\EEAS
when $\beta_0 \geq -\frac{1}{t}$,
\BEAS
\frac{1}{t} (\left| 1 + t \beta_0 \right|-1 )
= \beta_0 
\EEAS
% also, for $t<1$, we also have the expansion
% \BEAS
% && \Expect_{I}[ \left( \| \beta_{I_{(0)}} \|_2^2+(\frac{1}{t}+ \beta_0)^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
% &=& \beta_0 + \frac{t}{2} \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] + \frac{t}{2} \beta_0^2 - 
% \frac{1}{8t} (2t\beta_0 +t^2 (\beta_0^2 + \| \beta_{I_{(0)}} \|_2^2) )^2 + \frac{1}{16t} (2t\beta_0 +t^2 (\beta_0^2 + \| \beta_{I_{(0)}} \|_2^2) )^3 + \ldots \\
% &=& \beta_0 + \frac{t}{2} \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] + \frac{t}{2} \beta_0^2 - \frac{t}{2} \beta_0^2 
% -  \frac{t^2}{2} \beta_0 \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] 
% - \frac{t^2}{2} \beta_0^3  +  \frac{t^2}{2} \beta_0^3 
% + O(t^3)\\
% &=& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \EEAS
% When $\beta_0 <0$, then
% \BEAS
% && \Expect_{I}[ \left( \| \beta_{I_{(0)}} \|_2^2+(\frac{1}{t}+ \beta_0)^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
% &=& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)\\
% &\geq& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2
% \EEAS

\end{proof}

\begin{theorem}
\label{thm:bound_diff}
We have upper bound and lower bound 
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\leq 
(1-p)\Big( V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2}\Big) + 
p\Big(\beta_0  +
  \frac{t}{2} \beta_0^2 
 +
 p\frac{t}{2}  (1-\beta_0^2) \Big)
\EEAS
and lower bound 
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\geq 
(1-p)\Big( V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2}\Big) + 
p\Big(\frac{1}{t} (\left| 1 + t \beta_0 \right|-1 \Big)
\EEAS
Specially, when $t\leq 1$, $\frac{1}{t} (\left| 1 + t \beta_0 \right|-1 = \beta_0$, therefore,
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\geq 
(1-p)\Big( V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2}\Big) + 
p\beta_0 = \lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\EEAS
\end{theorem}

Qingyun's Remark: this bound is numerically verified for $t\leq 5$ with Matlab. 
Where we use the fact that $p\leq V_1(\beta_{{(0)}}) \leq \sqrt{p},$ for both $\beta_0 = 1, -0.5, -1/\sqrt{N}, 0,1/\sqrt{N}, 0.5, 1 $, we tested the two extreme points  
\[
\beta^a = ( \beta_0,\sqrt{1-\beta_0^2}, 0,\ldots,0 )
\]
and 
\[
\beta^b = (\beta_0,\frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2},\ldots, \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} ) = \beta_0 e_0 + \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} (\sum_{i\neq 0} e_i)
\]

\begin{coro}
\label{coro:bound_diff}
We have upper bound 
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
&\leq& 
(1-p)\Big( \sqrt{p} \sqrt{1-\beta_0^2}\Big) + 
p\Big(\beta_0  +
  \frac{t}{2} \beta_0^2 
 +
 p\frac{t}{2}  (1-\beta_0^2) \Big) \\
 &\leq& 
 (1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{t}{2} 
 +
 p\frac{t}{2}   \Big)
\EEAS



\end{coro}


\begin{coro}
\label{coro:bound_diff}
We have  lower bound for $p<p^\star(\epsilon)$ and $t\leq 1$:
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
&\geq&
\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\geq
\epsilon
\EEAS


\end{coro}


% \paragraph{Minor result}


% \begin{coro}
% We have upper bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big)\\
% &\leq& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2\big)\\
% &\leq& (1-p)  \sqrt{p} \| \beta_{{(0)}} \|_2 + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2\big)\\
% \EEAS
% \end{coro}


% \begin{lemma}
% We have asymptotic relation for $t<1$, 
% \BEAS
% && \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}\\
% &=& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + 
% p\big(
% \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 
% -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \big)\\
% &=& (1-p) V_1(\beta_{{(0)}}) \| \beta_{{(0)}} \|_2 + 
% p\big(
% \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 
% -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \big)\\
% &=& (1-p) V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2} + 
% p\beta_0 + p^2\big(
%  \frac{t}{2}  (1-\beta_0^2) 
% -  \frac{t^2}{2} \beta_0 (1-\beta_0^2) \big) + O(t^3)
% % \\
% % &=& (1-p) V_1(\beta_{{(0)}}) \cos (\angle(e_0,\beta)) + 
% % p\sin (\angle(e_0,\beta)) + p^2 \big(\frac{t}{2}  \cos (\angle(e_0,\beta))^2 
% % -  \frac{t^2}{2} \sin (\angle(e_0,\beta))  \cos (\angle(e_0,\beta))^2 + O(t^3)
% % \big)
% \EEAS
% \end{lemma}


% \begin{coro}
% If $t<1$, and $\beta_0<0$, we have lower bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big)\\
% &\geq& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  \big)\\
% &\geq& (1-p)  p \| \beta_{{(0)}} \|_2 + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 \big)\\
% \EEAS
% \end{coro}


% \begin{coro}
% If $\beta_0<0$ and  $t\geq \frac{1}{|\beta_0|}$ so that it allows $(1+t \beta_0)^2 =0$ is achievable, we have lower bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 +p\frac{1}{t}[ \E_{I_{(0)}} \left(  \| t \beta_{I_{(0)}} \|_2^2+(1+t \beta_0)^2 \right)^{1/2} -1]\\
% &\geq& (1-p)  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 +p  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 - \frac{p}{t}\\
% &=& \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 - \frac{p}{t}\\
% &\geq& p\| \beta_{{(0)}} \|_2 - \frac{p}{t}
% % \\
% % &\geq& p(\| \beta_{{(0)}} \|_2 - \max\{|\beta_0|,\frac{1}{t}\} )
% \EEAS
% \end{coro}

% % \begin{proof}


% % \end{proof}







% In the following, we use mean value theorem to calculate this quantity in a different way.
% \paragraph{Mean value theorem}
% \begin{lemma}[Lebourg’s mean value theorem, Theorem $2.3.7$ of \cite{clarke1990optimization}]
% Let $x,y$ be distinct points in $\reals^d$, and suppose that $f: \reals^d \rightarrow \reals$ is locally Lipschitz on an open set $U$ containing the line segment $[x, y]$. Then there exists a $\eta \in (0,1)$ such that
% \[
% f(y) - f(x) \in \langle \partial f (x+ \eta(y-x)) , y - x\rangle . 
% \]
% Let $t :=\|y-x\|_2 $, and let $\beta:= \frac{y-x}{t}$ be a unit vector along the direction of $y-x$ so that $y-x = t\beta$. We could reformulate the theorem as that there exists a constant $\eta \in (0,1)$ such that
% \[
% f(x+t\beta) - f(x) \in 
% \langle \partial f (x+ t \eta \beta) , t\beta\rangle . 
% \]
% \end{lemma}
% Using Lebourg’s mean value theorem for $\E_I [\| (\psi)_I \|_2| 0 \in I ]$ near $e_0$ to use its locally Lipschitz property, 
% the result is that there exists a constant $\eta \in (0,1)$ such that
% \[
% \frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t}
%  \in 
%  {\Expect}_I \langle  [N(e_0+ t \eta \beta_I)] , \beta\rangle  | 0 \in I ]
% \]


























% (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}$
% and for $\beta\in \{\|\beta\|_2=1,  \|e_0+\beta\|_2 = 1, (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}.$






% and use the fact that $(1+\beta_0)^2 > \beta_i^2, \forall i\neq 0$, we have $(1+\beta_0)^2> \frac{1}{N-1}\| \beta_{(0)} \|_2^2$,
% \BEAS
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+(1+\beta_0)^2 \right)^{1/2} -1]
% &\geq& 
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+\frac{1}{N-1}\| \beta_{(0)} \|_2^2 \right)^{1/2} -1]
% \\
% &\geq& 
% [ \E_{I_{(0)}} \left( \frac{ \| \beta_{I_{(0)}} \|_2^2}{\| \beta_{(0)} \|_2^2}+\frac{1}{N-1} \right)^{1/2} \| \beta_{(0)} \|_2-1]
% \\
% &\geq& 
% [ \E_{I_{(0)}} \left( \frac{ \| \beta_{I_{(0)}} \|_2^2}{\| \beta_{(0)} \|_2^2}+\frac{1}{N-1} \right)^{1/2} \| \beta_{(0)} \|_2-1]
% \EEAS


% For $\beta\in \{\|\beta\|_2=1,  \|e_0+\beta\|_2 = 1, (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}$, we have
% $(1+\beta_0)^2 = 1-\| \beta_{(0)} \|_2^2,$ let $\bar{I}_{(0)}$ be the complement $\cT-\{0\}- I.$
% \BEAS
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+(1+\beta_0)^2 \right)^{1/2} -1]
% &=& 
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+1-\| \beta_{(0)} \|_2^2 \right)^{1/2} -1]
% \\
% &=& 
% [ \E_{\bar{I}_{(0)}} \left( 1-\| \beta_{\bar{I}_{(0)}} \|_2^2 \right)^{1/2} -1]
% \\
% &=& 
% -\sum_{\ell =0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\E_{\bar{I}_{(0)}}\| \beta_{\bar{I}_{(0)}} \|_2^{2(\ell+1)}
% \EEAS


% \paragraph{Upper bound}


% \begin{lemma}  
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%  &\leq p(\beta_0 +t) + (1-p)\sqrt{p} \|\beta_{(0)}\|_2 \\
% &= pt + p\sin (\angle(e_0,\beta)) + (1-p)\sqrt{p} \cos (\angle(e_0,\beta))
% \end{array}
%   \] 
% \end{lemma}


% \begin{proof}
% \[
%  \begin{array}{ll}
% {\Expect}_I [N((e_0+ t \eta \beta)_I)]
% &= 
% p {\Expect}_{I_{(0)}} [N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big)] 
%  + (1-p) {\Expect}_{I_{(0)}} [N\big( t \eta \beta_{I_{(0)}}\big)] \\
%  &= 
% p {\Expect}_{I_{(0)}} [N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big)] 
%  + (1-p) {\Expect}_{I_{(0)}}[ N\big(\beta_{I_{(0)}}\big)]
% \end{array}
%   \]
% then
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%  &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) {\Expect}_{I_{(0)}} [\langle N\big(\beta_{I_{(0)}}\big), \beta\rangle]\\
%   &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
% \end{array}
%   \]
%  where
%  \[
%  \begin{array}{ll}
%  {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  &=  {\Expect}_{I_{(0)}}[  \frac{\beta_0 +t \eta (1 - \|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2}   ]\\
%  &= (\beta_0 +t \eta) {\Expect}_{I_{(0)}} \| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2^{-1} - {\Expect}_{I_{(0)}}\frac{t \eta (\|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2} \\
%  &\leq \beta_0 +t\eta\\
%  &\leq \sin (\angle(e_0,\beta))+t
% \end{array}
%   \]
%  The first inequality comes with the fact that ${\Expect}_{I_{(0)}} \| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2^{-1}\leq 1$, and 
%  ${\Expect}_{I_{(0)}}\frac{t \eta (\|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2} \geq 0$.
 
%  The second inequality comes with the fact that $\eta <1$.
%  and
%   \[
%  \frac{\beta_0}{\|\beta\|_2} = \sin (\angle(e_0,\beta)) .
%  \]

%  Therefore,
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%   &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t ) + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t) + (1-p)\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t) + (1-p)\sqrt{p} \|\beta_{(0)}\|_2 
% \end{array}
%   \] 
%  \end{proof}
 
%  \begin{coro}
%  \[
%  \frac{\E_I  \| (e_0+t\beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t\|\beta\|_2} \leq  
%  pt + p\sin (\angle(e_0,\beta)) + (1-p)\sqrt{p} \cos (\angle(e_0,\beta))
%  \]
%  \end{coro}

==> old_sec/sec_old/backup.tex <==
\begin{proof}
In the following proof, for clarity, we write $\gamma$ simply as $\gamma$.

Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\beq
\label{FoldedGaussianMean_Obj}
\Expect|\psi^T X+\mu| =   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)\right]
\eeq



This is hard to compute, but to give upper and lower bounds, we can leverage a few simple facts:
first, 
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &\geq  1- \frac{ \gamma^2}{2}
\end{array}
  \] 
Second, the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 

% (see: https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function)


Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ O( \gamma^4) ]/[1 + \frac{ \gamma^2}{2}+ O( \gamma^4)] \\
&= 1 -\frac{ \gamma^2}{6}+ O( \gamma^4)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!} \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-1}{12} \gamma^4  +   \frac{\gamma^{4}}{(-2)^2 (2)!} + O(\gamma^6)\\
&=    \frac{1}{24} \gamma^4   + O(\gamma^6)\\
\\
&\geq 0
\end{array}
\] 
We observe that it is only a function of $\mu^2$ and $\psi$, and when $\gamma^{2}\rightarrow 0$, the residual $\mbox{Res}\rightarrow 0$:
\[
 \begin{array}{ll}
\lim_{|\gamma|\rightarrow 0}\mbox{Res} &:= 0
\end{array}
\] 

Then we give an lower bound:
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&= \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]+   \mbox{Res}\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}








%   For $\sigma_2 =0$. If there is $C(\phi^*) \in [C_-, C_+]$ so that
%     \[
%     \begin{array}{ll}
%   \Expect_I \cos[\angle( (I\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]
%   &= C(\phi^*) \cos[\angle( (1\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]\\
%  &= C(\phi^*) \cos[\angle( (e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
%   then 
  
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= C(\phi^*) \langle  \partial  F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\

% \end{array}
%   \]






% Let $f$ be a extended real-valued convex function $f:\reals^d \rightarrow [-\infty, \infty]$, $\imath_{K}$ be the indicator function over $K$, that is, the function that returns $0$ if the argument belongs to $K$ and $+\infty$ otherwise.
% We define convex conjugate of $f$ as $f^*:\reals^d \rightarrow [-\infty, \infty]$, where
% \[
% f^{{*}}(u) := \sup_{x \in \reals^d} \left \{ \langle u , x \rangle - f \left( x \right) \right\}\,,\qquad u \in \reals^d\,.
% \]
% From Fenchel's duality theorem, we have the following lemma
% \begin{lemma}[duality lemma]

% \begin{align}
% \min_{x \in K} f(x) &= \min_{x \in \reals^d} f(x) + \imath_{K}(x)\\
%  &= \min_{x \in \reals^d} \max_{u \in \reals^d}\Big\{\langle x, u\rangle - f^*(u)\Big\} + \imath_{K}(x)\\
% &= \max_{u \in \reals^d}\min_{x \in \reals^d}\Big\{ \imath_{K}(x) + \langle x,u\rangle\Big\} - f^*(u)\\
% &= \max_{u \in \reals^d} (-\imath_{K}^*(-u) - f^*(u)),
% \label{eq:pd_relationship}
% \end{align}
% \end{lemma}  







% \paragraph{Primitive calculation}  
% Notice that
% \[
%  \begin{array}{ll}
%   \sup_{\|Z\|_2\leq 1} \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ] ] 
% = \|\psi\|_2
% \end{array}
%   \]
% We could focus on 
% \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Then we study the difference,
% \[
%  \begin{array}{ll}
% \Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|
% &= \Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )| \\
% % &= \Expect [\mbox{sign}\left((e_0 +\phi)^T (I\cdot G+\eta Z )\right) (e_0 +\phi)^T (I\cdot G ) \\
% % - \mbox{sign}\left( (e_0)^T (I\cdot G+\eta Z )\right) (e_0)^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Let $\eta$ be very small and we study the asymptotic behavior.
% We want to study
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% =& \sup_{\|Z\|_2\leq 1}[\Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )|] \\
% =& \sup_{\|Z\|_2\leq 1}[\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]-\Expect [\mbox{sign}((I\cdot G+\eta Z )_0)  (I\cdot G )_0] 
% \\
%  &+ \eta (\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ])] 
% \end{array}
%   \]
%  We use some crude approximation to gain insight:
  
%  If $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(e_0^T (I\cdot G+\eta Z ))$, then
%  \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}(\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ]) \\
% =& \sup_{\|Z\|_2\leq 1}\Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  \phi^T Z ]\\
% =& \|\phi\|_2
% \end{array}
%   \]
% On the other hand, if  $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(\psi^T (I\cdot G )) $ for all $\psi$, then
% we could use the formula
%   \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G)) \psi^T (I\cdot G) ]
% = \sqrt{\frac{2}{\pi}} \cdot  \Expect_I \| \psi_I\|_2
% \end{array}
%   \]
% So we could have an crude approximate as 
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% \approx & \sqrt{\frac{2}{\pi}} \cdot  \Expect_I [\| (e_0+\phi)_I\|_2-\| (e_0)_I\|_2]
%  + \eta \|\phi\|_2
% \end{array}
%   \]
  

==> old_sec/sec_old/concentration.tex <==
\section{Old concentration results}
% \subsection{Guarantee of inverse kernel recovery}
% \subsubsection{Random model } 
% We first study the following finite sample setting.
% \begin{itemize} 

%   \item We sample a length-$n$ observation $y\in \reals^n$,  
%   from the circular convolution model 
%   \[ 
%   y =  a*x.
%   \]
 
%  \item  Here $x\in \reals^n$ is a random vector where each entry $x_{i} = \Omega_{i} G_{i}$, where  $\Omega$  i.i.d. sampled from Bernoulli distribution $\mbox{Ber}(p)$ and $G$  i.i.d. sampled from Gaussian random variable with variance $1$, $\Omega$ and $G$ are independent.   We define $|S| = \sum_i \Omega_{i}$. 
 
%  We assume $1/4 \geq p\geq 2/n$.

%   \item The kernel $a$ has an inverse filter $w^0$ of length $k+1$, such that 
%   \[
%   a*w^0 =e_1,
%   \]
%   where $*$  is circular convolution of  length $n$.
  
%  To fix the scale and shift of $w^0$, without loss of generality, we assume $w^0_{j} =1$ for some $j$, and it is the entry with largest absolute value. 
 
%   Let $C(a),C(w^0)$ to be the circulant matrix of size $n$ by $n$ generated by $a, w^0$ after zero-padding. Then $C(w^0)= C(a)^{-1}.$  
  
%   We define the condition number of $C(a)$ to be $\delta_a$, which is the ratio of the largest absolute eigenvalue over the smallest absolute eigenvalue.
  
  
% \subsubsection{Perturbation }  
% Consider perturbed filter $w = w^0 + \epsilon v$, and 
% we define 
% \[
% h=  a*v  = a*(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|x+\epsilon h*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*v, v_0 = 1\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 


% %   \item  We define the autocorrelation of $a$ as 
% % \[
% % R(a) = a * \bar{a},
% %  \]
% %  where $\bar{a}$ is the flipped version of $a$.
% % And the $d$-th element of $R(a)$ is the  
% % $d$-lag correlation of $a$ as 
% % \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d},
% %  \]
% %  where we assume periodic boundary condition, $a_{n+d} = a_d$.
% % %  \js{What about the boundary? My understanding is R(a) is a length $n$ vector defined as $R(a) = a \cconv a(-)$ (here $a(-)$ is $a$ flipped), i.e., $R(a)$ is the autocorrelation sequence defined based on circulant convolution. Now $R_d(a)$ is the $d$-th element in this sequence. An alternative way is $R(a) = aC(a)$. }
 
% % Clearly $R_0(a) =  \|a\|_2^2$.
% %  We assume that there is a constant $C$ such that for all $d\neq 0$, 
% %  \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d} \leq C/n^{\beta_{d}}\|a\|_2^2
% %  \]
% % where $\beta_d\geq 1/2$. 


% \end{itemize}
% \begin{theorem} 
% Under the above assumption,
% there exists constant $C_0$, $C$, for all $n>C k^2 \log^2(kp)$, 
% the minimizer $w^*$ of the optimization problem 
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|w*y\|_1\\
% \mbox{subject to}  
% & w_{k+1}=1,\\
% & w \in \reals^{k+1},
% \end{array}
%   \]
% equals $w^0$  with probability $1-\delta$, where 
% \[
%  \begin{array}{ll}
% \delta 
% \leq \exp\left( -C_0 \delta_a^2 k\log(kp)\right)
% \end{array}
% \]
% % \js{I understand this is probably not the final form yet ... What is the $\epsilon$ here? Why setting $n$ to be on the complexity order stated above can make this $\delta$ ``small'' (I suppose this depends on what we set $\epsilon$)?}
% convergences to zero asymptotically as $k$ grows to infinity.

% % \js{(1) $p$ is an important parameter for the problem, should be brought in the problem statement. (2) About $\delta$: mathematical signal processing and relevant communities often asks for the more concrete rate. When people in these fields say something holds with high probability, there's a precise meaning: decay of $\delta$ cannot be slower than $O(n^{-1})$. As a counter-example, $O(\log^{-1}n)$ is too slow to be considered as the event holding with high probability. }
% \end{theorem}
% \begin{proof} 
% To prove the theorem, we do a change of variable 
% \[
% h=  a*w- e_1 = C(a) w- e_1 = C(a)(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|(h+e_1)*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*w- e_1 =  C(w^0)^{-1}(w-w^0)\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 

% Without loss of generality, we assume $\|v\|_2=1$.
  

% We define the difference 
% \[
%  \begin{array}{ll}
% D &= \|(h+e_1)*x\|_1 - \|x\|_1.
% \end{array}
%   \]
% To prove the theorem, we need to prove that the difference $D$ is non-negative.

% Since the problem is convex, we only need to prove that the difference is non-negative  for small perturbation.







% % We define $S$ to be the support of $x$.
% % \[
% %  \begin{array}{ll}
% % D &=  \|h*x+x\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|(h*x)_{S^c}\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|h*x-(h*x)_{S}\|_1 - \|x\|_1\\
% % &\geq  \|h*x\|_1- 2\|(h*x)_{S}\|_1
% % \end{array}
% %   \]
% % Furthermore, 
 




% %  \[
% %  \begin{array}{ll}
% % |\langle C(a^{(i)}) v, x\rangle| \geq  u |\langle v, x\rangle|
% % \end{array}
% %   \]
% % since the smallest absolute value of the absolute eigenvalue of the circulant matrix
% % $ C(a)$ is  $u = |\hat a|_{\min}$.

% Now
% \[
%  \begin{array}{ll}
% D
% &\geq \|h*x\|_1- 2\|(h*x)_{S}\|_1\\
%   &= \sum_{i\in S_j^c} |\langle C(a^{(i)}) v, x\rangle|-\sum_{i\in S_j} |\langle C(a^{(i)}) v, x\rangle|
% \end{array}
%   \]
  
% Let's calculate the expectation 
%   \[
%  \begin{array}{ll}
% \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% &=   \expect \left[ (n-2|S|)  |(h*x)_0| \right] \\
%  &\geq 
% n/2 \expect |(h*x)_0|  
% \end{array}
%   \]
% For a generic $h\in\reals^n$, we have a lower bound on expectation using $\|h\|_2$.
% Let $G_{j}=\mbox{sign}(G_{j}) |G_{j}|$, then $\mbox{sign}(G_{j})$ are IID Rademacher ( $\pm 1$) random variables.
%   \[
%  \begin{array}{ll}
% & \expect  \|h*x\|_1\\
% =& n \expect |(h*x)_0|\\  
%  =& n \expect  |\sum_{j=1}^n h_j\Omega_{j} G_{j}|\\
%  =& n \expect   |\sum_{j=1}^n h_j \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
%  \geq&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j\Omega_{j}G_{j})^2}\\
%  =&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j x_{j})^2}\\
%  \geq&   \frac{n}{\sqrt{2}}   \sqrt{\sum_{j=1}^{n} p h_j^2}\\
%   =&   \frac{n\sqrt{p}}{\sqrt{2}}   \| h\|_2 
% \end{array}
%   \]  
% The first inequality is the
% Khintchine inequality.
% The second inequality is Jensen's inequality, because the function is a convex function of $x$,  
% and the second moment of each entry of $x$ is
% \[ \expect(x_{i})^2  = \expect(\Omega_{i})^2(G_{i})^2=\expect(\Omega_{i})\expect(G_{i})^2 = p.\]
% % We can derive another bound using $h=C(a)v$.
% % \[
% %  \begin{array}{ll}
% % \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% % &=   \expect \left[ (1-2|S|/n) \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle|\right] \\
% %  &\geq 
% % 1/2 \expect \left[\sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right] \\
% % \end{array}
% %   \]
  

% %   We want to find the optimal objective value of the problem
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}   &  \expect \left[ \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle| \right]   \\
% % \mbox{subject to}  & \|v\|_1 =1;
% % \end{array}
% %   \]
% % Using the fact that the objective is a convex function of $v$, and is invariant to permutations,  we know that this function is minimized at the point
% %   $(\frac{1}{ k},\ldots,\frac{1}{ k} )$,
% %    \[
% %  \begin{array}{ll}
% %  &  \expect \left[  \sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right]  \\
% %  \geq&  \frac{1}{ k} \expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} G_{j}| \\
% %  =& \frac{1}{ k}\expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
% %  \geq&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j}G_{j})^2}\\
% %  =&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)x_{j})^2}\\
% %  \geq&   \frac{1}{k\sqrt{2}}  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} p(\sum_{t=1}^{k} |a_{i-t+j}|)^2}\\
% %   =&   \frac{\sqrt{np}}{\sqrt{2}}    \sqrt{(\sum_{i=1}^{n} |a_{i}|)^2}\\
% %    =&   \frac{\sqrt{np}}{\sqrt{2}}   \| a\|_1 
% % \end{array}
% %   \]


 

% As a summary of all the inequalities, we get a lower bound on $\expect D $:
% \[
% \expect D  \geq    \frac{\sqrt{p}}{2^{3/2}}  n \| h\|_2.
% \]
% and
% \[
% \expect D  \geq   \frac{ \sqrt{np} }{2^{3/2}}   \| a\|_1\| v\|_1
% \]

% Also we have bound on the second moment.
% First we define the $s$-lag correlation of $a$ to be 
% \[
% R_s(a) = \sum_{t=1}^n a_{t}a_{t+s},
% \]
% and define the sum of the $s$-lag correlation of $a$ as  
% \[
% \begin{array}{ll}
% R(a) = \sum_{s=1}^{n-1}  R_{s}(a) = \sum_{s=1}^{n-1} \sum_{t=1}^n a_{t}a_{t+s}.
% \end{array}
% \]

% \[
% \begin{array}{ll}
% \mbox{Var} \left(  \|h*x\|_1 \right)
% &= \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x v^T C(a^{(i_2)})^T x|\right)\\
% &=   \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x x^T C(a^{(i_2)}) v|\right)\\
% &\leq   p\left(\sum_{i_1\neq i_2}|v^T C(a^{(i_1)})^T C(a^{(i_2)}) v|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}   (\sum_{t=1}^n a_{t}a_{t+(i_2-i_1)})|\sum_{r_1=1}^k\sum_{r_2=1}^k v_{r_1}v_{r_2}|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}  R_{i_2-i_1}(a) \|v\|_2^2 \right)\\
% &= p   n R(a)\|v\|_2^2
% \end{array}
% \]

% And we have bound on the absolute value,
% % let  $\|X_j\|_{\infty} = \tau$, where $\tau\leq 4$ with probability 
% % $1-\Phi(4)$ for $\Phi$ the Gaussian c.d.f, 
% % and since 
% \[
%  \begin{array}{ll}
% | \langle C(a^{(j)}) v, x\rangle|
% &=  | \sum_{i=1}^n  \sum_{t=1}^k a_{i-t+j} v_t x_{i}|\\
% &\leq   \|a\|_{\infty}|\sum_{t=1}^k v_t|| \sum_{i=1}^n x_{i}|\\
% &\leq  \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| \\
% &\leq    \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| 
% \end{array}
% \]
% with probability $1-\exp{(-Cn)}$, 
% \[
%  | \sum_{i=1}^n x_{i}| \leq 8\tau \sqrt{n},
% \]
% then, 
% \[
%  \begin{array}{ll}
% |\langle C(a^{(j)}) v, x\rangle|
% &\leq     8 \sqrt{n} \|v\|_1 \|a\|_{\infty} \tau 
% \end{array}
% \]


Now we need to derive a concentration inequality on $D$. 
We focus on deriving a concentration inequality on $\|h*x\|_1$, and the concentration inequality 
on  $\|(h*x)_S\|_1$ can be derived similarly.

We remark that $ \|h*x\|_1 =\sum_{j=1}^n |h^{(j),T} x|= \sum_{j=1}^n |\langle C(a^{(j)}) v, x\rangle|$, 
if they are independent random variables, we can bound the deviation of $ \|h*x\|_1$ from its mean
using tail bounds via Bernstein’s inequality, by using the previous two bound on
variance and absolute value. 
This is the strategy to derive concentration inequality in dictionary learning\cite{luh2016dictionary,blasiok2016improved}.
This is also the strategy to derive concentration inequality for multiple observation blind deconvolution setting, since there are independence across different observations.

However, here due to the nature of the convolution, we cannot directly apply Bernstein’s inequality. There are additional dependencies that cause technical difficulties. 

% We need to derive concentration via decoupling, by controlling the moments.
Therefore, we use the dual representation of the $1$-norm and use Talagrand-Bernstein’s inequality on supreme of random function to derive concentration.
We put this part of the proof in the following lemma, since they are technical and they could be of independent interest for other problems with dependency structure. 




From the lemma, if we let $Z = \|h*x\|_1$, then we have 
 \[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&= \prob \left[  |Z- \expect Z | > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.

From the previous calculation, we recall that we have a lower bound on expectation 
$ \expect \|h*x\|_1$,
\[
\expect \|h*x\|_1\geq    \sqrt{\frac{p}{2}}  n \| h\|_2 
\] 
\[
\expect Z = \expect \|h*x\|_1 \geq  \sqrt{\frac{p}{2}}  n \| h\|_2
\]
  









Now we calculate $\sigma^2, K$:
 \[
  \begin{array}{ll}
\sigma^2 &=\expect \langle w, C(h)x \rangle^2,\\
&=\expect (C(h)^* w)^T xx^* C(h)^* w  \\
&\leq  p \|C(h)^* w\|_2^2\\
&=p \langle w, C(h)C(h)^* w \rangle 
\end{array}
  \]  
Let $C(h)=UD(\hat{h})U^*$ be the eigen-decomposition, where $U$ is the unitary Fourier matrix, $D(\hat{h})$ is the diagonal matrix with $\hat{h}$ as its diagonal entries. Then using $h=a*v$, $\hat{h}=\hat{a}\hat{v}$, we have
      \[
  \begin{array}{ll}
(C(h)C(h)*) 
&=   UD(\hat{h})U^* U D(\hat{h})^* U^* \\
&=  UD(|\hat{h}|^2) U^* \\
&=  UD(|\hat{a}\hat{v}|^2) U^*. \\
\end{array}
  \] 
Now we have
 \[
  \begin{array}{ll}
\sigma^2 &\leq 
 p \langle w, C(h)C(h)^* w \rangle \\
&= p  \langle w,  UD(|\hat{a}\hat{v}|^2) U^* w \rangle \\
&= p  \langle U^* w,  D(|\hat{a}\hat{v}|^2) U^* w \rangle 
\end{array}
  \] 
Let $\tilde{w} = \langle U^* w $, using the fact that $\|w\|_{\infty}\leq 1$, we have  $\|\tilde{w}\|_{\infty}\leq 1$, therefore,
 \[
  \begin{array}{ll}
\sigma^2 &\leq  p  \langle \tilde{w},  D(|\hat{a}\hat{v}|^2) \tilde{w} \rangle \\
&=  p  \sum_{i=1}^n \tilde{w}_i^2 |\hat{a}_i\hat{v}_i|^2)  \\
&\leq  p  \sum_{i=1}^n  |\hat{a}_i\hat{v}_i|^2 \\
&\leq  p  \max_{i=1}^n |\hat{a}_i|^2\sum_{i=1}^n  |\hat{v}_i|^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 \|v\|_2^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 
\end{array}
  \] 
  
  Now we derive the absolute value bound. First, since $x_i$ are iid sampled from the product of Bernoulli random variable and standard Gaussian, the supreme of the absolute value $\tau = \max_i |x_i|$ is upper bounded by the  supreme of standard Gaussian, which is less than $  2\log^{1/2} n$ with probability $1-\exp(-Cn^2)$. In the following, we only consider this case and assume $\tau \leq 2\log^{1/2} n$ and add the tail probability into the tail probability in the concentration inequality.
  
 Using other side of Khintchine inequality, we have
  \[
 \begin{array}{ll}
&  |(h*x)_i|\\
 =&  |\sum_{j=1}^n h_{i-j} \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
\leq&  
  \sqrt{\sum_{j=1}^{n} (h_{i-j} \Omega_{j}|G_{j}|)^2}\\
 \leq&  \tau  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n}  h_{i-j}^2}\\
   =&   \tau  \| h\|_2 
\end{array}
  \]  
Therefore, we can take $K=  \tau  \| h\|_2  .$
%    \[
%   \begin{array}{ll}
%  |(C(h)^T w)_i x_i|
% &\leq  \tau |(h^{(i),T} w|\\
% &=  \tau |\sum_{j=1}^n h_{i-j}  w_{j}|\\
% &\leq  \tau \|h\|_1.
% \end{array}
%   \]  

 
%  Notice 
%   \[
%   \begin{array}{ll}
% \|h\|_1 \leq \|h\|_2 n^{1/2}.
% \end{array}
%   \]  
%   We have $K\leq  \tau \|h\|_2 n^{1/2} .$
%  Using Young's inequality
%     \[
%   \begin{array}{ll}
% K= \tau \|h\|_1
% \leq  \tau \|a\|_1\|v\|_1 .
% \end{array}
%   \]   











% Moreover, for $1$-norm of $\|h\|_1$, we have Young's inequality
%     \[
%   \begin{array}{ll}
%   \|h\|_1
% \leq  \|a\|_1\|v\|_1 .
% \end{array}
%   \]     

We point out that the eigenvalues of $C(a)$ is the Fourier transform of $\hat a$ of $a$, which is the 
the entry-wise inverse $1/\hat w^{0}$. And the singular values of $C(a)$ are the absolute values $|\hat a|$. 
% \[
%  \begin{array}{ll}
% \min_i |\hat a_i| = \min_i \frac{1}{ |\hat w^0_i|} 
% =\frac{1}{\max_i |\hat w^0_i|} = u.
% \end{array}
% \]
Therefore, using the fact that $\|v\|_2=1$,
\[
 \begin{array}{ll}
 \min_i |\hat a_i| \leq \|h\|_2 =  \|C(a)v\|_2 \leq \max_i |\hat a_i| 
\end{array}
  \]
  
Then the condition number of $C(a)$ can be represented as $\delta_a =   \max_i |\hat a_i|/\min_i |\hat a_i|$.



Overall, for $Z = \|h*x\|_1$, we have $\expect Z \geq \sqrt{\frac{p}{2}}  n \| h\|_2$, we choose $t = \sqrt{\frac{p}{2}}  n \| h\|_2$. Since 
 \[
  \begin{array}{ll}
 \prob \left[  |Z- \expect Z | > t   \right] 
\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right),
\end{array}
  \]  
we calculate
\[
  \begin{array}{ll}
 &  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\\
=&  -\frac{1   }{2(\sigma^2/t^2+K(2\expect Z+t/3)/t^2)}\\
\leq &  -\frac{1   }{2(\sigma^2/t^2+K(2+1/3)/t)}\\
 \end{array}
  \]  
% It can be viewed as $ -\frac{1   }{4} $ multiple the harmonic average of 
% $t^2/\sigma^2$ and $t^2/ K(2\expect Z+t/3)$. We find 
Now, we calculate both terms on the denominator,
  \[
  \begin{array}{ll}
   \sigma^2/t^2 &\leq (p  \max_{i=1}^n |\hat{a}_i|^2)/( \sqrt{\frac{p}{2}}  n \| h\|_2)^2 \\
  &\leq 2\max_{i=1}^n |\hat{a}_i|^2)/(\min_{i=1}^n |\hat{a}_i|^2 n^2 \\
   &\leq 2\delta_a^2/ n^2 ,
 \end{array}
  \]  
   \[
  \begin{array}{ll}
  (2+1/3)K/t 
 &\leq  \frac{7}{3}\tau  \| h\|_2 /\sqrt{\frac{p}{2}}  n \| h\|_2\\
  &\leq \frac{7\sqrt{2}}{3}\tau  /\sqrt{p}  n \\
   &\leq \frac{7}{2}\tau  /\sqrt{p}  n 
 \end{array}
  \]  
  
 As we discussed before, since $\tau$ is the maximum of IID Gaussian random variable, 
 $\tau \leq C_1 \log^{1/2}(n)$ with probability $1 - \exp(-C_2 n^2)$ for $C_1$ large enough.
 
And from the assumption we have $ \delta_a \leq C_0 n^{1/2}/ \log^{1/4}(n)$.
  
Therefore, 
\[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7\tau  /\sqrt{p}  n  } \right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-n   }{  \log^{1/2}(n) (4C_0+  C_3 \sqrt{p})} -C_2 n^2 \right)\\
&\leq   \exp\left( \frac{- C n   }{  (p\log(n))^{1/2}}  \right)
 \end{array}
  \]  
  
  

  
  
  
  
  
  
  
  
% Here the two quantity we care are
% \[
% \langle h, h^{(d)}\rangle / \|h\|_2^2
% \]

% \[
%  \|h\|_1 / \|h\|_2
% \]

In the lemma below, we use a covering argument to give a union bound for $v\in B_k=\{v
\in\reals^k\mid \|v\|_2=1\}$. 
We want to cover $B_k$ with $\epsilon$ balls. From classical covering argument,
we know that we need at most $|N| = (3/\epsilon)^k$ $\epsilon$ balls to cover $B_k$, and we use symmetrization trick to find the proper $\epsilon$.

Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
  
Since  $n>  k \log(k/p)$, for large enough constant $C$, we showed in the lemma that there exist a positive constant $C_0$, 
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq  \exp\left(  k\log(3\tau \sqrt{n}np \|a\|_1) - \frac{ C_6 n   }{  (p\log(n))^{1/2}}\right) \\
&\leq    \exp\left( k(\log(3\tau)+\log(\|a\|_1)+\log(p)+3/2 \log(n)) -\frac{ C n   }{  (p\log(n))^{1/2}}\right) 
\end{array}
  \] 
  
% Now we have a tail bound on $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$, which implies a tail bound on 
% $
% \mathcal{X}_v-\mathcal{X}_{v'}$.
%  For all $v, v'\in B_k$,  
%  \[
%   \begin{array}{ll}
% & \prob \left[ |\mathcal{X}_v-\mathcal{X}_{v'}| > \epsilon  \frac{n^{3/2}\sqrt{kp} }{2^{3/2}}    |\bar a| \right] \\
% &\lesssim   \exp\left( Ck\log(\sqrt{n}np \|a\|_1) - \frac{\epsilon^2 \frac{p}{2 }  n^2 \|h\|_2^2 }
% {2pn  (Cn^{1/2}+2k)+2\tau \|h\|_1 \|h\|_2 \sqrt{\frac{p}{2}}  n  (2+\epsilon/3)}\right)
% \end{array}
%   \]  
%  Then we use theorem $19$ of \cite{blasiok2016improved}, we can deduce the tail bound for supremum of $|\mathcal{X}_v|$.
%  \[
%   \begin{array}{ll}
%  \prob \left(\sup_{v \in B_k} |\mathcal{X}_v| > M + \sqrt{t} D_1 + t D_2\right) < e^{-t}
% \end{array}
%   \] 
% Where
% \begin{align*}
% 	M  & := C_1 (\sqrt{2 p}  \gamma_2(B_k, d_2) + \gamma_1(B_k, d_\infty))\\
% 	D_1 & := C_2 \Delta(B_k, \sqrt{2  p} d_2) \\
% 	D_2 & := C_3 \Delta(B_k, d_\infty)
% \end{align*}
% with $d_2, d_\infty$ being the metrics on $\reals^k$ induced by norms $\ell_2, \ell_\infty$ respectively, and $C_1, C_2, C_3$ are universal constants.

Then bound on $\sup_{v \in B_k} |\mathcal{X}_v|$ would imply the same bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$.
And with this bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$, we proved that 
for all $v\neq 0, v \in B_k$, $D>0$ with probability $1-\delta$, where
\[
\delta \leq  \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right)
\]
Therefore, when $n>C_1k^2\log(kp)$, 
$
\delta \leq   \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right),
$
then $\delta$ converges to zero as $k$ goes to infinity.
\end{proof}





\begin{lemma}
Let $Z = \|h*x\|_1$ where $h \in \mathcal{H}$, then 
 \[
  \begin{array}{ll}
& \prob \left[  Z - \expect Z  > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.
\end{lemma}
\begin{proof}
Using duality of $1$-norm, we know that
\[
\|h*x\|_1 = \sup_{\|w\|_\infty\leq 1}\langle w, C(h)x \rangle
\]
 From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
 for the supreme of functions $\langle w, C(h)x \rangle$, since $\expect \langle w, C(h)x \rangle=0$,
 $ \langle w, C(h)x \rangle\leq K$, 
 \[
 \sigma^2 =\expect \langle w, C(h)x \rangle^2,
 \]
 we have
 \[
  \begin{array}{ll}
 \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
\end{proof}
We also remark that the essential concentration inequality that we are trying to derive is the following:
let's consider the case when $x$ is IID standard Gaussian, we define $z = h*x = C(h)x$,
then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,\Sigma(h)),\] where 
\[  \Sigma(h)_{ij} = \langle h^{(i)},  h^{(j)}\rangle\]
And we are trying to derive a concentration inequality for $\|z\|_1$.






\begin{lemma}
For all $v\in B_k$, the probability 
\[
  \begin{array}{ll}
& \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
\leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{lemma}
\begin{proof}
Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{proof}

==> old_sec/sec_old/finite_sample.tex <==
\section{Finite sample analysis}
\paragraph{Finite sample setting}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$ Additionally, in finite sample setting, we assume $a^{-1}$ is zero outside of a centered window of radius $2k+1$, namely, the non-zero part can be written as $(\beta_{-k}, \ldots, \beta_0, \ldots, \beta_k)\in V$. 

We fix the shift and scaling effect by assuming $v^T a^{-1} = 1$ for a generic $v$ that has one single largest entry. 
\item
Let $Y= a* X$ be a linear process, we are given a series of observation $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$.
\item
 We denote $X^{(i)}$ as the sequence being flipped and shifted for $i$ step from $X$ s that $X^{(i)}_k = X_{-k +i}$. Let $J_N$ be the support of $X$.
 We define the length $N=2T+1$ window as $\cT := [-T, T].$
\EIT
Now we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse,
\BEQ
 \begin{array}{ll}
 \underset{w\in V}{  \mbox{minimize} }   & \frac{1}{N}\|w*Y\|_{1,\cT}\\
 \mbox{subject to}  
& v^T w =1.
\end{array}
\tag{$P_{v}^T$}
\EEQ


% Let $C_i(w)$ be $\tilde{w}$ with $i$ step right shift, and define 
% $L_i := |C_i(w)^T Y|$, then 
% \[
% \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]} = \frac{1}{2T+1}\sum_{|i|\in \cT} |[w*Y]_i|  = \frac{1}{2T+1}\sum_{|i|\in \cT} L_i
% \]
% We know that
% \[
% L_i = |C_i(w)^T Y| = |C_i(e_0 +\phi)^T X| = |(e_0 +\phi)^T C_i(X)|
% \]


First, after change of variable,
\[
 \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{N}\|\psi*X\|_{1,\cT}
\]
Then the empirical average can be represented as sum of shifted and flipped inner products.
\[
\frac{1}{N}\|\psi*X\|_{1,\cT}  = \frac{1}{N}\sum_{|i|\in \cT} |[\psi*X]_i| = \frac{1}{N}\sum_{|i|\in \cT}|\psi^T X^{(i)}|
\]
We define 
\[
p_N = \frac{1}{N}\sum_{i\in \cT} I_i
\]
The population average is being calculated,  as
\[
\E  \|\psi*X \|_1:= \E|C_i(\psi)^T X| = \E|\tilde{\psi}^T X|
\]
We know the mean of $p_N$ is $p$, the variance of $p_N$ as
\[
\E[p_N-p]^2=\frac{1}{N}p(1-p)
\]


% \paragraph{Concerntration of finite sample subdifferential}
% Remark:
% From Proposition~$3.5$ (Uniform convergence of subdifferential) in the dictionary learning paper \cite{bai2018subgradient}, we have 
% uniform convergence of subdifferential under Hausdoff distance for all $\psi$ in $2-$norm sphere $S^{n-1}$.


% We want to study 
% \[
% \frac{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}{t} 
% \]

% Notice that
%  \BEAS
%  (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1) = \sqrt{\frac{2}{\pi}} \E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%  \EEAS

% We want to use the empirical formula of sub-gradient:
%  \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}]\\
%   &=& \lim_{t\rightarrow 0^+}\frac{1}{t}[
%   (\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1) 
%   -\sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)\\
%   && + \sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   - (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)]
%  \EEAS
%  and for the second term, diving the constant $\sqrt{\frac{2}{\pi}}$, we have
%   \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{
%  (\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   -\E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%   }]\\
%  &=&  \left(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)-\left(p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)
%  \EEAS
%  If is easy to see that  
% using the fact
% \[
% \E[p_N-p]^2=\frac{1}{N}p(1-p)
% \] 
% we only need to bound
%   \BEAS
%  && (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
%  and we can do further reduction to
%  a bound on 
%   \BEAS
%  && \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]- \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
 
 
 
 \paragraph{Finite sample directional derivative}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (\psi+t\beta)*X \|_1 - \hat{\E}  \| \psi*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{\psi} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}(\psi^T X^{(i)})X^{(i),T}\beta
 \EEAS
Now to study the finite sample convex problem, we need to calculate the directional derivative at $ \psi = e_0$.
Then
\begin{theorem}
For any $X$ sequence with support  $J_N$,
\BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
% \\
%   &=& 
% p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
% (1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
% \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
 
\end{theorem}
\begin{proof}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
 \EEAS
\end{proof}
\begin{coro}
For Gaussian IID sequence $X$, 
 the random variable $ \frac{\|X\|_{1,J_N}}{N} = p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|})$ has mean $p\sqrt{\frac{2}{\pi}}$. 
 And the random expression
\BEAS
& &  \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
\\
  &=& 
p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
 \EEAS
 has mean $\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])$.
\end{coro}
\begin{proof}
 \BEAS
& & 
\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
 \\
  &=& 
p_N ( \frac{\|X\|_{1,J_N}}{|J_N|})\beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
where $p_N = \frac{|J_N|}{N} = \frac{1}{N}\sum_{|i|\in \cT}  1_{X_{-i}\neq 0}$ has mean $p$ and variance $\frac{1}{N} p(1-p)$.
And notice that for the Gaussian IID case 
\[
\E [ p_N\frac{\|X\|_{1,J_N}}{|J_N|}] = \E[p_N|X_{0}|\mid X_{0}\neq 0]  = p\sqrt{\frac{2}{\pi}},
\]
\[
\E [(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N} ] = \sqrt{\frac{2}{\pi}}\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]).
\]
\end{proof}

\begin{coro}
 For symmetric IID sequence $X$, 
  \[
  \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot (\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} ) 
  \]
  where 
  $\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} $ is independent of $X_i$, therefore independent of $(1_{X_{-i}> 0}-1_{X_{-i}< 0}) $.
  Specifically, it has mean $0$
   \[
 \E \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = 0
  \]
  for $q\leq 2$,
    \[
  \frac{1}{N}\E|\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} |^q \leq 
  \frac{1}{N} \E[]|\sum_{i\in J_N}|1_{X_{-i}> 0}-1_{X_{-i}< 0}||^q\cdot  \max_j |X^{(j),T}\beta_{(0)} |^q]
  \]
  
\end{coro}
%   \[
%  p^\star(u):= 
%  \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1 }(-p \cdot \sqrt{1-\| P_{u}^{\perp} P_{e_0}^{\perp} \beta\|_2^2} + (1-p) \cdot  \E_I\| (P_{u}^{\perp} P_{e_0}^{\perp} \beta)_I\|_2 ) > 0\}
%  \]



 \paragraph{Concerntration of $\|\psi*X\|_{1}$ }
The next step is to provide an uniform bound of the finite sample derivation of $\|X\|_{1,J_N}$ and 
$\|X*\beta_{(0)}\|_{1,\cT-J_N}$.

In general, for any random subset $I$ of $\cT$, we study the uniform concentration of 
\[
\|\psi*X\|_{1,I} 
\]
for $\psi = a*w \in a*B_1(V_k),$ by providing moments and tail bound on
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]

For clarity of the argument, we only state the concentration for $\|\psi*X\|_{1,\cT}.$ Also the result about $\cT$ would easy carry to a random subset $I$.

Let the minimal and maximal eigenvalue of the (convolutional) linear operator $a*$ be
\[
\lambda_{m}(a) := \inf_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\[
\lambda_{M}(a) := \sup_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\begin{lemma}
Using circluar embedding of Topelitz matrix, 
\[
\lambda_{M}(a) \leq \max| \hat{a}|
\]
\end{lemma}

Following the idea of lemma~$4$ of the paper of Adamczak on sparse dictionary learning\cite{adamczak2016note} and lemma~$16$ of the paper \cite{spielman2012exact}, we derive a similar bound for convolutional case.
\begin{lemma}
In the following, we define 
\[
Z :=  \frac{1}{N}\|w*a*X\|_{1,\cT}
\]
We find the lower bound of $\E Z$ as a function of the $1-$norm  of $w$:
\[
\E Z  \geq \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1} 
\]
For convenience, we define
\[
\mu_{\mbox{min}}:=\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1}
\]

\end{lemma}
\begin{proof}
WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
\BEAS
\E_X Z 
&=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
&\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
\EEAS
By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
$\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
\BEAS
\E_X Z 
&\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
&\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
&\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
&=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
\EEAS
\end{proof}

% \begin{proof}
% WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
% \BEAS
% \E_X Z 
% &=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
% &\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
% \EEAS
% By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
% then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
% $\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
% \BEAS
% \E_X Z 
% &\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
% &\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
% &\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
% &=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
% \EEAS
% \end{proof}

Now we define the intersection of $1-$norm ball of the $k-$dimensional subspace $V_k$ as $B_1(V_k)$, then we consider $w\in B_1(V_k).$ 
\begin{lemma}
Hence we consider $\psi = a*w \in a*B_1(V_k),$ and we define
\[
W:= \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) |
\]

For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E W^q\leq 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{lemma}

\begin{proof}
Let $\varepsilon_1, \ldots, \varepsilon_N$ be a sequence of IID Rademacher ($\pm 1$)  random variables indepedent of $X$,  By the symmetrization inequality, see e.g. lemma~$6.3$ of book \cite{ledoux2013probability}, we have the first inequality. Then since the function $t \rightarrow |t| $ is a contraction, an application of Talagrand’s contraction principle (see lemma~$8$ of \cite{adamczak2016note}) with $F (x) = |x|^q$ 
conditionally on $X$ gives the second inequality.
\BEAS
\E W^q 
&\leq& 2^q \E \sup_{\psi \in a*B_1(V_k)} 
|\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j |(\psi*X)_{j}| |^q\\
&\leq&
2^{2q}\E \sup_{\psi \in a*B_1(V_k)} |\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j (\psi*X)_{j} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{\psi \in a*B_1(V_k)} |\sum_{i\in [-T,T] }\psi_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{w \in B_1(V_k)} |\sum_{i\in [-T,T] }(w*a)_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&\leq&
2^{2q}\frac{1}{N^q}\E \max_{s\in [k]}|\sum_{i\in [-T,T] }a_{i-s}( \sum_{j\in [-T,T] } \varepsilon_j X_{j-i}) |^q\\
&\leq&
2^{2q}(\frac{\lambda_{M}(a)}{N})^q   \sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q
\EEAS
Now by the moment version of Bernstein’s inequality (see lemma~$7$, equation $(18)$ of\cite{adamczak2016note}), we know that there exists a universal constant $C$,
\BEAS
\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q \leq C^q(\sqrt{Npq}+q)^q
\EEAS
Therefore, 
\BEAS
\E W^q &\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q    
\sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q \\
&\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\EEAS
Then
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
therefore, we could get the tail bound using the Chebyshev inequality for the moments,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np(q+\log(k))}+q +\log(k)))\leq e^{-q}
\EEAS
We set $q = \log(\frac{1}{\delta})$, then we will get an upper bound for $W$ which is satisfied with probability at least $1-\delta$:
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{proof}

\begin{lemma}
Let the condition number of the linear operator $a*$ be
\[
\kappa_a := \frac{\lambda_M(a)}{\lambda_m(a)}.
\]
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
and  $p\geq \frac{1}{N}$, 
then
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{lemma}
\begin{proof}
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
then 
\[
\frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})} \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
additionally, if $p\geq \frac{1}{N}$, 
then a weaker inequality is also true:
\[
\frac{4eC\lambda_{M}(a) }{N}  
 \log(\frac{k}{\delta}) \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
therefore, combining the two parts and the previous inequality,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
we have
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{proof}


\begin{theorem}
Let the solution of finite sample convex optimization be $w^\star$, 
for small $\epsilon>0$ and concentration level $\delta>0$, 
there exists universal constant $C$, if there are 
% \[
% N=2T+1 \geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
% \]
\[
N \geq k\log(\frac{k}{\delta}) ( \frac{C\kappa_a}{\epsilon}  )^2
\]
and  $ \frac{1}{N}\leq p< p^\star(\epsilon)$, we have 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
% Therefore with probability at least $1-\delta$, $a*w^\star =e_0$ and we recover the sparse vector exactly.

% \textbf{ToDO:}
% or
% $\|a*w^\star -e_0\|_1<\epsilon_1$ provided $p< p_N^\star$ for some $p_N^\star\leq p^\star$.
  \end{theorem}
\begin{proof}
From previous lemma, we know that with the conditions, 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
Therefore, with probability at least $1-\delta$,
\BEAS
W = \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) | \leq \epsilon \mu_{\mbox{min}}
\EEAS
When this is true, for all $\psi \in a*B_1(V_k)$, we have a uniform bound 
\[
 \E |(\psi*X)_{j}|-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
\]
\end{proof}
% then
% \[
%  (\E |(\psi*X)_{j}| - \E |X_{j}|)/\| \psi\|_2-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - |(X)_{j}|)/\| \psi\|_2 \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
% \]
% and from previous condition and the expression of directional derivative, 
% \[
% |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | < 2\epsilon
% \]
% If $p<p^\star(u, \epsilon)$, we know from population result that
% \[
% \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
% \]


\begin{coro}
For $\psi = a*w \in a*B_1(V_k),$ 
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]
For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E U_I^q\leq 2^{2q}(\lambda_{M}(a))^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|U_I\|_q \leq 4eC \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( U_I > 4eC\lambda_{M}(a)  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{coro}

% \textbf{ToDO:  Study the finite sample phase transition condition directly} 
\paragraph{Uniform bound of directional derivative}
We  define the uniform bound of directional derivative
\[
W_D  =\sup_{\|\beta\|_2=1, u^T \beta =0, \beta +e_0 \in a*B_1(V_k)}|\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | 
\]
Notice that
\BEAS
& &\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  
\\
&=& 
\left[\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}\right)\right]-
\\
& &
\left[\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])\right]
\EEAS
From previous uniform bound, with high probability, we have the following three uniform bounds on
\[
|\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}|
\]
\[
|(\frac{1}{N} \|X\|_{1,J_N}-\sqrt{\frac{2}{\pi}}p)|
\]
\[
|\frac{1}{N}\|X*\beta_{(0)}\|_{1,\cT-J_N}-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]|
\]
If $p<p^\star(u, \epsilon)$, we know from population result that
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
\]
If with high probability,  
\[
W_D  \leq \epsilon/2
\]
then using the convexity argument, 
for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]
then $a*w^\star-e_0=0$. 
% \paragraph{Uniform bound of finite difference}
% In the end, we define the uniform bound of finite difference, let 
% $t:=\| \psi-e_0\|_2$,
% \BEAS
% W_{D,t}  = \sup_{\psi \in a*B_1(V_k)}
% |\frac{1}{N}\sum_{j\in [-T,T] } ((|(\psi*X)_{j}|-|X_{j}|) - (\E |(\psi*X)_{j}- \E |X_{j}|)|) |/t
% \EEAS
% then from previous lower bound of finite difference by directional derivative, for all $t\in (0,1]$,
% \[
% W_D  = \lim_{t\rightarrow 0}W_{D,t} \leq   W_{D,t}
% \]
% % Using Lipschitz property of finite difference, if directional derivatives are $L-$Lipschitz function, then
% % \[
% % |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = \phi^\star} \rangle   | < L\epsilon_1
% % \]





% % \textbf{ToDO:}
% % Finish the detail proof and find relation of $\epsilon_1$ to other constant!

% \end{proof}

% \paragraph{Concentration tools}
% \begin{lemma}[Gaussian concentration inequality]\label{lem:gaussian_concentration} Let $ x = ( x_1,\ldots,  x_n)$ be a vector of $n$ independent standard normal variables. Let $f: \reals^n\to \reals$ be an $L$-Lipschitz function. Then for all $t>0$,
% \[
% 	\prob{(|f( x) - \E f( x)| \geq t)} \leq 2\exp\left(-\frac{t^2}{2L^2} \right). 
% \]
% \end{lemma}

% \begin{lemma}[Moment control Bernstein inequality for scalar r.v.s]\emph{(\cite{foucart2013mathematical}, Theorem 7.30)}\label{lem:mc_bernstein_scalar}
% Let $  x_1, \dots,   x_n$ be independent real-valued random variables. Suppose that there exist some positive number $R$ and $\sigma^2$ such that $\frac1n\sum_{i=1}^n\expect{  X_i^2}\leq \sigma^2$ and
% \begin{align*}
% \tfrac1n\textstyle\sum_{i=1}^n\expect{\abs{  x_k}^p} \leq \frac{1}{2}\sigma^2 R^{p-2}p!, \; \; \text{for all integers}\; p \ge 3.
% \end{align*}
% Let $S \doteq \sum_{i=1}^n   x_i$, then for all $t > 0$, it holds  that 
% \begin{align}
% \prob{\abs{S - \expect{S}} \ge t} \leq 2\exp\left(-\frac{t^2}{2n\sigma^2 + 2Rt}\right).   
% \end{align}
% \end{lemma}

% \begin{lemma}[$\eps$-net on sphere]\label{lem:epsnet}\emph{\cite{vershynin2010introduction}}  Let $(X, d)$ be a metric space and let $\eps > 0$.
% A subset of $X$ is called an $\eps$-net of $X$ if for every point $x\in X$ there exists some point $y \in  N(x,\eps)$ so that $d(x, y) \leq\eps$. There exists an $\eps$-net for the sphere $ S^{n-1}$ of size
% 	$ (\frac{3}{\epsilon})^n$.
% \end{lemma}


% \begin{lemma}[Young's convolution inequality]
% For 
% $\frac{1}{p} + \frac{1}{q} = \frac{1}{r} +1,$
% \[
% \lVert f*g\rVert_r\le\lVert f\rVert_p\lVert g\rVert_q
% \]
% \end{lemma}




% \paragraph{Finite sample concentration overview}
% We show the concentration in $3$ steps. First, for a fixed direction  $\beta \in V$, we define the event 
% \[
% \mathcal{X}(\psi)  := (|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X| |\geq t) 
% \]
% % notice that
% % where
% % \[
% % \E[|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} \mid I] = \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} 
% % \]
% % and 
% % \[
% % \E|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} = \E\sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} = \E|\tilde{\psi}^T X| = 
% % \]
% here we can break it into $2$ terms:
% \[
% |\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} |\geq t_1 
% \]

% \[
% | \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} -\sqrt{\frac{\pi}{2}} \E_I \|\psi_{I}\|_{2,[-T,T]} |\geq t_2 
% \]

% and we bound the tail probability 
% \[
% P(\mathcal{X}(\psi) ) = P(|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X|   | \geq t) 
% \]
% Second, we find the Lipschitz constant $L$ of the mapping  $\psi \rightarrow \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]},$ and we replace point event $\mathcal{X}(\psi)$ with a $\epsilon-$ball event 
% $\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi')$ with $\epsilon = \frac{1}{L}.$

% Third, we use $\epsilon-$net to cover the entire $k$-dimensional  space with $k+1$ is the length allowed for the approximate inverse filter $w$ ($w$ is in a $k$-dimensional vector space $V_k$), since the forward filter $a$ is fixed, $\psi = a*w$ is also in a $k$-dimensional vector space $a*V_k$.
% Therefore, 
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]

% \paragraph{Concentration inequality}
% Let $C(\psi)$ be the circulant matrix spanned by the flipped version of $\psi$ as the first column vector.

% Using duality of $1$-norm, we know that
% \[
%  \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} =  \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]} 
% \]

% The Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_x =\sup_{\|b\|_\infty\leq 1}  \|C(\psi)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(\psi) )
%  \]
 
%  On the other hand, $\psi = w*a,$
%  the Lipschitz constant of the mapping $w \rightarrow \frac{1}{2T+1}E_X\sup_{\|b\|_\infty\leq 1}\langle C(w) C(a) b , X\rangle_{[-T,T]}$ is 
%   \[
%  L_w =\sup_{\|b\|_\infty\leq 1}  \|C(a)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(a) )= \|\hat{a}\|_\infty
%  \]

% \begin{lemma}
% From theorem~$8$ of paper \cite{van2013bernstein}, the Bernoulli Gaussian random variable  have sub-exponential tails, and satisfy Bernstein condition with $K =2$.

% Let $Z =\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]}  $, then $\E Z =  \E|\tilde{\psi}^T X|\leq \sqrt{p}\|\psi\|_2$,
%  \[
%   \begin{array}{ll}
% & \prob \left[  Z - \expect Z  > t   \right] \\
% &\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)\\
% &\leq \exp\left(  \frac{-t^2/2   }{\frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 +2(2\sqrt{p}\|\psi\|_2+t/3)}\right)
% \end{array}
%   \]  
% where $\sigma^2=  \expect Z^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 $.
% \end{lemma}

% \begin{proof}
% % Let $\hat{p} := \frac{1}{2T+1}\sum_{|i|\in \cT} 1_{X_i \neq 0}$
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  = 
% % \hat{p} \beta_0 +(1-\hat{p}) \hat{\E}\|\beta * X_{{(0)}}\|_1 
% % \]



% % \[
% %   \| (e_0+t\beta)*X \|_1   = \hat{\E}\sup_{\|b\|_\infty\leq 1}\langle b*(e_0+t\beta) , X\rangle
% % \]
%  From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
%  for the supreme of functions $\langle b*(e_0+t\beta) , X\rangle$, since $\expect \langle b*(e_0+t\beta) , X\rangle=0$,
%  $ \langle b*(e_0+t\beta) , X\rangle\leq K$, 
%  \[
%  \sigma^2 =\expect \frac{1}{(2T+1)^2}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]}^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 
%  \]
%  we have
%  \[
%   \begin{array}{ll}
%  \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
% \end{array}
%   \]  
% \end{proof}
% We also remark that the essential concentration inequality that we are trying to derive is the following:
% let's consider the case when $x$ is IID standard Gaussian, we define $z = \psi*x = C(\psi)^T x$,
% then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,C(\psi) C(\psi)^T),\] where 
% \[  (C(\psi) C(\psi)^T)_{ij} = \langle \psi^{(i)},  \psi^{(j)}\rangle\]
% And we are trying to derive a concentration inequality for $\|z\|_1$.

% \begin{lemma}
% Since $\forall w \in V_k, \|w\|_\infty \leq 1 $, 
% from Young's convolution inequality,
% \[
% \|a*w\|_2 \leq \|w\|_\infty \|a\|_{\frac{2}{3}} = \|a\|_{\frac{2}{3}}
% \]
% and 
% \[
% \| \tilde{a}*a*\tilde{w}*w \|_1\leq \|w\|_\infty^2 \| \tilde{a}*a \|_{\frac{1}{3}} = \| \tilde{a}*a \|_{\frac{1}{3}}
% \]
% \end{lemma}

% \begin{theorem}[Uniform convergence from covering]
% Let $\epsilon:= \frac{1}{L_w},$  then from the $\epsilon-$net covering lemma,
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]
% Here the Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_w
%  = \| \hat{a}\|_\infty
%  \]
%  here $\| \hat{a}\|_\infty$ is the infinity norm (max absolute value of entries) of the Fourier transform of $a$,
%  then
% \BEAS
% &&\prob \left[  Z - \expect Z  > t ,\forall w \in V_k, \|w\|_\infty \leq 1 \right]
% \\
% &=& P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) \\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a*\tilde{w}*w \|_1 p +2(2\sqrt{p}\|a*w\|_2+t/3)}\right)\\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a \|_{\frac{1}{3}} p +2(2\sqrt{p}\|a\|_{\frac{2}{3}}+t/3)}\right)
% \EEAS
% \end{theorem}
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           

% % \begin{lemma}
% % For all $v\in B_k$, the probability 
% % \[
% %   \begin{array}{ll}
% % & \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
% % \leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{lemma}
% % \begin{proof}
% % Let the deviation be
% % \[
% % \tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
% % \]  
% % We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% % % The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

% % We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
% % \[
% % \mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
% % \]  
% %  then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
% %  \[
% %  \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
% %  \]
% %  This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
% % Since  
% % \[
% % \mathcal{X}_v-\mathcal{X}_{v'} =  
% % \sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
% % \]

% % Then use the fact that 
% % \[
% % | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
% % \]
% % and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
% % $s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
% % $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
% % we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

% % From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
% %  \[
% %   \begin{array}{ll}
% % \sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
% % &\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
% % &\leq  \tau \sqrt{n}np \|a\|_1
% % \end{array}
% %   \]  
  
% % Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
% % at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
% % We have a concentration inequality in each ball,
% % We define the tail event 
% % \[
% % \mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
% % \]
% % we can take a union bound,
% %  \[
% %   \begin{array}{ll}
% %  \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
% % &\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{proof}

% % Second, we show that 
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle 
% % \]
% % is locally Lipschitz 
% % % The (set valued) sub-gradient at zero is
% % % \[
% % %   \nabla{L_i} =   \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X),
% % % \]
% % % the directional derivative at zero is
% % % \[
% % %   \nabla_{\phi}{L} = \phi^T \nabla{L_i} =  \mbox{sign}((e_0 +\phi)^T C_i(X))  (\phi^T C_i(X)) ,
% % %   \]
% % % the (set valued) Riemannian subdifferential at zero on the hyperplane defined by $u^T \phi = 0$ is given by
% % % \[
% % %   P_u \nabla{L_i} = (I- uu^T)  \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X) 
% % % \]




% % %  \BEQ
% % %   \begin{array}{ll}
% % %   \expect \nabla{L_i}  &=  p\expect[\nabla{L_i} \mid X_i \neq 0 ] + (1-p)\expect[\nabla{L_i} \mid X_i = 0 ] \\
% % %   &=  p\expect[ \mbox{sign}(X_i) C_i(X)\mid X_i \neq 0 ] + (1-p)\expect[ \mbox{sign}((\phi_{(i)})^T C_i(X)_{(i)}) C_i(X)_{(i)}\mid X_i = 0 ] 
% % %   \end{array}
% % %  \EEQ  



==> old_sec/sec_old/inequal.tex <==
\subsection{$E{| \psi^T X| }$ for IID Bernoulli Gaussian $X$ }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ are unit variance,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \|a\|_2^2.
\]
The ratio indicate the sparsity level of random variable $Z = \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\|a\|_2} 
\]
Now, we consider some settings where exact calculation of $E{|\sum_{i} \psi_i X_i| }$ are possible.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i G_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $G_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
E_X{|\sum_{i} \psi_i X_i| }  
= E_B E_G {|\sum_{i} \psi_i B_i G_i| }
= E_I E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]
then
\[
E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot E_I \|\psi_I\|_2
= \sqrt{\frac{2}{\pi}} \cdot (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2.
\]
Here the last equality use the lemma below, and we define that $\|a\|_0= \#\{ t : \psi_t \neq 0\}$.
\begin{lemma} (Expectation of $2-$norm over Bernoulli support)
\label{lem:BLemma}
\BEQ
E_I \|\psi_I\|_2 = (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2
\EEQ
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:BLemma}]
We have the power series representation $\sqrt{x} = \sum_k c_k x^k$ valid on $(1/A,A)$
for large $A \gg 1$. 
Let $N = |\cT|$. Fix $A > 1/\eps^2$; then every sum $ \sum_{t \in I} \psi_t^2 \in (1/A,A)$;
using this:
\begin{eqnarray*}
 \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  &=&  
 \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \cdot ( \sum_{t \in I} \psi_t^2  )^k \\
 &=& \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&   \sum_k  c_k \sum_{I \subset \cT} \pi(I)   \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 \end{eqnarray*}
 Hence from $ \pi(I) = (p)^{|I|} (1-p)^{|\cT \Delta I|}$
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \sum_{n=1}^{N}  \sum_{|I| = n} (p)^n (1-p)^{N-n}  \cdot  \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  %\\
 \end{eqnarray*}
 Since the inner two sums  cover $ {N \choose n} n^k$ terms in a uniform way,
 we can write
% \clearpage
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \cdot \left( \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n} \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 \end{eqnarray*}
Now use the identity $1 = \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}$  for the complete binomial sum, 
hence the incomplete sum $\sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}= 1-(1-p)^N$. We get
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \cdot \left( 1-(1-p)^N \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 &=& \left( 1-(1-p)^N \right) \cdot \sum_k c_k  \left ( \sum_{t \in \cT} \psi_t^2  \right )^k \\
 &=&  \left( 1-(1-p)^N \right) \cdot  \sqrt{\sum_{t \in \cT} \psi_t^2 } .
\end{eqnarray*}
\end{proof}

==> old_sec/sec_old_2020/Discrete_structure.tex <==

\section{Discrete signal structure}
\paragraph{Random model for discrete digital signals.}
We define a random model for discrete digital signals. 

Let $(X_t)$ be an independent
sequence of random variable indexed by  $t \in Z$, with a symmetric distribution with CDF $F$. 
\begin{itemize}
\item The two point symmetric distribution on real number, $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$ 
\item The four point symmetric distribution on complex number, 
$F = 1/4 \delta_{1+i} + 1/4 \delta_{-1+i}+1/4 \delta_{1-i}
+1/4 \delta_{-1-i}.$ 
\item A symmetric distribution on $\reals^s$,
$F = 1/2^s( \sum_{c\in \{\pm 1\}^s} \delta_{\sum_{i\in[s]} c_i e_i } ).$ 

\item Constallantion in unit sphere.
The $2k$ point symmetric distribution on complex number, 
$F_p = \sum_{j=0}^{2k-1} p_j \delta_{\exp{(i\pi\frac{j}{k})}},$
where $\sum_{j=0}^{2k-1} p_j =1, p_j>0.$
\end{itemize}



\paragraph{Convex loss for discrete digital structure.}
The convex loss  we choose could be a relaxation of the convex indictor function of the points.

\begin{itemize}
\item For the two point symmetric distribution on real number, 
\[
g(x) = (|x|-1)_+
\]
\item The four point symmetric distribution on complex number, 
\[
g(z) = (|z|-1)_+,
\]
or more accurately,
\[
g(z) = (\|z\|_{\infty}-1)_+.
\]
\item For $s$-dimensional symmetric distribution on $\{\pm 1\}^s$,
\[
g(x) = (\|x\|_{\infty}-1)_+.
\] 
\end{itemize}


\paragraph{Blind recovery problem.}
For observation $Y$, assume that there exist inverse filter $\mu^* (e_0 + f^*)$, where $f^*_0 = 0$. We try to find it by solving a convex problem,
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E \sum g(\mu (Y+ f*Y)).
\end{eqnarray*}
First, when we know the correct scale $\mu^*$.

Let 
\[
e_0+h = ( e_0 + f)(e_0 + f^*)^{-1},
\]
we have
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E g( x_0+ h*x)).
\end{eqnarray*}
For $g(x) =(|x|-1)_+$, then the sub-gradient is
\[
g'(x) =  \left.
  \begin{cases}
    1, & \text{for } x > 1 \\
    0, & \text{for } -1 < x < 1 \\
    -1, & \text{for }-1 > x \\
    [0,1], & \text{for }x = 1  \\
    [-1,0], & \text{for }x = -1
  \end{cases}
  \right\}
\]

And the proximal operator $\mbox{prox}_{\rho g}$ is
\[
\mbox{prox}_{\rho g}(x) =  \left.
  \begin{cases}
    x-\rho, & \text{for } x > 1+\rho \\
    x, & \text{for } -1 < x < 1 \\
    x+\rho, & \text{for }-1-\rho > x \\
    1, & \text{for }1 \leq x \leq 1 +\rho \\
    -1, & \text{for } -1 -\rho\leq x \leq -1
  \end{cases}
  \right\}
\]


Assume $(X_t)$ are independent
sequence of random variable with CDF $F_{p}^t = \sum_{j=0}^{1} p^t_j \delta_{(-1)^j},$
where $\sum_{j=0}^{1} p^t_j =1, p^t_j>0.$ We choose the objective
\[
g(z) = (|z|-1)_+.
\] 
To show that $h=0$ is the global minimizer of the convex problem, we only need to show that for any $h\neq 0$, there exists small $\epsilon>0$, 
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)>0.
\end{eqnarray*}
We use sub-gradient information,
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)
    &\approx& 
    E g'( x_0)(\epsilon h*x)\\
    &=&
    \epsilon( p^0 _1 g'( +1)(h_0)+p^0_{-1}g'( -1)(-h_0)  )
    \geq 0.
\end{eqnarray*}

\paragraph{Polar form and extension to complex plane}
We can rewrite a point on the complex plane as its polar form
\[
z = r \exp{i\theta},
\]
where $r\geq 0$.

Under the polar form, the loss function is 
\[
g(z) = (|z|-1)_+ = (r-1)_+,
\]

We can reparametrize

Using this polar form, we are able to generalize our result to the complex setting.

\paragraph{Non-convex loss for discrete digital structure.}
If we are allowed to use non-convex loss, then we can fix the scale by the loss function.

Instead of convex loss
\[
g(x) = (|x|-1)_+,
\]
or
\[
g(x) = (|x|^2-1)_+,
\]
we can choose
\begin{itemize}
\item The smooth loss 
\[
g(x) = (|x|^2-1)^2,
\]
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (|x|-1)^2,
\]
\item The composition of  smooth function with convex non-smooth function,
\[
g(x) = ||x|^2-1|,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = ||x|-1|.
\]
\end{itemize}


And instead of
\[
g(x) = (\|x\|_{\infty}-1)_+,
\]
we can choose
\begin{itemize}
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (\|x\|_{\infty}-1)^2,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = |\|x\|_{\infty}-1|.
\]
\end{itemize}

\subsection{Noisy observation}
We consider the noisy recovery problem, there are two noise model, one is
\[
y = w_0 * (x+  n),
\]
the other is 
\[
y = w_0 * x+  u = w_0 * (x+ w_0^{-1} *u).
\]
When $u$ is Gaussian $N(0,\Sigma) $ , $w_0^{-1} *u$ is Gaussian $N(0,C_{w_0}^{-1}\Sigma C_{w_0}^{-1,T}) $. Therefore, we could reduce this problem as a colored noise $n$. 

\paragraph{Post-process}
For noisy observation $y$, we apply the algorithm on $y$ to get a solution $\hat x$, then we apply our prior knowledge to project the solution to the constellation points by taking $\title{x} = \mbox{sign}(\hat x).$

Then we measure the ratio of correct recovery by mean of
$1_{\title{x} = x}$ over multiple MC samples.
\paragraph{Population analysis}
Assume that the observation model are $y = w_0 * (x+  \sigma n),$ where $n$ is IID $N(0,1)$. Then we analyze the population risk,
 \begin{eqnarray*}
    \min_{h_0 = 0} &    
     E_x E_n g( x_0+ \sigma n_0+ h^T (x+\sigma n) ).
\end{eqnarray*}
Here $g(x) =(|x|-1)_+$.

Assume that the optimal solution is $h^*_\sigma$, when $\sigma = 0$ we proved before that $h^*=0.$ Here we get
$\hat x_0 = x_0+ \sigma n_0+ h^{*,T} (x+\sigma n) $
want to prove
\[
\tilde x_0 = \mbox{sign}(x_0+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n) ) = x_0,
\]
when $\sigma<\sigma_{m}$.
Without loss of generality, we assume $x_0=1$, we want to ask that when would $1+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n)\leq 0$, in general, the condition we need to charaterize is when 
$ |\sigma n_0+ h_\sigma^{*,T} (x+\sigma n)|\leq 1$.

\paragraph{Huber version of loss}
Instead of using $g(x) =(|x|-1)_+$, when there are Gaussian noise on $x$, we can use the Huber version 
\[
g_{\mu}(x) =\min_z  \frac{\mu}{2}\|x-z\|^2_2+ (|z|-1)_+  .
\]
% \section{Numerical results}
% \subsection{Convex loss}
% For observation $Y\in \reals^{2N+1}$,  assume that there exist inverse filter $w^* = \mu^* (e_0 + f^*)$, where $f^*_0 = 0$, such that $w^* *Y=X$ is IID distributed by $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$  Let
% \[
% g(x) = (\|x\|_{\infty}-1)_+,
% \]
% we try to find it by solving a convex problem,
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2k+1}} &    
%      \sum g(\mu (Y+ f*Y)).
% \end{eqnarray*}
% And we also solve 
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2N+1}} &    
%      \sum g(\mu (Y+ f*Y))+\lambda \|f\|_1.
% \end{eqnarray*}

% In the following, we assume $\mu^* =1$ WOLG.

% We select $\mu$ in algorithmically by a line search over different choices.

% And the criteria to select is to look at the non-convex loss, say 
% \[
% h(x) = ||x|^2-1|^2,
% \]
% or its gradient. When $g$ or $g'$ is zero, then we know we selected the right scale.

% % \begin{algorithm}
% %   \caption{\textbf{Deconvolution t}}
% %   \label{alg:AA}
% % \begin{algorithmic}[1]
% %   \State {\bfseries Input:} initial point $x_0$, operator $F(\cdot)$, memory $m$
% %   \For{$k=1, 2, \dots$}
% %   \State $m_k=\min\{m, k\}$
% %   \State $\alpha^k$ determined by either the type $1$ or the type $2$ formula above.
% %   \State $x_{k+1} =   \alpha^{k,T}(X^k - \beta_k G_{k})$.
% %   \EndFor
% % \end{algorithmic}
% % \end{algorithm}

% Here is the matlab code,
% \begin{verbatim}
% % % Param
% T = 100;
% n_left = T;
% n_right = T;
% lam = 1e1;
% mu = 1e2;
% k_0 = 10;
% k_1 = 10; 
% k_2 = 100; 
% k_4 = 10;

% scale = 1.;
% % MAX_ITER = 1e1;
% % STEP_SIZE = 1e-4;
% % STEP_MIN = 1e-5;
% % GRAD_TOL = 1e-8;
% % mem_size= 10;
% % beta = 0.5;
% % EPS = 1e-2?;

% % % Set up
% n = n_left+n_right+1;
% delta = [zeros(n_left,1);1; zeros(n_right,1)];

% % % % Model
% % Create x

% % x0 = x0.*randn(n, 1);
% x0 = sign(randn(n, 1));
% % x0_mat = circulant(x0,1);
% J_1 = (x0 > 0);
% J_2 = (x0 < 0);



% % Create forward and inverse filter
% % inverse
% t = 0.1;
% w0_left =[t];
% for j=2:1:k_0
%     w0_left(j,1) =t^j;
% end
% % p1= 0.4;
% % w0_left = t*(rand(k_0, 1) < p1);

% w0 = [zeros(k_0,1);1; -w0_left ];
% w_pad =  [zeros(n_left-k_0,1); w0 ; zeros(n_right-k_0,1)];
% J_w = (max(1,n_left-2*k_0-2):min(2*T,n_left+2*k_0+2));
% % forward
% a0 = ifft(1./fft(w_pad,n),n);
% a_shift = circshift(a0,T);

% % % Property
% % Cos
% cos = norm(w_pad ,inf)/norm(w_pad ,2);
% % Correlation
% w0_mat =  circulant(w0,1);
% w_flip = w0_mat(1,:)';
% R_w = conv(w0, w_flip);

% % Y observation
% y = cconv(a0, x0, n); 
% y_mat =  circulant(y,1);



% cost = @(z) sum(((z).^2-1).^2); 
% grad = @(z) 2*sum(((z).^2-1).*(2*z)); 


% % % % Algorithm compare

% % % Algorithm1
% % %	Exact problem
% % 

% y_mtruc = y_mat(1:n,1:2*k_1+1);
% cvx_begin quiet
% cvx_solver mosek
%   variable w_1(2*k_1+1),
%   minimize( sum(pos(abs(scale*y_mtruc*w_1)-1)))
%   subject to
%       w_1(1+k_1) ==1
% cvx_end

% w_1pad = [zeros(n_left-k_1,1);w_1; zeros( n_right-k_1,1)];
% x_1 = cconv(w_1pad, y, n); 
% delta_1 = cconv(w_1pad,a_shift,n);
% c1 = cost(x_1);
% g1 = grad(x_1);
% % % Algorithm2
% % %	Regularized problem

% y_mtruc2 = y_mat(1:n,1:2*k_2+1);

% cvx_begin quiet
% cvx_solver mosek
%   variable w_2(2*k_2+1),
%   minimize(  sum(pos(abs(scale*y_mtruc2*w_2)-1))+lam* norm(w_2,1))
%   subject to
%       w_2(1+k_2) ==1
% cvx_end

% w_2pad = [zeros(n_left-k_2,1);w_2; zeros( n_right-k_2,1)];
% x_2 = cconv(w_2pad, y, n); 
% delta_2 = cconv(w_2pad,a_shift,n);
% c2 = cost(x_2);
% g2 = grad(x_2);
% \end{verbatim}


==> old_sec/sec_old_2020/Expectation.tex <==
\section{Expectation calculation}
\subsection{Expectation over Bernoulli support}

We previously considered the identity
\beq \label{eq:startingPoint}
    \E | \sum_{i \in \cT}  \psi_i X_i | = \sqrt{\frac{2}{\pi}} \cdot \E_I \| \psi \|_{\ell_2(I)},
\eeq
where $X$ is a Bernoulli-Gaussian RV $BG(p;0,1)$,
and where $I$ is a random subset of the domain $\cT$
determined by Bernoulli-$p$ coin tossing.

% (Qingyun:)
% First of all, we know that 
% \[
% \E_I \| \psi \|^{s}_{\ell_2(I)} \leq \| \psi \|^s_{\ell_2(T)}
% \]
% for any $s \in \integers$.

% Because $$


This leads us to consider
\[
  \E_I \| \psi \|_{\ell_2(I)}^{2k}
 \]
 where $I$ is again a random subset, and $k \geq 1$ is an integer.
 The following lemma shows that $\E_I \| \psi \|_{\ell_2(I)}^{2k} \approx \| \psi \|_{\ell_2(\cT)}^{2k}$.

\begin{lemma} \label{lem:BGPropLemmaSub}
Let $\psi$ denote a vector in $\reals^N$.
\[
 \| \psi\|_2^{2k} \cdot \bar{B}(k-1;n,p)    \leq \E_I  \| \psi \|_{\ell_2(I)}^{2k}  \leq     \| \psi\|_2^{2k} ,
\]
where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
is the survivor function (Complementary CDF) of the Binomial.
\end{lemma}

In particular, if $k \leq n \cdot p - 3 \cdot \sqrt{np (1-p)}$ for large $n$, then $\bar{B}(k-1;n,p) > 0.99$.
 The following lemma infers from this that $\E_I \| \psi \|_{\ell_2(I)} \approx \| \psi \|_{\ell_2(\cT)}$.
 
\begin{lemma} \label{lem:BGPropLemmaNorm}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$ as $\eps_N$ could be quite large!}


There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
and so that for each $N$ and for each 
vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
\beq \label{eq:LemmConclu}
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\eeq
\end{lemma}
Applying (\ref{eq:startingPoint}), we get:
\begin{coro} \label{lem:BGPropLemma}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$!}
There exists a sequence $(\eps_N)$ depending only on $N$, so that  $\eps_N \goto 0$ and
and so that for each $N$ and for each 
vector $\psi$in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$.
\[
(1 - \eps_N) \cdot (1-N^{-1}) \leq  \frac{E | \sum_{i \in \cT}  \psi_i X_i |}{\sqrt{\frac{2}{\pi}}  \| \psi \|_{\ell_2(\cT)}}  \leq   ( 1 + \eps_N).
\]
% and
% \[
% E | \sum_{i \in \cT}  \psi_i X_i |  \geq  (1 - \eps_N) \cdot (1-N^{-1}) \cdot \sqrt{\frac{2}{\pi}} \cdot E \| \psi \|_{\ell_2(\cT)} .
% \]
\end{coro}


\subsection{Proof of Lemma \ref{lem:BGPropLemmaSub}}

\begin{proof}[Proof of Lemma \ref{lem:BGPropLemmaSub}]
Let's first suppose that $|\psi_t| \geq \eps > 0$ for $-T \leq t \leq T$. Let $N = 2T+1$, and
let $I$ denote a subset of indices in $ \cT = \{-T,\dots,T\}$ and
let $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|}$. 
\begin{eqnarray*}
\E_I  \| \psi \|_{\ell_2(I)}^{2k}  &=&  \sum_{n=1}^{N}  \sum_{ |I |=n} \pi(I)   \| \psi \|_{\ell_2(I)}^{2k} \\
% &=& 
%   \sum_{I \subset \cT} \pi(I)    \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&   \sum_{n=1}^{N}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k}  \\
   \end{eqnarray*}
where we used $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|} $.
We partition the sum  $\sum_{n=1}^{N} = \sum_{n=1}^{k-1} + \sum_{k}^N =  \sum_{n<k} + \sum_{n\geq k}$, say.
Now from $\#\{ |I|\leq n\} = {N \choose n}$ and $ \| \psi \|_{\ell_2(I)} \leq \| \psi \|_{\ell_2(\cT)}$,
\begin{eqnarray*}
 \sum_{n<k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
     &\leq&   \left( \sum_{n=1}^{k-1} (1-p)^n p^{N-n} {N \choose n} \right) \cdot  \left( \| \psi \|_{\ell_2}^{2k} \right) \\
     &=& B(k-1;n,p) \cdot   \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
where $B(x;n,p)$ denotes the cumulative distribution function of the binomial distribution.
For the sum $\sum_{n\geq k}$, we may write $\sum_{|I|=n} = {N \choose n}  \cdot Ave_{|I| = n}$
and $\sum_{t_1,\dots, t_k \in I} =  {n^k} \cdot  Ave_{t_1,\dots, t_k \in I}$, so
\begin{eqnarray*}
 \sum_{|I| = n}  \| \psi \|_{\ell_2(I)}^{2k} &=& \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2 \\
& =& {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2 \\
&=& {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot \sum_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot  \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
because the inner two averages  cover the $ {N \choose n} n^k$ terms in a uniform way.
We arrive at 
% \clearpage
 \begin{eqnarray*}
 \sum_{n\geq k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
  &=&     \| \psi \|_{\ell_2}^{2k} \cdot  \left( \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} \right) \\
  &=&    \| \psi \|_{\ell_2}^{2k} \cdot \bar{B}(k-1;n,p) .
 \end{eqnarray*} 
Here $\bar{B}(x;n,p) = 1- B(x;n,p)$ denotes the 
survivor function (complementary distribution function) of the binomial distribution.
We obtain:
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  
  & = &  \left( \sum_{n \geq k} + \sum_{n<k}   \right) \sum_{|I|=n}  \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k} \\
 &\leq &    \|\psi\|_2^{2k} \cdot  \left( \bar{B}(k-1;p,n)  + B(k-1;p,n) \right) \\
 & = &  \|\psi\|_2^{2k} .
 \end{eqnarray*}
 while
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}   & \geq & \sum_{n \geq k} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  \\
 &= &    \|\psi\|_2^{2k} \cdot \bar{B}(k-1;p,n) .
  \end{eqnarray*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:BGPropLemmaNorm}}

\begin{proof}
Fix $A > 0$ and $p \in (0,1)$
By the Weierstrass approximation theorem, we may find a sequence of polynomials $S_K(t) = \sum_{k=0}^{K} c_k t^k$
so that
\[
    | \sqrt{x} - S_K(x) |_{L^\infty([0,A])} \leq \eps_K, \quad \mbox { and } \eps_K \goto 0 \mbox{ as } K \goto \infty.
\]
Pick a sequence $(K_N)$ so that $K_N \goto \infty$ while
$K_N < N \cdot p -  \sqrt{2 \log(N) \sqrt{N} p (1-p)} $ and
\[
\bar{B}(K_N-1; n,p) > 1 - N^{-1}.
\]
Relabel $S_N  \equiv S_{K_N}$ and $\eps_N \equiv \eps_{K_N} $.
Then $\eps_N \goto 0$ as $N \goto \infty$.

Fix $N$. For each $I \subset \cT$,
let  $x_I \equiv \E_I \| \psi \|_{\ell_2(I)}^{2}$.  Then
\[
     E _I \| \psi \|_{\ell_2(I)} = \E_I \sqrt{\| \psi \|_{\ell_2(I)}^2} = \E_I \sqrt{ x_I }.
\]
while
\[
     E _I \| \psi \|_{\ell_2(I)}^{2k} = \E_I  x_I^k.
\]
Invoking our earlier lemma,
\[
 \bar{B}(k-1;n,p) \leq  \frac{\E_I  x_I^k}{\| \psi \|_{\ell_2(\cT)}^{2k}} \leq 1.
\]

Armed with  polynomial $S_N$ of degree $K_N$, consider
\begin{eqnarray*}
     \E_I S_{N}( x_I ) &=& \E_I \sum_{k=1}^{K_N} c_k x_I^{k}\\
     &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\leq& \sum_{k=1}^{K_N} c_k   \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& S_{N}( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\leq& ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} + \eps_{N} . 
\end{eqnarray*}
where we used $\E_I x_I^{k} \leq  \| \psi \|_{\ell_2(\cT)}^{2k}$ from the previous Lemma.
Similarly,
\begin{eqnarray*}
     \E_I S_N( x_I )   &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\geq& \sum_{k=1}^{K_N} c_k   \cdot \bar{B}(k-1; n,p) \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &\geq& \bar{B}(K_N-1; n,p) \cdot \sum_{k=1}^{K} c_k   \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& \bar{B}(K_N-1; n,p)  \cdot S_K( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\geq&  \bar{B}(K_N-1; n,p)  \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  \\
   &\geq&  (1- N^{-1}) \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  . 
\end{eqnarray*}
Here  we used $\E_I x_I^{k} \geq  \| \psi \|_{\ell_2(\cT)}^{2k} \cdot \bar{B}(k-1;n,p)$ from the previous Lemma.
We also used the monotonicity 
of the survivor function $\bar{B}(x) \geq \bar{B}(x+1)$.
We obtain (\ref{eq:LemmConclu}):
\[
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\]
\end{proof}


We define the functional  $\Gamma: \psi  \mapsto \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$,
from the previous calculation we know $\Gamma(\psi) $ is only a function of $\| \psi\|_0$. 
So we can identify  $\Gamma(\psi) $ as  $\Gamma(\| \psi\|_0)$. 





\subsection{Sharper bounds on $\frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$}




\begin{lemma}
\label{TaylorSqrt}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{1/2}
=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{1/2}
=\sum_{\ell=0}^\infty\binom{1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{1/2}{\ell}
&=\frac{\frac12(\frac12-1)(\frac12-2)\cdots(\frac12-\ell+1)}{\ell!}\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-3)\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}\frac{(2\ell-2)!}{2^{\ell-1}(\ell-1)!}\\
&=\frac{(-1)^{\ell-1}}{\ell2^{2\ell-1}}\binom{2\ell-2}{\ell-1}
\end{align}
then
\begin{align}
(1-x)^{1/2}
&=1-\sum_{\ell=1}^\infty\frac2\ell\binom{2\ell-2}{\ell-1}\left(\frac x4\right)^\ell\\
&=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}





% leveraging the 
%  Taylor series of $\sqrt{x}$ around any $a>0$:
%  \[
%  \sqrt{x} = \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {{a}^{\frac{1}{2}-n} \left( x-a\right)^{n}}{\Gamma\left( \frac{3}{2}-n \right)n! }}.
%  \]
%  We could apply the  Taylor series expansion around $1$ to  $\frac{ \| \psi \|_{\ell_2(I)}}{\| \psi \|_{\ell_2(T)}}$,
%  \begin{eqnarray*}
%   \sqrt{\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}} 
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}-1\right)^{n}\\
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \sum_{i=0}^n 
%  {n \choose i} (\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}})^i (-1)^{n-i}\right)
%  \end{eqnarray*}

\end{proof}

\begin{lemma}
\beq 
0 \leq 1- Q(N, p)\leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 .
\eeq
where 
\[
Q(N, p) := \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p),
\]
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|_{\ell_2(J)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(J)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq 1 .
\eeq
Therefore, 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ \frac{ \| \psi \|^2_{\ell_2(I)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq \E_I 1 = 1 .
\eeq

On the other hand, let 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}}}  .
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.

Applying Lemma \ref{TaylorSqrt},
\begin{align}
(1-\rho_J)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\rho_J^{\ell+1}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_I)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell;n,1-p)    \leq \E_I \rho_I^{\ell+1} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}\\
&\geq  1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1- \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
&= 1- Q(N, p)
\end{align}
% {\bf NOTE: I am not getting the inequality $Q(N,P) \leq N^{-1}$.
% See Below.}
{\bf Qingyun NOTE: I observe numerically that $Q(N,p)$ could be between $0$ and $1$ in a wide range, and $Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$, with $Q(N,1) = 0$, $\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$
.}
\end{proof}

\paragraph{Beta function and $Q(N,p)$}
If we define the complete beta function as 
\[
\Beta(a,b) := \int_0^1 t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then
% \[
% \Beta(x,y)=\frac{\Gamma(x)\,\Gamma(y)}{\Gamma(x+y)}
% \]
% therefore,
\[
\binom{n}{k} = \frac{1}{(n+1) \Beta(n-k+1, k+1)}
\]
the incomplete beta function as
\[
\Beta(x;\,a,b) = \int_0^x t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then the regularized incomplete beta function is defined in terms of the incomplete beta function and the complete beta function:
\[
I_x(a,b) = \frac{\Beta(x;\,a,b)}{\Beta(a,b)}.
\]
then
\[
I_p(k,N-k-1)= \bar{B}(k-1;N,p) = \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}
\]
and
\[
I_{1-p}(k+1, N-k) = 1 - I_p(N-k, k+1) = \bar{B}(k;N,1-p).
\]
Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$, from the classical De Moivre–Laplace theorem on normal approximation to the binomial, 
\[
{N \choose k}\, p^k q^{N-k} \approx \frac{1}{\sqrt{2 \pi Np(1-p)}}\,e^{-\frac{(k-Np)^2}{2Np(1-p)}}
\]
therefore, 
\[
I_{1-p}(\ell+1, N-\ell) = \bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;

\BEAS
Q(N,p) 
&\equiv& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&=& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1} \frac{1}{(2\ell+1) \Beta(\ell+1, \ell+1)}  I_{1-p}(\ell+1, N-\ell)\\
&\approx& \sum_{\ell=0}^N\frac{1}{2(\ell+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{-\frac{(\ell-\frac{N}{2})^2}{\frac{N}{2}}}  \bar{\Phi}( (\ell - N \cdot (1-p))/\sqrt{N \cdot p \cdot (1-p)} )\\
&\approx& \int_0^1 \frac{1}{2(Nt+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{- 2N(t-\frac{1}{2})^2}  \bar{\Phi}( \frac{\sqrt{N}(t - (1-p))}{\sqrt{ p \cdot (1-p)}} ) \,dt
\EEAS

Numerically, we can see that the first term in the sum is always $0.5.$
Also we know that by definition $Q(N, 1) = 1$ for any $N$.
From numerically calculation we guess that
$Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$.
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
$\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$


\begin{lemma}
Define:
\[
Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
\]
Then, 
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
\[
\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.
\]
\end{lemma}


% \begin{lemma}
% Define:
% \[
% Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
% \]
% Then, as $N \rightarrow \infty$ with $p$ fixed:
% \[
% Q(N,p)  \approx O(N^{-1/2}).
% \]
% \end{lemma}
\begin{proof}
The first term in the sum is $0.5$.

(Sketch). 
{\bf The sum has the lower bound $Q \geq 1/10$ just by inspecting
the first 10 terms (say), which are all positive and all greater
than $0.01$ (say). The following argument shows that later terms
add up to at least $\Omega(N^{-1/2})$.}
First, we know that
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]

Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$ 
\[
\bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;
this is the classical De Moivre theorem on normal approximation to the binomial. It can be made precise in many ways
that have been well documented over the centuries.
Roughly speaking, in terms of variable $z = (\ell - \mu)/\sigma$,
we have
\[
\bar{B}(\ell;N,1-p)  \approx \left \{ \begin{array}{ll}
1 & z < 3 \\
0 & z > 3 .
\end{array}
\right .
\]

Hence, defining for $m = \mu - 3 \sigma$
\[
\bar{B}(\ell;N,1-p) \approx 1, \mbox{ for } \ell \leq m.
\]
Now of course
\begin{eqnarray*}
Q(N,p) &\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} .
\end{eqnarray*}
Now from DeMoivre's theorem (case $p=1/2$, $N=2\ell$) we also know that
\[
    2^{-2\ell} { 2 \ell \choose \ell} = bin(\ell; 2 \ell, 1/2) \sim \sqrt{\frac{1}{\ell \cdot \pi}},
\]
where $bin(k;N,p)$ is the usual binomial probability mass function.
We obtain
\[
  \sum_{\ell=0}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2} \geq 
  \sum_{\ell=m/2}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2}  \geq 
  Const  \cdot m^{-1/2}
\]

\end{proof}





\subsection{Bounds on $\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}$}
\begin{lemma}
\label{TaylorSqrtInv}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(x\right)^{\ell}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\binom{-1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{-1/2}{\ell}(-1)^\ell
&=\frac{-\frac12(-\frac12-1)(-\frac12-2)\cdots(-\frac12-\ell+1)}{\ell!}\\
&=\frac{1}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-1)\\
&=\frac{1}{2^\ell\ell!}\frac{(2\ell)!}{2^{\ell}(\ell)!}\\
&=\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}
\end{align}
\end{proof}

\begin{lemma}
\label{TaylorSqrtInvExpect}
\beq 
1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p) \geq  \frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} \geq 1 .
\eeq
where 
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|^{-1}_{\ell_2(J)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(\cT)} }{\| \psi \|^2_{\ell_2(J)}}} \geq 1 .
\eeq
Therefore, 
\beq 
\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}  
 \geq   1 .
\eeq

On the other hand, let 
\beq 
\E_I (\frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} )^{-1}
 = \E_I ( 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}})^{-1/2}.
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.


\begin{align}
(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(\rho_J\right)^{\ell}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell-1;n,1-p)    \leq \E_I \rho_I^{\ell} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\\
&\geq  \sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)
\end{align}

\end{proof}





\subsection{Numerically calculate $\E_I  \| \psi_I \|_2/\| \psi \|_2$}

We numerically compute $Q(N,p)$, the result is in the following table. Compare the table with the tables of MC approximation, we see that our previous bound is still too loose.
\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{$Q(N,p)$} \\
\hline
  $p=$ &0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0.9439 & 0.9406 & 0.9370 & 0.920  & 0.8172 & 0.3358 & 0.0482 & 0 \\
\hline
$N=500$ & 0.9748  & 0.9734 & 0.9718 & 0.9643 & 0.9199 & 0.7302 & 0.209 & 0 \\
\hline      
\end{tabular}
\label{Q_table}
\end{table}

Then we use MC approximation to calculate $\E_I  \| \psi_I \|_2/\|  \psi \|_2$ for a few different $\psi.$
We will know that
\BIT
\item 
When $\psi = e_0$,  $\E_I  \| (e_0)_I \|_2=p$ 

\item
When $\psi = e_0+e_1$,  
\[
\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2 = \sqrt{\frac12} \E_I  \| (e_0+e_1)_I \|_2 = 
\E_I \sqrt{\frac{\sum_{i=\{0,1\}} I_i}{2}}=p^2+ 2p(1-p)\sqrt{\frac12}
\]
\item
We know that when $\psi = a =(1,\ldots,1)$, then
\[
\E_I  \| a_I \|_2/\| a \|_2=\E_I \sqrt{\frac{\sum_{i=[N]} I_i}{N}} 
\]
Using law of large numbers, 
\[
\lim_{N\rightarrow \infty }\sqrt{\frac{\sum_{i=[N]} I_i}{N}}  = \sqrt{p}.
\]
\item
For fixed support $J$, we can choose $\psi = \sum_{i\in J} e_i,$ then $\| \psi_J \|_2/\|  \psi \|_2 =1.$
However, the expectation is not going to be one. Let $M := |J|,$
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} = \sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}\leq \sqrt{p}
\]
The inequality can be seeing using central limit theorem, we have normal approximation  $\frac{\sum_{i\in J} I_i}{|J|} \sim N(p,  \frac{p(1-p)}{\sqrt{|J|}})$, then using Jensen's inequality, since square root fucntion is concave,
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} \approx \E_G\sqrt{p+ \frac{p(1-p)}{\sqrt{|J|}}G}  \leq \sqrt{\E_G[p+ \frac{p(1-p)}{\sqrt{|J|}}G]} =\sqrt{p} 
\]
\EIT
Using symmetry, we guess that the maximum value of $\E_I  \| \psi_I \|_2/\|  \psi \|_2$  is $\sqrt{p}$ instead of $1$, and the maximum value is achieved when $\psi$ is dense.

\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \| a_I \|_2/\| a \|_2$ where $a=(1,\ldots,1)$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0 & 0.3123 & 0.4460 & 0.7063  & 0.94865 & 0.9950 & 0.9995 & 1 \\
\hline
$N=500$ &0 &0.3153  & 0.4464 & 0.7068 & 0.94874 & 0.9950 & 0.9995 & 1\\
\hline      
\end{tabular}
\label{allone_table}
\end{table}


\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=500$ & 0 &0.1375 &	0.2667 &	0.6034 &	0.9365 &	0.9946 &	0.9994 & 1 \\
\hline      
\end{tabular}
\label{coordinatevector_table}
\end{table}



\subsection{Tight bound and stationary points of $\E_I  \| \psi_I \|_2/\| \psi \|_2$}
\begin{lemma}
\beq 
p \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq \sqrt{p}  .
\eeq
where the lower bound is achieved by $1-$sparse vectors $\pm e_i$, the upper bound is achieve by $\{\frac{\sum_{i\in \cT} \pm e_i}{\sqrt{N}}\}$.
Furthermore, all the stationary points of this objective are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ for different support $J\subset \cT$. 
\end{lemma}
\begin{proof}
This problem can be reformulate as the projection pursuit with sphere constraint,
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
Then from \cite{bai2018subgradient} Proposition $3.3$, we get the result. 

The main idea of the proof is to calculate the projected gradient
for $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$, when $|J| = M,$
\[
e_j^T  \E_I  \partial\| q_I \|_2 = q_j [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] 
\]
so
\[
(I-q q^T)  \E_I  \partial\| q_I \|_2 = [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q-[\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q = 0.
\]
then $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ is stationary points.
 
The other direction (all other points are not stationary) is implied by (the proof of) theorem $3.4$ in  \cite{bai2018subgradient}.
\end{proof}

==> old_sec/sec_old_2020/Expectation_Updated.tex <==
\section{Expectation calculation}
In the following, we calculate $\E| \psi^T X| $ for $X_t$ IID sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0.$
\subsection{Expectation of inner product for sparse $X$}
In the following, we study in detail the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ have variance $\sigma^2$,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \sigma^2 \|\psi\|_2^2.
\]
The ratio indicates the sparsity level of the random variable $ \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\sigma^2 \|\psi\|_2} 
\]
Now, we consider $E{|\sum_{i} \psi_i X_i| }$ in the general symmetric setting, where a lower bound can be derived.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i Z_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $Z_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
\E_X{|\sum_{i} \psi_i X_i| }  
= \E_B \E_G {|\sum_{i} \psi_i B_i G_i| }
= \E_I \E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the fact that linear transforms of Gaussians are also Gaussian, we get
\[
\E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]


\paragraph{Upper and lower bound for symmetric distribution}
It is worth commenting that we could still calculate the upper and lower bound of $\E{| \psi^T X| }$ in terms of $\E_I\| \psi_I\|_2$ for $X_t$ IID sampled from any Bernoulli symmetric $p G +(1-p) \delta_0$, where $G$ is a symmetric distribution. 
% Dave Comment:
% Put the generalization in the end.
% Focus on Bernoulli Gaussian for the main part, and then talk about extension.


% \paragraph{General symmetric distribution case}
\begin{lemma} \label{lem:sym_Khintchine_inequality}
If we only know $\Xi_i$ are IID sampled from a symmetric distribution $F$ with unit variance, then we already have a lower bound,  
\[
     1/\sqrt{2}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
\] 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:sym_Khintchine_inequality}]
The upper bound come from Cauchy inequality.
 
Now we derive the lower bound. We write $\Xi_i = \sigma_i |\Xi_i|$, where $s_i =\pm 1$ with equal probability since $\Xi_i$ are symmetric RV, and $\{s_i,|\Xi_i|\}$  are all independent random variables. We could use Khintchine inequality,


\begin{eqnarray*}
\E_\Xi |\sum_i a_i \Xi_i| &=& E_{|\Xi_i|}E_{s_i} |\sum_i a_i s_i |\Xi_i||\\
&\geq&  
  1/\sqrt{2}  \sum_i a_i^2  E_{|\Xi_i|} |\Xi_i|^2 \\
  &=&   1/\sqrt{2}  \|a\|_2^2.
\end{eqnarray*}
\end{proof}

Let $\psi_I = a$, we have a corollary for Bernoulli Symmetric case,
\[
 \E_I \|\psi_I\|_2  \geq \E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]


\begin{theorem}
Let $X_i = B_i \Xi_i$ be IID, where $B_i$ is sampled from Bernoulli with parameter $p$, let $I$ be the support where $B_i =1$. And $\Xi_i$ is variance $1$, sampled from: 
\begin{itemize}
    \item $N(0,1)$
    % \item sub-Gaussian with sub-Gaussian norm $K = \|Z\|_{\Psi_2}$
    \item general symmetric distribution with variance $1$.
\end{itemize}
% Here sub-Gaussian norm is defined as
% $
% \|X\|_{\Psi_2} := \sup_{r\geq 1} r^{-1/2}  (E|X|^r)^{1/r}.
% $

Then 
\begin{itemize}
    \item(for Bernoulli Gaussian:)
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot \E_I \|\psi_I\|_2
\]
%     \item (for Bernoulli sub-Gaussian:) 
%      \[
% \E_X{|\sum_{i} \psi_i X_i| }  
% \geq  3^{-3/2}C^{-3} K^{-3}  \cdot (1-(1-p)^{\|\psi\|_0})^{1/2}   \cdot  \|\psi\|_2.
% \]
    \item (for Bernoulli symmetric R.V. :) 
    \[
\E_I \|\psi_I\|_2 \geq \E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]
\end{itemize}

\end{theorem}

\subsection{Expectation over Bernoulli support}

We previously considered the identity
\beq \label{eq:startingPoint}
    \E | \sum_{i \in \cT}  \psi_i X_i | = \sqrt{\frac{2}{\pi}} \cdot \E_I \| \psi \|_{\ell_2(I)},
\eeq
where $X$ is a Bernoulli-Gaussian RV $BG(p;0,1)$,
and where $I$ is a random subset of the domain $\cT$
determined by Bernoulli-$p$ coin tossing.

% Comment:
Let $J \subset \cT$ be the support of $X$, where $  N:=|\cT|$, $N_J:=|J|$. Let $\psi_J : = \psi\cdot 1_J$ denote the elementwise product of vector $\psi$ with the indicator vector of subset $J$. Then we can consider our problem on the space $\cT$ by default, and rewrite for simplicity
\[
\| \psi_J \|_{2} : = \| \psi_J \|_{\ell_2(\cT)} = \| \psi \|_{\ell_2(J)}.
\]

This leads us to consider the following ratio:
\[
  V^J_k(\psi) := \frac{\| \psi \|_{\ell_2(J)}^{k}}{\| \psi \|_{\ell_2(\cT)}^{k}},
 \]
 and its expectation over all Bernoulli random subset,
\[
  V_k(\psi) := \frac{\E_I \| \psi \|_{\ell_2(I)}^{k}}{\| \psi \|_{\ell_2(\cT)}^{k}},
 \]
 where $I$ is again a random subset.
%  The following lemma shows that $\E_I \| \psi \|_{\ell_2(I)}^{2k} \approx \| \psi \|_{\ell_2(\cT)}^{2k}$.
We remark that the lower bound of $V_k(\psi)$ is the optimal value of the optimization problem:
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|^k_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1,
\end{eqnarray*}
and the upper bound of $V_k(\psi)$ is the optimal value of the optimization problem
 \begin{eqnarray*}
    \max&   \E_I  \| \psi_I \|^k_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}




\begin{lemma} \label{lem:BGPropLemmaSub_fix}
Let $\psi$ denote a vector in $\reals^N$. For fixed support $J\subset [N]$ then for any $k\neq 0$, the deterministic quantity $V^J_{k}(\psi)$ satisfies:
\[
0 \leq V^J_{k}(\psi) \leq 1.
\]
The upper bound is approached by the vectors $\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in J}\pm e_j\}$, where  $\| \psi_J \|_2^k/\|  \psi \|_2^k =1$,
 and the lower bound is approached by 
any $\psi$ that has all of its entries on $J$ to be zero.
\end{lemma}

\begin{lemma} \label{lem:BGPropLemmaSub_2}
Let $\psi$ denote a vector in $\reals^N$.
\[
V_2(\psi) =   p.
\]
\end{lemma}



\begin{theorem} \label{thm:BGPropLemmaNorm}
Let $\psi$ denote a vector in $\reals^N$, then
\[
p \leq V_{1}(\psi) \leq V_{1}(\frac{\sum_{j\in [N]}\pm e_j}{\sqrt{N}} ) \leq \sqrt{p} .
\]
the lower bound is approached by on-sparse vectors $\psi \in \{ \pm e_i, i\in [N]\}$, and the upper bound is approached by 
$\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$.

Furthermore, all the stationary points of $V_{1}(\psi)$ are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm e_i, i\in [N]\}$ are the global minimizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$ are the global maximizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ are saddle points with value
\[
V_1(\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}) = \E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}\sqrt{\frac{j}{N_J}}.
\]
\end{theorem}
Remark:
Specifically,
\[
V_1( e_i) = p.
\]
\[
V_1(\frac{ e_i+e_j}{\sqrt{2}}) = p(\sqrt{2}+(1-\sqrt{2}p)).
\]



\begin{theorem} \label{thm:BGPropLemmaSub_k}
For $k\geq 2$, let $\psi$ denote a vector in $\reals^N$, then
\[
p^k \leq V_{2k}(\frac{\sum_{j\in [N]}\pm e_j}{\sqrt{N}} ) \leq V_{2k}(\psi) \leq p.
\]
the upper bound is approached by on-sparse vectors $\psi \in \{ \pm e_i, i\in [N]\}$, and the lower bound is approached by 
$\psi  \in \{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$.

Furthermore, all the stationary points of $V_{2k}(\psi)$ are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ for different support $J\subset \cT$, where $\{ \pm e_i, i\in [N]\}$ are the set of global maximizers, and $\{  \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j\}$ are the set of all the global minimizers. And for $J$ with $1<N_J<N$, $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ are saddle points with value
\[
V_{2k}(\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}) = \E_I (\frac{\sum_{i\in J} 1_{I_i}}{N_J})^k = \sum_{j=0}^{N_J} (1-p)^{N_J-j} p^{j} {N_J \choose j}(\frac{j}{N_J})^k.
\]
\end{theorem}







\paragraph{Tight bound on $V_1$ and $V_{2k}$ using mean and variance of $\frac{\sum_{i\in J} 1_{I_i}}{N_J}$}

Now notice that 
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} 
\]
has mean $p$ and variance $\frac{p(1-p)}{N_J}$.
We could define a zero mean unit variance random variable $g^J$ as a function of $\{1_{I_i}\mid i\in J\}$ 
\[
g^J := \left(\frac{\sum_{i\in J} 1_{I_i}}{N_J}-p\right)/ \left( \sqrt{\frac{p(1-p)}{N_J}} \right)
\]
namely, $\E_I \left( g^I\right)=0, \E_I \left( g^I\right)^{2}=1$.
then
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} := p + \sqrt{\frac{p(1-p)}{N_J}} g^J = p(1 + \sqrt{\frac{1-p}{p N_J}} g^J)
\]
then
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \E_I\sqrt{p- \sqrt{\frac{p(1-p)}{N_J}}g^I} 
= \sqrt{p} \E_I\sqrt{1+ \sqrt{\frac{1-p}{pN_J}}g^I}  
\]
\[
\E_I \left(\frac{\sum_{i\in J} 1_{I_i}}{N_J}\right)^k 
= p^k \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^k 
\]
\begin{lemma}
\label{TaylorSqrt}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{1/2}
=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{lemma}

\begin{lemma}[Taylor expansion for $V_1$]
\label{TaylorSqrt_Expect}
Using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
\BEAS
\frac{1}{\sqrt{p}}\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} 
&=& \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^{1/2} \\
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_I \left( g^I\right)^{\ell+1}\\
&=& 1- 2^{-3}({\frac{1-p}{pN_J}}) +O\left( ({\frac{1-p}{pN_J}})^2 \right).
\EEAS
\end{lemma}

\begin{lemma}[Taylor expansion for $V_{2k}$]
\label{TaylorSqrt_Expect_k}
Using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
\BEAS
\frac{1}{p^k}\E_I ({\frac{\sum_{i\in J} 1_{I_i}}{N_J}})^k  
&=& \E_I\left({1+ \sqrt{\frac{1-p}{pN_J}}g^I}\right)^{k} \\
&=& 1 +\sum_{\ell=1}^{k} \binom{k}{\ell} ({\frac{1-p}{pN_J}})^{\ell/2} \E_I (g^I)^{\ell}\\
&=& 1 + \frac{k(k-1)}{2} ({\frac{1-p}{pN_J}}) +O\left( ({\frac{1-p}{pN_J}})^2 \right).
\EEAS
\end{lemma}
Therefore, we know what when $N_J>>1$, 
$V_1(\frac{\sum_{i\in J} 1_{I_i}}{N_J})$ is close to its upper bound $\sqrt{p}$, 
and for $k\geq 2$, 
$V_k(\frac{\sum_{i\in J} 1_{I_i}}{N_J})$ is close to its lower bound $p^k$. Namely 
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} \approx \sqrt{p},
\]
\[
\E_I (\frac{\sum_{i\in J} 1_{I_i}}{N_J})^k \approx p^k.
\]

% Using central limit theorem, when $N_J\rightarrow \infty$,
% \[
% \frac{\sum_{i\in J} 1_{I_i}}{N_J} \sim N(p,  \frac{p(1-p)}{N_J})
% \]
% we can further calculate the asymptotic using moments of Gaussian.
% \begin{lemma}[Taylor expansion and Gaussian approximation for $V_1$]
% \label{TaylorSqrt_Expect}
% and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
% \BEAS
% \frac{1}{\sqrt{p}}\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} 
% &\approx&  \E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G} \\
% &=& 1-\sum_{s=1}^\infty\frac1{s}\frac{(4s-2)!}{(2s-1)!(2s-1)!}2^{-4s} \frac{(2s-1)!}{2^{s-1}(s-1)!} (p^{-1}-1)^{s}  N_J^{-s}
% \EEAS
% \end{lemma}

% \begin{lemma}[Taylor expansion and Gaussian approximation for $V_{2k}$]
% \label{TaylorSqrt_Expect_k}
% and using Taylor expansion, asymptotically when $N_J\rightarrow \infty$, 
% \BEAS
% \frac{1}{p^k}\E_I ({\frac{\sum_{i\in J} 1_{I_i}}{N_J}})^k  
% &\approx&  \E_G({1+ \sqrt{\frac{1-p}{pN_J}}G})^k \\
% &=& 1 +\sum_{\ell=1}^{k} \binom{k}{\ell} ({\frac{1-p}{pN_J}})^{\ell/2} \E_G G^{\ell}\\
% &=& 1 +\sum_{s=1}^{\left\lfloor{k/2}\right\rfloor} \binom{k}{2s} ({\frac{1-p}{pN_J}})^{s} (2s-1)!!
% \EEAS
% \end{lemma}




\begin{figure} 
\includegraphics[width=.7\textwidth]{./figures_BD/Ju_landscape.png}
% \includegraphics[width=.45\textwidth]{./figures_BD/Ju_landscape_m100.png}
\caption{The value of $V_1$ on a two-dimensional sphere in $\reals^3$, normalized by the affine transform to send the value in $[0,1].$  
Figure credit to Ju Sun's talk based on the paper \cite{bai2018subgradient}
}
\label{fig-landscape-V1}
\end{figure}





\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/Full_compare_with_baseline.png}
\caption{The value of $V_1(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is $V_1(\psi)$. }
\label{fig-V1}
\end{figure}

\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/L4_plot.png}
\caption{The value of $V_4(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is $V_4(\psi)$. }
\label{fig-V4}
\end{figure}



\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/ratio/L8_plot.png}
\caption{The value of $V_8(\psi)$ for different $\psi$, $x-$axis is the sparsity parameter $p$, $y-$axis is $V_8(\psi)$. }
\label{fig-V4}
\end{figure}



\subsection{Proofs}


\begin{proof}[Proof of Theorem~\ref{thm:BGPropLemmaNorm}]
First, we show that the upper and lower bound value we give is achievable.
\BIT
\item 
When $\psi = e_0$,  
\[
\E_I  \| (e_0)_I \|_2=p\| (e_0)\|_2+(1-p)\| 0\|_2 = p.
\]
\item
When $\psi = \frac{1}{\sqrt{N}}\sum_{j\in [N]}\pm e_j,$ then  
\[
V_1(\psi) = \E_I \sqrt{\frac{\sum_{i\in [N]} 1_{I_i}}{N}} \leq   \sqrt{\E_I \frac{\sum_{i\in [N]} 1_{I_i}}{N}} = \sqrt{p}.
\]
The inequality comes from Jensen's inequality, since square root function is concave.
\item
For fixed support $J$, when $\psi = \frac{1}{\sqrt{N_J}}\sum_{i\in J} e_i,$  then $\| \psi_J \|_2/\|  \psi \|_2 =1.$
However, the expectation is going to be smaller for $p<1$. 
\[
V_1(\psi) = \E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} = \sum_{k=0}^{N_J} (1-p)^{N_J-k} p^{k} {N_J \choose k}\sqrt{\frac{k}{N_J}}.
\]
\EIT

This problem can be reformulated as projection pursuit with sphere constraint,
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
Then from \cite{bai2018subgradient} Proposition $3.3$, we get the result. 

The main idea of the proof is to calculate the projected gradient
for $q  \in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$, when $N_J = M,$
\[
e_j^T  \E_I  \partial\| (q)_I \|_2 = q_j [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] ,
\]
therefore,
\[
  \E_I  \partial\| (q)_I \|_2 =  [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] q,
\]
so
\[
(I-q q^T)  \E_I  \partial\| q_I \|_2 = [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q -[\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q  = 0.
\]
then $q \in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{N_J}}\}$ are stationary points.
 
The other direction (all other points are not stationary) is implied by (the proof of) Theorem $3.4$ in  \cite{bai2018subgradient}.
\end{proof}





\begin{proof}[Proof of Lemma~\ref{TaylorSqrt}]
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{1/2}
=\sum_{\ell=0}^\infty\binom{1/2}{\ell}(-x)^\ell.
\eeq

\begin{align}
\binom{1/2}{\ell}
&=\frac{\frac12(\frac12-1)(\frac12-2)\cdots(\frac12-\ell+1)}{\ell!}\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-3)\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}\frac{(2\ell-2)!}{2^{\ell-1}(\ell-1)!}\\
&=\frac{(-1)^{\ell-1}}{\ell2^{2\ell-1}}\binom{2\ell-2}{\ell-1},
\end{align}
then
\begin{align}
(1-x)^{1/2}
&=1-\sum_{\ell=1}^\infty\frac2\ell\binom{2\ell-2}{\ell-1}\left(\frac x4\right)^\ell\\
&=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}.
\end{align}
\end{proof}







\begin{proof}[Proof of Lemma~\ref{TaylorSqrt_Expect}]
\BEAS
\E_I\sqrt{1- \sqrt{\frac{1-p}{pN_J}}g^I}  
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_I \left( g^I\right)^{\ell+1}\\
&=& 1- 2^{-3}({\frac{1-p}{pN_J}}) - O(({\frac{1-p}{pN_J}})^2)
\EEAS
Using the central limit theorem, when $N_J\rightarrow \infty$, we have normal approximation for $g^J$ so that
\[
\frac{\sum_{i\in J} 1_{I_i}}{N_J} \sim N(p,  \sqrt{\frac{p(1-p)}{N_J}}),
\]
then for $G\sim N(0,1),$ asymptotically when $N_J\rightarrow \infty$,
\[
\E_I \sqrt{\frac{\sum_{i\in J} 1_{I_i}}{N_J}} \approx  \sqrt{p} \E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G} =
\sqrt{p} \left( 1- 2^{-3}(1-p)^{2}  N_J^{-1} + O((1-p)^{4}  N_J^{-2})\right),
\]
where
\BEAS
\E_I\sqrt{1- \sqrt{\frac{1-p}{pN_J}}g^I}  
&\approx &\E_G\sqrt{1- \sqrt{\frac{1-p}{pN_J}}G}\\
&=& 1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1}\E_G \left( G\right)^{\ell+1}\\
&=& 1-\sum_{\ell \mbox{ is odd}}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\left( \sqrt{\frac{1-p}{pN_J}}\right)^{\ell+1} (\ell)!!\\
&=& 1-\sum_{s=1}^\infty\frac1{s}\binom{4s-2}{2s-1}2^{-4s} (2s-1)!! (p^{-1}-1)^{s}  N_J^{-s}\\
&=& 1-\sum_{s=1}^\infty\frac1{s}\frac{(4s-2)!}{(2s-1)!(2s-1)!}2^{-4s} \frac{(2s-1)!}{2^{s-1}(s-1)!} (p^{-1}-1)^{s}  N_J^{-s}\\
&=& 1-\sum_{s=1}^\infty\frac{(4s-2)!}{(2s-1)!(s)!}2^{-5s+1}  (p^{-1}-1)^{s}  N_J^{-s}.
\EEAS
\end{proof}






==> old_sec/sec_old_2020/Inequality.tex <==
\subsection{$E{| \psi^T X| }$ for IID Bernoulli Symmetric $X$ }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ have variance $\sigma^2$,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \sigma^2 \|\psi\|_2^2.
\]
The ratio indicate the sparsity level of random variable $ \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\sigma^2 \|\psi\|_2} 
\]
Now, we consider $E{|\sum_{i} \psi_i X_i| }$ for general symmetric setting when lower bound can be derived.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i Z_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $Z_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
\E_X{|\sum_{i} \psi_i X_i| }  
= \E_B \E_G {|\sum_{i} \psi_i B_i G_i| }
= \E_I \E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
\E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]


\paragraph{Symmetric distribution}

Dave Comment:
Put the generalization in the end.
Focus on Bernoulli Gaussian for the main part, and then talk about extension.


% \paragraph{General symmetric distribution case}
\begin{lemma} \label{lem:sym_Khintchine_inequality}
For we only know $\Xi_i$ are IID sampled from a symmetric distribution $F$ with unit variance, then we already have a lower bound,  
\[
     1/\sqrt{2}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
\] 
\end{lemma}
 \begin{proof}[Proof of Lemma \ref{lem:sym_Khintchine_inequality}]
 The upper bound come from Cauchy inequality.
 
Now we derive the lower bound. We write $\Xi_i = \sigma_i |\Xi_i|$, where $s_i =\pm 1$ with equal probability since $\Xi_i$ are symmetric RV, and $\{s_i,|\Xi_i|\}$  are all independent random variables.  
we could use Khintchine inequality,
here is the Wiki link for more detail:
\begin{quote}
\href{https://en.wikipedia.org/wiki/Khintchine_inequality}{Khintchine inequality}.
\end{quote}




\begin{eqnarray*}
\E_\Xi |\sum_i a_i \Xi_i| &=& E_{|\Xi_i|}E_{s_i} |\sum_i a_i s_i |\Xi_i||\\
&\geq&  
  1/\sqrt{2}  \sum_i a_i^2  E_{|\Xi_i|} |\Xi_i|^2 \\
  &=&   1/\sqrt{2}  \|a\|_2^2.
\end{eqnarray*}
\end{proof}

Let $\psi_I = a$, we have a corollary for Bernoulli Symmetric case,
   \[
 \E_I \|\psi_I\|_2  \geq \E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]


\begin{theorem}
Let $X_i = B_i \Xi_i$ be IID, where $B_i$ is sampled from Bernoulli with parameter $p$, let $I$ be the support where $B_i =1$. And $\Xi_i$ is variance $1$, sampled from: 
\begin{itemize}
    \item $N(0,1)$
    % \item sub-Gaussian with sub-Gaussian norm $K = \|Z\|_{\Psi_2}$
\item general symmetric distribution with variance $1$.
\end{itemize}
% Here sub-Gaussian norm is defined as
% $
% \|X\|_{\Psi_2} := \sup_{r\geq 1} r^{-1/2}  (E|X|^r)^{1/r}.
% $

Then 
\begin{itemize}
    \item(for Bernoulli Gaussian:)
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot \E_I \|\psi_I\|_2
\]
%     \item (for Bernoulli sub-Gaussian:) 
%      \[
% \E_X{|\sum_{i} \psi_i X_i| }  
% \geq  3^{-3/2}C^{-3} K^{-3}  \cdot (1-(1-p)^{\|\psi\|_0})^{1/2}   \cdot  \|\psi\|_2.
% \]
\item (for Bernoulli symmetric R.V. :) 
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]
\end{itemize}

\end{theorem}




% \paragraph{Sub-Gaussian case}
% For a sub-Gaussian random variable $\Xi$ with unit variance and symmetric c.d.f $F$, we define 
% \[
% K = \|\Xi\|_{\Psi_2} = \sup_{r\geq 1} r^{-1/2}  (E|\Xi|^r)^{1/r}
% \]
% as the sub-gaussian norm of $X$
% \begin{lemma} \label{lem:Khintchine}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then for all $r \geq 2$,
% \[
% \|\psi\|_2 \leq (E(Z)^p)^{1/p} \leq C K p^{1/2} \|\psi\|_2
% \]
% where $C$ is absolute constant.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% The lower bound follows by independence and Holder’s inequality.
% For the upper bound, since we have 
% \[
% \|\sum_i a_i X_i\|_{\Psi_2}^2\leq C\sum_i a_i^2 \| X_i\|_{\Psi_2}^2\leq C\|\psi\|_2^2 K^2,
% \]
% And $Z = \sum_i a_i X_i$ is sub-Gaussian, so for all $p\geq 2$,
% \[
%  (E(Z)^p)^{1/p} \leq \|Z\|_{\Psi_2} p^{1/2} \leq C^{1/2} p^{1/2}\|\psi\|_2 K 
% \]
% \end{proof}
% \begin{lemma} \label{lem:Khintchine for $p=1$}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then
% \[
%      3^{-3/2}C^{-3} K^{-3}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
% \] 
% \[
%      3^{-3/2}C^{-3} K^{-3}  \|\psi\|_2 \leq E |\sum_i a_i X_i| \leq \|\psi\|_2
% \]
% where $C$ is absolute constant, $K = \|X\|_{\Psi_2}$.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% We use the extrapolation trick. 
% Let $Z=\sum_i a_i X_i$, since we have 
% \[ (E(Z)^2){1/2} \leq (E|Z|)^{1/4}((E(Z)^3)^{1/3})^{3/4},\]
% we get 
% \[E|Z|\geq (E(Z)^2)^{2}/ (E(Z)^3).\]

% We get a bound on 
% \[
% \|\psi\|_2 \leq (E(Z)^r)^{1/r} \leq C K p^{1/2} \|\psi\|_2
% \]
% from Khinthine’s inequality for $r = 3$.
% \end{proof}




==> old_sec/sec_old_2020/Intro.tex <==
\section{Introduction}
\subsection{Introducing the blind deconvolution problem}
Blind deconvolution is the problem of recovering a filter and a signal from their (noisy or corrupted) convolution.
This is a ubiquitous problem, occuring in fields across signal processing, machine learning, computer vision, seismology, and neuro-science.
Blind deconvolution is also a crucial problem at the core of digital communication that powers our modern society by enabling cell phone communication.

One important example of blind deconvolution occurs when the signal is sparse. We call this problem \emph{sparse blind deconvolution}. The sparse signal setting of blind deconvolution appears in seismology, microscopy, astronomy, neuro-science spike identification. In representation learning for computer vision, computational imaging and speech analysis, sparse blind deconvolution is also interpreted as single-channel convolutional dictionary learning.

Despite the importance of blind deconvolution, until recently there has been little understanding of when, how and why these non-convex algorithms succeed.
Practitioners have accumulated poetic yet vague observations like "when the initialization is close, gradient-based methods find the true signal", but there is no clear understanding of this statement.

This work demonstrates that a convex formulation hiding behind the scene can explain the success of this poetic heuristic. Our mathematical formulation gives a crisp, clean view that clears all the fog in the claims of past practitioners. 

\subsection{Previous works on the blind deconvolution problem}
\paragraph{Non-convexity for blind deconvolution problems}
Suppose there is a sparse signal $X$ and a forward filter $a$, the observation is their convolution $Y$, defined as $Y = a * X$. Blind deconvolution is the problem of finding the sparse signal $X$ from the observation $Y$ without knowing the forward filter $a$. 

As both the sparse signal and the forward filter $a$ are unknown, the problem is bilinear in $a$ and $X$. And the expression $a*x$ has scaling and shift symmetry for $(a,x)$.
Therefore, blind deconvolution is often formulated as a non-convex problem. 

\paragraph{Searching the inverse filter}
Instead of trying to recover $a$ and $X$ together from $a*X$, 
we could formulate this problem as looking for an approximate inverse  filter $w$ so that $w*Y$ is special or \textit{simple}. 

 To make our discussion concrete, we define inverse filter formally.
  
\paragraph{Inverse filter }
Let $e_0$ be the sequence with $1$ at $0$ coordinate and $0$ elsewhere, then it is the unit of convolution.  For the forward filter $a\in l_1(\integers) $, we want to give a condition that guarantees there exists an inverse filter $a^{-1}\in l_1(\integers)$ so that $a^{-1}*a = e_0.$

This condition is that $a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$ 
From Wiener's lemma, we know that this condition on $a$ would ensure that $a$ is invertible and the inverse filter $a^{-1} \in l_1(\integers)$.
\begin{lemma}
If $a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T,$ we could define the inverse filter of $a$ as:
$$a^{-1} := \mathcal{F}^{-1}(\frac{1}{\mathcal{F} a})$$
so that $a^{-1}*a = e_0.$
From Wiener's lemma on $\mathcal{F} a$,   $a^{-1} \in l_1(\integers)$ .
\end{lemma}
 
\paragraph{Minimal entropy deconvolution}
This formulation of searching inverse filter is adapted in the earlier work of Wiggins \cite{wiggins1978minimum} and Donoho \cite{donoho1981minimum} for minimum entropy deconvolution, or maximum high order cumulant deconvolution, with seismology as the motivating application. The core idea is to find an approximate inverse filter $w\approx a^{-1}$, so that $w*Y$ is the most non-Gaussian.
Namely, we want to find $w\neq 0$, so that  
\[
 \begin{array}{ll}
 \underset{w\neq 0}{\mbox{maximize}}   & J(w*Y)
\end{array}
 \]
  Here the non-Gaussianity objective $J$ could be the negative entropy $J(z) = -\mbox{Entropy}(p_z)$, the normalized $4$-th order cumulant, $J(z) = {\|z\|_4^4}/{\|z\|_2^4}$, or the varimax norm: $J(z) = \|z\|_\infty/\|z\|_2$ (proposed in the paper \cite{cabrelli1985minimum,wiggins1978minimum,donoho1981minimum}).
  \paragraph{Blind equalization}
  There are a series of digital communication work on blind deconvolution when the digital signal is discrete, which is called \textbf{blind equalization}. Examples of digital signals are PAM signaling, which is a $\pm 1$ binary signal, and QAM signaling, where the signal has equally spaced points on unit sphere in complex space \cite{kennedy1992blind,ding2000fast}.  
  In the work \cite{vembu1994convex}, using the condition that $X$ are IID and bounded by a known constant, for example, $ \|X\|_\infty =1$ after rescaling, the authors propose to solve a non-convex problem
   \[
 \begin{array}{ll}
 \underset{w}{\mbox{maximize}}   &  
 \|w * Y\|_8 
 \\
\mbox{subject to} 
& \|w*Y\|_2 = 1
\end{array}
  \]
using projected gradient descent, where the $\ell_8$ norm objective is used as an approximation of the  $\ell_\infty$ norm objective $\|w * Y\|_\infty $.
Later, the work \cite{ding2000fast} uses linear programming to solve the $\infty$ norm problem directly.

 
%  In the middle of the work \cite{vembu1994convex}, an ideal convex problem for blind equalization is proposed, although it is not computable without knowing $a$. The ideal convex problem is 
%   find $w$ so that $w*a = e_0 = (\ldots,0,1,0, \ldots)$ as minimizer of the ideal convex problem
%   \[
%  \begin{array}{ll}
%  \underset{w}{\mbox{minimize}}   & \| w*a\|_1 
%  \\
% \mbox{subject to} 
% & (w*a)_0 = 1.
% \end{array}
%   \]  
% Although this ideal problem is more of a theoretical proof tool for authors of that time, it is a 

\section{Main results overview}
\subsection{Convex formulation of sparse blind deconvolution}






\paragraph{Scalable convex formulation for finding sparsing transform}
Now we propose a scalable convex optimization framework for blind deconvolution.

First, we set up the finite-sample observation model. Given a series of observations $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$, we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse, where $V$ is a $2k+1$ dimensional subspace of the doubly infinite sequences. Let $\|\cdot\|_{1,[-T,T]} =\|\cdot\|_{\ell_1(\cT)} $ be the $1$-norm over the centered window of radius $T$. Let $N:= 2T+1$ be the size of the window $\cT$.

In the searching for inverse filter framework, if we look for an approximate inverse filter $w$ so that $w*Y$ is sparse, then we could formulate the problem as 
\[
 \begin{array}{ll}
 \underset{w\neq 0}{\mbox{maximize}}   & \|w*Y\|_{\ell_0(\cT)}
\end{array}
  \]
  
First, we could do convex relaxation of the $\ell_0$ norm, replacing it with the $\ell_1$ norm we have a convex objective.

Second, we need to fix the scale of $w$ to break the scale symmetry.

For a given matrix $A$, we set up the following optimization problem to fix the scale of $w$:
\BEQ
 \begin{array}{ll}
 \underset{w}{ \mbox{minimize} }   & \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
\mbox{subject to}  
& \|Aw\|_\infty =1, 
\end{array}
% \tag{$P_{v}^T$ }
\EEQ

This is equivalent to finding the minimum objective solution out of $k$ convex optimization problems:

\BEQ
 \begin{array}{ll}
 \underset{w}{ \mbox{minimize} }   & \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
\mbox{subject to}  
& A_i w =1, \|Aw\|_\infty \leq 1, 
\end{array}
% \tag{$P_{v}^T$ }
\EEQ

In the case of perfect shift symmetry of convolution (circular convolution for finite observation or linear convolution on double infinite sequence), when $A$ is a circular matrix with the first column vector  
$\tilde{a}$
, then we only need to
solve one convex problem.
 $w$:
\BEQ
 \begin{array}{ll}
 \underset{w}{ \mbox{minimize} }   & \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
\mbox{subject to}  
& (\Tilde{a}*w)_0 =1, 
\end{array}
% \tag{$P_{v}^T$ }
\EEQ



 This formulation is a convex formulation for the $\ell_\infty$ box constraint with a fixed location of largest entry under shift:
Based on the fact that $a^{-1}*a = e_0$, we know $(a^{-1}*a)_0 = 1$ is a constraint on the largest entry. It would be an oracle constraint if we know $a$. In practice, we could choose an initial guess  $\Tilde{a}$ of the forward filter.


% The $\ell_1$ norm or $\ell_2$ norm ball would still led to 



% If $G$ is some sub-Gaussian distribution instead, then we called it \emph{Bernoulli$(p)$-sub-Gaussian} model.
\subsection{Phase transition theorem for blind deconvolution
}
\paragraph{Random model for sparse signals}
For better theoretical analysis, we define a random model for sparse signals. Let $(X_t)$ be an independent
sequence of random variables indexed by $t \in Z$, with a symmetric distribution with CDF $F_t$, such that $F_t(x) = 1 - F_t(-x)$. 
And we assume $F_0$ has an atom at $0$, $F_0 = (1-p) H +p G$, where $H$ is the Heaviside distribution and $G$ is the standard Gaussian distribution, we called it the \emph{Bernoulli$(p)$-Gaussian} model. 

\paragraph{Surprising phase transition for sparse blind deconvolution with convex optimization}

The convex optimization problem exhibits a phase transition phenomenon for a ideal sparse signal modeled by random sparse process with independent entries. 

To demonstrate the flavor of the phase transition, we present the population phase transition theorem for the special case when the forward filter is $(\ldots,s^3, s^2,s, 1 )$ with $|s|\leq 1$, then the inverse filter is a basic short filter  $a^{-1} = ( -s, 1 )$. 
\begin{theorem}
For a process $Y = a * X$ with
\BIT
\item
$a = (\ldots,s^3, s^2,s, 1 )$ then $a^{-1} = ( -s, 1 )$ where $|s|\leq 1$; and
\item 
$X_t$ IID sampled from the \emph{Bernoulli$(p)$-Gaussian} distribution 
$p N(0,1) +(1-p) \delta_0$.
\EIT
 Let $w^\star$ be the solution of the convex optimization problem 
 \[
 \begin{array}{ll}
 \underset{w }{\mbox{minimize}}   & \Expect|(w*Y)_0|\\
\mbox{subject to}  & w_0 =1;
\end{array}
% \tag{$BD_{e_0}$ }
  \]
 then  there exists a threshold
\[
p^\star  = 1-|s| ,
\]
$w^\star$ is $a^{-1}$ up to shift and scaling provided $p<p^\star$, and $w^\star$ is not $a^{-1}$ up to shift and scaling provided $p> p^\star$.
  \end{theorem}
  
Then we could empirically verify the phase transition, by repeatedly running the finite-sample experiments with independent randomness and count the probability of successful recovery of the true inverse filter $a^{-1}$ and sparse signal $X$.
The resulting plot of success probability is in figure~\ref{fig-PT-finite}, where we get a phase transition line (logistic-regressed $50\%$ success probability line). Indeed $p^\star  = 1-|s|$.
\begin{figure} 
\centering
\includegraphics[width=.8\textwidth]{./figures_BD/PT_BD_1root_none.png}
\caption{ The finite sample phase transition diagram when ground truth filter is $w^\star = (-s,1,0)$ with $T=200$. Here the horizontal axis is sparsity level $p$ ranging from $0.01$ to $0.99$, the vertical axis is $|s|$, ranging from $0$ to $0.99$.  The red region is failure and the blue region is success. }
\label{fig-PT-finite}
\end{figure}


\paragraph{Phase transition for sparse blind deconvolution with general filter}
Now we calculate the phase transition condition of blind deconvolution of general inverse filter.
	\begin{theorem}
	For a process $Y = a * X$ with
$X_t$ IID sampled from the \emph{Bernoulli$(p)$-Gaussian} distribution 
$p N(0,1) +(1-p) \delta_0$.
 Let $w^\star$ be the solution of the convex optimization problem 
 \[
 \begin{array}{ll}
 \underset{w }{\mbox{minimize}}   & \Expect|(w*Y)_0|\\
\mbox{subject to}  
& w_0 =1,
\end{array}
% \tag{$BD_{e_0}$ }
  \]
 then  there exists threshold $p^\star$ determined by
\[
\frac{p^\star}{1-p^\star}=  \inf_{\| \beta\|_2=1, u^T \beta =0} \tan(\angle( \beta_{(0)}, -e_0)) V_1(\beta_{(0)})
\]
 $w^\star$ is $a^{-1}$ up to shift and scaling provided $p<p^\star$,
and  $w^\star$ is not $a^{-1}$ up to shift and scaling provided $p> p^\star$.

The threshold $p^\star$ satisfies 
		\[ 
\tan(\angle( P_u^\perp (-e_0), -e_0)) p^\star \leq \frac{p^\star}{1-p^\star} \leq	\tan(\angle( P_u^\perp (-e_0), -e_0)) V_1(P_u^\perp (-e_0))
		\]
	\end{theorem}

The proof of this theorem is given in the later section. 
To understand the phase transition, we will look at  the population version of the problem.



We could reformulate this theorem into a theorem above stochastic angle:

	\begin{theorem}
 Let the true inverse filter be $a^{-1}$ of length $k$, the angle distance between initialization and ground truth be $\theta$.
% $$\theta = \min_{i,j} \angle(\bar{A_i}*a^{-1}, e_j )$$
For $N$ samples of $X \overset{iid}{\sim} p N(0,1) +(1-p) \delta_0$, if $N \geq  O(k\log(k)),$ \\ then  with probability $1-e^{-CN}$, the solution $w^\star$ of $C_{A}^{\infty}$ satisfies 
$$
  \begin{cases}
w^\star =a^{-1}& \theta \geq \theta^\star(p) \\
w^\star \neq a^{-1}& \theta < \theta^\star(p)
\end{cases}
$$
	\end{theorem}

\section{A fundamental phase transition for blind deconvolution and dictionary learning (also called sparse projection pursuit) :  }
In this section, we will show that after change of variables, the population version of blind deconvolution is the same as the population version of sparse projection pursuit, which is a convex formulation used for dictionary learning or sparse blind source separation. 

Therefore, the phase transition phenomenon presented above is a fundamental phase transition that works for a simple but fundamental population convex problem.

% convex formulation of sparse projection pursuit, also called dictionary learning or sparse blind source separation.

\paragraph{Change of variable for  convex sparse blind deconvolution}
We could rewrite the population version of our convex sparse blind deconvolution problem, with the population objective 
$\Expect\frac{1}{N} \| w*Y\|_{\ell_1(\cT)} =\Expect|(w*Y)_0|=\Expect|(w*a*X)_0|$ due to  the ergodic property of stationary process and shift invariance. Then the convex problem becomes 
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|(w*a*X)_0|\\
\mbox{subject to}  
& ((\alpha*a^{-1})*(a*w))_0 =1,
\end{array}
 \]
Let $\psi$ be the flipped version of $a*w$, such that $\tilde{\psi} := a*w$, then 
 $(w*Y)_0 = (w*a*X)_0 = (\tilde{\psi}*X)_0 = \psi^T X.$  
  Let $u:= \alpha*a^{-1}$. 
 Now we arrive at a simple and fundamental  population convex problem: 
 \[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1.
\end{array}
\tag{$P_{u}$ }
  \]
In the following, we show that this population convex problem is also the population convex problem of sparse projection pursuit after change of variables.

\paragraph{Sparse projection pursuit and dictionary learning}
Sparse projection pursuit is the problem of finding  one sparse element $d^T Y$ each time from a high dimensional data matrix $Y\in \reals^{n\times M}$. Here $Y= D X$ is a matrix product of dictionary $D\in \reals^{n\times d}$ and sparse coefficient $X\in \reals^{d\times M}$. 

The projection pursuit problem was studied in \cite{friedman1974projection,friedman1981projection,friedman1987exploratory,huber1985projection,jones1987projection}. It is also related to blind source separation, independent component analysis (ICA) and the cocktail-party problem.
In the case of an orthogonal dictionary $D$, we could simply transform the problem into finding its inverse $D^{-1} = D^T$, such that $D^T Y = X$ sparse. A work by Daniel Spielman and John Wright\cite{spielman2012exact} used sparse projection pursuit formulation to find the orthogonal basis of $D$ one-by-one, by proposing a set of rule to select the initial guess $v$ and give theoretical guarantee of the convex method. In this work, due to this common population problem, the phase transition phenomenon would also be applicable to dictionary learning, as the first phase transition result for dictionary learning.

The sparse projection pursuit formulation is to solve the following linear-constrained convex optimization problem for some vector $v$:
\[
 \begin{array}{ll}
 \underset{q }{\mbox{minimize}}   & \frac{1}{M}\|q^T Y\|_{1}\\
\mbox{subject to}  & v^T q =1.
\end{array}
  \]
 
%   In the case of other dictionary $D$, the convolutional dictionary learning problem, also called convolutional sparse coding, could all be solved by  
  
The population version is 
\[
 \begin{array}{ll}
 \underset{d }{\mbox{minimize}}   & \Expect|q^T D X|\\
\mbox{subject to}  & v^T q =1.
\end{array}
  \]
We could also do a change of variable by assuming $\psi:= D^T q$, $u:=D^T q$, then the population sparse projection pursuit also becomes
   \[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  & u^T \psi =1.
\end{array}
\tag{$P_{u}$ }
  \]
Without loss of generality, we could assume $\|u\|_2=1$ by rescaling.
  
  
  
  
  
  
% \paragraph{Ratio of norm formulation for blind deconvolution}
% First, from the paper \cite{donoho1981minimum}, we know that we could minimize the ratio of norm of $X$ to recover $X$.

% For example, \cite{donoho1981minimum,wiggins1978minimum} propose to study $(\ell_{2k}/\ell_2)$ problem for $k=2, 3, 4,\ldots$.
% \begin{eqnarray*}
%     (\ell_{2k}/\ell_2) \qquad  \max&    \frac{1}{N} \| w*Y\|^{2k}_{\ell_{2k}(\cT)}\\
%     \mbox{ subject to }&   \frac{1}{N} \| w*Y\|^2_{\ell_2(\cT)} \geq 1.
% \end{eqnarray*}


% For $\ell_1/\ell_2$ ratio, we propose to use a non-convex (convex objective concave constraint) problem for blind deconvultion:
% \begin{eqnarray*}
%     (\ell_1/\ell_2) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&   \frac{1}{N} \| w*Y\|_{\ell_2(\cT)} \geq 1.
% \end{eqnarray*}

% Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} \geq 1.
% \end{eqnarray*}

% Leverage translation invariance, WLOG, we assume that the $0$-index achieves the maximum in absolute value, then  $  \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} =  \frac{1}{N}(w*Y)_0 =  \frac{1}{N}\Tilde Y^T w.$

% Then we have
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N}\Tilde Y^T w = 1.
% \end{eqnarray*}


\paragraph{General phase transition for projection pursuit}
Now we state the general phase transition with light assumption. Here we don't need to even assume that $X$ are independent, we just need to know the existence of one sparse element $X_0$.

\begin{theorem}[Projection pursuit to find a sparse element]
Given a sequence $\{X_t\}_{t\in \integers}$ where one element $X_0$ is a sparse element with $p G + (1-p) \delta_0$ for a symmetric distribution $G$.
Let $\psi^\star$ be the solution of  $P_{u}$:
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1
\end{array}
\tag{$P_{u}$ }
  \]
then there exists a threshold
$
p^\star
$,
$\psi^\star = e_0$ provided $p<p^\star$,
and  $\psi^\star \neq e_0$ provided $p> p^\star$.

Here $p^\star$ is determined by $G$, the distribution of $\{X_t, t\neq 0\}$ and the direction of $u$:
  \[
  \frac{p^\star}{1-p^\star} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]\|\beta_{(0)}\|_2} \tan(\angle( \beta, -e_0))
  \]
 where $\beta_{(0)}$ is $\beta$ with the $0-$th entry deleted.
   

  \end{theorem}

\begin{proof}
The phase transition condition proof is based on  calculating the directional derivative.

First, we want to find a threshold $p^\star$ such that for all $p<p^\star$, the directional derivative at $\psi = e_0$ is non-negative along all direction $\beta$ on unit sphere such that $u^T \beta =0$:
	 \[
	 \nabla_{\beta}{\Expect|(e_0+\beta)^T X|}\geq 0
	 \]
Second, we calculate $\nabla_{\beta}{\Expect|(e_0+\beta)^T X|} $ based on whether $X_0$ is zero or not:
	 \[
	 \begin{array}{ll}
	     \nabla_{\beta}{\Expect|(e_0+\beta)^T X|} = p \beta_0 \Expect[|X_{0}| \mid X_0 \neq 0]  + (1-p) \Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]
	 \end{array}
	\]
It is non-negative in case either $\beta_{0} > 0$, or in case $\beta_0 < 0$ and
	\[
	\frac{p}{1-p} < \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]||\beta_0|}
	\]
	for all $\beta \in \{\| \beta\|_2=1, u^T \beta =0\}$.
% 	\item
$p^\star$ is the least upper bound of all $p$ satisfying this inequality. 
Therefore,  
	\[
	\frac{p^\star}{1-p^\star} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]|\beta_0|} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]\|\beta_{(0)}\|_2} \tan(\angle( \beta, -e_0))
	\]
\end{proof}



\paragraph{Special case: geometric phase transition condition for sparse Bernoulli Gaussian $X_0$ and Gaussian $\{X_t, t\neq 0\}$}

Now we study the implication of the general phase transition problem in a simplest projection pursuit case, where $X_t$ are independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ and the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$.

\begin{theorem}
Let $X_t$ be independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$.
Let $\psi^\star$ be the solution of  $P_{u}$:
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1
\end{array}
\tag{$P_{u}$ }
  \]
then there exists a threshold
$
p^\star
$,
$\psi^\star = e_0$ provided $p<p^\star$,
and  $\psi^\star \neq e_0$ provided $p> p^\star$.

Here $p^\star$ is determined by the direction of $u$:
  \[
  \frac{p^\star}{1-p^\star} = \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0)) = \cot(\angle(u, e_0))
  \]
  \end{theorem}
\begin{proof}
First, when the rest of $X_t, t\neq 0$ is independent of $X_0$, and IID sampled from $ N(0,1),$
	\[
 \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\|\beta_{(0)}\|_2} = 
\sqrt{\frac{2}{\pi}}
\]
Since  
\[
	 \Expect[|G|] = \sqrt{\frac{2}{\pi}},
	 \]
we have a simple phase transition condition that is completely geometric.
	 \[
  \frac{p^\star}{1-p^\star} = \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0))
  \]
 
Second, we know that there is a geometric structure:
\[
\inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\|\beta_{(0)}\|_2}{|\beta_0|}
= \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0)) = \cot(\angle(u, e_0)),
\]
as indicated by figure~\ref{fig-Angle}. 
When $\beta = P_u^\perp (-e_0)$,
	\[
	\begin{array}{ll}
	\inf_{\| \beta\|_2=1, u^T \beta =0} 
		\tan(\angle( \beta, -e_0)) 
		&=
		\tan(\angle( P_u^\perp (-e_0), -e_0)) \\
		&= \cot(\angle(u, e_0)).
	\end{array}
	\]
	
Therefore, $ \frac{p^\star}{1-p^\star}  = \cot(\angle(u, e_0)) $,
	

% \begin{figure} 
% \centering
% \includegraphics[width=.8\textwidth]{./figures_BD/Angle_Diagram_label.png}
% \caption{Demonstration of relation between
%   $\angle( \beta, -e_0)$ and ${\angle(u, e_0)}$}
% \label{fig-Angle}
% \end{figure}
\end{proof}
    
\begin{figure} 
\centering
\includegraphics[width=.8\textwidth]{./figures_BD/Phase_T_sine_p.png}
\caption{The population phase transition diagram of $ \frac{p^\star}{1-p^\star}  = \cot(\angle(u, e_0)) $ for the special case when $X_t$ is independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ and the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$. The red region is failure, and the blue region is success. }
\label{fig-PT-project}
\end{figure}




==> old_sec/sec_old_2020/Inverse.tex <==

\section{Analysis of the inverse kernel method}
\subsection{Inverse kernel approximation}
Now we consider a setting where there is a kernel whose corresponding the inverse kernel is infinite, and we give a finite length approximation. 
We assume that $a =  (a_{-t},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t) = \delta_0 + a_L + a_R$ 
is a length $ l= 2t+1$ filter, 
  and $\sum_{i\neq 0} |a_i|\leq M < 1$.    
 \begin{theorem} 
For a kernel $a = (a_{-s},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t)$ of length $l=1+s+t$, if 
\[
\sum_{i\neq 0} |a_i|\leq M < 1,
\]
 then there exists an approximate inverse kernel $w^r$ of length $rl$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M),\\
\end{array}
  \]
\end{theorem}
\begin{proof}
Consider the $z$ transform of $a$ to be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
let $\bar A(z) = 1-A(z)$, then 
from the condition 
$\sum_{i\neq 0} |a_i|\leq M < 1$,
we define $M' $ to be the maximum absolute value of $\bar A(z)$ on unit circle, as
\[
 \begin{array}{ll}
\mbox{maximize}   & |\bar A(z)| \\
\mbox{subject to}  & z\in \complex,|z|=1.
\end{array}
  \]
Then 
\[
 \begin{array}{ll}
M' \leq \sum_{i\neq 0} |a_i|\leq M<1.
\end{array}
  \]
The Z-transform of the inverse kernel of $a$ is defined by
\[
 \begin{array}{ll}
1/A(z) &=  (1-\bar A(z))^{-1},\\
&= 1+ \sum_{i=1}^{\infty} (\bar A(z))^i
\end{array}
  \]
 The infinite series absolutely converge on $|z| = 1$ because $|\bar A(z)|\leq M<1$.
Let the finite approximation of level $r$ of $w = a^{-1}$ be $w^r$, 
 its Z-transform is  $\sum_{i=0}^{r} (\bar A(z))^i$,
its length is at most $r(s+t+1)$, 
the $j$-th term of $w^r$ is $\sum_{b}bj_i=j \prod_{i} a_i^{j_i}$.
We have that for all  $|z| = 1$,
 \[
 \begin{array}{ll}
|1/A(z) - \sum_{i=0}^{r} (\bar A(z))^i | 
&= |\sum_{i=r+1}^{\infty} (\bar A(z))^i|\\
&\leq M^{r+1}/(1-M).
\end{array}
  \]
Therefore, 
   \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]
%   \[
%  \begin{array}{ll}
% \|a*w^r - e_0 \|_{1} &= \|a*(w^r - w) \|_{1}\\
% &\leq \|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} \\
% &\leq M^{r+1}/(1-M) \\
% &= M^{r+1}(1+M)/(1-M)
% \end{array}
%   \]
 
\end{proof}

Using this inverse approximation, we know for any kernel $a$ of length $l$ with possibly infinite inverse kernel $w$, there exists a length-$rl$ approximate inverse kernel $w^r$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]

Therefore, we can prove the following theorem on sparse blind deconvolution algorithm. 


\paragraph{Simple example.}
We consider a simple example, when $a = (0,\ldots, 0, 1, r, 0, \ldots, 0) = \delta_0 - r\delta_1$, $|r|<1$. Then $a^{-1} = \delta_0 + \sum_{j=1}^\infty  r^j \delta_j.$ Now our data generation model is $y = a*x.$ 

We analysis the optimization problem 
 \begin{eqnarray*}
    \min_{f_0 = 0} &    
    E_x\| (\delta_0+f)*a*x\|_1.
\end{eqnarray*}
Here $f = (0, 0, f_R)$ is in a $K$ dimensional subspace of the double infinite sequence.

% We also analysis the constrained optimization problem 
%  \begin{eqnarray*}
%     \min_{f_0 = 0} &    
%     E_x\| (\delta_0+f)*a*x\|_1,
%     \\
%     \mbox{ subject to }&  \|f\|_1\leq C.
% \end{eqnarray*}

For the objective, using IID property of $x$, we only need to analyze
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| .
\end{eqnarray*}
Let $f^*_K$ be the best length $K$ approximation, as the solution of 
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    \| (\delta_0+f)*a\|_2,
\end{eqnarray*}

In this specific example, $f^*_K = \sum_{j=1}^K  r^j \delta_j.$ And $(\delta_0+f^*_K)*a = (\delta_0 - r^{K+1}\delta_{K+1})*(\delta_0 - r^{1}\delta_{1})^{-1}$.
Let $\tilde{x} = (\delta_0 - r^{K+1}\delta_{K+1})*x$, as one approximation of $x$.
Since $x$ is IID symmetric, $ \tilde{x}$ is identically-distributed, symmetric and weakly correlated for $|r^{K+1}|$ small enough, and $\tilde{x}_0, \ldots, \tilde{x}_K$ are independent.

Let 
\begin{eqnarray*} 
\delta_0+h &=& (\delta_0+f)*(\delta_0+f^*_K)^{-1}\\
&=& (\delta_0+f)*(\delta_0 - r^{K+1}\delta_{K+1})
\end{eqnarray*}
then 
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| 
    &=& E_x | ((\delta_0+h)*\tilde{x})_0|\\
&=& E_x | \tilde{x}_0|+\mbox{sign}(\tilde{x}_0)(h*\tilde{x})_0\\
&\approx& 
 |1+  h_{0}| \cdot E |\tilde{x}_0| \cdot (1-\eta)+   \cdot  E{| (h*\tilde{x})_0| } \cdot \eta.
\end{eqnarray*}

Following the same analysis as the phase transition analysis, we have
\begin{eqnarray*}
     \min_\delta &E | ((\delta_0+f)*a*\tilde{x})_0 | \\
    \mbox{ subject to }  &f_{0} = 0.
\end{eqnarray*}


==> old_sec/sec_old_2020/Metric.tex <==
 \subsection{Distance metrics}
% \paragraph{Distances to measure stability}
We care about three types of metrics, first, distance  in $w$ space, between the computed composed filter $w$ and ground truth $a^{-1}$; second, distance in $w$ space, between the computed inverse filter $w$ and ground truth inverse filter $a^{-1}$, second, distance  in $\psi = w*a$ space, between the computed composed filter $w*a$ and ground truth $e_0$; third,  distance  in $x$ space, between recovered signal sequence and true sparse signal sequence. 

First, the MSE in space of $\psi = w*a$,
  \[
 \begin{array}{ll}
d_{\psi,2}^2 := \|\phi\|_2^2 =  \|\psi-e_0\|_2^2= \|a*(w-a^{-1})\|_2^2
\end{array}
  \] 
 The MSE in space of $w$. 
   \[
 \begin{array}{ll}
d_{w,2}^2  = \|w-a^{-1}\|_2^2 = \|a^{-1}*(\psi-e_0))\|_2^2 = \|a^{-1}*\phi\|_2^2
\end{array}
  \]
Last, $\ell_1$ and $\ell_2$ distance in $x$ space:
\[
 \begin{array}{ll}
d_{x,1} &:= \frac{1}{2T+1}\|w*Y-X\|_{1,[-T,T]} =  \frac{1}{2T+1}\|\tilde \phi* X\|_{1,[-T,T]} \\
d_{x,2}^2 &:= \frac{1}{2T+1}\|w*Y-X\|_{2,[-T,T]}^2 = \frac{1}{2T+1}\|\tilde \phi* X\|_{2,[-T,T]}^2
\end{array}
  \]
We compute their expectation: 
\[
 \begin{array}{ll}
\Expect d_{x,1}  &=  \Expect|\phi^T X| = \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2\\
\Expect d_{x,2}^2 &=  \Expect|\phi^T X|^2 = p \|\phi\|^2  = p \|\psi-e_0\|^2 
\end{array}
  \]  
We remark that in the following we focus on distance in $x$ space to recover the signal. 

% And using the fact that $\Expect d_{x,1}= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2$ and $\Expect d_{x,2}^2 = p \|\phi\|^2$, we focus on calculate 
% \BIT
% \item $\Expect d_{x,1} \propto  \Expect_I \|\phi \cdot I\|_2$
% \item $\Expect d_{x,2}^2 = \Expect_I \|\phi \cdot I\|_2^2 = p\|\phi\|^2  = p d_{\psi,2}^2$ 
% \EIT



==> old_sec/sec_old_2020/Noise.tex <==
\section{Stability for noisy observation}


\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]
\subsection{Stability for adversarial perturbation of sparse signal }
\paragraph{Mathematical formulation: sparse signal plus adversarial perturbation}

\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
$Z$ is a unit vector in $2$ sphere. 
\item
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
\Expect|(w*Y)_0|
&= \Expect|\psi^T (X+\eta Z )| \\
% &= \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
\end{array}
  \]

  
  
  
 \paragraph{Study the noisy problem}
Under the data generative model, 
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
    the constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta}   & \Expect|\psi^T (X+\eta Z ) - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
  
\paragraph{Worst case objective over $Z$}  
For the constrained problem, we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
  \]
Which is equivalent to 
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
In the following we study the min-max objective
  \[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi) : = \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| 
\end{array}
  \]
  
\paragraph{Robust optimization}
Let the deterministic residual function of $\psi, Z, \zeta$ be
\[
\mu_{\eta, \epsilon}(\psi, Z, \zeta): = \eta  \psi^T Z  - \epsilon \zeta
\]
We reparametrize $\epsilon$ as by defining 
\[
\tau :=  \frac{\epsilon}{\eta}
\]
then 
\[
\mu_{\eta, \epsilon} = \eta ( \psi^T Z  - \tau \zeta)
\]






\begin{lemma}
For any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, $Z$ is along the direction of $s\psi$ so that $s\psi^T Z = \|\psi\|_2$.

\end{lemma}  


\begin{lemma}[Hölder's inequality]
For any given sign $s =\pm 1$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $s|\psi|^q$ so that $s\psi^T Z = \|\psi\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
The min-max quantity  
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2 = (\eta \|\psi\|_2  - \epsilon )_+^2 = \eta^2 ( \|\psi\|_2  - \tau )_+^2
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}^2 
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2\\
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} [(\eta  \psi^T Z)^2+  (\epsilon \zeta)^2 - 2(\eta  \psi^T Z)(\epsilon \zeta)]\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \sup_{Z: \|Z\|_2\leq 1} [ (\psi^T Z)^2] + 2\eta \epsilon |\zeta|   \sup_{Z: \|Z\|_2\leq 1}[ (-\sign(\zeta) \psi^T Z)]\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \|\psi\|_2^2 + 2\eta \epsilon |\zeta|   \|\psi\|_2\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{  (\eta \|\psi\|_2  - \epsilon |\zeta| )^2\}\\
&= (\eta \|\psi\|_2  - \epsilon )_+^2
\end{array}
\]
The fourth equation is because for any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_2\leq 1}(s \psi^T Z) = \|\psi\|_2.
\]
\[
\sup_{Z: \|Z\|_2\leq 1}( \psi^T Z)^2 = \|\psi\|_2^2.
\]



\end{proof}

We have the following result, generalizing $\|Z\|_2\leq 1$ to $\|Z\|_p\leq 1, \quad, p\geq 1$, and then to $Z\in K$ for a closed compact convex set $K\in \reals^N$.



\begin{lemma}
\label{min-maxErrorL_p}
The min-max quantity 
for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates,
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_p\leq 1} F( \eta (\psi^T Z  - \tau \zeta)) = 
F(\eta( \|\psi\|_q  - \tau )_+)
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}

\begin{coro}
 \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_2  - \tau )_+|
\end{array}
  \]
  in general, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_p\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}


\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then for any constant $\mu$, using the rotation invariance of Gaussian, $\psi^T X +\mu$ is  Gaussian with mean $\mu$ and standard deviation $\|\psi_I\|_2$, therefore,
\[
|\psi^T X +\mu |
\]
following the folded Gaussian distribution.
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}

From general theory of folded Gaussian $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
hence
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
\end{array}
\]

\end{lemma}
\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}







==> old_sec/sec_old_2020/Noise2.tex <==

% \paragraph{Bound on min-max objective}

% First of all, we find a lower and upper bound that is true independent of the distribution of $X$.
% \begin{lemma}
% Let $\psi^T X $ be fixed, we have upper and lower bound on the constrained problem objective:
%  \[
%  \begin{array}{ll}
% \sup_{s=\pm 1}|(\psi^T X +s\eta \|\psi\|_2  - \epsilon)_+| \leq
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} |\psi^T X +\eta  \psi^T Z  - \epsilon \zeta| 
% \leq |\psi^T X | +|(\eta \|\psi\|_2  - \epsilon)_+ |
% \end{array}
%   \] 
% \end{lemma}  
% \begin{proof}
% Let $A:=\psi^T X $ be fixed
% First, if we let $Z$ be along the direction of $s\psi$, we have a lower bound on the objective for both $s =\pm 1$,
%   \[
%  \begin{array}{ll}
%   \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| 
% \geq
%  |A +\eta s\|\psi\|_2  - \epsilon \zeta|
% \end{array}
%   \] 
%   Therefore, we can 
%   \[
%  \begin{array}{ll}
%  &\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \geq&
% \inf_{\zeta: \zeta^2 \leq 1} |A +\eta s\|\psi\|_2  - \epsilon \zeta|\\
% =&
%  |(A +s\eta \|\psi\|_2  - \epsilon)_+|
% \end{array}
%   \] 
% Second, if we let $ \sign(\eta  \psi^T Z  - \epsilon \zeta) = s'$ then
%   \[
%  \begin{array}{ll}
%  & \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \leq&
% \inf_{\zeta: \zeta^2 \leq 1}  \sup_{Z: \|Z\|_2\leq 1}   (|A |+ |\eta  \psi^T Z  - \epsilon \zeta|) \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} |\eta  \psi^T Z  - \epsilon \zeta| \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\sup_{Z: \|Z\|_2\leq 1} [\eta  s'\psi^T Z]  -s' \epsilon \zeta\} \\
%     =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\eta \|\psi\|_2  -s' \epsilon \zeta\} \\
%   =&
%   |A | +|(\eta \|\psi\|_2  - \epsilon)_+ |\\
% \end{array}
%   \] 
  
% \end{proof}
\paragraph{Folded Gaussian mean and asymptotically tight lower bound}
Now we exploit the property of folded Gaussian mean, and we find an exact asymptotic formula.
For simplicity of expression, we also define the deterministic residual function of $\psi, I$ to be
\[
\gamma_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}(\psi, Z, \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\psi\|_2 - \tau)_+}{\|\psi_I\|_2}
\]

\begin{coro}
\label{Cor:PerturbedObjectiveLowerBound}
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)
&= \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| \\
&= \sqrt{\frac{2}{\pi}}  \Expect_I \left[ \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I \left[\|\psi_I\|_2(1 + \frac{3}{2}\gamma_{\eta, \epsilon}^2 + \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma_{\eta, \epsilon}^6)\right]
\end{array}
\]
As $\gamma_{\eta, \epsilon}^2<1,$ 
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)-L_{0, 0}(\psi)
&\geq 3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}(\psi)^2\Expect_I \|\psi_I\|_2^{-1}
\end{array}
\]
\end{coro}
% \begin{proof}
% In the following proof, for clarity, we write $\gamma_{\eta, \epsilon}$ simply as $\gamma$.

% Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
% we have
% \beq
% \label{FoldedGaussianMean_Obj}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| = \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]
% \eeq
% Then we can plug in the lemma \ref{ExpansionMeanFoldedGaussian}.
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \{ 1- \frac{\gamma_{\eta, \epsilon}^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \sqrt{\frac{2}{\pi}}\Expect_I  \left[ \|\psi_I\|_2 
% \{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2_{\eta, \epsilon}))\gamma_{\eta, \epsilon}^2 +   \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} \}\right]\\
% \end{array}
% \] 
% Here the residual of this expansion after first order is
% \[
%  \begin{array}{ll}
% \mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2_{\eta, \epsilon})-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!} \\
% &=    \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma^6)
% \end{array}
% \] 
% From the lower bound in lemma \ref{ExpansionMeanFoldedGaussian}, we have that when $\gamma_{\eta, \epsilon}^2<1, \mbox{Res}(\gamma^2)\geq 0$
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}\mu_{\eta, \epsilon}^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \] 
% Now we could plug in lemma~\ref{min-maxError} to prove the last equation.
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \]
% \end{proof}









% We branch out to show a low-hanging result for the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem}.
% \begin{coro}
% For
% the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem} with min-max lower bound as objective
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]
%  If $\epsilon \geq \eta,$ then the minimizer is $1$-sparse vector $e_i$, the same as the minimizer of 
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]

% \end{coro}


  \paragraph{Calculate the robust objective at $e_0$}
First, at $\psi = e_0$, $X_0 =e_0^T X = I_0 G_0$, where $G_0$ is standard normal, $I_0$ is Bernoulli, we take expectation over $I_0$ first, 
Let 
 \[
 \mu_0 :=  \mu_{\eta, \epsilon}(e_0) = \eta ( 1-\tau)_+ 
 \]
 When $\epsilon\geq \eta,$ $\mu_0=0$; when $\epsilon< \eta,$ $\mu_0>0$.
 \begin{lemma}
  \label{Lemma:ObjectiveDiffAtEzero}
     \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
 \end{lemma}
%   \begin{lemma}
%   \label{Lemma:ObjectiveRatioAtEzero}
%      \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &=  [(1-p)\mu_0\sqrt{\frac{\pi}{2}}  + p  (e^{-\frac{\mu_0 ^2}{2}} )+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)]/p
% \end{array}
%   \] 
%  \end{lemma}
 
 \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveDiffAtEzero}]
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&= \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}\Expect |X_0+\eta   Z_0  - \epsilon \zeta|-\Expect | X_0| \\
&= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|-\Expect | X_0| \\
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
 \end{proof}
%   \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveRatioAtEzero}]
%   Using lemma~\ref{ExpansionMeanFoldedGaussian}, let $\gamma = \eta ( \|e_0\|_2-\tau)_+/B_0,a$
%     \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|/\Expect | X_0|\\

% % \Expect_I |(e_0)_I+\eta ( \|e_0\|_2-\tau)_+|/\Expect_I | (e_0)_I| 
% % &=  \sqrt{{\pi}\frac{2}} (1-p)\mu_0  + p (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
% % &= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
% \end{array}
%   \] 
% The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
%  \end{proof}
 
 
We observe that 
\BIT
\item
if $\tau\geq 1$,   $( 1-\tau)_+ = 0$, then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) = 0;$
\item
if $\tau < 1$ , then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) \approx (1-p)\mu_0  + p O(\mu_0^2).$
\EIT

  
  \paragraph{Bound $\|\phi^\star\|_2$ using the difference of objective }
   Now use the change of variable that $\psi =e_0+\phi$,
   the constrained problem becomes
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & L_{\eta, \epsilon}(e_0+\phi) \\
\mbox{subject to}  
&u^T \phi =0
\end{array}
  \] 
First, we assume the minimizer is $\phi^\star$. Since $e_0$ is  minimizer of $L_{0, 0}$ and $e_0+ \phi^\star$ is  minimizer of $L_{\eta, \epsilon}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star) 
 \geq L_{0, 0}(e_0+\phi^\star)
 \geq L_{0, 0}(e_0) 
\end{array}
  \] 

Remark: This chain is true for all  $\phi^\star$ that $L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star),$ we can pick a dense sequence converging to $\phi^\star$ in $\ell_2$ norm)  
  
 Then using the fact that $L_{\eta, \epsilon}(e_0) -L_{\eta, \epsilon}(e_0+\phi^\star) \geq 0,$ we have
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
 \geq   [L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)]+ 
 [L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) ]
\end{array}
  \]   
  
 Notice that 
      \[
 \begin{array}{ll}
 L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)  = \Expect |(e_0+\phi^\star)^T X| - \Expect |(e_0)^T X| 
 = \sqrt{\frac{2}{\pi}} B(p,N)  \|\phi^\star\|_2
\end{array}
  \] 
  where $N = \|\phi^\star\|_0$, since $\phi^\star$ is dense due to our assumption, we have .
    \[
  \lim_{N \rightarrow \infty } B(p,N) = B(p,\infty) =  [ p (-\cot{\theta}) + (1-p)].
  \]
  if $p<p^\star$, $\lim_{N \rightarrow \infty } B(p,N) > 0.$
 
\begin{theorem}


\label{Thm:StabilityMSE}
When $\epsilon\geq \eta,$ and $p<p^\star$, then
$\|\phi^\star\|_2 =0$, the minimizer of the min-max problem is exactly $\psi^\star = e_0.$
 
 When $\epsilon< \eta,$  and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B(p,\infty)\right) \|\phi^\star\|_2 
 &\leq& 
 \left(L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)\right)-\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)\\
  &\leq&  \left(  (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4) \right) - 
  \left(  3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}((e_0+\phi^\star))^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} \right)\\
    &\leq& 
    (1-p)\mu_0  +  
    3\sqrt{\frac{1}{2\pi}}\left(  p \mu_0 ^2- \mu_{\eta, \epsilon}((e_0+\phi^\star))^2 \|e_0+\phi^\star\|_2^{-1} \right) + O(\mu_0 ^4)
 \EEAS
\end{theorem}
\begin{proof}
The first inequality comes from the chain of inequality between objectives. 

The second inequality combines the previous calculation of $L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)$ with lemma~\ref{ExpansionMeanFoldedGaussian} and lemma~\ref{Lemma:ObjectiveDiffAtEzero}.

For the last inequality comes from lemma~\ref{TaylorSqrtInvExpect}, 
\[
\frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}} \geq 1 .
\]
\end{proof}

\paragraph{Interpretation}
For simplicity, we focus on the case when the optimization problem is the original one where $\epsilon = 0$,
then 
\[
 \mu_{\eta, 0}(e_0) = \eta.
\]
\BIT
\item
We comment that when our optimization constraint is sphere constraint $\|\psi\|_2 =1$, 
then
\[
 \mu_{\eta, 0}(\psi)  = \eta
\]
then
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B_s(p,\infty)\right) \|\phi^\star\|_2 
    &\leq& 
    (1-p)
    [\eta  - 
    3\sqrt{\frac{1}{2\pi}} \eta^2] + O(\eta^4)
 \EEAS

\item
For the case when our optimization constraint is $u^T \phi =0$, 
\[
 \|e_0+\phi^\star\|_2^2= 1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 
 \]
 Since it is dependent on $\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2$, and using the condition $u^T \phi^\star =0$, we could use the same argument as figure~\ref{fig-Angle} and lemma~\ref{Angle_Inequality}, we know that 
 \[
 |\cos{\angle(\phi^\star,e_0)}| \leq \sin\theta
 \]
 therefore,
 \[
 |\frac{\|e_0+\phi^\star\|_2^2 - (1+\|\phi^\star \|_2^2)}{\|\phi^\star \|_2 }| \leq 2\sin\theta
 \]
 \EIT
 
We first have a weak corollary by only using $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)$ and just use loose bound $L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\geq 0.$


\begin{coro}
\label{Cor:StabilityMSE_}
 When $\epsilon< \eta,$ and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \|\phi^\star\|_2 &\leq& (L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0))/(\sqrt{\frac{2}{\pi}} B(p,\infty))\\
 &\approx& 
 \eta \{\sqrt{\frac{\pi}{2}}(1-p) +  \frac{3p}{2}\eta \}/  
 \{ p (-\cot{\theta}) + (1-p)\}+ O(\eta^4)
 \EEAS
\end{coro}  

  To strengthen this bound, we further compute 
$L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) $.

  
\begin{coro}
 When $\epsilon =0,$ and $p<p^\star$, as $\eta\rightarrow 0$, $\|\phi^\star\|_2$  is bounded by a function of $\eta$:
  \BEAS
\|\phi^\star\|_2 
 &\leq& 
 \frac{    (1-p)\{\sqrt{\frac{\pi}{2}}\eta -  \frac{3}{2}\eta^2 )}{   p (-\cot{\theta}) + (1-p) + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} } + O(\eta^4)
 \EEAS 
\end{coro}    
\begin{proof}
Let 
\[
\Gamma_{-1}(e_0+\phi^\star) := \frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}}
\]
From lemma~\ref{TaylorSqrtInvExpect}, we have 
\[
\Gamma_{-1} \geq 1 .
\]
we have
  \[
 \begin{array}{ll}
\sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} 
&= \sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2
\Gamma_{-1}(e_0+\phi^\star)
\end{array}
  \] 
Now we use Taylor expansion,  we could expand $\|\phi^\star \|_2$ around $0$ to first order 
\[
 \begin{array}{ll}
 \|(e_0+\phi^\star)\|_2
&=  (1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{\frac{1}{2}}\\
&= 1+\sum_{\ell=1}^\infty \binom{\frac{1}{2}}{\ell}
[\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)
\end{array}
  \] 
  
 
  
  \BEAS
- \sqrt{\frac{\pi}{2}}\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)
 &\leq& 
 - \frac{3}{2} \eta^2 \Gamma_{-1}(e_0+\phi^\star) (1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\eta^2))
 \EEAS 
 Therefore
  \BEAS
 \left(  [p (-\cot{\theta}) + (1-p)] + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} \right)\|\phi^\star\|_2 
 &\leq& 
 \eta (1-p) \{\sqrt{\frac{\pi}{2}} -  \frac{3}{2}\eta )+ O(\eta^4)
 \EEAS 
% \[
%  \begin{array}{ll}
%  \|(e_0+\phi^\star)\|_2^{-1}
% &=  (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}\\
% &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \]   


  
% \[
%  \begin{array}{ll}
%  \Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}
% &=  \Expect_I(1+\|\phi^\star_I \|_2^2 + \cos{\angle(\phi^\star_I,e_0)}\|\phi^\star_I \|_2)^{-\frac{1}{2}}
% % &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% % [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \] 
 
  

% Therefore,
%  \[
%  \begin{array}{ll}
 
% &  p\sqrt{\frac{2}{\pi}}\left[ \frac{3}{2}\mu_0^2\right]+(1-p)\mu_0
%  \\
% \geq& \frac{3}{2}(\eta \|(e_0+\phi^\star)\|_2  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) \|e_0+\phi^\star\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % =& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}+ B(p) \|\phi^\star\|_2\\
% \end{array}
%   \] 



\end{proof}
 













\subsection{Other setting on $Z$}
\paragraph{ Adversarial outer noise} 
If our generative model is
\[
\begin{array}{ll}
Y&= a* X + \eta_2 Z_2\\
&= a* (X +\eta_2 a^{-1}* Z_2)
\end{array}
\] 
And we consider the worst case objective over $\|Z_2\|_p\leq 1, \quad p\geq 1.$

Let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, then following previous calculation,
\begin{coro}
For $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z_2\|_p \leq 1}  &  \Expect|\psi^T X+\eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|C_{a^{-1}}^T \psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}

Let $C_{a^{-1}}^T \psi =\bar{a}^{-1}*\psi$, where $\tilde{a}^{-1}$ is defined by flipping the coordinate of $a^{-1}$ (reflecting the coordinates around zero by map $i$ to $-i$ for $i\in \integers$.)
 
 We can replace the definition of $\gamma$ and $\mu_0$  by:
 \[
 \gamma^{a}_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\bar{a}^{-1}*\psi\|_q  - \tau)_+}{\|\psi_I\|_2}
\]
\[
\mu_0^{a} := \eta( \|\tilde{a}^{-1}\|_q-\tau)_+
\]
We can get the same result as theorem~\ref{Thm:StabilityMSE}.

% \paragraph{Distributional robust setting}
% When $Z$ following a distribution $P_Z \in \Pi$, where $\Pi$ is a closed convex set in probability simplex for probability defined on $\reals^N$, then our distributional robust objective is
%   \[
%  \begin{array}{ll}
%  \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{P_Z \in \Pi}  & \Expect_Z \Expect_X|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| 
% \end{array}
%   \]
% then 
% for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates, the quantity 
% \[
%  \begin{array}{ll}
%  \sup_{P_Z \in \Pi}  & \Expect_Z F( \psi^T  Z ) 
% \end{array}
% \]
% could be computed following the same approach as the distributional robust Kelly problem if $\Pi$ can be represented by finite combination of atoms.
  

  

\subsection{ Gaussian additional noise}
\paragraph{ Gaussian additional observation inner and outer noise} 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+  \sigma_1 G_1) +  \sigma_2 G_2\\
&= a* (X+\sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\] 
let $C_{a^{-1}}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, then $C_{a^{-1}} = C_a^{-1}$ and 
\[
\begin{array}{ll}
Z: = \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\sim N(0, \sigma_1^2 I_N + \sigma_2^2 C_{a^{-1}} C_{a^{-1}}^T)
\end{array}
\] 
then
\[
\begin{array}{ll}
\psi^T Z
\sim N(0, \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2 )
\end{array}
\] 
 Let $G$ be another standard normal $N(0,I_N)$, for any fixed vector $\mu \in \reals^N, $
 \[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2)  | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  |
\end{array}
  \]
In this case, it seems the previous constrained problem no longer can help us find exact solution $\psi^\star =e_0.$ 



We first study $\sigma_2 = 0$ case.
\[
\Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}G_3 | = 
\sqrt{\frac{2}{\pi}} \cdot \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) =  \sqrt{\frac{2}{\pi}} \cdot \|\psi\|_2 \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma_1^2})
\]
Define worst case objective
\[
F_{\sigma}(\psi):= \sup_{\sigma_1 \leq \sigma} \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) = \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma^2\|\psi\|_2^2})
\]
The second equality comes from monotonicity.

Again, we assume the minimizer is $\psi^\star $. Since $e_0$ is  minimizer of $L_{0}$ and $\psi^\star $ is  minimizer of $L_{\sigma}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\sigma}(e_0)
 \geq F_{\sigma}(\psi^\star ) 
 \geq F_{0}(\psi^\star )
 \geq F_{0}(e_0) 
\end{array}
  \] 
Then
    \[
 \begin{array}{ll}
F_{\eta}(e_0)/F_{0}(e_0)
 \geq (F_{\eta}(\psi^\star )/F_{0}(\psi^\star ))(F_{0}(\psi^\star )/F_{0}(e_0) )
\end{array}
  \] 

   \[
 \begin{array}{ll}
 F_{\eta}(\psi)/F_{0}(\psi) = \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )
\end{array}
  \] 
  
     \[
 \begin{array}{ll}
 F_{\eta}(e_0)/F_{0}(e_0) = \Expect_I(\sqrt{ \frac{\|(e_0)_I\|_2^2}{\|e_0\|_2^2} + \sigma^2})/\Expect_I(\frac{\|(e_0)_I\|_2}{\|e_0\|_2} )= (p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p
\end{array}
  \] 
  
    \[
 \begin{array}{ll}
 F_{0}(\psi)/F_{0}(e_0) 
 &= \Expect_I\|\psi_I\|_2/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+(\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2)/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+ (B(p,N)/\Expect_I\|(e_0)_I\|_2) \|\psi -e_0\|_2\\
 &= 1+ (B(p,N)/p) \|\phi\|_2
\end{array}
  \] 

   \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi\|_2 &\leq (F_{\eta}(e_0)/F_{0}(e_0))/ (F_{\eta}(\psi)/F_{0}(\psi)) \\
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}/\{\Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )\}
\end{array}
  \] 
  First, a loose bound on $\|\phi^\star\|_2$:
  \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi^\star\|_2 
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}
\end{array}
  \] 
We found that
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq (\{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}-1)/(B(p,N)/p) \\
&\leq ((p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})-p)/B(p,N)
\end{array}
  \] 

In general, when $\sigma_1, \sigma_2$ both non-zero, using the same argument,
\[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq \frac{(p[\sqrt{ 1 + \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2}-1]+ (1-p) \sqrt{ \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2})}{B(p,N)}
\end{array}
  \] 

\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Inner and outer Gaussian and adversarial noise together}
When 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
$Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$.

Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
We define our robust objective as   
\[
 \begin{array}{ll}
& F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)\\
:=& 
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2-\epsilon \zeta |
\end{array}
  \]  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  
 
  
  
  
  
  
  
  
  
  
  
  
  
  
% % \paragraph{Mathematical formulation: sparse plus gaussian signal with additional noise}

% % \BIT
% % \item
% % Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
% %  \item
% % The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
% % \item
% % $Z_1$ is IID sampled from  $N(0,I)$, $Z_2$ is IID sampled from  $N(0,I)$, they are independent.
% % \item
% % \[
% % \begin{array}{ll}
% % Y&= a* (X+\sigma_1 Z_1) + \sigma_2 Z_2\\
% % &= a* (X+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)\\
% % &= a* (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \end{array}
% % \]
% % let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, if we condition on $I$ fixed, then 
% % \[
% % \begin{array}{ll}
% % (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \sim N(0, (I+\sigma_1+\sigma_2 C_a^{-1} )(I+\sigma_1+\sigma_2 C_a^{-1} )^T)
% % \end{array}
% % \]
% % then let $\tilde{\psi} := w*a$,  
% % \[
% %  \begin{array}{ll}
% % \Expect|(w*Y)_0|
% % &= \Expect|\psi^T (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)| \\
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% % \end{array}
% %   \]

% % \EIT



% % \paragraph{The original convex problem analysis}
% % We still analyze 
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   & \Expect|(w*Y)_0|\\
% % \mbox{subject to}  
% % & v^T w =1,
% % \end{array}
% %   \]
% %   Which is 
% %   \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   &\sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2\\
% % \mbox{subject to}  
% % & u^T \psi =1,
% % \end{array}
% %   \]
% %   for $u = \tilde{a}^{-1}*v$.
% %  The subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % \partial [\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 ]
% % &= 
% % \Expect_I [N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
% %   the projected subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [
% % N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
  
% %   First the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| (I_0+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| (1+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_1 e_0+\sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
  
%  \paragraph{Study inner Gaussian noise only }
% %  First, we study the case when $\sigma_2 = 0$, $0<\sigma_1<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} | I_0+\sigma_1|
% %  &=p| 1+\sigma_1|+(1-p)| \sigma_1|\\
% %  &=p +\sigma_1
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( e_0\cdot (I+\sigma_1) )]
% % &= P_{u}^{\perp} e_0
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u=e_0$.
  

  
  
  
  
%   \paragraph{Study outer Gaussian noise only }
% %  First, we study the case when $\sigma_1 = 0$, $0<\sigma_2<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| I_0\cdot e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( I_0\cdot e_0+\sigma_2
% %  a^{-1} )]
% % &= P_{u}^{\perp} [p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )]
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u$ is along the direction of $p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )$.
  
  
%   \paragraph{Possible  goal}
%   \BIT
%   \item
%   Show that for minimizer $\psi^*$ of the noisy objective
%   \[
%  \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2 
%   \]
%   is small and bounded by $\sigma_1$ and $\sigma_2$.
  
  
  
%   \begin{lemma}
%   We get the upper bound and lower bound of optimal objective value between the noisy and the noiseless setting
%   \[
%   \Expect_I \|I\cdot e_0\|_2  \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2\leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  
%   \]
%   \end{lemma}
  
%     Now we get the bound of objective value between the noisy and the noiseless setting
%   \begin{lemma}
%   \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  p(\| (1+\sigma_1)e_0+\sigma_2
%  a^{-1}\|_2-1)+(1-p)\| \sigma_1 e_0+\sigma_2
%  a^{-1}\|_2 
%   \]
%     \[
%   \Expect_I \|(I\cdot+\sigma_1)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  \sigma_1
%   \]
%   \end{lemma}
%   \item
%   Describe the minimizer $\psi^*$ of the noisy objective by 
%      \[
%  \begin{array}{ll}
% 0= P_{u}^{\perp} \Expect_I [
% N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^* )]
% \end{array}
%   \]
%   Then find a norm $d$ so that
%   $
%   d(\psi^*, e_0) 
%   $
%   or
%   $
%   d(w^*, a^{-1}) 
%   $
%   is bounded by $\sigma_1$ and $\sigma_2$
%   \EIT
   
   
%  \paragraph{Lemma for expectation}  
%   Mimic the lemma from previous section, we know that 

% \begin{lemma} \label{lem:BGPropLemmaSub}
% \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq  \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
%   \[
%   \bar{B}(k-1;n,p) \cdot \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} + (1- \bar{B}(k-1;n,p)) \cdot \|(\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
% where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
% is the survivor function (Complementary CDF) of the Binomial.
% \end{lemma}



% \begin{lemma} 
% There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
% and so that for each $N$ and for each 
% vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
% \beq \label{eq:LemmObjNoise}
%  (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq 1 + \eps_N .
% \eeq
% \end{lemma}

 
 
 
%  \paragraph{Bound on objective and subgradient}
%   Using the lemma, we could link the objective to $2-$norm of $\phi^* = e_0 + \psi^*$, 
%   \[
%     \begin{array}{ll}
%   \|\psi^*-e_0\|_2 = \|\phi^*\|_2 
%   \end{array}
%   \]
  
  
  

% Define the following notation for function, where $I$ is a fixed support, 
% \[
%  \begin{array}{ll}
% F_1(\phi) &:=   \|(1 +\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F_I(\phi) &:=   \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F^E(\phi)&:= \Expect_I F_I(\phi)   
% \end{array}
% \]
% then
% \[
%  \begin{array}{ll}
% \partial  F_I(\phi) &:= N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi) )\\
% \partial F^E(\phi)&:= \partial \Expect_I F_I(\phi)  =   \Expect_I \partial  F_I(\phi)
% \end{array}
% \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% Using Lebourg’s mean value theorem, Theorem 2.3.7 of Clarke (1990) \cite{clarke1990optimization}, there exists $ t \in (0,1),$ so that
% \[
%  \begin{array}{ll}
% \Expect_I F_I(0) -   \Expect_I F_I( \phi^*)\in \langle  
% \partial \Expect_I F_I( t\phi^*), \phi^* \rangle
% \end{array}
% \]



%   We want to bound the finite difference:
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 } \in \langle  
% \partial \Expect_I F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
    
% % \frac{|\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi^*)\|_2| }{\|\phi^*\|_2 } 
% \end{array}
%   \]
%  And since $t\neq 1$, $\Expect_I N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) )$ is not a set but just a unit vector,
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
  
%   Since $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*)>0$ when the minimizer $\phi^*$ is not $0$, in this case,  a natural bound is
%   \[
%     \begin{array}{ll}
%  0 <  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   More specifically, there exists $\rho>0,$ 
%     \[
%     \begin{array}{ll}
%  \rho \leq  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   Therefore, using the fact that 
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 }  \in [\rho,1]
% \end{array}
%   \]
%  We could bound $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) $ by bound $\|\phi^*\|_2$.
   
   
% For $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
 
 
% We need a new lemma for subgradient, 
% % \begin{lemma} 
% % \beq \label{eq:LemmSubGradNoise}
% % C_{-}'  \leq  \frac{\partial\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\partial\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq C_+' .
% % \eeq
% % \end{lemma} 
 
%  \begin{lemma} 
%  For the minimizer $\phi^*$ so that $u^T \phi^* =0$,
% \beq \label{eq:LemmDirGradNoise}
% C_{-}  \leq  \frac{ \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   }{ \langle   \partial F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%  }  = \frac{\Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]}{\cos[\angle( (1+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]} \leq C_+ .
% \eeq
% \end{lemma} 
% \begin{proof}


% \begin{eqnarray*}
% & & E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   \end{eqnarray*}
 
 
% Using the fact that $\phi^*$ is minimizer,  we know that for any $\beta$ so that $u^T \beta = 0, \|\beta\|_2=1$,
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &\geq& 0
%   \end{eqnarray*}
% where
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &=& E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) ), \beta \rangle
%   \end{eqnarray*}
% It requires
% \begin{eqnarray*}
% 0 \in \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n}  P_{u}^{\perp} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) )
%   \end{eqnarray*}




%   \end{proof}   






















==> old_sec/sec_old_2020/Noise_updated.tex <==
\section{Robustness for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $\zeta_1$ and $\zeta_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 \zeta_1+  \sigma_1 G_1) + \eta_2 \zeta_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 

  
In the following,
let 
\[
D_R( \psi) :=  F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)-F_{0,0,0,0}(\psi).
\]
We use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$

Let $\phi^\star := \psi^\star-e_0$,
we have
   \[
 \begin{array}{ll}
D_R( e_0) &= F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)\\
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,\phi^\star) \|\psi^\star-e_0\|_2\\
 &\geq p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G| = \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
  \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_Monot}
$\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
\end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
\end{lemma}


\paragraph{Robust optimization}
% We want to find the min-max value 
% \[
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta)
% \]
% for a function $H$,
% \[
% H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
% \]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


% \begin{lemma}
% \label{min-maxError}
% For $A>0$, 
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
% \end{array}
% \]
% where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
% \end{lemma}
% \begin{lemma}
% \label{min-maxErrorL_p}
% Let
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
%  \end{array}
%   \]
%   where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
%   then
% \[
%  \begin{array}{ll}
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta) = 
% H( \mu(\psi))
% \end{array}
% \]

% \end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
%  \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
%  \end{array}
%   \]
 \[
 \begin{array}{ll}
 \mu(\psi) &=\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}\\
 \sigma_n^2(\psi) &=  \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}\Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2 |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}[\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
 
 The second inequality comes from the fact that $\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
  
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
For $p<p^\star_1 = 1-\tan(\theta),$
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2\leq 
  \frac{(1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

 
\end{theorem}  
\begin{proof}
 Since
 \[
 \begin{array}{ll}
  B(p,\phi^\star) \|\phi^\star\|_2\leq 
 D_R(e_0) = F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0) 
\end{array}
  \] 
  and
   \[
 \begin{array}{ll}
 p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2\leq  B(p,\phi^\star) \|\phi^\star\|_2 
\end{array}
  \]  
  where
\[
 \begin{array}{ll}
 D_R(e_0) = (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{proof}
\begin{coro}
When $\sigma_1 = \sigma_2 = 0,$
 \[
 \begin{array}{ll}
\|\psi^\star -e_0\|_2\leq 
 \frac{p\mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}

\begin{coro}
When $\eta_1 = \eta_2 = 0,$
 \[
 \begin{array}{ll}
 \|\psi^\star -e_0\|_2\leq 
 \frac{ (1-p) \sigma_n(e_0)^2 +  
 p\sqrt{1+ \sigma^2_n(e_0)}  - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}








\subsection{All the proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



% \subsection{Constrained Convex algorithms }
%  \paragraph{Constrained noisy convex problems}
% Then we define the constrained convex program that allows noise,
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,z}   & |\alpha| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
% \label{eq:ConstrainProb}
%   \]
%   If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \zeta^2 \leq 1
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
%   \]
% If we set $\epsilon = 0,$ then we recover 
% the original convex problems for noiseless setting
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
% \mbox{subject to}  
% & v^T w =1,
% \end{array}
% \tag{$P_1$}
%   \]

==> old_sec/sec_old_2020/Noise_updated_constraint.tex <==
\section{Stability for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )-\epsilon \zeta|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2]-\epsilon \zeta |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )-\epsilon \zeta|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 
In the following, we use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$
   \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,N) \|\psi^\star-e_0\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
% hence
% \[
%  \begin{array}{ll}
% E_G |\mu+ \sigma G|
% &\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
% \end{array}
% \]
\end{lemma}


\paragraph{Robust optimization}
We want to find the min-max value 
\[
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta)
\]
for a function $H$,
\[
H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
\]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
For $A>0$, 
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{lemma}
\label{min-maxErrorL_p}
Let
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
 \end{array}
  \]
  where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
  then
\[
 \begin{array}{ll}
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta) = 
H( \mu(\psi))
\end{array}
\]

\end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

\subsection{Proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]

==> old_sec/sec_old_2020/Numerical.tex <==

\section{Numerical experiments}
We set up a ground truth inverse filter as $a^{-1} = (0.5, 1, 0.5)$, and numerically run $10$ independent experiments of finding the inverse filter by the convex problem 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}^T$ }
\EEQ
We choose an accuracy $\epsilon = 10^{-3}$ and count the number of successfully accurate recovery of $a^{-1}$ where $\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<\epsilon$. We see a consistent sharp transition of success rate from $0$ to $1$ in a narrow parameter region.
\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/phase_transition_detail.png}
\caption{The finite sample phase transition phenomenon, where $a^{-1} = (0.5, 1, 0.5)$,  $x-$axis is the sparsity level $p$, $y-$axis is the empirical probability $P(\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<10^{-3})$. Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}

==> old_sec/sec_old_2020/Phase_Transition.tex <==

\subsection{Population Phase transition theorem}
Qingyun: Old proof without subgradient language:

\paragraph{Population phase transition theorem}
\begin{theorem}
Under the previous assumption,
$
         p^\star   =\frac{\sin{\theta}}{\sin{\theta}+ \cos{\theta}} .
$
 The solution of  $P_{1,v}$ is $w^\star$, then 
 $w^\star$ is $a^{-1}$ up to shift and scaling provided $p<p^\star$,
and  $w^\star$ is not $a^{-1}$ up to shift and scaling provided $p> p^\star$.
  \end{theorem}
The population phase transition diagram is in figure~\ref{fig-PT}.

\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/Phase_T_sine.png}
\caption{The population phase transition diagram, $x-$axis is $\sin{\theta}$, $y-$axis is the sparsity level $p$ . Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}



% \begin{theorem} \label{lem:ica}
% We observe a sequence $Y\in \reals^n$, and we know that there exists a ground-truth filter $w^0$, such that $w^0*Y = X$, $X$ satisfy Bernoulli$(p)$-Gaussian model.  
% And we assume that we have a solution $w^\star$ to the Sparse convolutional ICA problem.
% Then if the angle $\theta$ between the vector $v$ and $w^0$ and the sparsity level $p$ satisfy that 
% \[
% \frac{p}{1-p}<\gamma \cot(\theta),
% \]
% then  $w^\star$ equals $w^0$ up to scaling, namely $w^\star = cw^0$ for $c\in \reals$ with probability $1-\exp\left( -C_0 \kappa_{w^0}^{-2} k\log(kp)\right)$, where $C_0$ is a constant, $\kappa_{w^0}$ is the condition number of the circulant matrix generated by $w^0$.

% \end{theorem}


\paragraph{Proof of the population phase transition theorem}
\BIT
 \item
  Let $\phi  := \psi -e_0 = \tilde w*\tilde a -e_0,$  then $|[w*Y]_0| = |[(e_0 +\tilde \phi)*X]_0| =  |[(e_0 + \phi)^T X| $, we define
  \[
  L(\phi) = |[(e_0 + \phi)^T X|.
  \] 
  WLOG, we can assume the ground truth $a^{-1}$ is scaled so that $v^T \tilde{a}^{-1} =1$
%   , then after the change of variable $w =  a^{-1}*(e_0 +\phi)$,  the condition $v^T w = 1$ can be transformed to $u^T \phi = 0$ where 
% $u: =\tilde{a}^{-1}*v$.

  We want to find a threshold $p^\star$ so that for all $p<p^\star$, the directional derivative  $ \Expect \nabla_{\phi}{L}|_{\phi = 0}>0$ for all directions $\phi$ that satisfy $u^T \phi = 0$.

 We define the finite difference
  \[
  D = L(\phi)-L(0) =  |[(e_0 + \phi)^T X| -|X_0| 
  \]
  Let $\epsilon : = \|\phi\|_2 $ and taking limit of $D$ as $\epsilon  \rightarrow 0,$ we have
    \BEQ
  \begin{array}{ll}
   \expect D &=  p\expect[D\mid X_0 \neq 0 ] + 
   (1-p)\expect[D \mid X_0 = 0 ] \\
   &=  p\expect[\mbox{sign}(X_0) ( \phi_0 X_0 + \sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid   \\
   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  
   \end{array}
 \EEQ
The last equality is because 
 $
 \expect[\mbox{sign}(X_0) (\sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] = 0 
$
 as $X_j$ are sampled independently. Notice that for Bernoulli Gaussian $X$,
$
\Expect [|X_0|\mid X_0 \neq 0 ]=\sqrt{\frac{2}{\pi}}.
$
 
 Then  $ \Expect \nabla_{\phi}{L}|_{\phi = 0} = \Expect \lim_{\epsilon \rightarrow 0}\frac{D}{\epsilon}>0$ 
 in case either $\phi_{0} > 0$, or in case $\phi_0 < 0$ and
\[
          \frac{p}{1-p} < \frac{ \Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  }{|\phi_0| 
          \Expect [|X_0|\mid X_0 \neq 0 ]} = \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} \frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\|\phi_{(0)}\|_2 \sqrt{\frac{2}{\pi}}}  .
\]
Here  $X_{(0)} = (X_i)_{i\neq 0}$
\item (Geometric lower bound:)
Using the fact that $u^T \phi = 0$. We define $v = \cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$, then $u =\tilde{a}^{-1}*v = \tilde{a}^{-1}*(\cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2})^{\bot}) =\cos{(\theta)} \frac{e_0}{\|\tilde{a}\|_2}+\sin{(\theta)} \tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot} $, 
where $\tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$ is perpendicular to $e_0$, 
therefore, 
$0= u^T \phi = \frac{1}{\|\tilde{a}\|_2}[\cos{(\theta)} \phi_0+\sin{(\theta)} \phi_{(0)}]$, therefore,  
$\frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} = \frac{\cos(\theta)}{\sin(\theta)} =\cot(\theta).$
\[
 \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|}\geq  \cot(\theta)
 \]

 
% \item 
% Let $h=\phi$, i.e. $h_i=\phi_{-i}$; and let $h_{(0)} = (h_i)_{i\neq 0}$, then
%   \[
%           \frac{p}{1-p} < \frac{ \Expect | h_{(0)}^T X_{(0)} |}{| h_{0}| \Expect |X_0|} = \frac{ \Expect | h_{(0)}^T X_{(0)} |}{\|h_{(0)}\|_2 \Expect |X_0|}  \frac{\|h_{(0)}\|_2}{| h_{0}|} .
% \]
\item
We showed that for IID Bernoulli Gaussian $X$,
\[
\frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\sqrt{\frac{2}{\pi}} \|\phi_{(0)}\|_2} = \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \in [p,1)
\]
Using semicontinuous extension, we can choose sequence of $\phi$ that is dense on doubly infinite sequence space $V_{-\infty, \infty}$, then we know that $\frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2}$ should be replaced by its semicontinuous extension on $V_{-\infty, \infty}$, which is $1$.

The phase transition $p^\star$ is the smallest $p$ so that 
\[
          \frac{p}{1-p} \leq  \cot(\theta) \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \leq  \cot(\theta).
\]
%  \BEQ
%   \begin{array}{ll}
%   \Expect D 
%   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  \\
%   &=  
%   \sqrt{\frac{2}{\pi}}\|{\phi}_{(0)}\|_2[ p (\mbox{sign}(\phi_{0})\tan(\theta)) + (1-p) (1-(1-p)^{\|{\phi}_{(0)}\|_0})]
%   \end{array}
%  \EEQ
Therefore,  generically, $ \frac{p^\star}{1-p^\star}  = \cot(\theta) $.
\EIT

==> old_sec/sec_old_2020/Planted_Proj.tex <==
% \section{Projection pursuit for planted sparsity}
% \subsection{Setup} 
% \subsection{Perturbation analysis}
% First, without loss of generality, we suppose  there is a vector $\beta$, $\beta^T \Phi Y = X_0$.

% Consider a vector  $b $ which is a small perturbation of $\beta$, where
% $\beta^T \Phi =e_0$, we assume $ \cM_1$ is the constraint set for $b$. Let $b = \beta + \eps \delta$ where $\delta \in T_\beta \cM_1$, the tangent space at $\beta$. We assume the condition $\delta \in T_\beta \cM_1$ is given by $v^T \delta = 0$.


% Let $h = \Phi^T \delta$, then from $   v^T \delta = 0$, we have $   u^T h = 0$, where $ v = \Phi u$. We have
% \[
%     b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
% \]
%  where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 
%  Let 
% \[
% D_0 =  |(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -|X_0|, 
% \]
 
 
 
%  Then for sufficiently small $\eps$
% \begin{eqnarray*}
%  E D_0 = E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
%  (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot p+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot (1-p),
% \end{eqnarray*}
%  where $p = P(X_0\neq 0)$.
 
%  The perturbation increases the objective value 
% just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

% Now we consider the optimization problem
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
%     \mbox{ subject to }&  h_{0} = -1, \\
%     & h\in \Phi^T T_\beta \cM_1.
% \end{eqnarray*}


% We know $h = \Phi^T \delta$, then 
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
%     \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
%      & \delta \in T_\beta \cM_1.
% \end{eqnarray*}

% \subsection{Geometric lower bound}
% We know that from perturbation analysis, the condition for phase transition are
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

%  We know $X_0$ is random variable sampled from a symmetric distribution with atom at $0$, $F_p = p H +(1-p) F$, and $X_i, \quad i\neq 0$ are sampled from distribution $G$.
% Using the sparsity of $X_0$,
% \[
% E \{ D_0 | X_0\neq 0 \}  = (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0|.
% \]
% And
% \[
% E \{ D_0 | X_0 =  0 \}  = E{|h_{(0)}^T X_{(0)}| }.
% \]

% First, when $F_t$ are all Gaussian distributions for $t\neq 0$, we leverage the invariance property for linear transform of Gaussian, and get 
% \[
% E{|h_{(0)}^T X_{(0)}| } = \|h_{(0)}\|_2 E|G| = \sqrt{\frac{2}{\pi}} \cdot \|h_{(0)}\|_2.
% \]

% % And we have calculated $E{|h_{(0)}^T X_{(0)}| }$ for different cases of $F_t$. 
% % For example, it is  lower bounded by  a constant multiple $\|h_{(0)}\|_2$ .

% And since we know $v^T h=0$, when $X_i$ are IID Gaussian, then linear combination of Gaussian are still Gaussian, so without loss of generality, we can change coordinate and assume $h = h_0 e_0 + h_1 t_1 + h' $, where $e_0$ is the unit vector in the direction of ground truth, $t_1$ is the unit vector in the direction of the component of $v$ normal to $e_0$, and $h'$ is in the rest of directions .

% Then we have $\|h_{(0)}\|_2\geq |h_1|$,
% and 
 
% \[
%           \frac{1-p}{p} <  \frac{  |h_1|} {| h_{0}|} = \cot(\theta).
% \]


\section{Phase transition for sub-Gaussian}
From the Khinthine’s inequality for sub-Gaussian and $p = 1$, we have 
\[
E{|h_{(0)}^T X_{(0)}| }\geq  3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2,
\]
for Bernoulli-SubGaussian, we have,
\[
E{|h_{(0)}^T X_{(0)}| }\geq  (1-(1-p)^M)^{1/2} 3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2.
\]
In general, we define
\[
\gamma(F,p) = E{|h_{(0)}^T X_{(0)}| }/\|h_{(0)}\|_2 E |X_0|,
\]
as the ratio between the linear combination $E{|h_{(0)}^T X_{(0)}| }$ for $\|h_{(0)}\|_2=1$ and $ E |X_0|$.

Then we need
\[
          \frac{1-p}{p} < \frac{ \gamma(F,p)  \|h_{(0)}\|_2}{| h_{0}|}
\]
for all $h$ such that $   u^T h = 0$ .

Also, using the fact that
 
\[
         \frac{  \|h_{(0)}\|_2} {| h_{0}|} \geq \cot(\theta).
\]
we have 
\[
          \frac{1-p}{p} <\gamma(F,p) \cot(\theta).
\]

\section{Noisy  signal}
 \subsection{Folder Gaussian}
 For a Gaussian RV $Z \sim N(\mu, \sigma)$, then for RV $|Z|$,  
 \[
 \mu_{|Z|} = E|Z|=\sqrt{\frac{2}{\pi}}\sigma e^{-\frac{\mu^2}{2\sigma^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma}\right) \right] 
%  = f(\mu,\sigma),
 \]
  \[
 \sigma_{|Z|}^2 = \mu^2 + \sigma^2 - \mu_{|Z|}^2.,
 \]
%  Then for fixed $\sigma$, let
%  \[
%  h_\sigma(\mu) = f(\mu,\sigma) 
%  \]
%  then 
%   \[
%  h'_\sigma(\mu) = 
%  \]
 
 \subsection{Noisy perturbation analysis}
Consider a noisy perturbation $\bar X_i  =  X_i + \sigma  E_i $, where $E_i$ is standard Gaussian $N(0,1)$, $ X_i = B_i Z_i$ are iid product of Bernolli RV with parameter $p$ and subGaussian unit variance RV with c.d.f $F$. 

Then we let $b^{\sigma}$ be the solution of the optimization problem 
\[
E D_\sigma = E_X E_E( |(1+ \eps h_0)(X_0+\sigma  E_0) +  \eps h_{(0)}^T (X_{(0)}+\sigma  E_{(0)})| -|X_0+\sigma  E_0|)
% = E_X (h'_\sigma(\mu)), 
\]
for sufficiently small $\eps$, and fixed $\sigma<1$, we consider the asymptotic analysis when $\eps  << 1 $， $ \sigma<< 1 $. We know $\sigma ((1+ \eps h_0)(  E_0)+\eps h_{(0)}^T  E_{(0)}))$ is a centered Gaussian with standard deviation 
\[\sigma\sqrt{(1+ \eps h_0)^2+(\eps h_{(0)})^2}\approx \sigma(1+ \eps h_0)
\]
therefore,
\begin{eqnarray*}
 E D_\sigma &\approx&   E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}+\sigma (1+ \eps h_0) E_0| -E|X_0+\sigma  E_0| \\
 &\approx& 
  p \cdot(|1+\eps \cdot  h_{0}|-1) \cdot E |Z_0+\sigma  E_0| + (1-p) \cdot ( E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|} ),
\end{eqnarray*}
 where $p = P(X_0\neq 0)$.
 
 First we derive lower bounds,
 \[
 E |Z_0+\sigma  E_0|
 \geq E |Z_0| - E|\sigma  E_0| =   E |Z_0| - \sqrt{\frac{2}{\pi}}\sigma,
\]
 \begin{eqnarray*}
 E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|}&\geq& E{|\eps  \cdot h_{(0)}^T X_{(0)} | -2 E|\sigma  E_0|} \\
 &=&  E|\eps  \cdot h_{(0)}^T X_{(0)} | -2 \sqrt{\frac{2}{\pi}}\sigma
\end{eqnarray*}
Then we have 
\begin{eqnarray*}
 E D_\sigma 
\geq  E D_0 - (p+2(1-p)) \cdot \sqrt{\frac{2}{\pi}}\sigma.
\end{eqnarray*}

Therefore, in the existence of noise, we don't have exact recovery result, but we would have a lower bound. 
 
 Second, we use the mean of folded Gaussian to compute the condition expectation.
 
 Here, for a fixed $\mu$, we rescale the variance $\sigma' = \sigma/\eps$. Under the assumption $\eps/\sigma<< 1 $, using asymptotic expansion, we can compute the condition expectation 
 \begin{eqnarray*}
   E({|\mu+\sigma'  E_0| -|\sigma'  E_0|}\mid \mu)
 &=& \sqrt{\frac{2}{\pi}}\sigma' e^{-\frac{\mu^2}{2\sigma'^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma'}\right) \right] - \sqrt{\frac{2}{\pi}}\sigma'
 \\
 &\approx& -\sqrt{\frac{2}{\pi}}\sigma' {\frac{\mu^2}{2\sigma'^2}}+\mu\sqrt{\frac{2}{\pi}}(-\frac{\mu}{\sigma'}  )
 \\
  &=&- \sqrt{\frac{2}{\pi}}  {\frac{3\mu^2}{2\sigma'}}  
\end{eqnarray*}
The first equality is the formula for the mean of folded Gaussian.
The second equality uses the Taylor expansion of Gaussian c.d.f
\[
\Phi (z)  = \frac{1}{2}+  \frac{1}{\sqrt{\pi}} \left(z-\frac{z^3}{3}+\frac{z^5}{10}-\frac{z^7}{42}+\frac{z^9}{216}-\cdots\right)
\]

 Therefore, for $Z_0$ standard Gaussian,
  \begin{eqnarray*}
 E_X E_{E_0}(|Z_0+\sigma  E_0|) 
  &=&  \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}  
\end{eqnarray*}
 \begin{eqnarray*}
 E_X E_{E_0}({|\eps  \cdot h_{(0)}^T X_{(0)} +\sigma  E_0| -|\sigma  E_0|}) 
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{E_X( h_{(0)}^T X_{(0)})^2 }{2\sigma'}}  
   \\
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2\sigma'}}  
\end{eqnarray*}

Then 
\begin{eqnarray*}
 E D_\sigma 
 &\approx& 
 \eps \left[ p \cdot h_{0} \cdot \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}    - (1-p) \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2(\sigma/\eps)}} \right] .
\end{eqnarray*}



 

==> old_sec/sec_old_2020/Projection_set_up.tex <==



\section{Population loss and phase transition}
We first study population loss of the sparse deconvolution problem
 \begin{eqnarray*}
    (\mbox{Population sparse deconvolution}) \qquad  \min_{w\in \reals^k} &    
    E\| w * Y\|_1\\
    \mbox{ subject to }&  v^T w = 1,\\
    &  w\in \cM.
\end{eqnarray*}
\subsection{Population loss of projection pursuit}
Let's first consider the population objective $E|w^T \Phi X|$.

Consider a vector  $w \in \cM$ which is a small perturbation of $w^\star  \in \cM$, where
$w^T \Phi =e_0$. Let $w = w^\star + \eps \delta$ where $\delta \in T_{w^\star} \cM$, the tangent space at $w^\star$. And since $\delta \in T_{w^\star} \cM_1$ is a subspace, we assume the constraint is given by $M \delta = 0$.
Let $h = \Phi^T \delta$, then $   u^T \delta = 0$, where $ v = \Phi u$. We have
\[
    b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
\]
 where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 \subsection{Population phase transition}
 We want to study $E D =  E|(1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)}| -E|X_0|$.
 
 Then for sufficiently small $\eps$
\begin{eqnarray*}
 E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
 (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot (1-\eta)+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot \eta,
\end{eqnarray*}
 where $p = P(X_0=0)$.
 
 The perturbation increases the objective value 
just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
\[
          \frac{\eta}{1-\eta} > \frac{| h_{0}| E |X_0|}{ E | h_{(0)}^T X_{(0)} |. }
\]

Now we consider the optimization problem
\begin{eqnarray*}
    (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
    \mbox{ subject to }&  h_{0} = -1, \\
    & h\in \Phi^T T_\beta \cM_1.
\end{eqnarray*}


We know $h = \Phi^T \delta$, then 
\begin{eqnarray*}
    (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
    \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
     & \delta \in T_\beta \cM_1.
\end{eqnarray*}



Following the quadratic problem reduction, we can related $Q_1$ to the deterministic quadratic problem.

After the study of the general population model, we remark that for convolutional model, $A$ ad $B$ are both generated by the circular or Topelitz matrices from a single vector.





==> old_sec/sec_old_2020/ProofResults.tex <==
\begin{proof}[Proof of theorem~\ref{thm:fin_deriv}]
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
 \EEAS
\end{proof}

==> old_sec/sec_old_2020/Regularized_Noise.tex <==
\subsection{Regularized convex problems}
\paragraph{Regularized convex problems}
For any $\epsilon>0$, we can find the Lagrangian form  of the constrained problem to define the regularized convex program, where we can find a corresponding $\lambda = \Lambda(\epsilon)$ so that $\frac{1}{2\lambda}$ is the dual variable.
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & |\tilde{w}^T Y -\zeta |+ \frac{1}{2\lambda}((\zeta)^2-\epsilon^2) \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
The convention to use for optimization is to ignorne the constant $-\epsilon^2$, and write the problem as
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2] \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
  Define soft-threshold operator as 
  \[
  S_{\mu}(x): = \sign (x) (|x| -\mu)_+
  \]
  and define its complement
   \[
  \bar{S}_{\mu}(x): = x-S_{\mu}(x) =  \sign (x)(x- (|x| -\mu)_+) =  \sign (x)\max(|x| ,\mu).
  \]
 \begin{lemma}
 If we partially minimize over $\alpha,$ the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
    \[
 \begin{array}{ll}
\mbox{inf}_{\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]   = [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 

\end{array}
  \]
  \end{lemma} 
  
  
 
\begin{proof}
Due to the proximal operator of $\ell_1$ norm,  the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
The objective can be further simplified to
  \[
 \begin{array}{ll}
&\Expect[|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]\\
=&\Expect[|S_{\lambda}(\tilde{w}^T Y)|+ \frac{1}{2\lambda}(\bar{S}_{\lambda}(\tilde{w}^T Y) )^2]\\
=& [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 
\end{array}
  \]
 \end{proof} 

Using the data generative model and do change of variable, 
the partially minimized regularized problem is
 \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi}   & \Expect[|(|\psi^T (X+\eta Z )|-\lambda)_+|+ \frac{1}{2\lambda}(\max(|\psi^T (X+\eta Z )| ,\lambda) )^2] \\
\mbox{subject to}  
& u^T \psi =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
%   For the regularized problem we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,  
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]
%   However, it seems hard to study it directly since its order is similar to $\inf_{\lambda} \sup_{Z: \|Z\|_2\leq 1}  \Expect \inf_{\zeta(\lambda)}$ .)
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]

==> old_sec/sec_old_2020/Related_Work.tex <==
\section{Related Work}
\paragraph{Prior work: analysis approach, non-Gaussianity}
  \begin{itemize}
  \item
  Key idea $1$: Find inverse filter $a^{-1}$ so that
$ a^{-1}*y = x $.
\item Key idea $2$: 
If $x$ is non-Gaussian, then $a*x$ is closer to Gaussian. 
\item Find $w\neq 0$  
\[
 \begin{array}{ll}
 \underset{w}{\mbox{maximize}}   & J(w*y)
\end{array}
  \]
\item Non-Gaussianity: $J$ is negative entropy function or normalized $4$-th order cumulant $J(z) = \frac{\|z\|_4^4}{\|z\|_2^4}$ \cite{wiggins1978minimum, donoho1981minimum}
  \item Sparsity: 
  $J(z) = - \| z\|_1/\|z\|_2$,  \cite{gray1979variable,donoho1981minimum,kijko1994seismological}.
  \item varimax norm: $\max_i \frac{|z_i|}{\|z\|_2}$ \cite{cabrelli1985minimum}
\end{itemize}

\paragraph{Prior work: blind equalization for digital signal}
  \begin{itemize}
\item
Digital signal: PAM signaling $\pm 1$ binary signal or QAM signaling with $|x|=1, x\in \complex$ \cite{kennedy1992blind,ding2000fast}. 
\item More general,  $x$ are IID and bounded by $M = \mbox{max}(x_i)$ \cite{vembu1994convex,li2001blind}.
\item 
  Convex Cost Functions in Blind Equalization \cite{vembu1994convex}:
  find $w$ so that $w*a = e_0 = (\ldots,0,1,0, \ldots)$ as minimizer of the ideal convex problem (
 Not computable without knowing $a$!)
  \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   & \| w*a\|_1 
 \\
\mbox{subject to} 
& (w*a)_0 = 1.
\end{array}
  \]  
  
    \item
  When $x$ are IID and bounded by $M = \mbox{max}(x_i)$, using duality, use surrogate objective for $\| w*a\|_1$ as
   \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  \frac{1}{M} E \|w * y\|_\infty 
 \\
\mbox{subject to} 
& \|w*y\|_2 = 1.
\end{array}
  \]
   In \cite{vembu1994convex}, they use projected SGD on $E \|w * y\|_8 $ to approximate $E \|w * y\|_\infty$ .
  
  \item Later, use linear programming to solve $\infty$ norm problem directly \cite{ding2000fast}: 
    \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  E \|w * y\|_\infty
 \\
\mbox{subject to} 
& w_0 = 1.
\end{array}
  \]
\end{itemize}

\paragraph{Prior work: synthesis approach, sparsity}
In many papers \cite{kuo2019geometry, bristow2013fast, heide2015fast,zhang2017global,zhang2018structured}, researchers designed alternating-minimization algorithms that jointly find a short $a$ on sphere and a sparse $X$ from $Y$ by solving the following non-convex problem: 
  \[
 \begin{array}{ll}
 \underset{a, x}{\mbox{minimize}}   & \|Y-a*x\|_2^2+\lambda \|x\|_1 \\
\mbox{subject to}  & \|a\|_2 = 1.
\end{array}
  \]  
\BIT
% \item
% Sparse signal has a long history in seismology and communication,
% see \cite{kijko1994seismological}, \cite{vembu1994convex}, \cite{osman1996seismic}, \cite{wang2010seismic}, \cite{romberg2009compressive},\cite{mendelson2016improved} etc.
\item
  Convolutional dictionary learning formulation \cite{bristow2013fast, heide2015fast}, etc.
  \item
  Synthesis blind deconvolution with $2$ norm ball constraint  \cite{zhang2017global,zhang2018structured, kuo2019geometry}, etc.
  \item
  Short $a$ and sparse $x$: 
  \[
 \begin{array}{ll}
 \mbox{minimize}   & \|y-a*x\|_2^2+\lambda \|x\|_1 \\
\mbox{subject to}  & \|a\|_2 = 1.
\end{array}
  \]  
%   \item Only empirical result so far.
%   \item Landscape could be complex.
\EIT

\paragraph{Prior work: synthesis approach, subspace assumption}
\[
 \begin{array}{ll}
 y &= a^0 * x^0\\
 \hat y  &= \hat a^0 \circ \hat x^0
\end{array}
  \]
   \begin{itemize}
  \item  $\hat a^0= D_a c_a$.
  \item $\hat x^0 = D_X c_x$.
  \item $D_X$ is often a complex Gaussian matrix.  
\end{itemize}
% \begin{figure}
%  \includegraphics[width=5cm,keepaspectratio]{figures/subspace.png}
%  \includegraphics[width=5cm,keepaspectratio]{figures/shift2.png}
% \end{figure}
No translation symmetry in this assumption!


Lifting:
 \[
 \begin{array}{ll}
 \hat y &= (D_a c_a) \circ (D_X c_x)\\
 &= \mathcal{D}(c_a c_x^T)
\end{array}
  \]
 $\mathcal{D}$ is a linear operator defined as 
 \[
 \begin{array}{ll}
\mathcal{D}(c_a c_x^T)_i = \mbox{trace}((D_{a,i}D_{X,i}^T)(c_a c_x^T))
\end{array}
  \]
  Rank one matrix $Z=c_a c_x^T$.
   \[
      \hat y =  \mathcal{D}(Z)
  \]
  \begin{itemize}  
  \item Convex optimization  \cite{ahmed2014blind},\cite{ling2015self}, \cite{chi2016guaranteed},\cite{romberg2013multichannel},\cite{lee2017blind} etc.
  \item Non-convex optimization  \cite{li2016rapid}.
\end{itemize}

\paragraph{Projection pursuit  with linear constraint}
We point out that the population problem formulation for sparse blind deconvolution is also the population problem formulation for sparse projection pursuit, which might also be called convex sparse ICA, or convex sparse dictionary learning.
\BEQ
 \begin{array}{ll}
  \underset{\psi \in V}{ \mbox{minimize} }  &  \expect |\psi^T X|\\
 \mbox{subject to}  
&  u^T \psi =1.
\end{array}
\tag{$P_{1,v}$}
\EEQ


In sparse projection pursuit with linear constraint, we observe a matrix $Y_M\in \reals^{n\times M }$, and we know that there exists a ground-truth filter $w^0$, such that $w^{0,T} Y_M = X_M$, $X_M$ satisfy Bernoulli$(p)$-Gaussian model.  

We consider the "projection pursuit" problem.
 \begin{eqnarray*}
    (\mbox{Projection pursuit}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&  v^T w = 1.
\end{eqnarray*}
Here $w$ is in a $k$ dimensional subspace of the double infinite sequence. 


\paragraph{Projection pursuit with sphere constraint}
We comment that the results we derive in the following sections are also applicable to the projection pursuit (orthogonal dictionary learning) problem \cite{bai2018subgradient, sun2016complete, sun2015complete}.
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 = 1.
\end{eqnarray*}
or
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 \geq 1.
\end{eqnarray*}
\begin{lemma}
The population problem is:
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect |\psi^T X|  \\
\mbox{subject to}  
&\Expect |\psi^T X|^2 \geq \Expect (X_0)^2
\end{array}
  \]
is equivalent to the following convex-concave problem
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
\mbox{subject to}  
&\|\psi\|_2^2 \geq 1
\end{array}
  \]
We claim that  it has the same minimizer as the \textbf{ projection pursuit (orthogonal dictionary learning) problem with sphere constraint}.
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect_I \|\psi_I\|_2  \\
\mbox{subject to}  
&\|\psi\|_2 = 1
\end{array}
  \]
  which is also equivalent to
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect_I \|\psi_I\|_2/\|\psi\|_2 
\end{array}
  \]
  And  also equivalent to
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect |\psi^T X|/\sqrt{\Expect |\psi^T X|^2} 
\end{array}
  \]
\end{lemma}


Inspired by this formulation, we propose a non-convex (convex objective concave constraint) problem for blind deconvultion:
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_2 \geq 1.
\end{eqnarray*}

Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_\infty \geq 1.
\end{eqnarray*}


\paragraph{Infinity norm ball constraint}


Before stating the main theorem and its proof, we make some comments about the formulation.

If we study the population level, 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \expect |\tilde{w}^T Y|\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}$ }
\EEQ
then we only need solve one convex problems
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \expect |\tilde{w}^T Y|\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}$ }
\EEQ
Since the entry with largest magnitude will automatically be shifted to coordinate $0$ due to shift invariance.


If we want to solve the following non-convex problem with infinity norm ball constraint for finite sample,
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}^T$}
\EEQ
We can solve the following convex problems, and select the one with minimal objective value. This is equivalent to solve the problem with fixed infinity norm. 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_j =1.
\end{array}
\tag{$P_{e_j}^T$ }
\EEQ

% \paragraph{Dirac re-parametrization and connection to residual CNN}
% When $v = e_0$, we are imposing a constraint that the largest entry of $w$ is $w_0 =1$.  
% We can re-parametrize our filter, as $w = \delta_0 + f$, $f_0 = 0$. Then our problem became 
%  \begin{eqnarray*}
%     \min_{f, f_0 = 0} &    
%     \frac{1}{2T+1}\|(e_0 +f)*Y\|_{1,[-T,T]}.
% \end{eqnarray*}
% Here $f = (f_L, 0, f_R)$, $f_R$ and $f_L$ are in $k$ dimensional subspace of the double infinite sequence with positive and negative support.

% Allowing Noise:
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|x\|_ 1+\lambda/2\|Y+f*Y-x\|_2^2\\
% \mbox{subject to}  
% & f_0 =0,
% \end{array}
%   \]
%   with variables $f\in \reals^k$, $x\in \reals^n$. 
  
%  \texbf{General multi-channel approximate version}
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \sum_i(\|x^i\|_ 1+\lambda^i/2\|Y+f^i*Y-x^i\|_2^2)\\
% \mbox{subject to}  
% & f^i_0 =0,
% \end{array}
%   \]
%   with variables $f^i\in \reals^k$, $x^i\in \reals^n$. 
  
% \paragraph{Link to CNN}
% Partial minimization:(similar to one-layer Residual CNN)
% \[
%  \begin{array}{ll}
%  x^i = S_{1/\lambda^i}(Y+f^i*Y)
% \end{array}
%   \]
%   with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $. 


% \texbf{Method $1$: plug-in}
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \sum_i(\|S_{1/\lambda^i}(Y+f^i*Y)\|_ 1+\\
%  &\lambda^i/2\|Y+f^i*Y-S_{1/\lambda^i}(Y+f^i*Y)\|_2^2)\\
% \mbox{subject to}  
% & f^i_0 =0,
% \end{array}
%   \]
%   with variables $f^i\in \reals^k$, $x^i\in \reals^n$.   
  
% %   Let $C_Y$ be the circulant matrix with first column $Y$, let $\hat Y = F_nY$, where $F_n$ is discrete Fourier transform, $U = \frac{1}{\sqrt{n}}F_n$ as a unitary matrix,
% % \[
% % C_Y = U^*\mbox{diag}(\hat Y)U.
% % \]
% % Block coordinate update (alternating): initialize: $ f^i(0) = 0;$.
% % \[
% %  \begin{array}{ll}
% %  x^i(t) &= S_{1/\lambda^i}(Y+f^i(t-1)*Y);\\
% %  f^i(t) &= (C_Y^T C_Y)^{-1}[C^T_Y(x^i(t)-Y)+\mu(t) \delta_0^T]\\
% %  &= U^*\mbox{diag}(1/(\hat Y))U x^i(t)-\delta_0 
% %  + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T\\
% %  &= Y^{(-1)}*x^i(t) -\delta_0 + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T
% % \end{array}
% %   \]
% %   with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $, $\mu(t)$ is the dual variable.

==> old_sec/sec_old_2020/ResultFiniteSample.tex <==
\section{Main results for finite sample guarantee}
% \subsection{ Finite sample guarantee theorem for blind deconvolution}
\paragraph{Finite sample setting}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$ Additionally, in finite sample setting, we assume $a^{-1}$ is zero outside of a centered window of radius $k$.
% namely, the non-zero part can be written as $(\beta_{-k}, \ldots, \beta_0, \ldots, \beta_k)\in V$. 
\item
Let $Y= a* X$ be a linear process, we are given a series of observations $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$.
\item
 We denote $X^{(i)}$ as the sequence being flipped and shifted for $i$ step from $X$ so that $X^{(i)}_k = X_{-k +i}$. Let $J_N$ be the support of $X$.
 We define the length $N=2T+1$ window as $\cT := [-T, T].$
\EIT
Now we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse,
\BEQ
 \begin{array}{ll}
 \underset{w\in V}{  \mbox{minimize} }   & \frac{1}{N}\|w*Y\|_{1,\cT}\\
 \mbox{subject to}  
& (\alpha* w)_0 =1.
\end{array}
% \tag{$P_{\alpha}^N$}
\EEQ
\paragraph{Finite sample directional derivative}
Now to study the finite sample convex problem, we need to calculate the directional derivative at $ \psi = e_0$.
Then
\begin{theorem}
\label{thm:fin_deriv}
For any $X$ sequence with support  $J_N$,
\BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right).
% \\
%   &=& 
% p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
% (1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
% \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
 
\end{theorem}











 \paragraph{Concentration of $\|\psi*X\|_{1}$ }
 \begin{lemma}
 \label{lem:mu_min}
 Let 
 \[
\mu_{\mbox{min}}:=\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1},
\]
then it is the lower bound of $\E \frac{1}{N}\|w*a*X\|_{1,\cT}$:
\[
\E \frac{1}{N}\|w*a*X\|_{1,\cT}  \geq \mu_{\mbox{min}}.
\]
 \end{lemma}

Now we define the intersection of $1-$norm ball of the $k-$dimensional subspace $V_k$ as $B_1(V_k)$, then we consider $w\in B_1(V_k).$ 
 
\begin{lemma}
\label{lem:tail_W}
Hence we consider $\psi = a*w \in a*B_1(V_k),$ and we define
\[
W:= \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) |.
\]

For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E W^q\leq 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q,
\]
so
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k)),
\EEAS
and
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta.
\EEAS
\end{lemma}

\begin{theorem}
\label{thm:concen_W}
Let the solution of finite sample convex optimization be $w^\star$, 
for small $\epsilon>0$ and concentration level $\delta>0$, 
there exists universal constant $C$, if there are 
% \[
% N=2T+1 \geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
% \]
\[
N \geq k\log(\frac{k}{\delta}) ( \frac{C\kappa_a}{\epsilon}  )^2,
\]
and  $ \frac{1}{N}\leq p$, we have:
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
% Therefore with probability at least $1-\delta$, $a*w^\star =e_0$ and we recover the sparse vector exactly.

% \textbf{ToDO:}
% or
% $\|a*w^\star -e_0\|_1<\epsilon_1$ provided $p< p_N^\star$ for some $p_N^\star\leq p^\star$.
  \end{theorem}
 
\paragraph{Uniform bound of directional derivative}
We  define the uniform bound of directional derivative:
\[
W_D  =\sup_{\|\beta\|_2=1, u^T \beta =0, \beta +e_0 \in a*B_1(V_k)}|\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  |.
\]
Notice that
\BEAS
& &\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  
\\
&=& 
\left[\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}\right)\right]-
\\
& &
\left[\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])\right].
\EEAS

Combining the following three uniform bounds on
\[
|(\frac{1}{N} \|X\|_{1,J_N}-\sqrt{\frac{2}{\pi}}p)|,
\]
\[
|\frac{1}{N}\|X*\beta_{(0)}\|_{1,\cT-J_N}-\sqrt{\frac{2}{\pi}}(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]|,
\]
\[
|\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}|,
\]
with high probability, we have  
\[
W_D  < \epsilon \mu_{\mbox{min}}.
\]

We define $\delta_p(N,\epsilon)$ the one side finite $N$ band such that for all $p<p^\star -\delta_p(N,\epsilon)$, 
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon \mu_{\mbox{min}}.
\]
for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]
then using the convexity argument, $a*w^\star-e_0=0$. 

\paragraph{Finite sample guarantee}
From previous concentration of finite sample directional derivative, we have the following theorem.
	\begin{theorem}
	\label{thm:fin_guarantee}
		When $a^{-1}$ is length $k$, for small constant $\epsilon>0, \delta>0$, when the number of observation $N$ satisfies
		\[
N \geq  k\log(\frac{k}{\delta}) ( \frac{C\kappa_a}{\epsilon}  )^2,
\]
then 
\[
W_D  < \epsilon \mu_{\mbox{min}}.
\]
For $\frac{1}{N}\leq p \leq p^\star - \delta_p(N,\epsilon)$,
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon \mu_{\mbox{min}}.
\]
therefore, 	with probability $1-\delta$, for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]

		the solution of finite sample convex optimization $w^\star$ is $a^{-1}$ up to scaling and shift 
		with probability $1-\delta$.
	\end{theorem}
	
\section{Proofs for finite sample guarantee}	
	\begin{proof}[Proof of theorem~\ref{thm:fin_deriv}]
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right).
 \EEAS
\end{proof}
	
	
\begin{proof}[Proof of lemma~\ref{lem:mu_min}]
Without loss of generality, we rescale $w$ so that $\|w\|_1 =1$, now
\BEAS
\E_X Z 
&=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
&\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|.
\EEAS
By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
$\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
\BEAS
\E_X Z 
&\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
&\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
&\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
&=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}.\\
\EEAS
\end{proof}
 
\begin{proof}[Proof of Lemma~\ref{lem:tail_W}]
Let $\varepsilon_1, \ldots, \varepsilon_N$ be a sequence of IID Rademacher ($\pm 1$)  random variables independent of $X$.  By the symmetrization inequality, see e.g. Lemma~$6.3$ of book \cite{ledoux2013probability}, we have the first inequality. Then since the function $t \rightarrow |t| $ is a contraction, an application of Talagrand’s contraction principle (see Lemma~$8$ of \cite{adamczak2016note}) with $F (x) = |x|^q$ 
conditionally on $X$ gives the second inequality.
\BEAS
\E W^q 
&\leq& 2^q \E \sup_{\psi \in a*B_1(V_k)} 
|\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j |(\psi*X)_{j}| |^q\\
&\leq&
2^{2q}\E \sup_{\psi \in a*B_1(V_k)} |\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j (\psi*X)_{j} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{\psi \in a*B_1(V_k)} |\sum_{i\in [-T,T] }\psi_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{w \in B_1(V_k)} |\sum_{i\in [-T,T] }(w*a)_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&\leq&
2^{2q}\frac{1}{N^q}\E \max_{s\in [k]}|\sum_{i\in [-T,T] }a_{i-s}( \sum_{j\in [-T,T] } \varepsilon_j X_{j-i}) |^q\\
&\leq&
2^{2q}(\frac{\lambda_{M}(a)}{N})^q   \sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q.
\EEAS
Now by the moment version of Bernstein’s inequality (see Lemma~$7$, equation $(18)$ of~\cite{adamczak2016note}), we know that there exists a universal constant $C$,
\BEAS
\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q \leq C^q(\sqrt{Npq}+q)^q.
\EEAS
Therefore, 
\BEAS
\E W^q &\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q    
\sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q \\
&\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q.
\EEAS
Then
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k)).
\EEAS
Therefore, we could get the tail bound using the Chebyshev inequality for the moments,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np(q+\log(k))}+q +\log(k)))\leq e^{-q}.
\EEAS
We set $q = \log(\frac{1}{\delta})$, obtaining an upper bound for $W$ which is satisfied with probability at least $1-\delta$:
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta.
\EEAS
\end{proof}	
	
	
	
\begin{proof}[Proof of Theorem~\ref{thm:concen_W}]
From previous lemma, we know that with the conditions, 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
Therefore, with probability at least $1-\delta$,
\BEAS
W = \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) | \leq \epsilon \mu_{\mbox{min}}.
\EEAS
When this is true, for all $\psi \in a*B_1(V_k)$, we have a uniform bound:
\[
 \E |(\psi*X)_{j}|-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}.
\]
\end{proof}
	
	
	
	
\begin{proof}[Proof of Theorem~\ref{thm:fin_guarantee}]
Notice that
\BEAS
& &\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  
\\
&=& 
\left[\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}\right)\right]-
\\
& &
\left[\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])\right].
\EEAS
From the previous uniform bound, with high probability, we have the following three uniform bounds on
\[
|(\frac{1}{N} \|X\|_{1,J_N}-\sqrt{\frac{2}{\pi}}p)|,
\]
\[
|\frac{1}{N}\|X*\beta_{(0)}\|_{1,\cT-J_N}-\sqrt{\frac{2}{\pi}}(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]|.
\]
The uniform bound on 
\[
|\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}|
\]
comes from symmetric distribution assumption.

Combining all three uniform bounds, with high probability, we have:
\[
W_D  < \epsilon \mu_{\mbox{min}}.
\]

We define $\delta_p(N,\epsilon)$ the one-side finite $N$ band such that for all $p<p^\star -\delta_p(N,\epsilon)$, 
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon \mu_{\mbox{min}}.
\]
for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]
then using the convexity argument, $a*w^\star-e_0=0$. 

	
\end{proof}

	
	
	
	
	
	
	
	

% \begin{coro}
% When $\sigma_1 = \sigma_2 = 0,$
% \[
% \E_I  \| (\psi^\star)_I \|_2 -p\leq p\mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
% \]
%  \[
%  \begin{array}{ll}
% \|\psi^\star -e_0\|_2\leq 
%  \frac{p\mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
% (1-p)- \tan(\theta) )\cos{\theta} }
% \end{array}
%   \]  

% \end{coro}

% \begin{coro}
% When $\eta_1 = \eta_2 = 0,$
% \[
% \E_I  \| (\psi^\star)_I \|_2 -p \leq  (1-p) \sqrt{\sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} +
%  p\sqrt{1+ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2}  - p
% \]
%  \[
%  \begin{array}{ll}
%  \|\psi^\star -e_0\|_2\leq 
%  \frac{ (1-p) \sigma_n(e_0)^2 +  
%  p\sqrt{1+ \sigma^2_n(e_0)}  - p}{p (
% (1-p)- \tan(\theta) )\cos{\theta} }
% \end{array}
%   \]  

% \end{coro}


==> old_sec/sec_old_2020/Result_Stability.tex <==

	
\section{Stability of convex blind deconvolution with infinite length inverse filter approximation }
Now we consider a setting where there is a kernel whose corresponding inverse kernel has infinite support, and we give a finite-length approximation. 

Within the space $V_{-\infty,\infty}$ of bilaterally infinite real-valued sequences $(h(i))_{i \in \integers}$, consider the affine subspace $V_{N_{-}, N_{+}} = \{ (...,0,0,h_{-N_{-}},\ldots, h_{-1}, 1, h_1, h_2, \ldots, h_{N_{+}},0,0,...)\}$, an $N_{-}+N_{+}$-dimensional subspace of bilateral sequences with support at most $N_{-}+N_{+}+1$.
The coordinate that is fixed to one is 
located at index $i=0$.
Each coordinate is zero outside of a window
of size $N_{-}$ on the left of zero 
and  size $N_{+}$ on the right of zero.
The special sequence $e_0 = (\dots,0,0,1,0,0,\dots)$,
vanishing everywhere except the origin,
belongs to $V_{-\infty,\infty}$ and to every
$V_{N_-,N_+}$.

Let $a \in V_{N_-,N_+}$.
Then $a =  (...,0,0,a_{-N_{-}},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_{N_{+}},0,0,...)$.
We also write $a = e_0 + a_{(0)}$,
where $a_{(0)} \equiv (1-e_0) \cdot a$ 
denotes the `part of $a$ supported away from location
$i=0$'. We also write $a = e_0 + a_L + a_R$,
where $a_L = (a_L(i))_{i \in \integers} 
= (a(i) 1_{\{i < 0\}})_{i \in \integers}$ 
denotes the `part of $a$ supported to
the left of $i=0$' and 
where $a_R = (a_R(i))_{i \in \integers} 
= (a(i) 1_{\{i > 0\}})_{i \in \integers}$
denotes the `part of $a$
supported to the right of $i=0$'.
Finally, we say that $a \in V_{N_{-}, N_{+}}$ 
is a length $ L= N_{-}+N_{+}+1$ filter.

\textbf{First example}: let's look at a simple example of infinite length inverse filter approximation.
Let $s\in (-1,1)$. For $a=( 0, 1, -s)$, then $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$ is an infinite length inverse filter. 

If we choose a length $r$ approximation $w^{r}= (\ldots, 0, 1, s, s^2, s^3, \ldots, s^{r-1})$ then
\[
\|a*w^{r}-e_0\|_2^2 = |s|^{2r}.
\]


Now we consider general finite-length forward filter with infinite-length inverse filter.

We construct the finite-length approximation filter explicitly by truncation of Z-transform.

Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i}.
\end{array}
  \]
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.

\begin{theorem}
\label{thm:RootNorm}
Assuming we have a finite length forward filter $a$ with its Z-transform having roots inside the unit circle, namely $s_{k}:= e^{-\rho_k + i \varphi_k }$ with $|s_k|<1$ and $\rho_k>0$
for $k \in \{-N_{-}, \ldots -1, 1, \ldots N_{+}\}$.
\[
 \begin{array}{ll}
A(z) &=  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i}
\\
&= c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1}),
\end{array}
  \]
Where $c_0$ is a constant to make sure that the coefficient $a_0=1$.

Then for a vector index $r=(r_{-N_-}, \ldots, r_{-1}, r_{1},\ldots, r_{N_+} ) $, we could construct an approximate inverse filter $w^r$ with Z-transform
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r_{-j}-1} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r_{-j}-1} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r_i}) (1- s_{i} z^{-1})^{-1}.
\end{array}
\]
Let $\phi^r = w^r*a-e_0$, then
\[
 \begin{array}{ll}
\|\phi^r \|_2^2 = \|a*w^r-e_0\|_2^2
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big(- 2 \big(r_{k_1} \rho_{k_1}+ \ldots+  r_{k_n} \rho_{k_n} \big) \Big).
\end{array}
  \]
%   Let $\gamma^m := \min_{i}\big(r_{i} |\rho_{i}| \big) =  \min\{r_{-N_-}|\rho_{-N_-}|, \ldots, r_{-1}|\rho_{-1}|, r_{1}|\rho_{1}|, \ldots, r_{N_+}|\rho_{N_+}|\}.$
When $\min_j r_j \rightarrow \infty$, it converges to zero at an exponential rate. The convergence rate is determined by the slowest decaying exponential term as a function of $\min_i (r_i \rho_i)$.
\[
 \begin{array}{ll}
\|\phi^r \|_2
&= O(
\exp \Big(-  \min_i (r_i \rho_i) \Big) ), \quad \min_i r_i \rightarrow \infty.
\end{array}
  \]
 \end{theorem}

 \begin{theorem} 
 \label{thm:bd_stab}
 Let $a\in V_{N_-, N_+} $ be a forward filter with all the roots of Z-transform strictly in the unit circle. Let $w^\star \in V_{(r-1)N_-, (r-1)N_+} $ be the solution of the convex optimization problem. Let $w^r$ be the constructed filter in previous theorem with a uniform vector index $(r, \ldots, r, r,\ldots, r)$.
  Let $\phi^\star = w^\star*a-e_0$, 
 then the solution satisfy
  \[
 \begin{array}{ll}
  B(e_0,\phi^\star) \|\phi^\star \|_2 \leq B(e_0,\phi^r) \|\phi^r \|_2.
\end{array}
  \]
  Additionally, as $p<p^\star$, $B(e_0,\phi^\star)$ and $B(e_0,\phi^r)$ are both upper and lower bounded. 
  Therefore, using the previous asymptotic exponential convergence bound on $\|\phi^r \|_2$ as 
  $r \rightarrow \infty$, it converges to zero at an exponential rate
  \[
 \begin{array}{ll}
   \|\phi^\star \|_2 \leq \frac{B(e_0,\phi^r)}{B(e_0,\phi^\star)} \|\phi^r \|_2
   \leq
   O(
\exp \Big(-  r \min_i (\rho_i) \Big) ), \quad r \rightarrow \infty.
\end{array}
  \]
%   where $B(e_0,\phi^\star)$
%   \[
% B(p, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
% \]
% is upper and lower bounded.  
% by the bi-Liptiz property of the directional finite differencee of objective
 \end{theorem} 
 

\section{Proofs for stability results}	

\begin{proof}[Proof of Theorem~\ref{thm:RootNorm}]
Now let $\psi^r$ have Z-transform $\Psi(z)$, $\phi = a*w-e_0$ with Z-transform $\Phi(z)$,
\[
 \begin{array}{ll}
\Psi(z): = A(z)W(z) 
&=   \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i}).
\end{array}
\]
Therefore,
\[
 \begin{array}{ll}
\Phi(z): = A(z)W(z) -1 
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i}) -1.
\end{array}
  \]
Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible indicies.
And use polar representation of complex roots:
for any $k \in \cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$
\[
s_{k} := |s_{k}| e^{i \varphi_k } = e^{-\rho_k + i \varphi_k },
\]
where 
\[
 \begin{array}{ll}
\varphi_k := \operatorname{Im}(\log( s_{k} )) = -i \log(\frac{s_{k}}{|s_{k}|}),
\end{array}
\]
and since $|s_{k}|<1$ we have 
\[
\rho_k = -\operatorname{Re}(\log( s_{k} ))>0.
\]

Now we consider all $z = e^{2 \pi i t}$ on the unit circle for $t\in [\frac{-1}{2},\frac{1}{2}]$,
then for any $k \in \cI$
\[
 \begin{array}{ll}
- (s_{k} z^{-\mbox{sign}(k)})^{r_{k}} 
&= - |s_{k}|^{r_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot r_{k} \big)\\
&=   \exp \Big( -r_{k} \rho_k+ i \cdot \big( r_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big).
\end{array}
  \]
 Now we simplify the notation by defining 
 \[
 \upsilon_k(t) :=r_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi,
 \]
then
 \[
 \begin{array}{ll}
\Phi(z)
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_{i}}) -1\\
&=  \prod_{k \in \cI} \Big(1- |s_{k}|^{r_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot r_{k} \big)\Big)  -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( -r_{k} \rho_k+ i \cdot \big( r_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) \bigg)     -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( -r_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg) -1.
\end{array}
  \]
  
% \begin{lemma}
 For any $z = \exp{(2 \pi i t )}$ on the unit circle,
 \[
 \begin{array}{ll}
\Phi\big(\exp{(2 \pi i t )}\big)
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big(- r_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1\\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( -\big(r_{k_1} \rho_{k_1}+ \ldots+  r_{k_n} \rho_{k_n} \big)
+ i \cdot \big( \upsilon_{k_1}(t) + \ldots+  \upsilon_{k_n}(t)  \big) \Big).
\end{array}
  \]
%  \end{lemma}
 
%  \begin{lemma}
Additionally, for any $t \in [\frac{-1}{2},\frac{1}{2}]$,
\[
 \begin{array}{ll}
 |\Phi\big(\exp{(2 \pi i t )}\big)|^2  
= 
\sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( -2 \big(r_{k_1} \rho_{k_1}+ \ldots+  r_{k_n} \rho_{k_n} \big) \Big)
\end{array}
  \]
is independent of $t$, since the oscillation integral over the imaginary part is 
  \[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2}
\exp  \bigg( i \cdot \Big(  \big(\upsilon_{k_1}(t) - \upsilon_{k_1}(t) \big) + \ldots+  \big(\upsilon_{k_n}(t) -\upsilon_{k_n}(-t)\big)  \Big) \bigg)  dt
= 1.
\end{array}
  \]
Therefore, using Fourier isometry,
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 &= \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi\big(\exp{(2 \pi i t )}\big)|^2 dt \\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( -2 \big(r_{k_1} \rho_{k_1}+ \ldots+  r_{k_n} \rho_{k_n} \big) \Big).
\end{array}
  \]
When $\min_j r_j \rightarrow \infty$, it converges to zero at an exponential rate. The convergence rate is determined by the slowest decay exponential term as a function of $\min_i (r_i \rho_i)$.
\[
 \begin{array}{ll}
\|\phi^r \|_2
&= O(
\exp \Big(-  \min_i (r_i \rho_i) \Big) ), \quad \min_i r_i \rightarrow \infty.
\end{array}
  \]
  
%  \end{lemma}
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:bd_stab}]
Following the previous phase transition analysis, 
let the directional finite difference of the objective at $e_0$ be $D(w) = |(w*Y)_0| - |X_0|$, $I$ be the support of $\tilde{X}$, let $\phi = w*a-e_0$,  then we have 
\[
 \begin{array}{ll}
\Expect D(w) &= \sqrt{\frac{2}{\pi}}\Expect_I [\|(w*a)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\|{\phi}\|_2 B(p, \phi) . \\
\end{array}
  \]
Now using the optimality of $w^\star \in V_{(r-1)N_-, (r-1)N_+} $, for all $w^r in V_{(r-1)N_-, (r-1)N_+}$,
we have
 \[
 \begin{array}{ll}
\Expect_I [\|(w^\star*a)_I\|_2 \leq \Expect_I [\|(w^r*a)_I\|_2,
\end{array}
  \]
  therefore,
  \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2.
\end{array}
  \]
Due to the bi-Lipschitz property of $\Expect_I \|(e_0+\phi)_I\|_2$ around $e_0$, we know when $p<p^\star$, $B(p, \phi)$ is positive and bounded by a constant.

Therefore, as $p<p^\star$, $B(e_0,\phi^\star)$ and $B(e_0,\phi^r)$ are both upper and lower bounded. 
 \[
 \begin{array}{ll}
   \|\phi^\star \|_2 \leq \frac{B(e_0,\phi^r)}{B(e_0,\phi^\star)} \|\phi^r \|_2.
\end{array}
  \]
 Using the previous theorem, 
 \[
 \begin{array}{ll}
   \|\phi^\star \|_2 \leq \frac{B(e_0,\phi^r)}{B(e_0,\phi^\star)} \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( -2 r\big(\rho_{k_1}+ \ldots+ \rho_{k_n} \big) \Big),
\end{array}
  \]
 using asymptotic exponential convergence bound on $\|\phi^r \|_2$ as 
  $r \rightarrow \infty$, it converges to zero at an exponential rate
  \[
 \begin{array}{ll}
   \|\phi^\star \|_2 
   \leq
   O(
\exp \Big(-  r \min_i (\rho_i) \Big) ), \quad r \rightarrow \infty.
\end{array}
  \]
\end{proof}


==> old_sec/sec_old_2020/Result_noise.tex <==
\section{Robustness under moving average Gaussian noise }
Consider a convoluted Gaussian noise with an average standard deviation $\sigma$ and a forward moving average filter $b$ with unit norm $\|b\|_2=1$, then
 \[
\begin{array}{ll}
Y&= a* (X+ \sigma b*G).
\end{array}
\]


This model would include the case of IID mixture of sparse Gaussian and small Gaussian $X_t \sim p N(0,1) +(1-p) N(0,\sigma_1)$ with $\sigma = \sigma_1$ and $b=e_0 $.
It also includes the Gaussian observation noise model
\[
\begin{array}{ll}
Y&= a* X+  \sigma_2 G_2 = a* (X+  \sigma_2 a^{-1}*G_2),
\end{array}
\]
with $b = a^{-1}/\|a^{-1}\|_2$, and $\sigma = \sigma_2 \|a^{-1}\|_2$.

 \begin{theorem}
 \label{thm:rand_exact_rob}
 Let $\psi^\star$ be the solution of the convex optimization problem in Eq.(4.1) for the moving average random noisy model
  \[
\begin{array}{ll}
Y&= a* (X+ \sigma b*G),
\end{array}
\]
 then
\label{thm:Bound_Normal_Noise}
\[
B(e_0, \psi^\star-e_0) \|\psi^\star -e_0\|_2 = \E_I  \| (\psi^\star)_I \|_2 -\E_I  \| (e_0)_I \|_2 \leq  (1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1).
\]
When $\sigma\leq 1,$
\[
(1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1)  \leq \sigma,
\]
therefore, when $p<p^\star$, $\sigma\leq 1,$ there exists a constant $C$,
\[
 \|\psi^\star -e_0\|_2 \leq C \sigma.
\]
\end{theorem}  

\section{Robustness under adversarial noise }
In the adversarial noise setting, we observe
\[
	\begin{array}{ll}
	Y&= a* (X+  \zeta) 
	\end{array}
	\]
where $\zeta$ is a sequence chosen by an adversary under constraint:	
\[
	\| \zeta\|_\infty \leq \eta.
	\]
% \paragraph{Robustness of convex blind deconvolution}
 \begin{theorem}
\label{thm:adv_exact_rob}
	Under adversarial noise, 
% 	when the samples
% 		$
% N \geq  O(k\log(k)),
% $ and $p<p^\star - \epsilon_N$,
Let $w^\star$ be the solution of the population convex optimization
	\[
 \begin{array}{ll}
 \underset{w }{\mbox{minimize}}   &\E \frac{1}{N}\|w*Y\|_{\ell_1(\cT_N)}\\
\mbox{subject to}  
& (\alpha*w)_0 =1.
\end{array}
  \]
Define $\psi^\star = a*w^\star$; then $\psi^\star$ satisfies the following bound:
 \[
 \begin{array}{ll}
B(e_0, \psi^\star-e_0) \|\psi^\star -e_0\|_2 = \E_I  \| (\psi^\star)_I \|_2 -\E_I  \| (e_0)_I \|_2 \leq 
 p\sqrt{\frac{2}{\pi}}(\mathcal{R}(\eta) - 1)+(1-p)\eta.
\end{array}
  \]  
  Here $\mathcal{R}(\eta)$
is the folded Gaussian mean, for standard Gaussian $G$:
\[
\mathcal{R}(\eta) :=  \sqrt{\frac{\pi}{2}} E_G |\eta+  G| = \exp\{-\eta^2/2\} + \sqrt{\frac{\pi}{2}}\eta \left(1 - 2\Phi\left(-\eta\right) \right).
\]  
$\mathcal{R}(\eta)-1$ is an even function that is monotonically non-decreasing for $\eta \geq 0$ with quadratic upper and lower bound: there exists constants $C_1\leq C_2$,
  \[
C_1 \eta^2 \leq \mathcal{R}(\eta)-1 \leq C_2 \eta^2, \forall \eta.
\]
  
Therefore, when $p<p^\star$, $B(e_0, \psi^\star-e_0)$ is a bounded positive constant, there exists a constant $C$, so that
 \[
 \|\psi^\star -e_0\|_2  \leq C  \eta, \forall \eta > 0.
 \]
\end{theorem}  



% 	\begin{theorem}
% 	\label{thm:adv_relax_rob}
% 	Under adversarial noise $\| \zeta\|_2 \leq \eta$, 
% % 	when the samples
% % 		$
% % N \geq  O(k\log(k)),
% % $ and $p<p^\star - \epsilon_N$,
% the solution of the population convex optimization
% 	\[
%  \begin{array}{ll}
%  \underset{w, z }{\mbox{minimize}}   & \E \frac{1}{N}\|w*Y -z\|_{\ell_1(\cT_N)}\\
% \mbox{subject to}  
% &  \|z\|_2^2 \leq \eta^2\\
% & (\alpha*w)_0 =1
% \end{array}
%   \]
%   is $w^\star$ and $z^\star$,then
% $x^\star:=w^\star*Y -z^\star$	is $(X_t)_{t\in [N]}$ up to shift and scaling.	
% 	\end{theorem}


\section{Proofs}
\subsection{Gaussian noise robustness proof}
\begin{proof}[Proof of Theorem~\ref{thm:rand_exact_rob}]
Consider the noisy model
 \[
\begin{array}{ll}
Y&= a* (X+  \sigma b*G).
\end{array}
\]
 First, 
\[
 \begin{array}{ll}
 F_{\sigma}(\psi)= \Expect_{G} \Expect_X|\psi^T X+\sigma \psi^T (b* G) | = 
   \Expect_{G} \Expect_I | \sqrt{ \|\psi_I\|_2^2  + \sigma^2\|C_{b}^T \psi\|_2^2}G |,
\end{array}
  \]
where $C_{b}$ is the Topelitz matrix with the first column being $b$.
  
Let $\psi^\star $ be the optimization solution, when $p<p^\star$,  we have  a chain of inequality:
    \[
 \begin{array}{ll}
F_{\sigma}(e_0)
 \geq F_{\sigma}(\psi^\star ) 
 \geq F_{0}(\psi^\star )
 \geq F_{0}(e_0).
\end{array}
  \]
  We have 
\[
 \begin{array}{ll}
 F_{\sigma}(e_0)
 &= 
\Expect_{G} \Expect_I | \sqrt{ \|(e_0)_I\|_2^2  + \sigma^2\|b\|_2^2}G | \\
&= 
\Expect_{G} \Expect_I | \sqrt{ \|(e_0)_I\|_2^2  + \sigma^2}G | \\
  &=
 \sqrt{\frac{2}{\pi}}[ 
 (1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }) ].
\end{array}
  \]
  
Therefore, when $p<p^\star$
   \[
 \begin{array}{ll}
F_{\sigma}(e_0)-F_{0}(e_0) 
 \geq F_{0}(\psi^\star )-F_{0}(e_0) \geq 0.
\end{array}
  \]
  \[
B(e_0, \psi^\star-e_0) \|\psi^\star -e_0\|_2 = \E_I  \| (\psi^\star)_I \|_2 -\E_I  \| (e_0)_I \|_2 \leq  (1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1). 
\]
When $\sigma\leq 1,$
\[
(1-p) \sigma +
 p(\sqrt{1+ \sigma^2 }-1)  \leq \sigma,
\]
therefore, when $p<p^\star$, $\sigma\leq 1,$ there exists a constant $C$,
\[
 \|\psi^\star -e_0\|_2 \leq C \sigma.
\]
\end{proof}



\subsection{Adversarial noise robustness proof}
Our data generative model is
\[
	\begin{array}{ll}
	Y&= a* (X+  \zeta),
	\end{array}
	\]
where 	
\[
	\| \zeta\|_\infty \leq \eta.
	\]

% \begin{proof}[Proof of theorem~\ref{thm:adv_exact_rob} and theorem~\ref{thm:rand_exact_rob} jointly]

\begin{proof}[Proof of Theorem~\ref{thm:adv_exact_rob}]
The population convex optimization is
	\[
 \begin{array}{ll}
 \underset{w, z }{\mbox{minimize}}   & \E \frac{1}{N}\|w*Y\|_{\ell_1(\cT_N)}\\
\mbox{subject to}  
& (\alpha*w)_0 =1.
\end{array}
  \]
 By change of variable $\tilde{\psi} = w*a$, it could be reduced to a simpler problem 
  \[
 \begin{array}{ll}
 \mbox{minimize}_{w,s}   & \Expect|\psi^T (X+  \zeta)| \\
\mbox{subject to}  
& u^T \psi =1.
\end{array}
  \]
% Let $\psi(\zeta)$ be the optimization solution of problem with respect to a fixed $\zeta$.
% Let the objective be
% \[
% F(\psi,\zeta):=\Expect|\psi^T (X+ \zeta)| = \Expect_I  | \|\psi_I\|_2 G  +  \psi^T\zeta  |
% \]
 Let $\psi^\star $ be the optimization solution of the worst-case objective  over all possible $\zeta$, defined as $F_{\eta}(\psi)$:
 \[
 \begin{array}{ll}
 F_{\eta}(\psi)
 &= \sup_{\zeta: \| \zeta\|_\infty \leq \eta } \Expect|\psi^T (X+ \zeta)| \\
 &= \sup_{\zeta: \| \zeta\|_\infty \leq \eta } \Expect_I  | \|\psi_I\|_2 G  + \psi^T \zeta  |,
\end{array}
  \] 
   when $p<p^\star$,  we have a chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta}(e_0)
 \geq F_{\eta}(\psi^\star ) 
%  \geq F(\psi(\zeta),\zeta)
 \geq F_{0}(\psi^\star )
 \geq F_{0}(e_0).
\end{array}
  \]
%   and 
%   \[
%  \begin{array}{ll}
% F_{\eta}(e_0)
%  \geq F_{\eta}(\psi^\star ) 
%  \geq F(\psi(\zeta),\zeta)
%  \geq F_{0}(\psi(\zeta) )
%  \geq F_{0}(e_0) 
% \end{array}
%   \]
   Therefore, when $p<p^\star$
   \[
 \begin{array}{ll}
F_{\eta}(e_0)-F_{0}(e_0) 
\geq F(\psi(\zeta),\zeta)-F_{0}(e_0)
 \geq F_{0}(\psi^\star )-F_{0}(e_0) \geq 0.
\end{array}
  \]
  Therefore,
 \[
 \begin{array}{ll}
B(e_0, \psi^\star-e_0) \|\psi^\star -e_0\|_2 = \E_I  \| (\psi^\star)_I \|_2 -\E_I  \| (e_0)_I \|_2 .
\end{array}
  \]   
  
From the folded Gaussian mean formula, let $G$ be scalar standard Gaussian, we have 
\[
 \begin{array}{ll}
 F_{\eta}(e_0)
  &= \sup_{\zeta: \| \zeta\|_\infty \leq \eta } \Expect_I  \E_G| \|(e_0)_I\|_2 G  +  \zeta_0  |\\
&= 
\sup_{\zeta: \| \zeta\|_\infty \leq \eta} [p\E_G | G  +  \zeta_0  |+ (1-p)|\zeta_0|]\\
  &=
\sup_{\zeta: \| \zeta\|_\infty \leq \eta}[  p \sqrt{\frac{2}{\pi}} \mathcal{R}(\zeta_0) + (1-p)|\zeta_0|]
\\
 &=
p \sqrt{\frac{2}{\pi}} \mathcal{R}(\eta) + (1-p)\eta.
\end{array}
  \]
 The last inequality comes from the fact that $\mathcal{R}(\zeta_0)$ is an even function that is monotonically non-decreasing for $\zeta_0 \geq 0$. 
 We will prove this conclusion below:
 \[
 \begin{array}{ll}
B(e_0, \psi^\star-e_0) \|\psi^\star -e_0\|_2 = \E_I  \| (\psi^\star)_I \|_2 -\E_I  \| (e_0)_I \|_2 \leq 
 (1-p)\eta + p \sqrt{\frac{2}{\pi}} (\mathcal{R}(\eta) - 1).
\end{array}
  \] 



\end{proof}


% \subsection{Tool: folded Gaussian mean formula}
\paragraph{Tool: folded Gaussian mean formula}
From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right),
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
As a related remark, its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2.
\eeq  
% The variance will be useful for concentration with finite sample.  

 \begin{lemma}
\label{lem:FoldedGaussian}
We define the ratio of folded Gaussian mean as 
\[
\mathcal{R}(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G| = \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right).
\]

$\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.

We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8).
\EEA
When $\gamma<1,$ 
\[
 (\frac{3}{2} + \frac{1}{24}) \gamma^2 \geq  \mathcal{R}(\gamma) -1\geq  \frac{3}{2}\gamma^2.
\]
When $\gamma<M$ for $M>1$, this lemma can be generalized:
there exists constants $C'\leq C$,
\[
C' \gamma^2 \leq \mathcal{R}(\gamma)-1 \leq C \gamma^2.
\]
 \end{lemma}
\paragraph{Proof for folded Gaussian mean}
\begin{proof}[Proof of lemma~\ref{lem:FoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right).
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma,
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right],
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right].
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!},
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8). 
\end{array}
  \] 
  
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition with the inner function being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1.
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6).
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4)).\\
\end{array}
\] 
Combining the above:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right].\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8).
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0.
\end{array}
\] 

When $\gamma<1,$ 
\[
 (\frac{3}{2} + \frac{1}{24}) \gamma^2 \geq  \mathcal{R}(\gamma) -1\geq  \frac{3}{2}\gamma^2.
\]
When $\gamma<M$ for $M>1$, this lemma can be generalized:
there exist constants $C'\leq C$,
\[
C' \gamma^2 \leq \mathcal{R}(\gamma)-1 \leq C \gamma^2.
\]
\end{proof}



% \begin{proof}[Proof of  theorem~\ref{thm:adv_relax_rob} ]
% The population convex optimization for a general choice $\epsilon \in [0, \eta]$ is
% 	\[
%  \begin{array}{ll}
%  \underset{w, z }{\mbox{minimize}}   & \E \frac{1}{N}\|w*Y -z\|_{\ell_1(\cT_N)}\\
% \mbox{subject to}  
% &  \|z\|_2^2 \leq \epsilon^2\\
% & (\alpha*w)_0 =1
% \end{array}
%   \]
%  by change of variable $\tilde{\psi} = w*a$, it could be reduced to a simpler problem 
%   \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,s}   & \Expect|\psi^T (X+  h*\zeta) -  \epsilon s| \\
% \mbox{subject to}  
% & u^T \psi =1,\\
% & s^2 \leq 1
% \end{array}
% % \tag{$P^c_{1,\epsilon}$}
%   \]
%   When $\epsilon =0$, we have the original problem.
  
  
  
 






==> old_sec/sec_old_2020/Stability_old.tex <==

\paragraph{Finite length approximation by Z-transform truncation }

Let $\gamma>0$, then we define 
\[
\bar a^{\gamma} :=e_0-\gamma a
\]
with Z-transform 
\[
\bar A^{\gamma}(z) :=1-\gamma A(z)
\]
then
\[
 \begin{array}{ll}
1/A(z) &=  \gamma(1-\bar A^{\gamma}(z))^{-1}\\
&= \gamma[ 
\sum_{i=0}^{\infty} (\bar A^{\gamma})^i]
\end{array}
  \]
We can construct an approximation 
$w^{r,\gamma} \in V_{rs, rt} $ of length $r(1+s+t)$ 
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
with Z-transform
\[
 \begin{array}{ll}
W^{r,\gamma}(z) 
&= \gamma[\sum_{i=0}^{r} (\bar A^{\gamma}(z))^i] \\
&= \frac{1-(\bar A^{\gamma}(z))^{r+1}}{A(z)} 
\end{array}
\]
then
\[
a*(a^{-1}-w^{r,\gamma}) 
= *_{r+1} (\bar a^{\gamma})
\]
\begin{lemma}
\[
\|a*(a^{-1}-w^{r,\gamma})\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 
= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
 \]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt\\
&= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
\end{array} \]
\end{proof}


First, since:
%   \[
%  \begin{array}{ll}
%  \|\hat{\bar a}^{\gamma}\|_{\infty} \geq \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% Notice that 

\[
 \begin{array}{ll}
 \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2} = (|\hat{\bar a}^{\gamma}|^2(t_0))^{r+1} \geq  \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt
\end{array}
\]
We have a natural upper bound as
\[
 \begin{array}{ll}
\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}\leq \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2}
\end{array} \]
In the following we give a more accurate calculation of $\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}$ using Laplace method.
% Then using Parseval’s identity, 
%   \[
%  \begin{array}{ll}
% \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% (Here we remark that the Fourier transform and inverse Fourier transform are define as follows so that the there is no constant for Parseval’s identity)
% \[
% \mathcal{F}a(\omega) = \hat{a}(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]
% \[
% (\mathcal{F}^{-1} \hat{a})(n) =  \int_{\frac{-1}{2}}^\frac{1}{2} \hat{a}(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
% \]

%  Since $\|\hat{\bar a}^{\gamma}\|^2_{\infty} \geq
%  \|\hat{\bar a}^{\gamma}\|^2_{\infty} \leq \|\hat{\bar a}^{\gamma_2}\|^2_{2}  = \|\bar a^{\gamma} \|_{2} =  \sin{\theta}$.



\paragraph{Laplace's method}
 \begin{theorem}[Laplace's method]
 \label{Laplace}
  For $\bar a^{\gamma} :=e_0-\gamma a$, $a$ has a length $L$ window of non-zero entries.
 \BIT
 \item
 let $F(t) = |\bar a^{\gamma}(t)|^2$, and let $f(t) := \log F(t) = \log| \hat{\bar a}^{\gamma}|^2$ and $t_0 = \arg\max_{t\in [\frac{-1}{2},\frac{1}{2}]} F(t)$ achieves the global maximum, and let the maximum value be $F_{\max} :=F(t_0) = |\hat{\bar a}^{\gamma}(t_0)|^2$. 
\item
We define the second moment 
%   $M_2\leq \sum_{|k|\leq 2L} k^2$,
  \[M_2: = \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k)\]
  then $M_2$ is finite, upper bounded by $\frac{16}{3}(L+1)^3 \| \bar a^{\gamma}\|_2^2$ and $f$ is twice  differentiable near $t_0$.
%   with $|f''(t_0)|\leq M_2/F_{\max} $.
% \item
%  Assume
%  $F_{\max}<1$.
 \EIT
We have
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}  
  &= \int_{\frac{-1}{2}}^\frac{1}{2}  \exp((r+1)f(t)) dt  \\
  &=  [(\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0))](1+O(r^{-1})) 
  \\
  &=   [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.
\end{theorem}
\begin{proof}
From optimality $F'(t_0) =0,$ and 
\[
 \begin{array}{ll}
|f''(t_0)| &= |\partial^2 \log F(t_0)| \\
&= \frac{ |F''(t_0)|}{|F(t_0)|} 
\end{array}
\]

For $f$ to be twice  differentiable near $t_0$ with $|f''(t_0)|$, we only need to upper bound 
\[
|F''(t_0)|=|[\hat{\bar a}^{\gamma}]''(t_0)|^2 \leq \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k).
\]
As
\[
\frac{ M_2}{\|\bar a^{\gamma}\|_2^2}\leq \sum_{|k|\leq 2L} k^2.
\]
and  $a$ is of length $L = 1+s+t$, we know that $\bar a^{\gamma}  *  \tilde{\bar a}^{\gamma} $ is of length at most $2L$, then 
\[
\sum_{|k|\leq 2L} k^2 = 1+\frac{2L(2L+1)(4L+1)}{3}\leq \frac{16}{3}(L+1)^3.
\]

Then $f$ to be twice  differentiable near $t_0$ and
\[
 \begin{array}{ll}
|f''(t_0)| 
&= \frac{ |F''(t_0)|}{|F(t_0)|} \\
&\leq  \frac{ M_2}{F_{\max}}
\end{array}
\]

Now we go back to the main quantity,
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} &= \int_{\frac{-1}{2}}^\frac{1}{2} |\hat{\bar a}^{\gamma}(t)|^{2r+2} dt  \\
  &= \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  
\end{array}
\]
By Laplace's asymptotic method,
 \[
  \begin{array}{ll}
  & \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  \\
  =&\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.

Combining all the previous bounds, we have
\[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} 
  &= \sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))  \\
 &= [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
\end{proof}

\paragraph{Stability theorem}
Combing the calculation of expectation, the construction of finite length inverse, the Laplace method calculation, we arrive at our final result.
\begin{theorem} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then provided $p<p^\star - \delta$, we have
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq  [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
 \]
\end{theorem}
\begin{proof}
From previous result, 
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq \|a*(w^{r,c} -a^{-1}) \|_2^2
 \]
 and previous the previous construction of $w^{r,c}$, we know that 
 \[
 \|a*(w^{r,c} -a^{-1}) \|_2^2 \leq [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1})).
 \]
Hence we prove the geometric convergence for any $F_{\max} <1$.
\end{proof}


\paragraph{Sufficient condition for $F_{\max} <1$}
\begin{lemma}
Let
 \[
 \gamma_2 = \arg\min_{\gamma>0} \|\bar a^{\gamma} \|_{2}^2
 \]
 Then $\gamma_2 = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
And
  \[
 \|\bar a^{\gamma_2} \|_{2}^2 = 1- \gamma_2^2 = \sin^2{\theta}
 \]
 
\end{lemma}
\begin{proof}
Using the fact that $a_0 =1$, $\|a\|_2 = \frac{1}{\cos{\theta}}$,
\[
 \begin{array}{ll}
\|\bar a^{\gamma} \|_{2}^2 
&= 1+ \gamma^2 \|a\|_2^2 -2\gamma a_0\\
&= 1+ \gamma^2 \frac{1}{\cos^2{\theta}} -2\gamma \\
&= \frac{1}{\cos^2{\theta}} (\gamma - \cos^2{\theta})^2 + (1-\cos^2{\theta})
\end{array} \]
Hence $\|\bar a^{\gamma} \|_{2}^2 $ is mimimized at $\gamma_2 = \cos^2{\theta}$ with value $1-\cos^2{\theta}=\sin^2{\theta}$.
\end{proof}

Remark:
Is there any way to directly optimize $\|\hat{\bar a}^{\gamma}\|_{\infty}$? Would there be an improvement over optimize 2 norm?

\begin{lemma}
Let $S_a := \sum_{j\neq 0} |a_j|$, 
\[
 \gamma_\infty = \arg\min_{\gamma} \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 \]
 if $S_a<1,$ then  
 \[
 \gamma_\infty = 1
 \]
 and 
  \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]

%  Then $c = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
% And
%   \[
%  \|\bar a^{c} \|_{2}^2 = 1- c^2 = \sin^2{\theta}
%  \]
 
\end{lemma}
\begin{proof}
 Since
 \[
 \begin{array}{ll}
|\hat{\bar a}^{\gamma}(t)|^2
 &=  |\bar A^{\gamma}(e^{2\pi i  t})|^2  \\
 &= |1-\gamma A(e^{2\pi i  t})|^2 \\
 &= (1-\gamma A(e^{2\pi i  t}))(1-\gamma A(e^{-2\pi i  t})) \\
 &= 1 + \gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))
 \end{array} \]

 \[
 \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 = 1 + \max_{t\in [\frac{-1}{2},\frac{1}{2}]} [\gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))]
 \]
Since the coefficient $a_i$ are all really, we check different $t.$
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(0)|^2
  &= |1-\gamma (\sum_j a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} a_j)|^2
  \end{array}
 \]
 
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(\frac{1}{2})|^2
  &= |1-\gamma (\sum_i (-1)^{|j|} a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (-1)^{|j|}  a_j)|^2
  \end{array}
 \]
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2
  \end{array}
 \]
then
\[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2\\
  &\leq |(1-\gamma) + \gamma S_a|^2
  \end{array}
 \]
 if $S_a<1,$ then
 \[
  \begin{array}{ll}
  \min_\gamma |(1-\gamma) + \gamma S_a|^2 =  |S_a|^2<1.
  \end{array}
 \]
 Therefore if $S_a<1$,  $\gamma_\infty =1,$ and 
 \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]
\end{proof}

Remark: from this paragraph, we see upper and lower bound for $F_{\max}$, by choosing $\gamma =1,$ we have
\[
F_{\max}   \leq |S_a|^2
\]
also, we see that
\[
F_{\max}   \geq  \|\bar a^{1} \|_{2}^2 
=  \frac{1}{\cos^2{\theta}} -1 = \tan^2{\theta}
\]
So a natural consequence is that 
\[
\tan^2{\theta}   \leq |S_a|^2
\]
If $S_a<1$, we need $\tan^2{\theta}<1$, therefore $\theta<\frac{\pi}{4}$.

\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

For $\gamma\in (0,1)$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
\[
\|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
=  (1-\gamma_2)^2 + (\gamma_2 s)^2 
= \frac{s^2}{1+s^2}
\]
And in this case,
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty
&= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
&=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
 \end{array} \]
 
 Therefore, 
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
 \end{array} \]

==> old_sec/sec_old_2020/Subgradient.tex <==
\section{Phase transition based on directional derivative and subgradient condition}
\paragraph{Exact calculation of subgradient for phase transition }
In this section, we give a clean proof of phase transition theorems presented before using sub-gradient and directional derivative.

\begin{lemma}
Let $J \subset [n]$ be the support of $X$, let $\psi_J : = \psi\cdot 1_J$ denote the elementwise product of vector $\psi$ with the indicator vector of subset $J$.  Let $B_J$ denote the central section of the euclidean  ball $B(\reals^n)$,
where the slice is produced the linear space $\mbox{span} \{e_i : i\in J \}$.
Alternatively, we may write
$B_J: = \{ v_J: \| v_J\|_2 \leq 1\}$.  The set-valued subgradient
operator applied to $\|\psi_J\|$
evaluates as follows:
 \[
 \begin{array}{ll}
\partial_{\psi}    \| \psi_J \|
&=  N(\psi_J).
\end{array}
  \]
Here $N$ maps $\reals^n$ into  subsets of $\reals^n$,
and is given by:
\[
N(\psi_J):= 
\begin{cases}
    \psi_J/\|\psi_J\|_2, &  \psi_J\neq 0 \\
    B_J, &  \psi_J = 0
  \end{cases}.
\]  
\end{lemma}

\begin{definition}
Consider a probability space containing just the possible  
outcomes  $J \subset [n]$.
Let $S_J$, $J \subset [n]$,  denote a closed compact subset of $\reals^n$.
Let $I$ be a random subset of
$[n]$ drawn at random from this probability space with probability $\pi_J = P\{ I = J \}$
of elementary event $J$.
Consider the set-valued random variable $S \equiv S_J$. We define its expectation as
\[
 {\Expect} S  := \sum_J \pi_J \cdot S_J.
\]
On the right side, we mean the closure of the 
compact set produced by all sums of the form
\[
 \sum_J \pi_J \cdot s_J
\]
where each $s_J \in S_J$.
\end{definition}

\begin{lemma}
For any $\psi \in \reals^n$, and $X = (X_i)_{i=1}^n$ with $X_i \sim_{iid} BG(p,0,1)$.
Let now $I \subset [n]$ be the random support of $X$.
Let $\partial_\psi $ denote the set-valued subgradient
operator.
  \[
 \begin{array}{ll}
\partial_\psi [E{|\sum_{i} \psi_i X_i| }  ]
%&=  {\Expect}\,{\mbox{\rm sign}(\psi^T X) X }  \\
&= \sqrt{\frac{2}{\pi}} \cdot {\Expect}_I [N(\psi_I)].
\end{array}
  \]
\end{lemma}

\paragraph{Subgradient and directional derivative at $e_0$}
Now we focus on $e_0$. Note that for any subset $J \subset [n]$, $(e_0)_J$ is either the zero
vector or else $e_0$. Hence $N((e_0)_J)$
is either $B_{J}$ or $\{e_0\}$. What drives
this dichotomy is whether $0 \in J$ or not.

\begin{lemma}  
\[
 \begin{array}{ll}
\Expect_I [N((e_0)_I) ]
&= p e_0 + \sum_{J,0\not\in J } \pi_{J} B_{J} \\
& = p e_0 + (1-p) {\cal B}_0,
\end{array}
  \]
where
\[
 \begin{array}{ll}
{\cal B}_0 = \Expect_{I}[ B_{I} | 0 \not \in I ] = 
(1-p)^{-1} \cdot \sum_{J,0\not\in J } {\pi_{J}} B_{J}.
\end{array}
\]
 
\end{lemma}


\begin{proof}
\begin{eqnarray*}
\Expect_I [N((e_0)_I) ] &=& \sum_{J } \pi_{J} B_{J} \\
&=&  \sum_{J, 0 \in J}   \pi_{J} e_0 +  \sum_{J,0\not\in J }  \pi_{J} B_{J}\\
&=& p \cdot e_0 + (1-p) \cdot {\cB}_0 .
\end{eqnarray*}
 \end{proof}
To compute with $\Expect_I [N((e_0)_I) ]$,
we need:
\begin{lemma} \label{eq:ComputeExpect}
For each fixed $\beta \in \reals^n$:
\[
  \sup_{b \in {\cal B}_0} \langle \beta, b \rangle
   = \Expect_{I}[ \|\beta_I\|_2 | 0 \not \in I  ].
  \]
\end{lemma}

\begin{proof}
Note that in the definition of the set 
\[
{\cal B}_0 = \Expect_{I}[ B_{I} | 0 \not \in I ],
\]
 each term $B_J$ obeys the bound
$\sup_{g_J \in B_J} \|g_J\|_2 = 1 $.
Now, given the fixed vector $\beta \in \reals^n$, define:
\begin{eqnarray*}
    b^* &=& \Expect_{I}[ \frac{\beta_I}{\| \beta_I \|_2} | 0 \not \in I  ]\\
     &=&  \sum_{0 \not \in J} \pi_J \frac{\beta_J }{\|\beta_J\|_2}.
 \end{eqnarray*}
 Since each term in this sum has Euclidean norm at most $1$, $b^* \in {\cB}_0$.
Now
\begin{eqnarray*}
\langle  \beta, b^* \rangle &=&
\langle \beta , \sum_{0 \not \in J} \pi_J \frac{\beta_J }{\|\beta_J\|_2} \rangle \\
&=& \sum_{0 \not \in J} \pi_J \langle \beta , \frac{\beta_J }{\|\beta_J\|_2} \rangle \\
&=& \sum_{0 \not \in J} \pi_J \|\beta_J\|_2 .
 \end{eqnarray*}
On the other hand, for any fixed 
vector $g = \sum \pi_J g_J $,
with each $g_J \in B_J$,
we have
\begin{eqnarray*}
\langle  \beta, g \rangle &=&  \sum_{0 \not \in J} \pi_J \langle \beta , g_J  \rangle \\
&\leq& \sum_{0 \not \in J} \pi_J  \|\beta_J \|_2 \|g_J\|_2 \\
& \leq & \sum_{0 \not \in J} \pi_J  \|\beta_J \|_2 
= \langle  \beta, b^* \rangle.
 \end{eqnarray*}
\end{proof}

Lemma (\ref{eq:ComputeExpect}) 
can be viewed as a special instance of
Theorem \textbf{A.15} from \cite{bai2018subgradient}:
\begin{lemma}[Interchangeability of set expectation and support function] 
Suppose a random compact set $S \subset \reals^n$ is integrably bounded and the underlying probability space is non-atomic, then $\E[S]$ is a convex set and for any fixed vector $\beta \in \reals^n,$
 \begin{equation} \label{eq:SetExpectEquality}
 \sup_{g\in \Expect S} \langle\beta, g\rangle =  \sup_{g\in  S} \Expect\langle\beta, g\rangle .
 \end{equation}
\end{lemma}

Define $\beta_{(0)} = \beta \cdot 1_{\{0\}^c}$ as the part of $\beta$ supported away from $0$.
Further define 
\[
V_1(\beta_{(0)}):= \frac{\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]}{\|\beta_{(0)}\|_2}.
\]
Let $N = \|\beta_{(0)}\|_0$; then 
 $V_1(\beta_{(0)})$ satisfies
\beq 
 p  \leq  V_1(\beta_{(0)}) \leq \sqrt{p} .
\eeq

\begin{lemma}


 The directional derivative at $e_0$ along $\beta$ 
 evaluates to the following:
 \BEAS
 \lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2]) 
 &=&  p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
 &=& [p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} V_1(\beta_{(0)})] \|\beta\|_2.
 \EEAS
\end{lemma}
 \begin{proof}

Let $\langle b, v \rangle  \equiv b^T v$.

Applying Lemma \ref{eq:ComputeExpect}, we proceed as follows:
\[
 \begin{array}{ll}
\lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
&= \sup_{g\in \Expect_I [N((e_0)_I)]} \langle\beta, g\rangle\\
% &= \sup_{g\in  [N((e_0)_I)]} \Expect_I\langle\beta, g\rangle\\
&= p \cdot \langle\beta, e_0\rangle + (1-p) \cdot  \sup_{g\in {\cal B}_0 } \langle\beta, g\rangle\\

&= p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] \\
&= [p \cdot \cos{\angle(\beta, e_0)} + (1-p) \cdot  \sin{\angle(\beta, e_0)} V_1(\beta_{(0)})] \|\beta\|_2.
\end{array}
  \]
  \end{proof}


\paragraph{Projected subgradient}
\begin{lemma} 
If $\beta$ must satisfy a constraint $u^T \beta =0$, then we only consider directional derivative at $e_0$ along $\beta$ for those $\beta$ that $u^T \beta =0$.
Therefore, let $P_{u}^{\perp}$ be the projection onto the hyperplane as the orthogonal complement of $u$, then the following three equivalent conditions all make sure $e_0$ is the stationary point.
\BIT
\item
  \[
 \begin{array}{ll}
0\in P_{u}^{\perp} \Expect_I [N((e_0)_I) ].
\end{array}
  \]
  \item
Equivalently, there exists a subgradient $g\in  P_{u}^{\perp} \Expect_I [N((e_0)_I) ]$ such that for all $\beta$ satisfying $u^T \beta = 0$,
\[
\beta^T g \geq 0.
\]
\item
Also equivalently, for all $\beta$,
\[
 \begin{array}{ll}
\sup_{g\in  [N((e_0)_I)]}\Expect_I[ \langle   P_{u}^{\perp}  \beta, g\rangle] \quad \geq 0.
\end{array}
  \]
  \EIT
\end{lemma}
 
Let $\theta = \angle({u, e_0})$, for $\beta$ need to satisfy a constraint $u^T \beta =0$, we get
\[
 \begin{array}{ll}
\lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
% &= \sup_{g\in \Expect_I [N((e_0)_I)]} <\beta, g\rangle\\
&= [p \cos{\angle(\beta, e_0)} + (1-p)  V_1(\beta_{(0)}) \sin{\angle(\beta, e_0)}] \|\beta\|_2.
\end{array}
  \]
Here $\angle(\beta, e_0)\in [0, \pi], \sin{\angle(\beta, e_0)}\in [0,1]$. 
  
\begin{figure} 
\centering
\includegraphics[width=.55\textwidth]{./figures_BD/Angle_Diagram_label.png}
\caption{Demonstration of the relation between
  $\angle( \beta, -e_0)$ and ${\angle(u, e_0)}$.}
\label{fig-Angle}
\end{figure}
  
\begin{lemma}
  \label{Angle_Inequality}
   \[
  \angle(  \beta, - e_0) \geq \angle(P_u^\perp (-e_0), -e_0)= \frac{\pi}{2} - \theta
  \]
  
    \[
  \tan(\angle(  \beta, - e_0)) \geq \tan\angle(P_u^\perp (-e_0), -e_0) =\cot{\theta}
  \]
\end{lemma}
  
\begin{proof}
   
%   Let  $e_{0,u} = N(P_{u}^{\perp} e_0)$ be the unit vector along $P_{u}^{\perp} e_0$, then 
We know that geometrically, using the property that projection of $e_0$ on the hyperplane with normal vector $u$ has the smallest angle among all the $\beta$ in that hyperplane, we have that if
   \[
  \angle(  \beta, - e_0) \geq \angle(P_u^\perp (-e_0), -e_0) = \frac{\pi}{2} - \angle(u, e_0) = \frac{\pi}{2} - \theta,
  \]
then
  \[
  \tan\angle(  \beta, - e_0) \geq \tan\angle(P_u^\perp (-e_0), -e_0)= \cot{\theta}.
  \]
 
\end{proof}
  
Let $H_u=\{\beta : \quad u^T \beta =0 \}$. We define the phase transition threshold as
  \[
 p^\star:= 
 \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))> 0\}.
 \]
 \begin{lemma}
Then 
 \[
\frac{p^\star}{1-p^\star}=  \inf_{\| \beta\|_2=1, u^T \beta =0} \tan(\angle( \beta_{(0)}, -e_0)) V_1(\beta_{(0)}).
\]
For all $p<p^\star$ the convex program finds the correct inverse filter $a^{-1}$ and hence the sparse signal $X$.
\end{lemma}
  


\begin{proof}
 
We know that the KKT condition of the convex program is
  \[
  p \cos{\angle(\beta, e_0)} + (1-p)  V_1(\beta_{(0)}) \sin{\angle(\beta, e_0)}>0,
  \]
  if and only if 
  $\cos{\angle(\beta, e_0)}\geq 0,$ or $\cos{\angle(\beta, e_0)}<0$ and 
  \[
      \frac{1-p}{ p}  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}>1.
  \]
  If $\cos{\angle(\beta, e_0)}<0, \cos{\angle(\beta, -e_0)}>0, \angle(\beta, -e_0) \in [0, \frac{\pi}{2}).$ 
  
  Therefore,
  \[
      \frac{1-p}{ p}  \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan\angle(  \beta, - e_0)>1,
  \]
  
  \[
\frac{p^\star}{1-p^\star}=  \inf_{\| \beta\|_2=1, u^T \beta =0} \tan(\angle( \beta_{(0)}, -e_0)) V_1(\beta_{(0)}).
\]
   \end{proof}
 
  
\begin{theorem}
 \label{thm:PT_lower}
The threshold $p^\star$ satisfies 
		\[ 
\tan(\angle( P_u^\perp (-e_0), -e_0)) p^\star \leq \frac{p^\star}{1-p^\star} \leq	\tan(\angle( P_u^\perp (-e_0), -e_0)) V_1(P_u^\perp (-e_0)).
		\]
\end{theorem}
 
%   \begin{theorem}
%  \label{thm:PT_upper}
%  Let $p^\star_2$ be the solution of 
%   \[
% \tan{\theta}  = 
%  (1-p^\star)(\sqrt{2}+(1-\sqrt{2})p^\star)
%  \]

%  \end{theorem}
\begin{proof}
  First, we prove the lower bound
    \BEAS
      \frac{p^\star}{1-p^\star} &=&  \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan\angle(  \beta, - e_0)\\
      &\geq& \inf_{\beta\in H_u} V_1(\beta_{(0)}) \inf_{\beta\in H_u}\tan(\angle(\beta, -e_0))\\
      &=& p \tan{(\angle(P_u^\perp (-e_0), -e_0))}.
  \EEAS
 
Moreover, the lower bound is achieved when $\beta_{(0)}$ is one-sparse. Since $\tan{(\angle(P_u^\perp (-e_0), -e_0))}=\cot\theta$, the lower bound of $p^\star$ is $1- \tan\theta$.
 
For the upper bound, we plug in $\beta = P_u^\perp (-e_0)$, then
	\[ 
	\inf_{\| \beta\|_2=1, u^T \beta =0} 
	\tan(\angle( \beta, -e_0))V_1(\beta_{(0)}) \leq
	\tan(\angle( P_u^\perp (-e_0), -e_0))
	V_1(P_u^\perp (-e_0)).
	\]
It is worth commenting that since $V_1(P_u^\perp (-e_0))\leq \sqrt{p}$, and $\tan(\angle( P_u^\perp (-e_0), -e_0))=\cot(\angle(u, e_0))=\cot\theta$, we have
	\[ 
	 \tan(\angle( P_u^\perp (-e_0), -e_0))
 V_1(P_u^\perp (-e_0)) 
	\leq \cot(\angle(u, e_0)) \sqrt{p}.
	\]
 
  \end{proof}
  
  
  
  
  
% \paragraph{Detailed characterization of phase transition threshold}
%   We define 
%   \[
%   b:= \beta_{(0)}/\|\beta\|_2
%   \]
%   \[
%   \nu:= u_{(0)}/\|u_{(0)}\|_2=u_{(0)}/\sin{\theta}
%   \]
%   so that $\|\nu\|_2=1$.
%   Then using the fact that $u_0= \cos{\theta}$, $\|u\|_2=1$ and $\beta_0 = -\sqrt{1-\| \beta_{(0)}\|_2^2}$,
%   the condition $u^T \beta =0$ can be translated into
%   \[
%   -\cos{\theta}\sqrt{1-\| b\|_2^2} + \sin{\theta} \nu^T b =0
%   \]
%   Then
%   \[
%   \nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}
%   \]
%   Therefore, using Cauchy inequality, we recover the geometric conclusion
%     \[
%   \|b\|_2/\sqrt{1-\| b\|_2^2}  \geq \nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}
%   \]
%   \begin{lemma}
%   We define the phase transition threshold as
%   \[
%  p^\star(u):= 
%  \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))> 0\}
%  \]
% then
%  \[
%  p^\star(u):= 
%  \sup_{p\in [0,1]}\{\inf_{\| P_{u}^{\perp}\beta\|_2=1 }(-p \cdot \sqrt{1-\| P_{e_0}^{\perp}  P_{u}^{\perp}\beta\|_2^2} + (1-p) \cdot  \E_I\| ( P_{e_0}^{\perp} P_{u}^{\perp} \beta)_I\|_2 ) > 0\}
%  \]

%  Additionally, for a given $\epsilon>0$, we can define $p^\star(\epsilon),$ as 
%  \[
%  p^\star(u,\epsilon):= 
%  \sup_{p}\{\inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))> \epsilon\}
%  \]
%  Then $p^\star(u,\epsilon)<p^\star(u).$
%  \end{lemma}
 
 
%     \begin{theorem}
%  \label{thm:PT_upper}
%  Let the $\mu$ dependent upper bound $p^\star_2(u)$ be the solution of the equation
%       \[
%   \tan{\theta}  = 
%  \frac{1-p^\star}{p^\star}V_1(\nu)
%  \] 
% then for a given initial choice $v$ and true inverse filter $a^{-1}$, we define $u$ by $\title{u}= a^{-1} * v$, and reparemetrize $u = \cos{\theta} e_0 +\sin{\theta}\nu$, then the phase transition point has an upper bound given by $p^\star_2(u)$.
% If $p> p^\star_2$, then the solution of the convex program is not the correct inverse filter $a^{-1}$.

% And there is a $\mu$ independent upper bound $p^\star_3$, as the solution of the equation
%     \[
%   \tan{\theta}  = 
%  \frac{1-p^\star}{p^\star}\sqrt{p^\star}
%  \] 
%  then $p^\star_1 \leq p^\star(u)\leq p^\star_2(u)\leq p^\star_3$.
%  \end{theorem}
%  \begin{coro}
% If $u$ is two sparse, there exists $i$ such that $u_i = \pm \sin{\theta},$ then $u$ is also two sparse and we could get a two sparse $\beta = (0, \ldots,0, \beta_0, 0, \ldots,0, \beta_i, 0, \ldots,0). $ Then $ p_2^\star(u) = p^\star_1$, therefore, $p^\star(u) = p^\star_1 = 1-\tan{\theta} $. 
%  \end{coro}
  
%   \begin{proof}
%   We want to calculate 
%   \[
%  B(p)= \inf_{\|\beta\|_2=1, u^T \beta =0 }(-p \cdot \sqrt{1-\| \beta_{(0)}\|_2^2} + (1-p) \cdot  \| \beta_{(0)}\|_2 V_1(\beta_{(0)}))
%   \]
%  After the change of variable,
%   \[
%   B(p)= \inf_{\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta} }(-p \cdot \sqrt{1-\|b\|_2^2} + (1-p) \cdot  \| b\|_2 V_1(b))
%   \]
%   $\frac{b}{\|b\|_2}=\nu$, $\|b\|_2 =\cos{\theta}$ is one feasible point to the equation $\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta}$, it correspond to $\beta = P_u (-e_0)$. 
%   Therefore, plug in this specific $\beta$,
%   \[
%  \cot{\theta}(-p \cdot \sin{\theta} + (1-p) \cdot  \cos{\theta} V_1(\nu)) \geq \inf_{\nu^T b /\sqrt{1-\| b\|_2^2} = \cot{\theta} }(-p \cdot \sqrt{1-\|b\|_2^2} + (1-p) \cdot  \| b\|_2 V_1(b))
%   \]
%   we find an upper bound on phase transition point  $p^\star_2(u) \geq p^\star(u)$. 
%   Here $p^\star_2(u)$ is defined by
%   \[
%  p_2^\star(u):= 
%  \sup_{p\in [0,1]}\{\cot{\theta} }(-p \cdot \sin{\theta} + (1-p) \cdot  \cos{\theta} V_1(\nu)) > 0\}
%  \]
%  then $p^\star_2(u)$ is the solution of the equation
%   \[
%   \tan{\theta}  = 
%  \frac{1-p^\star}{p^\star}V_1(\nu)
%  \] 
%  Since $V_1(\nu)\leq \sqrt{p}$,
%  the $\mu$ independent upper bound $p^\star_3$ is the solution of the equation
%     \[
%   \tan{\theta}  = 
%  \frac{1-p^\star}{p^\star}\sqrt{p^\star}
%  \] 
%   \end{proof}
  
  

%   \begin{lemma}
%   To find the phase transition parameter $p^\star$, we need to solve the constrained optimization problem 
%   \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}\\
%  \mbox{subject to}  
% &  u^T \beta = 0,\\
% &   \|\beta\|_2^2 =1.
% \end{array}
% \EEQ
% Assuming $\| u\|_2=1$.
% Using the fact that 
% \[
% \angle(\beta, -e_0))\geq \frac{\pi}{2}-\angle(u, e_0))=\frac{\pi}{2}-\theta
% \]
% We have an additional condition
% \[
% u^Te_0 = u_0 = \cos{\theta}
% \]
%   \[
%       \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]
%   \]
% Therefore, we could add a third condition into the optimization  
%  \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}\\
%  \mbox{subject to}  
% &  u^T \beta = 0,\\
% &   \|\beta\|_2^2 =1,\\
% & e_0^T \beta = \beta_0 \geq \sin{\theta}.
% \end{array}
% \EEQ
% There are two candidate solution, one is when $\beta_0 = \sin{\theta},$ then $\|\beta_{(0)}\|_2 =  \cos{\theta}$, and 
% the problem becomes
% \BEQ
%  \begin{array}{ll}
%   \underset{\beta}{ \mbox{minimize} }  &  V_1(\beta_{(0)}) \cot{\theta}\\
%  \mbox{subject to}  
% &  u^T \beta = u_0 \beta+ u_{(0)}^T\beta_{(0)} = \cos{\theta}\sin{\theta}+u_{(0)}^T\beta_{(0)}= 0,\\
% &   \|\beta_{(0)}\|_2^2 =\cos{\theta}^2.
% \end{array}
% \EEQ
 

% If $u$ is denser than two sparse, then we can choose a $3-$sparse $\beta$, so that $\beta_0 = \sin{\theta}.$Then let 
% $r =\cos{\theta} \beta_{(0)},$  reducing the constant $\cot{\theta}$, our problem becomes 
% \BEQ
%  \begin{array}{ll}
%  \underset{r}{ \mbox{minimize} }  & V_1(r)  \\
%  \mbox{subject to}  
% &  \sin{\theta}+u_{(0)}^T r= 0,\\
% &   \|r\|_2 =1.
% \end{array}
% \EEQ
% then if there does not exist $i$ such that $u_i = \pm \sin{\theta},$ we need to have a $r$ that is at least $2-$ sparse.
%   Noticing that   
%   \[
% V_1(\frac{ e_i+e_j}{\sqrt{2}}) = p(\sqrt{2}+(1-\sqrt{2}p)).
% \]
% is the maximum value of $V_1(r)$ among all  $2-$ sparse $r$ on sphere.

% Then 
% \[
% p\leq V_1(r)\leq p(\sqrt{2}+(1-\sqrt{2}p))
% \]
% We want to choose a $2-$sparse $r$ on the sphere $\|r\|_2 =1$ that is as unbalanced as possible so that $V_1(r)$ and still satisfy $\sin{\theta}+u_{(0)}^T r= 0.$

  \end{lemma}
  
  
%   Comment:
%  \[
%  V_1(\beta_{(0)})
%  \]
%   should be between $[p,\sqrt{p}]$, from empirical observation, it is closer to $\sqrt{p}$.
  
 
 


% % So that   
% %   \[
% % p^\star \cot{\theta} \leq \frac{ p^\star}{1-p^\star}  \leq
% %  \sqrt{p^\star}\cot{\theta} 
% %   \]
  
% %   So 
% %     \[
% % 1- \tan{\theta}  \leq p^\star  \leq \sqrt{(1+\tan{\theta}^2/2)^2 -1}+(1+\tan{\theta}^2/2)
% %   \]
  
%  If we know that for $\beta \in H_u$ near the direction $P_u^\perp (-e_0)$ must not be $1-$sparse but could be $2-$sparse, then  
%   \[
%       \inf_{\beta\in H_u} [V_1(\beta_{(0)}) \tan{(\angle(\beta, -e_0))}]\leq  p(\sqrt{2}+(1-\sqrt{2}p)) \cot{\theta} 
%   \]
  
%   If this is indeed the correct condition, then
%     \[
%   1  = 
%  \frac{1-p^\star}{ p^\star}
%  p^\star(\sqrt{2}+(1-\sqrt{2}p^\star))\cot{\theta} 
%  \]

%     \[
%   \tan{\theta}  = 
%  (1-p^\star)
% (\sqrt{2}+(1-\sqrt{2}p^\star)) 
%  \]


 
  
% \subsection{Locally robust objective and semi-continuous extension}  
% Now, we study the \textbf{lower semicontinuous extension}.


% \paragraph{Locally robust objective}
%  Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
%  \[
%  \begin{array}{ll}
%   \underset{w}{ \mbox{minimize} }  & \sup_{\|\omega-w\|_2\leq \epsilon} \Expect|(\omega*Y)_0|\\
%  \mbox{subject to}  
% &  \omega_0 =1, \quad w_0 =1, \quad w, \omega \in V_{rs, rt}.
% \end{array}
%   \]
% after change of variables, and modulo constant $\sqrt{\frac{2}{\pi}}$, we have
%   \[
%  \begin{array}{ll}
%   \underset{\psi    }{ \mbox{minimize} }  & \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2\\
%  \mbox{subject to}  
% &  u^T \psi =1, \quad a^{-1}*\psi \in V_{rs, rt}.
% \end{array}
% \tag{$P_\epsilon$}
%   \]
%   Our first question is to understand the relation between this objective and the following deterministic objective as $\epsilon \rightarrow 0$.
%   \[
%  \begin{array}{ll}
%   \underset{\psi    }{ \mbox{minimize} }  & \|\psi\|_2\\
%  \mbox{subject to}  
% &  u^T \psi =1, \quad a^{-1}*\psi \in V_{rs, rt}.
% \end{array}
% \tag{$P'_0$}
%   \]

% \begin{lemma} 
% Let
% \[
% V_1(\psi):=\frac{\Expect_I\|\psi_I\|_2}{\|\psi\|_2} 
% \]
% then
%  \[
%  \begin{array}{ll}
%  &\lim_{\epsilon\rightarrow 0^+}   \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2 \\
%  = & [\lim_{\epsilon\rightarrow 0^+}\sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h)] \|\psi\|_2
% \end{array}
%   \]
%   However, 
%   \[
%  \begin{array}{ll}
% p \leq  [\lim_{\epsilon\rightarrow 0^+}\sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h)] \leq \sqrt{p}
% \end{array}
%   \]
%   it does dependent on $\psi.$
%  \end{lemma} 
% \begin{proof}
%  \[
%  \begin{array}{ll}
%  &  \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \Expect_I\|\psi_I+\epsilon \cdot h_I\|_2 \\
%  =&   \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} \frac{\Expect_I\|\psi_I+\epsilon \cdot h_I\|_2}{\|\psi+\epsilon \cdot h\|_2} \|\psi+\epsilon \cdot h\|_2\\
%  = & \sup_{\|h\|_2\leq 1, u^T h =0, a^{-1}*h \in V_{rs, rt}} V_1(\psi+\epsilon \cdot h) \|\psi+\epsilon \cdot h\|_2
% \end{array}
%   \]
%   where 
%     \[
%  \begin{array}{ll}
%  &  \lim_{\epsilon\rightarrow 0^+}  \|\psi+\epsilon \cdot h\|_2 = \|\psi\|_2
% \end{array}
%   \]
%   But $p \leq  V_1(\psi+\epsilon \cdot h) \leq \sqrt{p} $ and it does dependent on $\psi$ globally.
% \end{proof}





























% Question:
% how to calculate the expectation
% \[
%  \begin{array}{ll}
% P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}
% \end{array}
% \]
% To show that 
% \[
%  \begin{array}{ll}
% 0\in P_{u}^{\perp} \Expect_I [N((e_0)_I) ]
% \end{array}
% \]
% we need to prove
% \[
%  \begin{array}{ll}
% \frac{p \sin{\theta} }{(1-p) \cos{\theta}}e_{0,u} \in \frac{1}{\cos{\theta}} P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}
% \end{array}
% \]
% This quantity should be something like
% \[
%  \begin{array}{ll}
%  \frac{1}{\cos{\theta}} P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}} = (1-(1-p)^n)\cdot D_1
% \end{array}
% \]
% where $D_1$ should be a unit disk that contains $-e_{0,u}$, but I am not sure how to prove it since I don't know how to calculate $\Expect_{I_{(0)}}D_{I_{(0)}}$ and $P_{u}^{\perp} \Expect_{I_{(0)}}D_{I_{(0)}}$.

% \paragraph{Directional derivative}

% We can go back to the previous \textbf{directional finite difference} analysis by
% \begin{lemma}
%  The directional derivative
% \[
%  \begin{array}{ll}
% \lim_{t\rightarrow 0^+}\frac{1}{t}(\Expect_I [\|(e_0+t\beta)_I\|_2 - \|(e_0)_I\|_2])
% &= \sup_{u\in \Expect_I [N((e_0)_I)]} <\beta, u\rangle\\
% \end{array}
%   \]
%  First, 
% \[
%  \begin{array}{ll}
% \sup_{u\in \Expect_I [N((e_0)_I)]} <\beta, u\rangle
% &= p <\beta,e_0\rangle + (1-p) \sup_{u\in \Expect_{I_{(0)}}D_{I_{(0)}} } <\beta, u\rangle
% \end{array}
%   \]
%  Second, 
% \[
%  \begin{array}{ll}
% \sup_{u\in P_{u}^{\perp} \Expect_I [N((e_0)_I)]} <\beta, u\rangle
% &= p   \sin{\theta} <\beta,e_{0,u}\rangle + (1-p)\cos{\theta} \sup_{u\in \Expect_{I_{(0)}}D_{I_{(0)}} } <\beta, u\rangle
% \end{array}
%   \]
% \end{lemma}





\section{Finite difference of objective}
We study the upper and lower bound of: 
\[
B(e_0, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
\]

This upper and lower bound allows us to connect objective $\E_I  \| \psi_I \|_2$ and the $2-$norm of $ \psi - e_0$:
\[
\E_I  \| \psi_I \|_2 - \E_I  \| (e_0)_I \|_2 = \E_I  \| \psi_I \|_2 - p=B(e_0, \psi - e_0) \| \psi - e_0\|_2
\]

% \subsection{Bi-Lipschitzness of finite difference of objective for sphere constraint}
% \begin{lemma}
% For the sphere constraint $\|e_0 + \phi\|_2 =1$ for any $\phi$, 
%   \[
%  \begin{array}{ll}
% \frac{1}{16}p(1-p) \|\phi\|_2 \leq  
% % \Expect_I\|(e_0+\phi)_I\|_2 -  \Expect_I\|(e_0)_I\|_2 = 
% V_1(e_0+\phi) - V_1(e_0) \leq 2\sqrt{N} \|\phi\|_2
% \end{array}
%   \]
% \end{lemma}
% This lemma is based on Proposition $C.7$(upper bound) and $C.8$(lower bound) of section $C.6$ of the paper \cite{bai2018subgradient}, proof can be found in there.








% \paragraph{A new metric to solve gradient non-Lipschitzness}

% First, $\psi \mapsto \| \psi \|_2$ is Lipschitz for $\ell_2$ convergence. And 
% $\psi \mapsto \E_I\| \psi_I \|_2$ is Lipschitz for $\ell_2$ convergence.
% Then $\beta \mapsto \Expect_I [\|(\psi+ \beta)_I\|_2 - \|(\psi)_I\|_2]$
% is Lipschitz for $\ell_2$ strong convergence.

% However, notice that 
%  $\beta \mapsto \lim_{t\rightarrow 0^+} 
% \frac{1}{t}\Expect_I [\|(\psi+ \beta)_I\|_2 - \|(\psi)_I\|_2]$
% and 
%  $
%  \E{\partial_\psi\| (\psi)_I\|_2 }  =  \E_I [N(\psi_I)]
% $
% are not Lipschitz in $\psi$ with respect to the Euclidean metric $d_2(a,b) :=\|a-b\|_2$ nor the angle metric $d_A(a,b) := \frac{1}{\pi}\angle(a, b)$. 

% They are Lipschitz with respect to a stronger metric on the sphere which is sign-pattern aware and averages all “subset angles” (see \cite{bai2018subgradient} section $4.2$ for detailed discussion and lemma $F.4$ for the proof of  Lipschitz property):
% \[
% d_E(a, b) := \frac{1}{\pi} \E_I\angle(a_I, b_I)
% \]


 
%   The directional gradient of the locally robust objective for a give direction $\beta$ so that $\|\beta\|_2 =1, u^T \beta =0, a^{-1}*\beta \in V_{rs, rt}.$ we study
%   \[
%  \begin{array}{ll}
% \lim_{\epsilon\rightarrow 0^+} \sup_{\|h\|_2\leq 1} \Expect_I\|\psi_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 
% \end{array}
%   \]
  
% \begin{lemma}
%  The locally robust directional derivative at $e_0$ along $\beta$ 
%  evaluates to the following:
%   \[
%  \begin{array}{ll}

%  & \lim_{\epsilon\rightarrow 0^+} \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2) \\
% =&\|\beta\|_2 \{p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} \lim_{\epsilon\rightarrow 0^+} [\sup_{\|h\|_2\leq 1} V_1((\beta+\epsilon \cdot h)_{(0)})] \} .
% \end{array}
%   \]
% \end{lemma}
%  \begin{proof}
% Applying Lemma \ref{eq:ComputeExpect}, we proceed as follows:
% \[
%  \begin{array}{ll}
%  & \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2)\\
% =& \sup_{\|h\|_2\leq 1} \sup_{g\in \Expect_I [N((e_0)_I)]} \langle\beta +\epsilon \cdot h, g\rangle\\
% % &= \sup_{g\in  [N((e_0)_I)]} \Expect_I\langle\beta, g\rangle\\
% =& \sup_{\|h\|_2\leq 1}[p \cdot \langle\beta +\epsilon \cdot h, e_0\rangle + (1-p) \cdot  \sup_{g\in {\cal B}_0 } \langle\beta +\epsilon \cdot h, g\rangle]\\
% =& \sup_{\|h\|_2\leq 1}[p \cdot \langle\beta +\epsilon \cdot h, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|(\beta +\epsilon \cdot h)_{I}\|_2 | 0 \not \in I ] ]\\
% =& \sup_{\|h\|_2\leq 1}[[p \cdot \cos{\angle(\beta +\epsilon \cdot h, e_0)} + (1-p) \cdot  \sin{\angle(\beta +\epsilon \cdot h, e_0)} V_1((\beta +\epsilon \cdot h)_{(0)})] \|\beta +\epsilon \cdot h\|_2]
% \end{array}
%   \]
%   Taking limit for $\epsilon\rightarrow 0^+$,using the fact that $\| \cdot \|_2, \sin(\cdot), \cos(\cdot) $ are all Lipschitz function, 
%  \[
%  \begin{array}{ll}
%  &\lim_{\epsilon\rightarrow 0^+} \lim_{t\rightarrow 0^+} \frac{1}{t}(\sup_{\|h\|_2\leq 1} \Expect_I\|(e_0)_I+t\cdot \beta_I+\epsilon \cdot h_I\|_2 -  \Expect_I\|(e_0)_I\|_2)\\
% =& \lim_{\epsilon\rightarrow 0^+} \{\|\beta +\epsilon \cdot h\|_2 [p \cdot  \cos{\angle(\beta +\epsilon \cdot h, e_0)} + (1-p) \cdot  \sin{\angle(\beta +\epsilon \cdot h, e_0)} V_1((\beta +\epsilon \cdot h)_{(0)})]\} \\
% =&\|\beta\|_2 \{p \cos{\angle(\beta, e_0)} + (1-p)   \sin{\angle(\beta, e_0)} \lim_{\epsilon\rightarrow 0^+} [\sup_{\|h\|_2\leq 1} V_1((\beta+\epsilon \cdot h)_{(0)})] \}
% \end{array}
%   \] 
%   \end{proof}

\paragraph{Bi-Lipschitzness of finite difference of objective near $e_0$ for linear constraint}
We normalize the problem by defining $t:=\|\phi\|_2, \beta:=\frac{\phi}{\|\phi\|_2}$.
After normalization, and taking into account the linear constraint $u^T \phi = 0$, we will study, for $\beta\in \mathcal{B}_t :=\{\|\beta\|_2=1, u^T \beta = 0,  \|e_0+t\beta\|_\infty\leq 1 \}$ for finite $t$, the upper and lower bound of 
\[
\frac{\E_I  \| (e_0+t\beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}.
\]

First, if $t\rightarrow 0^+$, then we get the directional derivative along direction of $\beta$. 
\BEAS
\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}.
\EEAS

Due to convexity of the function $\beta \rightarrow \E_I  \| (e_0+t \beta)_I \|_2$, we have the finite difference lower bounded by directional derivative:
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
\geq 
 \lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} .
\EEAS



% where  $\|\beta_{(0)}\|_2 = \sqrt{1-\beta_0^2} $ since  $\|\beta\|_2 = 1$, and
% \[
% V_1(\beta_{{(0)}})= \frac{\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]}{\|\beta_{(0)}\|_2}.
% \]
% We know that for 
% \BEAS
% p \leq V_1(\beta_{{(0)}})
% \leq \sqrt{p}
% \EEAS
% Where  
% \[
% \beta^a = ( \beta_0,\sqrt{1-\beta_0^2}, 0,\ldots,0 )
% \]
% achieves lower bound,
% and 
% \[
% \beta^b = (\beta_0,\frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2},\ldots, \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} ) = \beta_0 e_0 + \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} (\sum_{i\neq 0} e_i)
% \]
% achieves upper bound.


\begin{theorem}
\label{thm:bound_diff}
We have upper and lower bound
\BEAS
0 \leq \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} -\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
\leq 
  \frac{t}{2}p\Big( 
   \beta_0^2 
 +
 p  (1-\beta_0^2) \Big) \leq \frac{pt}{2}.
\EEAS
This leads to
\[
0\leq B(e_0, \phi) -	 \nabla_{\phi}{\E_I  \| (e_0+\phi)_I \|_2}\mid_{\phi=0}\leq \frac{p}{2}\|\phi \|_2.
\]
% and lower bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% \geq 
% (1-p)\Big( V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2}\Big) + 
% p\Big(\frac{1}{t} (\left| 1 + t \beta_0 \right|-1 \Big)
% \EEAS
% Specially, when $t\leq 1$, $\frac{1}{t} (\left| 1 + t \beta_0 \right|-1) = \beta_0$, we have the finite difference with $t\leq 1$ lower bounded by directional derivative:
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% \geq 
%  \lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% \EEAS
\end{theorem}


\begin{proof}
As mentioned before, the lower bound is derived from convexity.

In the proof, for finite $t$, we calculate the finite difference condition on $I_0$:
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
&=&
(1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big).
\EEAS
And
\BEAS
\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
&=&
(1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\beta_0.
\EEAS
In the following, we prove an upper bound 
\BEAS
 \frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t}- \beta_0
\leq   \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2.
\EEAS

For finite $t$,
\BEAS
\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t}
&=&
\Expect_{I}[ \left( (\frac{1}{t}+ \beta_0)^2+\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
&=& \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ].
\EEAS



% and a higher order upper bound that is tighter for $x\leq 2,$
% \[
% \sqrt{1+x}-1 - \frac{x}{2}\leq -\frac{1}{8}x^2+1/16x^3
% \]
% for any $x\geq 0$, we also have lower bound:
% \[
%   -\frac{1}{8}x^2 \leq \sqrt{1+x}-1-\frac{x}{2}
% \]
Additionally, using concavity of the function $\sqrt{1+x}$, we have
\BEAS
 && \frac{1}{t}\Expect_{I}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1| 0 \in I ]\\
&\leq&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2\Expect_{I}\| \beta_{I_{(0)}} \|_2^2| 0 \in I ] \right)^{1/2} -1]\\
&=&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p \| \beta_{{(0)}} \|_2^2 \right)^{1/2} -1]\\
&=&  \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p (1-\beta_0^2) \right)^{1/2} -1].
\EEAS
Now, apply the inequality: 
for any $x\geq -1$:
\[
\sqrt{1+x} -1 \leq \frac{x}{2},
\]
we have
\BEAS
 \frac{1}{t}[ \left( 1+ 2t\beta_0 + t^2 \beta_0^2+t^2 p \| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -1]
&\leq&  \beta_0 + \frac{t}{2} (p \| \beta_{{(0)}} \|_2^2  +  \beta_0^2).
\EEAS
Therefore, 
\BEAS
\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} -\lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
\leq 
  \frac{t}{2}p\Big( 
   \beta_0^2 
 +
 p  (1-\beta_0^2) \Big) \leq \frac{pt}{2}.
\EEAS
The last inequality is due to $\beta_0^2 \leq 1$.
% On the other hand,
% \BEAS
% \frac{1}{t} \Expect_{I}[ \left( (1+ t\beta_0)^2+t^2\| \beta_{I_{(0)}} \|_2^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]
% &\geq&  \frac{1}{t} (\left| 1 + t \beta_0 \right|-1 )
% \EEAS
% when $\beta_0 \geq -\frac{1}{t}$,
% \BEAS
% \frac{1}{t} (\left| 1 + t \beta_0 \right|-1 )
% = \beta_0 
% \EEAS
% also, for $t<1$, we also have the expansion
% \BEAS
% && \Expect_{I}[ \left( \| \beta_{I_{(0)}} \|_2^2+(\frac{1}{t}+ \beta_0)^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
% &=& \beta_0 + \frac{t}{2} \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] + \frac{t}{2} \beta_0^2 - 
% \frac{1}{8t} (2t\beta_0 +t^2 (\beta_0^2 + \| \beta_{I_{(0)}} \|_2^2) )^2 + \frac{1}{16t} (2t\beta_0 +t^2 (\beta_0^2 + \| \beta_{I_{(0)}} \|_2^2) )^3 + \ldots \\
% &=& \beta_0 + \frac{t}{2} \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] + \frac{t}{2} \beta_0^2 - \frac{t}{2} \beta_0^2 
% -  \frac{t^2}{2} \beta_0 \Expect_{I}[ \| \beta_{I_{(0)}} \|_2^2 | 0 \in I ] 
% - \frac{t^2}{2} \beta_0^3  +  \frac{t^2}{2} \beta_0^3 
% + O(t^3)\\
% &=& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \EEAS
% When $\beta_0 <0$, then
% \BEAS
% && \Expect_{I}[ \left( \| \beta_{I_{(0)}} \|_2^2+(\frac{1}{t}+ \beta_0)^2 \right)^{1/2} -\frac{1}{t}| 0 \in I ]\\
% &=& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)\\
% &\geq& \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2
% \EEAS

\end{proof}




% Qingyun's Remark: this bound is numerically verified for $t\leq 5$ with Matlab. 
% Where we use the fact that $p\leq V_1(\beta_{{(0)}}) \leq \sqrt{p},$ for both $\beta_0 = 1, -0.5, -1/\sqrt{N}, 0,1/\sqrt{N}, 0.5, 1 $, we tested the two extreme points  
% \[
% \beta^a = ( \beta_0,\sqrt{1-\beta_0^2}, 0,\ldots,0 )
% \]
% and 
% \[
% \beta^b = (\beta_0,\frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2},\ldots, \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} ) = \beta_0 e_0 + \frac{1}{\sqrt{N-1}}\sqrt{1-\beta_0^2} (\sum_{i\neq 0} e_i)
% \]

% \begin{coro}
% \label{coro:bound_diff}
% We have upper bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% &\leq& 
% (1-p)\Big( \sqrt{p} \sqrt{1-\beta_0^2}\Big) + 
% p\Big(\beta_0  +
%   \frac{t}{2} \beta_0^2 
%  +
%  p\frac{t}{2}  (1-\beta_0^2) \Big) \\
%  &\leq& 
%  (1-p)\sqrt{p}  + 
% p\Big(1  +
%   \frac{t}{2} 
%  +
%  p\frac{t}{2}   \Big)
% \EEAS



% \end{coro}


% \begin{coro}
% \label{coro:bound_diff}
% when $t\leq 1$, we have the finite difference with $t\leq 1$ lower bounded by directional derivative:
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% &\geq&
% \lim_{t\rightarrow 0^+}\frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t} 
% \EEAS


% \end{coro}






% \paragraph{Minor result}


% \begin{coro}
% We have upper bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big)\\
% &\leq& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2\big)\\
% &\leq& (1-p)  \sqrt{p} \| \beta_{{(0)}} \|_2 + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  + \frac{t}{2} \beta_0^2\big)\\
% \EEAS
% \end{coro}


% \begin{lemma}
% We have asymptotic relation for $t<1$, 
% \BEAS
% && \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}\\
% &=& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + 
% p\big(
% \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 
% -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \big)\\
% &=& (1-p) V_1(\beta_{{(0)}}) \| \beta_{{(0)}} \|_2 + 
% p\big(
% \beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 
% -  \frac{t^2}{2} \beta_0 p \| \beta_{{(0)}} \|_2^2 + O(t^3)
% \big)\\
% &=& (1-p) V_1(\beta_{{(0)}}) \sqrt{1-\beta_0^2} + 
% p\beta_0 + p^2\big(
%  \frac{t}{2}  (1-\beta_0^2) 
% -  \frac{t^2}{2} \beta_0 (1-\beta_0^2) \big) + O(t^3)
% % \\
% % &=& (1-p) V_1(\beta_{{(0)}}) \cos (\angle(e_0,\beta)) + 
% % p\sin (\angle(e_0,\beta)) + p^2 \big(\frac{t}{2}  \cos (\angle(e_0,\beta))^2 
% % -  \frac{t^2}{2} \sin (\angle(e_0,\beta))  \cos (\angle(e_0,\beta))^2 + O(t^3)
% % \big)
% \EEAS
% \end{lemma}


% \begin{coro}
% If $t<1$, and $\beta_0<0$, we have lower bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t} \big)\\
% &\geq& (1-p)  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ] + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2  \big)\\
% &\geq& (1-p)  p \| \beta_{{(0)}} \|_2 + p\big(\beta_0 + \frac{t}{2} p \| \beta_{{(0)}} \|_2^2 \big)\\
% \EEAS
% \end{coro}


% \begin{coro}
% If $\beta_0<0$ and  $t\geq \frac{1}{|\beta_0|}$ so that it allows $(1+t \beta_0)^2 =0$ is achievable, we have lower bound 
% \BEAS
% \frac{\E_I  \| (e_0+t \beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t}
% &=&
% (1-p)  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 +p\frac{1}{t}[ \E_{I_{(0)}} \left(  \| t \beta_{I_{(0)}} \|_2^2+(1+t \beta_0)^2 \right)^{1/2} -1]\\
% &\geq& (1-p)  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 +p  \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 - \frac{p}{t}\\
% &=& \E_{I_{(0)}}  \| \beta_{I_{(0)}} \|_2 - \frac{p}{t}\\
% &\geq& p\| \beta_{{(0)}} \|_2 - \frac{p}{t}
% % \\
% % &\geq& p(\| \beta_{{(0)}} \|_2 - \max\{|\beta_0|,\frac{1}{t}\} )
% \EEAS
% \end{coro}

% % \begin{proof}


% % \end{proof}







% In the following, we use mean value theorem to calculate this quantity in a different way.
% \paragraph{Mean value theorem}
% \begin{lemma}[Lebourg’s mean value theorem, Theorem $2.3.7$ of \cite{clarke1990optimization}]
% Let $x,y$ be distinct points in $\reals^d$, and suppose that $f: \reals^d \rightarrow \reals$ is locally Lipschitz on an open set $U$ containing the line segment $[x, y]$. Then there exists a $\eta \in (0,1)$ such that
% \[
% f(y) - f(x) \in \langle \partial f (x+ \eta(y-x)) , y - x\rangle . 
% \]
% Let $t :=\|y-x\|_2 $, and let $\beta:= \frac{y-x}{t}$ be a unit vector along the direction of $y-x$ so that $y-x = t\beta$. We could reformulate the theorem as that there exists a constant $\eta \in (0,1)$ such that
% \[
% f(x+t\beta) - f(x) \in 
% \langle \partial f (x+ t \eta \beta) , t\beta\rangle . 
% \]
% \end{lemma}
% Using Lebourg’s mean value theorem for $\E_I [\| (\psi)_I \|_2| 0 \in I ]$ near $e_0$ to use its locally Lipschitz property, 
% the result is that there exists a constant $\eta \in (0,1)$ such that
% \[
% \frac{\E_I [ \| e_0+t\beta_I \|_2 -   1 | 0 \in I ]}{t}
%  \in 
%  {\Expect}_I \langle  [N(e_0+ t \eta \beta_I)] , \beta\rangle  | 0 \in I ]
% \]


























% (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}$
% and for $\beta\in \{\|\beta\|_2=1,  \|e_0+\beta\|_2 = 1, (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}.$






% and use the fact that $(1+\beta_0)^2 > \beta_i^2, \forall i\neq 0$, we have $(1+\beta_0)^2> \frac{1}{N-1}\| \beta_{(0)} \|_2^2$,
% \BEAS
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+(1+\beta_0)^2 \right)^{1/2} -1]
% &\geq& 
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+\frac{1}{N-1}\| \beta_{(0)} \|_2^2 \right)^{1/2} -1]
% \\
% &\geq& 
% [ \E_{I_{(0)}} \left( \frac{ \| \beta_{I_{(0)}} \|_2^2}{\| \beta_{(0)} \|_2^2}+\frac{1}{N-1} \right)^{1/2} \| \beta_{(0)} \|_2-1]
% \\
% &\geq& 
% [ \E_{I_{(0)}} \left( \frac{ \| \beta_{I_{(0)}} \|_2^2}{\| \beta_{(0)} \|_2^2}+\frac{1}{N-1} \right)^{1/2} \| \beta_{(0)} \|_2-1]
% \EEAS


% For $\beta\in \{\|\beta\|_2=1,  \|e_0+\beta\|_2 = 1, (1+\beta_0)^2 > \beta_i^2, \forall i\neq 0  \}$, we have
% $(1+\beta_0)^2 = 1-\| \beta_{(0)} \|_2^2,$ let $\bar{I}_{(0)}$ be the complement $\cT-\{0\}- I.$
% \BEAS
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+(1+\beta_0)^2 \right)^{1/2} -1]
% &=& 
% [ \E_{I_{(0)}} \left(  \| \beta_{I_{(0)}} \|_2^2+1-\| \beta_{(0)} \|_2^2 \right)^{1/2} -1]
% \\
% &=& 
% [ \E_{\bar{I}_{(0)}} \left( 1-\| \beta_{\bar{I}_{(0)}} \|_2^2 \right)^{1/2} -1]
% \\
% &=& 
% -\sum_{\ell =0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}2^{-2(\ell+1)}\E_{\bar{I}_{(0)}}\| \beta_{\bar{I}_{(0)}} \|_2^{2(\ell+1)}
% \EEAS


% \paragraph{Upper bound}


% \begin{lemma}  
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%  &\leq p(\beta_0 +t) + (1-p)\sqrt{p} \|\beta_{(0)}\|_2 \\
% &= pt + p\sin (\angle(e_0,\beta)) + (1-p)\sqrt{p} \cos (\angle(e_0,\beta))
% \end{array}
%   \] 
% \end{lemma}


% \begin{proof}
% \[
%  \begin{array}{ll}
% {\Expect}_I [N((e_0+ t \eta \beta)_I)]
% &= 
% p {\Expect}_{I_{(0)}} [N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big)] 
%  + (1-p) {\Expect}_{I_{(0)}} [N\big( t \eta \beta_{I_{(0)}}\big)] \\
%  &= 
% p {\Expect}_{I_{(0)}} [N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big)] 
%  + (1-p) {\Expect}_{I_{(0)}}[ N\big(\beta_{I_{(0)}}\big)]
% \end{array}
%   \]
% then
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%  &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) {\Expect}_{I_{(0)}} [\langle N\big(\beta_{I_{(0)}}\big), \beta\rangle]\\
%   &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
% \end{array}
%   \]
%  where
%  \[
%  \begin{array}{ll}
%  {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  &=  {\Expect}_{I_{(0)}}[  \frac{\beta_0 +t \eta (1 - \|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2}   ]\\
%  &= (\beta_0 +t \eta) {\Expect}_{I_{(0)}} \| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2^{-1} - {\Expect}_{I_{(0)}}\frac{t \eta (\|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2} \\
%  &\leq \beta_0 +t\eta\\
%  &\leq \sin (\angle(e_0,\beta))+t
% \end{array}
%   \]
%  The first inequality comes with the fact that ${\Expect}_{I_{(0)}} \| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2^{-1}\leq 1$, and 
%  ${\Expect}_{I_{(0)}}\frac{t \eta (\|\beta_{\cT -I_{(0)} } \|_2^2) }{\| e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\|_2} \geq 0$.
 
%  The second inequality comes with the fact that $\eta <1$.
%  and
%   \[
%  \frac{\beta_0}{\|\beta\|_2} = \sin (\angle(e_0,\beta)) .
%  \]

%  Therefore,
% \[
%  \begin{array}{ll}
% \langle {\Expect}_I [N((e_0+ t \eta \beta)_I)], \beta\rangle
%   &= 
% p {\Expect}_{I_{(0)}} [\langle N\big(e_0+t \eta \beta_0+ t \eta \beta_{I_{(0)}}\big), \beta\rangle] 
%  + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t ) + (1-p) 
%  \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t) + (1-p)\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\\
%  &\leq p(\sin (\angle(e_0,\beta)) +t) + (1-p)\sqrt{p} \|\beta_{(0)}\|_2 
% \end{array}
%   \] 
%  \end{proof}
 
%  \begin{coro}
%  \[
%  \frac{\E_I  \| (e_0+t\beta)_I \|_2 - \E_I  \| (e_0)_I \|_2}{t\|\beta\|_2} \leq  
%  pt + p\sin (\angle(e_0,\beta)) + (1-p)\sqrt{p} \cos (\angle(e_0,\beta))
%  \]
%  \end{coro}

==> old_sec/sec_old_2020/backup.tex <==
\begin{proof}
In the following proof, for clarity, we write $\gamma$ simply as $\gamma$.

Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\beq
\label{FoldedGaussianMean_Obj}
\Expect|\psi^T X+\mu| =   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)\right]
\eeq



This is hard to compute, but to give upper and lower bounds, we can leverage a few simple facts:
first, 
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &\geq  1- \frac{ \gamma^2}{2}
\end{array}
  \] 
Second, the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 

% (see: https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function)


Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ O( \gamma^4) ]/[1 + \frac{ \gamma^2}{2}+ O( \gamma^4)] \\
&= 1 -\frac{ \gamma^2}{6}+ O( \gamma^4)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!} \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-1}{12} \gamma^4  +   \frac{\gamma^{4}}{(-2)^2 (2)!} + O(\gamma^6)\\
&=    \frac{1}{24} \gamma^4   + O(\gamma^6)\\
\\
&\geq 0
\end{array}
\] 
We observe that it is only a function of $\mu^2$ and $\psi$, and when $\gamma^{2}\rightarrow 0$, the residual $\mbox{Res}\rightarrow 0$:
\[
 \begin{array}{ll}
\lim_{|\gamma|\rightarrow 0}\mbox{Res} &:= 0
\end{array}
\] 

Then we give an lower bound:
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&= \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]+   \mbox{Res}\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}








%   For $\sigma_2 =0$. If there is $C(\phi^*) \in [C_-, C_+]$ so that
%     \[
%     \begin{array}{ll}
%   \Expect_I \cos[\angle( (I\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]
%   &= C(\phi^*) \cos[\angle( (1\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]\\
%  &= C(\phi^*) \cos[\angle( (e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
%   then 
  
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= C(\phi^*) \langle  \partial  F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\

% \end{array}
%   \]






% Let $f$ be a extended real-valued convex function $f:\reals^d \rightarrow [-\infty, \infty]$, $\imath_{K}$ be the indicator function over $K$, that is, the function that returns $0$ if the argument belongs to $K$ and $+\infty$ otherwise.
% We define convex conjugate of $f$ as $f^*:\reals^d \rightarrow [-\infty, \infty]$, where
% \[
% f^{{*}}(u) := \sup_{x \in \reals^d} \left \{ \langle u , x \rangle - f \left( x \right) \right\}\,,\qquad u \in \reals^d\,.
% \]
% From Fenchel's duality theorem, we have the following lemma
% \begin{lemma}[duality lemma]

% \begin{align}
% \min_{x \in K} f(x) &= \min_{x \in \reals^d} f(x) + \imath_{K}(x)\\
%  &= \min_{x \in \reals^d} \max_{u \in \reals^d}\Big\{\langle x, u\rangle - f^*(u)\Big\} + \imath_{K}(x)\\
% &= \max_{u \in \reals^d}\min_{x \in \reals^d}\Big\{ \imath_{K}(x) + \langle x,u\rangle\Big\} - f^*(u)\\
% &= \max_{u \in \reals^d} (-\imath_{K}^*(-u) - f^*(u)),
% \label{eq:pd_relationship}
% \end{align}
% \end{lemma}  







% \paragraph{Primitive calculation}  
% Notice that
% \[
%  \begin{array}{ll}
%   \sup_{\|Z\|_2\leq 1} \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ] ] 
% = \|\psi\|_2
% \end{array}
%   \]
% We could focus on 
% \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Then we study the difference,
% \[
%  \begin{array}{ll}
% \Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|
% &= \Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )| \\
% % &= \Expect [\mbox{sign}\left((e_0 +\phi)^T (I\cdot G+\eta Z )\right) (e_0 +\phi)^T (I\cdot G ) \\
% % - \mbox{sign}\left( (e_0)^T (I\cdot G+\eta Z )\right) (e_0)^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Let $\eta$ be very small and we study the asymptotic behavior.
% We want to study
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% =& \sup_{\|Z\|_2\leq 1}[\Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )|] \\
% =& \sup_{\|Z\|_2\leq 1}[\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]-\Expect [\mbox{sign}((I\cdot G+\eta Z )_0)  (I\cdot G )_0] 
% \\
%  &+ \eta (\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ])] 
% \end{array}
%   \]
%  We use some crude approximation to gain insight:
  
%  If $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(e_0^T (I\cdot G+\eta Z ))$, then
%  \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}(\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ]) \\
% =& \sup_{\|Z\|_2\leq 1}\Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  \phi^T Z ]\\
% =& \|\phi\|_2
% \end{array}
%   \]
% On the other hand, if  $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(\psi^T (I\cdot G )) $ for all $\psi$, then
% we could use the formula
%   \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G)) \psi^T (I\cdot G) ]
% = \sqrt{\frac{2}{\pi}} \cdot  \Expect_I \| \psi_I\|_2
% \end{array}
%   \]
% So we could have an crude approximate as 
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% \approx & \sqrt{\frac{2}{\pi}} \cdot  \Expect_I [\| (e_0+\phi)_I\|_2-\| (e_0)_I\|_2]
%  + \eta \|\phi\|_2
% \end{array}
%   \]
  

==> old_sec/sec_old_2020/concentration.tex <==
\section{Old concentration results}
% \subsection{Guarantee of inverse kernel recovery}
% \subsubsection{Random model } 
% We first study the following finite sample setting.
% \begin{itemize} 

%   \item We sample a length-$n$ observation $y\in \reals^n$,  
%   from the circular convolution model 
%   \[ 
%   y =  a*x.
%   \]
 
%  \item  Here $x\in \reals^n$ is a random vector where each entry $x_{i} = \Omega_{i} G_{i}$, where  $\Omega$  i.i.d. sampled from Bernoulli distribution $\mbox{Ber}(p)$ and $G$  i.i.d. sampled from Gaussian random variable with variance $1$, $\Omega$ and $G$ are independent.   We define $|S| = \sum_i \Omega_{i}$. 
 
%  We assume $1/4 \geq p\geq 2/n$.

%   \item The kernel $a$ has an inverse filter $w^0$ of length $k+1$, such that 
%   \[
%   a*w^0 =e_1,
%   \]
%   where $*$  is circular convolution of  length $n$.
  
%  To fix the scale and shift of $w^0$, without loss of generality, we assume $w^0_{j} =1$ for some $j$, and it is the entry with largest absolute value. 
 
%   Let $C(a),C(w^0)$ to be the circulant matrix of size $n$ by $n$ generated by $a, w^0$ after zero-padding. Then $C(w^0)= C(a)^{-1}.$  
  
%   We define the condition number of $C(a)$ to be $\delta_a$, which is the ratio of the largest absolute eigenvalue over the smallest absolute eigenvalue.
  
  
% \subsubsection{Perturbation }  
% Consider perturbed filter $w = w^0 + \epsilon v$, and 
% we define 
% \[
% h=  a*v  = a*(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|x+\epsilon h*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*v, v_0 = 1\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 


% %   \item  We define the autocorrelation of $a$ as 
% % \[
% % R(a) = a * \bar{a},
% %  \]
% %  where $\bar{a}$ is the flipped version of $a$.
% % And the $d$-th element of $R(a)$ is the  
% % $d$-lag correlation of $a$ as 
% % \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d},
% %  \]
% %  where we assume periodic boundary condition, $a_{n+d} = a_d$.
% % %  \js{What about the boundary? My understanding is R(a) is a length $n$ vector defined as $R(a) = a \cconv a(-)$ (here $a(-)$ is $a$ flipped), i.e., $R(a)$ is the autocorrelation sequence defined based on circulant convolution. Now $R_d(a)$ is the $d$-th element in this sequence. An alternative way is $R(a) = aC(a)$. }
 
% % Clearly $R_0(a) =  \|a\|_2^2$.
% %  We assume that there is a constant $C$ such that for all $d\neq 0$, 
% %  \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d} \leq C/n^{\beta_{d}}\|a\|_2^2
% %  \]
% % where $\beta_d\geq 1/2$. 


% \end{itemize}
% \begin{theorem} 
% Under the above assumption,
% there exists constant $C_0$, $C$, for all $n>C k^2 \log^2(kp)$, 
% the minimizer $w^*$ of the optimization problem 
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|w*y\|_1\\
% \mbox{subject to}  
% & w_{k+1}=1,\\
% & w \in \reals^{k+1},
% \end{array}
%   \]
% equals $w^0$  with probability $1-\delta$, where 
% \[
%  \begin{array}{ll}
% \delta 
% \leq \exp\left( -C_0 \delta_a^2 k\log(kp)\right)
% \end{array}
% \]
% % \js{I understand this is probably not the final form yet ... What is the $\epsilon$ here? Why setting $n$ to be on the complexity order stated above can make this $\delta$ ``small'' (I suppose this depends on what we set $\epsilon$)?}
% convergences to zero asymptotically as $k$ grows to infinity.

% % \js{(1) $p$ is an important parameter for the problem, should be brought in the problem statement. (2) About $\delta$: mathematical signal processing and relevant communities often asks for the more concrete rate. When people in these fields say something holds with high probability, there's a precise meaning: decay of $\delta$ cannot be slower than $O(n^{-1})$. As a counter-example, $O(\log^{-1}n)$ is too slow to be considered as the event holding with high probability. }
% \end{theorem}
% \begin{proof} 
% To prove the theorem, we do a change of variable 
% \[
% h=  a*w- e_1 = C(a) w- e_1 = C(a)(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|(h+e_1)*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*w- e_1 =  C(w^0)^{-1}(w-w^0)\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 

% Without loss of generality, we assume $\|v\|_2=1$.
  

% We define the difference 
% \[
%  \begin{array}{ll}
% D &= \|(h+e_1)*x\|_1 - \|x\|_1.
% \end{array}
%   \]
% To prove the theorem, we need to prove that the difference $D$ is non-negative.

% Since the problem is convex, we only need to prove that the difference is non-negative  for small perturbation.







% % We define $S$ to be the support of $x$.
% % \[
% %  \begin{array}{ll}
% % D &=  \|h*x+x\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|(h*x)_{S^c}\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|h*x-(h*x)_{S}\|_1 - \|x\|_1\\
% % &\geq  \|h*x\|_1- 2\|(h*x)_{S}\|_1
% % \end{array}
% %   \]
% % Furthermore, 
 




% %  \[
% %  \begin{array}{ll}
% % |\langle C(a^{(i)}) v, x\rangle| \geq  u |\langle v, x\rangle|
% % \end{array}
% %   \]
% % since the smallest absolute value of the absolute eigenvalue of the circulant matrix
% % $ C(a)$ is  $u = |\hat a|_{\min}$.

% Now
% \[
%  \begin{array}{ll}
% D
% &\geq \|h*x\|_1- 2\|(h*x)_{S}\|_1\\
%   &= \sum_{i\in S_j^c} |\langle C(a^{(i)}) v, x\rangle|-\sum_{i\in S_j} |\langle C(a^{(i)}) v, x\rangle|
% \end{array}
%   \]
  
% Let's calculate the expectation 
%   \[
%  \begin{array}{ll}
% \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% &=   \expect \left[ (n-2|S|)  |(h*x)_0| \right] \\
%  &\geq 
% n/2 \expect |(h*x)_0|  
% \end{array}
%   \]
% For a generic $h\in\reals^n$, we have a lower bound on expectation using $\|h\|_2$.
% Let $G_{j}=\mbox{sign}(G_{j}) |G_{j}|$, then $\mbox{sign}(G_{j})$ are IID Rademacher ( $\pm 1$) random variables.
%   \[
%  \begin{array}{ll}
% & \expect  \|h*x\|_1\\
% =& n \expect |(h*x)_0|\\  
%  =& n \expect  |\sum_{j=1}^n h_j\Omega_{j} G_{j}|\\
%  =& n \expect   |\sum_{j=1}^n h_j \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
%  \geq&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j\Omega_{j}G_{j})^2}\\
%  =&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j x_{j})^2}\\
%  \geq&   \frac{n}{\sqrt{2}}   \sqrt{\sum_{j=1}^{n} p h_j^2}\\
%   =&   \frac{n\sqrt{p}}{\sqrt{2}}   \| h\|_2 
% \end{array}
%   \]  
% The first inequality is the
% Khintchine inequality.
% The second inequality is Jensen's inequality, because the function is a convex function of $x$,  
% and the second moment of each entry of $x$ is
% \[ \expect(x_{i})^2  = \expect(\Omega_{i})^2(G_{i})^2=\expect(\Omega_{i})\expect(G_{i})^2 = p.\]
% % We can derive another bound using $h=C(a)v$.
% % \[
% %  \begin{array}{ll}
% % \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% % &=   \expect \left[ (1-2|S|/n) \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle|\right] \\
% %  &\geq 
% % 1/2 \expect \left[\sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right] \\
% % \end{array}
% %   \]
  

% %   We want to find the optimal objective value of the problem
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}   &  \expect \left[ \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle| \right]   \\
% % \mbox{subject to}  & \|v\|_1 =1;
% % \end{array}
% %   \]
% % Using the fact that the objective is a convex function of $v$, and is invariant to permutations,  we know that this function is minimized at the point
% %   $(\frac{1}{ k},\ldots,\frac{1}{ k} )$,
% %    \[
% %  \begin{array}{ll}
% %  &  \expect \left[  \sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right]  \\
% %  \geq&  \frac{1}{ k} \expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} G_{j}| \\
% %  =& \frac{1}{ k}\expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
% %  \geq&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j}G_{j})^2}\\
% %  =&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)x_{j})^2}\\
% %  \geq&   \frac{1}{k\sqrt{2}}  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} p(\sum_{t=1}^{k} |a_{i-t+j}|)^2}\\
% %   =&   \frac{\sqrt{np}}{\sqrt{2}}    \sqrt{(\sum_{i=1}^{n} |a_{i}|)^2}\\
% %    =&   \frac{\sqrt{np}}{\sqrt{2}}   \| a\|_1 
% % \end{array}
% %   \]


 

% As a summary of all the inequalities, we get a lower bound on $\expect D $:
% \[
% \expect D  \geq    \frac{\sqrt{p}}{2^{3/2}}  n \| h\|_2.
% \]
% and
% \[
% \expect D  \geq   \frac{ \sqrt{np} }{2^{3/2}}   \| a\|_1\| v\|_1
% \]

% Also we have bound on the second moment.
% First we define the $s$-lag correlation of $a$ to be 
% \[
% R_s(a) = \sum_{t=1}^n a_{t}a_{t+s},
% \]
% and define the sum of the $s$-lag correlation of $a$ as  
% \[
% \begin{array}{ll}
% R(a) = \sum_{s=1}^{n-1}  R_{s}(a) = \sum_{s=1}^{n-1} \sum_{t=1}^n a_{t}a_{t+s}.
% \end{array}
% \]

% \[
% \begin{array}{ll}
% \mbox{Var} \left(  \|h*x\|_1 \right)
% &= \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x v^T C(a^{(i_2)})^T x|\right)\\
% &=   \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x x^T C(a^{(i_2)}) v|\right)\\
% &\leq   p\left(\sum_{i_1\neq i_2}|v^T C(a^{(i_1)})^T C(a^{(i_2)}) v|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}   (\sum_{t=1}^n a_{t}a_{t+(i_2-i_1)})|\sum_{r_1=1}^k\sum_{r_2=1}^k v_{r_1}v_{r_2}|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}  R_{i_2-i_1}(a) \|v\|_2^2 \right)\\
% &= p   n R(a)\|v\|_2^2
% \end{array}
% \]

% And we have bound on the absolute value,
% % let  $\|X_j\|_{\infty} = \tau$, where $\tau\leq 4$ with probability 
% % $1-\Phi(4)$ for $\Phi$ the Gaussian c.d.f, 
% % and since 
% \[
%  \begin{array}{ll}
% | \langle C(a^{(j)}) v, x\rangle|
% &=  | \sum_{i=1}^n  \sum_{t=1}^k a_{i-t+j} v_t x_{i}|\\
% &\leq   \|a\|_{\infty}|\sum_{t=1}^k v_t|| \sum_{i=1}^n x_{i}|\\
% &\leq  \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| \\
% &\leq    \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| 
% \end{array}
% \]
% with probability $1-\exp{(-Cn)}$, 
% \[
%  | \sum_{i=1}^n x_{i}| \leq 8\tau \sqrt{n},
% \]
% then, 
% \[
%  \begin{array}{ll}
% |\langle C(a^{(j)}) v, x\rangle|
% &\leq     8 \sqrt{n} \|v\|_1 \|a\|_{\infty} \tau 
% \end{array}
% \]


Now we need to derive a concentration inequality on $D$. 
We focus on deriving a concentration inequality on $\|h*x\|_1$, and the concentration inequality 
on  $\|(h*x)_S\|_1$ can be derived similarly.

We remark that $ \|h*x\|_1 =\sum_{j=1}^n |h^{(j),T} x|= \sum_{j=1}^n |\langle C(a^{(j)}) v, x\rangle|$, 
if they are independent random variables, we can bound the deviation of $ \|h*x\|_1$ from its mean
using tail bounds via Bernstein’s inequality, by using the previous two bound on
variance and absolute value. 
This is the strategy to derive concentration inequality in dictionary learning\cite{luh2016dictionary,blasiok2016improved}.
This is also the strategy to derive concentration inequality for multiple observation blind deconvolution setting, since there are independence across different observations.

However, here due to the nature of the convolution, we cannot directly apply Bernstein’s inequality. There are additional dependencies that cause technical difficulties. 

% We need to derive concentration via decoupling, by controlling the moments.
Therefore, we use the dual representation of the $1$-norm and use Talagrand-Bernstein’s inequality on supreme of random function to derive concentration.
We put this part of the proof in the following lemma, since they are technical and they could be of independent interest for other problems with dependency structure. 




From the lemma, if we let $Z = \|h*x\|_1$, then we have 
 \[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&= \prob \left[  |Z- \expect Z | > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.

From the previous calculation, we recall that we have a lower bound on expectation 
$ \expect \|h*x\|_1$,
\[
\expect \|h*x\|_1\geq    \sqrt{\frac{p}{2}}  n \| h\|_2 
\] 
\[
\expect Z = \expect \|h*x\|_1 \geq  \sqrt{\frac{p}{2}}  n \| h\|_2
\]
  









Now we calculate $\sigma^2, K$:
 \[
  \begin{array}{ll}
\sigma^2 &=\expect \langle w, C(h)x \rangle^2,\\
&=\expect (C(h)^* w)^T xx^* C(h)^* w  \\
&\leq  p \|C(h)^* w\|_2^2\\
&=p \langle w, C(h)C(h)^* w \rangle 
\end{array}
  \]  
Let $C(h)=UD(\hat{h})U^*$ be the eigen-decomposition, where $U$ is the unitary Fourier matrix, $D(\hat{h})$ is the diagonal matrix with $\hat{h}$ as its diagonal entries. Then using $h=a*v$, $\hat{h}=\hat{a}\hat{v}$, we have
      \[
  \begin{array}{ll}
(C(h)C(h)*) 
&=   UD(\hat{h})U^* U D(\hat{h})^* U^* \\
&=  UD(|\hat{h}|^2) U^* \\
&=  UD(|\hat{a}\hat{v}|^2) U^*. \\
\end{array}
  \] 
Now we have
 \[
  \begin{array}{ll}
\sigma^2 &\leq 
 p \langle w, C(h)C(h)^* w \rangle \\
&= p  \langle w,  UD(|\hat{a}\hat{v}|^2) U^* w \rangle \\
&= p  \langle U^* w,  D(|\hat{a}\hat{v}|^2) U^* w \rangle 
\end{array}
  \] 
Let $\tilde{w} = \langle U^* w $, using the fact that $\|w\|_{\infty}\leq 1$, we have  $\|\tilde{w}\|_{\infty}\leq 1$, therefore,
 \[
  \begin{array}{ll}
\sigma^2 &\leq  p  \langle \tilde{w},  D(|\hat{a}\hat{v}|^2) \tilde{w} \rangle \\
&=  p  \sum_{i=1}^n \tilde{w}_i^2 |\hat{a}_i\hat{v}_i|^2)  \\
&\leq  p  \sum_{i=1}^n  |\hat{a}_i\hat{v}_i|^2 \\
&\leq  p  \max_{i=1}^n |\hat{a}_i|^2\sum_{i=1}^n  |\hat{v}_i|^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 \|v\|_2^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 
\end{array}
  \] 
  
  Now we derive the absolute value bound. First, since $x_i$ are iid sampled from the product of Bernoulli random variable and standard Gaussian, the supreme of the absolute value $\tau = \max_i |x_i|$ is upper bounded by the  supreme of standard Gaussian, which is less than $  2\log^{1/2} n$ with probability $1-\exp(-Cn^2)$. In the following, we only consider this case and assume $\tau \leq 2\log^{1/2} n$ and add the tail probability into the tail probability in the concentration inequality.
  
 Using other side of Khintchine inequality, we have
  \[
 \begin{array}{ll}
&  |(h*x)_i|\\
 =&  |\sum_{j=1}^n h_{i-j} \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
\leq&  
  \sqrt{\sum_{j=1}^{n} (h_{i-j} \Omega_{j}|G_{j}|)^2}\\
 \leq&  \tau  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n}  h_{i-j}^2}\\
   =&   \tau  \| h\|_2 
\end{array}
  \]  
Therefore, we can take $K=  \tau  \| h\|_2  .$
%    \[
%   \begin{array}{ll}
%  |(C(h)^T w)_i x_i|
% &\leq  \tau |(h^{(i),T} w|\\
% &=  \tau |\sum_{j=1}^n h_{i-j}  w_{j}|\\
% &\leq  \tau \|h\|_1.
% \end{array}
%   \]  

 
%  Notice 
%   \[
%   \begin{array}{ll}
% \|h\|_1 \leq \|h\|_2 n^{1/2}.
% \end{array}
%   \]  
%   We have $K\leq  \tau \|h\|_2 n^{1/2} .$
%  Using Young's inequality
%     \[
%   \begin{array}{ll}
% K= \tau \|h\|_1
% \leq  \tau \|a\|_1\|v\|_1 .
% \end{array}
%   \]   











% Moreover, for $1$-norm of $\|h\|_1$, we have Young's inequality
%     \[
%   \begin{array}{ll}
%   \|h\|_1
% \leq  \|a\|_1\|v\|_1 .
% \end{array}
%   \]     

We point out that the eigenvalues of $C(a)$ is the Fourier transform of $\hat a$ of $a$, which is the 
the entry-wise inverse $1/\hat w^{0}$. And the singular values of $C(a)$ are the absolute values $|\hat a|$. 
% \[
%  \begin{array}{ll}
% \min_i |\hat a_i| = \min_i \frac{1}{ |\hat w^0_i|} 
% =\frac{1}{\max_i |\hat w^0_i|} = u.
% \end{array}
% \]
Therefore, using the fact that $\|v\|_2=1$,
\[
 \begin{array}{ll}
 \min_i |\hat a_i| \leq \|h\|_2 =  \|C(a)v\|_2 \leq \max_i |\hat a_i| 
\end{array}
  \]
  
Then the condition number of $C(a)$ can be represented as $\delta_a =   \max_i |\hat a_i|/\min_i |\hat a_i|$.



Overall, for $Z = \|h*x\|_1$, we have $\expect Z \geq \sqrt{\frac{p}{2}}  n \| h\|_2$, we choose $t = \sqrt{\frac{p}{2}}  n \| h\|_2$. Since 
 \[
  \begin{array}{ll}
 \prob \left[  |Z- \expect Z | > t   \right] 
\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right),
\end{array}
  \]  
we calculate
\[
  \begin{array}{ll}
 &  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\\
=&  -\frac{1   }{2(\sigma^2/t^2+K(2\expect Z+t/3)/t^2)}\\
\leq &  -\frac{1   }{2(\sigma^2/t^2+K(2+1/3)/t)}\\
 \end{array}
  \]  
% It can be viewed as $ -\frac{1   }{4} $ multiple the harmonic average of 
% $t^2/\sigma^2$ and $t^2/ K(2\expect Z+t/3)$. We find 
Now, we calculate both terms on the denominator,
  \[
  \begin{array}{ll}
   \sigma^2/t^2 &\leq (p  \max_{i=1}^n |\hat{a}_i|^2)/( \sqrt{\frac{p}{2}}  n \| h\|_2)^2 \\
  &\leq 2\max_{i=1}^n |\hat{a}_i|^2)/(\min_{i=1}^n |\hat{a}_i|^2 n^2 \\
   &\leq 2\delta_a^2/ n^2 ,
 \end{array}
  \]  
   \[
  \begin{array}{ll}
  (2+1/3)K/t 
 &\leq  \frac{7}{3}\tau  \| h\|_2 /\sqrt{\frac{p}{2}}  n \| h\|_2\\
  &\leq \frac{7\sqrt{2}}{3}\tau  /\sqrt{p}  n \\
   &\leq \frac{7}{2}\tau  /\sqrt{p}  n 
 \end{array}
  \]  
  
 As we discussed before, since $\tau$ is the maximum of IID Gaussian random variable, 
 $\tau \leq C_1 \log^{1/2}(n)$ with probability $1 - \exp(-C_2 n^2)$ for $C_1$ large enough.
 
And from the assumption we have $ \delta_a \leq C_0 n^{1/2}/ \log^{1/4}(n)$.
  
Therefore, 
\[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7\tau  /\sqrt{p}  n  } \right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-n   }{  \log^{1/2}(n) (4C_0+  C_3 \sqrt{p})} -C_2 n^2 \right)\\
&\leq   \exp\left( \frac{- C n   }{  (p\log(n))^{1/2}}  \right)
 \end{array}
  \]  
  
  

  
  
  
  
  
  
  
  
% Here the two quantity we care are
% \[
% \langle h, h^{(d)}\rangle / \|h\|_2^2
% \]

% \[
%  \|h\|_1 / \|h\|_2
% \]
\begin{proof}
In the lemma below, we use a covering argument to give a union bound for $v\in B_k=\{v
\in\reals^k\mid \|v\|_2=1\}$. 
We want to cover $B_k$ with $\epsilon$ balls. From classical covering argument,
we know that we need at most $|N| = (3/\epsilon)^k$ $\epsilon$ balls to cover $B_k$, and we use symmetrization trick to find the proper $\epsilon$.

Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
  
Since  $n>  k \log(k/p)$, for large enough constant $C$, we showed in the lemma that there exist a positive constant $C_0$, 
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq  \exp\left(  k\log(3\tau \sqrt{n}np \|a\|_1) - \frac{ C_6 n   }{  (p\log(n))^{1/2}}\right) \\
&\leq    \exp\left( k(\log(3\tau)+\log(\|a\|_1)+\log(p)+3/2 \log(n)) -\frac{ C n   }{  (p\log(n))^{1/2}}\right) 
\end{array}
  \] 
  
% Now we have a tail bound on $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$, which implies a tail bound on 
% $
% \mathcal{X}_v-\mathcal{X}_{v'}$.
%  For all $v, v'\in B_k$,  
%  \[
%   \begin{array}{ll}
% & \prob \left[ |\mathcal{X}_v-\mathcal{X}_{v'}| > \epsilon  \frac{n^{3/2}\sqrt{kp} }{2^{3/2}}    |\bar a| \right] \\
% &\lesssim   \exp\left( Ck\log(\sqrt{n}np \|a\|_1) - \frac{\epsilon^2 \frac{p}{2 }  n^2 \|h\|_2^2 }
% {2pn  (Cn^{1/2}+2k)+2\tau \|h\|_1 \|h\|_2 \sqrt{\frac{p}{2}}  n  (2+\epsilon/3)}\right)
% \end{array}
%   \]  
%  Then we use theorem $19$ of \cite{blasiok2016improved}, we can deduce the tail bound for supremum of $|\mathcal{X}_v|$.
%  \[
%   \begin{array}{ll}
%  \prob \left(\sup_{v \in B_k} |\mathcal{X}_v| > M + \sqrt{t} D_1 + t D_2\right) < e^{-t}
% \end{array}
%   \] 
% Where
% \begin{align*}
% 	M  & := C_1 (\sqrt{2 p}  \gamma_2(B_k, d_2) + \gamma_1(B_k, d_\infty))\\
% 	D_1 & := C_2 \Delta(B_k, \sqrt{2  p} d_2) \\
% 	D_2 & := C_3 \Delta(B_k, d_\infty)
% \end{align*}
% with $d_2, d_\infty$ being the metrics on $\reals^k$ induced by norms $\ell_2, \ell_\infty$ respectively, and $C_1, C_2, C_3$ are universal constants.

Then bound on $\sup_{v \in B_k} |\mathcal{X}_v|$ would imply the same bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$.
And with this bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$, we proved that 
for all $v\neq 0, v \in B_k$, $D>0$ with probability $1-\delta$, where
\[
\delta \leq  \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right)
\]
Therefore, when $n>C_1k^2\log(kp)$, 
$
\delta \leq   \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right),
$
then $\delta$ converges to zero as $k$ goes to infinity.
\end{proof}





\begin{lemma}
Let $Z = \|h*x\|_1$ where $h \in \mathcal{H}$, then 
 \[
  \begin{array}{ll}
& \prob \left[  Z - \expect Z  > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.
\end{lemma}
\begin{proof}
Using duality of $1$-norm, we know that
\[
\|h*x\|_1 = \sup_{\|w\|_\infty\leq 1}\langle w, C(h)x \rangle
\]
 From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
 for the supreme of functions $\langle w, C(h)x \rangle$, since $\expect \langle w, C(h)x \rangle=0$,
 $ \langle w, C(h)x \rangle\leq K$, 
 \[
 \sigma^2 =\expect \langle w, C(h)x \rangle^2,
 \]
 we have
 \[
  \begin{array}{ll}
 \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
\end{proof}
We also remark that the essential concentration inequality that we are trying to derive is the following:
let's consider the case when $x$ is IID standard Gaussian, we define $z = h*x = C(h)x$,
then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,\Sigma(h)),\] where 
\[  \Sigma(h)_{ij} = \langle h^{(i)},  h^{(j)}\rangle\]
And we are trying to derive a concentration inequality for $\|z\|_1$.






\begin{lemma}
For all $v\in B_k$, the probability 
\[
  \begin{array}{ll}
& \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
\leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{lemma}
\begin{proof}
Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{proof}

==> old_sec/sec_old_2020/extension.tex <==




% \paragraph{Sub-Gaussian case}
% For a sub-Gaussian random variable $\Xi$ with unit variance and symmetric c.d.f $F$, we define 
% \[
% K = \|\Xi\|_{\Psi_2} = \sup_{r\geq 1} r^{-1/2}  (E|\Xi|^r)^{1/r}
% \]
% as the sub-gaussian norm of $X$
% \begin{lemma} \label{lem:Khintchine}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then for all $r \geq 2$,
% \[
% \|\psi\|_2 \leq (E(Z)^p)^{1/p} \leq C K p^{1/2} \|\psi\|_2
% \]
% where $C$ is absolute constant.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% The lower bound follows by independence and Holder’s inequality.
% For the upper bound, since we have 
% \[
% \|\sum_i a_i X_i\|_{\Psi_2}^2\leq C\sum_i a_i^2 \| X_i\|_{\Psi_2}^2\leq C\|\psi\|_2^2 K^2,
% \]
% And $Z = \sum_i a_i X_i$ is sub-Gaussian, so for all $p\geq 2$,
% \[
%  (E(Z)^p)^{1/p} \leq \|Z\|_{\Psi_2} p^{1/2} \leq C^{1/2} p^{1/2}\|\psi\|_2 K 
% \]
% \end{proof}
% \begin{lemma} \label{lem:Khintchine for $p=1$}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then
% \[
%      3^{-3/2}C^{-3} K^{-3}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
% \] 
% \[
%      3^{-3/2}C^{-3} K^{-3}  \|\psi\|_2 \leq E |\sum_i a_i X_i| \leq \|\psi\|_2
% \]
% where $C$ is absolute constant, $K = \|X\|_{\Psi_2}$.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% We use the extrapolation trick. 
% Let $Z=\sum_i a_i X_i$, since we have 
% \[ (E(Z)^2){1/2} \leq (E|Z|)^{1/4}((E(Z)^3)^{1/3})^{3/4},\]
% we get 
% \[E|Z|\geq (E(Z)^2)^{2}/ (E(Z)^3).\]

% We get a bound on 
% \[
% \|\psi\|_2 \leq (E(Z)^r)^{1/r} \leq C K p^{1/2} \|\psi\|_2
% \]
% from Khinthine’s inequality for $r = 3$.
% \end{proof}


==> old_sec/sec_old_2020/finite_sample.tex <==
\section{Finite sample analysis}
\paragraph{Finite sample setting}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$ Additionally, in finite sample setting, we assume $a^{-1}$ is zero outside of a centered window of radius $2k+1$, namely, the non-zero part can be written as $(\beta_{-k}, \ldots, \beta_0, \ldots, \beta_k)\in V$. 

We fix the shift and scaling effect by assuming $v^T a^{-1} = 1$ for a generic $v$ that has one single largest entry. 
\item
Let $Y= a* X$ be a linear process, we are given a series of observation $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$.
\item
 We denote $X^{(i)}$ as the sequence being flipped and shifted for $i$ step from $X$ s that $X^{(i)}_k = X_{-k +i}$. Let $J_N$ be the support of $X$.
 We define the length $N=2T+1$ window as $\cT := [-T, T].$
\EIT
Now we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse,
\BEQ
 \begin{array}{ll}
 \underset{w\in V}{  \mbox{minimize} }   & \frac{1}{N}\|w*Y\|_{1,\cT}\\
 \mbox{subject to}  
& v^T w =1.
\end{array}
\tag{$P_{v}^T$}
\EEQ


% Let $C_i(w)$ be $\tilde{w}$ with $i$ step right shift, and define 
% $L_i := |C_i(w)^T Y|$, then 
% \[
% \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]} = \frac{1}{2T+1}\sum_{|i|\in \cT} |[w*Y]_i|  = \frac{1}{2T+1}\sum_{|i|\in \cT} L_i
% \]
% We know that
% \[
% L_i = |C_i(w)^T Y| = |C_i(e_0 +\phi)^T X| = |(e_0 +\phi)^T C_i(X)|
% \]


First, after change of variable,
\[
 \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{N}\|\psi*X\|_{1,\cT}
\]
Then the empirical average can be represented as sum of shifted and flipped inner products.
\[
\frac{1}{N}\|\psi*X\|_{1,\cT}  = \frac{1}{N}\sum_{|i|\in \cT} |[\psi*X]_i| = \frac{1}{N}\sum_{|i|\in \cT}|\psi^T X^{(i)}|
\]
We define 
\[
p_N = \frac{1}{N}\sum_{i\in \cT} I_i
\]
The population average is being calculated,  as
\[
\E  \|\psi*X \|_1:= \E|C_i(\psi)^T X| = \E|\tilde{\psi}^T X|
\]
We know the mean of $p_N$ is $p$, the variance of $p_N$ as
\[
\E[p_N-p]^2=\frac{1}{N}p(1-p)
\]


% \paragraph{Concerntration of finite sample subdifferential}
% Remark:
% From Proposition~$3.5$ (Uniform convergence of subdifferential) in the dictionary learning paper \cite{bai2018subgradient}, we have 
% uniform convergence of subdifferential under Hausdoff distance for all $\psi$ in $2-$norm sphere $S^{n-1}$.


% We want to study 
% \[
% \frac{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}{t} 
% \]

% Notice that
%  \BEAS
%  (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1) = \sqrt{\frac{2}{\pi}} \E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%  \EEAS

% We want to use the empirical formula of sub-gradient:
%  \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}]\\
%   &=& \lim_{t\rightarrow 0^+}\frac{1}{t}[
%   (\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1) 
%   -\sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)\\
%   && + \sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   - (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)]
%  \EEAS
%  and for the second term, diving the constant $\sqrt{\frac{2}{\pi}}$, we have
%   \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{
%  (\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   -\E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%   }]\\
%  &=&  \left(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)-\left(p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)
%  \EEAS
%  If is easy to see that  
% using the fact
% \[
% \E[p_N-p]^2=\frac{1}{N}p(1-p)
% \] 
% we only need to bound
%   \BEAS
%  && (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
%  and we can do further reduction to
%  a bound on 
%   \BEAS
%  && \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]- \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
 
 
 
 \paragraph{Finite sample directional derivative}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (\psi+t\beta)*X \|_1 - \hat{\E}  \| \psi*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{\psi} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}(\psi^T X^{(i)})X^{(i),T}\beta
 \EEAS
Now to study the finite sample convex problem, we need to calculate the directional derivative at $ \psi = e_0$.
Then
\begin{theorem}
For any $X$ sequence with support  $J_N$,
\BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
% \\
%   &=& 
% p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
% (1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
% \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
 
\end{theorem}
\begin{proof}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
 \EEAS
\end{proof}
\begin{coro}
For Gaussian IID sequence $X$, 
 the random variable $ \frac{\|X\|_{1,J_N}}{N} = p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|})$ has mean $p\sqrt{\frac{2}{\pi}}$. 
 And the random expression
\BEAS
& &  \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
\\
  &=& 
p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
 \EEAS
 has mean $\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])$.
\end{coro}
\begin{proof}
 \BEAS
& & 
\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
 \\
  &=& 
p_N ( \frac{\|X\|_{1,J_N}}{|J_N|})\beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
where $p_N = \frac{|J_N|}{N} = \frac{1}{N}\sum_{|i|\in \cT}  1_{X_{-i}\neq 0}$ has mean $p$ and variance $\frac{1}{N} p(1-p)$.
And notice that for the Gaussian IID case 
\[
\E [ p_N\frac{\|X\|_{1,J_N}}{|J_N|}] = \E[p_N|X_{0}|\mid X_{0}\neq 0]  = p\sqrt{\frac{2}{\pi}},
\]
\[
\E [(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N} ] = \sqrt{\frac{2}{\pi}}\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]).
\]
\end{proof}

\begin{coro}
 For symmetric IID sequence $X$, 
  \[
  \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot (\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} ) 
  \]
  where 
  $\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} $ is independent of $X_i$, therefore independent of $(1_{X_{-i}> 0}-1_{X_{-i}< 0}) $.
  Specifically, it has mean $0$
   \[
 \E \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = 0
  \]
  for $q\leq 2$,
    \[
  \frac{1}{N}\E|\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} |^q \leq 
  \frac{1}{N} \E[]|\sum_{i\in J_N}|1_{X_{-i}> 0}-1_{X_{-i}< 0}||^q\cdot  \max_j |X^{(j),T}\beta_{(0)} |^q]
  \]
  
\end{coro}
%   \[
%  p^\star(u):= 
%  \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1 }(-p \cdot \sqrt{1-\| P_{u}^{\perp} P_{e_0}^{\perp} \beta\|_2^2} + (1-p) \cdot  \E_I\| (P_{u}^{\perp} P_{e_0}^{\perp} \beta)_I\|_2 ) > 0\}
%  \]



 \paragraph{Concerntration of $\|\psi*X\|_{1}$ }
The next step is to provide an uniform bound of the finite sample derivation of $\|X\|_{1,J_N}$ and 
$\|X*\beta_{(0)}\|_{1,\cT-J_N}$.

In general, for any random subset $I$ of $\cT$, we study the uniform concentration of 
\[
\|\psi*X\|_{1,I} 
\]
for $\psi = a*w \in a*B_1(V_k),$ by providing moments and tail bound on
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]

For clarity of the argument, we only state the concentration for $\|\psi*X\|_{1,\cT}.$ Also the result about $\cT$ would easy carry to a random subset $I$.

Let the minimal and maximal eigenvalue of the (convolutional) linear operator $a*$ be
\[
\lambda_{m}(a) := \inf_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\[
\lambda_{M}(a) := \sup_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\begin{lemma}
Using circluar embedding of Topelitz matrix, 
\[
\lambda_{M}(a) \leq \max| \hat{a}|
\]
\end{lemma}

Following the idea of lemma~$4$ of the paper of Adamczak on sparse dictionary learning\cite{adamczak2016note} and lemma~$16$ of the paper \cite{spielman2012exact}, we derive a similar bound for convolutional case.
\begin{lemma}
In the following, we define 
\[
Z :=  \frac{1}{N}\|w*a*X\|_{1,\cT}
\]
We find the lower bound of $\E Z$ as a function of the $1-$norm  of $w$:
\[
\E Z  \geq \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1} 
\]
For convenience, we define
\[
\mu_{\mbox{min}}:=\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1}
\]

\end{lemma}
\begin{proof}
WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
\BEAS
\E_X Z 
&=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
&\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
\EEAS
By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
$\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
\BEAS
\E_X Z 
&\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
&\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
&\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
&=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
\EEAS
\end{proof}

% \begin{proof}
% WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
% \BEAS
% \E_X Z 
% &=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
% &\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
% \EEAS
% By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
% then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
% $\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
% \BEAS
% \E_X Z 
% &\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
% &\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
% &\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
% &=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
% \EEAS
% \end{proof}

Now we define the intersection of $1-$norm ball of the $k-$dimensional subspace $V_k$ as $B_1(V_k)$, then we consider $w\in B_1(V_k).$ 
\begin{lemma}
Hence we consider $\psi = a*w \in a*B_1(V_k),$ and we define
\[
W:= \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) |
\]

For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E W^q\leq 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{lemma}

\begin{proof}
Let $\varepsilon_1, \ldots, \varepsilon_N$ be a sequence of IID Rademacher ($\pm 1$)  random variables independent of $X$,  By the symmetrization inequality, see e.g. lemma~$6.3$ of book \cite{ledoux2013probability}, we have the first inequality. Then since the function $t \rightarrow |t| $ is a contraction, an application of Talagrand’s contraction principle (see lemma~$8$ of \cite{adamczak2016note}) with $F (x) = |x|^q$ 
conditionally on $X$ gives the second inequality.
\BEAS
\E W^q 
&\leq& 2^q \E \sup_{\psi \in a*B_1(V_k)} 
|\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j |(\psi*X)_{j}| |^q\\
&\leq&
2^{2q}\E \sup_{\psi \in a*B_1(V_k)} |\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j (\psi*X)_{j} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{\psi \in a*B_1(V_k)} |\sum_{i\in [-T,T] }\psi_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{w \in B_1(V_k)} |\sum_{i\in [-T,T] }(w*a)_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&\leq&
2^{2q}\frac{1}{N^q}\E \max_{s\in [k]}|\sum_{i\in [-T,T] }a_{i-s}( \sum_{j\in [-T,T] } \varepsilon_j X_{j-i}) |^q\\
&\leq&
2^{2q}(\frac{\lambda_{M}(a)}{N})^q   \sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q
\EEAS
Now by the moment version of Bernstein’s inequality (see lemma~$7$, equation $(18)$ of\cite{adamczak2016note}), we know that there exists a universal constant $C$,
\BEAS
\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q \leq C^q(\sqrt{Npq}+q)^q
\EEAS
Therefore, 
\BEAS
\E W^q &\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q    
\sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q \\
&\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\EEAS
Then
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
therefore, we could get the tail bound using the Chebyshev inequality for the moments,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np(q+\log(k))}+q +\log(k)))\leq e^{-q}
\EEAS
We set $q = \log(\frac{1}{\delta})$, then we will get an upper bound for $W$ which is satisfied with probability at least $1-\delta$:
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{proof}

\begin{lemma}
Let the condition number of the linear operator $a*$ be
\[
\kappa_a := \frac{\lambda_M(a)}{\lambda_m(a)}.
\]
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
and  $p\geq \frac{1}{N}$, 
then
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{lemma}
\begin{proof}
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
then 
\[
\frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})} \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
additionally, if $p\geq \frac{1}{N}$, 
then a weaker inequality is also true:
\[
\frac{4eC\lambda_{M}(a) }{N}  
 \log(\frac{k}{\delta}) \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
therefore, combining the two parts and the previous inequality,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
we have
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{proof}


\begin{theorem}
Let the solution of finite sample convex optimization be $w^\star$, 
for small $\epsilon>0$ and concentration level $\delta>0$, 
there exists universal constant $C$, if there are 
% \[
% N=2T+1 \geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
% \]
\[
N \geq k\log(\frac{k}{\delta}) ( \frac{C\kappa_a}{\epsilon}  )^2
\]
and  $ \frac{1}{N}\leq p< p^\star(\epsilon)$, we have 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
% Therefore with probability at least $1-\delta$, $a*w^\star =e_0$ and we recover the sparse vector exactly.

% \textbf{ToDO:}
% or
% $\|a*w^\star -e_0\|_1<\epsilon_1$ provided $p< p_N^\star$ for some $p_N^\star\leq p^\star$.
  \end{theorem}
\begin{proof}
From previous lemma, we know that with the conditions, 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
Therefore, with probability at least $1-\delta$,
\BEAS
W = \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) | \leq \epsilon \mu_{\mbox{min}}
\EEAS
When this is true, for all $\psi \in a*B_1(V_k)$, we have a uniform bound 
\[
 \E |(\psi*X)_{j}|-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
\]
\end{proof}
% then
% \[
%  (\E |(\psi*X)_{j}| - \E |X_{j}|)/\| \psi\|_2-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - |(X)_{j}|)/\| \psi\|_2 \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
% \]
% and from previous condition and the expression of directional derivative, 
% \[
% |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | < 2\epsilon
% \]
% If $p<p^\star(u, \epsilon)$, we know from population result that
% \[
% \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
% \]


\begin{coro}
For $\psi = a*w \in a*B_1(V_k),$ 
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]
For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E U_I^q\leq 2^{2q}(\lambda_{M}(a))^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|U_I\|_q \leq 4eC \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( U_I > 4eC\lambda_{M}(a)  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{coro}

% \textbf{ToDO:  Study the finite sample phase transition condition directly} 
\paragraph{Uniform bound of directional derivative}
We  define the uniform bound of directional derivative
\[
W_D  =\sup_{\|\beta\|_2=1, u^T \beta =0, \beta +e_0 \in a*B_1(V_k)}|\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | 
\]
Notice that
\BEAS
& &\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  
\\
&=& 
\left[\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}\right)\right]-
\\
& &
\left[\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])\right]
\EEAS
From previous uniform bound, with high probability, we have the following three uniform bounds on
\[
|\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}|
\]
\[
|(\frac{1}{N} \|X\|_{1,J_N}-\sqrt{\frac{2}{\pi}}p)|
\]
\[
|\frac{1}{N}\|X*\beta_{(0)}\|_{1,\cT-J_N}-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]|
\]
If $p<p^\star(u, \epsilon)$, we know from population result that
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
\]
If with high probability,  
\[
W_D  \leq \epsilon/2
\]
then using the convexity argument, 
for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]
then $a*w^\star-e_0=0$. 
% \paragraph{Uniform bound of finite difference}
% In the end, we define the uniform bound of finite difference, let 
% $t:=\| \psi-e_0\|_2$,
% \BEAS
% W_{D,t}  = \sup_{\psi \in a*B_1(V_k)}
% |\frac{1}{N}\sum_{j\in [-T,T] } ((|(\psi*X)_{j}|-|X_{j}|) - (\E |(\psi*X)_{j}- \E |X_{j}|)|) |/t
% \EEAS
% then from previous lower bound of finite difference by directional derivative, for all $t\in (0,1]$,
% \[
% W_D  = \lim_{t\rightarrow 0}W_{D,t} \leq   W_{D,t}
% \]
% % Using Lipschitz property of finite difference, if directional derivatives are $L-$Lipschitz function, then
% % \[
% % |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = \phi^\star} \rangle   | < L\epsilon_1
% % \]





% % \textbf{ToDO:}
% % Finish the detail proof and find relation of $\epsilon_1$ to other constant!

% \end{proof}

% \paragraph{Concentration tools}
% \begin{lemma}[Gaussian concentration inequality]\label{lem:gaussian_concentration} Let $ x = ( x_1,\ldots,  x_n)$ be a vector of $n$ independent standard normal variables. Let $f: \reals^n\to \reals$ be an $L$-Lipschitz function. Then for all $t>0$,
% \[
% 	\prob{(|f( x) - \E f( x)| \geq t)} \leq 2\exp\left(-\frac{t^2}{2L^2} \right). 
% \]
% \end{lemma}

% \begin{lemma}[Moment control Bernstein inequality for scalar r.v.s]\emph{(\cite{foucart2013mathematical}, Theorem 7.30)}\label{lem:mc_bernstein_scalar}
% Let $  x_1, \dots,   x_n$ be independent real-valued random variables. Suppose that there exist some positive number $R$ and $\sigma^2$ such that $\frac1n\sum_{i=1}^n\expect{  X_i^2}\leq \sigma^2$ and
% \begin{align*}
% \tfrac1n\textstyle\sum_{i=1}^n\expect{\abs{  x_k}^p} \leq \frac{1}{2}\sigma^2 R^{p-2}p!, \; \; \text{for all integers}\; p \ge 3.
% \end{align*}
% Let $S \doteq \sum_{i=1}^n   x_i$, then for all $t > 0$, it holds  that 
% \begin{align}
% \prob{\abs{S - \expect{S}} \ge t} \leq 2\exp\left(-\frac{t^2}{2n\sigma^2 + 2Rt}\right).   
% \end{align}
% \end{lemma}

% \begin{lemma}[$\eps$-net on sphere]\label{lem:epsnet}\emph{\cite{vershynin2010introduction}}  Let $(X, d)$ be a metric space and let $\eps > 0$.
% A subset of $X$ is called an $\eps$-net of $X$ if for every point $x\in X$ there exists some point $y \in  N(x,\eps)$ so that $d(x, y) \leq\eps$. There exists an $\eps$-net for the sphere $ S^{n-1}$ of size
% 	$ (\frac{3}{\epsilon})^n$.
% \end{lemma}


% \begin{lemma}[Young's convolution inequality]
% For 
% $\frac{1}{p} + \frac{1}{q} = \frac{1}{r} +1,$
% \[
% \lVert f*g\rVert_r\le\lVert f\rVert_p\lVert g\rVert_q
% \]
% \end{lemma}




% \paragraph{Finite sample concentration overview}
% We show the concentration in $3$ steps. First, for a fixed direction  $\beta \in V$, we define the event 
% \[
% \mathcal{X}(\psi)  := (|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X| |\geq t) 
% \]
% % notice that
% % where
% % \[
% % \E[|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} \mid I] = \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} 
% % \]
% % and 
% % \[
% % \E|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} = \E\sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} = \E|\tilde{\psi}^T X| = 
% % \]
% here we can break it into $2$ terms:
% \[
% |\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} |\geq t_1 
% \]

% \[
% | \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} -\sqrt{\frac{\pi}{2}} \E_I \|\psi_{I}\|_{2,[-T,T]} |\geq t_2 
% \]

% and we bound the tail probability 
% \[
% P(\mathcal{X}(\psi) ) = P(|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X|   | \geq t) 
% \]
% Second, we find the Lipschitz constant $L$ of the mapping  $\psi \rightarrow \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]},$ and we replace point event $\mathcal{X}(\psi)$ with a $\epsilon-$ball event 
% $\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi')$ with $\epsilon = \frac{1}{L}.$

% Third, we use $\epsilon-$net to cover the entire $k$-dimensional  space with $k+1$ is the length allowed for the approximate inverse filter $w$ ($w$ is in a $k$-dimensional vector space $V_k$), since the forward filter $a$ is fixed, $\psi = a*w$ is also in a $k$-dimensional vector space $a*V_k$.
% Therefore, 
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]

% \paragraph{Concentration inequality}
% Let $C(\psi)$ be the circulant matrix spanned by the flipped version of $\psi$ as the first column vector.

% Using duality of $1$-norm, we know that
% \[
%  \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} =  \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]} 
% \]

% The Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_x =\sup_{\|b\|_\infty\leq 1}  \|C(\psi)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(\psi) )
%  \]
 
%  On the other hand, $\psi = w*a,$
%  the Lipschitz constant of the mapping $w \rightarrow \frac{1}{2T+1}E_X\sup_{\|b\|_\infty\leq 1}\langle C(w) C(a) b , X\rangle_{[-T,T]}$ is 
%   \[
%  L_w =\sup_{\|b\|_\infty\leq 1}  \|C(a)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(a) )= \|\hat{a}\|_\infty
%  \]

% \begin{lemma}
% From theorem~$8$ of paper \cite{van2013bernstein}, the Bernoulli Gaussian random variable  have sub-exponential tails, and satisfy Bernstein condition with $K =2$.

% Let $Z =\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]}  $, then $\E Z =  \E|\tilde{\psi}^T X|\leq \sqrt{p}\|\psi\|_2$,
%  \[
%   \begin{array}{ll}
% & \prob \left[  Z - \expect Z  > t   \right] \\
% &\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)\\
% &\leq \exp\left(  \frac{-t^2/2   }{\frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 +2(2\sqrt{p}\|\psi\|_2+t/3)}\right)
% \end{array}
%   \]  
% where $\sigma^2=  \expect Z^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 $.
% \end{lemma}

% \begin{proof}
% % Let $\hat{p} := \frac{1}{2T+1}\sum_{|i|\in \cT} 1_{X_i \neq 0}$
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  = 
% % \hat{p} \beta_0 +(1-\hat{p}) \hat{\E}\|\beta * X_{{(0)}}\|_1 
% % \]



% % \[
% %   \| (e_0+t\beta)*X \|_1   = \hat{\E}\sup_{\|b\|_\infty\leq 1}\langle b*(e_0+t\beta) , X\rangle
% % \]
%  From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
%  for the supreme of functions $\langle b*(e_0+t\beta) , X\rangle$, since $\expect \langle b*(e_0+t\beta) , X\rangle=0$,
%  $ \langle b*(e_0+t\beta) , X\rangle\leq K$, 
%  \[
%  \sigma^2 =\expect \frac{1}{(2T+1)^2}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]}^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 
%  \]
%  we have
%  \[
%   \begin{array}{ll}
%  \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
% \end{array}
%   \]  
% \end{proof}
% We also remark that the essential concentration inequality that we are trying to derive is the following:
% let's consider the case when $x$ is IID standard Gaussian, we define $z = \psi*x = C(\psi)^T x$,
% then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,C(\psi) C(\psi)^T),\] where 
% \[  (C(\psi) C(\psi)^T)_{ij} = \langle \psi^{(i)},  \psi^{(j)}\rangle\]
% And we are trying to derive a concentration inequality for $\|z\|_1$.

% \begin{lemma}
% Since $\forall w \in V_k, \|w\|_\infty \leq 1 $, 
% from Young's convolution inequality,
% \[
% \|a*w\|_2 \leq \|w\|_\infty \|a\|_{\frac{2}{3}} = \|a\|_{\frac{2}{3}}
% \]
% and 
% \[
% \| \tilde{a}*a*\tilde{w}*w \|_1\leq \|w\|_\infty^2 \| \tilde{a}*a \|_{\frac{1}{3}} = \| \tilde{a}*a \|_{\frac{1}{3}}
% \]
% \end{lemma}

% \begin{theorem}[Uniform convergence from covering]
% Let $\epsilon:= \frac{1}{L_w},$  then from the $\epsilon-$net covering lemma,
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]
% Here the Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_w
%  = \| \hat{a}\|_\infty
%  \]
%  here $\| \hat{a}\|_\infty$ is the infinity norm (max absolute value of entries) of the Fourier transform of $a$,
%  then
% \BEAS
% &&\prob \left[  Z - \expect Z  > t ,\forall w \in V_k, \|w\|_\infty \leq 1 \right]
% \\
% &=& P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) \\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a*\tilde{w}*w \|_1 p +2(2\sqrt{p}\|a*w\|_2+t/3)}\right)\\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a \|_{\frac{1}{3}} p +2(2\sqrt{p}\|a\|_{\frac{2}{3}}+t/3)}\right)
% \EEAS
% \end{theorem}
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           

% % \begin{lemma}
% % For all $v\in B_k$, the probability 
% % \[
% %   \begin{array}{ll}
% % & \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
% % \leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{lemma}
% % \begin{proof}
% % Let the deviation be
% % \[
% % \tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
% % \]  
% % We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% % % The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

% % We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
% % \[
% % \mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
% % \]  
% %  then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
% %  \[
% %  \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
% %  \]
% %  This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
% % Since  
% % \[
% % \mathcal{X}_v-\mathcal{X}_{v'} =  
% % \sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
% % \]

% % Then use the fact that 
% % \[
% % | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
% % \]
% % and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
% % $s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
% % $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
% % we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

% % From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
% %  \[
% %   \begin{array}{ll}
% % \sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
% % &\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
% % &\leq  \tau \sqrt{n}np \|a\|_1
% % \end{array}
% %   \]  
  
% % Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
% % at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
% % We have a concentration inequality in each ball,
% % We define the tail event 
% % \[
% % \mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
% % \]
% % we can take a union bound,
% %  \[
% %   \begin{array}{ll}
% %  \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
% % &\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{proof}

% % Second, we show that 
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle 
% % \]
% % is locally Lipschitz 
% % % The (set valued) sub-gradient at zero is
% % % \[
% % %   \nabla{L_i} =   \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X),
% % % \]
% % % the directional derivative at zero is
% % % \[
% % %   \nabla_{\phi}{L} = \phi^T \nabla{L_i} =  \mbox{sign}((e_0 +\phi)^T C_i(X))  (\phi^T C_i(X)) ,
% % %   \]
% % % the (set valued) Riemannian subdifferential at zero on the hyperplane defined by $u^T \phi = 0$ is given by
% % % \[
% % %   P_u \nabla{L_i} = (I- uu^T)  \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X) 
% % % \]




% % %  \BEQ
% % %   \begin{array}{ll}
% % %   \expect \nabla{L_i}  &=  p\expect[\nabla{L_i} \mid X_i \neq 0 ] + (1-p)\expect[\nabla{L_i} \mid X_i = 0 ] \\
% % %   &=  p\expect[ \mbox{sign}(X_i) C_i(X)\mid X_i \neq 0 ] + (1-p)\expect[ \mbox{sign}((\phi_{(i)})^T C_i(X)_{(i)}) C_i(X)_{(i)}\mid X_i = 0 ] 
% % %   \end{array}
% % %  \EEQ  



==> old_sec/sec_old_2020/inequal.tex <==
\subsection{$E{| \psi^T X| }$ for IID Bernoulli Gaussian $X$ }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ are unit variance,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \|a\|_2^2.
\]
The ratio indicate the sparsity level of random variable $Z = \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\|a\|_2} 
\]
Now, we consider some settings where exact calculation of $E{|\sum_{i} \psi_i X_i| }$ are possible.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i G_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $G_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
E_X{|\sum_{i} \psi_i X_i| }  
= E_B E_G {|\sum_{i} \psi_i B_i G_i| }
= E_I E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]
then
\[
E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot E_I \|\psi_I\|_2
= \sqrt{\frac{2}{\pi}} \cdot (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2.
\]
Here the last equality use the lemma below, and we define that $\|a\|_0= \#\{ t : \psi_t \neq 0\}$.
\begin{lemma} (Expectation of $2-$norm over Bernoulli support)
\label{lem:BLemma}
\BEQ
E_I \|\psi_I\|_2 = (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2
\EEQ
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:BLemma}]
We have the power series representation $\sqrt{x} = \sum_k c_k x^k$ valid on $(1/A,A)$
for large $A \gg 1$. 
Let $N = |\cT|$. Fix $A > 1/\eps^2$; then every sum $ \sum_{t \in I} \psi_t^2 \in (1/A,A)$;
using this:
\begin{eqnarray*}
 \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  &=&  
 \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \cdot ( \sum_{t \in I} \psi_t^2  )^k \\
 &=& \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&   \sum_k  c_k \sum_{I \subset \cT} \pi(I)   \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 \end{eqnarray*}
 Hence from $ \pi(I) = (p)^{|I|} (1-p)^{|\cT \Delta I|}$
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \sum_{n=1}^{N}  \sum_{|I| = n} (p)^n (1-p)^{N-n}  \cdot  \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  %\\
 \end{eqnarray*}
 Since the inner two sums  cover $ {N \choose n} n^k$ terms in a uniform way,
 we can write
% \clearpage
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \cdot \left( \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n} \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 \end{eqnarray*}
Now use the identity $1 = \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}$  for the complete binomial sum, 
hence the incomplete sum $\sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}= 1-(1-p)^N$. We get
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \cdot \left( 1-(1-p)^N \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 &=& \left( 1-(1-p)^N \right) \cdot \sum_k c_k  \left ( \sum_{t \in \cT} \psi_t^2  \right )^k \\
 &=&  \left( 1-(1-p)^N \right) \cdot  \sqrt{\sum_{t \in \cT} \psi_t^2 } .
\end{eqnarray*}
\end{proof}

==> old_sec/sec_old_2020/population.tex <==

\section{Problem setting for blind deconvolution}
% \subsection{Population problem setting}
\paragraph{Doubly infinite sequence setting}
First, we study the population objective under doubly infinite sequence setting:
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $(Y_t)$, defined by $Y_t \equiv \sum_{h\in \integers} a_h X_{t-h}$, be a linear process, i.e.
\[
Y= a* X,
\]

\subsection{Inverse filter}
\paragraph{Fourier transform and inverse filter}
The discrete-time Fourier transform $\mathcal{F}$ is defined by $\mathcal{F} a = \hat{a}$ where
\[
\hat{a}(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [-\frac{1}{2}, \frac{1}{2}];
\]
the inverse Fourier transform $\mathcal{F}^{-1}$ is defined by
\[
(\mathcal{F}^{-1} f)(n) =  \int_{-\frac{1}{2}}^\frac{1}{2} f(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
\]
Now, our condition on the filter $a$ is:
\[a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.
\]
In the following theorem, we show that this condition would provide the existence of an inverse filter in  $l_1(\integers)$.
\begin{theorem}
If $a\in l_1(\integers) ,  
(\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T,$ we could define the inverse filter of $a$ as
$$a^{-1} := \mathcal{F}^{-1}(\frac{1}{\mathcal{F} a})$$
so that $a^{-1}*a = e_0.$ Here $e_0$ is the sequence with $1$ at $0$ coordinate and $0$ elsewhere.
From Wiener's lemma on $\mathcal{F} a$,   $a^{-1} \in l_1(\integers)$ .
\end{theorem}

\begin{lemma}{\textbf{Wiener's lemma:}}
Assume that a function $f$ on unit circle has an absolutely converging Fourier series, and $f(t)\neq 0$ for all $t \in T$, then $1/f$ also has an absolutely convergent Fourier series.
\end{lemma}



==> old_sec/sec_old_2020/stability.tex <==
\section{Stability for approximation of infinite length inverse filter}

 
 
 

\paragraph{Reduction}
 \begin{lemma} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then the previous convex optimization problem can be reduced to 
  \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  & B(p, \phi) \|\phi \|_2\\
 \mbox{subject to}  
&  \phi = a*w -e_0, \quad w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
  where
  \[
B(p, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
\]
 \end{lemma} 
  
  
\begin{proof}
Following the previous phase transition analysis, 
let the directional finite difference of the objective at $e_0$ be $D(w) = |(w*Y)_0| - |X_0|$, $I$ be the support of $\tilde{X}$, let $\phi = w*a-e_0$,  then we have 
\[
 \begin{array}{ll}
\Expect D(w) &= \sqrt{\frac{2}{\pi}}\Expect_I [\|(w*a)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\|{\phi}\|_2 B(p, \phi)  \\
\end{array}
  \]
The last inequality comes from the bi-Lipschitz property of $\Expect_I \|(e_0+\phi)_I\|_2$ around $e_0$. 

% Now, we use the \textbf{lower semicontinuous extension}!

% First, $\phi \mapsto \Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]$
% is Lipschitz for $\ell_2$ strong convergence.

% Second $\phi \mapsto \| \phi \|_2$ is Lipschitz for $\ell_2$ convergence.

% Hence we need to use a version of $B(p,\| \phi\|_0)$ that is continuous!
% (Qingyun: add a theorem to quote here!)

% Consider the USC (upper semicontinuous) envelope of $B(p,\| \phi\|_0)$:
% \[
% B^+ := \limsup_{\phi_k -> \phi}   B(p,\| \phi\|_0)
% \]
% where the $\limsup$ is over all sequences that converge to $\phi$.

% If we are dealing with $\phi\in \reals^n$,
% then
% \[
% B^+ =  B(p,n)
% \]

% For any contemplated optimizer $\phi^*$ of $\Expect D$ we can find a
% minor perturbation $\phi^{\epsilon}$ with full support, and with at worst a small
% increase in objective over the limit value!

Now using the optimality of $w^\star$ in $V_{rs, rt}$, for all $w in V_{s,t}, w\neq w^\star$,
we have
 \[
 \begin{array}{ll}
\Expect D(w^\star) \leq \Expect D(w)
\end{array}
  \]
We could directly reduce the problem to 
  \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2 
\end{array}
  \]
\end{proof}   
 
% \textbf{Qingyun: this argumemnt has a gap to the deterministic quantity because $B(p, \phi)$ is dependent on configuration of $\phi$. }

% \textbf{TODO}:

\begin{coro}
If there exists a $\phi$ with $\|{\phi}\|_2<1$ such that \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
 for  $\epsilon> 0$ when $p\leq p^\star(\epsilon)$, then 
  \[
  B(p, \phi) \geq \epsilon.
  \]
  for all $\phi$, 
  then
    \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 \leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  is also bounded.
\end{coro}
\begin{proof}
From
 \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
  We have
  \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 
&\leq \frac{B(p, \phi)}{B(p, \phi^\star)}
\|{\phi}\|_2 \\
&\leq \frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
p\Big(\phi_0  +
  \frac{\|{\phi}\|_2}{2} \phi_0^2 
 +
 p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}\|{\phi}\|_2 \\
&\leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  \end{proof}
% Now we want to show that there exists some constant $C$, depending on the worst case directional configuration of $\phi$ and $\phi^\star$,
% \[
% C \geq  \sup_{\phi, \phi^\star}\frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
% p\Big(\phi_0  +
%   \frac{\|{\phi}\|_2}{2} \phi_0^2 
%  +
%  p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
% p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}
% \]
% so that
%   \[
%  \begin{array}{ll}
% \|{\phi^\star}\|_2 \leq C \|{\phi}\|_2
% \end{array}
%   \]
  In the following we constructed a filter to give an upper bound on $\|{\phi}\|_2$. 


\paragraph{Setting for finite length approximation}
Now we consider a setting where there is a kernel whose corresponding inverse kernel has infinite support, and we give a finite-length approximation. 

Within the space $V_{-\infty,\infty}$ of bilaterally infinite real-valued sequences $(h(i))_{i \in \integers}$, consider the affine subspace $V_{N_{-}, N_{+}} = \{ (...,0,0,h_{-N_{-}},\ldots, h_{-1}, 1, h_1, h_2, \ldots, h_{N_{+}},0,0,...)\}$, an $N_{-}+N_{+}$-dimensional subspace of bilateral sequences with support at most $N_{-}+N_{+}+1$.
The coordinate that is fixed to one is 
located at index $i=0$.
Each coordinate is zero outside of a window
of size $N_{-}$ on the left of zero 
and  size $N_{+}$ on the right of zero.
The special sequence $e_0 = (\dots,0,0,1,0,0,\dots)$,
vanishing everywhere except the origin,
belongs to $V_{-\infty,\infty}$ and to every
$V_{N_-,N_+}$.

Let $a \in V_{N_-,N_+}$.
Then $a =  (...,0,0,a_{-N_{-}},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_{N_{+}},0,0,...)$.
We also write $a = e_0 + a_{(0)}$,
where $a_{(0)} \equiv (1-e_0) \cdot a$ 
denotes the `part of $a$ supported away from location
$i=0$'. We also write $a = e_0 + a_L + a_R$,
where $a_L = (a_L(i))_{i \in \integers} 
= (a(i) 1_{\{i < 0\}})_{i \in \integers}$ 
denotes the `part of $a$ supported to
the left of $i=0$' and 
where $a_R = (a_R(i))_{i \in \integers} 
= (a(i) 1_{\{i > 0\}})_{i \in \integers}$
denotes the `part of $a$
supported to the right of $i=0$'.
Finally, we say that $a \in V_{N_{-}, N_{+}}$ 
is a length $ L= N_{-}+N_{+}+1$ filter.

An interesting, if not implementable, objective
function for the blind deconvolution problem
is to minimize
$\Expect [|(w*a*X)_0| - |X_0|] $,
particularly when combined with constraints 
somehow ensuring ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
Defining $\phi \equiv w*a-e_0$, 
\[
 \begin{array}{lll}
\Expect [|(w*a*X)_0| - |X_0|] &=&\Expect [|((e_0 +\phi)*X)_0| - |X_0|].
\end{array}
  \]
  Below we establish the relation
  \[
   \begin{array}{lll}
\Expect [|((e_0 +\phi)*X)_0| - |X_0|] 
&\approx&  C \|{\phi}\|_2 ; \\
\end{array}
\]
This suggests that we should  seek to
minimize $\Expect |(w*Y)_0| $,
while constraining $w$ in some way that
ensures ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
This  the deterministic objective as 
$$
d_a(w, a^{-1}) :=\|{\phi}\|_2 = \|a*w -e_0 \|_2 =  \|a*(w -a^{-1}) \|_2.
$$

Therefore, we want to construct a finite length approximation of $a^{-1}$ to bound $d_a(w^\star, a^{-1}) = \|a*w -e_0 \|_2$ for the optimal point $w^\star$.








We construct the finite length approximation filter explicitly by truncation of Z-transform.

Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.






 
\subsection{ Stability for factorized filter}
\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

If we choose this approximation $w^{r,1},$ then
\[
\|a*w^{r,1}-e_0\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 = s^{2(r+1)} 
\]

In the following, we show that this is indeed the best 

For $\gamma\in (0,1]$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem 
% \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

% If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
% \[
% \|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
% =  (1-\gamma_2)^2 + (\gamma_2 s)^2 
% = \frac{s^2}{1+s^2}
% \]
% And in this case,
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty
% &= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
% &=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
%  \end{array} \]
 
%  Therefore, 
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
%  \end{array} \]


\paragraph{Finite length approximation constructing using Z-transform truncation on factorization form }
Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i},
\end{array}
  \]
We can factorize the Z-transform as product of factors with roots $s_{-j}$ for $j = 1, \ldots N_{-}$ and  $i = 1, \ldots N_{+}.$
\[
 \begin{array}{ll}
A(z) =  c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1}),
\end{array}
  \]
  Where $c_0$ is a constant to make sure that the coefficient $a_0=1$.
  
 We assume that $|s_k|<1,$ for any $k = -N_{-}, \ldots , N_+.$  
  
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.
\[
 \begin{array}{ll}
1/A(z) &=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1})^{-1}\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{\infty} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{\infty} s^{\ell_i}_{i} z^{\ell_i} )
\end{array}
  \]

From previous single root study, we get a hint to study a single truncation of length $ 1 + \sum_{j=1}^{N_{-}} r_{-j}  +  \sum_{j=1}^{N_{+}}  r_i$,  we construct
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r_{-j}} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r_{-j}} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r_i+1}) (1- s_{i} z^{-1})^{-1}
\end{array}
  \]
Let the corresponding filter being $w$.
  
  
Now let $\psi =  a*w$ with Z-transform $\Psi(z)$, $\phi = a*w-e_0$ with Z-transform $\Phi(z)$,we have
\[
 \begin{array}{ll}
\Psi(z): = A(z)W(z) 
&=   \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) 
\end{array}
  \]
  therefore,
\[
 \begin{array}{ll}
\Phi(z): = A(z)W(z) -1 
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) -1
\end{array}
  \]
\paragraph{Upper Bound on  $\|\phi\|_2^2$ for constructed finite length approximation}
In the following,  we want to give upper bound for
  \[
\|a*w -e_0\|_2^2 =\|\phi\|_2^2 
 \]  
  
Redefine the index $\tau_{-j} := r_{-j}+1; \tau_{i} = r_i+1.$
Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible index.
And we define polar representation of complex roots:
for any $k \in \cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$
\[
s_{k} := |s_{k}| e^{i \varphi_k } = e^{\rho_k + i \varphi_k }
\]
where 
\[
 \begin{array}{ll}
\varphi_k := \operatorname{Im}(\log( s_{k} )) = -i \log(\frac{s_{k}}{|s_{k}|}) 
\end{array}
\]
and since $|s_{k}|<1$ we have 
\[
\rho_k = -\operatorname{Re}(\log( s_{k} ))>0
\]

Now we consider all $z = e^{2 \pi i t}$ on the unit circle for $t\in [\frac{-1}{2},\frac{1}{2}]$,
then for any $k \in \cI$
\[
 \begin{array}{ll}
- (s_{k} z^{-\mbox{sign}(k)})^{\tau_{k}} 
&= - |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\\
&=   \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) 
\end{array}
  \]
 Now we simplify the notation by defining 
 \[
 \upsilon_k(t) :=\tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi
 \]
then
 \[
 \begin{array}{ll}
\Phi(z)
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{\tau_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{\tau_{i}}) -1\\
&=  \prod_{k \in \cI} \Big(1- |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\Big)  -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) \bigg)     -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1
\end{array}
  \]
  
\begin{lemma}
 For any $z = \exp{(2 \pi i t )}$ on the unit circle,
 \[
 \begin{array}{ll}
\Phi\big(\exp{(2 \pi i t )}\big)
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1\\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big)
+ i \cdot \big( \upsilon_{k_1}(t) + \ldots+  \upsilon_{k_n}(t)  \big) \Big)  
\end{array}
  \]
 \end{lemma}
 
 \begin{lemma}
Additionally, for any $t \in [\frac{-1}{2},\frac{1}{2}]$,
\[
 \begin{array}{ll}
 |\Phi\big(\exp{(2 \pi i t )}\big)|^2  
= 
\sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
is independent of $t$, since the oscillation integral over the imaginary part is 
  \[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2}
\exp  \bigg( i \cdot \Big(  \big(\upsilon_{k_1}(t) - \upsilon_{k_1}(t) \big) + \ldots+  \big(\upsilon_{k_n}(t) -\upsilon_{k_n}(-t)\big)  \Big) \bigg)  dt
= 1
\end{array}
  \]
Therefore, using Fourier isometry,
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 &= \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi\big(\exp{(2 \pi i t )}\big)|^2 dt \\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
  
 \end{lemma}

\begin{theorem}
\label{thm: Root_2_norm}
Since $|s_{k}|<1$, i.e. $\rho_{k}<0$ for all $k\in \cI$.
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big) 
\end{array}
  \]
  Let $\gamma^m := \min_{i}\big(\tau_{i} |\rho_{i}| \big) =  \min\{\tau_{-N_-}|\rho_{-N_-}|, \ldots, \tau_{-1}|\rho_{-1}|, \tau_{1}|\rho_{1}|, \ldots, \tau_{N_+}|\rho_{N_+}|\}.$
When $\gamma^m \rightarrow \infty$, we have a finite sum of exponential rate  converging terms: the convergence rate is determined by the exponential term as a function of $\gamma^m$.
   \[
 \begin{array}{ll}
 \|\phi\|_2^2 
=    O(\exp \Big( -2 \min_{i}\big(\tau_{i} |\rho_{i}| \big) \Big))
= O(\exp \Big( -2 \gamma^m  \big) \Big))
\rightarrow 0
\end{array}
  \]

 \end{theorem}

 
% \begin{proof}
% Using the expansion, for $Z = \exp{(2 \pi i t )},$ then 
% \[
%  \left|(-1)^n( \prod_{j=1}^n \frac{s_{\ell_j}}{|s_{\ell_j}|}  (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })\right| = 1
% \]
% therefore, for any $t\in [\frac{-1}{2},\frac{1}{2} ]$ 
%  \[
%  \begin{array}{ll}
% \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|
% % &= |\sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % [(-1)^n( \sign[ \prod_{j=1}^n s_{\ell_j}] (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })]|\\
% &\leq \sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % \\
% % &= \prod_{\ell \in \cI} (1+ |s_{\ell}|^{r_\ell+1})-1 
% \end{array}
%   \]
% Therefore, from 
% \[
%  \begin{array}{ll}
% & \|\phi\|_2^2\\
%  =& \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt \\
%   \leq & \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|^2
% \end{array} \]
% we conclude the proof.




%  \[
%  \begin{array}{ll}
% S_{-j}(t) &:= \log(s_{-j} \exp{(2 \pi i t )}) \\
% &= \log(|s_{-j}|)+ i (\pi 1_{s_{-j}<0}+ 2 \pi  t)\\
% S_{i}(t) &:= \log(s_{i} \exp{(-2 \pi i t )})] \\
% &= \log(|s_{i}|)+ i ( \pi 1_{s_{i}<0}+ 2 \pi  t)
% \end{array} \]
% % \[
% %  \begin{array}{ll}
% % R_{+}^{j, r_{-j}}(t) &:= (s_{-j} \exp{(2 \pi i t )})^{r_{-j}+1} \\
% % &= \exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\}\\
% % R_{-}^{i, r_i}(t) &:= (s_{i} \exp{(-2 \pi i t )})^{r_i+1} \\
% % &= \exp\left\{(r_{-j}+1)S_{i}(t) \right\}
% % \end{array} \]
% % and let
% % \[
% %  \begin{array}{ll}
% % Q_{+}^{j, r_{-j}}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\} )\\
% % Q_{-}^{i, r_i}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{i}(t)  \right\} )
% % \end{array} \]

% \[
%  \begin{array}{ll}
%   \Psi(\exp{(2 \pi i t )})
% % &= \gamma \prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t))\\
% % &= \gamma \exp\{ \sum_{j=1}^{N_{-}} Q_{+}^{j, r_{-j}}(t) + \sum_{i=1}^{N_{+}} Q_{-}^{i, r_i}(t)  \}  \\
% &=  \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &=  \int_{\frac{-1}{2}}^\frac{1}{2}  |\Psi(\exp{(2 \pi i t )}) -1|^{2} dt\\
% &= \int_{\frac{-1}{2}}^\frac{1}{2}  | \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
% \end{array} \]
% Consider the case when all the $r_\ell$ are the same as $r,$ and $r\rightarrow \infty$.
% % From the fact that for $x\leq 0,$
% % \[\log( 1-\exp(-x)) = -x + \log(\exp(x) -1)\]
% % and the Laplace's method, 
% we know that to compute
% $\int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt,$
% We only need to compute the maximum value of $\sum_{ \ell \in \cI } S_{\ell}(t)$.
% The maximum value is gonna be $\sum_{ \ell \in \cI } \log(|s_{\ell}|)$, and it is achieved at either $t_0 = 0$, or $t_0 = 1,$ depending on the sum of all the $\sum_{ \ell \in \cI } 1_{s_{\ell}<0}$ is odd or even.

% Therefore, 
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2}  |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
%   \leq&    |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)\log(|s_{\ell}|  \right\} )  \right\} -1|^{2} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\ 
% \end{array} \]
% \end{proof}

==> sec/Discrete_structure.tex <==

\section{Discrete signal structure}
\paragraph{Random model for discrete digital signals.}
We define a random model for discrete digital signals. 

Let $(X_t)$ be an independent
sequence of random variable indexed by  $t \in Z$, with a symmetric distribution with CDF $F$. 
\begin{itemize}
\item The two point symmetric distribution on real number, $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$ 
\item The four point symmetric distribution on complex number, 
$F = 1/4 \delta_{1+i} + 1/4 \delta_{-1+i}+1/4 \delta_{1-i}
+1/4 \delta_{-1-i}.$ 
\item A symmetric distribution on $\reals^s$,
$F = 1/2^s( \sum_{c\in \{\pm 1\}^s} \delta_{\sum_{i\in[s]} c_i e_i } ).$ 

\item Constallantion in unit sphere.
The $2k$ point symmetric distribution on complex number, 
$F_p = \sum_{j=0}^{2k-1} p_j \delta_{\exp{(i\pi\frac{j}{k})}},$
where $\sum_{j=0}^{2k-1} p_j =1, p_j>0.$
\end{itemize}



\paragraph{Convex loss for discrete digital structure.}
The convex loss  we choose could be a relaxation of the convex indictor function of the points.

\begin{itemize}
\item For the two point symmetric distribution on real number, 
\[
g(x) = (|x|-1)_+
\]
\item The four point symmetric distribution on complex number, 
\[
g(z) = (|z|-1)_+,
\]
or more accurately,
\[
g(z) = (\|z\|_{\infty}-1)_+.
\]
\item For $s$-dimensional symmetric distribution on $\{\pm 1\}^s$,
\[
g(x) = (\|x\|_{\infty}-1)_+.
\] 
\end{itemize}


\paragraph{Blind recovery problem.}
For observation $Y$, assume that there exist inverse filter $\mu^* (e_0 + f^*)$, where $f^*_0 = 0$. We try to find it by solving a convex problem,
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E \sum g(\mu (Y+ f*Y)).
\end{eqnarray*}
First, when we know the correct scale $\mu^*$.

Let 
\[
e_0+h = ( e_0 + f)(e_0 + f^*)^{-1},
\]
we have
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    E g( x_0+ h*x)).
\end{eqnarray*}
For $g(x) =(|x|-1)_+$, then the sub-gradient is
\[
g'(x) =  \left.
  \begin{cases}
    1, & \text{for } x > 1 \\
    0, & \text{for } -1 < x < 1 \\
    -1, & \text{for }-1 > x \\
    [0,1], & \text{for }x = 1  \\
    [-1,0], & \text{for }x = -1
  \end{cases}
  \right\}
\]

And the proximal operator $\mbox{prox}_{\rho g}$ is
\[
\mbox{prox}_{\rho g}(x) =  \left.
  \begin{cases}
    x-\rho, & \text{for } x > 1+\rho \\
    x, & \text{for } -1 < x < 1 \\
    x+\rho, & \text{for }-1-\rho > x \\
    1, & \text{for }1 \leq x \leq 1 +\rho \\
    -1, & \text{for } -1 -\rho\leq x \leq -1
  \end{cases}
  \right\}
\]


Assume $(X_t)$ are independent
sequence of random variable with CDF $F_{p}^t = \sum_{j=0}^{1} p^t_j \delta_{(-1)^j},$
where $\sum_{j=0}^{1} p^t_j =1, p^t_j>0.$ We choose the objective
\[
g(z) = (|z|-1)_+.
\] 
To show that $h=0$ is the global minimizer of the convex problem, we only need to show that for any $h\neq 0$, there exists small $\epsilon>0$, 
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)>0.
\end{eqnarray*}
We use sub-gradient information,
\begin{eqnarray*}    
    E g( x_0+ \epsilon h*x)-E g( x_0)
    &\approx& 
    E g'( x_0)(\epsilon h*x)\\
    &=&
    \epsilon( p^0 _1 g'( +1)(h_0)+p^0_{-1}g'( -1)(-h_0)  )
    \geq 0.
\end{eqnarray*}

\paragraph{Polar form and extension to complex plane}
We can rewrite a point on the complex plane as its polar form
\[
z = r \exp{i\theta},
\]
where $r\geq 0$.

Under the polar form, the loss function is 
\[
g(z) = (|z|-1)_+ = (r-1)_+,
\]

We can reparametrize

Using this polar form, we are able to generalize our result to the complex setting.

\paragraph{Non-convex loss for discrete digital structure.}
If we are allowed to use non-convex loss, then we can fix the scale by the loss function.

Instead of convex loss
\[
g(x) = (|x|-1)_+,
\]
or
\[
g(x) = (|x|^2-1)_+,
\]
we can choose
\begin{itemize}
\item The smooth loss 
\[
g(x) = (|x|^2-1)^2,
\]
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (|x|-1)^2,
\]
\item The composition of  smooth function with convex non-smooth function,
\[
g(x) = ||x|^2-1|,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = ||x|-1|.
\]
\end{itemize}


And instead of
\[
g(x) = (\|x\|_{\infty}-1)_+,
\]
we can choose
\begin{itemize}
\item The composition of convex non-smooth function with smooth function,
\[
g(x) = (\|x\|_{\infty}-1)^2,
\]
\item The composition of  two convex non-smooth functions,
\[
g(x) = |\|x\|_{\infty}-1|.
\]
\end{itemize}

\subsection{Noisy observation}
We consider the noisy recovery problem, there are two noise model, one is
\[
y = w_0 * (x+  n),
\]
the other is 
\[
y = w_0 * x+  u = w_0 * (x+ w_0^{-1} *u).
\]
When $u$ is Gaussian $N(0,\Sigma) $ , $w_0^{-1} *u$ is Gaussian $N(0,C_{w_0}^{-1}\Sigma C_{w_0}^{-1,T}) $. Therefore, we could reduce this problem as a colored noise $n$. 

\paragraph{Post-process}
For noisy observation $y$, we apply the algorithm on $y$ to get a solution $\hat x$, then we apply our prior knowledge to project the solution to the constellation points by taking $\title{x} = \mbox{sign}(\hat x).$

Then we measure the ratio of correct recovery by mean of
$1_{\title{x} = x}$ over multiple MC samples.
\paragraph{Population analysis}
Assume that the observation model are $y = w_0 * (x+  \sigma n),$ where $n$ is IID $N(0,1)$. Then we analyze the population risk,
 \begin{eqnarray*}
    \min_{h_0 = 0} &    
     E_x E_n g( x_0+ \sigma n_0+ h^T (x+\sigma n) ).
\end{eqnarray*}
Here $g(x) =(|x|-1)_+$.

Assume that the optimal solution is $h^*_\sigma$, when $\sigma = 0$ we proved before that $h^*=0.$ Here we get
$\hat x_0 = x_0+ \sigma n_0+ h^{*,T} (x+\sigma n) $
want to prove
\[
\tilde x_0 = \mbox{sign}(x_0+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n) ) = x_0,
\]
when $\sigma<\sigma_{m}$.
Without loss of generality, we assume $x_0=1$, we want to ask that when would $1+ \sigma n_0+ h_\sigma^{*,T} (x+\sigma n)\leq 0$, in general, the condition we need to charaterize is when 
$ |\sigma n_0+ h_\sigma^{*,T} (x+\sigma n)|\leq 1$.

\paragraph{Huber version of loss}
Instead of using $g(x) =(|x|-1)_+$, when there are Gaussian noise on $x$, we can use the Huber version 
\[
g_{\mu}(x) =\min_z  \frac{\mu}{2}\|x-z\|^2_2+ (|z|-1)_+  .
\]
% \section{Numerical results}
% \subsection{Convex loss}
% For observation $Y\in \reals^{2N+1}$,  assume that there exist inverse filter $w^* = \mu^* (e_0 + f^*)$, where $f^*_0 = 0$, such that $w^* *Y=X$ is IID distributed by $F = 1/2 \delta_{+1} + 1/2 \delta_{-1}.$  Let
% \[
% g(x) = (\|x\|_{\infty}-1)_+,
% \]
% we try to find it by solving a convex problem,
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2k+1}} &    
%      \sum g(\mu (Y+ f*Y)).
% \end{eqnarray*}
% And we also solve 
% \begin{eqnarray*}
%     \min_{f_0 = 0, f\in \reals^{2N+1}} &    
%      \sum g(\mu (Y+ f*Y))+\lambda \|f\|_1.
% \end{eqnarray*}

% In the following, we assume $\mu^* =1$ WOLG.

% We select $\mu$ in algorithmically by a line search over different choices.

% And the criteria to select is to look at the non-convex loss, say 
% \[
% h(x) = ||x|^2-1|^2,
% \]
% or its gradient. When $g$ or $g'$ is zero, then we know we selected the right scale.

% % \begin{algorithm}
% %   \caption{\textbf{Deconvolution t}}
% %   \label{alg:AA}
% % \begin{algorithmic}[1]
% %   \State {\bfseries Input:} initial point $x_0$, operator $F(\cdot)$, memory $m$
% %   \For{$k=1, 2, \dots$}
% %   \State $m_k=\min\{m, k\}$
% %   \State $\alpha^k$ determined by either the type $1$ or the type $2$ formula above.
% %   \State $x_{k+1} =   \alpha^{k,T}(X^k - \beta_k G_{k})$.
% %   \EndFor
% % \end{algorithmic}
% % \end{algorithm}

% Here is the matlab code,
% \begin{verbatim}
% % % Param
% T = 100;
% n_left = T;
% n_right = T;
% lam = 1e1;
% mu = 1e2;
% k_0 = 10;
% k_1 = 10; 
% k_2 = 100; 
% k_4 = 10;

% scale = 1.;
% % MAX_ITER = 1e1;
% % STEP_SIZE = 1e-4;
% % STEP_MIN = 1e-5;
% % GRAD_TOL = 1e-8;
% % mem_size= 10;
% % beta = 0.5;
% % EPS = 1e-2?;

% % % Set up
% n = n_left+n_right+1;
% delta = [zeros(n_left,1);1; zeros(n_right,1)];

% % % % Model
% % Create x

% % x0 = x0.*randn(n, 1);
% x0 = sign(randn(n, 1));
% % x0_mat = circulant(x0,1);
% J_1 = (x0 > 0);
% J_2 = (x0 < 0);



% % Create forward and inverse filter
% % inverse
% t = 0.1;
% w0_left =[t];
% for j=2:1:k_0
%     w0_left(j,1) =t^j;
% end
% % p1= 0.4;
% % w0_left = t*(rand(k_0, 1) < p1);

% w0 = [zeros(k_0,1);1; -w0_left ];
% w_pad =  [zeros(n_left-k_0,1); w0 ; zeros(n_right-k_0,1)];
% J_w = (max(1,n_left-2*k_0-2):min(2*T,n_left+2*k_0+2));
% % forward
% a0 = ifft(1./fft(w_pad,n),n);
% a_shift = circshift(a0,T);

% % % Property
% % Cos
% cos = norm(w_pad ,inf)/norm(w_pad ,2);
% % Correlation
% w0_mat =  circulant(w0,1);
% w_flip = w0_mat(1,:)';
% R_w = conv(w0, w_flip);

% % Y observation
% y = cconv(a0, x0, n); 
% y_mat =  circulant(y,1);



% cost = @(z) sum(((z).^2-1).^2); 
% grad = @(z) 2*sum(((z).^2-1).*(2*z)); 


% % % % Algorithm compare

% % % Algorithm1
% % %	Exact problem
% % 

% y_mtruc = y_mat(1:n,1:2*k_1+1);
% cvx_begin quiet
% cvx_solver mosek
%   variable w_1(2*k_1+1),
%   minimize( sum(pos(abs(scale*y_mtruc*w_1)-1)))
%   subject to
%       w_1(1+k_1) ==1
% cvx_end

% w_1pad = [zeros(n_left-k_1,1);w_1; zeros( n_right-k_1,1)];
% x_1 = cconv(w_1pad, y, n); 
% delta_1 = cconv(w_1pad,a_shift,n);
% c1 = cost(x_1);
% g1 = grad(x_1);
% % % Algorithm2
% % %	Regularized problem

% y_mtruc2 = y_mat(1:n,1:2*k_2+1);

% cvx_begin quiet
% cvx_solver mosek
%   variable w_2(2*k_2+1),
%   minimize(  sum(pos(abs(scale*y_mtruc2*w_2)-1))+lam* norm(w_2,1))
%   subject to
%       w_2(1+k_2) ==1
% cvx_end

% w_2pad = [zeros(n_left-k_2,1);w_2; zeros( n_right-k_2,1)];
% x_2 = cconv(w_2pad, y, n); 
% delta_2 = cconv(w_2pad,a_shift,n);
% c2 = cost(x_2);
% g2 = grad(x_2);
% \end{verbatim}


==> sec/Expectation.tex <==
\section{Expectation calculation}
\subsection{Expectation over Bernoulli support}

We previously considered the identity
\beq \label{eq:startingPoint}
    \E | \sum_{i \in \cT}  \psi_i X_i | = \sqrt{\frac{2}{\pi}} \cdot \E_I \| \psi \|_{\ell_2(I)},
\eeq
where $X$ is a Bernoulli-Gaussian RV $BG(p;0,1)$,
and where $I$ is a random subset of the domain $\cT$
determined by Bernoulli-$p$ coin tossing.

% (Qingyun:)
% First of all, we know that 
% \[
% \E_I \| \psi \|^{s}_{\ell_2(I)} \leq \| \psi \|^s_{\ell_2(T)}
% \]
% for any $s \in \integers$.

% Because $$


This leads us to consider
\[
  \E_I \| \psi \|_{\ell_2(I)}^{2k}
 \]
 where $I$ is again a random subset, and $k \geq 1$ is an integer.
 The following lemma shows that $\E_I \| \psi \|_{\ell_2(I)}^{2k} \approx \| \psi \|_{\ell_2(\cT)}^{2k}$.

\begin{lemma} \label{lem:BGPropLemmaSub}
Let $\psi$ denote a vector in $\reals^N$.
\[
 \| \psi\|_2^{2k} \cdot \bar{B}(k-1;n,p)    \leq \E_I  \| \psi \|_{\ell_2(I)}^{2k}  \leq     \| \psi\|_2^{2k} ,
\]
where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
is the survivor function (Complementary CDF) of the Binomial.
\end{lemma}

In particular, if $k \leq n \cdot p - 3 \cdot \sqrt{np (1-p)}$ for large $n$, then $\bar{B}(k-1;n,p) > 0.99$.
 The following lemma infers from this that $\E_I \| \psi \|_{\ell_2(I)} \approx \| \psi \|_{\ell_2(\cT)}$.
 
\begin{lemma} \label{lem:BGPropLemmaNorm}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$ as $\eps_N$ could be quite large!}


There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
and so that for each $N$ and for each 
vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
\beq \label{eq:LemmConclu}
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\eeq
\end{lemma}
Applying (\ref{eq:startingPoint}), we get:
\begin{coro} \label{lem:BGPropLemma}
{\bf Qingyun: Numerically, I found this is not true even for fully dense $\psi$!}
There exists a sequence $(\eps_N)$ depending only on $N$, so that  $\eps_N \goto 0$ and
and so that for each $N$ and for each 
vector $\psi$in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$.
\[
(1 - \eps_N) \cdot (1-N^{-1}) \leq  \frac{E | \sum_{i \in \cT}  \psi_i X_i |}{\sqrt{\frac{2}{\pi}}  \| \psi \|_{\ell_2(\cT)}}  \leq   ( 1 + \eps_N).
\]
% and
% \[
% E | \sum_{i \in \cT}  \psi_i X_i |  \geq  (1 - \eps_N) \cdot (1-N^{-1}) \cdot \sqrt{\frac{2}{\pi}} \cdot E \| \psi \|_{\ell_2(\cT)} .
% \]
\end{coro}


\subsection{Proof of Lemma \ref{lem:BGPropLemmaSub}}

\begin{proof}[Proof of Lemma \ref{lem:BGPropLemmaSub}]
Let's first suppose that $|\psi_t| \geq \eps > 0$ for $-T \leq t \leq T$. Let $N = 2T+1$, and
let $I$ denote a subset of indices in $ \cT = \{-T,\dots,T\}$ and
let $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|}$. 
\begin{eqnarray*}
\E_I  \| \psi \|_{\ell_2(I)}^{2k}  &=&  \sum_{n=1}^{N}  \sum_{ |I |=n} \pi(I)   \| \psi \|_{\ell_2(I)}^{2k} \\
% &=& 
%   \sum_{I \subset \cT} \pi(I)    \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&   \sum_{n=1}^{N}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k}  \\
   \end{eqnarray*}
where we used $ \pi(I) = (1-p)^{|I|} p^{|\cT \Delta I|} $.
We partition the sum  $\sum_{n=1}^{N} = \sum_{n=1}^{k-1} + \sum_{k}^N =  \sum_{n<k} + \sum_{n\geq k}$, say.
Now from $\#\{ |I|\leq n\} = {N \choose n}$ and $ \| \psi \|_{\ell_2(I)} \leq \| \psi \|_{\ell_2(\cT)}$,
\begin{eqnarray*}
 \sum_{n<k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
     &\leq&   \left( \sum_{n=1}^{k-1} (1-p)^n p^{N-n} {N \choose n} \right) \cdot  \left( \| \psi \|_{\ell_2}^{2k} \right) \\
     &=& B(k-1;n,p) \cdot   \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
where $B(x;n,p)$ denotes the cumulative distribution function of the binomial distribution.
For the sum $\sum_{n\geq k}$, we may write $\sum_{|I|=n} = {N \choose n}  \cdot Ave_{|I| = n}$
and $\sum_{t_1,\dots, t_k \in I} =  {n^k} \cdot  Ave_{t_1,\dots, t_k \in I}$, so
\begin{eqnarray*}
 \sum_{|I| = n}  \| \psi \|_{\ell_2(I)}^{2k} &=& \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2 \\
& =& {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2 \\
&=& {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot \sum_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2,\\
&=& {N \choose n}  \cdot  \| \psi \|_{\ell_2}^{2k} ,
\end{eqnarray*}
because the inner two averages  cover the $ {N \choose n} n^k$ terms in a uniform way.
We arrive at 
% \clearpage
 \begin{eqnarray*}
 \sum_{n\geq k}  (1-p)^n p^{N-n}  \cdot  \sum_{|I| =n} \| \psi \|_{\ell_2(I)}^{2k} 
  &=&     \| \psi \|_{\ell_2}^{2k} \cdot  \left( \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} \right) \\
  &=&    \| \psi \|_{\ell_2}^{2k} \cdot \bar{B}(k-1;n,p) .
 \end{eqnarray*} 
Here $\bar{B}(x;n,p) = 1- B(x;n,p)$ denotes the 
survivor function (complementary distribution function) of the binomial distribution.
We obtain:
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  
  & = &  \left( \sum_{n \geq k} + \sum_{n<k}   \right) \sum_{|I|=n}  \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k} \\
 &\leq &    \|\psi\|_2^{2k} \cdot  \left( \bar{B}(k-1;p,n)  + B(k-1;p,n) \right) \\
 & = &  \|\psi\|_2^{2k} .
 \end{eqnarray*}
 while
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}   & \geq & \sum_{n \geq k} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{k}  \\
 &= &    \|\psi\|_2^{2k} \cdot \bar{B}(k-1;p,n) .
  \end{eqnarray*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:BGPropLemmaNorm}}

\begin{proof}
Fix $A > 0$ and $p \in (0,1)$
By the Weierstrass approximation theorem, we may find a sequence of polynomials $S_K(t) = \sum_{k=0}^{K} c_k t^k$
so that
\[
    | \sqrt{x} - S_K(x) |_{L^\infty([0,A])} \leq \eps_K, \quad \mbox { and } \eps_K \goto 0 \mbox{ as } K \goto \infty.
\]
Pick a sequence $(K_N)$ so that $K_N \goto \infty$ while
$K_N < N \cdot p -  \sqrt{2 \log(N) \sqrt{N} p (1-p)} $ and
\[
\bar{B}(K_N-1; n,p) > 1 - N^{-1}.
\]
Relabel $S_N  \equiv S_{K_N}$ and $\eps_N \equiv \eps_{K_N} $.
Then $\eps_N \goto 0$ as $N \goto \infty$.

Fix $N$. For each $I \subset \cT$,
let  $x_I \equiv \E_I \| \psi \|_{\ell_2(I)}^{2}$.  Then
\[
     E _I \| \psi \|_{\ell_2(I)} = \E_I \sqrt{\| \psi \|_{\ell_2(I)}^2} = \E_I \sqrt{ x_I }.
\]
while
\[
     E _I \| \psi \|_{\ell_2(I)}^{2k} = \E_I  x_I^k.
\]
Invoking our earlier lemma,
\[
 \bar{B}(k-1;n,p) \leq  \frac{\E_I  x_I^k}{\| \psi \|_{\ell_2(\cT)}^{2k}} \leq 1.
\]

Armed with  polynomial $S_N$ of degree $K_N$, consider
\begin{eqnarray*}
     \E_I S_{N}( x_I ) &=& \E_I \sum_{k=1}^{K_N} c_k x_I^{k}\\
     &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\leq& \sum_{k=1}^{K_N} c_k   \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& S_{N}( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\leq& ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} + \eps_{N} . 
\end{eqnarray*}
where we used $\E_I x_I^{k} \leq  \| \psi \|_{\ell_2(\cT)}^{2k}$ from the previous Lemma.
Similarly,
\begin{eqnarray*}
     \E_I S_N( x_I )   &=&  \sum_{k=1}^{K_N} c_k  \E_I x_I^{k} \\
     &\geq& \sum_{k=1}^{K_N} c_k   \cdot \bar{B}(k-1; n,p) \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &\geq& \bar{B}(K_N-1; n,p) \cdot \sum_{k=1}^{K} c_k   \cdot \| \psi \|_{\ell_2(\cT)}^{2k}\\
     &=& \bar{B}(K_N-1; n,p)  \cdot S_K( \| \psi \|_{\ell_2(\cT)}^2)  \\
     &\geq&  \bar{B}(K_N-1; n,p)  \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  \\
   &\geq&  (1- N^{-1}) \cdot \left( ( \| \psi \|_{\ell_2(\cT)}^2)^{1/2} - \eps_N \right)  . 
\end{eqnarray*}
Here  we used $\E_I x_I^{k} \geq  \| \psi \|_{\ell_2(\cT)}^{2k} \cdot \bar{B}(k-1;n,p)$ from the previous Lemma.
We also used the monotonicity 
of the survivor function $\bar{B}(x) \geq \bar{B}(x+1)$.
We obtain (\ref{eq:LemmConclu}):
\[
 (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 + \eps_N .
\]
\end{proof}


We define the functional  $\Gamma: \psi  \mapsto \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$,
from the previous calculation we know $\Gamma(\psi) $ is only a function of $\| \psi\|_0$. 
So we can identify  $\Gamma(\psi) $ as  $\Gamma(\| \psi\|_0)$. 





\subsection{Sharper bounds on $\frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}}$}




\begin{lemma}
\label{TaylorSqrt}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{1/2}
=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{1/2}
=\sum_{\ell=0}^\infty\binom{1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{1/2}{\ell}
&=\frac{\frac12(\frac12-1)(\frac12-2)\cdots(\frac12-\ell+1)}{\ell!}\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-3)\\
&=\frac{(-1)^{\ell-1}}{2^\ell\ell!}\frac{(2\ell-2)!}{2^{\ell-1}(\ell-1)!}\\
&=\frac{(-1)^{\ell-1}}{\ell2^{2\ell-1}}\binom{2\ell-2}{\ell-1}
\end{align}
then
\begin{align}
(1-x)^{1/2}
&=1-\sum_{\ell=1}^\infty\frac2\ell\binom{2\ell-2}{\ell-1}\left(\frac x4\right)^\ell\\
&=1-\sum_{\ell=0}^\infty\frac2{\ell+1}\binom{2\ell}{\ell}\left(\frac x4\right)^{\ell+1}
\end{align}





% leveraging the 
%  Taylor series of $\sqrt{x}$ around any $a>0$:
%  \[
%  \sqrt{x} = \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {{a}^{\frac{1}{2}-n} \left( x-a\right)^{n}}{\Gamma\left( \frac{3}{2}-n \right)n! }}.
%  \]
%  We could apply the  Taylor series expansion around $1$ to  $\frac{ \| \psi \|_{\ell_2(I)}}{\| \psi \|_{\ell_2(T)}}$,
%  \begin{eqnarray*}
%   \sqrt{\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}} 
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}}-1\right)^{n}\\
%  &=&  \sum _{n=0}^{\infty }\frac{\sqrt {\pi }}{2}\,{\frac {1}{\Gamma\left( \frac{3}{2}-n \right)n! }}  \left( \sum_{i=0}^n 
%  {n \choose i} (\frac{ \| \psi \|^2_{\ell_2(I)}}{\| \psi \|^2_{\ell_2(T)}})^i (-1)^{n-i}\right)
%  \end{eqnarray*}

\end{proof}

\begin{lemma}
\beq 
0 \leq 1- Q(N, p)\leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq 1 .
\eeq
where 
\[
Q(N, p) := \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p),
\]
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|_{\ell_2(J)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(J)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq 1 .
\eeq
Therefore, 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ \frac{ \| \psi \|^2_{\ell_2(I)} }{\| \psi \|^2_{\ell_2(\cT)}}} \leq \E_I 1 = 1 .
\eeq

On the other hand, let 
\beq 
\E_I \frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} 
 = \E_I \sqrt{ 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}}}  .
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.

Applying Lemma \ref{TaylorSqrt},
\begin{align}
(1-\rho_J)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\rho_J^{\ell+1}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_I)^{1/2}
=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell;n,1-p)    \leq \E_I \rho_I^{\ell+1} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell}
\E_I \rho_I^{\ell+1}\\
&\geq  1-\sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1- \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p)\\
&= 1- Q(N, p)
\end{align}
% {\bf NOTE: I am not getting the inequality $Q(N,P) \leq N^{-1}$.
% See Below.}
{\bf Qingyun NOTE: I observe numerically that $Q(N,p)$ could be between $0$ and $1$ in a wide range, and $Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$, with $Q(N,1) = 0$, $\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$
.}
\end{proof}

\paragraph{Beta function and $Q(N,p)$}
If we define the complete beta function as 
\[
\Beta(a,b) := \int_0^1 t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then
% \[
% \Beta(x,y)=\frac{\Gamma(x)\,\Gamma(y)}{\Gamma(x+y)}
% \]
% therefore,
\[
\binom{n}{k} = \frac{1}{(n+1) \Beta(n-k+1, k+1)}
\]
the incomplete beta function as
\[
\Beta(x;\,a,b) = \int_0^x t^{a-1}\,(1-t)^{b-1}\,dt.
\]
then the regularized incomplete beta function is defined in terms of the incomplete beta function and the complete beta function:
\[
I_x(a,b) = \frac{\Beta(x;\,a,b)}{\Beta(a,b)}.
\]
then
\[
I_p(k,N-k-1)= \bar{B}(k-1;N,p) = \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}
\]
and
\[
I_{1-p}(k+1, N-k) = 1 - I_p(N-k, k+1) = \bar{B}(k;N,1-p).
\]
Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$, from the classical De Moivre–Laplace theorem on normal approximation to the binomial, 
\[
{N \choose k}\, p^k q^{N-k} \approx \frac{1}{\sqrt{2 \pi Np(1-p)}}\,e^{-\frac{(k-Np)^2}{2Np(1-p)}}
\]
therefore, 
\[
I_{1-p}(\ell+1, N-\ell) = \bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;

\BEAS
Q(N,p) 
&\equiv& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&=& \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1} \frac{1}{(2\ell+1) \Beta(\ell+1, \ell+1)}  I_{1-p}(\ell+1, N-\ell)\\
&\approx& \sum_{\ell=0}^N\frac{1}{2(\ell+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{-\frac{(\ell-\frac{N}{2})^2}{\frac{N}{2}}}  \bar{\Phi}( (\ell - N \cdot (1-p))/\sqrt{N \cdot p \cdot (1-p)} )\\
&\approx& \int_0^1 \frac{1}{2(Nt+1)} \frac{1}{\sqrt{\frac{\pi}{2} N}}\,e^{- 2N(t-\frac{1}{2})^2}  \bar{\Phi}( \frac{\sqrt{N}(t - (1-p))}{\sqrt{ p \cdot (1-p)}} ) \,dt
\EEAS

Numerically, we can see that the first term in the sum is always $0.5.$
Also we know that by definition $Q(N, 1) = 1$ for any $N$.
From numerically calculation we guess that
$Q(N,p)$ is monotonically increasing with $N$, and monotonically decreasing with $p$.
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
$\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.$


\begin{lemma}
Define:
\[
Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
\]
Then, 
\[
Q(N,p') \geq Q(N,p), \quad, p>p'
\]
and 
\[
\lim_{N\rightarrow \infty}\lim_{p\rightarrow 0} Q(N,p) = 1.
\]
\end{lemma}


% \begin{lemma}
% Define:
% \[
% Q(N,p) \equiv \sum_{\ell=0}^N\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p).
% \]
% Then, as $N \rightarrow \infty$ with $p$ fixed:
% \[
% Q(N,p)  \approx O(N^{-1/2}).
% \]
% \end{lemma}
\begin{proof}
The first term in the sum is $0.5$.

(Sketch). 
{\bf The sum has the lower bound $Q \geq 1/10$ just by inspecting
the first 10 terms (say), which are all positive and all greater
than $0.01$ (say). The following argument shows that later terms
add up to at least $\Omega(N^{-1/2})$.}
First, we know that
\[
\bar{B}(\ell;N,1-p) \equiv  \sum_{n=0}^{N-\ell-1} (1-p)^n p^{N-n} {N \choose n}.
\]

Let $\mu = N \cdot (1-p)$ and 
$\sigma = \sqrt{N \cdot p \cdot (1-p)}$.

We note that, for large $N$ 
\[
\bar{B}(\ell;N,1-p)  \approx \bar{\Phi}( (\ell - \mu)/\sigma ) ,
\]
where $\Phi$ denotes the standard Normal $N(0,1)$ CDF
and $\bar{\Phi} \equiv 1-\Phi$ 
the corresponding survivor function;
this is the classical De Moivre theorem on normal approximation to the binomial. It can be made precise in many ways
that have been well documented over the centuries.
Roughly speaking, in terms of variable $z = (\ell - \mu)/\sigma$,
we have
\[
\bar{B}(\ell;N,1-p)  \approx \left \{ \begin{array}{ll}
1 & z < 3 \\
0 & z > 3 .
\end{array}
\right .
\]

Hence, defining for $m = \mu - 3 \sigma$
\[
\bar{B}(\ell;N,1-p) \approx 1, \mbox{ for } \ell \leq m.
\]
Now of course
\begin{eqnarray*}
Q(N,p) &\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} \bar{B}(\ell;N,1-p) \\
&\geq& \sum_{\ell=0}^m\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} .
\end{eqnarray*}
Now from DeMoivre's theorem (case $p=1/2$, $N=2\ell$) we also know that
\[
    2^{-2\ell} { 2 \ell \choose \ell} = bin(\ell; 2 \ell, 1/2) \sim \sqrt{\frac{1}{\ell \cdot \pi}},
\]
where $bin(k;N,p)$ is the usual binomial probability mass function.
We obtain
\[
  \sum_{\ell=0}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2} \geq 
  \sum_{\ell=m/2}^m\frac{2^{-(1)}}{\ell+1} \ell^{-1/2}  \geq 
  Const  \cdot m^{-1/2}
\]

\end{proof}





\subsection{Bounds on $\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}$}
\begin{lemma}
\label{TaylorSqrtInv}
For $ 0 \leq x\leq 1,$
\begin{align}
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(x\right)^{\ell}
\end{align}
\end{lemma}

\begin{proof}
From generalized binomial theorem, we know that for $ 0 \leq x\leq 1,$
\beq
(1-x)^{-1/2}
=\sum_{\ell=0}^\infty\binom{-1/2}{\ell}(-x)^\ell
\eeq

\begin{align}
\binom{-1/2}{\ell}(-1)^\ell
&=\frac{-\frac12(-\frac12-1)(-\frac12-2)\cdots(-\frac12-\ell+1)}{\ell!}\\
&=\frac{1}{2^\ell\ell!}1\cdot3\cdot5\cdots(2\ell-1)\\
&=\frac{1}{2^\ell\ell!}\frac{(2\ell)!}{2^{\ell}(\ell)!}\\
&=\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}
\end{align}
\end{proof}

\begin{lemma}
\label{TaylorSqrtInvExpect}
\beq 
1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p) \geq  \frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} \geq 1 .
\eeq
where 
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\end{lemma}
\begin{proof}
For any fixed support $J\subset \cT,$ 
\beq 
 \frac{ \| \psi \|^{-1}_{\ell_2(J)} }{\| \psi \|^{-1}_{\ell_2(\cT)}} 
 = \sqrt{ \frac{ \| \psi \|^2_{\ell_2(\cT)} }{\| \psi \|^2_{\ell_2(J)}}} \geq 1 .
\eeq
Therefore, 
\beq 
\frac{\E_I  \| \psi \|^{-1}_{\ell_2(I)} }{\| \psi \|^{-1}_{\ell_2(\cT)}}  
 \geq   1 .
\eeq

On the other hand, let 
\beq 
\E_I (\frac{ \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} )^{-1}
 = \E_I ( 1- \frac{ \| \psi \|^2_{\ell_2(\cT-I)} }{\| \psi \|^2_{\ell_2(\cT)}})^{-1/2}.
\eeq

For a fixed subset $J \subset [n]$ define 
the ratio $\rho_J \equiv  \frac{ \| \psi \|^2_{\ell_2(\cT-J)} }{\| \psi \|^2_{\ell_2(\cT)}}$; it 
obeys $0 \leq \rho_J \leq 1$.


\begin{align}
(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\left(\rho_J\right)^{\ell}
\end{align}
Now with $I$ a random subset as earlier, we
induce a random variable $\rho_I$.
\begin{align}
\E_I(1-\rho_J)^{-1/2}
=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\end{align}
Modify the argument behind Lemma \ref{lem:BGPropLemmaSub} so it applies to $\E_I \rho_I^{\ell+1}$. In the new argument the set $I$ is everywhere replaced by its complement $T-I$. The conclusion is correspondingly modified so that $p$ in the final formula is replaced by $q \equiv 1-p$.
We obtain:
\[
 \bar{B}(\ell-1;n,1-p)    \leq \E_I \rho_I^{\ell} \leq    1,
\]
where, if $k \in \{0,1,\dots,N\}$,
$\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n}  = 1- \sum_{n=0}^{k-1} (1-p)^n p^{N-n} {N \choose n}$, while if $k \geq N$, $\bar{B}(k) = 0$, and if $k < 0$,
$\bar{B}(k) =1$.
Then
\[
\bar{B}(\ell-1;N,1-p) \equiv  \sum_{n=0}^{N-\ell} (1-p)^n p^{N-n} {N \choose n} 
\]
\begin{align}
\E_I(1-\rho_I)^{1/2}
&=\sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\E_I\left(\rho_J\right)^{\ell}
\\
&\geq  \sum_{\ell=0}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)\\
%&=1- \sum_{\ell=0}^\infty\frac{2^{-(2\ell+1)}}{\ell+1}\binom{2\ell}{\ell} [\sum_{n=\ell}^{N} (1-p)^n p^{N-n} {N \choose n} ]\\
&=1+\sum_{\ell=1}^\infty\frac{1}{2^{2\ell}}\binom{2\ell}{\ell}\bar{B}(\ell-1;N,1-p)
\end{align}

\end{proof}





\subsection{Numerically calculate $\E_I  \| \psi_I \|_2/\| \psi \|_2$}

We numerically compute $Q(N,p)$, the result is in the following table. Compare the table with the tables of MC approximation, we see that our previous bound is still too loose.
\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{$Q(N,p)$} \\
\hline
  $p=$ &0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0.9439 & 0.9406 & 0.9370 & 0.920  & 0.8172 & 0.3358 & 0.0482 & 0 \\
\hline
$N=500$ & 0.9748  & 0.9734 & 0.9718 & 0.9643 & 0.9199 & 0.7302 & 0.209 & 0 \\
\hline      
\end{tabular}
\label{Q_table}
\end{table}

Then we use MC approximation to calculate $\E_I  \| \psi_I \|_2/\|  \psi \|_2$ for a few different $\psi.$
We will know that
\BIT
\item 
When $\psi = e_0$,  $\E_I  \| (e_0)_I \|_2=p$ 

\item
When $\psi = e_0+e_1$,  
\[
\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2 = \sqrt{\frac12} \E_I  \| (e_0+e_1)_I \|_2 = 
\E_I \sqrt{\frac{\sum_{i=\{0,1\}} I_i}{2}}=p^2+ 2p(1-p)\sqrt{\frac12}
\]
\item
We know that when $\psi = a =(1,\ldots,1)$, then
\[
\E_I  \| a_I \|_2/\| a \|_2=\E_I \sqrt{\frac{\sum_{i=[N]} I_i}{N}} 
\]
Using law of large numbers, 
\[
\lim_{N\rightarrow \infty }\sqrt{\frac{\sum_{i=[N]} I_i}{N}}  = \sqrt{p}.
\]
\item
For fixed support $J$, we can choose $\psi = \sum_{i\in J} e_i,$ then $\| \psi_J \|_2/\|  \psi \|_2 =1.$
However, the expectation is not going to be one. Let $M := |J|,$
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} = \sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}\leq \sqrt{p}
\]
The inequality can be seeing using central limit theorem, we have normal approximation  $\frac{\sum_{i\in J} I_i}{|J|} \sim N(p,  \frac{p(1-p)}{\sqrt{|J|}})$, then using Jensen's inequality, since square root fucntion is concave,
\[
\E_I \sqrt{\frac{\sum_{i\in J} I_i}{|J|}} \approx \E_G\sqrt{p+ \frac{p(1-p)}{\sqrt{|J|}}G}  \leq \sqrt{\E_G[p+ \frac{p(1-p)}{\sqrt{|J|}}G]} =\sqrt{p} 
\]
\EIT
Using symmetry, we guess that the maximum value of $\E_I  \| \psi_I \|_2/\|  \psi \|_2$  is $\sqrt{p}$ instead of $1$, and the maximum value is achieved when $\psi$ is dense.

\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \| a_I \|_2/\| a \|_2$ where $a=(1,\ldots,1)$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=100$ &0 & 0.3123 & 0.4460 & 0.7063  & 0.94865 & 0.9950 & 0.9995 & 1 \\
\hline
$N=500$ &0 &0.3153  & 0.4464 & 0.7068 & 0.94874 & 0.9950 & 0.9995 & 1\\
\hline      
\end{tabular}
\label{allone_table}
\end{table}


\begin{table}[]
\begin{tabular}{|p{3cm}||llllllll}
\hline
\multicolumn{9}{|c|}{MC approximation ($M=10^4$) of $\E_I  \|(e_0+e_1)_I \|_2 /\| e_0+e_1 \|_2$} \\
\hline
  $p=$ & 0   & 0.1   & 0.2       &   0.5     &   0.9     &   0.99     &  0.999 &1      \\
 \hline\hline
$N=500$ & 0 &0.1375 &	0.2667 &	0.6034 &	0.9365 &	0.9946 &	0.9994 & 1 \\
\hline      
\end{tabular}
\label{coordinatevector_table}
\end{table}



\subsection{Tight bound and stationary points of $\E_I  \| \psi_I \|_2/\| \psi \|_2$}
\begin{lemma}
\beq 
p \leq  \frac{\E_I  \| \psi \|_{\ell_2(I)} }{\| \psi \|_{\ell_2(\cT)}} \leq \sqrt{p}  .
\eeq
where the lower bound is achieved by $1-$sparse vectors $\pm e_i$, the upper bound is achieve by $\{\frac{\sum_{i\in \cT} \pm e_i}{\sqrt{N}}\}$.
Furthermore, all the stationary points of this objective are $\{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ for different support $J\subset \cT$. 
\end{lemma}
\begin{proof}
This problem can be reformulate as the projection pursuit with sphere constraint,
 \begin{eqnarray*}
    \min&   \E_I  \| \psi_I \|_2\\
    \mbox{ subject to }&   \| \psi \|_2 = 1.
\end{eqnarray*}
Then from \cite{bai2018subgradient} Proposition $3.3$, we get the result. 

The main idea of the proof is to calculate the projected gradient
for $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$, when $|J| = M,$
\[
e_j^T  \E_I  \partial\| q_I \|_2 = q_j [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}] 
\]
so
\[
(I-q q^T)  \E_I  \partial\| q_I \|_2 = [\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q-[\sum_{k=0}^{M} (1-p)^{M-k} p^{k} {M \choose k}\sqrt{\frac{k}{M}}]q = 0.
\]
then $q\in \{\frac{\sum_{i\in J} \pm e_i}{\sqrt{|J|}}\}$ is stationary points.
 
The other direction (all other points are not stationary) is implied by (the proof of) theorem $3.4$ in  \cite{bai2018subgradient}.
\end{proof}

==> sec/Image_exp.tex <==
\section{Image deblur experiments}
We set up a ground truth inverse filter as $a^{-1} = (0.5, 1, 0.5)$, and numerically run $10$ independent experiments of finding the inverse filter by the convex problem 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}^T$ }
\EEQ
We choose an accuracy $\epsilon = 10^{-3}$ and count the number of successfully accurate recovery of $a^{-1}$ where $\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<\epsilon$. We see a consistent sharp transition of success rate from $0$ to $1$ in a narrow parameter region.
\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/phase_transition_detail.png}
\caption{The finite sample phase transition phenomenon, where $a^{-1} = (0.5, 1, 0.5)$,  $x-$axis is the sparsity level $p$, $y-$axis is the empirical probability $P(\|w^\star -a^{-1}\|_1/\|a^{-1}\|_\infty<10^{-3})$. Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}

==> sec/Inequality.tex <==
\subsection{$E{| \psi^T X| }$ for IID Bernoulli Symmetric $X$ }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ have variance $\sigma^2$,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \sigma^2 \|\psi\|_2^2.
\]
The ratio indicate the sparsity level of random variable $ \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\sigma^2 \|\psi\|_2} 
\]
Now, we consider $E{|\sum_{i} \psi_i X_i| }$ for general symmetric setting when lower bound can be derived.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i Z_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $Z_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
\E_X{|\sum_{i} \psi_i X_i| }  
= \E_B \E_G {|\sum_{i} \psi_i B_i G_i| }
= \E_I \E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
\E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]


\paragraph{Symmetric distribution}

Dave Comment:
Put the generalization in the end.
Focus on Bernoulli Gaussian for the main part, and then talk about extension.


% \paragraph{General symmetric distribution case}
\begin{lemma} \label{lem:sym_Khintchine_inequality}
For we only know $\Xi_i$ are IID sampled from a symmetric distribution $F$ with unit variance, then we already have a lower bound,  
\[
     1/\sqrt{2}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
\] 
\end{lemma}
 \begin{proof}[Proof of Lemma \ref{lem:sym_Khintchine_inequality}]
 The upper bound come from Cauchy inequality.
 
Now we derive the lower bound. We write $\Xi_i = \sigma_i |\Xi_i|$, where $s_i =\pm 1$ with equal probability since $\Xi_i$ are symmetric RV, and $\{s_i,|\Xi_i|\}$  are all independent random variables.  
we could use Khintchine inequality,
here is the Wiki link for more detail:
\begin{quote}
\href{https://en.wikipedia.org/wiki/Khintchine_inequality}{Khintchine inequality}.
\end{quote}




\begin{eqnarray*}
\E_\Xi |\sum_i a_i \Xi_i| &=& E_{|\Xi_i|}E_{s_i} |\sum_i a_i s_i |\Xi_i||\\
&\geq&  
  1/\sqrt{2}  \sum_i a_i^2  E_{|\Xi_i|} |\Xi_i|^2 \\
  &=&   1/\sqrt{2}  \|a\|_2^2.
\end{eqnarray*}
\end{proof}

Let $\psi_I = a$, we have a corollary for Bernoulli Symmetric case,
   \[
 \E_I \|\psi_I\|_2  \geq \E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]


\begin{theorem}
Let $X_i = B_i \Xi_i$ be IID, where $B_i$ is sampled from Bernoulli with parameter $p$, let $I$ be the support where $B_i =1$. And $\Xi_i$ is variance $1$, sampled from: 
\begin{itemize}
    \item $N(0,1)$
    % \item sub-Gaussian with sub-Gaussian norm $K = \|Z\|_{\Psi_2}$
\item general symmetric distribution with variance $1$.
\end{itemize}
% Here sub-Gaussian norm is defined as
% $
% \|X\|_{\Psi_2} := \sup_{r\geq 1} r^{-1/2}  (E|X|^r)^{1/r}.
% $

Then 
\begin{itemize}
    \item(for Bernoulli Gaussian:)
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot \E_I \|\psi_I\|_2
\]
%     \item (for Bernoulli sub-Gaussian:) 
%      \[
% \E_X{|\sum_{i} \psi_i X_i| }  
% \geq  3^{-3/2}C^{-3} K^{-3}  \cdot (1-(1-p)^{\|\psi\|_0})^{1/2}   \cdot  \|\psi\|_2.
% \]
\item (for Bernoulli symmetric R.V. :) 
    \[
\E_X{|\sum_{i} \psi_i X_i| }  
\geq \sqrt{\frac{1}{2}} \cdot \E_I \|\psi_I\|_2.
\]
\end{itemize}

\end{theorem}




% \paragraph{Sub-Gaussian case}
% For a sub-Gaussian random variable $\Xi$ with unit variance and symmetric c.d.f $F$, we define 
% \[
% K = \|\Xi\|_{\Psi_2} = \sup_{r\geq 1} r^{-1/2}  (E|\Xi|^r)^{1/r}
% \]
% as the sub-gaussian norm of $X$
% \begin{lemma} \label{lem:Khintchine}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then for all $r \geq 2$,
% \[
% \|\psi\|_2 \leq (E(Z)^p)^{1/p} \leq C K p^{1/2} \|\psi\|_2
% \]
% where $C$ is absolute constant.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% The lower bound follows by independence and Holder’s inequality.
% For the upper bound, since we have 
% \[
% \|\sum_i a_i X_i\|_{\Psi_2}^2\leq C\sum_i a_i^2 \| X_i\|_{\Psi_2}^2\leq C\|\psi\|_2^2 K^2,
% \]
% And $Z = \sum_i a_i X_i$ is sub-Gaussian, so for all $p\geq 2$,
% \[
%  (E(Z)^p)^{1/p} \leq \|Z\|_{\Psi_2} p^{1/2} \leq C^{1/2} p^{1/2}\|\psi\|_2 K 
% \]
% \end{proof}
% \begin{lemma} \label{lem:Khintchine for $p=1$}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then
% \[
%      3^{-3/2}C^{-3} K^{-3}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
% \] 
% \[
%      3^{-3/2}C^{-3} K^{-3}  \|\psi\|_2 \leq E |\sum_i a_i X_i| \leq \|\psi\|_2
% \]
% where $C$ is absolute constant, $K = \|X\|_{\Psi_2}$.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% We use the extrapolation trick. 
% Let $Z=\sum_i a_i X_i$, since we have 
% \[ (E(Z)^2){1/2} \leq (E|Z|)^{1/4}((E(Z)^3)^{1/3})^{3/4},\]
% we get 
% \[E|Z|\geq (E(Z)^2)^{2}/ (E(Z)^3).\]

% We get a bound on 
% \[
% \|\psi\|_2 \leq (E(Z)^r)^{1/r} \leq C K p^{1/2} \|\psi\|_2
% \]
% from Khinthine’s inequality for $r = 3$.
% \end{proof}




==> sec/Intro_backup.tex <==

%   \paragraph{Spikiness of a vector up to scaling and shift}


% First, for any vector $z$, 
% \BIT
% \item
% we define $i_m(z) = \arg\max_{i\in \integers} |z_i|$ ( if there are multiple index that achieves the maximum value, then we make an convention to choose the smallest index);
% \item
% we define the operator $'$ and $P_m$ that project a vector outside of its maximum direction :
% \[
% z' = P_m(z):=  z - z_{i_m(z)} e_{i_m(z)}
% \]
% as the vector projected to be orthogonal to $e_{i_m(z)}$.
% \EIT
% \item
% we define the operator  $v_m$ that project and normalize a vector outside of its maximum direction:
% \[
% v_m(z):=  \frac{P_m(z)}{\|z\|_\infty} =  \frac{z}{z_{i_m(z)}} - e_{i_m(z)}
% \]
% as the vector projected to be orthogonal to $e_{i_m(z)}$.
% \EIT

% Now we define two measure of \textbf{spikiness} of $z$ that is invariant up to scaling and shift:
% \[
% \textbf{spk}_{\infty,\infty}(z) :=  \frac{\|z'\|_{\ell_\infty(\cT)} }{\|z\|_{\ell_\infty(\cT)}} =  \frac{|z|_{(2)} }{|z|_{(1)}
% \]

% \[
% \textbf{spk}_{2,\infty}(z) :=  \frac{\|z'\|_{\ell_2(\cT)} }{\|z\|_{\ell_\infty(\cT)}} = \inf_{i\in \integers} \tan(\angle( z , e_i)) = \tan(\angle( z , e_{i_m(z)})) 
% \]

%   \paragraph{A measure of closeness between $\widetilde{a}$ and $a$ by Spikiness of $\widetilde{a}*a^{-1}$}
% Then we could define change variables on $\widetilde{a}*a^{-1}$:
% \BIT
% \item
% $u= \widetilde{a}*a^{-1}/\|\widetilde{a}*a^{-1}\|_2$;
% \item
% $v = (\widetilde{a}*a^{-1})'/\|(\widetilde{a}*a^{-1}) \|_\infty $
% \EIT

% We define the closeness between $\widetilde{a}$ and $a$ that is invariant up to scaling and shift as the spikiness of $\widetilde{a}*a^{-1}$.

% \[
% d_\cT(\widetilde{a}, a) := \textbf{spk}_\cT (z) = \frac{\|\widetilde{a}*a^{-1}\|_{\ell_2(\cT-\{0\})}}{\|\widetilde{a}*a^{-1}\|_{\ell_\infty(\cT)}}
% \]

% Furthermore, we could define a expected closeness for a random support $I$:
% \[
%  \E_I d_I(\widetilde{a}, a) := \E_I \textbf{spk}_I(\widetilde{a}*a^{-1}) = \frac{\E_I\|\widetilde{a}*a^{-1}\|_{\ell_2(I-\{0\})}}{\|\widetilde{a}*a^{-1}\|_{\ell_\infty(\cT)}}
% \]

% When $\widetilde{a} =a$, $\widetilde{a}*a^{-1} = e_0$, then 
% $\|\widetilde{a}*a^{-1}\|_{\ell_2(\cT-\{0\})}= \|e_0\|_{\ell_2(\cT-\{0\})}=0$.
% The $\ell_\infty$ norm normalization makes $d_\cT(\widetilde{a}, a)$ and $ \E_I d_I(\widetilde{a}, a)$ scale invariant.



% It is worth pointing out that this closeness measure is not a distance as it is not symmetric between $\widetilde{a}$ and $a$.



==> sec/Inverse.tex <==

\section{Analysis of the inverse kernel method}
\subsection{Inverse kernel approximation}
Now we consider a setting where there is a kernel whose corresponding the inverse kernel is infinite, and we give a finite length approximation. 
We assume that $a =  (a_{-t},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t) = \delta_0 + a_L + a_R$ 
is a length $ l= 2t+1$ filter, 
  and $\sum_{i\neq 0} |a_i|\leq M < 1$.    
 \begin{theorem} 
For a kernel $a = (a_{-s},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_t)$ of length $l=1+s+t$, if 
\[
\sum_{i\neq 0} |a_i|\leq M < 1,
\]
 then there exists an approximate inverse kernel $w^r$ of length $rl$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M),\\
\end{array}
  \]
\end{theorem}
\begin{proof}
Consider the $z$ transform of $a$ to be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
let $\bar A(z) = 1-A(z)$, then 
from the condition 
$\sum_{i\neq 0} |a_i|\leq M < 1$,
we define $M' $ to be the maximum absolute value of $\bar A(z)$ on unit circle, as
\[
 \begin{array}{ll}
\mbox{maximize}   & |\bar A(z)| \\
\mbox{subject to}  & z\in \complex,|z|=1.
\end{array}
  \]
Then 
\[
 \begin{array}{ll}
M' \leq \sum_{i\neq 0} |a_i|\leq M<1.
\end{array}
  \]
The Z-transform of the inverse kernel of $a$ is defined by
\[
 \begin{array}{ll}
1/A(z) &=  (1-\bar A(z))^{-1},\\
&= 1+ \sum_{i=1}^{\infty} (\bar A(z))^i
\end{array}
  \]
 The infinite series absolutely converge on $|z| = 1$ because $|\bar A(z)|\leq M<1$.
Let the finite approximation of level $r$ of $w = a^{-1}$ be $w^r$, 
 its Z-transform is  $\sum_{i=0}^{r} (\bar A(z))^i$,
its length is at most $r(s+t+1)$, 
the $j$-th term of $w^r$ is $\sum_{b}bj_i=j \prod_{i} a_i^{j_i}$.
We have that for all  $|z| = 1$,
 \[
 \begin{array}{ll}
|1/A(z) - \sum_{i=0}^{r} (\bar A(z))^i | 
&= |\sum_{i=r+1}^{\infty} (\bar A(z))^i|\\
&\leq M^{r+1}/(1-M).
\end{array}
  \]
Therefore, 
   \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]
%   \[
%  \begin{array}{ll}
% \|a*w^r - e_0 \|_{1} &= \|a*(w^r - w) \|_{1}\\
% &\leq \|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} \\
% &\leq M^{r+1}/(1-M) \\
% &= M^{r+1}(1+M)/(1-M)
% \end{array}
%   \]
 
\end{proof}

Using this inverse approximation, we know for any kernel $a$ of length $l$ with possibly infinite inverse kernel $w$, there exists a length-$rl$ approximate inverse kernel $w^r$, such that 
  \[
 \begin{array}{ll}
\|\mathcal{F}w-\mathcal{F}w^r \|_{\infty} 
&\leq M^{r+1}/(1-M).
\end{array}
  \]

Therefore, we can prove the following theorem on sparse blind deconvolution algorithm. 


\paragraph{Simple example.}
We consider a simple example, when $a = (0,\ldots, 0, 1, r, 0, \ldots, 0) = \delta_0 - r\delta_1$, $|r|<1$. Then $a^{-1} = \delta_0 + \sum_{j=1}^\infty  r^j \delta_j.$ Now our data generation model is $y = a*x.$ 

We analysis the optimization problem 
 \begin{eqnarray*}
    \min_{f_0 = 0} &    
    E_x\| (\delta_0+f)*a*x\|_1.
\end{eqnarray*}
Here $f = (0, 0, f_R)$ is in a $K$ dimensional subspace of the double infinite sequence.

% We also analysis the constrained optimization problem 
%  \begin{eqnarray*}
%     \min_{f_0 = 0} &    
%     E_x\| (\delta_0+f)*a*x\|_1,
%     \\
%     \mbox{ subject to }&  \|f\|_1\leq C.
% \end{eqnarray*}

For the objective, using IID property of $x$, we only need to analyze
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| .
\end{eqnarray*}
Let $f^*_K$ be the best length $K$ approximation, as the solution of 
\begin{eqnarray*}
    \min_{f_0 = 0} &    
    \| (\delta_0+f)*a\|_2,
\end{eqnarray*}

In this specific example, $f^*_K = \sum_{j=1}^K  r^j \delta_j.$ And $(\delta_0+f^*_K)*a = (\delta_0 - r^{K+1}\delta_{K+1})*(\delta_0 - r^{1}\delta_{1})^{-1}$.
Let $\tilde{x} = (\delta_0 - r^{K+1}\delta_{K+1})*x$, as one approximation of $x$.
Since $x$ is IID symmetric, $ \tilde{x}$ is identically-distributed, symmetric and weakly correlated for $|r^{K+1}|$ small enough, and $\tilde{x}_0, \ldots, \tilde{x}_K$ are independent.

Let 
\begin{eqnarray*} 
\delta_0+h &=& (\delta_0+f)*(\delta_0+f^*_K)^{-1}\\
&=& (\delta_0+f)*(\delta_0 - r^{K+1}\delta_{K+1})
\end{eqnarray*}
then 
 \begin{eqnarray*} 
    E_x | ((\delta_0+f)*(\delta_0 - r\delta_1)*x)_0| 
    &=& E_x | ((\delta_0+h)*\tilde{x})_0|\\
&=& E_x | \tilde{x}_0|+\mbox{sign}(\tilde{x}_0)(h*\tilde{x})_0\\
&\approx& 
 |1+  h_{0}| \cdot E |\tilde{x}_0| \cdot (1-\eta)+   \cdot  E{| (h*\tilde{x})_0| } \cdot \eta.
\end{eqnarray*}

Following the same analysis as the phase transition analysis, we have
\begin{eqnarray*}
     \min_\delta &E | ((\delta_0+f)*a*\tilde{x})_0 | \\
    \mbox{ subject to }  &f_{0} = 0.
\end{eqnarray*}


==> sec/Metric.tex <==
 \subsection{Distance metrics}
% \paragraph{Distances to measure stability}
We care about three types of metrics, first, distance  in $w$ space, between the computed composed filter $w$ and ground truth $a^{-1}$; second, distance in $w$ space, between the computed inverse filter $w$ and ground truth inverse filter $a^{-1}$, second, distance  in $\psi = w*a$ space, between the computed composed filter $w*a$ and ground truth $e_0$; third,  distance  in $x$ space, between recovered signal sequence and true sparse signal sequence. 

First, the MSE in space of $\psi = w*a$,
  \[
 \begin{array}{ll}
d_{\psi,2}^2 := \|\phi\|_2^2 =  \|\psi-e_0\|_2^2= \|a*(w-a^{-1})\|_2^2
\end{array}
  \] 
 The MSE in space of $w$. 
   \[
 \begin{array}{ll}
d_{w,2}^2  = \|w-a^{-1}\|_2^2 = \|a^{-1}*(\psi-e_0))\|_2^2 = \|a^{-1}*\phi\|_2^2
\end{array}
  \]
Last, $\ell_1$ and $\ell_2$ distance in $x$ space:
\[
 \begin{array}{ll}
d_{x,1} &:= \frac{1}{2T+1}\|w*Y-X\|_{1,[-T,T]} =  \frac{1}{2T+1}\|\tilde \phi* X\|_{1,[-T,T]} \\
d_{x,2}^2 &:= \frac{1}{2T+1}\|w*Y-X\|_{2,[-T,T]}^2 = \frac{1}{2T+1}\|\tilde \phi* X\|_{2,[-T,T]}^2
\end{array}
  \]
We compute their expectation: 
\[
 \begin{array}{ll}
\Expect d_{x,1}  &=  \Expect|\phi^T X| = \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2\\
\Expect d_{x,2}^2 &=  \Expect|\phi^T X|^2 = p \|\phi\|^2  = p \|\psi-e_0\|^2 
\end{array}
  \]  
We remark that in the following we focus on distance in $x$ space to recover the signal. 

% And using the fact that $\Expect d_{x,1}= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|\phi \cdot I\|_2$ and $\Expect d_{x,2}^2 = p \|\phi\|^2$, we focus on calculate 
% \BIT
% \item $\Expect d_{x,1} \propto  \Expect_I \|\phi \cdot I\|_2$
% \item $\Expect d_{x,2}^2 = \Expect_I \|\phi \cdot I\|_2^2 = p\|\phi\|^2  = p d_{\psi,2}^2$ 
% \EIT



==> sec/Noise.tex <==
\section{Stability for noisy observation}


\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]
\subsection{Stability for adversarial perturbation of sparse signal }
\paragraph{Mathematical formulation: sparse signal plus adversarial perturbation}

\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
$Z$ is a unit vector in $2$ sphere. 
\item
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
\Expect|(w*Y)_0|
&= \Expect|\psi^T (X+\eta Z )| \\
% &= \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
\end{array}
  \]

  
  
  
 \paragraph{Study the noisy problem}
Under the data generative model, 
\[
\begin{array}{ll}
Y&= a* (X+\eta Z ) 
\end{array}
\]
    the constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta}   & \Expect|\psi^T (X+\eta Z ) - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
  
\paragraph{Worst case objective over $Z$}  
For the constrained problem, we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi,\zeta} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1,\\
& \zeta^2 \leq 1
\end{array}
  \]
Which is equivalent to 
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
In the following we study the min-max objective
  \[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi) : = \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta  \psi^T Z  - \epsilon \zeta| 
\end{array}
  \]
  
\paragraph{Robust optimization}
Let the deterministic residual function of $\psi, Z, \zeta$ be
\[
\mu_{\eta, \epsilon}(\psi, Z, \zeta): = \eta  \psi^T Z  - \epsilon \zeta
\]
We reparametrize $\epsilon$ as by defining 
\[
\tau :=  \frac{\epsilon}{\eta}
\]
then 
\[
\mu_{\eta, \epsilon} = \eta ( \psi^T Z  - \tau \zeta)
\]






\begin{lemma}
For any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, $Z$ is along the direction of $s\psi$ so that $s\psi^T Z = \|\psi\|_2$.

\end{lemma}  


\begin{lemma}[Hölder's inequality]
For any given sign $s =\pm 1$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(s \psi^T Z) = \|\psi\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $s|\psi|^q$ so that $s\psi^T Z = \|\psi\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
The min-max quantity  
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2 = (\eta \|\psi\|_2  - \epsilon )_+^2 = \eta^2 ( \|\psi\|_2  - \tau )_+^2
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}^2 
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} (\eta  \psi^T Z  - \epsilon \zeta)^2\\
&=\inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} [(\eta  \psi^T Z)^2+  (\epsilon \zeta)^2 - 2(\eta  \psi^T Z)(\epsilon \zeta)]\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \sup_{Z: \|Z\|_2\leq 1} [ (\psi^T Z)^2] + 2\eta \epsilon |\zeta|   \sup_{Z: \|Z\|_2\leq 1}[ (-\sign(\zeta) \psi^T Z)]\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{   \epsilon^2( \zeta)^2+ \eta^2 \|\psi\|_2^2 + 2\eta \epsilon |\zeta|   \|\psi\|_2\}\\
&=\inf_{\zeta: \zeta^2 \leq 1}\{  (\eta \|\psi\|_2  - \epsilon |\zeta| )^2\}\\
&= (\eta \|\psi\|_2  - \epsilon )_+^2
\end{array}
\]
The fourth equation is because for any given sign $s =\pm 1$,
\[
\sup_{Z: \|Z\|_2\leq 1}(s \psi^T Z) = \|\psi\|_2.
\]
\[
\sup_{Z: \|Z\|_2\leq 1}( \psi^T Z)^2 = \|\psi\|_2^2.
\]



\end{proof}

We have the following result, generalizing $\|Z\|_2\leq 1$ to $\|Z\|_p\leq 1, \quad, p\geq 1$, and then to $Z\in K$ for a closed compact convex set $K\in \reals^N$.



\begin{lemma}
\label{min-maxErrorL_p}
The min-max quantity 
for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates,
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_p\leq 1} F( \eta (\psi^T Z  - \tau \zeta)) = 
F(\eta( \|\psi\|_q  - \tau )_+)
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}

\begin{coro}
 \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_2  - \tau )_+|
\end{array}
  \]
  in general, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_p\leq 1}  &  \Expect|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|\psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}


\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then for any constant $\mu$, using the rotation invariance of Gaussian, $\psi^T X +\mu$ is  Gaussian with mean $\mu$ and standard deviation $\|\psi_I\|_2$, therefore,
\[
|\psi^T X +\mu |
\]
following the folded Gaussian distribution.
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}

From general theory of folded Gaussian $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
hence
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
\end{array}
\]

\end{lemma}
\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}







==> sec/Noise2.tex <==

% \paragraph{Bound on min-max objective}

% First of all, we find a lower and upper bound that is true independent of the distribution of $X$.
% \begin{lemma}
% Let $\psi^T X $ be fixed, we have upper and lower bound on the constrained problem objective:
%  \[
%  \begin{array}{ll}
% \sup_{s=\pm 1}|(\psi^T X +s\eta \|\psi\|_2  - \epsilon)_+| \leq
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} |\psi^T X +\eta  \psi^T Z  - \epsilon \zeta| 
% \leq |\psi^T X | +|(\eta \|\psi\|_2  - \epsilon)_+ |
% \end{array}
%   \] 
% \end{lemma}  
% \begin{proof}
% Let $A:=\psi^T X $ be fixed
% First, if we let $Z$ be along the direction of $s\psi$, we have a lower bound on the objective for both $s =\pm 1$,
%   \[
%  \begin{array}{ll}
%   \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| 
% \geq
%  |A +\eta s\|\psi\|_2  - \epsilon \zeta|
% \end{array}
%   \] 
%   Therefore, we can 
%   \[
%  \begin{array}{ll}
%  &\inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \geq&
% \inf_{\zeta: \zeta^2 \leq 1} |A +\eta s\|\psi\|_2  - \epsilon \zeta|\\
% =&
%  |(A +s\eta \|\psi\|_2  - \epsilon)_+|
% \end{array}
%   \] 
% Second, if we let $ \sign(\eta  \psi^T Z  - \epsilon \zeta) = s'$ then
%   \[
%  \begin{array}{ll}
%  & \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1}  |A +\eta  \psi^T Z  - \epsilon \zeta| \\
% \leq&
% \inf_{\zeta: \zeta^2 \leq 1}  \sup_{Z: \|Z\|_2\leq 1}   (|A |+ |\eta  \psi^T Z  - \epsilon \zeta|) \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\sup_{Z: \|Z\|_2\leq 1} |\eta  \psi^T Z  - \epsilon \zeta| \\
%  =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\sup_{Z: \|Z\|_2\leq 1} [\eta  s'\psi^T Z]  -s' \epsilon \zeta\} \\
%     =&
%     |A |+ \inf_{\zeta: \zeta^2 \leq 1}\{\eta \|\psi\|_2  -s' \epsilon \zeta\} \\
%   =&
%   |A | +|(\eta \|\psi\|_2  - \epsilon)_+ |\\
% \end{array}
%   \] 
  
% \end{proof}
\paragraph{Folded Gaussian mean and asymptotically tight lower bound}
Now we exploit the property of folded Gaussian mean, and we find an exact asymptotic formula.
For simplicity of expression, we also define the deterministic residual function of $\psi, I$ to be
\[
\gamma_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \mu_{\eta, \epsilon}(\psi, Z, \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\psi\|_2 - \tau)_+}{\|\psi_I\|_2}
\]

\begin{coro}
\label{Cor:PerturbedObjectiveLowerBound}
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)
&= \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| \\
&= \sqrt{\frac{2}{\pi}}  \Expect_I \left[ \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I \left[\|\psi_I\|_2(1 + \frac{3}{2}\gamma_{\eta, \epsilon}^2 + \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma_{\eta, \epsilon}^6)\right]
\end{array}
\]
As $\gamma_{\eta, \epsilon}^2<1,$ 
\[
 \begin{array}{ll}
L_{\eta, \epsilon}(\psi)-L_{0, 0}(\psi)
&\geq 3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}(\psi)^2\Expect_I \|\psi_I\|_2^{-1}
\end{array}
\]
\end{coro}
% \begin{proof}
% In the following proof, for clarity, we write $\gamma_{\eta, \epsilon}$ simply as $\gamma$.

% Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
% we have
% \beq
% \label{FoldedGaussianMean_Obj}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| = \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \mu_{\eta, \epsilon} \left(1 - 2\Phi\left(-\gamma_{\eta, \epsilon}\right) \right)\right]
% \eeq
% Then we can plug in the lemma \ref{ExpansionMeanFoldedGaussian}.
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \exp\{-\gamma_{\eta, \epsilon}^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \Expect_I \left[ \sqrt{\frac{2}{\pi}} \|\psi_I\|_2 \{ 1- \frac{\gamma_{\eta, \epsilon}^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu_{\eta, \epsilon}^2 \frac{1}{\|\psi_I\|_2} C_\Phi(\gamma^2_{\eta, \epsilon})\right]\\
% &= \sqrt{\frac{2}{\pi}}\Expect_I  \left[ \|\psi_I\|_2 
% \{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2_{\eta, \epsilon}))\gamma_{\eta, \epsilon}^2 +   \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!}\} \}\right]\\
% \end{array}
% \] 
% Here the residual of this expansion after first order is
% \[
%  \begin{array}{ll}
% \mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2_{\eta, \epsilon})-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma_{\eta, \epsilon}^{2n}}{(-2)^n (n)!} \\
% &=    \frac{1}{24} \gamma_{\eta, \epsilon}^4   + O(\gamma^6)
% \end{array}
% \] 
% From the lower bound in lemma \ref{ExpansionMeanFoldedGaussian}, we have that when $\gamma_{\eta, \epsilon}^2<1, \mbox{Res}(\gamma^2)\geq 0$
% \[
%  \begin{array}{ll}
% \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}\mu_{\eta, \epsilon}^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \] 
% Now we could plug in lemma~\ref{min-maxError} to prove the last equation.
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \Expect|\psi^T X+\mu_{\eta, \epsilon}| 
% &\geq \sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right]
% \end{array}
% \]
% \end{proof}









% We branch out to show a low-hanging result for the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem}.
% \begin{coro}
% For
% the  \textbf{adversarial perturbed sphere constrained non-convex  projection pursuit (orthogonal dictionary learning) problem} with min-max lower bound as objective
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 + \frac{3}{2}(\eta \|\psi\|_2  - \epsilon )_+^2\Expect_I \|\psi_I\|_2^{-1}\right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]
%  If $\epsilon \geq \eta,$ then the minimizer is $1$-sparse vector $e_i$, the same as the minimizer of 
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
% \mbox{subject to}  
% &\|\psi\|_2^2 =1
% \end{array}
%   \]

% \end{coro}


  \paragraph{Calculate the robust objective at $e_0$}
First, at $\psi = e_0$, $X_0 =e_0^T X = I_0 G_0$, where $G_0$ is standard normal, $I_0$ is Bernoulli, we take expectation over $I_0$ first, 
Let 
 \[
 \mu_0 :=  \mu_{\eta, \epsilon}(e_0) = \eta ( 1-\tau)_+ 
 \]
 When $\epsilon\geq \eta,$ $\mu_0=0$; when $\epsilon< \eta,$ $\mu_0>0$.
 \begin{lemma}
  \label{Lemma:ObjectiveDiffAtEzero}
     \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
 \end{lemma}
%   \begin{lemma}
%   \label{Lemma:ObjectiveRatioAtEzero}
%      \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &=  [(1-p)\mu_0\sqrt{\frac{\pi}{2}}  + p  (e^{-\frac{\mu_0 ^2}{2}} )+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)]/p
% \end{array}
%   \] 
%  \end{lemma}
 
 \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveDiffAtEzero}]
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
&= \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z\|_2\leq 1}\Expect |X_0+\eta   Z_0  - \epsilon \zeta|-\Expect | X_0| \\
&= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|-\Expect | X_0| \\
&=  (1-p)\mu_0  + p\sqrt{\frac{2}{\pi}}  (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
&= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
\end{array}
  \] 
The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
 \end{proof}
%   \begin{proof}[Proof of lemma~\ref{Lemma:ObjectiveRatioAtEzero}]
%   Using lemma~\ref{ExpansionMeanFoldedGaussian}, let $\gamma = \eta ( \|e_0\|_2-\tau)_+/B_0,a$
%     \[
%  \begin{array}{ll}
% L_{\eta, \epsilon}(e_0)/L_{0, 0}(e_0)
% &= \Expect |X_0+\eta ( \|e_0\|_2-\tau)_+|/\Expect | X_0|\\

% % \Expect_I |(e_0)_I+\eta ( \|e_0\|_2-\tau)_+|/\Expect_I | (e_0)_I| 
% % &=  \sqrt{{\pi}\frac{2}} (1-p)\mu_0  + p (e^{-\frac{\mu_0 ^2}{2}} -1)+ \mu_0 \left(1 - 2\Phi\left(-\mu_0\right) \right)\\
% % &= (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4)
% \end{array}
%   \] 
% The last approximation come from Taylor expansion in lemma~\ref{ExpansionMeanFoldedGaussian}.
  
%  \end{proof}
 
 
We observe that 
\BIT
\item
if $\tau\geq 1$,   $( 1-\tau)_+ = 0$, then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) = 0;$
\item
if $\tau < 1$ , then $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0) \approx (1-p)\mu_0  + p O(\mu_0^2).$
\EIT

  
  \paragraph{Bound $\|\phi^\star\|_2$ using the difference of objective }
   Now use the change of variable that $\psi =e_0+\phi$,
   the constrained problem becomes
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & L_{\eta, \epsilon}(e_0+\phi) \\
\mbox{subject to}  
&u^T \phi =0
\end{array}
  \] 
First, we assume the minimizer is $\phi^\star$. Since $e_0$ is  minimizer of $L_{0, 0}$ and $e_0+ \phi^\star$ is  minimizer of $L_{\eta, \epsilon}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star) 
 \geq L_{0, 0}(e_0+\phi^\star)
 \geq L_{0, 0}(e_0) 
\end{array}
  \] 

Remark: This chain is true for all  $\phi^\star$ that $L_{\eta, \epsilon}(e_0)
 \geq L_{\eta, \epsilon}(e_0+\phi^\star),$ we can pick a dense sequence converging to $\phi^\star$ in $\ell_2$ norm)  
  
 Then using the fact that $L_{\eta, \epsilon}(e_0) -L_{\eta, \epsilon}(e_0+\phi^\star) \geq 0,$ we have
    \[
 \begin{array}{ll}
L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)
 \geq   [L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)]+ 
 [L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) ]
\end{array}
  \]   
  
 Notice that 
      \[
 \begin{array}{ll}
 L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)  = \Expect |(e_0+\phi^\star)^T X| - \Expect |(e_0)^T X| 
 = \sqrt{\frac{2}{\pi}} B(p,N)  \|\phi^\star\|_2
\end{array}
  \] 
  where $N = \|\phi^\star\|_0$, since $\phi^\star$ is dense due to our assumption, we have .
    \[
  \lim_{N \rightarrow \infty } B(p,N) = B(p,\infty) =  [ p (-\cot{\theta}) + (1-p)].
  \]
  if $p<p^\star$, $\lim_{N \rightarrow \infty } B(p,N) > 0.$
 
\begin{theorem}


\label{Thm:StabilityMSE}
When $\epsilon\geq \eta,$ and $p<p^\star$, then
$\|\phi^\star\|_2 =0$, the minimizer of the min-max problem is exactly $\psi^\star = e_0.$
 
 When $\epsilon< \eta,$  and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B(p,\infty)\right) \|\phi^\star\|_2 
 &\leq& 
 \left(L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)\right)-\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)\\
  &\leq&  \left(  (1-p)\mu_0  +  3\sqrt{\frac{1}{2\pi}} p \mu_0 ^2 + O(\mu_0 ^4) \right) - 
  \left(  3\sqrt{\frac{1}{2\pi}} \mu_{\eta, \epsilon}((e_0+\phi^\star))^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} \right)\\
    &\leq& 
    (1-p)\mu_0  +  
    3\sqrt{\frac{1}{2\pi}}\left(  p \mu_0 ^2- \mu_{\eta, \epsilon}((e_0+\phi^\star))^2 \|e_0+\phi^\star\|_2^{-1} \right) + O(\mu_0 ^4)
 \EEAS
\end{theorem}
\begin{proof}
The first inequality comes from the chain of inequality between objectives. 

The second inequality combines the previous calculation of $L_{0, 0}(e_0+\phi^\star) - L_{0, 0}(e_0)$ with lemma~\ref{ExpansionMeanFoldedGaussian} and lemma~\ref{Lemma:ObjectiveDiffAtEzero}.

For the last inequality comes from lemma~\ref{TaylorSqrtInvExpect}, 
\[
\frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}} \geq 1 .
\]
\end{proof}

\paragraph{Interpretation}
For simplicity, we focus on the case when the optimization problem is the original one where $\epsilon = 0$,
then 
\[
 \mu_{\eta, 0}(e_0) = \eta.
\]
\BIT
\item
We comment that when our optimization constraint is sphere constraint $\|\psi\|_2 =1$, 
then
\[
 \mu_{\eta, 0}(\psi)  = \eta
\]
then
 \BEAS
 \left(\sqrt{\frac{2}{\pi}} B_s(p,\infty)\right) \|\phi^\star\|_2 
    &\leq& 
    (1-p)
    [\eta  - 
    3\sqrt{\frac{1}{2\pi}} \eta^2] + O(\eta^4)
 \EEAS

\item
For the case when our optimization constraint is $u^T \phi =0$, 
\[
 \|e_0+\phi^\star\|_2^2= 1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 
 \]
 Since it is dependent on $\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2$, and using the condition $u^T \phi^\star =0$, we could use the same argument as figure~\ref{fig-Angle} and lemma~\ref{Angle_Inequality}, we know that 
 \[
 |\cos{\angle(\phi^\star,e_0)}| \leq \sin\theta
 \]
 therefore,
 \[
 |\frac{\|e_0+\phi^\star\|_2^2 - (1+\|\phi^\star \|_2^2)}{\|\phi^\star \|_2 }| \leq 2\sin\theta
 \]
 \EIT
 
We first have a weak corollary by only using $L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0)$ and just use loose bound $L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\geq 0.$


\begin{coro}
\label{Cor:StabilityMSE_}
 When $\epsilon< \eta,$ and $p<p^\star$,  $\|\phi^\star\|_2$  is bounded by a function of $\mu_0$:
 \BEAS
 \|\phi^\star\|_2 &\leq& (L_{\eta, \epsilon}(e_0) -L_{0, 0}(e_0))/(\sqrt{\frac{2}{\pi}} B(p,\infty))\\
 &\approx& 
 \eta \{\sqrt{\frac{\pi}{2}}(1-p) +  \frac{3p}{2}\eta \}/  
 \{ p (-\cot{\theta}) + (1-p)\}+ O(\eta^4)
 \EEAS
\end{coro}  

  To strengthen this bound, we further compute 
$L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star) $.

  
\begin{coro}
 When $\epsilon =0,$ and $p<p^\star$, as $\eta\rightarrow 0$, $\|\phi^\star\|_2$  is bounded by a function of $\eta$:
  \BEAS
\|\phi^\star\|_2 
 &\leq& 
 \frac{    (1-p)\{\sqrt{\frac{\pi}{2}}\eta -  \frac{3}{2}\eta^2 )}{   p (-\cot{\theta}) + (1-p) + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} } + O(\eta^4)
 \EEAS 
\end{coro}    
\begin{proof}
Let 
\[
\Gamma_{-1}(e_0+\phi^\star) := \frac{\E_I  \|(e_0+\phi^\star)_I\|_2^{-1} }{\|e_0+\phi^\star\|_2^{-1}}
\]
From lemma~\ref{TaylorSqrtInvExpect}, we have 
\[
\Gamma_{-1} \geq 1 .
\]
we have
  \[
 \begin{array}{ll}
\sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1} 
&= \sqrt{\frac{2}{\pi}}\frac{3}{2} \eta^2  \|(e_0+\phi^\star)\|_2
\Gamma_{-1}(e_0+\phi^\star)
\end{array}
  \] 
Now we use Taylor expansion,  we could expand $\|\phi^\star \|_2$ around $0$ to first order 
\[
 \begin{array}{ll}
 \|(e_0+\phi^\star)\|_2
&=  (1+\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{\frac{1}{2}}\\
&= 1+\sum_{\ell=1}^\infty \binom{\frac{1}{2}}{\ell}
[\|\phi^\star \|_2^2 + 2\cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)\\
&= 1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\|\phi^\star \|_2^2)
\end{array}
  \] 
  
 
  
  \BEAS
- \sqrt{\frac{\pi}{2}}\left(L_{\eta, \epsilon}(e_0+\phi^\star)  - L_{0, 0}(e_0+\phi^\star)\right)
 &\leq& 
 - \frac{3}{2} \eta^2 \Gamma_{-1}(e_0+\phi^\star) (1+ \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2 + O(\eta^2))
 \EEAS 
 Therefore
  \BEAS
 \left(  [p (-\cot{\theta}) + (1-p)] + \frac{3}{2} \eta^2 \cos{\angle(\phi^\star,e_0)} \right)\|\phi^\star\|_2 
 &\leq& 
 \eta (1-p) \{\sqrt{\frac{\pi}{2}} -  \frac{3}{2}\eta )+ O(\eta^4)
 \EEAS 
% \[
%  \begin{array}{ll}
%  \|(e_0+\phi^\star)\|_2^{-1}
% &=  (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}\\
% &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \]   


  
% \[
%  \begin{array}{ll}
%  \Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}
% &=  \Expect_I(1+\|\phi^\star_I \|_2^2 + \cos{\angle(\phi^\star_I,e_0)}\|\phi^\star_I \|_2)^{-\frac{1}{2}}
% % &= 1+\sum_{\ell=1}^\infty\frac{(-1)^{\ell}}{2^{2\ell}}\binom{2\ell}{\ell}
% % [\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2]^\ell
% \end{array}
%   \] 
 
  

% Therefore,
%  \[
%  \begin{array}{ll}
 
% &  p\sqrt{\frac{2}{\pi}}\left[ \frac{3}{2}\mu_0^2\right]+(1-p)\mu_0
%  \\
% \geq& \frac{3}{2}(\eta \|(e_0+\phi^\star)\|_2  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2\Expect_I \|(e_0+\phi^\star)_I\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % \geq& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) \|e_0+\phi^\star\|_2^{-1}+ B(p) \|\phi^\star\|_2\\
% % =& \frac{3}{2}(\eta \sqrt{1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2}  - \epsilon )_+^2 \Gamma_{-1}(p) (1+\|\phi^\star \|_2^2 + \cos{\angle(\phi^\star,e_0)}\|\phi^\star \|_2)^{-\frac{1}{2}}+ B(p) \|\phi^\star\|_2\\
% \end{array}
%   \] 



\end{proof}
 













\subsection{Other setting on $Z$}
\paragraph{ Adversarial outer noise} 
If our generative model is
\[
\begin{array}{ll}
Y&= a* X + \eta_2 Z_2\\
&= a* (X +\eta_2 a^{-1}* Z_2)
\end{array}
\] 
And we consider the worst case objective over $\|Z_2\|_p\leq 1, \quad p\geq 1.$

Let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, then following previous calculation,
\begin{coro}
For $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
   \[
 \begin{array}{ll}
 \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{Z: \|Z_2\|_p \leq 1}  &  \Expect|\psi^T X+\eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)| =\Expect|\psi^T X+\eta( \|C_{a^{-1}}^T \psi\|_q  - \tau )_+|
\end{array}
  \]
\end{coro}

Let $C_{a^{-1}}^T \psi =\bar{a}^{-1}*\psi$, where $\tilde{a}^{-1}$ is defined by flipping the coordinate of $a^{-1}$ (reflecting the coordinates around zero by map $i$ to $-i$ for $i\in \integers$.)
 
 We can replace the definition of $\gamma$ and $\mu_0$  by:
 \[
 \gamma^{a}_{\eta, \epsilon}(\psi, I): = \inf_{\zeta: \zeta^2 \leq 1} \sup_{Z: \|Z\|_2\leq 1} \eta_2  (\psi^T C_a^{-1} Z  - \tau \zeta)/\|\psi_I\|_2 = \eta \frac{ (\|\bar{a}^{-1}*\psi\|_q  - \tau)_+}{\|\psi_I\|_2}
\]
\[
\mu_0^{a} := \eta( \|\tilde{a}^{-1}\|_q-\tau)_+
\]
We can get the same result as theorem~\ref{Thm:StabilityMSE}.

% \paragraph{Distributional robust setting}
% When $Z$ following a distribution $P_Z \in \Pi$, where $\Pi$ is a closed convex set in probability simplex for probability defined on $\reals^N$, then our distributional robust objective is
%   \[
%  \begin{array}{ll}
%  \inf_{\zeta: \zeta^2 \leq 1} \quad \sup_{P_Z \in \Pi}  & \Expect_Z \Expect_X|\psi^T X+\eta (\psi^T Z  - \tau \zeta)| 
% \end{array}
%   \]
% then 
% for a one-dimensional convex even function $F$ that is monotonically non-decreasing for positive coordinates, the quantity 
% \[
%  \begin{array}{ll}
%  \sup_{P_Z \in \Pi}  & \Expect_Z F( \psi^T  Z ) 
% \end{array}
% \]
% could be computed following the same approach as the distributional robust Kelly problem if $\Pi$ can be represented by finite combination of atoms.
  

  

\subsection{ Gaussian additional noise}
\paragraph{ Gaussian additional observation inner and outer noise} 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+  \sigma_1 G_1) +  \sigma_2 G_2\\
&= a* (X+\sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\] 
let $C_{a^{-1}}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, then $C_{a^{-1}} = C_a^{-1}$ and 
\[
\begin{array}{ll}
Z: = \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\sim N(0, \sigma_1^2 I_N + \sigma_2^2 C_{a^{-1}} C_{a^{-1}}^T)
\end{array}
\] 
then
\[
\begin{array}{ll}
\psi^T Z
\sim N(0, \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2 )
\end{array}
\] 
 Let $G$ be another standard normal $N(0,I_N)$, for any fixed vector $\mu \in \reals^N, $
 \[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2)  | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  |
\end{array}
  \]
In this case, it seems the previous constrained problem no longer can help us find exact solution $\psi^\star =e_0.$ 



We first study $\sigma_2 = 0$ case.
\[
\Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}G_3 | = 
\sqrt{\frac{2}{\pi}} \cdot \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) =  \sqrt{\frac{2}{\pi}} \cdot \|\psi\|_2 \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma_1^2})
\]
Define worst case objective
\[
F_{\sigma}(\psi):= \sup_{\sigma_1 \leq \sigma} \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2}) = \Expect_I(\sqrt{ \|\psi_I\|_2^2 + \sigma^2\|\psi\|_2^2})
\]
The second equality comes from monotonicity.

Again, we assume the minimizer is $\psi^\star $. Since $e_0$ is  minimizer of $L_{0}$ and $\psi^\star $ is  minimizer of $L_{\sigma}$, we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\sigma}(e_0)
 \geq F_{\sigma}(\psi^\star ) 
 \geq F_{0}(\psi^\star )
 \geq F_{0}(e_0) 
\end{array}
  \] 
Then
    \[
 \begin{array}{ll}
F_{\eta}(e_0)/F_{0}(e_0)
 \geq (F_{\eta}(\psi^\star )/F_{0}(\psi^\star ))(F_{0}(\psi^\star )/F_{0}(e_0) )
\end{array}
  \] 

   \[
 \begin{array}{ll}
 F_{\eta}(\psi)/F_{0}(\psi) = \Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )
\end{array}
  \] 
  
     \[
 \begin{array}{ll}
 F_{\eta}(e_0)/F_{0}(e_0) = \Expect_I(\sqrt{ \frac{\|(e_0)_I\|_2^2}{\|e_0\|_2^2} + \sigma^2})/\Expect_I(\frac{\|(e_0)_I\|_2}{\|e_0\|_2} )= (p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p
\end{array}
  \] 
  
    \[
 \begin{array}{ll}
 F_{0}(\psi)/F_{0}(e_0) 
 &= \Expect_I\|\psi_I\|_2/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+(\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2)/\Expect_I\|(e_0)_I\|_2 \\
 &= 1+ (B(p,N)/\Expect_I\|(e_0)_I\|_2) \|\psi -e_0\|_2\\
 &= 1+ (B(p,N)/p) \|\phi\|_2
\end{array}
  \] 

   \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi\|_2 &\leq (F_{\eta}(e_0)/F_{0}(e_0))/ (F_{\eta}(\psi)/F_{0}(\psi)) \\
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}/\{\Expect_I(\sqrt{ \frac{\|\psi_I\|_2^2}{\|\psi\|_2^2} + \sigma^2})/\Expect_I(\frac{\|\psi_I\|_2}{\|\psi\|_2} )\}
\end{array}
  \] 
  First, a loose bound on $\|\phi^\star\|_2$:
  \[
 \begin{array}{ll}
1+ (B(p,N)/p) \|\phi^\star\|_2 
&\leq \{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}
\end{array}
  \] 
We found that
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq (\{(p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})/p\}-1)/(B(p,N)/p) \\
&\leq ((p\sqrt{ 1 + \sigma^2}+ (1-p) \sqrt{ \sigma^2})-p)/B(p,N)
\end{array}
  \] 

In general, when $\sigma_1, \sigma_2$ both non-zero, using the same argument,
\[
 \begin{array}{ll}
 \|\phi^\star\|_2 
&\leq \frac{(p[\sqrt{ 1 + \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2}-1]+ (1-p) \sqrt{ \sigma_1^2+ \sigma_2^2\|\tilde a^{-1}\|_2^2})}{B(p,N)}
\end{array}
  \] 

\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Inner and outer Gaussian and adversarial noise together}
When 
If $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
$Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$.

Our generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
We define our robust objective as   
\[
 \begin{array}{ll}
& F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)\\
:=& 
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2-\epsilon \zeta |
\end{array}
  \]  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  
 
  
  
  
  
  
  
  
  
  
  
  
  
  
% % \paragraph{Mathematical formulation: sparse plus gaussian signal with additional noise}

% % \BIT
% % \item
% % Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
% %  \item
% % The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
% % \item
% % $Z_1$ is IID sampled from  $N(0,I)$, $Z_2$ is IID sampled from  $N(0,I)$, they are independent.
% % \item
% % \[
% % \begin{array}{ll}
% % Y&= a* (X+\sigma_1 Z_1) + \sigma_2 Z_2\\
% % &= a* (X+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)\\
% % &= a* (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \end{array}
% % \]
% % let $C_a^{-1}$ be the linear operator represents $a^{-1}*$, now using the property for sum of independent Gaussian, if we condition on $I$ fixed, then 
% % \[
% % \begin{array}{ll}
% % (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)
% % \sim N(0, (I+\sigma_1+\sigma_2 C_a^{-1} )(I+\sigma_1+\sigma_2 C_a^{-1} )^T)
% % \end{array}
% % \]
% % then let $\tilde{\psi} := w*a$,  
% % \[
% %  \begin{array}{ll}
% % \Expect|(w*Y)_0|
% % &= \Expect|\psi^T (I\cdot G+\sigma_1 Z_1+\sigma_2 a^{-1}* Z_2)| \\
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% % \end{array}
% %   \]

% % \EIT



% % \paragraph{The original convex problem analysis}
% % We still analyze 
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   & \Expect|(w*Y)_0|\\
% % \mbox{subject to}  
% % & v^T w =1,
% % \end{array}
% %   \]
% %   Which is 
% %   \[
% %  \begin{array}{ll}
% %  \mbox{minimize}_{w}   &\sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2\\
% % \mbox{subject to}  
% % & u^T \psi =1,
% % \end{array}
% %   \]
% %   for $u = \tilde{a}^{-1}*v$.
% %  The subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % \partial [\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 ]
% % &= 
% % \Expect_I [N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
% %   the projected subgradient of objective is  
% %     \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [
% % N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi )]
% % \end{array}
% %   \]
  
% %   First the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| (I_0+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| (1+\sigma_1)e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_1 e_0+\sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
  
%  \paragraph{Study inner Gaussian noise only }
% %  First, we study the case when $\sigma_2 = 0$, $0<\sigma_1<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} | I_0+\sigma_1|
% %  &=p| 1+\sigma_1|+(1-p)| \sigma_1|\\
% %  &=p +\sigma_1
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( e_0\cdot (I+\sigma_1) )]
% % &= P_{u}^{\perp} e_0
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u=e_0$.
  

  
  
  
  
%   \paragraph{Study outer Gaussian noise only }
% %  First, we study the case when $\sigma_1 = 0$, $0<\sigma_2<1$.
% %  Then the scaled objective at $e_0$ is
% %   \[
% %  \begin{array}{ll}
% %   \Expect_{I_0} \| I_0\cdot e_0+\sigma_2
% %  a^{-1}\|_2
% %  &=p\| e_0+\sigma_2
% %  a^{-1}\|_2+(1-p)\| \sigma_2
% %  a^{-1}\|_2
% % \end{array}
% %   \]
% % \[
% %  \begin{array}{ll}
% % P_{u}^{\perp} \Expect_I [N( I_0\cdot e_0+\sigma_2
% %  a^{-1} )]
% % &= P_{u}^{\perp} [p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )]
% % \end{array}
% %   \]
% %   so $e_0$ is not the stationary point unless $u$ is along the direction of $p N(  e_0+\sigma_2
% %  a^{-1} )+(1-p) N( a^{-1} )$.
  
  
%   \paragraph{Possible  goal}
%   \BIT
%   \item
%   Show that for minimizer $\psi^*$ of the noisy objective
%   \[
%  \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2 
%   \]
%   is small and bounded by $\sigma_1$ and $\sigma_2$.
  
  
  
%   \begin{lemma}
%   We get the upper bound and lower bound of optimal objective value between the noisy and the noiseless setting
%   \[
%   \Expect_I \|I\cdot e_0\|_2  \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^*\|_2\leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  
%   \]
%   \end{lemma}
  
%     Now we get the bound of objective value between the noisy and the noiseless setting
%   \begin{lemma}
%   \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  p(\| (1+\sigma_1)e_0+\sigma_2
%  a^{-1}\|_2-1)+(1-p)\| \sigma_1 e_0+\sigma_2
%  a^{-1}\|_2 
%   \]
%     \[
%   \Expect_I \|(I\cdot+\sigma_1)e_0\|_2  - \Expect_I \|I\cdot e_0\|_2  =  \sigma_1
%   \]
%   \end{lemma}
%   \item
%   Describe the minimizer $\psi^*$ of the noisy objective by 
%      \[
%  \begin{array}{ll}
% 0= P_{u}^{\perp} \Expect_I [
% N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi^* )]
% \end{array}
%   \]
%   Then find a norm $d$ so that
%   $
%   d(\psi^*, e_0) 
%   $
%   or
%   $
%   d(w^*, a^{-1}) 
%   $
%   is bounded by $\sigma_1$ and $\sigma_2$
%   \EIT
   
   
%  \paragraph{Lemma for expectation}  
%   Mimic the lemma from previous section, we know that 

% \begin{lemma} \label{lem:BGPropLemmaSub}
% \[
%   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq  \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
%   \[
%   \bar{B}(k-1;n,p) \cdot \|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} + (1- \bar{B}(k-1;n,p)) \cdot \|(\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k} \leq \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2^{2k}
%  \]
% where $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
% is the survivor function (Complementary CDF) of the Binomial.
% \end{lemma}



% \begin{lemma} 
% There exists a sequence $(\eps_N)$ depending only on $N$ and $A$ so that  $\eps_N \goto 0$ 
% and so that for each $N$ and for each 
% vector $\psi$  in $\reals^N$, with $\|\psi\|_{\ell_2} \leq A$ and $\|\psi\|_{\ell_0} = N$,
% \beq \label{eq:LemmObjNoise}
%  (1-N^{-1}) \cdot(1 - \eps_N)  \leq  \frac{\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq 1 + \eps_N .
% \eeq
% \end{lemma}

 
 
 
%  \paragraph{Bound on objective and subgradient}
%   Using the lemma, we could link the objective to $2-$norm of $\phi^* = e_0 + \psi^*$, 
%   \[
%     \begin{array}{ll}
%   \|\psi^*-e_0\|_2 = \|\phi^*\|_2 
%   \end{array}
%   \]
  
  
  

% Define the following notation for function, where $I$ is a fixed support, 
% \[
%  \begin{array}{ll}
% F_1(\phi) &:=   \|(1 +\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F_I(\phi) &:=   \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi)\|_2\\
% F^E(\phi)&:= \Expect_I F_I(\phi)   
% \end{array}
% \]
% then
% \[
%  \begin{array}{ll}
% \partial  F_I(\phi) &:= N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi) )\\
% \partial F^E(\phi)&:= \partial \Expect_I F_I(\phi)  =   \Expect_I \partial  F_I(\phi)
% \end{array}
% \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% % \[
% %  \begin{array}{ll}

% % \end{array}
% % \]

% Using Lebourg’s mean value theorem, Theorem 2.3.7 of Clarke (1990) \cite{clarke1990optimization}, there exists $ t \in (0,1),$ so that
% \[
%  \begin{array}{ll}
% \Expect_I F_I(0) -   \Expect_I F_I( \phi^*)\in \langle  
% \partial \Expect_I F_I( t\phi^*), \phi^* \rangle
% \end{array}
% \]



%   We want to bound the finite difference:
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 } \in \langle  
% \partial \Expect_I F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
    
% % \frac{|\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)e_0\|_2 -   \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)( e_0 + \phi^*)\|_2| }{\|\phi^*\|_2 } 
% \end{array}
%   \]
%  And since $t\neq 1$, $\Expect_I N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) )$ is not a set but just a unit vector,
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
  
%   Since $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*)>0$ when the minimizer $\phi^*$ is not $0$, in this case,  a natural bound is
%   \[
%     \begin{array}{ll}
%  0 <  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   More specifically, there exists $\rho>0,$ 
%     \[
%     \begin{array}{ll}
%  \rho \leq  \Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \leq 1
% \end{array}
%   \]
%   Therefore, using the fact that 
%   \[
%     \begin{array}{ll}
    
%     \frac{\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) }{\|\phi^*\|_2 }  \in [\rho,1]
% \end{array}
%   \]
%  We could bound $\Expect_I F_I(0) -   \Expect_I F_I(  \phi^*) $ by bound $\|\phi^*\|_2$.
   
   
% For $\bar{B}(k-1;N,p) \equiv  \sum_{n=k}^{N} (1-p)^n p^{N-n} {N \choose n} $
 
 
% We need a new lemma for subgradient, 
% % \begin{lemma} 
% % \beq \label{eq:LemmSubGradNoise}
% % C_{-}'  \leq  \frac{\partial\Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2 }{\partial\|(1+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2} \leq C_+' .
% % \eeq
% % \end{lemma} 
 
%  \begin{lemma} 
%  For the minimizer $\phi^*$ so that $u^T \phi^* =0$,
% \beq \label{eq:LemmDirGradNoise}
% C_{-}  \leq  \frac{ \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   }{ \langle   \partial F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%  }  = \frac{\Expect_I \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]}{\cos[\angle( (1+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)]} \leq C_+ .
% \eeq
% \end{lemma} 
% \begin{proof}


% \begin{eqnarray*}
% & & E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*), \phi^*)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   \end{eqnarray*}
 
 
% Using the fact that $\phi^*$ is minimizer,  we know that for any $\beta$ so that $u^T \beta = 0, \|\beta\|_2=1$,
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &\geq& 0
%   \end{eqnarray*}
% where
% \begin{eqnarray*}
% \langle  E_I \partial F_I( \phi^*), \beta \rangle &=& E_I  \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} \cos[\angle( (I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*), \beta)] \\
% &=&   
% \langle \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) ), \beta \rangle
%   \end{eqnarray*}
% It requires
% \begin{eqnarray*}
% 0 \in \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot  \sum_{|I| =n}  P_{u}^{\perp} N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +\phi^*) )
%   \end{eqnarray*}




%   \end{proof}   






















==> sec/Noise_updated.tex <==
\section{Robustness for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $\zeta_1$ and $\zeta_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 \zeta_1+  \sigma_1 G_1) + \eta_2 \zeta_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 

  
In the following,
let 
\[
D_R( \psi) :=  F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)-F_{0,0,0,0}(\psi).
\]
We use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$

Let $\phi^\star := \psi^\star-e_0$,
we have
   \[
 \begin{array}{ll}
D_R( e_0) &= F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)\\
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,\phi^\star) \|\psi^\star-e_0\|_2\\
 &\geq p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G| = \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
  \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_Monot}
$\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
\end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
\end{lemma}


\paragraph{Robust optimization}
% We want to find the min-max value 
% \[
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta)
% \]
% for a function $H$,
% \[
% H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
% \]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


% \begin{lemma}
% \label{min-maxError}
% For $A>0$, 
% \[
%  \begin{array}{ll}
% \inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
% \end{array}
% \]
% where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
% \end{lemma}
% \begin{lemma}
% \label{min-maxErrorL_p}
% Let
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
%  \end{array}
%   \]
%   where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
%   then
% \[
%  \begin{array}{ll}
% \inf_{\zeta^2\leq 1}\sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2)  - \epsilon \zeta) = 
% H( \mu(\psi))
% \end{array}
% \]

% \end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
%  \[
%  \begin{array}{ll}
%  \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
%  \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
%  \end{array}
%   \]
 \[
 \begin{array}{ll}
 \mu(\psi) &=\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}\\
 \sigma_n^2(\psi) &=  \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}\Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2 |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \sup_{\zeta_1, \zeta_2: \|\zeta_1\|_{p_1} \leq 1; \|\zeta_2\|_{p_2} \leq 1}[\eta_1 \zeta_1 +\eta_2 a^{-1}* \zeta_2] |\\
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
 
 The second inequality comes from the fact that $\mathcal{R}(\gamma)$ is an even function that is monotonically non-decreasing for $\gamma \geq 0$.
  
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
For $p<p^\star_1 = 1-\tan(\theta),$
 \[
 \begin{array}{ll}
 \|\phi^\star\|_2\leq 
  \frac{(1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

 
\end{theorem}  
\begin{proof}
 Since
 \[
 \begin{array}{ll}
  B(p,\phi^\star) \|\phi^\star\|_2\leq 
 D_R(e_0) = F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0) 
\end{array}
  \] 
  and
   \[
 \begin{array}{ll}
 p (
(1-p)- \tan(\theta) )\cos{\theta} \|\phi^\star\|_2\leq  B(p,\phi^\star) \|\phi^\star\|_2 
\end{array}
  \]  
  where
\[
 \begin{array}{ll}
 D_R(e_0) = (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{proof}
\begin{coro}
When $\sigma_1 = \sigma_2 = 0,$
 \[
 \begin{array}{ll}
\|\psi^\star -e_0\|_2\leq 
 \frac{p\mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}

\begin{coro}
When $\eta_1 = \eta_2 = 0,$
 \[
 \begin{array}{ll}
 \|\psi^\star -e_0\|_2\leq 
 \frac{ (1-p) \sigma_n(e_0)^2 +  
 p\sqrt{1+ \sigma^2_n(e_0)}  - p}{p (
(1-p)- \tan(\theta) )\cos{\theta} }
\end{array}
  \]  

\end{coro}








\subsection{All the proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



% \subsection{Constrained Convex algorithms }
%  \paragraph{Constrained noisy convex problems}
% Then we define the constrained convex program that allows noise,
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,z}   & |\alpha| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
% \label{eq:ConstrainProb}
%   \]
%   If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
% \mbox{subject to}  
% & v^T w =1,\\
% & \zeta^2 \leq 1
% \end{array}
% \tag{$P^c_{1,\epsilon}$}
%   \]
% If we set $\epsilon = 0,$ then we recover 
% the original convex problems for noiseless setting
% \[
%  \begin{array}{ll}
%  \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
% \mbox{subject to}  
% & v^T w =1,
% \end{array}
% \tag{$P_1$}
%   \]

==> sec/Noise_updated_constraint.tex <==
\section{Stability for noisy observation}
\subsection{Inner and outer Gaussian and adversarial noise}
\paragraph{Mathematical formulation: sparse signal plus inner and outer adversarial perturbation and Gaussian noise}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$, write $X_t = I_t \cdot G_t$ where $I_t$ is IID sampled from Bernoulli, $G_t$ is IID sampled from standard Gaussian.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$
\item
Let $G_1$ and $G_2$ are two independent standard normal $N(0,I_N)$. 
\item
Let $Z_1$ and $Z_2$ are inner and outer adversarial noise with $p_1$ and $p_2$ norm bounded by $1$, where for $p_1, p_2\geq 1, $ $q_1$ and $q_2$ is defined by $\frac{1}{p_i}+\frac{1}{q_i} =1.$
\item
Our data generative model is
\[
\begin{array}{ll}
Y&= a* (X+ \eta_1 Z_1+  \sigma_1 G_1) + \eta_2 Z_2+ \sigma_2 G_2\\
&= a* (X +\eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2)
\end{array}
\]
\item
Let the total perturbation be
\[
\begin{array}{ll}
Z= \eta_1 Z_1 +\eta_2 a^{-1}* Z_2+  \sigma_1 G_1+\sigma_2 a^{-1}* G_2
\end{array}
\]
We can write data generative model  simply as
\[
\begin{array}{ll}
Y&= a* (X+ Z ) 
\end{array}
\]
\EIT
Let $\tilde{\psi} := w*a$,   $\phi: = \psi - e_0$, then
\[
 \begin{array}{ll}
(w*Y)_0
&= \psi^T (X+  Z ) 
\end{array}
  \]

 \paragraph{Perturbation analysis of the robust convex problems}
The original convex problems is
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]  
Our objective is
\[
|\psi^T (X+  Z )-\epsilon \zeta|  = |\psi^T X+\psi^T[\sigma_1  G_1+\sigma_2 (a^{-1}* G_2) + \eta_1 Z_1 +\eta_2 a^{-1}* Z_2]-\epsilon \zeta |
\]
\paragraph{Worst case robust objective over adversarial perturbation}  
For the constrained problem, we first take expectation over Gaussian noise and over the Bernoulli Gaussian signal, then we optimize over the worst case expected objective for all adversarial perturbation, we define our robust objective as   
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
:=
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1}
\Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T (X+  Z )-\epsilon \zeta|
\end{array}
  \]  
then our robust constrained problem becomes
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi) \\
\mbox{subject to}  
&u^T \psi =1
\end{array}
  \]
Assume that the minimizer of the robust problem is $\psi^\star$, then we have the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) =p
\end{array}
  \] 
In the following, we use this fact and the bi-lipschitz property of noiseless objective around $e_0$ to bound the $\ell_2$ norm deviation $\|\psi^\star-e_0\|_2.$
   \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)-F_{0,0,0,0}(e_0)
 &\geq F_{0,0,0,0}(\psi^\star )-F_{0,0,0,0}(e_0) \\
 &\geq B(p,N) \|\psi^\star-e_0\|_2
\end{array}
  \] 

This bound is not tight but it is tight in order and it is easy to compute since we only need to compute  $F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)$, the robust objective at $e_0$.
 
\subsection{Folded Gaussian}
\paragraph{Folded Gaussian}
For Bernoulli Gaussian $X$ with support $I$, if we condition on $I$ fixed, then  using the rotation invariance of Gaussian, $\psi^T X$ is  Gaussian with mean $0$ and standard deviation $\|\psi_I\|_2$.

From general theory of folded Gaussian,
\footnote{see: \url{ https://en.wikipedia.org/wiki/Folded_normal_distribution}.}
 $ |\mu+ \sigma G |, \quad  G \sim \N(0, 1).$
Then its mean is
\beq
\label{FoldedGaussianMean}
E_G |\mu+ \sigma G| =  \sqrt{\frac{2}{\pi}} \sigma \exp\{-\mu^2/(2\sigma^2)\} + \mu \left(1 - 2\Phi\left(\frac{-\mu}{\sigma}\right) \right)
\eeq
where $\Phi$  is the normal cumulative distribution function:
\[
\Phi(x) = \frac 1 {\sqrt{2\pi}} \int_{-\infty}^x e^{-t^2/2} \, dt.
\]
Its variance is
\beq
\label{FoldedGaussianVar}
\Var_G |\mu+ \sigma G| = E_G( |\mu+ \sigma G|-E_G |\mu+ \sigma G|)^2 =\sigma^2+ \mu^2 -(E_G |\mu+ \sigma G|)^2
\eeq  
The variance will be useful for concentration with finite sample.  

\paragraph{Asymptotic expansion for mean of folded Gaussian}
Notice that if $\sigma =0$, then
\[
E_G |\mu+ 0\cdot G| =   |\mu|.
\]
If $\mu =0$, then we go back to mean of half-normal,
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
Let 
\[
\gamma:= \frac{\mu}{\sigma}
\] 

\begin{lemma}
\label{ExpansionMeanFoldedGaussian}
We define the ratio of folded gaussian mean as 
\[
\mathcal{R}^f(\gamma) := \frac{E_G |\mu+ \sigma G|}{E_G |\sigma G|} = \frac{E_G |\mu+ \sigma G|}{\sqrt{\frac{2}{\pi}}\sigma} = \sqrt{\frac{\pi}{2}} E_G |\gamma+  G|
\]
We have three different expressions (asymptotic expansion around  $\gamma$) for $\mathcal{R}^f(\gamma)$:
\BEA
\label{FoldedGaussianMean_ratio}
\mathcal{R}^f(\gamma)
&=&  \exp\{-\gamma^2/2\} + \sqrt{\frac{\pi}{2}}\gamma \left(1 - 2\Phi\left(-\gamma\right) \right)\\
&=&  \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
&=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\EEA
 \end{lemma}
 
 \begin{lemma}
 \label{ExpansionMeanFoldedGaussian_LB}
when $\gamma<2,$ 
\[
\mathcal{R}^f(\gamma) \geq 1 + \frac{3}{2}\gamma^2
\]
% hence
% \[
%  \begin{array}{ll}
% E_G |\mu+ \sigma G|
% &\geq \sqrt{\frac{2}{\pi}}\left[\sigma + \frac{3}{2}\mu^2/\sigma \right]
% \end{array}
% \]
\end{lemma}


\paragraph{Robust optimization}
We want to find the min-max value 
\[
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta)
\]
for a function $H$,
\[
H(t) := \Expect_{G_1} \Expect_{G_2} \Expect_X|t+ \psi^T (X+  \sigma_1  G_1+\sigma_2 (a^{-1}* G_2) )|
\]
\begin{lemma}
From Hölder's inequality, for any vector $a \in \reals^N$, for $p\geq 1, \frac{1}{p}+\frac{1}{q} =1,$
\[
\sup_{Z: \|Z\|_p\leq 1}(a^T Z) = \|a\|_q,
\]
specifically, when $|Z|^p$ is along the direction of $\mbox{sign}(a)|a|^q$ so that $a^T Z = \|a\|_q$.

\end{lemma}  


\begin{lemma}
\label{min-maxError}
For $A>0$, 
\[
 \begin{array}{ll}
\inf_{\zeta: \zeta^2 \leq 1} (A - \epsilon \zeta) = (A - \epsilon )_+
\end{array}
\]
where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function.
\end{lemma}
\begin{lemma}
\label{min-maxErrorL_p}
Let
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+
 \end{array}
  \]
  where $(\cdot)_+: = \max{(0, \cdot)}$ is the ReLU function,
  then
\[
 \begin{array}{ll}
\inf_{\zeta^2\leq 1}\sup_{Z_1, Z_2: \|Z_1\|_{p_1} \leq 1; \|Z_2\|_{p_2} \leq 1} H( \psi^T (\eta_1 Z_1 +\eta_2 a^{-1}* Z_2)  - \epsilon \zeta) = 
H( \mu(\psi))
\end{array}
\]

\end{lemma}
\paragraph{Bound on the noisy solution using robust objective}  
\begin{lemma}
\label{lemma:Obj_Folded_FullNoise}
Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &=(\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}
 \end{array}
  \]
then the objective is a mean of a folded Gaussian random variable:
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&= \Expect_I\Expect_{G}  | \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} G  + \mu(\psi) |\\
&= \sqrt{\frac{2}{\pi}} \Expect_I[ \sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)} 
\mathcal{R}^f(\frac{\mu(\psi)}{\sqrt{\|\psi_I\|_2^2 + \sigma_n^2(\psi)}})]
\end{array}
  \] 
  where $G$ is scalar standard Gaussian.
\end{lemma}
From a simple inequality:
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]  
we have  
\begin{theorem}
\label{thm:Bound_FullNoise}
\[
 \begin{array}{ll}
 B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) - p
\end{array}
  \]  
where
\[
 \begin{array}{ll}
 \mu(e_0) &= (\eta_1 + \eta_2 \| a^{-1} \|_{q_2}-\epsilon)_+\\
 \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2\|a^{-1}\|_2^2} 
 \end{array}
  \]
\end{theorem}  

\subsection{Proofs}    
\begin{proof}[Proof of lemma~\ref{lemma:Obj_Folded_FullNoise}]
 First, for any fixed vector $\mu$,
\[
 \begin{array}{ll}
  \Expect_{G_1} \Expect_{G_2} \Expect_X|\psi^T X+\sigma_1 \psi^T G_1+\sigma_2 \psi^T (a^{-1}* G_2) + \mu | = 
   \Expect_I\Expect_{G_3}  | \sqrt{ \|\psi_I\|_2^2 + \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}G_3  + \mu|
\end{array}
  \]
  Let 
 \[
 \begin{array}{ll}
 \mu(\psi) &= (\eta_1\|\psi\|_{q_1}+ \eta_2\|C_{a^{-1}}^T \psi\|_{q_2}-\epsilon)_+\\
 \sigma_n^2(\psi) &= \sqrt{ \sigma_1^2\|\psi\|_2^2 + \sigma_2^2\|C_{a^{-1}}^T \psi\|_2^2}\\
  \sigma_s^2(\psi_I) &=  \|\psi_I\|_2^2 \\
 \sigma^2 (\psi, \psi_I) &= \sigma_s^2(\psi_I) + \sigma_n^2(\psi) 
 \end{array}
  \]
 Using lemma~\ref{min-maxErrorL_p}, we have
\[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(\psi)
&=\Expect_I\Expect_{G}  | \sigma (\psi, \psi_I) G  + \mu(\psi) | \\
&=\Expect_I\Expect_{G}  | \sqrt{\sigma_s^2(\psi_I) + \sigma_n^2(\psi)} G  + \mu(\psi) | \\
\end{array}
  \]    

\end{proof}

\begin{proof}[Proof of theorem~\ref{thm:Bound_FullNoise}]  
Additionally, for $\tilde a^{-1} $, define its norm as
\[
M_q: = \|\tilde a^{-1} \|_{q} = \| a^{-1} \|_{q}
\]

 When $\psi = e_0$, then
 \[
 \begin{array}{ll}
 \mu(e_0) &= \eta_1 + \eta_2 M_{q_2}\\
  \sigma_n(e_0) &=\sqrt{ \sigma_1^2 + \sigma_2^2 M_{2}^2} \\
 \sigma_s((e_0)_I) &= I_0 
 \end{array}
  \]

  
We have 
\[
 \begin{array}{ll}
 F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
 &= 
  \Expect_{G} \Expect_{I_0} |  \sigma(e_0, (e_0)_{I_0})  G  +  \mu(e_0)| \\
  &= 
 (1-p)\Expect_{G} |  \sigma_n(e_0) G  +  \mu(e_0)|+ p\Expect_{G} | \sqrt{1+ \sigma^2_n(e_0)}  G  +  \mu(e_0)|\\
   &=
 \sqrt{\frac{2}{\pi}}[ (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) ]
\end{array}
  \]
  Using the chain of inequality:
    \[
 \begin{array}{ll}
F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((e_0)
 \geq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}((\psi^\star ) 
 \geq F_{0,0,0,0}(\psi^\star )
 \geq F_{0,0,0,0}(e_0) 
\end{array}
  \] 
and the fact that
  \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star )
 &= \Expect_I\|\psi_I\|_2 \\
 &= \Expect_I\|(e_0)_I\|_2 + (\Expect_I\|\psi_I\|_2-\Expect_I\|(e_0)_I\|_2) \\
 &= \sqrt{\frac{2}{\pi}}[p+ B(p,N) \|\psi -e_0\|_2]
\end{array}
  \]   
  From
   \[
 \begin{array}{ll}
 F_{0,0,0,0}(\psi^\star ) &\leq F_{\eta_1,\eta_2, \sigma_1,\sigma_2}(e_0)
\end{array}
  \]   
we have
  \[
 \begin{array}{ll}
p+ B(p,N) \|\psi^\star -e_0\|_2\leq (1-p) \sigma_n(e_0)^2 \mathcal{R}^f(\frac{\mu(e_0)}{\sigma_n(e_0)})+  
 p\sqrt{1+ \sigma^2_n(e_0)} \mathcal{R}^f(\frac{\mu(e_0)}{\sqrt{1+ \sigma^2_n(e_0)}}) 
\end{array}
  \]   

\end{proof}  







\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian}]
Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\[
E_G |\mu+ \sigma G| = \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)
\]
Divide it by 
\[
E_G |\sigma G| =   \sqrt{\frac{2}{\pi}} \sigma
\]
we get the first equality.

Since the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 
% \footnote{see: \href{https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function}{en.wikipedia.org/wiki/Normal_distributionCumulative_distribution_function} }

\[
1 - 2\Phi(-\gamma)  = \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2}\left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
This gives the second inequality.

Additionally,
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}
\end{array}
  \] 
then
 \[
 \begin{array}{ll}
& \exp\{-\gamma^2/2\}\{1 + \frac{1}{2}\gamma \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]\}\\
=& (\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!})\{1 + \frac{1}{2}\gamma \left[ \sum_{n=0}^{\infty} \frac{ \gamma^{2n+1}}{(2n+1)!!} \right]\}\\

=& 1 + \frac{3}{2}\gamma^2 + \frac{1}{24} \gamma^4   - \frac{ \gamma^6}{120}  + O(\gamma^8) 
\end{array}
  \] 
\end{proof}


\begin{proof}[Proof of lemma~\ref{ExpansionMeanFoldedGaussian_LB}]
Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ +  \frac{ \gamma^4}{15}+ O( \gamma^6) ]/[1 + \frac{ \gamma^2}{2}+ +  \frac{ \gamma^4}{8}+O( \gamma^6)] \\
&= 1 -\frac{ \gamma^2}{6}+  \frac{ \gamma^4}{40}+ O( \gamma^6)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G|
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&:= \frac{ (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2)
\\
&= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  (\exp\{-\gamma^2/2\} - 1 + \gamma^2/2) \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-\gamma^4 }{12}  +    \frac{ \gamma^6}{80} +\frac{\gamma^{4}}{(-2)^2 (2)!} +\frac{\gamma^{6}}{(-2)^3 (3)!}+
O(\gamma^8)\\
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)
\end{array}
\] 
We know that if $\gamma^2<1,$ 
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) 
&=    \frac{\gamma^4 }{24}  - \frac{ \gamma^6}{120}  + O(\gamma^8)\\
&\geq 0
\end{array}
\] 
(We comment that we could push the range for $\mbox{Res}(\gamma^2) 
\geq 0$ further to at least $\gamma^2<5$ if needed.)
Then we give an lower bound:
\[
 \begin{array}{ll}
E_G |\mu+ \sigma G| 
&= \sqrt{\frac{2}{\pi}} \sigma\left[ 1 + \frac{3}{2}\gamma^2+   \mbox{Res}\right]\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}



\subsection{Constrained Convex algorithms }
 \paragraph{Constrained noisy convex problems}
Then we define the constrained convex program that allows noise,
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,z}   & |\alpha| \\
\mbox{subject to}  
& v^T w =1,\\
& \Expect(\alpha -\tilde{w}^T Y)^2 \leq \epsilon^2
\end{array}
\tag{$P^c_{1,\epsilon}$}
\label{eq:ConstrainProb}
  \]
  If we write $\alpha =\tilde{w}^T Y - \epsilon \zeta $ , then
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & \Expect|\tilde{w}^T Y - \epsilon \zeta| \\
\mbox{subject to}  
& v^T w =1,\\
& \zeta^2 \leq 1
\end{array}
\tag{$P^c_{1,\epsilon}$}
  \]
If we set $\epsilon = 0,$ then we recover 
the original convex problems for noiseless setting
\[
 \begin{array}{ll}
 \mbox{minimize}_{w}   & \Expect|\tilde{w}^T Y|\\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_1$}
  \]

==> sec/Phase_Transition.tex <==

\subsection{Population Phase transition theorem}
Qingyun: Old proof without subgradient language:

\paragraph{Population phase transition theorem}
\begin{theorem}
Under the previous assumption,
$
         p^\star   =\frac{\sin{\theta}}{\sin{\theta}+ \cos{\theta}} .
$
 The solution of  $P_{1,v}$ is $w^\star$, then 
 $w^\star$ is $a^{-1}$ up to shift and scaling provided $p<p^\star$,
and  $w^\star$ is not $a^{-1}$ up to shift and scaling provided $p> p^\star$.
  \end{theorem}
The population phase transition diagram is in figure~\ref{fig-PT}.

\begin{figure} 
\centering
\includegraphics[width=.7\textwidth]{./figures_BD/Phase_T_sine.png}
\caption{The population phase transition diagram, $x-$axis is $\sin{\theta}$, $y-$axis is the sparsity level $p$ . Red part is failure, Blue part is success.}
\label{fig-PT}
\end{figure}



% \begin{theorem} \label{lem:ica}
% We observe a sequence $Y\in \reals^n$, and we know that there exists a ground-truth filter $w^0$, such that $w^0*Y = X$, $X$ satisfy Bernoulli$(p)$-Gaussian model.  
% And we assume that we have a solution $w^\star$ to the Sparse convolutional ICA problem.
% Then if the angle $\theta$ between the vector $v$ and $w^0$ and the sparsity level $p$ satisfy that 
% \[
% \frac{p}{1-p}<\gamma \cot(\theta),
% \]
% then  $w^\star$ equals $w^0$ up to scaling, namely $w^\star = cw^0$ for $c\in \reals$ with probability $1-\exp\left( -C_0 \kappa_{w^0}^{-2} k\log(kp)\right)$, where $C_0$ is a constant, $\kappa_{w^0}$ is the condition number of the circulant matrix generated by $w^0$.

% \end{theorem}


\paragraph{Proof of the population phase transition theorem}
\BIT
 \item
  Let $\phi  := \psi -e_0 = \tilde w*\tilde a -e_0,$  then $|[w*Y]_0| = |[(e_0 +\tilde \phi)*X]_0| =  |[(e_0 + \phi)^T X| $, we define
  \[
  L(\phi) = |[(e_0 + \phi)^T X|.
  \] 
  WLOG, we can assume the ground truth $a^{-1}$ is scaled so that $v^T \tilde{a}^{-1} =1$
%   , then after the change of variable $w =  a^{-1}*(e_0 +\phi)$,  the condition $v^T w = 1$ can be transformed to $u^T \phi = 0$ where 
% $u: =\tilde{a}^{-1}*v$.

  We want to find a threshold $p^\star$ so that for all $p<p^\star$, the directional derivative  $ \Expect \nabla_{\phi}{L}|_{\phi = 0}>0$ for all directions $\phi$ that satisfy $u^T \phi = 0$.

 We define the finite difference
  \[
  D = L(\phi)-L(0) =  |[(e_0 + \phi)^T X| -|X_0| 
  \]
  Let $\epsilon : = \|\phi\|_2 $ and taking limit of $D$ as $\epsilon  \rightarrow 0,$ we have
    \BEQ
  \begin{array}{ll}
   \expect D &=  p\expect[D\mid X_0 \neq 0 ] + 
   (1-p)\expect[D \mid X_0 = 0 ] \\
   &=  p\expect[\mbox{sign}(X_0) ( \phi_0 X_0 + \sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid   \\
   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  
   \end{array}
 \EEQ
The last equality is because 
 $
 \expect[\mbox{sign}(X_0) (\sum_{ j\neq 0}\phi_{j} X_{j} )\mid X_0 \neq 0 ] = 0 
$
 as $X_j$ are sampled independently. Notice that for Bernoulli Gaussian $X$,
$
\Expect [|X_0|\mid X_0 \neq 0 ]=\sqrt{\frac{2}{\pi}}.
$
 
 Then  $ \Expect \nabla_{\phi}{L}|_{\phi = 0} = \Expect \lim_{\epsilon \rightarrow 0}\frac{D}{\epsilon}>0$ 
 in case either $\phi_{0} > 0$, or in case $\phi_0 < 0$ and
\[
          \frac{p}{1-p} < \frac{ \Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  }{|\phi_0| 
          \Expect [|X_0|\mid X_0 \neq 0 ]} = \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} \frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\|\phi_{(0)}\|_2 \sqrt{\frac{2}{\pi}}}  .
\]
Here  $X_{(0)} = (X_i)_{i\neq 0}$
\item (Geometric lower bound:)
Using the fact that $u^T \phi = 0$. We define $v = \cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$, then $u =\tilde{a}^{-1}*v = \tilde{a}^{-1}*(\cos{(\theta)}\frac{\tilde{a}}{\|\tilde{a}\|_2} + \sin{(\theta)} (\frac{\tilde{a}}{\|\tilde{a}\|_2})^{\bot}) =\cos{(\theta)} \frac{e_0}{\|\tilde{a}\|_2}+\sin{(\theta)} \tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot} $, 
where $\tilde{a}^{-1}*(\frac{\tilde{a}}{\|\tilde{a}\|_2} )^{\bot}$ is perpendicular to $e_0$, 
therefore, 
$0= u^T \phi = \frac{1}{\|\tilde{a}\|_2}[\cos{(\theta)} \phi_0+\sin{(\theta)} \phi_{(0)}]$, therefore,  
$\frac{\|\phi_{(0)}\|_2}{| \phi_{0}|} = \frac{\cos(\theta)}{\sin(\theta)} =\cot(\theta).$
\[
 \frac{\|\phi_{(0)}\|_2}{| \phi_{0}|}\geq  \cot(\theta)
 \]

 
% \item 
% Let $h=\phi$, i.e. $h_i=\phi_{-i}$; and let $h_{(0)} = (h_i)_{i\neq 0}$, then
%   \[
%           \frac{p}{1-p} < \frac{ \Expect | h_{(0)}^T X_{(0)} |}{| h_{0}| \Expect |X_0|} = \frac{ \Expect | h_{(0)}^T X_{(0)} |}{\|h_{(0)}\|_2 \Expect |X_0|}  \frac{\|h_{(0)}\|_2}{| h_{0}|} .
% \]
\item
We showed that for IID Bernoulli Gaussian $X$,
\[
\frac{ \Expect | \phi_{(0)}^T X_{(0)} |}{\sqrt{\frac{2}{\pi}} \|\phi_{(0)}\|_2} = \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \in [p,1)
\]
Using semicontinuous extension, we can choose sequence of $\phi$ that is dense on doubly infinite sequence space $V_{-\infty, \infty}$, then we know that $\frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2}$ should be replaced by its semicontinuous extension on $V_{-\infty, \infty}$, which is $1$.

The phase transition $p^\star$ is the smallest $p$ so that 
\[
          \frac{p}{1-p} \leq  \cot(\theta) \frac{ \Expect_{I_{(0)}}\| \phi_{I_{(0)}}\|_2}{ \|\phi_{(0)}\|_2} \leq  \cot(\theta).
\]
%  \BEQ
%   \begin{array}{ll}
%   \Expect D 
%   &= p \phi_0 \Expect [|X_0|\mid X_0 \neq 0 ] + (1-p)\Expect\mid \sum_{ j\neq 0}\phi_{j} X_{j}\mid  \\
%   &=  
%   \sqrt{\frac{2}{\pi}}\|{\phi}_{(0)}\|_2[ p (\mbox{sign}(\phi_{0})\tan(\theta)) + (1-p) (1-(1-p)^{\|{\phi}_{(0)}\|_0})]
%   \end{array}
%  \EEQ
Therefore,  generically, $ \frac{p^\star}{1-p^\star}  = \cot(\theta) $.
\EIT

==> sec/Planted_Proj.tex <==
% \section{Projection pursuit for planted sparsity}
% \subsection{Setup} 
% \subsection{Perturbation analysis}
% First, without loss of generality, we suppose  there is a vector $\beta$, $\beta^T \Phi Y = X_0$.

% Consider a vector  $b $ which is a small perturbation of $\beta$, where
% $\beta^T \Phi =e_0$, we assume $ \cM_1$ is the constraint set for $b$. Let $b = \beta + \eps \delta$ where $\delta \in T_\beta \cM_1$, the tangent space at $\beta$. We assume the condition $\delta \in T_\beta \cM_1$ is given by $v^T \delta = 0$.


% Let $h = \Phi^T \delta$, then from $   v^T \delta = 0$, we have $   u^T h = 0$, where $ v = \Phi u$. We have
% \[
%     b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
% \]
%  where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 
%  Let 
% \[
% D_0 =  |(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -|X_0|, 
% \]
 
 
 
%  Then for sufficiently small $\eps$
% \begin{eqnarray*}
%  E D_0 = E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
%  (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot p+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot (1-p),
% \end{eqnarray*}
%  where $p = P(X_0\neq 0)$.
 
%  The perturbation increases the objective value 
% just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

% Now we consider the optimization problem
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
%     \mbox{ subject to }&  h_{0} = -1, \\
%     & h\in \Phi^T T_\beta \cM_1.
% \end{eqnarray*}


% We know $h = \Phi^T \delta$, then 
% \begin{eqnarray*}
%     (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
%     \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
%      & \delta \in T_\beta \cM_1.
% \end{eqnarray*}

% \subsection{Geometric lower bound}
% We know that from perturbation analysis, the condition for phase transition are
% \[
%           \frac{1-p}{p} < \frac{ E | h_{(0)}^T X_{(0)} |}{| h_{0}| E |X_0|}.
% \]

%  We know $X_0$ is random variable sampled from a symmetric distribution with atom at $0$, $F_p = p H +(1-p) F$, and $X_i, \quad i\neq 0$ are sampled from distribution $G$.
% Using the sparsity of $X_0$,
% \[
% E \{ D_0 | X_0\neq 0 \}  = (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0|.
% \]
% And
% \[
% E \{ D_0 | X_0 =  0 \}  = E{|h_{(0)}^T X_{(0)}| }.
% \]

% First, when $F_t$ are all Gaussian distributions for $t\neq 0$, we leverage the invariance property for linear transform of Gaussian, and get 
% \[
% E{|h_{(0)}^T X_{(0)}| } = \|h_{(0)}\|_2 E|G| = \sqrt{\frac{2}{\pi}} \cdot \|h_{(0)}\|_2.
% \]

% % And we have calculated $E{|h_{(0)}^T X_{(0)}| }$ for different cases of $F_t$. 
% % For example, it is  lower bounded by  a constant multiple $\|h_{(0)}\|_2$ .

% And since we know $v^T h=0$, when $X_i$ are IID Gaussian, then linear combination of Gaussian are still Gaussian, so without loss of generality, we can change coordinate and assume $h = h_0 e_0 + h_1 t_1 + h' $, where $e_0$ is the unit vector in the direction of ground truth, $t_1$ is the unit vector in the direction of the component of $v$ normal to $e_0$, and $h'$ is in the rest of directions .

% Then we have $\|h_{(0)}\|_2\geq |h_1|$,
% and 
 
% \[
%           \frac{1-p}{p} <  \frac{  |h_1|} {| h_{0}|} = \cot(\theta).
% \]


\section{Phase transition for sub-Gaussian}
From the Khinthine’s inequality for sub-Gaussian and $p = 1$, we have 
\[
E{|h_{(0)}^T X_{(0)}| }\geq  3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2,
\]
for Bernoulli-SubGaussian, we have,
\[
E{|h_{(0)}^T X_{(0)}| }\geq  (1-(1-p)^M)^{1/2} 3^{-3/2}C^{-3} K^{-3}  \|h_{(0)}\|_2.
\]
In general, we define
\[
\gamma(F,p) = E{|h_{(0)}^T X_{(0)}| }/\|h_{(0)}\|_2 E |X_0|,
\]
as the ratio between the linear combination $E{|h_{(0)}^T X_{(0)}| }$ for $\|h_{(0)}\|_2=1$ and $ E |X_0|$.

Then we need
\[
          \frac{1-p}{p} < \frac{ \gamma(F,p)  \|h_{(0)}\|_2}{| h_{0}|}
\]
for all $h$ such that $   u^T h = 0$ .

Also, using the fact that
 
\[
         \frac{  \|h_{(0)}\|_2} {| h_{0}|} \geq \cot(\theta).
\]
we have 
\[
          \frac{1-p}{p} <\gamma(F,p) \cot(\theta).
\]

\section{Noisy  signal}
 \subsection{Folder Gaussian}
 For a Gaussian RV $Z \sim N(\mu, \sigma)$, then for RV $|Z|$,  
 \[
 \mu_{|Z|} = E|Z|=\sqrt{\frac{2}{\pi}}\sigma e^{-\frac{\mu^2}{2\sigma^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma}\right) \right] 
%  = f(\mu,\sigma),
 \]
  \[
 \sigma_{|Z|}^2 = \mu^2 + \sigma^2 - \mu_{|Z|}^2.,
 \]
%  Then for fixed $\sigma$, let
%  \[
%  h_\sigma(\mu) = f(\mu,\sigma) 
%  \]
%  then 
%   \[
%  h'_\sigma(\mu) = 
%  \]
 
 \subsection{Noisy perturbation analysis}
Consider a noisy perturbation $\bar X_i  =  X_i + \sigma  E_i $, where $E_i$ is standard Gaussian $N(0,1)$, $ X_i = B_i Z_i$ are iid product of Bernolli RV with parameter $p$ and subGaussian unit variance RV with c.d.f $F$. 

Then we let $b^{\sigma}$ be the solution of the optimization problem 
\[
E D_\sigma = E_X E_E( |(1+ \eps h_0)(X_0+\sigma  E_0) +  \eps h_{(0)}^T (X_{(0)}+\sigma  E_{(0)})| -|X_0+\sigma  E_0|)
% = E_X (h'_\sigma(\mu)), 
\]
for sufficiently small $\eps$, and fixed $\sigma<1$, we consider the asymptotic analysis when $\eps  << 1 $， $ \sigma<< 1 $. We know $\sigma ((1+ \eps h_0)(  E_0)+\eps h_{(0)}^T  E_{(0)}))$ is a centered Gaussian with standard deviation 
\[\sigma\sqrt{(1+ \eps h_0)^2+(\eps h_{(0)})^2}\approx \sigma(1+ \eps h_0)
\]
therefore,
\begin{eqnarray*}
 E D_\sigma &\approx&   E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}+\sigma (1+ \eps h_0) E_0| -E|X_0+\sigma  E_0| \\
 &\approx& 
  p \cdot(|1+\eps \cdot  h_{0}|-1) \cdot E |Z_0+\sigma  E_0| + (1-p) \cdot ( E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|} ),
\end{eqnarray*}
 where $p = P(X_0\neq 0)$.
 
 First we derive lower bounds,
 \[
 E |Z_0+\sigma  E_0|
 \geq E |Z_0| - E|\sigma  E_0| =   E |Z_0| - \sqrt{\frac{2}{\pi}}\sigma,
\]
 \begin{eqnarray*}
 E{|\eps  \cdot h_{(0)}^T X_{(0)}+\sigma  E_0| -E|\sigma  E_0|}&\geq& E{|\eps  \cdot h_{(0)}^T X_{(0)} | -2 E|\sigma  E_0|} \\
 &=&  E|\eps  \cdot h_{(0)}^T X_{(0)} | -2 \sqrt{\frac{2}{\pi}}\sigma
\end{eqnarray*}
Then we have 
\begin{eqnarray*}
 E D_\sigma 
\geq  E D_0 - (p+2(1-p)) \cdot \sqrt{\frac{2}{\pi}}\sigma.
\end{eqnarray*}

Therefore, in the existence of noise, we don't have exact recovery result, but we would have a lower bound. 
 
 Second, we use the mean of folded Gaussian to compute the condition expectation.
 
 Here, for a fixed $\mu$, we rescale the variance $\sigma' = \sigma/\eps$. Under the assumption $\eps/\sigma<< 1 $, using asymptotic expansion, we can compute the condition expectation 
 \begin{eqnarray*}
   E({|\mu+\sigma'  E_0| -|\sigma'  E_0|}\mid \mu)
 &=& \sqrt{\frac{2}{\pi}}\sigma' e^{-\frac{\mu^2}{2\sigma'^2}}+\mu\left[1-2\Phi\left(-\frac{\mu}{\sigma'}\right) \right] - \sqrt{\frac{2}{\pi}}\sigma'
 \\
 &\approx& -\sqrt{\frac{2}{\pi}}\sigma' {\frac{\mu^2}{2\sigma'^2}}+\mu\sqrt{\frac{2}{\pi}}(-\frac{\mu}{\sigma'}  )
 \\
  &=&- \sqrt{\frac{2}{\pi}}  {\frac{3\mu^2}{2\sigma'}}  
\end{eqnarray*}
The first equality is the formula for the mean of folded Gaussian.
The second equality uses the Taylor expansion of Gaussian c.d.f
\[
\Phi (z)  = \frac{1}{2}+  \frac{1}{\sqrt{\pi}} \left(z-\frac{z^3}{3}+\frac{z^5}{10}-\frac{z^7}{42}+\frac{z^9}{216}-\cdots\right)
\]

 Therefore, for $Z_0$ standard Gaussian,
  \begin{eqnarray*}
 E_X E_{E_0}(|Z_0+\sigma  E_0|) 
  &=&  \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}  
\end{eqnarray*}
 \begin{eqnarray*}
 E_X E_{E_0}({|\eps  \cdot h_{(0)}^T X_{(0)} +\sigma  E_0| -|\sigma  E_0|}) 
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{E_X( h_{(0)}^T X_{(0)})^2 }{2\sigma'}}  
   \\
  &=&-\eps \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2\sigma'}}  
\end{eqnarray*}

Then 
\begin{eqnarray*}
 E D_\sigma 
 &\approx& 
 \eps \left[ p \cdot h_{0} \cdot \sqrt{\frac{2}{\pi}}   \sqrt{1+\sigma^2}    - (1-p) \cdot 3\sqrt{\frac{2}{\pi}}  {\frac{\|h_{(0)}\|^2 }{2(\sigma/\eps)}} \right] .
\end{eqnarray*}



 

==> sec/Projection_set_up.tex <==



\section{Population loss and phase transition}
We first study population loss of the sparse deconvolution problem
 \begin{eqnarray*}
    (\mbox{Population sparse deconvolution}) \qquad  \min_{w\in \reals^k} &    
    E\| w * Y\|_1\\
    \mbox{ subject to }&  v^T w = 1,\\
    &  w\in \cM.
\end{eqnarray*}
\subsection{Population loss of projection pursuit}
Let's first consider the population objective $E|w^T \Phi X|$.

Consider a vector  $w \in \cM$ which is a small perturbation of $w^\star  \in \cM$, where
$w^T \Phi =e_0$. Let $w = w^\star + \eps \delta$ where $\delta \in T_{w^\star} \cM$, the tangent space at $w^\star$. And since $\delta \in T_{w^\star} \cM_1$ is a subspace, we assume the constraint is given by $M \delta = 0$.
Let $h = \Phi^T \delta$, then $   u^T \delta = 0$, where $ v = \Phi u$. We have
\[
    b^T Y = X_0 + \eps \delta^T \Phi X=X_0 + \eps h^T  X = (1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)} .
\]
 where $h_{(0)}$, $X_{(0)}$ are $h$, $X$ without $0$-th coordinate.
 \subsection{Population phase transition}
 We want to study $E D =  E|(1+ \eps h_0)X_0 +  + \eps h_{(0)}^T X_{(0)}| -E|X_0|$.
 
 Then for sufficiently small $\eps$
\begin{eqnarray*}
 E|(1+ \eps h_0)X_0 +  \eps h_{(0)}^T X_{(0)}| -E|X_0| &\approx& 
 (|1+\eps \cdot  h_{0}|-1) \cdot E |X_0| \cdot (1-\eta)+ \eps \cdot  E{|h_{(0)}^T X_{(0)}| } \cdot \eta,
\end{eqnarray*}
 where $p = P(X_0=0)$.
 
 The perturbation increases the objective value 
just in case either $h_{0} > 0$, or in case $h_{0} < 0$ and
\[
          \frac{\eta}{1-\eta} > \frac{| h_{0}| E |X_0|}{ E | h_{(0)}^T X_{(0)} |. }
\]

Now we consider the optimization problem
\begin{eqnarray*}
    (Q_1) \qquad  \min_h&   E | h_{(0)}^T X_{(0)} |\\
    \mbox{ subject to }&  h_{0} = -1, \\
    & h\in \Phi^T T_\beta \cM_1.
\end{eqnarray*}


We know $h = \Phi^T \delta$, then 
\begin{eqnarray*}
    (Q_1) \qquad  \min_\delta &E | \delta^T \Phi_{(0)} X_{(0)} | \\
    \mbox{ subject to }  &\Phi_0^T \delta = -1, \\
     & \delta \in T_\beta \cM_1.
\end{eqnarray*}



Following the quadratic problem reduction, we can related $Q_1$ to the deterministic quadratic problem.

After the study of the general population model, we remark that for convolutional model, $A$ ad $B$ are both generated by the circular or Topelitz matrices from a single vector.





==> sec/ProofResults.tex <==
\begin{proof}[Proof of theorem~\ref{thm:fin_deriv}]
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
 \EEAS
\end{proof}

==> sec/Regularized_Noise.tex <==
\subsection{Regularized convex problems}
\paragraph{Regularized convex problems}
For any $\epsilon>0$, we can find the Lagrangian form  of the constrained problem to define the regularized convex program, where we can find a corresponding $\lambda = \Lambda(\epsilon)$ so that $\frac{1}{2\lambda}$ is the dual variable.
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\zeta}   & |\tilde{w}^T Y -\zeta |+ \frac{1}{2\lambda}((\zeta)^2-\epsilon^2) \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
The convention to use for optimization is to ignorne the constant $-\epsilon^2$, and write the problem as
\[
 \begin{array}{ll}
 \mbox{minimize}_{w,\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2] \\
\mbox{subject to}  
& v^T w =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
  Define soft-threshold operator as 
  \[
  S_{\mu}(x): = \sign (x) (|x| -\mu)_+
  \]
  and define its complement
   \[
  \bar{S}_{\mu}(x): = x-S_{\mu}(x) =  \sign (x)(x- (|x| -\mu)_+) =  \sign (x)\max(|x| ,\mu).
  \]
 \begin{lemma}
 If we partially minimize over $\alpha,$ the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
    \[
 \begin{array}{ll}
\mbox{inf}_{\alpha}   & [|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]   = [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 

\end{array}
  \]
  \end{lemma} 
  
  
 
\begin{proof}
Due to the proximal operator of $\ell_1$ norm,  the minimizer is $\alpha = S_{\lambda}(\tilde{w}^T Y)$, 
The objective can be further simplified to
  \[
 \begin{array}{ll}
&\Expect[|\alpha|+ \frac{1}{2\lambda}(\alpha -\tilde{w}^T Y)^2]\\
=&\Expect[|S_{\lambda}(\tilde{w}^T Y)|+ \frac{1}{2\lambda}(\bar{S}_{\lambda}(\tilde{w}^T Y) )^2]\\
=& [(|\tilde{w}^T Y|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\tilde{w}^T Y| ,\lambda) )^2] 
\end{array}
  \]
 \end{proof} 

Using the data generative model and do change of variable, 
the partially minimized regularized problem is
 \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi}   & \Expect[|(|\psi^T (X+\eta Z )|-\lambda)_+|+ \frac{1}{2\lambda}(\max(|\psi^T (X+\eta Z )| ,\lambda) )^2] \\
\mbox{subject to}  
& u^T \psi =1,
\end{array}
\tag{$P_{1,\lambda}$}
  \]
%   For the regularized problem we optimize over the worst case objective for all $Z$ that $\|Z\|_2\leq 1$,  
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]
%   However, it seems hard to study it directly since its order is similar to $\inf_{\lambda} \sup_{Z: \|Z\|_2\leq 1}  \Expect \inf_{\zeta(\lambda)}$ .)
%   \[
%  \begin{array}{ll}
% \inf_\lambda \mbox{minimize}_{\psi}  \quad \sup_{Z: \|Z\|_2\leq 1} & \Expect[(|\psi^T X+\eta  \psi^T Z|-\lambda)_+ + \frac{1}{2\lambda}(\max(|\psi^T X+\eta  \psi^T Z| ,\lambda) )^2] \\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
%   \]

==> sec/Related_Work.tex <==
\section{Related Work}
Qingyun: Will turn these slides into proper writting latter, just trying to collect all the related reference for now.
\paragraph{Prior work: analysis approach, non-Gaussianity}
  \begin{itemize}
  \item
  Key idea $1$: Find inverse filter $a^{-1}$ so that
$ a^{-1}*y = x $.
\item Key idea $2$: 
If $x$ is non-Gaussian, then $a*x$ is closer to Gaussian. 
\item Find $w\neq 0$  
\[
 \begin{array}{ll}
 \underset{w}{\mbox{maximize}}   & J(w*y)
\end{array}
  \]
\item Non-Gaussianity: $J$ is negative entropy function or normalized $4$-th order cumulant $J(z) = \frac{\|z\|_4^4}{\|z\|_2^4}$ \cite{wiggins1978minimum, donoho1981minimum}
  \item Sparsity: 
  $J(z) = - \| z\|_1/\|z\|_2$,  \cite{gray1979variable,donoho1981minimum,kijko1994seismological}.
  \item varimax norm: $\max_i \frac{|z_i|}{\|z\|_2}$ \cite{cabrelli1985minimum}
\end{itemize}

\paragraph{Prior work: blind equalization for digital signal}
  \begin{itemize}
\item
Digital signal: PAM signaling $\pm 1$ binary signal or QAM signaling with $|x|=1, x\in \complex$ \cite{kennedy1992blind,ding2000fast}. 
\item More general,  $x$ are IID and bounded by $M = \mbox{max}(x_i)$ \cite{vembu1994convex,li2001blind}.
\item 
  Convex Cost Functions in Blind Equalization \cite{vembu1994convex}:
  find $w$ so that $w*a = e_0 = (\ldots,0,1,0, \ldots)$ as minimizer of the ideal convex problem (
 Not computable without knowing $a$!)
  \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   & \| w*a\|_1 
 \\
\mbox{subject to} 
& (w*a)_0 = 1.
\end{array}
  \]  
  
    \item
  When $x$ are IID and bounded by $M = \mbox{max}(x_i)$, using duality, use surrogate objective for $\| w*a\|_1$ as
   \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  \frac{1}{M} E \|w * y\|_\infty 
 \\
\mbox{subject to} 
& \|w*y\|_2 = 1.
\end{array}
  \]
   In \cite{vembu1994convex}, they use projected SGD on $E \|w * y\|_8 $ to approximate $E \|w * y\|_\infty$ .
  
  \item Later, use linear programming to solve $\infty$ norm problem directly \cite{ding2000fast}: 
    \[
 \begin{array}{ll}
 \underset{w}{\mbox{minimize}}   &  E \|w * y\|_\infty
 \\
\mbox{subject to} 
& w_0 = 1.
\end{array}
  \]
\end{itemize}

\paragraph{Prior work: synthesis approach, sparsity}
\BIT
% \item
% Sparse signal has a long history in seismology and communication,
% see \cite{kijko1994seismological}, \cite{vembu1994convex}, \cite{osman1996seismic}, \cite{wang2010seismic}, \cite{romberg2009compressive},\cite{mendelson2016improved} etc.
\item
  Convolutional dictionary learning formulation \cite{bristow2013fast, heide2015fast}, etc.
  \item
  Synthesis blind deconvolution with $2$ norm ball constraint  \cite{zhang2017global,zhang2018structured, kuo2019geometry}, etc.
  \item
  Short $a$ and sparse $x$: 
  \[
 \begin{array}{ll}
 \mbox{minimize}   & \|y-a*x\|_2^2+\lambda \|x\|_1 \\
\mbox{subject to}  & \|a\|_2 = 1.
\end{array}
  \]  
%   \item Only empirical result so far.
%   \item Landscape could be complex.
\EIT

\paragraph{Prior work: synthesis approach, subspace assumption}
\[
 \begin{array}{ll}
 y &= a^0 * x^0\\
 \hat y  &= \hat a^0 \circ \hat x^0
\end{array}
  \]
   \begin{itemize}
  \item  $\hat a^0= D_a c_a$.
  \item $\hat x^0 = D_X c_x$.
  \item $D_X$ is often a complex Gaussian matrix.  
\end{itemize}
% \begin{figure}
%  \includegraphics[width=5cm,keepaspectratio]{figures/subspace.png}
%  \includegraphics[width=5cm,keepaspectratio]{figures/shift2.png}
% \end{figure}
No translation symmetry in this assumption!


Lifting:
 \[
 \begin{array}{ll}
 \hat y &= (D_a c_a) \circ (D_X c_x)\\
 &= \mathcal{D}(c_a c_x^T)
\end{array}
  \]
 $\mathcal{D}$ is a linear operator defined as 
 \[
 \begin{array}{ll}
\mathcal{D}(c_a c_x^T)_i = \mbox{trace}((D_{a,i}D_{X,i}^T)(c_a c_x^T))
\end{array}
  \]
  Rank one matrix $Z=c_a c_x^T$.
   \[
      \hat y =  \mathcal{D}(Z)
  \]
  \begin{itemize}  
  \item Convex optimization  \cite{ahmed2014blind},\cite{ling2015self}, \cite{chi2016guaranteed},\cite{romberg2013multichannel},\cite{lee2017blind} etc.
  \item Non-convex optimization  \cite{li2016rapid}.
\end{itemize}

\paragraph{Projection pursuit  with linear constraint}
We point out that the population problem formulation for sparse blind deconvolution is also the population problem formulation for sparse projection pursuit, which might also be called convex sparse ICA, or convex sparse dictionary learning.
\BEQ
 \begin{array}{ll}
  \underset{\psi \in V}{ \mbox{minimize} }  &  \expect |\psi^T X|\\
 \mbox{subject to}  
&  u^T \psi =1.
\end{array}
\tag{$P_{1,v}$}
\EEQ


In sparse projection pursuit with linear constraint, we observe a matrix $Y_M\in \reals^{n\times M }$, and we know that there exists a ground-truth filter $w^0$, such that $w^{0,T} Y_M = X_M$, $X_M$ satisfy Bernoulli$(p)$-Gaussian model.  

We consider the "projection pursuit" problem.
 \begin{eqnarray*}
    (\mbox{Projection pursuit}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&  v^T w = 1.
\end{eqnarray*}
Here $w$ is in a $k$ dimensional subspace of the double infinite sequence. 


\paragraph{Projection pursuit with sphere constraint}
We comment that the results we derive in the following sections are also applicable to the projection pursuit (orthogonal dictionary learning) problem \cite{bai2018subgradient, sun2016complete, sun2015complete}.
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 = 1.
\end{eqnarray*}
or
 \begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| \tilde{w}^T Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| \tilde{w}^T Y_M\|_2 \geq 1.
\end{eqnarray*}
\begin{lemma}
The population problem is:
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect |\psi^T X|  \\
\mbox{subject to}  
&\Expect |\psi^T X|^2 \geq \Expect (X_0)^2
\end{array}
  \]
is equivalent to the following convex-concave problem
\[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad &\sqrt{\frac{2}{\pi}}\left[\Expect_I \|\psi_I\|_2 \right] \\
\mbox{subject to}  
&\|\psi\|_2^2 \geq 1
\end{array}
  \]
We claim that  it has the same minimizer as the \textbf{ projection pursuit (orthogonal dictionary learning) problem with sphere constraint}.
  \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi} \quad & \Expect_I \|\psi_I\|_2  \\
\mbox{subject to}  
&\|\psi\|_2 = 1
\end{array}
  \]
  which is also equivalent to
   \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect_I \|\psi_I\|_2/\|\psi\|_2 
\end{array}
  \]
  And  also equivalent to
    \[
 \begin{array}{ll}
 \mbox{minimize}_{\psi\neq 0} \quad & \Expect |\psi^T X|/\sqrt{\Expect |\psi^T X|^2} 
\end{array}
  \]
\end{lemma}


Inspired by this formulation, we propose a non-convex (convex objective concave constraint) problem for blind deconvultion:
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_2 \geq 1.
\end{eqnarray*}

Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
\begin{eqnarray*}
    (\mbox{Projection pursuit with sphere constraint}) \qquad  \min&    \frac{1}{M} \| w*Y_M\|_1\\
    \mbox{ subject to }&   \frac{1}{M} \| w*Y_M\|_\infty \geq 1.
\end{eqnarray*}


\paragraph{Infinity norm ball constraint}


Before stating the main theorem and its proof, we make some comments about the formulation.

If we study the population level, 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \expect |\tilde{w}^T Y|\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}$ }
\EEQ
then we only need solve one convex problems
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \expect |\tilde{w}^T Y|\\
 \mbox{subject to}  
&  w_0 =1.
\end{array}
\tag{$P_{e_0}$ }
\EEQ
Since the entry with largest magnitude will automatically be shifted to coordinate $0$ due to shift invariance.


If we want to solve the following non-convex problem with infinity norm ball constraint for finite sample,
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &    \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
    \mbox{ subject to }
    & \|w\|_{\infty}= 1.
\end{array}
\tag{$P_{\infty}^T$}
\EEQ
We can solve the following convex problems, and select the one with minimal objective value. This is equivalent to solve the problem with fixed infinity norm. 
\BEQ
 \begin{array}{ll}
  \underset{w\in V}{ \mbox{minimize} }  &  \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]}\\
 \mbox{subject to}  
&  w_j =1.
\end{array}
\tag{$P_{e_j}^T$ }
\EEQ

\paragraph{Dirac re-parametrization and connection to residual CNN}
When $v = e_0$, we are imposing a constraint that the largest entry of $w$ is $w_0 =1$.  
We can re-parametrize our filter, as $w = \delta_0 + f$, $f_0 = 0$. Then our problem became 
 \begin{eqnarray*}
    \min_{f, f_0 = 0} &    
    \frac{1}{2T+1}\|(e_0 +f)*Y\|_{1,[-T,T]}.
\end{eqnarray*}
Here $f = (f_L, 0, f_R)$, $f_R$ and $f_L$ are in $k$ dimensional subspace of the double infinite sequence with positive and negative support.

Allowing Noise:
\[
 \begin{array}{ll}
 \mbox{minimize}   & \|x\|_ 1+\lambda/2\|Y+f*Y-x\|_2^2\\
\mbox{subject to}  
& f_0 =0,
\end{array}
  \]
  with variables $f\in \reals^k$, $x\in \reals^n$. 
  
 \texbf{General multi-channel approximate version}
\[
 \begin{array}{ll}
 \mbox{minimize}   & \sum_i(\|x^i\|_ 1+\lambda^i/2\|Y+f^i*Y-x^i\|_2^2)\\
\mbox{subject to}  
& f^i_0 =0,
\end{array}
  \]
  with variables $f^i\in \reals^k$, $x^i\in \reals^n$. 
  
\paragraph{Link to CNN}
Partial minimization:(similar to one-layer Residual CNN)
\[
 \begin{array}{ll}
 x^i = S_{1/\lambda^i}(Y+f^i*Y)
\end{array}
  \]
  with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $. 


\texbf{Method $1$: plug-in}
\[
 \begin{array}{ll}
 \mbox{minimize}   & \sum_i(\|S_{1/\lambda^i}(Y+f^i*Y)\|_ 1+\\
 &\lambda^i/2\|Y+f^i*Y-S_{1/\lambda^i}(Y+f^i*Y)\|_2^2)\\
\mbox{subject to}  
& f^i_0 =0,
\end{array}
  \]
  with variables $f^i\in \reals^k$, $x^i\in \reals^n$.   
  
%   Let $C_Y$ be the circulant matrix with first column $Y$, let $\hat Y = F_nY$, where $F_n$ is discrete Fourier transform, $U = \frac{1}{\sqrt{n}}F_n$ as a unitary matrix,
% \[
% C_Y = U^*\mbox{diag}(\hat Y)U.
% \]
% Block coordinate update (alternating): initialize: $ f^i(0) = 0;$.
% \[
%  \begin{array}{ll}
%  x^i(t) &= S_{1/\lambda^i}(Y+f^i(t-1)*Y);\\
%  f^i(t) &= (C_Y^T C_Y)^{-1}[C^T_Y(x^i(t)-Y)+\mu(t) \delta_0^T]\\
%  &= U^*\mbox{diag}(1/(\hat Y))U x^i(t)-\delta_0 
%  + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T\\
%  &= Y^{(-1)}*x^i(t) -\delta_0 + U^*\mbox{diag}(|\hat Y|^{-2})U\mu(t)\delta_0^T
% \end{array}
%   \]
%   with $S_{b}(z) :=\mbox{sign}(z)(|z|-b)_+ $, $\mu(t)$ is the dual variable.

==> sec/Stability_old.tex <==

\paragraph{Finite length approximation by Z-transform truncation }

Let $\gamma>0$, then we define 
\[
\bar a^{\gamma} :=e_0-\gamma a
\]
with Z-transform 
\[
\bar A^{\gamma}(z) :=1-\gamma A(z)
\]
then
\[
 \begin{array}{ll}
1/A(z) &=  \gamma(1-\bar A^{\gamma}(z))^{-1}\\
&= \gamma[ 
\sum_{i=0}^{\infty} (\bar A^{\gamma})^i]
\end{array}
  \]
We can construct an approximation 
$w^{r,\gamma} \in V_{rs, rt} $ of length $r(1+s+t)$ 
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
with Z-transform
\[
 \begin{array}{ll}
W^{r,\gamma}(z) 
&= \gamma[\sum_{i=0}^{r} (\bar A^{\gamma}(z))^i] \\
&= \frac{1-(\bar A^{\gamma}(z))^{r+1}}{A(z)} 
\end{array}
\]
then
\[
a*(a^{-1}-w^{r,\gamma}) 
= *_{r+1} (\bar a^{\gamma})
\]
\begin{lemma}
\[
\|a*(a^{-1}-w^{r,\gamma})\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 
= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
 \]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt\\
&= \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}
\end{array} \]
\end{proof}


First, since:
%   \[
%  \begin{array}{ll}
%  \|\hat{\bar a}^{\gamma}\|_{\infty} \geq \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% Notice that 

\[
 \begin{array}{ll}
 \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2} = (|\hat{\bar a}^{\gamma}|^2(t_0))^{r+1} \geq  \int_{\frac{-1}{2}}^\frac{1}{2}  |\hat{\bar a}^{\gamma}|^{2r+2} dt
\end{array}
\]
We have a natural upper bound as
\[
 \begin{array}{ll}
\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}\leq \|\hat{\bar a}^{\gamma}\|_{\infty}^{2r+2}
\end{array} \]
In the following we give a more accurate calculation of $\|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}$ using Laplace method.
% Then using Parseval’s identity, 
%   \[
%  \begin{array}{ll}
% \|\hat{\bar a}^{\gamma}\|_{2}  = \|\bar a^{\gamma} \|_{2}
%   \end{array}
% \]
% (Here we remark that the Fourier transform and inverse Fourier transform are define as follows so that the there is no constant for Parseval’s identity)
% \[
% \mathcal{F}a(\omega) = \hat{a}(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]
% \[
% (\mathcal{F}^{-1} \hat{a})(n) =  \int_{\frac{-1}{2}}^\frac{1}{2} \hat{a}(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
% \]

%  Since $\|\hat{\bar a}^{\gamma}\|^2_{\infty} \geq
%  \|\hat{\bar a}^{\gamma}\|^2_{\infty} \leq \|\hat{\bar a}^{\gamma_2}\|^2_{2}  = \|\bar a^{\gamma} \|_{2} =  \sin{\theta}$.



\paragraph{Laplace's method}
 \begin{theorem}[Laplace's method]
 \label{Laplace}
  For $\bar a^{\gamma} :=e_0-\gamma a$, $a$ has a length $L$ window of non-zero entries.
 \BIT
 \item
 let $F(t) = |\bar a^{\gamma}(t)|^2$, and let $f(t) := \log F(t) = \log| \hat{\bar a}^{\gamma}|^2$ and $t_0 = \arg\max_{t\in [\frac{-1}{2},\frac{1}{2}]} F(t)$ achieves the global maximum, and let the maximum value be $F_{\max} :=F(t_0) = |\hat{\bar a}^{\gamma}(t_0)|^2$. 
\item
We define the second moment 
%   $M_2\leq \sum_{|k|\leq 2L} k^2$,
  \[M_2: = \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k)\]
  then $M_2$ is finite, upper bounded by $\frac{16}{3}(L+1)^3 \| \bar a^{\gamma}\|_2^2$ and $f$ is twice  differentiable near $t_0$.
%   with $|f''(t_0)|\leq M_2/F_{\max} $.
% \item
%  Assume
%  $F_{\max}<1$.
 \EIT
We have
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2}  
  &= \int_{\frac{-1}{2}}^\frac{1}{2}  \exp((r+1)f(t)) dt  \\
  &=  [(\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0))](1+O(r^{-1})) 
  \\
  &=   [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.
\end{theorem}
\begin{proof}
From optimality $F'(t_0) =0,$ and 
\[
 \begin{array}{ll}
|f''(t_0)| &= |\partial^2 \log F(t_0)| \\
&= \frac{ |F''(t_0)|}{|F(t_0)|} 
\end{array}
\]

For $f$ to be twice  differentiable near $t_0$ with $|f''(t_0)|$, we only need to upper bound 
\[
|F''(t_0)|=|[\hat{\bar a}^{\gamma}]''(t_0)|^2 \leq \sum_k k^2 |[\bar a^{\gamma} ] * [ \tilde{\bar a}^{\gamma} ]|(k).
\]
As
\[
\frac{ M_2}{\|\bar a^{\gamma}\|_2^2}\leq \sum_{|k|\leq 2L} k^2.
\]
and  $a$ is of length $L = 1+s+t$, we know that $\bar a^{\gamma}  *  \tilde{\bar a}^{\gamma} $ is of length at most $2L$, then 
\[
\sum_{|k|\leq 2L} k^2 = 1+\frac{2L(2L+1)(4L+1)}{3}\leq \frac{16}{3}(L+1)^3.
\]

Then $f$ to be twice  differentiable near $t_0$ and
\[
 \begin{array}{ll}
|f''(t_0)| 
&= \frac{ |F''(t_0)|}{|F(t_0)|} \\
&\leq  \frac{ M_2}{F_{\max}}
\end{array}
\]

Now we go back to the main quantity,
 \[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} &= \int_{\frac{-1}{2}}^\frac{1}{2} |\hat{\bar a}^{\gamma}(t)|^{2r+2} dt  \\
  &= \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  
\end{array}
\]
By Laplace's asymptotic method,
 \[
  \begin{array}{ll}
  & \int_{\frac{-1}{2}}^\frac{1}{2} \exp((r+1)f(t)) dt  \\
  =&\sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))
\end{array}
\]
where $O(r^{-1}) = O(\frac{1}{r}) \rightarrow 0$ as $r\rightarrow \infty$.

Combining all the previous bounds, we have
\[
  \begin{array}{ll}
  \|\hat{\bar a}^{\gamma}\|_{2r+2}^{2r+2} 
  &= \sqrt{\frac{2\pi}{(r+1)|f''(t_0)|}}
  \exp((r+1)f(t_0)(1+ O(r^{-1}))  \\
 &= [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
\end{array}
\]
\end{proof}

\paragraph{Stability theorem}
Combing the calculation of expectation, the construction of finite length inverse, the Laplace method calculation, we arrive at our final result.
\begin{theorem} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then provided $p<p^\star - \delta$, we have
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq  [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1}))
 \]
\end{theorem}
\begin{proof}
From previous result, 
 \[
\|a*(w^\star -a^{-1}) \|_2^2  \leq \|a*(w^{r,c} -a^{-1}) \|_2^2
 \]
 and previous the previous construction of $w^{r,c}$, we know that 
 \[
 \|a*(w^{r,c} -a^{-1}) \|_2^2 \leq [\sqrt{\frac{2\pi}{M_2(r+1)}}
  (  F_{\max})^{r+\frac{3}{2}}](1+O(r^{-1})).
 \]
Hence we prove the geometric convergence for any $F_{\max} <1$.
\end{proof}


\paragraph{Sufficient condition for $F_{\max} <1$}
\begin{lemma}
Let
 \[
 \gamma_2 = \arg\min_{\gamma>0} \|\bar a^{\gamma} \|_{2}^2
 \]
 Then $\gamma_2 = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
And
  \[
 \|\bar a^{\gamma_2} \|_{2}^2 = 1- \gamma_2^2 = \sin^2{\theta}
 \]
 
\end{lemma}
\begin{proof}
Using the fact that $a_0 =1$, $\|a\|_2 = \frac{1}{\cos{\theta}}$,
\[
 \begin{array}{ll}
\|\bar a^{\gamma} \|_{2}^2 
&= 1+ \gamma^2 \|a\|_2^2 -2\gamma a_0\\
&= 1+ \gamma^2 \frac{1}{\cos^2{\theta}} -2\gamma \\
&= \frac{1}{\cos^2{\theta}} (\gamma - \cos^2{\theta})^2 + (1-\cos^2{\theta})
\end{array} \]
Hence $\|\bar a^{\gamma} \|_{2}^2 $ is mimimized at $\gamma_2 = \cos^2{\theta}$ with value $1-\cos^2{\theta}=\sin^2{\theta}$.
\end{proof}

Remark:
Is there any way to directly optimize $\|\hat{\bar a}^{\gamma}\|_{\infty}$? Would there be an improvement over optimize 2 norm?

\begin{lemma}
Let $S_a := \sum_{j\neq 0} |a_j|$, 
\[
 \gamma_\infty = \arg\min_{\gamma} \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 \]
 if $S_a<1,$ then  
 \[
 \gamma_\infty = 1
 \]
 and 
  \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]

%  Then $c = \cos^2{\theta}$, where $\cos{\theta}:= \frac{\|a\|_\infty}{\|a\|_2} =\frac{1}{\|a\|_2}$, since $\|a\|_\infty = a_0 = 1$. 
% And
%   \[
%  \|\bar a^{c} \|_{2}^2 = 1- c^2 = \sin^2{\theta}
%  \]
 
\end{lemma}
\begin{proof}
 Since
 \[
 \begin{array}{ll}
|\hat{\bar a}^{\gamma}(t)|^2
 &=  |\bar A^{\gamma}(e^{2\pi i  t})|^2  \\
 &= |1-\gamma A(e^{2\pi i  t})|^2 \\
 &= (1-\gamma A(e^{2\pi i  t}))(1-\gamma A(e^{-2\pi i  t})) \\
 &= 1 + \gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))
 \end{array} \]

 \[
 \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{\gamma}(t)|^2
 = 1 + \max_{t\in [\frac{-1}{2},\frac{1}{2}]} [\gamma^2 | A(e^{2\pi i  t})|^2 -\gamma (A(e^{2\pi i  t})+ A(e^{-2\pi i  t}))]
 \]
Since the coefficient $a_i$ are all really, we check different $t.$
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(0)|^2
  &= |1-\gamma (\sum_j a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} a_j)|^2
  \end{array}
 \]
 
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(\frac{1}{2})|^2
  &= |1-\gamma (\sum_i (-1)^{|j|} a_j)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (-1)^{|j|}  a_j)|^2
  \end{array}
 \]
 \[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2
  \end{array}
 \]
then
\[
  \begin{array}{ll}
  |\hat{\bar a}^{\gamma}(t)|^2
  &= |1-\gamma (\sum_j (e^{-j 2\pi i  t}) a_i)|^2\\
  &= |(1-\gamma) + \gamma(\sum_{j\neq 0} (e^{-j 2\pi i  t}) a_i|^2\\
  &\leq |(1-\gamma) + \gamma S_a|^2
  \end{array}
 \]
 if $S_a<1,$ then
 \[
  \begin{array}{ll}
  \min_\gamma |(1-\gamma) + \gamma S_a|^2 =  |S_a|^2<1.
  \end{array}
 \]
 Therefore if $S_a<1$,  $\gamma_\infty =1,$ and 
 \[
 F_{\max} = \max_{t\in [\frac{-1}{2},\frac{1}{2}]} |\hat{\bar a}^{1}(t)|^2 \leq |S_a|^2<1
 \]
\end{proof}

Remark: from this paragraph, we see upper and lower bound for $F_{\max}$, by choosing $\gamma =1,$ we have
\[
F_{\max}   \leq |S_a|^2
\]
also, we see that
\[
F_{\max}   \geq  \|\bar a^{1} \|_{2}^2 
=  \frac{1}{\cos^2{\theta}} -1 = \tan^2{\theta}
\]
So a natural consequence is that 
\[
\tan^2{\theta}   \leq |S_a|^2
\]
If $S_a<1$, we need $\tan^2{\theta}<1$, therefore $\theta<\frac{\pi}{4}$.

\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

For $\gamma\in (0,1)$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
\[
\|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
=  (1-\gamma_2)^2 + (\gamma_2 s)^2 
= \frac{s^2}{1+s^2}
\]
And in this case,
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty
&= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
&=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
 \end{array} \]
 
 Therefore, 
 \[
  \begin{array}{ll}
\||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
 \end{array} \]

==> sec/backup.tex <==
\begin{proof}
In the following proof, for clarity, we write $\gamma$ simply as $\gamma$.

Plug in the formula for mean of folded Gaussian \ref{FoldedGaussianMean}, 
we have
\beq
\label{FoldedGaussianMean_Obj}
\Expect|\psi^T X+\mu| =   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \mu \left(1 - 2\Phi\left(-\gamma\right) \right)\right]
\eeq



This is hard to compute, but to give upper and lower bounds, we can leverage a few simple facts:
first, 
 \[
 \begin{array}{ll}
  e^{- \gamma^2/2} &=\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &=  1- \frac{ \gamma^2}{2} + \sum_{n=2}^{\infty} \frac{ \gamma^{2n}}{(-2)^n (n)!}\\
  &\geq  1- \frac{ \gamma^2}{2}
\end{array}
  \] 
Second, the CDF of the standard normal distribution can be expanded by integration by parts into a series:
\[
\Phi( \gamma)=\frac{1}{2} + \frac{1}{\sqrt{2\pi}}\cdot e^{- \gamma^2/2} \left[ \gamma + \frac{ \gamma^3}{3} + \frac{ \gamma^5}{3\cdot 5} + \cdots + \frac{ \gamma^{2n+1}}{(2n+1)!!} + \cdots\right]
\]
where $!!$ denotes the double factorial. 

% (see: https://en.wikipedia.org/wiki/Normal_distribution#Cumulative_distribution_function)


Let $C_\Phi( \gamma^2)$ be a function of $ \gamma$, then it is a composition function with the inner funciton being $ \gamma^2,$ defined as follows: 
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&:= (2\Phi( \gamma)-1)/\left(\frac{ \gamma}{\sqrt{2\pi}}\right) \\
&= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{2^n (n)!}] \\
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&\leq 1
\end{array}
\]
We remark further that
\[
 \begin{array}{ll}
C_\Phi( \gamma^2) 
&= [\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n+1)!!} ]/[\sum_{n=0}^{\infty} \frac{ \gamma^{2n}}{(2n)!!}] \\
&= [1 + \frac{ \gamma^2}{3}+ O( \gamma^4) ]/[1 + \frac{ \gamma^2}{2}+ O( \gamma^4)] \\
&= 1 -\frac{ \gamma^2}{6}+ O( \gamma^4)
\end{array}
\]
% \[
%  \begin{array}{ll}
% C_\Phi( \gamma^2) &:= e^{- \gamma^2/2} \left[1 + \frac{ \gamma^2}{3} + \frac{ \gamma^4}{3\cdot 5} + \cdots + \frac{ \gamma^{2n}}{(2n+1)!!} + \cdots\right]\\
% &= \frac{1}{ \gamma+1}\exp{( -\frac{ ^2}{2})} 
% \end{array}
% \]
Then
 \[
 \begin{array}{ll}
\mu \left(1 - 2\Phi\left(-\gamma\right) \right)
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\\
&= \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} (1-\gamma^2/6 +O(\gamma^4))\\
\end{array}
\] 
Plug in all the fact together
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \exp\{-\gamma^2/2\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&=   \left[ \sqrt{\frac{2}{\pi}} \sigma \{ 1- \frac{\gamma^2}{2} + \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} + \frac{1}{\sqrt{2\pi}}\cdot \mu^2 \frac{1}{\sigma} C_\Phi(\gamma^2)\right]\\
&= \sqrt{\frac{2}{\pi}}   \left[ \sigma 
\{ 1 + (1+\frac{1}{2}\cdot C_\Phi(\gamma^2))\gamma^2 +   \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \}\right]\\
\end{array}
\] 
Define the residual of this expansion as
\[
 \begin{array}{ll}
\mbox{Res}(\gamma^2) &:= \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2 +  \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!} \\
&=    \frac{ C_\Phi(\gamma^2)-1}{2}\cdot \gamma^2  +   \{ \sum_{n=2}^{\infty} \frac{\gamma^{2n}}{(-2)^n (n)!}\} \} \\
&=    \frac{-1}{12} \gamma^4  +   \frac{\gamma^{4}}{(-2)^2 (2)!} + O(\gamma^6)\\
&=    \frac{1}{24} \gamma^4   + O(\gamma^6)\\
\\
&\geq 0
\end{array}
\] 
We observe that it is only a function of $\mu^2$ and $\psi$, and when $\gamma^{2}\rightarrow 0$, the residual $\mbox{Res}\rightarrow 0$:
\[
 \begin{array}{ll}
\lim_{|\gamma|\rightarrow 0}\mbox{Res} &:= 0
\end{array}
\] 

Then we give an lower bound:
\[
 \begin{array}{ll}
\Expect|\psi^T X+\mu| 
&= \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]+   \mbox{Res}\\
&\geq \sqrt{\frac{2}{\pi}}\left[  \sigma + \frac{3}{2}\mu^2  \sigma^{-1}\right]
\end{array}
\] 


\end{proof}








%   For $\sigma_2 =0$. If there is $C(\phi^*) \in [C_-, C_+]$ so that
%     \[
%     \begin{array}{ll}
%   \Expect_I \cos[\angle( (I\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]
%   &= C(\phi^*) \cos[\angle( (1\cdot+\sigma_1)(e_0 +t\phi^*), \phi^*)]\\
%  &= C(\phi^*) \cos[\angle( (e_0 +t\phi^*), \phi^*)]
% \end{array}
%   \]
%   then 
  
%   \[
%     \begin{array}{ll}
    
%   \langle  \Expect_I \partial F_I( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle
%   &=  \Expect_I \langle N((I\cdot+\sigma_1+\sigma_2  a^{-1}*)(e_0 +t\phi^*) ), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\
% &= C(\phi^*) \langle  \partial  F_1( t\phi^*), \frac{\phi^* }{\|\phi^*\|_2 }  \rangle\\

% \end{array}
%   \]






% Let $f$ be a extended real-valued convex function $f:\reals^d \rightarrow [-\infty, \infty]$, $\imath_{K}$ be the indicator function over $K$, that is, the function that returns $0$ if the argument belongs to $K$ and $+\infty$ otherwise.
% We define convex conjugate of $f$ as $f^*:\reals^d \rightarrow [-\infty, \infty]$, where
% \[
% f^{{*}}(u) := \sup_{x \in \reals^d} \left \{ \langle u , x \rangle - f \left( x \right) \right\}\,,\qquad u \in \reals^d\,.
% \]
% From Fenchel's duality theorem, we have the following lemma
% \begin{lemma}[duality lemma]

% \begin{align}
% \min_{x \in K} f(x) &= \min_{x \in \reals^d} f(x) + \imath_{K}(x)\\
%  &= \min_{x \in \reals^d} \max_{u \in \reals^d}\Big\{\langle x, u\rangle - f^*(u)\Big\} + \imath_{K}(x)\\
% &= \max_{u \in \reals^d}\min_{x \in \reals^d}\Big\{ \imath_{K}(x) + \langle x,u\rangle\Big\} - f^*(u)\\
% &= \max_{u \in \reals^d} (-\imath_{K}^*(-u) - f^*(u)),
% \label{eq:pd_relationship}
% \end{align}
% \end{lemma}  







% \paragraph{Primitive calculation}  
% Notice that
% \[
%  \begin{array}{ll}
%   \sup_{\|Z\|_2\leq 1} \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ] ] 
% = \|\psi\|_2
% \end{array}
%   \]
% We could focus on 
% \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Then we study the difference,
% \[
%  \begin{array}{ll}
% \Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|
% &= \Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )| \\
% % &= \Expect [\mbox{sign}\left((e_0 +\phi)^T (I\cdot G+\eta Z )\right) (e_0 +\phi)^T (I\cdot G ) \\
% % - \mbox{sign}\left( (e_0)^T (I\cdot G+\eta Z )\right) (e_0)^T (I\cdot G )]+ \eta \Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]
% % &= \sqrt{\frac{2}{\pi}} \cdot \Expect_I \|(I\cdot+\sigma_1+\sigma_2  a^{-1}*)\psi\|_2
% \end{array}
%   \]

% Let $\eta$ be very small and we study the asymptotic behavior.
% We want to study
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% =& \sup_{\|Z\|_2\leq 1}[\Expect|\psi^T (I\cdot G+\eta Z )|-\Expect|e_0^T (I\cdot G+\eta Z )|] \\
% =& \sup_{\|Z\|_2\leq 1}[\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T (I\cdot G )]-\Expect [\mbox{sign}((I\cdot G+\eta Z )_0)  (I\cdot G )_0] 
% \\
%  &+ \eta (\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ])] 
% \end{array}
%   \]
%  We use some crude approximation to gain insight:
  
%  If $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(e_0^T (I\cdot G+\eta Z ))$, then
%  \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}(\Expect [\mbox{sign}(\psi^T (I\cdot G+\eta Z )) \psi^T Z ]- \Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  Z_0 ]) \\
% =& \sup_{\|Z\|_2\leq 1}\Expect [\mbox{sign}( (I\cdot G+\eta Z )_0)  \phi^T Z ]\\
% =& \|\phi\|_2
% \end{array}
%   \]
% On the other hand, if  $\mbox{sign}(\psi^T (I\cdot G+\eta Z )) = \mbox{sign}(\psi^T (I\cdot G )) $ for all $\psi$, then
% we could use the formula
%   \[
%  \begin{array}{ll}
% \Expect [\mbox{sign}(\psi^T (I\cdot G)) \psi^T (I\cdot G) ]
% = \sqrt{\frac{2}{\pi}} \cdot  \Expect_I \| \psi_I\|_2
% \end{array}
%   \]
% So we could have an crude approximate as 
% \[
%  \begin{array}{ll}
%  & \sup_{\|Z\|_2\leq 1}[\Expect|(w*Y)_0|-\Expect|(a^{-1}*Y)_0|]\\
% \approx & \sqrt{\frac{2}{\pi}} \cdot  \Expect_I [\| (e_0+\phi)_I\|_2-\| (e_0)_I\|_2]
%  + \eta \|\phi\|_2
% \end{array}
%   \]
  

==> sec/concentration.tex <==
\section{Old concentration results}
% \subsection{Guarantee of inverse kernel recovery}
% \subsubsection{Random model } 
% We first study the following finite sample setting.
% \begin{itemize} 

%   \item We sample a length-$n$ observation $y\in \reals^n$,  
%   from the circular convolution model 
%   \[ 
%   y =  a*x.
%   \]
 
%  \item  Here $x\in \reals^n$ is a random vector where each entry $x_{i} = \Omega_{i} G_{i}$, where  $\Omega$  i.i.d. sampled from Bernoulli distribution $\mbox{Ber}(p)$ and $G$  i.i.d. sampled from Gaussian random variable with variance $1$, $\Omega$ and $G$ are independent.   We define $|S| = \sum_i \Omega_{i}$. 
 
%  We assume $1/4 \geq p\geq 2/n$.

%   \item The kernel $a$ has an inverse filter $w^0$ of length $k+1$, such that 
%   \[
%   a*w^0 =e_1,
%   \]
%   where $*$  is circular convolution of  length $n$.
  
%  To fix the scale and shift of $w^0$, without loss of generality, we assume $w^0_{j} =1$ for some $j$, and it is the entry with largest absolute value. 
 
%   Let $C(a),C(w^0)$ to be the circulant matrix of size $n$ by $n$ generated by $a, w^0$ after zero-padding. Then $C(w^0)= C(a)^{-1}.$  
  
%   We define the condition number of $C(a)$ to be $\delta_a$, which is the ratio of the largest absolute eigenvalue over the smallest absolute eigenvalue.
  
  
% \subsubsection{Perturbation }  
% Consider perturbed filter $w = w^0 + \epsilon v$, and 
% we define 
% \[
% h=  a*v  = a*(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|x+\epsilon h*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*v, v_0 = 1\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 


% %   \item  We define the autocorrelation of $a$ as 
% % \[
% % R(a) = a * \bar{a},
% %  \]
% %  where $\bar{a}$ is the flipped version of $a$.
% % And the $d$-th element of $R(a)$ is the  
% % $d$-lag correlation of $a$ as 
% % \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d},
% %  \]
% %  where we assume periodic boundary condition, $a_{n+d} = a_d$.
% % %  \js{What about the boundary? My understanding is R(a) is a length $n$ vector defined as $R(a) = a \cconv a(-)$ (here $a(-)$ is $a$ flipped), i.e., $R(a)$ is the autocorrelation sequence defined based on circulant convolution. Now $R_d(a)$ is the $d$-th element in this sequence. An alternative way is $R(a) = aC(a)$. }
 
% % Clearly $R_0(a) =  \|a\|_2^2$.
% %  We assume that there is a constant $C$ such that for all $d\neq 0$, 
% %  \[
% % R_d(a) = \sum_{j=1}^n a_{j}a_{j+d} \leq C/n^{\beta_{d}}\|a\|_2^2
% %  \]
% % where $\beta_d\geq 1/2$. 


% \end{itemize}
% \begin{theorem} 
% Under the above assumption,
% there exists constant $C_0$, $C$, for all $n>C k^2 \log^2(kp)$, 
% the minimizer $w^*$ of the optimization problem 
% \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|w*y\|_1\\
% \mbox{subject to}  
% & w_{k+1}=1,\\
% & w \in \reals^{k+1},
% \end{array}
%   \]
% equals $w^0$  with probability $1-\delta$, where 
% \[
%  \begin{array}{ll}
% \delta 
% \leq \exp\left( -C_0 \delta_a^2 k\log(kp)\right)
% \end{array}
% \]
% % \js{I understand this is probably not the final form yet ... What is the $\epsilon$ here? Why setting $n$ to be on the complexity order stated above can make this $\delta$ ``small'' (I suppose this depends on what we set $\epsilon$)?}
% convergences to zero asymptotically as $k$ grows to infinity.

% % \js{(1) $p$ is an important parameter for the problem, should be brought in the problem statement. (2) About $\delta$: mathematical signal processing and relevant communities often asks for the more concrete rate. When people in these fields say something holds with high probability, there's a precise meaning: decay of $\delta$ cannot be slower than $O(n^{-1})$. As a counter-example, $O(\log^{-1}n)$ is too slow to be considered as the event holding with high probability. }
% \end{theorem}
% \begin{proof} 
% To prove the theorem, we do a change of variable 
% \[
% h=  a*w- e_1 = C(a) w- e_1 = C(a)(w-w^0) = C(w^0)^{-1}(w-w^0),
% \]
% then the optimization problem is:
%  \[
%  \begin{array}{ll}
%  \mbox{minimize}   & \|(h+e_1)*x\|_1\\
% \mbox{subject to}  & h \in\mathcal H.
% \end{array}
%   \]
% Here $h$ is the variable in the $k$ dimensional subspace $\mathcal H$. 
% \[
% \mathcal H = \{h = a*w- e_1 =  C(w^0)^{-1}(w-w^0)\}.
%  \]
% Since $w, w^0 \in \reals^{k+1}$, and $w_{k+1} = w^0_{k+1} =1$, $w-w^0$ is in a $k$-dimensional subspace, therefore $\mathcal H$ is a $k$-dimensional subspace. We define 
% $v$ as the length $n$ vector zero-padded from $w-w^0$.

%  \[
%   \begin{array}{ll}
%   (h*x)_i 
%   &= \langle C(h)_i, x\rangle \\
%   &= \langle C(a^{(i)}) v, x\rangle
%   \end{array}
%   \]
%   where $a^{(i)}=(a_i, a_{i+1}, \ldots, a_n, a_1,\ldots, a_{i-1})$ is the vector circular-shifted $i-1$ steps  from $a$.
%   Here for convenience, we define $\langle C(h)_i, x\rangle$ as $ C(h)_i^T x$ to represent the inner product. 

% Without loss of generality, we assume $\|v\|_2=1$.
  

% We define the difference 
% \[
%  \begin{array}{ll}
% D &= \|(h+e_1)*x\|_1 - \|x\|_1.
% \end{array}
%   \]
% To prove the theorem, we need to prove that the difference $D$ is non-negative.

% Since the problem is convex, we only need to prove that the difference is non-negative  for small perturbation.







% % We define $S$ to be the support of $x$.
% % \[
% %  \begin{array}{ll}
% % D &=  \|h*x+x\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|(h*x)_{S^c}\|_1 - \|x\|_1\\
% % &=  \|x+(h*x)_{S }\|_1+\|h*x-(h*x)_{S}\|_1 - \|x\|_1\\
% % &\geq  \|h*x\|_1- 2\|(h*x)_{S}\|_1
% % \end{array}
% %   \]
% % Furthermore, 
 




% %  \[
% %  \begin{array}{ll}
% % |\langle C(a^{(i)}) v, x\rangle| \geq  u |\langle v, x\rangle|
% % \end{array}
% %   \]
% % since the smallest absolute value of the absolute eigenvalue of the circulant matrix
% % $ C(a)$ is  $u = |\hat a|_{\min}$.

% Now
% \[
%  \begin{array}{ll}
% D
% &\geq \|h*x\|_1- 2\|(h*x)_{S}\|_1\\
%   &= \sum_{i\in S_j^c} |\langle C(a^{(i)}) v, x\rangle|-\sum_{i\in S_j} |\langle C(a^{(i)}) v, x\rangle|
% \end{array}
%   \]
  
% Let's calculate the expectation 
%   \[
%  \begin{array}{ll}
% \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% &=   \expect \left[ (n-2|S|)  |(h*x)_0| \right] \\
%  &\geq 
% n/2 \expect |(h*x)_0|  
% \end{array}
%   \]
% For a generic $h\in\reals^n$, we have a lower bound on expectation using $\|h\|_2$.
% Let $G_{j}=\mbox{sign}(G_{j}) |G_{j}|$, then $\mbox{sign}(G_{j})$ are IID Rademacher ( $\pm 1$) random variables.
%   \[
%  \begin{array}{ll}
% & \expect  \|h*x\|_1\\
% =& n \expect |(h*x)_0|\\  
%  =& n \expect  |\sum_{j=1}^n h_j\Omega_{j} G_{j}|\\
%  =& n \expect   |\sum_{j=1}^n h_j \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
%  \geq&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j\Omega_{j}G_{j})^2}\\
%  =&   \frac{n}{\sqrt{2}} 
%  \expect    \sqrt{\sum_{j=1}^{n} (h_j x_{j})^2}\\
%  \geq&   \frac{n}{\sqrt{2}}   \sqrt{\sum_{j=1}^{n} p h_j^2}\\
%   =&   \frac{n\sqrt{p}}{\sqrt{2}}   \| h\|_2 
% \end{array}
%   \]  
% The first inequality is the
% Khintchine inequality.
% The second inequality is Jensen's inequality, because the function is a convex function of $x$,  
% and the second moment of each entry of $x$ is
% \[ \expect(x_{i})^2  = \expect(\Omega_{i})^2(G_{i})^2=\expect(\Omega_{i})\expect(G_{i})^2 = p.\]
% % We can derive another bound using $h=C(a)v$.
% % \[
% %  \begin{array}{ll}
% % \expect D  &\geq  \expect \left[  \|h*x\|_1- 2\|(h*x)_{S_j}\|_1 \right] \\
% % &=   \expect \left[ (1-2|S|/n) \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle|\right] \\
% %  &\geq 
% % 1/2 \expect \left[\sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right] \\
% % \end{array}
% %   \]
  

% %   We want to find the optimal objective value of the problem
% % \[
% %  \begin{array}{ll}
% %  \mbox{minimize}   &  \expect \left[ \sum_{i=1}^n|\langle C(a^{(i)}) v, x\rangle| \right]   \\
% % \mbox{subject to}  & \|v\|_1 =1;
% % \end{array}
% %   \]
% % Using the fact that the objective is a convex function of $v$, and is invariant to permutations,  we know that this function is minimized at the point
% %   $(\frac{1}{ k},\ldots,\frac{1}{ k} )$,
% %    \[
% %  \begin{array}{ll}
% %  &  \expect \left[  \sum_{i=1}^n |\langle C(a^{(i)}) v, x\rangle| \right]  \\
% %  \geq&  \frac{1}{ k} \expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} G_{j}| \\
% %  =& \frac{1}{ k}\expect  \sum_{i=1}^n |\sum_{j=1}^n (\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
% %  \geq&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)\Omega_{j}G_{j})^2}\\
% %  =&   \frac{1}{k\sqrt{2}} 
% %  \expect   \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} ((\sum_{t=1}^{k} |a_{i-t+j}|)x_{j})^2}\\
% %  \geq&   \frac{1}{k\sqrt{2}}  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n} p(\sum_{t=1}^{k} |a_{i-t+j}|)^2}\\
% %   =&   \frac{\sqrt{np}}{\sqrt{2}}    \sqrt{(\sum_{i=1}^{n} |a_{i}|)^2}\\
% %    =&   \frac{\sqrt{np}}{\sqrt{2}}   \| a\|_1 
% % \end{array}
% %   \]


 

% As a summary of all the inequalities, we get a lower bound on $\expect D $:
% \[
% \expect D  \geq    \frac{\sqrt{p}}{2^{3/2}}  n \| h\|_2.
% \]
% and
% \[
% \expect D  \geq   \frac{ \sqrt{np} }{2^{3/2}}   \| a\|_1\| v\|_1
% \]

% Also we have bound on the second moment.
% First we define the $s$-lag correlation of $a$ to be 
% \[
% R_s(a) = \sum_{t=1}^n a_{t}a_{t+s},
% \]
% and define the sum of the $s$-lag correlation of $a$ as  
% \[
% \begin{array}{ll}
% R(a) = \sum_{s=1}^{n-1}  R_{s}(a) = \sum_{s=1}^{n-1} \sum_{t=1}^n a_{t}a_{t+s}.
% \end{array}
% \]

% \[
% \begin{array}{ll}
% \mbox{Var} \left(  \|h*x\|_1 \right)
% &= \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x v^T C(a^{(i_2)})^T x|\right)\\
% &=   \left(\sum_{i_1\neq i_2} \expect |v^T C(a^{(i_1)})^T x x^T C(a^{(i_2)}) v|\right)\\
% &\leq   p\left(\sum_{i_1\neq i_2}|v^T C(a^{(i_1)})^T C(a^{(i_2)}) v|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}   (\sum_{t=1}^n a_{t}a_{t+(i_2-i_1)})|\sum_{r_1=1}^k\sum_{r_2=1}^k v_{r_1}v_{r_2}|\right)\\
% &\leq  p \left(\sum_{i_1\neq i_2}  R_{i_2-i_1}(a) \|v\|_2^2 \right)\\
% &= p   n R(a)\|v\|_2^2
% \end{array}
% \]

% And we have bound on the absolute value,
% % let  $\|X_j\|_{\infty} = \tau$, where $\tau\leq 4$ with probability 
% % $1-\Phi(4)$ for $\Phi$ the Gaussian c.d.f, 
% % and since 
% \[
%  \begin{array}{ll}
% | \langle C(a^{(j)}) v, x\rangle|
% &=  | \sum_{i=1}^n  \sum_{t=1}^k a_{i-t+j} v_t x_{i}|\\
% &\leq   \|a\|_{\infty}|\sum_{t=1}^k v_t|| \sum_{i=1}^n x_{i}|\\
% &\leq  \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| \\
% &\leq    \|a\|_{\infty} \|v\|_1 | \sum_{i=1}^n x_{i}| 
% \end{array}
% \]
% with probability $1-\exp{(-Cn)}$, 
% \[
%  | \sum_{i=1}^n x_{i}| \leq 8\tau \sqrt{n},
% \]
% then, 
% \[
%  \begin{array}{ll}
% |\langle C(a^{(j)}) v, x\rangle|
% &\leq     8 \sqrt{n} \|v\|_1 \|a\|_{\infty} \tau 
% \end{array}
% \]


Now we need to derive a concentration inequality on $D$. 
We focus on deriving a concentration inequality on $\|h*x\|_1$, and the concentration inequality 
on  $\|(h*x)_S\|_1$ can be derived similarly.

We remark that $ \|h*x\|_1 =\sum_{j=1}^n |h^{(j),T} x|= \sum_{j=1}^n |\langle C(a^{(j)}) v, x\rangle|$, 
if they are independent random variables, we can bound the deviation of $ \|h*x\|_1$ from its mean
using tail bounds via Bernstein’s inequality, by using the previous two bound on
variance and absolute value. 
This is the strategy to derive concentration inequality in dictionary learning\cite{luh2016dictionary,blasiok2016improved}.
This is also the strategy to derive concentration inequality for multiple observation blind deconvolution setting, since there are independence across different observations.

However, here due to the nature of the convolution, we cannot directly apply Bernstein’s inequality. There are additional dependencies that cause technical difficulties. 

% We need to derive concentration via decoupling, by controlling the moments.
Therefore, we use the dual representation of the $1$-norm and use Talagrand-Bernstein’s inequality on supreme of random function to derive concentration.
We put this part of the proof in the following lemma, since they are technical and they could be of independent interest for other problems with dependency structure. 




From the lemma, if we let $Z = \|h*x\|_1$, then we have 
 \[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&= \prob \left[  |Z- \expect Z | > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.

From the previous calculation, we recall that we have a lower bound on expectation 
$ \expect \|h*x\|_1$,
\[
\expect \|h*x\|_1\geq    \sqrt{\frac{p}{2}}  n \| h\|_2 
\] 
\[
\expect Z = \expect \|h*x\|_1 \geq  \sqrt{\frac{p}{2}}  n \| h\|_2
\]
  









Now we calculate $\sigma^2, K$:
 \[
  \begin{array}{ll}
\sigma^2 &=\expect \langle w, C(h)x \rangle^2,\\
&=\expect (C(h)^* w)^T xx^* C(h)^* w  \\
&\leq  p \|C(h)^* w\|_2^2\\
&=p \langle w, C(h)C(h)^* w \rangle 
\end{array}
  \]  
Let $C(h)=UD(\hat{h})U^*$ be the eigen-decomposition, where $U$ is the unitary Fourier matrix, $D(\hat{h})$ is the diagonal matrix with $\hat{h}$ as its diagonal entries. Then using $h=a*v$, $\hat{h}=\hat{a}\hat{v}$, we have
      \[
  \begin{array}{ll}
(C(h)C(h)*) 
&=   UD(\hat{h})U^* U D(\hat{h})^* U^* \\
&=  UD(|\hat{h}|^2) U^* \\
&=  UD(|\hat{a}\hat{v}|^2) U^*. \\
\end{array}
  \] 
Now we have
 \[
  \begin{array}{ll}
\sigma^2 &\leq 
 p \langle w, C(h)C(h)^* w \rangle \\
&= p  \langle w,  UD(|\hat{a}\hat{v}|^2) U^* w \rangle \\
&= p  \langle U^* w,  D(|\hat{a}\hat{v}|^2) U^* w \rangle 
\end{array}
  \] 
Let $\tilde{w} = \langle U^* w $, using the fact that $\|w\|_{\infty}\leq 1$, we have  $\|\tilde{w}\|_{\infty}\leq 1$, therefore,
 \[
  \begin{array}{ll}
\sigma^2 &\leq  p  \langle \tilde{w},  D(|\hat{a}\hat{v}|^2) \tilde{w} \rangle \\
&=  p  \sum_{i=1}^n \tilde{w}_i^2 |\hat{a}_i\hat{v}_i|^2)  \\
&\leq  p  \sum_{i=1}^n  |\hat{a}_i\hat{v}_i|^2 \\
&\leq  p  \max_{i=1}^n |\hat{a}_i|^2\sum_{i=1}^n  |\hat{v}_i|^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 \|v\|_2^2 \\
&=  p  \max_{i=1}^n |\hat{a}_i|^2 
\end{array}
  \] 
  
  Now we derive the absolute value bound. First, since $x_i$ are iid sampled from the product of Bernoulli random variable and standard Gaussian, the supreme of the absolute value $\tau = \max_i |x_i|$ is upper bounded by the  supreme of standard Gaussian, which is less than $  2\log^{1/2} n$ with probability $1-\exp(-Cn^2)$. In the following, we only consider this case and assume $\tau \leq 2\log^{1/2} n$ and add the tail probability into the tail probability in the concentration inequality.
  
 Using other side of Khintchine inequality, we have
  \[
 \begin{array}{ll}
&  |(h*x)_i|\\
 =&  |\sum_{j=1}^n h_{i-j} \Omega_{j} |G_{j}|\mbox{sign}(G_{j}) |\\
\leq&  
  \sqrt{\sum_{j=1}^{n} (h_{i-j} \Omega_{j}|G_{j}|)^2}\\
 \leq&  \tau  \sum_{i=1}^n \sqrt{\sum_{j=1}^{n}  h_{i-j}^2}\\
   =&   \tau  \| h\|_2 
\end{array}
  \]  
Therefore, we can take $K=  \tau  \| h\|_2  .$
%    \[
%   \begin{array}{ll}
%  |(C(h)^T w)_i x_i|
% &\leq  \tau |(h^{(i),T} w|\\
% &=  \tau |\sum_{j=1}^n h_{i-j}  w_{j}|\\
% &\leq  \tau \|h\|_1.
% \end{array}
%   \]  

 
%  Notice 
%   \[
%   \begin{array}{ll}
% \|h\|_1 \leq \|h\|_2 n^{1/2}.
% \end{array}
%   \]  
%   We have $K\leq  \tau \|h\|_2 n^{1/2} .$
%  Using Young's inequality
%     \[
%   \begin{array}{ll}
% K= \tau \|h\|_1
% \leq  \tau \|a\|_1\|v\|_1 .
% \end{array}
%   \]   











% Moreover, for $1$-norm of $\|h\|_1$, we have Young's inequality
%     \[
%   \begin{array}{ll}
%   \|h\|_1
% \leq  \|a\|_1\|v\|_1 .
% \end{array}
%   \]     

We point out that the eigenvalues of $C(a)$ is the Fourier transform of $\hat a$ of $a$, which is the 
the entry-wise inverse $1/\hat w^{0}$. And the singular values of $C(a)$ are the absolute values $|\hat a|$. 
% \[
%  \begin{array}{ll}
% \min_i |\hat a_i| = \min_i \frac{1}{ |\hat w^0_i|} 
% =\frac{1}{\max_i |\hat w^0_i|} = u.
% \end{array}
% \]
Therefore, using the fact that $\|v\|_2=1$,
\[
 \begin{array}{ll}
 \min_i |\hat a_i| \leq \|h\|_2 =  \|C(a)v\|_2 \leq \max_i |\hat a_i| 
\end{array}
  \]
  
Then the condition number of $C(a)$ can be represented as $\delta_a =   \max_i |\hat a_i|/\min_i |\hat a_i|$.



Overall, for $Z = \|h*x\|_1$, we have $\expect Z \geq \sqrt{\frac{p}{2}}  n \| h\|_2$, we choose $t = \sqrt{\frac{p}{2}}  n \| h\|_2$. Since 
 \[
  \begin{array}{ll}
 \prob \left[  |Z- \expect Z | > t   \right] 
\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right),
\end{array}
  \]  
we calculate
\[
  \begin{array}{ll}
 &  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\\
=&  -\frac{1   }{2(\sigma^2/t^2+K(2\expect Z+t/3)/t^2)}\\
\leq &  -\frac{1   }{2(\sigma^2/t^2+K(2+1/3)/t)}\\
 \end{array}
  \]  
% It can be viewed as $ -\frac{1   }{4} $ multiple the harmonic average of 
% $t^2/\sigma^2$ and $t^2/ K(2\expect Z+t/3)$. We find 
Now, we calculate both terms on the denominator,
  \[
  \begin{array}{ll}
   \sigma^2/t^2 &\leq (p  \max_{i=1}^n |\hat{a}_i|^2)/( \sqrt{\frac{p}{2}}  n \| h\|_2)^2 \\
  &\leq 2\max_{i=1}^n |\hat{a}_i|^2)/(\min_{i=1}^n |\hat{a}_i|^2 n^2 \\
   &\leq 2\delta_a^2/ n^2 ,
 \end{array}
  \]  
   \[
  \begin{array}{ll}
  (2+1/3)K/t 
 &\leq  \frac{7}{3}\tau  \| h\|_2 /\sqrt{\frac{p}{2}}  n \| h\|_2\\
  &\leq \frac{7\sqrt{2}}{3}\tau  /\sqrt{p}  n \\
   &\leq \frac{7}{2}\tau  /\sqrt{p}  n 
 \end{array}
  \]  
  
 As we discussed before, since $\tau$ is the maximum of IID Gaussian random variable, 
 $\tau \leq C_1 \log^{1/2}(n)$ with probability $1 - \exp(-C_2 n^2)$ for $C_1$ large enough.
 
And from the assumption we have $ \delta_a \leq C_0 n^{1/2}/ \log^{1/4}(n)$.
  
Therefore, 
\[
  \begin{array}{ll}
& \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7\tau  /\sqrt{p}  n  } \right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-1   }{ 4\delta_a^2/ n^2  + 7 C_1 \log^{1/2}(n)  /\sqrt{p}  n  } -C_2 n^2\right)\\
&\leq   \exp\left( \frac{-n   }{  \log^{1/2}(n) (4C_0+  C_3 \sqrt{p})} -C_2 n^2 \right)\\
&\leq   \exp\left( \frac{- C n   }{  (p\log(n))^{1/2}}  \right)
 \end{array}
  \]  
  
  

  
  
  
  
  
  
  
  
% Here the two quantity we care are
% \[
% \langle h, h^{(d)}\rangle / \|h\|_2^2
% \]

% \[
%  \|h\|_1 / \|h\|_2
% \]
\begin{proof}
In the lemma below, we use a covering argument to give a union bound for $v\in B_k=\{v
\in\reals^k\mid \|v\|_2=1\}$. 
We want to cover $B_k$ with $\epsilon$ balls. From classical covering argument,
we know that we need at most $|N| = (3/\epsilon)^k$ $\epsilon$ balls to cover $B_k$, and we use symmetrization trick to find the proper $\epsilon$.

Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
  
Since  $n>  k \log(k/p)$, for large enough constant $C$, we showed in the lemma that there exist a positive constant $C_0$, 
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq  \exp\left(  k\log(3\tau \sqrt{n}np \|a\|_1) - \frac{ C_6 n   }{  (p\log(n))^{1/2}}\right) \\
&\leq    \exp\left( k(\log(3\tau)+\log(\|a\|_1)+\log(p)+3/2 \log(n)) -\frac{ C n   }{  (p\log(n))^{1/2}}\right) 
\end{array}
  \] 
  
% Now we have a tail bound on $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$, which implies a tail bound on 
% $
% \mathcal{X}_v-\mathcal{X}_{v'}$.
%  For all $v, v'\in B_k$,  
%  \[
%   \begin{array}{ll}
% & \prob \left[ |\mathcal{X}_v-\mathcal{X}_{v'}| > \epsilon  \frac{n^{3/2}\sqrt{kp} }{2^{3/2}}    |\bar a| \right] \\
% &\lesssim   \exp\left( Ck\log(\sqrt{n}np \|a\|_1) - \frac{\epsilon^2 \frac{p}{2 }  n^2 \|h\|_2^2 }
% {2pn  (Cn^{1/2}+2k)+2\tau \|h\|_1 \|h\|_2 \sqrt{\frac{p}{2}}  n  (2+\epsilon/3)}\right)
% \end{array}
%   \]  
%  Then we use theorem $19$ of \cite{blasiok2016improved}, we can deduce the tail bound for supremum of $|\mathcal{X}_v|$.
%  \[
%   \begin{array}{ll}
%  \prob \left(\sup_{v \in B_k} |\mathcal{X}_v| > M + \sqrt{t} D_1 + t D_2\right) < e^{-t}
% \end{array}
%   \] 
% Where
% \begin{align*}
% 	M  & := C_1 (\sqrt{2 p}  \gamma_2(B_k, d_2) + \gamma_1(B_k, d_\infty))\\
% 	D_1 & := C_2 \Delta(B_k, \sqrt{2  p} d_2) \\
% 	D_2 & := C_3 \Delta(B_k, d_\infty)
% \end{align*}
% with $d_2, d_\infty$ being the metrics on $\reals^k$ induced by norms $\ell_2, \ell_\infty$ respectively, and $C_1, C_2, C_3$ are universal constants.

Then bound on $\sup_{v \in B_k} |\mathcal{X}_v|$ would imply the same bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$.
And with this bound on $\sup_{v \in B_k} |\tilde{\mathcal{X}}_v|$, we proved that 
for all $v\neq 0, v \in B_k$, $D>0$ with probability $1-\delta$, where
\[
\delta \leq  \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right)
\]
Therefore, when $n>C_1k^2\log(kp)$, 
$
\delta \leq   \exp\left(  -C_0 \delta_a^{-2} k\log(kp) \right),
$
then $\delta$ converges to zero as $k$ goes to infinity.
\end{proof}





\begin{lemma}
Let $Z = \|h*x\|_1$ where $h \in \mathcal{H}$, then 
 \[
  \begin{array}{ll}
& \prob \left[  Z - \expect Z  > t   \right] \\
&\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
where $\sigma^2\leq  \expect Z^2$, $K\leq \|Z\|_\infty$.
\end{lemma}
\begin{proof}
Using duality of $1$-norm, we know that
\[
\|h*x\|_1 = \sup_{\|w\|_\infty\leq 1}\langle w, C(h)x \rangle
\]
 From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
 for the supreme of functions $\langle w, C(h)x \rangle$, since $\expect \langle w, C(h)x \rangle=0$,
 $ \langle w, C(h)x \rangle\leq K$, 
 \[
 \sigma^2 =\expect \langle w, C(h)x \rangle^2,
 \]
 we have
 \[
  \begin{array}{ll}
 \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
\end{array}
  \]  
\end{proof}
We also remark that the essential concentration inequality that we are trying to derive is the following:
let's consider the case when $x$ is IID standard Gaussian, we define $z = h*x = C(h)x$,
then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,\Sigma(h)),\] where 
\[  \Sigma(h)_{ij} = \langle h^{(i)},  h^{(j)}\rangle\]
And we are trying to derive a concentration inequality for $\|z\|_1$.






\begin{lemma}
For all $v\in B_k$, the probability 
\[
  \begin{array}{ll}
& \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
\leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{lemma}
\begin{proof}
Let the deviation be
\[
\tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
\]  
We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
\[
\mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
\]  
 then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
 \[
 \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
 \]
 This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
Since  
\[
\mathcal{X}_v-\mathcal{X}_{v'} =  
\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
\]

Then use the fact that 
\[
| \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
\]
and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
$s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
$\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
 \[
  \begin{array}{ll}
\sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
&\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
&\leq  \tau \sqrt{n}np \|a\|_1
\end{array}
  \]  
  
Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
We have a concentration inequality in each ball,
We define the tail event 
\[
\mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
\]
we can take a union bound,
 \[
  \begin{array}{ll}
 \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
&\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
\end{array}
  \] 
\end{proof}

==> sec/extension.tex <==




% \paragraph{Sub-Gaussian case}
% For a sub-Gaussian random variable $\Xi$ with unit variance and symmetric c.d.f $F$, we define 
% \[
% K = \|\Xi\|_{\Psi_2} = \sup_{r\geq 1} r^{-1/2}  (E|\Xi|^r)^{1/r}
% \]
% as the sub-gaussian norm of $X$
% \begin{lemma} \label{lem:Khintchine}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then for all $r \geq 2$,
% \[
% \|\psi\|_2 \leq (E(Z)^p)^{1/p} \leq C K p^{1/2} \|\psi\|_2
% \]
% where $C$ is absolute constant.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% The lower bound follows by independence and Holder’s inequality.
% For the upper bound, since we have 
% \[
% \|\sum_i a_i X_i\|_{\Psi_2}^2\leq C\sum_i a_i^2 \| X_i\|_{\Psi_2}^2\leq C\|\psi\|_2^2 K^2,
% \]
% And $Z = \sum_i a_i X_i$ is sub-Gaussian, so for all $p\geq 2$,
% \[
%  (E(Z)^p)^{1/p} \leq \|Z\|_{\Psi_2} p^{1/2} \leq C^{1/2} p^{1/2}\|\psi\|_2 K 
% \]
% \end{proof}
% \begin{lemma} \label{lem:Khintchine for $p=1$}
% Let  $\Xi_i$ are IID sub-Gaussian with c.d.f $F$ and unit variance.  Then
% \[
%      3^{-3/2}C^{-3} K^{-3}  \| a\|_2 \leq \E |\sum_i a_i \Xi_i| \leq \|a\|_2.
% \] 
% \[
%      3^{-3/2}C^{-3} K^{-3}  \|\psi\|_2 \leq E |\sum_i a_i X_i| \leq \|\psi\|_2
% \]
% where $C$ is absolute constant, $K = \|X\|_{\Psi_2}$.
% \end{lemma}
%  \begin{proof}[Proof of Lemma \ref{lem:Khintchine}]
% We use the extrapolation trick. 
% Let $Z=\sum_i a_i X_i$, since we have 
% \[ (E(Z)^2){1/2} \leq (E|Z|)^{1/4}((E(Z)^3)^{1/3})^{3/4},\]
% we get 
% \[E|Z|\geq (E(Z)^2)^{2}/ (E(Z)^3).\]

% We get a bound on 
% \[
% \|\psi\|_2 \leq (E(Z)^r)^{1/r} \leq C K p^{1/2} \|\psi\|_2
% \]
% from Khinthine’s inequality for $r = 3$.
% \end{proof}


==> sec/finite_sample.tex <==
\section{Finite sample analysis}
\paragraph{Finite sample setting}
\BIT
\item
Let $(X_t)_{t \in \integers}$ be IID sampled from  $pN(0,1) + (1-p) \delta_0$.
 \item
The filter $a\in l_1(\integers), (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.$ Additionally, in finite sample setting, we assume $a^{-1}$ is zero outside of a centered window of radius $2k+1$, namely, the non-zero part can be written as $(\beta_{-k}, \ldots, \beta_0, \ldots, \beta_k)\in V$. 

We fix the shift and scaling effect by assuming $v^T a^{-1} = 1$ for a generic $v$ that has one single largest entry. 
\item
Let $Y= a* X$ be a linear process, we are given a series of observation $(Y_t)_{t\in [-(T+k),T+k]}$ from a centered window of radius $T+k$.
\item
 We denote $X^{(i)}$ as the sequence being flipped and shifted for $i$ step from $X$ s that $X^{(i)}_k = X_{-k +i}$. Let $J_N$ be the support of $X$.
 We define the length $N=2T+1$ window as $\cT := [-T, T].$
\EIT
Now we want to find an inverse filter 
$w = (w_{-k}, \ldots, w_0, \ldots, w_k) \in V$ such that the convolution $w*Y$ is sparse,
\BEQ
 \begin{array}{ll}
 \underset{w\in V}{  \mbox{minimize} }   & \frac{1}{N}\|w*Y\|_{1,\cT}\\
 \mbox{subject to}  
& v^T w =1.
\end{array}
\tag{$P_{v}^T$}
\EEQ


% Let $C_i(w)$ be $\tilde{w}$ with $i$ step right shift, and define 
% $L_i := |C_i(w)^T Y|$, then 
% \[
% \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{2T+1}\|w*Y\|_{1,[-T,T]} = \frac{1}{2T+1}\sum_{|i|\in \cT} |[w*Y]_i|  = \frac{1}{2T+1}\sum_{|i|\in \cT} L_i
% \]
% We know that
% \[
% L_i = |C_i(w)^T Y| = |C_i(e_0 +\phi)^T X| = |(e_0 +\phi)^T C_i(X)|
% \]


First, after change of variable,
\[
 \frac{1}{N}\|w*Y\|_{1,\cT} = \frac{1}{N}\|\psi*X\|_{1,\cT}
\]
Then the empirical average can be represented as sum of shifted and flipped inner products.
\[
\frac{1}{N}\|\psi*X\|_{1,\cT}  = \frac{1}{N}\sum_{|i|\in \cT} |[\psi*X]_i| = \frac{1}{N}\sum_{|i|\in \cT}|\psi^T X^{(i)}|
\]
We define 
\[
p_N = \frac{1}{N}\sum_{i\in \cT} I_i
\]
The population average is being calculated,  as
\[
\E  \|\psi*X \|_1:= \E|C_i(\psi)^T X| = \E|\tilde{\psi}^T X|
\]
We know the mean of $p_N$ is $p$, the variance of $p_N$ as
\[
\E[p_N-p]^2=\frac{1}{N}p(1-p)
\]


% \paragraph{Concerntration of finite sample subdifferential}
% Remark:
% From Proposition~$3.5$ (Uniform convergence of subdifferential) in the dictionary learning paper \cite{bai2018subgradient}, we have 
% uniform convergence of subdifferential under Hausdoff distance for all $\psi$ in $2-$norm sphere $S^{n-1}$.


% We want to study 
% \[
% \frac{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}{t} 
% \]

% Notice that
%  \BEAS
%  (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1) = \sqrt{\frac{2}{\pi}} \E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%  \EEAS

% We want to use the empirical formula of sub-gradient:
%  \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1)-(\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)}]\\
%   &=& \lim_{t\rightarrow 0^+}\frac{1}{t}[
%   (\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| X_0 \|_1) 
%   -\sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)\\
%   && + \sqrt{\frac{2}{\pi}}(\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   - (\E  \| (e_0+t\beta)*X \|_1 - \E  \| X_0 \|_1)]
%  \EEAS
%  and for the second term, diving the constant $\sqrt{\frac{2}{\pi}}$, we have
%   \BEAS
%  &&\lim_{t\rightarrow 0^+}\frac{1}{t}[{
%  (\hat{\E}  \| (e_0+t\beta)_I \|_2 - \hat{\E}  \| (e_0)_I \|_2)
%   -\E (  \| (e_0+t\beta)_I \|_2 -  \| (e_0)_I \|_2)
%   }]\\
%  &=&  \left(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)-\left(p \cdot \langle\beta, e_0\rangle + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]\right)
%  \EEAS
%  If is easy to see that  
% using the fact
% \[
% \E[p_N-p]^2=\frac{1}{N}p(1-p)
% \] 
% we only need to bound
%   \BEAS
%  && (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
%  and we can do further reduction to
%  a bound on 
%   \BEAS
%  && \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]- \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]
%  \EEAS 
 
 
 
 \paragraph{Finite sample directional derivative}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (\psi+t\beta)*X \|_1 - \hat{\E}  \| \psi*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{\psi} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}(\psi^T X^{(i)})X^{(i),T}\beta
 \EEAS
Now to study the finite sample convex problem, we need to calculate the directional derivative at $ \psi = e_0$.
Then
\begin{theorem}
For any $X$ sequence with support  $J_N$,
\BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
% \\
%   &=& 
% p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
% (1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
% \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
 
\end{theorem}
\begin{proof}
 \BEAS
& & \lim_{t\rightarrow 0^+}\frac{1}{t}[(\hat{\E}  \| (e_0+t\beta)*X \|_1 - \hat{\E}  \| e_0*X \|_1)
\\
  &=& 
 \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\psi}L_i}|_{e_0} \rangle \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_0^{(i)})X^{(i),T}\beta
 \\
 &=& 
 \frac{1}{N}\sum_{|i|\in \cT}  \mbox{sign}( X_{-i})X^{(i),T}\beta
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}= 0} \cdot |X^{(i),T}\beta|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta)  +
\frac{1}{N}\sum_{|i|\in \cT}  |X^{(i),T}\beta_{(0)}|
 \\
 &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X_{-i}\beta_0  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X_{-i}\beta_0)  + 
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\\
& &
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}> 0}  \cdot X^{(i),T}\beta_{(0)}  +
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}< 0}  \cdot (-X^{(i),T}\beta_{(0)})  
 \\
  &=& 
\frac{1}{N}\sum_{|i|\in \cT} 1_{X_{-i}\neq 0}  \cdot |X_{-i}|\beta_0  +
\frac{1}{N}  \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}   
 \\
  &=& 
 \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} \right) 
 \EEAS
\end{proof}
\begin{coro}
For Gaussian IID sequence $X$, 
 the random variable $ \frac{\|X\|_{1,J_N}}{N} = p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|})$ has mean $p\sqrt{\frac{2}{\pi}}$. 
 And the random expression
\BEAS
& &  \frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
\\
  &=& 
p_N   ( \frac{\|X\|_{1,J_N}}{|J_N|}) \beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
 \EEAS
 has mean $\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])$.
\end{coro}
\begin{proof}
 \BEAS
& & 
\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N} \right) 
 \\
  &=& 
p_N ( \frac{\|X\|_{1,J_N}}{|J_N|})\beta_0  +
(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N}
%  \\
%  &\approx& 
% \sqrt{\frac{2}{\pi}}(p_N \cdot \langle\beta, e_0\rangle + (1-p_N) \cdot \hat{\Expect}_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])
 \EEAS
where $p_N = \frac{|J_N|}{N} = \frac{1}{N}\sum_{|i|\in \cT}  1_{X_{-i}\neq 0}$ has mean $p$ and variance $\frac{1}{N} p(1-p)$.
And notice that for the Gaussian IID case 
\[
\E [ p_N\frac{\|X\|_{1,J_N}}{|J_N|}] = \E[p_N|X_{0}|\mid X_{0}\neq 0]  = p\sqrt{\frac{2}{\pi}},
\]
\[
\E [(1-p_N ) \frac{1}{|\cT-J_N|}  \|X*\beta_{(0)}\|_{1,\cT-J_N} ] = \sqrt{\frac{2}{\pi}}\Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]).
\]
\end{proof}

\begin{coro}
 For symmetric IID sequence $X$, 
  \[
  \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot (\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} ) 
  \]
  where 
  $\sum_{j\in J_N-\{i\} } X_j \beta_{i-j} $ is independent of $X_i$, therefore independent of $(1_{X_{-i}> 0}-1_{X_{-i}< 0}) $.
  Specifically, it has mean $0$
   \[
 \E \frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}  = 0
  \]
  for $q\leq 2$,
    \[
  \frac{1}{N}\E|\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)} |^q \leq 
  \frac{1}{N} \E[]|\sum_{i\in J_N}|1_{X_{-i}> 0}-1_{X_{-i}< 0}||^q\cdot  \max_j |X^{(j),T}\beta_{(0)} |^q]
  \]
  
\end{coro}
%   \[
%  p^\star(u):= 
%  \sup_{p\in [0,1]}\{\inf_{\|\beta\|_2=1 }(-p \cdot \sqrt{1-\| P_{u}^{\perp} P_{e_0}^{\perp} \beta\|_2^2} + (1-p) \cdot  \E_I\| (P_{u}^{\perp} P_{e_0}^{\perp} \beta)_I\|_2 ) > 0\}
%  \]



 \paragraph{Concerntration of $\|\psi*X\|_{1}$ }
The next step is to provide an uniform bound of the finite sample derivation of $\|X\|_{1,J_N}$ and 
$\|X*\beta_{(0)}\|_{1,\cT-J_N}$.

In general, for any random subset $I$ of $\cT$, we study the uniform concentration of 
\[
\|\psi*X\|_{1,I} 
\]
for $\psi = a*w \in a*B_1(V_k),$ by providing moments and tail bound on
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]

For clarity of the argument, we only state the concentration for $\|\psi*X\|_{1,\cT}.$ Also the result about $\cT$ would easy carry to a random subset $I$.

Let the minimal and maximal eigenvalue of the (convolutional) linear operator $a*$ be
\[
\lambda_{m}(a) := \inf_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\[
\lambda_{M}(a) := \sup_{y: \|y\|_2\leq 1} \frac{\|a*y\|_2}{\|y\|_2}
\]
\begin{lemma}
Using circluar embedding of Topelitz matrix, 
\[
\lambda_{M}(a) \leq \max| \hat{a}|
\]
\end{lemma}

Following the idea of lemma~$4$ of the paper of Adamczak on sparse dictionary learning\cite{adamczak2016note} and lemma~$16$ of the paper \cite{spielman2012exact}, we derive a similar bound for convolutional case.
\begin{lemma}
In the following, we define 
\[
Z :=  \frac{1}{N}\|w*a*X\|_{1,\cT}
\]
We find the lower bound of $\E Z$ as a function of the $1-$norm  of $w$:
\[
\E Z  \geq \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1} 
\]
For convenience, we define
\[
\mu_{\mbox{min}}:=\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}} \|w\|_{1}
\]

\end{lemma}
\begin{proof}
WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
\BEAS
\E_X Z 
&=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
&\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
\EEAS
By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
$\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
\BEAS
\E_X Z 
&\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
&\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
&\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
&\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
&=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
\EEAS
\end{proof}

% \begin{proof}
% WOLG, we rescale $w$ so that $\|w\|_1 =1$, now
% \BEAS
% \E_X Z 
% &=& \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|\\
% &\geq& \inf_{\|w\|_{1} = 1}\frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k w_i (a*X)_{j-i}|
% \EEAS
% By symmetry, we know the minimizer is $w = (\frac{1}{k}, \ldots,\frac{1}{k}),$
% then we use the symmetrization trick to insert a sequence of $k$ IID Rademacher ($\pm 1$)  random variables 
% $\varepsilon_1, \ldots, \varepsilon_k$ in the second inequality, and then apply Khintchine inequality as the third inequality,
% \BEAS
% \E_X Z 
% &\geq&  \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k (a*X)_{j-i}|\\
% &\geq& \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\E_X |\sum_{i=1}^k \varepsilon_i (a*X)_{j-i}|\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  (a*X)^2_{j-i}}\\
% &\geq&  \frac{1}{2} \frac{1}{k} \frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{1}{\sqrt{2}}\E_X \sqrt{ \sum_{i=1}^k  X^2_{j-i}}\\
% &\geq& \frac{1}{2}  \frac{1}{k} \frac{1}{\sqrt{2}}\frac{1}{N}\sum_{j\in [-T,T] }\lambda_{m}(a)\frac{2}{\pi}\sqrt{pk}\\
% &=&  \frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}\\
% \EEAS
% \end{proof}

Now we define the intersection of $1-$norm ball of the $k-$dimensional subspace $V_k$ as $B_1(V_k)$, then we consider $w\in B_1(V_k).$ 
\begin{lemma}
Hence we consider $\psi = a*w \in a*B_1(V_k),$ and we define
\[
W:= \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) |
\]

For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E W^q\leq 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{lemma}

\begin{proof}
Let $\varepsilon_1, \ldots, \varepsilon_N$ be a sequence of IID Rademacher ($\pm 1$)  random variables independent of $X$,  By the symmetrization inequality, see e.g. lemma~$6.3$ of book \cite{ledoux2013probability}, we have the first inequality. Then since the function $t \rightarrow |t| $ is a contraction, an application of Talagrand’s contraction principle (see lemma~$8$ of \cite{adamczak2016note}) with $F (x) = |x|^q$ 
conditionally on $X$ gives the second inequality.
\BEAS
\E W^q 
&\leq& 2^q \E \sup_{\psi \in a*B_1(V_k)} 
|\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j |(\psi*X)_{j}| |^q\\
&\leq&
2^{2q}\E \sup_{\psi \in a*B_1(V_k)} |\frac{1}{N}\sum_{j\in [-T,T] } \varepsilon_j (\psi*X)_{j} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{\psi \in a*B_1(V_k)} |\sum_{i\in [-T,T] }\psi_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&=&
2^{2q}\frac{1}{N^q}\E \sup_{w \in B_1(V_k)} |\sum_{i\in [-T,T] }(w*a)_{i}  \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q\\
&\leq&
2^{2q}\frac{1}{N^q}\E \max_{s\in [k]}|\sum_{i\in [-T,T] }a_{i-s}( \sum_{j\in [-T,T] } \varepsilon_j X_{j-i}) |^q\\
&\leq&
2^{2q}(\frac{\lambda_{M}(a)}{N})^q   \sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q
\EEAS
Now by the moment version of Bernstein’s inequality (see lemma~$7$, equation $(18)$ of\cite{adamczak2016note}), we know that there exists a universal constant $C$,
\BEAS
\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-i} |^q \leq C^q(\sqrt{Npq}+q)^q
\EEAS
Therefore, 
\BEAS
\E W^q &\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q    
\sum_{s\in [k] }\E| \sum_{j\in [-T,T] } \varepsilon_j X_{j-s} |^q \\
&\leq& 2^{2q}(\frac{\lambda_{M}(a)}{N})^q   k C^q(\sqrt{Npq}+q)^q
\EEAS
Then
\BEAS
 \|W\|_q \leq \frac{4eC}{N} \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
therefore, we could get the tail bound using the Chebyshev inequality for the moments,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np(q+\log(k))}+q +\log(k)))\leq e^{-q}
\EEAS
We set $q = \log(\frac{1}{\delta})$, then we will get an upper bound for $W$ which is satisfied with probability at least $1-\delta$:
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{proof}

\begin{lemma}
Let the condition number of the linear operator $a*$ be
\[
\kappa_a := \frac{\lambda_M(a)}{\lambda_m(a)}.
\]
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
and  $p\geq \frac{1}{N}$, 
then
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{lemma}
\begin{proof}
If
\[
N\geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
\]
then 
\[
\frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})} \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
additionally, if $p\geq \frac{1}{N}$, 
then a weaker inequality is also true:
\[
\frac{4eC\lambda_{M}(a) }{N}  
 \log(\frac{k}{\delta}) \leq \frac{1}{2}\epsilon (\frac{1}{\sqrt{2}\pi}\lambda_{m}(a)\sqrt{\frac{p}{k}}) \leq \frac{1}{2}\epsilon \mu_{\mbox{min}}
\]
therefore, combining the two parts and the previous inequality,
\BEAS
P( W > \frac{4eC\lambda_{M}(a) }{N}  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
we have
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta
\EEAS
\end{proof}


\begin{theorem}
Let the solution of finite sample convex optimization be $w^\star$, 
for small $\epsilon>0$ and concentration level $\delta>0$, 
there exists universal constant $C$, if there are 
% \[
% N=2T+1 \geq k\log(\frac{k}{\delta}) (2^7 \pi e^2 \frac{C^2}{\epsilon^2} \kappa_a^2 )
% \]
\[
N \geq k\log(\frac{k}{\delta}) ( \frac{C\kappa_a}{\epsilon}  )^2
\]
and  $ \frac{1}{N}\leq p< p^\star(\epsilon)$, we have 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
% Therefore with probability at least $1-\delta$, $a*w^\star =e_0$ and we recover the sparse vector exactly.

% \textbf{ToDO:}
% or
% $\|a*w^\star -e_0\|_1<\epsilon_1$ provided $p< p_N^\star$ for some $p_N^\star\leq p^\star$.
  \end{theorem}
\begin{proof}
From previous lemma, we know that with the conditions, 
\BEAS
P( W > \epsilon \mu_{\mbox{min}})\leq \delta.
\EEAS
Therefore, with probability at least $1-\delta$,
\BEAS
W = \sup_{\psi \in a*B_1(V_k)}
|\frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - \E |(\psi*X)_{j}|) | \leq \epsilon \mu_{\mbox{min}}
\EEAS
When this is true, for all $\psi \in a*B_1(V_k)$, we have a uniform bound 
\[
 \E |(\psi*X)_{j}|-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
\]
\end{proof}
% then
% \[
%  (\E |(\psi*X)_{j}| - \E |X_{j}|)/\| \psi\|_2-\epsilon\mu_{\mbox{min}} \leq \frac{1}{N}\sum_{j\in [-T,T] } (|(\psi*X)_{j}| - |(X)_{j}|)/\| \psi\|_2 \leq \E |(\psi*X)_{j}|+\epsilon\mu_{\mbox{min}}
% \]
% and from previous condition and the expression of directional derivative, 
% \[
% |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | < 2\epsilon
% \]
% If $p<p^\star(u, \epsilon)$, we know from population result that
% \[
% \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
% \]


\begin{coro}
For $\psi = a*w \in a*B_1(V_k),$ 
\[
U_I:= \sup_{\psi \in a*B_1(V_k)}
| \|\psi*X\|_{1,I}    - \E  \|\psi*X\|_{1,I}  |
\]
For all $q\geq \max(2, \log(k)),$ there exists constant $C$,
\[
\E U_I^q\leq 2^{2q}(\lambda_{M}(a))^q   k C^q(\sqrt{Npq}+q)^q
\]
so
\BEAS
 \|U_I\|_q \leq 4eC \lambda_{M}(a)  
 (\sqrt{Np(q+\log(k))}+q +\log(k))
\EEAS
and
\BEAS
P( U_I > 4eC\lambda_{M}(a)  
 (\sqrt{Np\log(\frac{k}{\delta})}+\log(\frac{k}{\delta})))\leq \delta
\EEAS
\end{coro}

% \textbf{ToDO:  Study the finite sample phase transition condition directly} 
\paragraph{Uniform bound of directional derivative}
We  define the uniform bound of directional derivative
\[
W_D  =\sup_{\|\beta\|_2=1, u^T \beta =0, \beta +e_0 \in a*B_1(V_k)}|\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  | 
\]
Notice that
\BEAS
& &\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle  
\\
&=& 
\left[\frac{1}{N} \left(\|X\|_{1,J_N} \beta_0  +
 \|X*\beta_{(0)}\|_{1,\cT-J_N}+ 
\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}\right)\right]-
\\
& &
\left[\sqrt{\frac{2}{\pi}}(p \cdot \beta_0 + (1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ])\right]
\EEAS
From previous uniform bound, with high probability, we have the following three uniform bounds on
\[
|\frac{1}{N}\sum_{i\in J_N} (1_{X_{-i}> 0}-1_{X_{-i}< 0})  \cdot X^{(i),T}\beta_{(0)}|
\]
\[
|(\frac{1}{N} \|X\|_{1,J_N}-\sqrt{\frac{2}{\pi}}p)|
\]
\[
|\frac{1}{N}\|X*\beta_{(0)}\|_{1,\cT-J_N}-(1-p) \cdot \Expect_{I}[ \|\beta_{I}\|_2 | 0 \not \in I ]|
\]
If $p<p^\star(u, \epsilon)$, we know from population result that
\[
\langle  \beta, \E \nabla_{\phi}L|_{\phi = 0} \rangle >\epsilon.
\]
If with high probability,  
\[
W_D  \leq \epsilon/2
\]
then using the convexity argument, 
for any direction $\beta \in V,$ the directional derivative at $\phi = 0$
\[
\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  >0,
\]
then $a*w^\star-e_0=0$. 
% \paragraph{Uniform bound of finite difference}
% In the end, we define the uniform bound of finite difference, let 
% $t:=\| \psi-e_0\|_2$,
% \BEAS
% W_{D,t}  = \sup_{\psi \in a*B_1(V_k)}
% |\frac{1}{N}\sum_{j\in [-T,T] } ((|(\psi*X)_{j}|-|X_{j}|) - (\E |(\psi*X)_{j}- \E |X_{j}|)|) |/t
% \EEAS
% then from previous lower bound of finite difference by directional derivative, for all $t\in (0,1]$,
% \[
% W_D  = \lim_{t\rightarrow 0}W_{D,t} \leq   W_{D,t}
% \]
% % Using Lipschitz property of finite difference, if directional derivatives are $L-$Lipschitz function, then
% % \[
% % |\langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  -   \langle  \beta, {\frac{1}{N}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = \phi^\star} \rangle   | < L\epsilon_1
% % \]





% % \textbf{ToDO:}
% % Finish the detail proof and find relation of $\epsilon_1$ to other constant!

% \end{proof}

% \paragraph{Concentration tools}
% \begin{lemma}[Gaussian concentration inequality]\label{lem:gaussian_concentration} Let $ x = ( x_1,\ldots,  x_n)$ be a vector of $n$ independent standard normal variables. Let $f: \reals^n\to \reals$ be an $L$-Lipschitz function. Then for all $t>0$,
% \[
% 	\prob{(|f( x) - \E f( x)| \geq t)} \leq 2\exp\left(-\frac{t^2}{2L^2} \right). 
% \]
% \end{lemma}

% \begin{lemma}[Moment control Bernstein inequality for scalar r.v.s]\emph{(\cite{foucart2013mathematical}, Theorem 7.30)}\label{lem:mc_bernstein_scalar}
% Let $  x_1, \dots,   x_n$ be independent real-valued random variables. Suppose that there exist some positive number $R$ and $\sigma^2$ such that $\frac1n\sum_{i=1}^n\expect{  X_i^2}\leq \sigma^2$ and
% \begin{align*}
% \tfrac1n\textstyle\sum_{i=1}^n\expect{\abs{  x_k}^p} \leq \frac{1}{2}\sigma^2 R^{p-2}p!, \; \; \text{for all integers}\; p \ge 3.
% \end{align*}
% Let $S \doteq \sum_{i=1}^n   x_i$, then for all $t > 0$, it holds  that 
% \begin{align}
% \prob{\abs{S - \expect{S}} \ge t} \leq 2\exp\left(-\frac{t^2}{2n\sigma^2 + 2Rt}\right).   
% \end{align}
% \end{lemma}

% \begin{lemma}[$\eps$-net on sphere]\label{lem:epsnet}\emph{\cite{vershynin2010introduction}}  Let $(X, d)$ be a metric space and let $\eps > 0$.
% A subset of $X$ is called an $\eps$-net of $X$ if for every point $x\in X$ there exists some point $y \in  N(x,\eps)$ so that $d(x, y) \leq\eps$. There exists an $\eps$-net for the sphere $ S^{n-1}$ of size
% 	$ (\frac{3}{\epsilon})^n$.
% \end{lemma}


% \begin{lemma}[Young's convolution inequality]
% For 
% $\frac{1}{p} + \frac{1}{q} = \frac{1}{r} +1,$
% \[
% \lVert f*g\rVert_r\le\lVert f\rVert_p\lVert g\rVert_q
% \]
% \end{lemma}




% \paragraph{Finite sample concentration overview}
% We show the concentration in $3$ steps. First, for a fixed direction  $\beta \in V$, we define the event 
% \[
% \mathcal{X}(\psi)  := (|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X| |\geq t) 
% \]
% % notice that
% % where
% % \[
% % \E[|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} \mid I] = \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} 
% % \]
% % and 
% % \[
% % \E|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} = \E\sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} = \E|\tilde{\psi}^T X| = 
% % \]
% here we can break it into $2$ terms:
% \[
% |\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} |\geq t_1 
% \]

% \[
% | \sqrt{\frac{\pi}{2}}|\frac{1}{2T+1}\|\psi*1_{I}\|_{2,[-T,T]} -\sqrt{\frac{\pi}{2}} \E_I \|\psi_{I}\|_{2,[-T,T]} |\geq t_2 
% \]

% and we bound the tail probability 
% \[
% P(\mathcal{X}(\psi) ) = P(|\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} - \E|\tilde{\psi}^T X|   | \geq t) 
% \]
% Second, we find the Lipschitz constant $L$ of the mapping  $\psi \rightarrow \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]},$ and we replace point event $\mathcal{X}(\psi)$ with a $\epsilon-$ball event 
% $\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi')$ with $\epsilon = \frac{1}{L}.$

% Third, we use $\epsilon-$net to cover the entire $k$-dimensional  space with $k+1$ is the length allowed for the approximate inverse filter $w$ ($w$ is in a $k$-dimensional vector space $V_k$), since the forward filter $a$ is fixed, $\psi = a*w$ is also in a $k$-dimensional vector space $a*V_k$.
% Therefore, 
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]

% \paragraph{Concentration inequality}
% Let $C(\psi)$ be the circulant matrix spanned by the flipped version of $\psi$ as the first column vector.

% Using duality of $1$-norm, we know that
% \[
%  \frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]} =  \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]} 
% \]

% The Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_x =\sup_{\|b\|_\infty\leq 1}  \|C(\psi)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(\psi) )
%  \]
 
%  On the other hand, $\psi = w*a,$
%  the Lipschitz constant of the mapping $w \rightarrow \frac{1}{2T+1}E_X\sup_{\|b\|_\infty\leq 1}\langle C(w) C(a) b , X\rangle_{[-T,T]}$ is 
%   \[
%  L_w =\sup_{\|b\|_\infty\leq 1}  \|C(a)  b\|_{\mathrm{op}} =  \sup_{\|b\|_\infty\leq 1} \lambda_{\max}( \mbox{diag}(b) C(a) )= \|\hat{a}\|_\infty
%  \]

% \begin{lemma}
% From theorem~$8$ of paper \cite{van2013bernstein}, the Bernoulli Gaussian random variable  have sub-exponential tails, and satisfy Bernstein condition with $K =2$.

% Let $Z =\frac{1}{2T+1}\|\psi*X\|_{1,[-T,T]}  $, then $\E Z =  \E|\tilde{\psi}^T X|\leq \sqrt{p}\|\psi\|_2$,
%  \[
%   \begin{array}{ll}
% & \prob \left[  Z - \expect Z  > t   \right] \\
% &\leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)\\
% &\leq \exp\left(  \frac{-t^2/2   }{\frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 +2(2\sqrt{p}\|\psi\|_2+t/3)}\right)
% \end{array}
%   \]  
% where $\sigma^2=  \expect Z^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 $.
% \end{lemma}

% \begin{proof}
% % Let $\hat{p} := \frac{1}{2T+1}\sum_{|i|\in \cT} 1_{X_i \neq 0}$
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle  = 
% % \hat{p} \beta_0 +(1-\hat{p}) \hat{\E}\|\beta * X_{{(0)}}\|_1 
% % \]



% % \[
% %   \| (e_0+t\beta)*X \|_1   = \hat{\E}\sup_{\|b\|_\infty\leq 1}\langle b*(e_0+t\beta) , X\rangle
% % \]
%  From the theorem $8.42$ of \cite{foucart2013mathematical}, we have the following inequality:
%  for the supreme of functions $\langle b*(e_0+t\beta) , X\rangle$, since $\expect \langle b*(e_0+t\beta) , X\rangle=0$,
%  $ \langle b*(e_0+t\beta) , X\rangle\leq K$, 
%  \[
%  \sigma^2 =\expect \frac{1}{(2T+1)^2}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , X\rangle_{[-T,T]}^2 = \frac{1}{(2T+1)^2} p \| \tilde{\psi}*\psi\|_1 
%  \]
%  we have
%  \[
%   \begin{array}{ll}
%  \prob \left[  Z - \expect Z  > t   \right] \leq   \exp\left(  \frac{-t^2/2   }{\sigma^2+K(2\expect Z+t/3)}\right)
% \end{array}
%   \]  
% \end{proof}
% We also remark that the essential concentration inequality that we are trying to derive is the following:
% let's consider the case when $x$ is IID standard Gaussian, we define $z = \psi*x = C(\psi)^T x$,
% then $z$ is a non-isotropic Gaussian vector \[\mathcal{N}(0,C(\psi) C(\psi)^T),\] where 
% \[  (C(\psi) C(\psi)^T)_{ij} = \langle \psi^{(i)},  \psi^{(j)}\rangle\]
% And we are trying to derive a concentration inequality for $\|z\|_1$.

% \begin{lemma}
% Since $\forall w \in V_k, \|w\|_\infty \leq 1 $, 
% from Young's convolution inequality,
% \[
% \|a*w\|_2 \leq \|w\|_\infty \|a\|_{\frac{2}{3}} = \|a\|_{\frac{2}{3}}
% \]
% and 
% \[
% \| \tilde{a}*a*\tilde{w}*w \|_1\leq \|w\|_\infty^2 \| \tilde{a}*a \|_{\frac{1}{3}} = \| \tilde{a}*a \|_{\frac{1}{3}}
% \]
% \end{lemma}

% \begin{theorem}[Uniform convergence from covering]
% Let $\epsilon:= \frac{1}{L_w},$  then from the $\epsilon-$net covering lemma,
% \[
% P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) = (\frac{3}{\epsilon})^k P(\cup_{\psi' \in N(\psi,\epsilon)} \mathcal{X}(\psi'))  =  (\frac{3}{\epsilon})^k P( \mathcal{X}(\psi))
% \]
% Here the Lipschitz constant of the mapping $x \rightarrow \frac{1}{2T+1}\sup_{\|b\|_\infty\leq 1}\langle C(\psi)  b , x\rangle_{[-T,T]}$ is 
%   \[
%  L_w
%  = \| \hat{a}\|_\infty
%  \]
%  here $\| \hat{a}\|_\infty$ is the infinity norm (max absolute value of entries) of the Fourier transform of $a$,
%  then
% \BEAS
% &&\prob \left[  Z - \expect Z  > t ,\forall w \in V_k, \|w\|_\infty \leq 1 \right]
% \\
% &=& P(\cup_{\psi' \in a*V_k}\mathcal{X}(\psi) ) \\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a*\tilde{w}*w \|_1 p +2(2\sqrt{p}\|a*w\|_2+t/3)}\right)\\
% &\leq& \exp\left( k \log(3\| \hat{a}\|_\infty) + \frac{-t^2/2   }{
% \frac{1}{(2T+1)^2}  \| \tilde{a}*a \|_{\frac{1}{3}} p +2(2\sqrt{p}\|a\|_{\frac{2}{3}}+t/3)}\right)
% \EEAS
% \end{theorem}
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           

% % \begin{lemma}
% % For all $v\in B_k$, the probability 
% % \[
% %   \begin{array}{ll}
% % & \prob \left[  |\|v*a*x\|_1- \expect \|v*a*x\|_1 | > t, v \in B_k  \right]   \\ 
% % \leq&  (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{lemma}
% % \begin{proof}
% % Let the deviation be
% % \[
% % \tilde{\mathcal{X}}_v =   \sum_{i=1}^n \left( | \langle C(a^{(i)}) v, x\rangle| - \expect | \langle C(a^{(i)}) v, x\rangle|\right).
% % \]  
% % We will choose $1/\epsilon$ to be the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ as a function of $v$. Let's compute the Lipschitz constant.

 
% % % The generic chain defintion and facts we will use are from section $3.2$ of \cite{blasiok2016improved}.
 

% % We introduce additional independent random sign $s_j$ , which are IID sampled from Rademacher variable by defining 
% % \[
% % \mathcal{X}_v =   \sum_{i=1}^n s_j \left( |\langle C(a^{(i)}) v, x\rangle| \right),
% % \]  
% %  then by lemma $24$ of \cite{blasiok2016improved}, for every integer $p$ we have 
% %  \[
% %  \| \sup_{v\in B_k} |\tilde{\mathcal{X}}_v | \|_p \lesssim \| \sup_{v\in B_k}  |\mathcal{X}_v| \|_p
% %  \]
% %  This is called symmetrization trick. Using this trick, we only need to analyze the tail behavior of the random variable $\mathcal{X}_v$. To obtain tail bounds for maximum  of  $\sup_{v\in B_k}  |\mathcal{X}_v|$, we need to bound tails of the random variables $\mathcal{X}_v-\mathcal{X}_{v'}$ for $v, v'\in B_k$.
 
% % Since  
% % \[
% % \mathcal{X}_v-\mathcal{X}_{v'} =  
% % \sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle|\right).
% % \]

% % Then use the fact that 
% % \[
% % | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| \leq   \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right),
% % \]
% % and  both $s_i | \langle C(a^{(i)}) v, x\rangle| -   | \langle C(a^{(i)}) v', x\rangle| $ and  
% % $s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ are symmetric, if we have a tail bound for 
% % $\sum_{i=1}^n s_i \left( | \langle C(a^{(i)}) (v-v'), x\rangle|  \right)$ , 
% % we also have tail bounds on $\mathcal{X}_v-\mathcal{X}_{v'}$.

% % From these calculation, we saw that the Lipschitz constant of  $\tilde{\mathcal{X}}_v$ is bounded by 
% %  \[
% %   \begin{array}{ll}
% % \sqrt{\sum_{j=1}^n (\sum_{i=1}^n s_i |\sum_{t=1}^n a^{i-j+t} x_t|)^2}
% % &\leq   \sqrt{n (\|a\|_1 \|x\|_1)^2}\\
% % &\leq  \tau \sqrt{n}np \|a\|_1
% % \end{array}
% %   \]  
  
% % Therefore, we can choose $1/\epsilon = \tau \sqrt{n}np \|a\|_1$, then
% % at most $|N| = (3\tau \sqrt{n}np \|a\|_1)^k$ balls can cover $B_k$.
% % We have a concentration inequality in each ball,
% % We define the tail event 
% % \[
% % \mathcal{E}_v = \{|\tilde{\mathcal{X}}_v | > t\}
% % \]
% % we can take a union bound,
% %  \[
% %   \begin{array}{ll}
% %  \prob \left(\cup_{v \in B_k} \mathcal{E}^c_v \right) &\leq |N| \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] \\
% % &\leq   (3\tau \sqrt{n}np \|a\|_1)^k \prob \left[  |\|h*x\|_1- \expect \|h*x\|_1 | > t   \right] 
% % \end{array}
% %   \] 
% % \end{proof}

% % Second, we show that 
% % \[
% % \langle  \beta, {\frac{1}{2T+1}\sum_{|i|\in \cT} \nabla_{\phi}L_i}|_{\phi = 0} \rangle 
% % \]
% % is locally Lipschitz 
% % % The (set valued) sub-gradient at zero is
% % % \[
% % %   \nabla{L_i} =   \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X),
% % % \]
% % % the directional derivative at zero is
% % % \[
% % %   \nabla_{\phi}{L} = \phi^T \nabla{L_i} =  \mbox{sign}((e_0 +\phi)^T C_i(X))  (\phi^T C_i(X)) ,
% % %   \]
% % % the (set valued) Riemannian subdifferential at zero on the hyperplane defined by $u^T \phi = 0$ is given by
% % % \[
% % %   P_u \nabla{L_i} = (I- uu^T)  \mbox{sign}((e_0 +\phi)^T C_i(X)) C_i(X) 
% % % \]




% % %  \BEQ
% % %   \begin{array}{ll}
% % %   \expect \nabla{L_i}  &=  p\expect[\nabla{L_i} \mid X_i \neq 0 ] + (1-p)\expect[\nabla{L_i} \mid X_i = 0 ] \\
% % %   &=  p\expect[ \mbox{sign}(X_i) C_i(X)\mid X_i \neq 0 ] + (1-p)\expect[ \mbox{sign}((\phi_{(i)})^T C_i(X)_{(i)}) C_i(X)_{(i)}\mid X_i = 0 ] 
% % %   \end{array}
% % %  \EEQ  



==> sec/inequal.tex <==
\subsection{$E{| \psi^T X| }$ for IID Bernoulli Gaussian $X$ }
we study in detail for the quantity  
\[
E{| \psi^T X| } = E{|\sum_{i} \psi_i X_i| }.
\]
We know when $X_i$ are unit variance,
\[
   E (\sum_i \psi_i X_i)^2 =  \sum_i   \psi_i^2 E(X_i)^2 = \|a\|_2^2.
\]
The ratio indicate the sparsity level of random variable $Z = \sum_i \psi_i X_i$
\[
\frac{ E{|\sum_{i} \psi_i X_i| }}{\sqrt{E (\sum_i \psi_i X_i)^2}} = \frac{ E{|\sum_{i} \psi_i X_i| }}{\|a\|_2} 
\]
Now, we consider some settings where exact calculation of $E{|\sum_{i} \psi_i X_i| }$ are possible.

\paragraph{Exact calculation for Bernoulli Gaussian}
% \paragraph{Exact calculation for Gaussian}
Let $X_i = B_i G_i$ be IID Bernoulli Gaussian, where $B_i$ is sampled from Bernoulli with parameter $p$, $G_i$ is sampled from $N(0,1)$. Let $I$ be the support where $B_i =1$.
\[
E_X{|\sum_{i} \psi_i X_i| }  
= E_B E_G {|\sum_{i} \psi_i B_i G_i| }
= E_I E_G {|\sum_{i\in I} \psi_i G_i| }
\]
Leveraging the invariance property for linear transform of Gaussian, we get
\[
E_G {|\sum_{i\in I} \psi_i G_i| } = 
\sqrt{\frac{2}{\pi}} \cdot\|\psi_I\|_2.
\]
then
\[
E_X{|\sum_{i} \psi_i X_i| }  
= \sqrt{\frac{2}{\pi}} \cdot E_I \|\psi_I\|_2
= \sqrt{\frac{2}{\pi}} \cdot (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2.
\]
Here the last equality use the lemma below, and we define that $\|a\|_0= \#\{ t : \psi_t \neq 0\}$.
\begin{lemma} (Expectation of $2-$norm over Bernoulli support)
\label{lem:BLemma}
\BEQ
E_I \|\psi_I\|_2 = (1-(1-p)^{\|a\|_0})^{1/2}   \cdot  \|a\|_2
\EEQ
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:BLemma}]
We have the power series representation $\sqrt{x} = \sum_k c_k x^k$ valid on $(1/A,A)$
for large $A \gg 1$. 
Let $N = |\cT|$. Fix $A > 1/\eps^2$; then every sum $ \sum_{t \in I} \psi_t^2 \in (1/A,A)$;
using this:
\begin{eqnarray*}
 \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  &=&  
 \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \cdot ( \sum_{t \in I} \psi_t^2  )^k \\
 &=& \sum_{I \subset \cT} \pi(I)   \sum_k  c_k \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&   \sum_k  c_k \sum_{I \subset \cT} \pi(I)   \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 \end{eqnarray*}
 Hence from $ \pi(I) = (p)^{|I|} (1-p)^{|\cT \Delta I|}$
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \sum_{n=1}^{N}  \sum_{|I| = n} (p)^n (1-p)^{N-n}  \cdot  \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  %\\
 \end{eqnarray*}
 Since the inner two sums  cover $ {N \choose n} n^k$ terms in a uniform way,
 we can write
% \clearpage
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot \sum_{|I| = n} \sum_{t_1,\dots, t_k \in I} \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot Ave_{|I| = n}  \cdot {n^k} \cdot  Ave_{t_1,\dots, t_k \in I} \; \prod_{i=1}^k \psi_{t_i}^2  \\
&=&  \sum_k c_k   \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}  \cdot {n^k} \cdot Ave_{t_1,\dots, t_k \in \cT} \; \prod_{i=1}^k \psi_{t_i}^2  \\
 &=&  \sum_k c_k   \cdot \left( \sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n} \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 \end{eqnarray*}
Now use the identity $1 = \sum_{n=0}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}$  for the complete binomial sum, 
hence the incomplete sum $\sum_{n=1}^{N}  (p)^n (1-p)^{N-n}  \cdot {N \choose n}= 1-(1-p)^N$. We get
 \begin{eqnarray*}
  \sum_{I \subset \cT} \pi(I)   ( \sum_{t \in I} \psi_t^2)^{1/2}  
 &=&  \sum_k c_k   \cdot \left( 1-(1-p)^N \right)  \cdot ( \sum_{t \in \cT} \psi_t^2  )^k \\
 &=& \left( 1-(1-p)^N \right) \cdot \sum_k c_k  \left ( \sum_{t \in \cT} \psi_t^2  \right )^k \\
 &=&  \left( 1-(1-p)^N \right) \cdot  \sqrt{\sum_{t \in \cT} \psi_t^2 } .
\end{eqnarray*}
\end{proof}

==> sec/population.tex <==

% \section{Technical background}
% \paragraph{Fourier transform and inverse filter}
% The discrete-time Fourier transform $\mathcal{F}$ is defined by $\mathcal{F} a $ where
% \[
%  (\mathcal{F} a)(\omega) : = \sum_{n=-\infty}^\infty a_n\, e^{2\pi i n \omega}, \quad  \omega\in T = [-\frac{1}{2}, \frac{1}{2}];
% \]
% the inverse Fourier transform $\mathcal{F}^{-1}$ is defined by
% \[
% (\mathcal{F}^{-1} f)(n) =  \int_{-\frac{1}{2}}^\frac{1}{2} f(\omega) e^{-2\pi i n \omega}  d\omega, \quad n\in \integers.
% \]
% Now, our condition on the filter $a$ is:
% \[a\in l_1(\integers) ,  
% (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T.
% \]
% In the following theorem, we show that this condition would provide the existence of an inverse filter in  $l_1(\integers)$.

% First, we present the standard Wiener's lemma.
% \begin{lemma}{\textbf{Wiener's lemma on periodic functions:}}
% Assume that a function $f$ on unit circle has an absolutely converging Fourier series, and $f(t)\neq 0$ for all $t \in T$, then $1/f$ also has an absolutely convergent Fourier series.
% \end{lemma}
% Then we can see clearly that the Fourier series version of the previous lemma would guarantee the existence of an inverse filter in  $l_1(\integers)$.
% \begin{lemma}{\textbf{Wiener's lemma on $l_1(\integers)$ sequences :}}
% If $a\in l_1(\integers) ,  
% (\mathcal{F} a)(\omega) \neq 0, \forall \omega\in T,$ we could define the inverse filter of $a$ as
% $$a^{-1} := \mathcal{F}^{-1}(\frac{1}{\mathcal{F} a})$$
% so that $a^{-1}*a = e_0.$ Here $e_0$ is the sequence with $1$ at $0$ coordinate and $0$ elsewhere.
% From Wiener's lemma on $\mathcal{F} a$,   $a^{-1} \in l_1(\integers)$ .
% \end{lemma}





% \section{Change of variables from convex blind deconvolution to convex projection pursuit}
% In this section, we will show that after change of variables, the population version of blind deconvolution is the same as the population version of sparse projection pursuit, which is a convex formulation used for dictionary learning or sparse blind source separation. 

% Therefore, the phase transition phenomenon presented above is a fundamental phase transition that works for a simple but fundamental population convex problem.

% % convex formulation of sparse projection pursuit, also called dictionary learning or sparse blind source separation.

% \paragraph{Change of variable for  convex sparse blind deconvolution}
% We could rewrite the population version of our convex sparse blind deconvolution problem, with the population objective 
% $\Expect\frac{1}{N} \| w*Y\|_{\ell_1(\cT)} =\Expect|(w*Y)_0|=\Expect|(w*a*X)_0|$ due to  the ergodic property of stationary process and shift invariance. Then the convex problem becomes 
% \[
%  \begin{array}{ll}
%  \underset{\psi}{\mbox{minimize}}   & \Expect|(w*a*X)_0|\\
% \mbox{subject to}  
% & ((\widetilde{a}*a^{-1})*(a*w))_0 =1,
% \end{array}
%  \]
% Let $\psi$ be the flipped version of $a*w$, such that $\tilde{\psi} := a*w$, then 
%  $(w*Y)_0 = (w*a*X)_0 = (\tilde{\psi}*X)_0 = \psi^T X.$  
%   Let $u:= \widetilde{a}*a^{-1}$. 
%  Now we arrive at a simple and fundamental  population convex problem: 
%  \[
%  \begin{array}{ll}
%  \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
% \mbox{subject to}  
% & u^T \psi =1.
% \end{array}
% \tag{$P_{u}$ }
%   \]
  
 
  
  
  
  
  
  
  
  
  
  
  
  
  

==> sec/projection_pursuit_PT_new.tex <==

\section{A common population convex problem: projection pursuit and its phase transition}
In this section, we will show that after change of variables, the population version of blind deconvolution is the same as the population version of sparse projection pursuit, which is a convex formulation used for dictionary learning or sparse blind source separation. 

Therefore, the phase transition phenomenon presented above is a fundamental phase transition that works for a simple but fundamental population convex problem.

% convex formulation of sparse projection pursuit, also called dictionary learning or sparse blind source separation.

\paragraph{Change of variable for  convex sparse blind deconvolution}
We could rewrite the population version of our convex sparse blind deconvolution problem, with the population objective 
$\Expect\frac{1}{N} \| w*Y\|_{\ell_1(\cT)} =\Expect|(w*Y)_0|=\Expect|(w*a*X)_0|$ due to  the ergodic property of stationary process and shift invariance. Then the convex problem becomes 
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|(w*a*X)_0|\\
\mbox{subject to}  
& ((\alpha*a^{-1})*(a*w))_0 =1,
\end{array}
 \]
Let $\psi$ be the flipped version of $a*w$, such that $\tilde{\psi} := a*w$, then 
 $(w*Y)_0 = (w*a*X)_0 = (\tilde{\psi}*X)_0 = \psi^T X.$  
  Let $u:= \alpha*a^{-1}$. 
 Now we arrive at a simple and fundamental  population convex problem: 
 \[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1.
\end{array}
\tag{$P_{u}$ }
  \]
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
In the following, we show that this population convex problem is also the population convex problem of sparse projection pursuit after change of variables.

\paragraph{Sparse projection pursuit and dictionary learning}
Sparse projection pursuit is the problem of finding  one sparse element $d^T Y$ each time from a high dimensional data matrix $Y\in \reals^{n\times M}$. Here $Y= D X$ is a matrix product of dictionary $D\in \reals^{n\times d}$ and sparse coefficient $X\in \reals^{d\times M}$. 


The sparse projection pursuit formulation is to solve the following linear-constrained convex optimization problem for some vector $v$:
\[
 \begin{array}{ll}
 \underset{q }{\mbox{minimize}}   & \frac{1}{M}\|q^T Y\|_{1}\\
\mbox{subject to}  & v^T q =1.
\end{array}
  \]
 
%   In the case of other dictionary $D$, the convolutional dictionary learning problem, also called convolutional sparse coding, could all be solved by  
  
The population version is 
\[
 \begin{array}{ll}
 \underset{d }{\mbox{minimize}}   & \Expect|q^T D X|\\
\mbox{subject to}  & v^T q =1.
\end{array}
  \]
We could also do a change of variable by assuming $\psi:= D^T q$, $u:=D^T q$, then the population sparse projection pursuit also becomes
   \[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  & u^T \psi =1.
\end{array}
\tag{$P_{u}$ }
  \]
Without loss of generality, we could assume $\|u\|_2=1$ by rescaling.
  
  
  
  
  
  
% \paragraph{Ratio of norm formulation for blind deconvolution}
% First, from the paper \cite{donoho1981minimum}, we know that we could minimize the ratio of norm of $X$ to recover $X$.

% For example, \cite{donoho1981minimum,wiggins1978minimum} propose to study $(\ell_{2k}/\ell_2)$ problem for $k=2, 3, 4,\ldots$.
% \begin{eqnarray*}
%     (\ell_{2k}/\ell_2) \qquad  \max&    \frac{1}{N} \| w*Y\|^{2k}_{\ell_{2k}(\cT)}\\
%     \mbox{ subject to }&   \frac{1}{N} \| w*Y\|^2_{\ell_2(\cT)} \geq 1.
% \end{eqnarray*}


% For $\ell_1/\ell_2$ ratio, we propose to use a non-convex (convex objective concave constraint) problem for blind deconvultion:
% \begin{eqnarray*}
%     (\ell_1/\ell_2) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&   \frac{1}{N} \| w*Y\|_{\ell_2(\cT)} \geq 1.
% \end{eqnarray*}

% Another choice is to use infinity norm ball constraint, which allows us to translate it to a convex problem.
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} \geq 1.
% \end{eqnarray*}

% Leverage translation invariance, WLOG, we assume that the $0$-index achieves the maximum in absolute value, then  $  \frac{1}{N} \| w*Y\|_{\ell_\infty(\cT)} =  \frac{1}{N}(w*Y)_0 =  \frac{1}{N}\Tilde Y^T w.$

% Then we have
% \begin{eqnarray*}
%   (\ell_1/\ell_\infty) \qquad  \min&    \frac{1}{N} \| w*Y\|_{\ell_1(\cT)}\\
%     \mbox{ subject to }&    \frac{1}{N}\Tilde Y^T w = 1.
% \end{eqnarray*}


\paragraph{General phase transition for projection pursuit}
Now we state the general phase transition with light assumption. Here we don't need to even assume that $X$ are independent, we just need to know the existence of one sparse element $X_0$.

\begin{theorem}[Projection pursuit to find a sparse element]
Given a sequence $\{X_t\}_{t\in \integers}$ where one element $X_0$ is a sparse element with $p G + (1-p) \delta_0$ for a symmetric distribution $G$.
Let $\psi^\star$ be the solution of  $P_{u}$:
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1
\end{array}
\tag{$P_{u}$ }
  \]
then there exists a threshold
$
p^\star
$,
$\psi^\star = e_0$ provided $p<p^\star$,
and  $\psi^\star \neq e_0$ provided $p> p^\star$.

Here $p^\star$ is determined by $G$, the distribution of $\{X_t, t\neq 0\}$ and the direction of $u$:
  \[
  \frac{p^\star}{1-p^\star} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]\|\beta_{(0)}\|_2} \tan(\angle( \beta, -e_0))
  \]
 where $\beta_{(0)}$ is $\beta$ with the $0-$th entry deleted.
   

  \end{theorem}

\begin{proof}
The phase transition condition proof is based on  calculating the directional derivative.

First, we want to find a threshold $p^\star$ such that for all $p<p^\star$, the directional derivative at $\psi = e_0$ is non-negative along all direction $\beta$ on unit sphere such that $u^T \beta =0$:
	 \[
	 \nabla_{\beta}{\Expect|(e_0+\beta)^T X|}\geq 0
	 \]
Second, we calculate $\nabla_{\beta}{\Expect|(e_0+\beta)^T X|} $ based on whether $X_0$ is zero or not:
	 \[
	 \begin{array}{ll}
	     \nabla_{\beta}{\Expect|(e_0+\beta)^T X|} = p \beta_0 \Expect[|X_{0}| \mid X_0 \neq 0]  + (1-p) \Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]
	 \end{array}
	\]
It is non-negative in case either $\beta_{0} > 0$, or in case $\beta_0 < 0$ and
	\[
	\frac{p}{1-p} < \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]||\beta_0|}
	\]
	for all $\beta \in \{\| \beta\|_2=1, u^T \beta =0\}$.
% 	\item
$p^\star$ is the least upper bound of all $p$ satisfying this inequality. 
Therefore,  
	\[
	\frac{p^\star}{1-p^\star} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]|\beta_0|} =  \inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\Expect[|G|]\|\beta_{(0)}\|_2} \tan(\angle( \beta, -e_0))
	\]
\end{proof}



\paragraph{Special case: geometric phase transition condition for sparse Bernoulli Gaussian $X_0$ and Gaussian $\{X_t, t\neq 0\}$}

Now we study the implication of the general phase transition problem in a simplest projection pursuit case, where $X_t$ are independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ and the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$.

\begin{theorem}
Let $X_t$ be independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$.
Let $\psi^\star$ be the solution of  $P_{u}$:
\[
 \begin{array}{ll}
 \underset{\psi}{\mbox{minimize}}   & \Expect|\psi^T X|\\
\mbox{subject to}  
& u^T \psi =1
\end{array}
\tag{$P_{u}$ }
  \]
then there exists a threshold
$
p^\star
$,
$\psi^\star = e_0$ provided $p<p^\star$,
and  $\psi^\star \neq e_0$ provided $p> p^\star$.

Here $p^\star$ is determined by the direction of $u$:
  \[
  \frac{p^\star}{1-p^\star} = \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0)) = \cot(\angle(u, e_0))
  \]
  \end{theorem}
\begin{proof}
First, when the rest of $X_t, t\neq 0$ is independent of $X_0$, and IID sampled from $ N(0,1),$
	\[
 \frac{\Expect[|X_{(0)}^T \beta_{(0)}| \mid X_0 =0]}{\|\beta_{(0)}\|_2} = 
\sqrt{\frac{2}{\pi}}
\]
Since  
\[
	 \Expect[|G|] = \sqrt{\frac{2}{\pi}},
	 \]
we have a simple phase transition condition that is completely geometric.
	 \[
  \frac{p^\star}{1-p^\star} = \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0))
  \]
 
Second, we know that there is a geometric structure:
\[
\inf_{\| \beta\|_2=1, u^T \beta =0} \frac{\|\beta_{(0)}\|_2}{|\beta_0|}
= \inf_{\| \beta\|_2=1, u^T \beta =0}\tan(\angle( \beta, -e_0)) = \cot(\angle(u, e_0)),
\]
as indicated by figure~\ref{fig-Angle}. 
When $\beta = P_u^\perp (-e_0)$,
	\[
	\begin{array}{ll}
	\inf_{\| \beta\|_2=1, u^T \beta =0} 
		\tan(\angle( \beta, -e_0)) 
		&=
		\tan(\angle( P_u^\perp (-e_0), -e_0)) \\
		&= \cot(\angle(u, e_0)).
	\end{array}
	\]
	
Therefore, $ \frac{p^\star}{1-p^\star}  = \cot(\angle(u, e_0)) $,
	

% \begin{figure} 
% \centering
% \includegraphics[width=.8\textwidth]{./figures_BD/Angle_Diagram_label.png}
% \caption{Demonstration of relation between
%   $\angle( \beta, -e_0)$ and ${\angle(u, e_0)}$}
% \label{fig-Angle}
% \end{figure}
\end{proof}
    
\begin{figure} 
\centering
\includegraphics[width=.8\textwidth]{./figures_BD/Phase_T_sine_p.png}
\caption{The population phase transition diagram of $ \frac{p^\star}{1-p^\star}  = \cot(\angle(u, e_0)) $ for the special case when $X_t$ is independent, $X_0$ is sampled from Bernoulli Gaussian $p N(0,1) +(1-p) \delta_0,$ and the rest $\{X_t, t\neq 0\}$ are sampled from Gaussian $N(0,1)$. The red region is failure, and the blue region is success. }
\label{fig-PT-project}
\end{figure}




==> sec/stability.tex <==
\section{Stability for approximation of infinite length inverse filter}

 
 
 

\paragraph{Reduction}
 \begin{lemma} 
 Let $w^\star \in V_{rs, rt} $ be the solution of the convex optimization problem
 \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  &  \Expect|(w*Y)_0|\\
 \mbox{subject to}  
&  w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
 Then the previous convex optimization problem can be reduced to 
  \[
 \begin{array}{ll}
  \underset{w}{ \mbox{minimize} }  & B(p, \phi) \|\phi \|_2\\
 \mbox{subject to}  
&  \phi = a*w -e_0, \quad w_0 =1, \quad w \in V_{rs, rt}.
\end{array}
  \]
  where
  \[
B(p, \phi) := \frac{\E_I  \| (e_0+\phi)_I \|_2 - \E_I  \| (e_0)_I \|_2}{\|\phi\|_2} 
\]
 \end{lemma} 
  
  
\begin{proof}
Following the previous phase transition analysis, 
let the directional finite difference of the objective at $e_0$ be $D(w) = |(w*Y)_0| - |X_0|$, $I$ be the support of $\tilde{X}$, let $\phi = w*a-e_0$,  then we have 
\[
 \begin{array}{ll}
\Expect D(w) &= \sqrt{\frac{2}{\pi}}\Expect_I [\|(w*a)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]\\
&= \sqrt{\frac{2}{\pi}}\|{\phi}\|_2 B(p, \phi)  \\
\end{array}
  \]
The last inequality comes from the bi-Lipschitz property of $\Expect_I \|(e_0+\phi)_I\|_2$ around $e_0$. 

% Now, we use the \textbf{lower semicontinuous extension}!

% First, $\phi \mapsto \Expect_I [\|(e_0+\phi)_I\|_2 - \|(e_0)_I\|_2]$
% is Lipschitz for $\ell_2$ strong convergence.

% Second $\phi \mapsto \| \phi \|_2$ is Lipschitz for $\ell_2$ convergence.

% Hence we need to use a version of $B(p,\| \phi\|_0)$ that is continuous!
% (Qingyun: add a theorem to quote here!)

% Consider the USC (upper semicontinuous) envelope of $B(p,\| \phi\|_0)$:
% \[
% B^+ := \limsup_{\phi_k -> \phi}   B(p,\| \phi\|_0)
% \]
% where the $\limsup$ is over all sequences that converge to $\phi$.

% If we are dealing with $\phi\in \reals^n$,
% then
% \[
% B^+ =  B(p,n)
% \]

% For any contemplated optimizer $\phi^*$ of $\Expect D$ we can find a
% minor perturbation $\phi^{\epsilon}$ with full support, and with at worst a small
% increase in objective over the limit value!

Now using the optimality of $w^\star$ in $V_{rs, rt}$, for all $w in V_{s,t}, w\neq w^\star$,
we have
 \[
 \begin{array}{ll}
\Expect D(w^\star) \leq \Expect D(w)
\end{array}
  \]
We could directly reduce the problem to 
  \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2 
\end{array}
  \]
\end{proof}   
 
% \textbf{Qingyun: this argumemnt has a gap to the deterministic quantity because $B(p, \phi)$ is dependent on configuration of $\phi$. }

% \textbf{TODO}:

\begin{coro}
If there exists a $\phi$ with $\|{\phi}\|_2<1$ such that \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
 for  $\epsilon> 0$ when $p\leq p^\star(\epsilon)$, then 
  \[
  B(p, \phi) \geq \epsilon.
  \]
  for all $\phi$, 
  then
    \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 \leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  is also bounded.
\end{coro}
\begin{proof}
From
 \[
 \begin{array}{ll}
B(p, \phi^\star) \|{\phi^\star}\|_2 \leq B(p, \phi)\|{\phi}\|_2
\end{array}
  \]
  We have
  \[
 \begin{array}{ll}
\|{\phi^\star}\|_2 
&\leq \frac{B(p, \phi)}{B(p, \phi^\star)}
\|{\phi}\|_2 \\
&\leq \frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
p\Big(\phi_0  +
  \frac{\|{\phi}\|_2}{2} \phi_0^2 
 +
 p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}\|{\phi}\|_2 \\
&\leq \frac{(1-p)\sqrt{p}  + 
p\Big(1  +
  \frac{\|{\phi}\|_2}{2} 
 +
 p\frac{\|{\phi}\|_2}{2}   \Big)}{\epsilon}\|{\phi}\|_2
\end{array}
  \]
  \end{proof}
% Now we want to show that there exists some constant $C$, depending on the worst case directional configuration of $\phi$ and $\phi^\star$,
% \[
% C \geq  \sup_{\phi, \phi^\star}\frac{(1-p)\Big( V_1(\phi_{{(0)}}) \sqrt{1-\phi_0^2}\Big) + 
% p\Big(\phi_0  +
%   \frac{\|{\phi}\|_2}{2} \phi_0^2 
%  +
%  p\frac{\|{\phi}\|_2}{2}  (1-\phi_0^2) \Big)}{(1-p)\Big( V_1(\phi^\star_{{(0)}}) \sqrt{1-(\phi^\star_0)^2}\Big) + 
% p\Big(\frac{1}{\|{\phi^\star}\|_2} (\left| 1 + \|{\phi^\star}\|_2 \phi^\star_0 \right|-1 \Big)}
% \]
% so that
%   \[
%  \begin{array}{ll}
% \|{\phi^\star}\|_2 \leq C \|{\phi}\|_2
% \end{array}
%   \]
  In the following we constructed a filter to give an upper bound on $\|{\phi}\|_2$. 


\paragraph{Setting for finite length approximation}
Now we consider a setting where there is a kernel whose corresponding inverse kernel has infinite support, and we give a finite-length approximation. 

Within the space $V_{-\infty,\infty}$ of bilaterally infinite real-valued sequences $(h(i))_{i \in \integers}$, consider the affine subspace $V_{N_{-}, N_{+}} = \{ (...,0,0,h_{-N_{-}},\ldots, h_{-1}, 1, h_1, h_2, \ldots, h_{N_{+}},0,0,...)\}$, an $N_{-}+N_{+}$-dimensional subspace of bilateral sequences with support at most $N_{-}+N_{+}+1$.
The coordinate that is fixed to one is 
located at index $i=0$.
Each coordinate is zero outside of a window
of size $N_{-}$ on the left of zero 
and  size $N_{+}$ on the right of zero.
The special sequence $e_0 = (\dots,0,0,1,0,0,\dots)$,
vanishing everywhere except the origin,
belongs to $V_{-\infty,\infty}$ and to every
$V_{N_-,N_+}$.

Let $a \in V_{N_-,N_+}$.
Then $a =  (...,0,0,a_{-N_{-}},\ldots, a_{-1}, 1, a_1, a_2, \ldots, a_{N_{+}},0,0,...)$.
We also write $a = e_0 + a_{(0)}$,
where $a_{(0)} \equiv (1-e_0) \cdot a$ 
denotes the `part of $a$ supported away from location
$i=0$'. We also write $a = e_0 + a_L + a_R$,
where $a_L = (a_L(i))_{i \in \integers} 
= (a(i) 1_{\{i < 0\}})_{i \in \integers}$ 
denotes the `part of $a$ supported to
the left of $i=0$' and 
where $a_R = (a_R(i))_{i \in \integers} 
= (a(i) 1_{\{i > 0\}})_{i \in \integers}$
denotes the `part of $a$
supported to the right of $i=0$'.
Finally, we say that $a \in V_{N_{-}, N_{+}}$ 
is a length $ L= N_{-}+N_{+}+1$ filter.

An interesting, if not implementable, objective
function for the blind deconvolution problem
is to minimize
$\Expect [|(w*a*X)_0| - |X_0|] $,
particularly when combined with constraints 
somehow ensuring ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
Defining $\phi \equiv w*a-e_0$, 
\[
 \begin{array}{lll}
\Expect [|(w*a*X)_0| - |X_0|] &=&\Expect [|((e_0 +\phi)*X)_0| - |X_0|].
\end{array}
  \]
  Below we establish the relation
  \[
   \begin{array}{lll}
\Expect [|((e_0 +\phi)*X)_0| - |X_0|] 
&\approx&  C \|{\phi}\|_2 ; \\
\end{array}
\]
This suggests that we should  seek to
minimize $\Expect |(w*Y)_0| $,
while constraining $w$ in some way that
ensures ${\Expect} |(w*a*X)_0|^2 \geq {\Expect}|X_0|^2$.
This  the deterministic objective as 
$$
d_a(w, a^{-1}) :=\|{\phi}\|_2 = \|a*w -e_0 \|_2 =  \|a*(w -a^{-1}) \|_2.
$$

Therefore, we want to construct a finite length approximation of $a^{-1}$ to bound $d_a(w^\star, a^{-1}) = \|a*w -e_0 \|_2$ for the optimal point $w^\star$.








We construct the finite length approximation filter explicitly by truncation of Z-transform.

Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-s}^t a_{i} z^{-i},
\end{array}
  \]
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.






 
\subsection{ Stability for factorized filter}
\subsection{Examples}
In the following, we study the simple case when there is only one root.
Let $s\in (-1,1)$. For $a=(\ldots, 0, 1, -s, 0, \ldots)$, $a^{-1} = (\ldots, 0, 1, s, s^2, s^3, \ldots)$, we could construct 
\[
w^{r,1}:=  (\ldots, 0, 1, s, s^2, s^3, \ldots, s^r)
\]

If we choose this approximation $w^{r,1},$ then
\[
\|a*w^{r,1}-e_0\|_2^2 = \|*_{r+1} (\bar a^{\gamma})\|_2^2 = s^{2(r+1)} 
\]

In the following, we show that this is indeed the best 

For $\gamma\in (0,1]$,
\[
\bar a^{\gamma} :=e_0-\gamma a= (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
\]
\[
 \begin{array}{ll}
w^{r,\gamma} 
&= a^{-1} - a^{-1}*_{r+1} (\bar a^{\gamma})
\end{array}
\]
\[
\begin{array}{ll}
a*(a^{-1}-w^{r,\gamma}) 
&= *_{r+1} (\bar a^{\gamma})\\
&= *_{r+1} (\ldots, 0, 1-\gamma,  \gamma s, 0, \ldots)
% \\
% &= (1-\gamma)^{r+1}*_{r+1} (\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)
\end{array}
\]

\[
\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)](t)  = (1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}, \quad  t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]

\[
|\mathcal{F}[(\ldots, 0, 1-\gamma, \gamma s, 0, \ldots)] |^2(t) = (1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} , \quad t\in T = [\frac{-1}{2}, \frac{1}{2}];
\]
% \[
% \mathcal{F}[(\ldots, 0, 1,  \frac{\gamma}{1-\gamma} s, 0, \ldots)]  = 1+   \frac{\gamma}{1-\gamma} s  \cdot e^{2\pi i  \omega}, \quad  \omega\in T = [\frac{-1}{2}, \frac{1}{2}];
% \]

\[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma})\|_2^2 
&= \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2\\
&=  \int_{\frac{-1}{2}}^\frac{1}{2}  |(1-\gamma)+   \gamma s  \cdot e^{2\pi i  t}|^{2r+2} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt
% \\
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt
\end{array} \]
Notice the following lemma, 
\begin{lemma}
For odd number, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k} 2^{-2k},
\]
\end{lemma}
\begin{proof}
\[
 \begin{array}{ll}
2^n\cos^n (2\pi  t)=(e^{i \cdot 2\pi  t}+e^{-i \cdot 2\pi  t})^n=\sum_{k=0}^n {n\choose k} (e^{i\cdot 2\pi  t})^k\ (e^{-i\cdot 2\pi  t})^{n-k}=\sum_{k=0}^n {n\choose k} e^{(2k-n)i\cdot 2\pi  t},
\end{array} \]

\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} e^{(2k-n)i\cdot 2\pi  t} dt= \delta_{2k-n}
\end{array} \]
\[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2} 2^n\cos^n (2\pi  t) dt =\sum_{k=0}^n {n\choose k} \delta_{2k-n},
\end{array} \]
therefore, for odd number $n=2k-1$, $\int_{\frac{-1}{2}}^\frac{1}{2}  \cos^{2k-1}{(2\pi  t)}  dt = 0$ for any $k\in \integers_+$; for even number $n=2k$, 
\[
\int_{\frac{-1}{2}}^\frac{1}{2} 2^{2k} \cos^{2k}{(2\pi  t)}  dt =  {2k\choose k}.
\]
\end{proof}

\begin{lemma}
Now
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := (1-\gamma) \gamma s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
=\sum_{k=0}^{\frac{r+1}{2}} [(1-\gamma)^2+ (\gamma s )^2]^{r+1-2k} [ (1-\gamma) \gamma s]^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{lemma}
\begin{proof}
Now define
$R_1 :=  (1-\gamma)^2+ (\gamma s )^2,$
$R_2 := {(1-\gamma)} {\gamma}s,$
\[
 \begin{array}{ll}
 \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2
&= \int_{\frac{-1}{2}}^\frac{1}{2}  [(1-\gamma)^2+ (\gamma s )^2+ 2 {(1-\gamma)} {\gamma}s \cos{(2\pi  t)} ]^{r+1} dt\\
&= \int_{\frac{-1}{2}}^\frac{1}{2}  
[R_1+ R_2 \cdot 2 \cos{(2\pi  t)} ]^{r+1} dt\\
&=\sum_{k=0}^{\frac{r+1}{2}} R_1^{r+1-2k} R_2^{2k}{2k\choose k}{r+1\choose 2k} 
\end{array} \]
\end{proof}
% Therefore,
% \[
%  \begin{array}{ll}
% \| (\hat{\bar a}^{\gamma})^{r+1}\|_2^2 
% &= (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}\int_{\frac{-1}{2}}^\frac{1}{2}  
% [1+ R \cos{(2\pi  t)} ]^{r+1} dt\\
% &=  (1-\gamma)^{2r+2} (1+ (\frac{\gamma}{1-\gamma} s)^2)^{r+1}
% \sum_{k=0}^{\frac{r+1}{2}} (R/2)^{2k} {r+1\choose 2k}  {2k\choose k}\\
% &= 
% \sum_{k=0}^{\frac{r+1}{2}} [s\gamma]^{2k} [(1-\gamma)^2+(s\gamma)^2]^{r+1-2k} {r+1\choose 2k}  {2k\choose k}
% \end{array} \]

% Since 
% \[
% \lim_{r\rightarrow \infty} \||\hat{\bar a}^{\gamma}|^2\|_{r+1} = \||\hat{\bar a}^{\gamma}|^2\|_\infty ,
% \]
Use the Laplace's method theorem 
% \ref{Laplace},
We could instead directly optimize  $\gamma$ over the $\ell_\infty$ norm of $|\hat{\bar a}^{\gamma}|^2$,
\begin{lemma}
\[
 \||\hat{\bar a}^{\gamma}|^2\|_\infty = \max_{ t\in [\frac{-1}{2}, \frac{1}{2}]}\{ (1-\gamma)^2 + (\gamma s)^2+ 2 (1-\gamma) \gamma s \cos{(2\pi  t)} \}  = (1-\gamma)^2 + (\gamma s)^2+ 2 |(1-\gamma) \gamma s| = (|1-\gamma|+|\gamma s|)^2 
\]
then

 \[
  \begin{array}{ll}
\gamma_\infty &= \arg\min_{\gamma>0}\||\hat{\bar a}^{\gamma}|^2\|_\infty \\
&= \arg\min_{\gamma>0}(|1-\gamma|+|\gamma s|)^2 \\
&= 1
 \end{array} \]
\[
\min_{\gamma\in (0,1)}\||\hat{\bar a}^{\gamma}|^2\|_\infty
= (|1-\gamma_\infty|+|\gamma_\infty s|)^2 
= |s|^2
\]
\end{lemma}
And
 \[
 \begin{array}{ll}
\|*_{r+1} (\bar a^{\gamma_\infty  })\|_2^2 
% &=  s^{2r+2} \sum_{k=0}^{\frac{r+1}{2}}   {r+1\choose 2k}  {2k\choose k}\\
&=  s^{2r+2} 
\end{array} \]

% If we instead choose $\gamma_2$ as $ \cos^2{\theta} = \frac{1}{1+s^2}$ to minimize the $\ell_2$ norm instead, then
% \[
% \|\hat{\bar a}^{\gamma_2}\|_2^2  = \min_{\gamma\in (0,1)}\|\hat{\bar a}^{\gamma}\|_2^2 
% =  (1-\gamma_2)^2 + (\gamma_2 s)^2 
% = \frac{s^2}{1+s^2}
% \]
% And in this case,
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty
% &= (|1- \frac{1}{1+s^2}|+| \frac{1}{1+s^2} s|)^2 \\
% &=  s^2 (\frac{1+|s|}{1+s^2})^2 \in (s^2, 1)
%  \end{array} \]
 
%  Therefore, 
%  \[
%   \begin{array}{ll}
% \||\hat{\bar a}^{\gamma_2}|^2\|_\infty \in (s^2, 1)
%  \end{array} \]


\paragraph{Finite length approximation constructing using Z-transform truncation on factorization form }
Let the Z-transform of $a$ be 
\[
 \begin{array}{ll}
A(z) =  \sum_{i=-N_{-}}^{N_{+}} a_{i} z^{-i},
\end{array}
  \]
We can factorize the Z-transform as product of factors with roots $s_{-j}$ for $j = 1, \ldots N_{-}$ and  $i = 1, \ldots N_{+}.$
\[
 \begin{array}{ll}
A(z) =  c_0\prod_{j=1}^{N_{-}} (1- s_{-j} z) \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1}),
\end{array}
  \]
  Where $c_0$ is a constant to make sure that the coefficient $a_0=1$.
  
 We assume that $|s_k|<1,$ for any $k = -N_{-}, \ldots , N_+.$  
  
Then Z-transform of the inverse kernel $a^{-1}$ is $1/A(z)$.
\[
 \begin{array}{ll}
1/A(z) &=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}} (1- s_{i} z^{-1})^{-1}\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{\infty} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{\infty} s^{\ell_i}_{i} z^{\ell_i} )
\end{array}
  \]

From previous single root study, we get a hint to study a single truncation of length $ 1 + \sum_{j=1}^{N_{-}} r_{-j}  +  \sum_{j=1}^{N_{+}}  r_i$,  we construct
\[
 \begin{array}{ll}
W(z) 
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (\sum_{\ell_j=0}^{r_{-j}} s^{\ell_j}_{-j} z^{-\ell_j} ) \prod_{i=1}^{N_{+}} (\sum_{\ell_i=0}^{r_{-j}} s^{\ell_i}_{i} z^{\ell_i} )\\
&=  \frac{1}{c_0}\prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1})(1- s_{-j} z)^{-1} \prod_{i=1}^{N_{+}}(1- (s_{i}  z^{-1})^{r_i+1}) (1- s_{i} z^{-1})^{-1}
\end{array}
  \]
Let the corresponding filter being $w$.
  
  
Now let $\psi =  a*w$ with Z-transform $\Psi(z)$, $\phi = a*w-e_0$ with Z-transform $\Phi(z)$,we have
\[
 \begin{array}{ll}
\Psi(z): = A(z)W(z) 
&=   \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) 
\end{array}
  \]
  therefore,
\[
 \begin{array}{ll}
\Phi(z): = A(z)W(z) -1 
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{r_{-j}+1}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{r_i+1}) -1
\end{array}
  \]
\paragraph{Upper Bound on  $\|\phi\|_2^2$ for constructed finite length approximation}
In the following,  we want to give upper bound for
  \[
\|a*w -e_0\|_2^2 =\|\phi\|_2^2 
 \]  
  
Redefine the index $\tau_{-j} := r_{-j}+1; \tau_{i} = r_i+1.$
Let $\cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$ as the set of all the possible index.
And we define polar representation of complex roots:
for any $k \in \cI = \{-N_{-},\ldots, -1, 1, \ldots, N_{+} \}$
\[
s_{k} := |s_{k}| e^{i \varphi_k } = e^{\rho_k + i \varphi_k }
\]
where 
\[
 \begin{array}{ll}
\varphi_k := \operatorname{Im}(\log( s_{k} )) = -i \log(\frac{s_{k}}{|s_{k}|}) 
\end{array}
\]
and since $|s_{k}|<1$ we have 
\[
\rho_k = -\operatorname{Re}(\log( s_{k} ))>0
\]

Now we consider all $z = e^{2 \pi i t}$ on the unit circle for $t\in [\frac{-1}{2},\frac{1}{2}]$,
then for any $k \in \cI$
\[
 \begin{array}{ll}
- (s_{k} z^{-\mbox{sign}(k)})^{\tau_{k}} 
&= - |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\\
&=   \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) 
\end{array}
  \]
 Now we simplify the notation by defining 
 \[
 \upsilon_k(t) :=\tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi
 \]
then
 \[
 \begin{array}{ll}
\Phi(z)
&=  \prod_{j=1}^{N_{-}} (1- (s_{-j} z)^{\tau_{-j}}) \prod_{i=1}^{N_{+}}(1- (s_{i} z^{-1})^{\tau_{i}}) -1\\
&=  \prod_{k \in \cI} \Big(1- |s_{k}|^{\tau_{k}} \exp \big(i [\varphi_k-  2 \pi t \mbox{sign}(k)]\cdot \tau_{k} \big)\Big)  -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \big( \tau_{k} (\varphi_k- 2 \pi t \mbox{sign}(k) ) + \pi  \big) \Big) \bigg)     -1\\
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1
\end{array}
  \]
  
\begin{lemma}
 For any $z = \exp{(2 \pi i t )}$ on the unit circle,
 \[
 \begin{array}{ll}
\Phi\big(\exp{(2 \pi i t )}\big)
&=  \prod_{k \in \cI} \bigg( 1+ \exp \Big( \tau_{k} \rho_k+ i \cdot \upsilon_k(t) \Big) \bigg)     -1\\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big)
+ i \cdot \big( \upsilon_{k_1}(t) + \ldots+  \upsilon_{k_n}(t)  \big) \Big)  
\end{array}
  \]
 \end{lemma}
 
 \begin{lemma}
Additionally, for any $t \in [\frac{-1}{2},\frac{1}{2}]$,
\[
 \begin{array}{ll}
 |\Phi\big(\exp{(2 \pi i t )}\big)|^2  
= 
\sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
is independent of $t$, since the oscillation integral over the imaginary part is 
  \[
 \begin{array}{ll}
\int_{\frac{-1}{2}}^\frac{1}{2}
\exp  \bigg( i \cdot \Big(  \big(\upsilon_{k_1}(t) - \upsilon_{k_1}(t) \big) + \ldots+  \big(\upsilon_{k_n}(t) -\upsilon_{k_n}(-t)\big)  \Big) \bigg)  dt
= 1
\end{array}
  \]
Therefore, using Fourier isometry,
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 &= \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi\big(\exp{(2 \pi i t )}\big)|^2 dt \\
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big)   
\end{array}
  \]
  
 \end{lemma}

\begin{theorem}
\label{thm: Root_2_norm}
Since $|s_{k}|<1$, i.e. $\rho_{k}<0$ for all $k\in \cI$.
 \[
 \begin{array}{ll}
 \|\phi\|_2^2 
&= \sum_{n=1}^{|\cI|}\sum_{ k_1, \ldots, k_n  \in \cI } 
\exp \Big( 2 \big(\tau_{k_1} \rho_{k_1}+ \ldots+  \tau_{k_n} \rho_{k_n} \big) \Big) 
\end{array}
  \]
  Let $\gamma^m := \min_{i}\big(\tau_{i} |\rho_{i}| \big) =  \min\{\tau_{-N_-}|\rho_{-N_-}|, \ldots, \tau_{-1}|\rho_{-1}|, \tau_{1}|\rho_{1}|, \ldots, \tau_{N_+}|\rho_{N_+}|\}.$
When $\gamma^m \rightarrow \infty$, we have a finite sum of exponential rate  converging terms: the convergence rate is determined by the exponential term as a function of $\gamma^m$.
   \[
 \begin{array}{ll}
 \|\phi\|_2^2 
=    O(\exp \Big( -2 \min_{i}\big(\tau_{i} |\rho_{i}| \big) \Big))
= O(\exp \Big( -2 \gamma^m  \big) \Big))
\rightarrow 0
\end{array}
  \]

 \end{theorem}

 
% \begin{proof}
% Using the expansion, for $Z = \exp{(2 \pi i t )},$ then 
% \[
%  \left|(-1)^n( \prod_{j=1}^n \frac{s_{\ell_j}}{|s_{\ell_j}|}  (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })\right| = 1
% \]
% therefore, for any $t\in [\frac{-1}{2},\frac{1}{2} ]$ 
%  \[
%  \begin{array}{ll}
% \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|
% % &= |\sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % [(-1)^n( \sign[ \prod_{j=1}^n s_{\ell_j}] (\exp{-(r_\ell+1)(\ell_1+ \ldots+ \ell_n)(2 \pi i t })]|\\
% &\leq \sum_{n=1}^{|\cI|}\sum_{ \ell_1, \ldots,\ell_n  \in \cI } (|s_{\ell_1}|\cdot \ldots \cdot |s_{\ell_n}|)^{r_\ell+1} 
% % \\
% % &= \prod_{\ell \in \cI} (1+ |s_{\ell}|^{r_\ell+1})-1 
% \end{array}
%   \]
% Therefore, from 
% \[
%  \begin{array}{ll}
% & \|\phi\|_2^2\\
%  =& \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt \\
%   \leq & \max_{t\in [\frac{-1}{2},\frac{1}{2} ]}|\Phi(\exp{(2 \pi i t )})|^2
% \end{array} \]
% we conclude the proof.




%  \[
%  \begin{array}{ll}
% S_{-j}(t) &:= \log(s_{-j} \exp{(2 \pi i t )}) \\
% &= \log(|s_{-j}|)+ i (\pi 1_{s_{-j}<0}+ 2 \pi  t)\\
% S_{i}(t) &:= \log(s_{i} \exp{(-2 \pi i t )})] \\
% &= \log(|s_{i}|)+ i ( \pi 1_{s_{i}<0}+ 2 \pi  t)
% \end{array} \]
% % \[
% %  \begin{array}{ll}
% % R_{+}^{j, r_{-j}}(t) &:= (s_{-j} \exp{(2 \pi i t )})^{r_{-j}+1} \\
% % &= \exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\}\\
% % R_{-}^{i, r_i}(t) &:= (s_{i} \exp{(-2 \pi i t )})^{r_i+1} \\
% % &= \exp\left\{(r_{-j}+1)S_{i}(t) \right\}
% % \end{array} \]
% % and let
% % \[
% %  \begin{array}{ll}
% % Q_{+}^{j, r_{-j}}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{-j}(t)  \right\} )\\
% % Q_{-}^{i, r_i}(t) &:=  \log( 1-\exp\left\{ (r_{-j}+1)S_{i}(t)  \right\} )
% % \end{array} \]

% \[
%  \begin{array}{ll}
%   \Psi(\exp{(2 \pi i t )})
% % &= \gamma \prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t))\\
% % &= \gamma \exp\{ \sum_{j=1}^{N_{-}} Q_{+}^{j, r_{-j}}(t) + \sum_{i=1}^{N_{+}} Q_{-}^{i, r_i}(t)  \}  \\
% &=  \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &=  \int_{\frac{-1}{2}}^\frac{1}{2}  |\Psi(\exp{(2 \pi i t )}) -1|^{2} dt\\
% &= \int_{\frac{-1}{2}}^\frac{1}{2}  | \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
% \end{array} \]
% Consider the case when all the $r_\ell$ are the same as $r,$ and $r\rightarrow \infty$.
% % From the fact that for $x\leq 0,$
% % \[\log( 1-\exp(-x)) = -x + \log(\exp(x) -1)\]
% % and the Laplace's method, 
% we know that to compute
% $\int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt,$
% We only need to compute the maximum value of $\sum_{ \ell \in \cI } S_{\ell}(t)$.
% The maximum value is gonna be $\sum_{ \ell \in \cI } \log(|s_{\ell}|)$, and it is achieved at either $t_0 = 0$, or $t_0 = 1,$ depending on the sum of all the $\sum_{ \ell \in \cI } 1_{s_{\ell}<0}$ is odd or even.

% Therefore, 
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2}  |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)S_{\ell}(t)  \right\} )  \right\} -1|^{2} dt\\ 
%   \leq&    |\gamma \exp\left\{ \sum_{ \ell \in \cI } \log( 1-\exp\left\{ (r_\ell+1)\log(|s_{\ell}|  \right\} )  \right\} -1|^{2} 
% \end{array} \]
% \[
%  \begin{array}{ll}
%   \int_{\frac{-1}{2}}^\frac{1}{2} |\Phi(\exp{(2 \pi i t )})|^2 dt 
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\
% &= \gamma^2  \int_{\frac{-1}{2}}^\frac{1}{2}  |\prod_{j=1}^{N_{-}} (1- R_{+}^{j, r_{-j}}(t)) \prod_{i=1}^{N_{+}}(1- R_{-}^{i, r_i}(t)) -\frac{1}{\gamma}|^{2} dt\\ 
% \end{array} \]
% \end{proof}
